Your Policy Regularizer is Secretly an Adversary

Policy regularization methods such as maximum entropy regularization are widely used in reinforcement learning to improve the robustness of a learned policy. In this paper, we show how this robustness arises from hedging against worst-case perturbations of the reward function, which are chosen from a limited set by an imagined adversary. Using convex duality, we characterize this robust set of adversarial reward perturbations under KL and alpha-divergence regularization, which includes Shannon and Tsallis entropy regularization as special cases. Importantly, generalization guarantees can be given within this robust set. We provide detailed discussion of the worst-case reward perturbations, and present intuitive empirical examples to illustrate this robustness and its relationship with generalization. Finally, we discuss how our analysis complements and extends previous results on adversarial reward robustness and path consistency optimality conditions.

==> Reward Robustness TMLR (3)/macros.tex <==
\newcommand{\omitindices}{}

\newtheorem{observation}{Observation}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}


\newcommand{\revhl}[1]{\textcolor{Black}{#1}}
\newcommand{\shiehl}{red}
% \newcommand{\revhl}[1]{\textcolor{DarkGreen}{#1}}

\newcommand{\RB}[1]{{\color{red}{RB: #1}}}
\newcommand{\TG}[1]{{\color{purple}{TG: #1}}}
\newcommand{\PO}[1]{{\color{red}{PO: #1}}}
\newcommand{\JG}[1]{{\color{red}{JG: #1}}}
\newcommand{\GD}[1]{{\color{red}{GD: #1}}}
\newcommand{\MK}[1]{{\color{red}{MK: #1}}}


\usepackage{pifont}
\newcommand{\header}{-.22cm}
\newcommand{\headerv}{\vspace*{-.175cm}}
%\newcommand{\0}{t_0}
%\newcommand{\0}{t}%{\0}
\newcommand{\past}{\underline{as}_{<\0}, s_t}
\newcommand{\leqt}{{\leq \0}}
\newcommand{\inner}[2]{{\langle {#1} , {#2} \rangle }}
\newcommand{\mudomain}{\mathcal{M}}%_{\gamma,p}

\newcommand{\taunotation}{\tau(\pi)}%{p_{\pi}(\tau)}% 
\newcommand{\rprimedomain}{\mathbb{R}^{\mathcal{A} \times \mathcal{S} } }%_{\gamma,p}
\newcommand{\rprimedomainconj}{\mathbb{R}^{\mathcal{X}} }
\newcommand{\mudomainfn}{\mathbb{R}_+^{\mathcal{A} \times \mathcal{S}}}
\newcommand{\mudomainconj}{\mathbb{R}_+^{\mathcal{X}}}

\newcommand{\tick}{^{\prime}}
\newcommand{\obj}{\mathcal{RL}}
\newcommand{\primalvar}{\mu}
\newcommand{\dualvar}{\Delta r}
% {r\tick}
\newcommand{\pir}{\pi_{\pr}}
\newcommand{\mur}{\mu_{\pr}}
\newcommand{\modifyr}{r\tick}
\newcommand{\perturbr}{\Delta r}
\newcommand{\modifiedr}{\modifyr}
\newcommand{\mr}{\modifyr}
\newcommand{\pr}{\perturbr}
\newcommand{\propt}{\prpi}
\newcommand{\mropt}{\mr_{\pi}}
% {\modifyr_*}
% \perturbr_*}

\newcommand{\prnew}{\Delta \tilde{r}}
\newcommand{\lambdaplus}{\lambda(a,s)}
\newcommand{\lambdaopt}{\lambda_*(a,s)}
\newcommand{\lambdazero}{\lambdaplus}
\newcommand{\mroptpi}{\mr_{\pi_*}}
\newcommand{\proptpi}{\pr_{\pi_*}}
\newcommand{\mrpiopt}{\mr_{\pi_*}}
\newcommand{\proptv}{\pr_{V_*}}
\newcommand{\prpi}{\pr_{\pi}}
\newcommand{\prpiopt}{\pr_{\pi_*}}
\newcommand{\prv}{\pr_{V}}
\newcommand{\prmu}{\pr_{\mu}}
\newcommand{\prrobust}{\pr} %\prpi
\newcommand{\prinit}{\pr} %\prpi # First part of Sec 3
\newcommand{\prrob}{\prrobust} %\prpi
\newcommand{\mrv}{\mr_{V}}
\newcommand{\mrvopt}{\mr_{V_*}}
\newcommand{\mrrobust}{r_*\tick}
\newcommand{\piopt}{\pi_*}
\newcommand{\tpiopt}{\tpi_*}
\newcommand{\normmu}{\psi_{\mu}}
\newcommand{\vpi}{V_{\pi}(s)}
\newcommand{\bullets}[1]{{#1}}

\newcommand{\variable}{a}
\newcommand{\vz}{\variable}
\newcommand{\highlight}{blue}
\newcommand{\lagr}{\mathcal{L}}
\newcommand{\concaveopt}{\mathcal{R}}
\newcommand{\normalizerexp}{\psi(s;\beta)}
\newcommand{\normalizeralpha}{\psi_{\alpha}(s;\beta)}
\newcommand{\normalizerpr}{\psi_{\alpha}(\pr, s;\beta)}
\newcommand{\normalizerexppi}{\psi_{\pi}(s;\beta)}
\newcommand{\normalizerexppistar}{\psi_{\pi_*}(s;\beta)}
\newcommand{\densityfnspace}{\mathcal{F}_{+}}
\newcommand{\densityfnspacea}{\densityfnspace^{|\mathcal{A}|}}
\newcommand{\fnspace}{\mathcal{F}}
\newcommand{\dualdomain}{ \mathcal{D}^*} % \mathbb{R}^{|\mathcal{A}|}}
\newcommand{\simplex}{\Delta^{|\mathcal{A}|}}
\newcommand{\feasibleset}{\mathcal{R}_{\pi}}
\newcommand{\discussiondual}{Q}
\newcommand{\myconst}{\psi_{\pr}(s;\beta)}%{(1-\alpha) D_{\alpha}[\pi_0:\pi]}
\newcommand{\psipi}{\myconst}%\psi_{\pi}(s;\beta)}
\newcommand{\psipr}{\psi_{\pr}(s;\beta)}
\newcommand{\psipiopt}{\psi_{\pr_{\pi_*}}(s;\beta)}
\newcommand{\psipropt}{\psi_{\pr_{\pi_*}}(s;\beta)}
\newcommand{\psiq}{\psi_{Q}(s;\beta)}
\newcommand{\psipiq}{\psiq}
\newcommand{\psiqopt}{\psi_{{Q_*}}(s;\beta)}
% \newcommand{\psipi}{\psi_{\pi}(s;\beta)}
% \newcommand{\psipiq}{\psi_{\pi_Q}(s;\beta)}
% \newcommand{\psipiqopt}{\psi_{\pi_{Q_*}}(s;\beta)}
\newcommand{\mydiv}[1]{(1-\alpha) D_{\alpha}[\pi_0:#1]}
\newcommand{\myconstopt}{\mydiv[\piopt]}
% (1-\alpha) D_{\alpha}[\pi_0:\pi_*]}

\newcommand{\alphaconjn}{\frac{1}{\beta}\Omega^{*(\alpha)}_{\pi_0, \beta}}
% \newcommand{\alphaconjnnnew}{\frac{1}{\beta}\Omega^{*(\alpha)}_{\pi_0, \beta, \pi}}
\newcommand{\alphaconjmu}{\frac{1}{\beta}\Omega^{*(\alpha)}_{\pi_0, \beta}}
% \newcommand{\alphaconjmunew}{\frac{1}{\beta}\Omega^{*(\alpha)}_{\pi_0, \beta, \mu}}
\newcommand{\alphaconju}{\frac{1}{\beta}\Omega^{*(\alpha)}_{\tpi_0, \beta}}
\newcommand{\alphaconj}{\frac{1}{\beta}\Omega^{*(\alpha)}_{\pi_0, \beta}}
\newcommand{\alphaconjm}{\frac{1}{\beta}\Omega^{*(\alpha)}_{\mu_0, \beta}}
\newcommand{\alphan}{\frac{1}{\beta}\Omega^{(\alpha)}_{\pi_0}(\pi)}
\newcommand{\omegamu}{\frac{1}{\beta}\Omega^{(\alpha)}_{\pi_0}(\mu)}
\newcommand{\alphaomegamu}{\frac{1}{\beta}\Omega^{(\alpha)}_{\mu_0}(\mu)}
\newcommand{\alphaomegapi}{\frac{1}{\beta}\Omega^{(\alpha)}_{\pi_0}(\mu)}
\newcommand{\omegapi}{\frac{1}{\beta}\Omega^{(\alpha)}_{\pi_0}(\pi)}
\newcommand{\omegapiopt}{\frac{1}{\beta}\Omega^{(\alpha)}_{\pi_0}(\piopt)}
\newcommand{\omegatpi}{\frac{1}{\beta}\Omega^{(\alpha)}_{\pi_0}(\tpi)}
\newcommand{\klconjmuu}{\frac{1}{\beta}\Omega^{*}_{\mu_0, \beta}}
\newcommand{\klconjpii}{\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}}
\newcommand{\klconjmu}{\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta, \mu}}
\newcommand{\klconjpi}{\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta, \pi}}
\newcommand{\klomegamu}{\frac{1}{\beta}\Omega^{}_{\pi_0}(\mu)}
\newcommand{\klomegapi}{\frac{1}{\beta}\Omega^{}_{\pi_0}(\pi)}
\newcommand{\klomegatpi}{\frac{1}{\beta}\Omega^{}_{\pi_0}(\tpi)}

\newcommand{\rklconjmu}{\frac{1}{\beta}\Omega^{*(0)}_{\pi_0, \beta, \mu}}
\newcommand{\rklconjpi}{\frac{1}{\beta}\Omega^{*(0)}_{\pi_0, \beta, \pi}}
\newcommand{\rklomegamu}{\frac{1}{\beta}\Omega^{(0)}_{\pi_0}(\mu)}
\newcommand{\rklomegapi}{\frac{1}{\beta}\Omega^{(0)}_{\pi_0}(\pi)}
\newcommand{\rklomegatpi}{\frac{1}{\beta}\Omega^{(0)}_{\pi_0}(\tpi)}


\newcommand{\alphanmu}{\omegamu}
\newcommand{\alphau}{\frac{1}{\beta}\Omega^{(\alpha)}_{\tpi_0}(\tpi)}
\newcommand{\alphanorm}{\normalizeralpha}



\newcommand{\normof}[1]{\psi_{\alpha}\big( #1(a,s); \beta \big)}
\newcommand{\alphanormof}[1]{\psi_{\alpha}\big( #1 (a,s); \beta \big) }


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\tcminus}[1]{\textcolor{FireBrick}{#1}}
\newcommand{\tclink}[1]{\textcolor{blue}{#1}}
\newcommand{\tcplus}[1]{\textcolor{DarkGreen}{#1}} %SeaGreen

\newcommand{\tp}{\tilde{\pi}}
\newcommand{\tpi}{\tilde{\pi}}
\newcommand{\tpo}{\tilde{\pi}_0}
\newcommand{\ptReg}{\dot{\Omega}}
\newcommand{\ptConj}{\dot{\Omega}^{*}}
\newcommand{\opt}{{\pi^{*}_{\textsc{mdp}}}}
%\newcommand{\opt}{\textcolor{red}{\pi_{Q^*}}}

\newcommand{\mysec}[1]{\hyperref[sec:#1]{Sec.~\ref*{sec:#1}}}
\newcommand{\myfig}[1]{\hyperref[fig:#1]{Fig.~\ref*{fig:#1}}}
\newcommand{\myapp}[1]{\hyperref[app:#1]{App.~\ref*{app:#1}}}
\newcommand{\myprop}[1]{\hyperref[prop:#1]{Prop.~\ref*{prop:#1}}}
\newcommand{\mythm}[1]{\hyperref[thm:#1]{Thm.~\ref*{thm:#1}}}
\newcommand{\mylem}[1]{\hyperref[lemma:#1]{Lemma~\ref*{lemma:#1}}}
\newcommand{\mylemma}[1]{\hyperref[lemma:#1]{Lemma~\ref*{lemma:#1}}}
\newcommand{\mycor}[1]{\hyperref[cor:#1]{Cor.~\ref*{cor:#1}}}
\newcommand{\mytab}[1]{\hyperref[table:#1]{Table~\ref*{table:#1}}}
\newcommand{\expof}[1]{ \exp \big\{ {#1} \big\} }
\newcommand{\of}[1]{\big\{ #1 \big\}}
\newcommand{\brangle}{\big \rangle}
\newcommand{\blangle}{\big \langle}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

%\newcommand{\transitionv}{{P^{s\tick}_{a,s}  V(s\tick)}}
\newcommand{\transitionv}{{\mathbb{E}^{s\tick}_{a,s} \big[ V(s\tick) \big] }}
\newcommand{\transitionvstar}{{\mathbb{E}^{s\tick}_{a,s} \big[ V_*(s\tick) \big] }}
\newcommand{\transitionvinds}{{\mathbb{E}^{s\tick}_{a,s} \big[ V \big] }}
\newcommand{\transitionvstarinds}{{\mathbb{E}^{s\tick}_{a,s} \big[ V_* \big] }}
\newcommand{\transitionvpi}{{\mathbb{E}^{s\tick}_{a,s} \big[ V_{\pi}(s\tick) \big] }}
\newcommand{\transitioninline}{\transitionv}
%\newcommand{\transitionv}{{\sum \limits_{s\tick} P(s\tick|a,s)  V(s\tick)}}
%\newcommand{\discountedvalue}{\gamma \int P(s\tick |s,a) V(s\tick) ds\tick}
%\newcommand{\transitioninline}{{\sum_{s\tick} P(s\tick|a,s)  V(s\tick)}}

\newcommand{\transitiontransp}{{\sum \limits_{a\tick, s\tick}P(s|a\tick,s\tick)}}

\usepackage[acronym,smallcaps,nowarn,section,nogroupskip,nonumberlist]{glossaries}
\glsdisablehyper
\newacronym{VI}{vi}{variational inference}
\newacronym{GVI}{gvi}{generalized variational inference}
\newacronym{MDP}{mdp}{Markov Decision Processes}
\newacronym{KL}{kl}{Kullback-Leibler}
\newcommand{\kl}{\textsc{kl} }
\newcommand{\KL}{D_{\textsc{KL}}}
\newacronym{LP}{lp}{linear programming}
\newacronym{RL}{rl}{reinforcement learning}
\newacronym{REPS}{reps}{Relative Entropy Policy Search}

\newcommand{\rulesep}{\unskip\ \vrule\ }

% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}[theorem]{Corollary}

% \newcommand{\fix}{\marginpar{FIX}}
% \newcommand{\new}{\marginpar{NEW}}
\newcommand{\nocontentsline}[3]{}
\newcommand{\tocless}[2]{\bgroup\let\addcontentsline=\nocontentsline#1{#2}\egroup}

==> Reward Robustness TMLR (3)/old/0_intro.tex <==
\section{Introduction}\label{sec:intro}
%\TG{Not very urgent, but I think the title of the paper can be improved - ideally it's catchy and summarizes the main finding/message of the paper. E.g. ``Meta-trained agents implement Bayes-optimal agents'' was a winner :)}
% While \gls{RL} algorithms have achieved remarkable success in challenging domains \citep{mnih2015human,silver2016mastering}, questions of optimization, exploration, and safe generalization remain activate areas of research.   
Regularization plays a crucial role in various settings across \gls{RL}, such as trust-region methods \citep{peters2010relative, schulman2015trust, schulman2017proximal, basserrano2021logistic}, offline learning \citep{levine2020offline, nachum2019dualdice, nachum2019algaedice, nachum2020reinforcement}, multi-task learning \citep{teh2017distral, galashov2020importance}, and soft 
$Q$-learning or actor-critic methods
% actor-critic methods 
\citep{fox2016taming, nachum2017bridging, haarnoja17a, haarnoja2018soft, grau2018soft}. 
% \textcolor{red}{SAC? Soft Q?}
%with stochastic policies 
Various justifications have been given for policy regularization, %the benefits of
such as improved optimization \citep{ahmed2019understanding},  
% implicit averaging of $Q$-values, \citep{viellard},
connections with probabilistic inference \citep{levine2018reinforcement, galashov2018information}, 
 %with purported benefits including X, Y, Z , 
 and robustness to perturbations in environment rewards or dynamics \citep{eysenbach2021maximum, husain2021regularized}.
%  The latter benefits may be particularly relevant for safety considerations \citep{amodei2016concrete, everitt2018agi}, where we are interested in agents which can generalize or adapt to new environments or distribution shift.
The latter 
is crucial in \textsc{ai} safety, where
% plays a crucial role in \textsc{ai} safety, where 
a primary goal
% the goal 
is to design agents that generalize and adapt safely to new situations or distributional shift.
% \citep{amodei2016concrete, everitt2018agi}.

% In this work, we provide a unified discussion of several recent works that interpret policy regularization as providing robustness to perturbations in the environmental rewards \TG{Suggestion: ``In this work we theoretically analyze the robustness-properties that arise form policy regularization in RL.'' Then skip to the next sentence (For a policy...) and mention the unified view later.} \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}.

In this work, we analyze the robustness properties which arise from policy regularization in \gls{RL}.
For a policy $\pi(a|s)$ regularized using a convex function $\Omega(\pi) = \mathbb{E}_{\pi}[\ptReg(\pi)]$ such as a statistical divergence, we investigate statements of the form %\citep{eysenbach2021maximum}
\begin{align}
\hspace*{-.2cm} &\max \limits_{\pi(a|s)} (1-\gamma) \mathbb{E}_{\tau \sim p^{\pi}(\tau)} \left[ \sum \limits_{t=0}^\infty \gamma^t \bigg( r(a_t, s_t) - \ptReg \big(\pi(a_t | s_t)\big) \bigg) \right] \nonumber \\
&= \max \limits_{\pi(a|s)} \min \limits_{r\tick(a,s) \in \feasibleset}  \mathbb{E}_{\tau \sim p^{\pi}(\tau)} \left[ \sum \limits_{t=0}^\infty \gamma^t \, r\tick(a_t,s_t) \right]
\label{eq:reward_perturbation_stmt}
\end{align}
where $r\tick(a,s)$ is the worst-case reward function chosen from an appropriate feasible set $\feasibleset$. %which depends on the policy $\pi$.
This robustness is intriguing, as it suggests regularized policies achieve a form of `zero-shot' generalization to new environments where the reward has been adversarially chosen. %of a policy

Using tools from convex duality, we provide a precise characterization of this reward robustness,
%which leads to a game-theoretic interpretation of soft value aggregation as hedging against adversarial perturbations which tend to equalize the reward function across actions in a particular state \citep{ortega2014adversarial}.
%and provide a unified discussion of several recent works that explore similar interpretations \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}
We find that the optimal modified reward $r_{*}\tick$ in \cref{eq:reward_perturbation_stmt} re-expresses the value of the objective for a given policy, which places restrictions on the set $\mathcal{R}$.  We discuss the implications of this particular form of robustness for generalization, along with a game-theoretic interpretation of soft value aggregation as hedging against adversarial perturbations that seek to 
equalize the reward obtained for each action in a particular state \citep{ortega2014adversarial}.
% how this impacts the nature of the robustness or `zero-shot' generalization induced by policy regularization
Our analysis unifies several recent works that explore similar interpretations \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}, and our main contributions include
%Our main contributions are:
% Using tools from convex duality, we show that adversarial reward interpretations may not align with this desired robustness. Instead, we find that the optimal modified reward $r\tick$ in \cref{eq:reward_perturbation_stmt} simply re-expresses the value of the objective for a given policy, with the minimax optimization corresponding to a particular game-theoretic interpretation \citep{ortega2014adversarial}. We make the following additional contributions
% \TG{Alternative for the previous para: ``Using tools from convex duality, we precisely characterize the `zero-shot' generalization regime and relate it to a game-theoretic interpretation where robustness arises from `hedging' against adversarial perturbations to the reward function \citep{ortega2014adversarial}. We find that the optimal modified reward $r\tick$ in \cref{eq:reward_perturbation_stmt} re-expresses the value of the objective for a given policy, which restricts the set $\mathcal{R}$. We discuss how this impacts the nature of the robustness or `zero-shot' generalization induced by policy regularization and provide a unified discussion of several recent works that explore similar interpretations \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}. Our main contributions are:}
\begin{itemize}
% \item A thorough analysis of the robustness associated with \KL and $\alpha$-divergence regularization of \gls{RL} policies, which includes popular Shannon \citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum} and Tsallis entropy \citep{lee2019tsallis} entropy regularization as a special cases.    We argue that using divergence regularization instead of entropy regularization avoids several unsatisfying conclusions from previous work. %\citep{lee2019tsallis, eysenbach2021maximum}.
% %Our derivations for $\alpha$-divergence regularization extend the Tsallis entropy \citep{lee2019tsallis}
\item A thorough analysis of the robustness associated with \KL and $\alpha$-divergence regularization of \gls{RL} policies.  This includes popular Shannon entropy regularization  
%schemes 
\citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum} as a special case, and our derivations for the $\alpha$-divergence generalize the Tsallis entropy \gls{RL} framework of \citep{lee2019tsallis}.  
% Our analysis covers popular Shannon entropy regularization schemes \citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum}, while our derivations for the $\alpha$-divergence extend the Tsallis entropy \gls{RL} framework of \citep{lee2019tsallis}.    
\item Our analysis of the $\alpha$-divergence highlights distinct roles for the value function and policy normalization constant, which coincide in the case of the \textsc{kl} divergence. 
% but not for the $\alpha$-divergence. 
% We argue that using divergence regularization instead of entropy regularization avoids several unsatisfying conclusions from previous work. %\citep{lee2019tsallis, eysenbach2021maximum}.
\item A precise characterization of the feasible set $\mathcal{R}$ of adversarial rewards against which a regularized policy is robust, as visualized in \cref{fig:feasible_set_main} and shown in \myprop{perturbations}-\ref{prop:perturbations_alpha}.
% which improves upon the analysis of \citet{eysenbach2021maximum}.  
Our use of divergence regularization instead of entropy regularization clarifies 
several unsatisfying conclusions from previous work.
% the analysis of \citet{eysenbach2021maximum}.
\item We link a game-theoretic `indifference condition', which occurs at an equilibrium between the agent and adversary \citep{ortega2014adversarial}, to the `path consistency' optimality condition, which has been used to construct learning objectives in \citep{nachum2017bridging, chow2018path}.  
% % for the optimal policy and reward perturbations  with notion of path consistency \citep{nachum2017bridging, chow2018path}.  
% \item \textcolor{red}{to be cut} A comparison of regularization of the joint state-action distribution and conditional policy distribution. 
% % with connections between adversarial reward perturbations and the notion of path consistency \citep{nachum2017bridging, chow2018path}.  
% \item An alternative derivation of the objective function used in Logistic $Q$-learning \citep{basserrano2021logistic}, in which adversarial reward perturbations provide a natural justification for including $Q$-values in convex programming formulations of \textsc{rl}. \RB{likely only one of these, derivation needs to be checked to prioritize this}
\end{itemize}
While the latter observations hold only for the optimal policy, we emphasize that our results provide a reward robustness interpretation for \textit{any} stochastic policy under a given regularization scheme.
%After interpreting the optimal adversarial rewards in terms of both the policy and $Q$-values of the agent, we argue that adversarial reward perturbation interpretations %of stochastic policies provide a natural way to include $Q$-values in \gls{LP} formulations of \gls{RL} and lead to an alternative derivation of the objective function used in Logistic $Q$-learning \citep{basserrano2021logistic}. 
%     \item \TG{Precise characterization of the robustness induced via policy regularization in RL. In particular we theoretically analyze KL- and alpha-divergence regularization, which includes the popular maximum entropy regularization (TODO: citation) as a special case.}
%     \item \TG{Theoretical and empirical analysis of the feasible set $\mathcal{R}$, which is the set of adversarial reward perturbations to which the regularized policy is `zero-shot' robust against.}
%     \item %We clarify the feasible set of adversarial rewards associated with a particular policy compared with \citet{eysenbach2021maximum}, 
%     Compared with \TG{Maybe better: ``Following up on''} \citet{eysenbach2021maximum}, we clarify the feasible set of adversarial rewards associated with a particular policy
%     and argue that using divergence regularization instead of entropy regularization avoids several unsatisfying conclusions.
%     %leads to several unsatisfying interpretations compared with divergence regularization.
%     %correct several unintuitive conclusions which arise from entropy regularization rather than divergence regularization.
%     \item We provide derivations and analysis for $\alpha$-divergence regularization, which generalizes the Tsallis entropy framework of \citet{lee2019tsallis}.    This provides insight into the distinct role of the value function and normalization constant of the policy, which coincide for the case of the \textsc{kl} divergence or Shannon entropy.   %and provides insight into the distinct role of the value function and normalization constant of the policy, which coincide for the case of the \textsc{kl} divergence or Shannon entropy.
%     \item After interpreting the optimal adversarial rewards in terms of both the policy and $Q$-values of the agent, 
%     we argue that adversarial reward perturbation interpretations %of stochastic policies
%     provide a natural way to include $Q$-values in \gls{LP} formulations of \gls{RL} and lead to an alternative derivation of the objective function used in Logistic $Q$-learning \citep{basserrano2021logistic}.   %To this end, %we provide an alternative derivation of the objective function in Logistic $Q$-learning.  %which does not rely on a relaxed \gls{LP}.
% \end{itemize}
% %Compared with previous works, we clarify the feasible set of adversarial rewards and correct several surprising conclusions which arise from entropy regularization rather than divergence regularization.  Finally, we provide additional derivations and analysis for $\alpha$-divergence regularization, which extends the Tsallis entropy \textsc{rl} framework of \citet{lee2019tsallis}.



% \textbf{Contributions}
% \begin{itemize}
%     \item  We extend the analysis of \citet{ortega2014adversarial} to the sequential setting using the convex programming tools, which leads to more extensive, game-theoretic analysis of the reward robustness described in \citet{eysenbach2021maximum}.    We also discuss connections with the more general results of \citet{husain2021regularized}, and clarify the feasible set of reward perturbations compared with \citep{eysenbach2021maximum}.
%     %provide a more precise characterization of the
%     %Further, the use of entropy regularization in \citet{eysenbach2021maximum} leads to the counter-intuitive conclusion that increasing regularization strength leads to \textit{less} robust agents.   
%     \item We extend derivations using the \textsc{kl} divergence to the $\alpha$-divergence, which includes the Tsallis entropy as a special case.  With detailed convex conjugacy derivations, we highlight distinct roles for the value function and policy normalization constant, which coincide in the case of the \textsc{kl} divergence but not for the $\alpha$-divergence. 
    
%     % \item We provide a more detailed amore precise characterization of the feasible set of perturbations
    
%     \item Finally, our reward robustness interpretations using convex duality suggest connections with the notion of path consistency \citep{nachum2017bridging, chow2018path} and may provide additional insight into a relaxed \textsc{lp} formulation from \citep{mehta2009q, lee2019stochastic, basserrano2021logistic}. 
%     %\item  We provide a more precise characterization of the feasible set of perturbations
%     %\item  We visualize the optimal perturbed rewards in a single step (\cref{fig:perturb_opt}) and \textcolor{red}{multi-step} setting 
%     %\item  We analysis applies similarly to the derivations of \citet{husain2021regularized}
% \end{itemize}

==> Reward Robustness TMLR (3)/old/1_prelim.tex <==
\section{Preliminaries}\label{sec:prelim}
% In this section, we provide background on primal and dual \gls{LP} formulations of %fully observed, 
% discounted \gls{MDP}, along with extensions using convex policy regularization.
% We begin by reviewing the convex conjugate function, %or Legendre-Fenchel transform, 
% which will play a crucial role throughout our paper.
In this section, we review
% provide background on 
\gls{LP} formulations of %fully observed, 
discounted \gls{MDP}, along with extensions to convex policy regularization.
We begin by reviewing the convex conjugate, %or Legendre-Fenchel transform, 
which will play a crucial role throughout our paper.


\subsection{Convex Conjugate}\label{sec:conj_intro}
% Before describing analogous primal and dual optimizations for regularized \gls{MDP}s, we review the convex conjugate function, or Legendre-Fenchel transform, which will play a crucial role throughout our paper.
%First,
For any convex function $\Omega(\pi)$ with domain $\pi \in \mathcal{D}$, 
%, where $\mathcal{D}$ may indicate the probability simplex $\Delta^{|A|}$ with possible additional constraints, such as $\mu_{\pi}(a,s) \in \mathcal{M}$
%over domain $\pi \in \Delta^{|\mathcal{A}|}$, possibly , 
%the Legendre-Fenchel transform or 
the conjugate function $\Omega^{*}$ is defined via the optimization
\begin{align}
    \Omega^{*}( \dualvar ) = \sup \limits_{\pi \in \mathcal{D}} \, \big \langle \pi, \dualvar \big \rangle - \Omega(\pi) \label{eq:conjstar}
\end{align} 
where $\dualvar \in \dualdomain$ is a function in the continuous dual space of $\pi$. %continuous function in the topological dual space of $\pi$. %arbitrary function whose domain has the same dimension as $\mathcal{D}$.  
 %The conjugate function 
 The conjugate operation is an involution for proper, lower semi-continuous, and convex $\Omega$ \citep{boyd2004convex},
 %(\citet{borwein2010convex} Sec. 4.3), 
 so that $(\Omega^{*})^{*} = \Omega$ and $\Omega^{*}$ is also convex.  
 We can thus represent $\Omega(\pi)$ via a conjugate optimization
 \begin{align}
     \Omega(\pi) = \sup_{\dualvar \in \dualdomain} \big \langle \pi, \dualvar \big \rangle - \Omega^{*}(\dualvar) \label{eq:conjomega}
 \end{align}
  Differentiating with respect to optimization variable in either \cref{eq:conjstar} or \cref{eq:conjomega} suggests optimality conditions for $\pi_*$ and $\dualvar$
%   Solving for the $\arg \sup$ in either \cref{eq:conjstar} or \cref{eq:conjomega} suggests optimality conditions for $\pi_*$ and $\dualvar$
% \begin{align}
%     \pi_*(a|s) = \big(\nabla \Omega(\pi) \big)^{-1}(\dualvar) \qquad \qquad \dualvar_*(a,s) = \big(\nabla \Omega^{*}(\dualvar) \big)^{-1}(\pi)
% \end{align}
 \begin{align}
     \pi_*(a|s) = \nabla \Omega^{*}( \dualvar )   \quad \qquad \dualvar_*(a,s) = \nabla \Omega(\pi)     \label{eq:optimal_policy_as_grad}
 \end{align}
From the above, conjugacy also implies relationships of the form $\pi_*(a|s) = (\nabla \Omega)^{-1}(\dualvar_*(a,s))$ when $\pi_*$ and $\dualvar_*$ are in dual correspondence.


%We show concrete examples of the conjugate function in \cref{table:conjugates}\footnote{Note, we distinguish between conjugate functions $\Omega_{\pi}(\pi)$ and $\Omega_{\tpi}(\tpi)$, where $\pi$ is explicitly constrained to be normalized while  $\tpi$  is not.}, with derivations in \myapp{kl_conj_all}-\ref{app:alpha_conj_all}, %and discussion in \mysec{conj_examples}
We proceed to describe how the conjugate arises in convex programming formulations of regularized \gls{MDP}s, before describing examples in \mysec{conj_examples}. %concrete


% \small
% \begin{figure*}[t]
% \centering
% % \begin{tabular}{ccc}
% %   \multicolumn{1}{c}{$\Omega(\pi)$} & \multicolumn{1}{c}{Definition of $D[\pi||\pi_0]$} & \multicolumn{1}{c}{Conjugate $\Omega^{*}(\dualvar)$} \\ \toprule
% %     $\frac{1}{\beta} D_{KL}[\pi:\pi_0]$ & $\sum \limits_{a} \pi \log \pi/\pi_0 $& $\frac{1}{\beta} \log \sum \limits_{a} \pi_0  \expof{\beta \cdot \dualvar} $ \\[1.25ex] %\sum \limits_{\pi_0}
% %     $\frac{1}{\beta}D_{KL}[\tpi:\tpi_0]$ & $\sum \limits_{a} \tpi \log \tpi/\tpi_0 - \sum \limits_{a} \tpi + \sum \limits_{a}\tpi_0$ & $\frac{1}{\beta} \sum \limits_{a} \tpi_0 \expof{\beta \cdot \dualvar} - \frac{1}{\beta} \sum \limits_{a} \tpi_0$  \\[1.25ex] % \mathbb{E}_{\pi_0}
% %     $\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $\frac{1}{\alpha(1-\alpha)}\big( 1 - \sum \limits_{a} \pi_0^{1-\alpha} \pi^{\alpha} \big)$ & \\[1.25ex]
% %     $\frac{1}{\beta}D_{\alpha}[\tpi:\tpi_0]$ & $\frac{1}{\alpha(1-\alpha)}\big( (1-\alpha) \sum \limits_{a} \tpi_0 + \alpha \sum \limits_{a} \tpi - \sum \limits_{a} \tpi_0^{1-\alpha} \tpi^{\alpha} \big)$ & $\frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a} \tpi_0^{1-\alpha} \tpi^{\alpha} - \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_a \tpi$ \\ \bottomrule
% % \end{tabular
% %\tiny
% % \begin{tabular}{lllll} %\pi_*= \tpi_*=
% %   \multicolumn{1}{c}{$D[\pi||\pi_0]$} & \multicolumn{1}{c}{$\Omega(\pi)$} &  \multicolumn{1}{c}{$\Omega^{*}(\dualvar)$} & $\pi_* = \nabla \Omega^{*}( \dualvar )  $ & $\dualvar_*= \nabla \Omega(\pi)$  \\ \toprule
% %     $\frac{1}{\beta} D_{KL}[\pi:\pi_0]$ & $\sum \limits_{a} \pi \log \pi/\pi_0 $& $\frac{1}{\beta} \log \sum \limits_{a} \pi_0  \expof{\beta \cdot \dualvar} $ & $\pi_0 \exp\{\beta  \big( \dualvar - \psi(\beta) \big) \}$ & \tiny $\frac{1}{\beta} \log \frac{\pi}{\pi_0} + \frac{1}{\beta} \sum \limits_a \pi_0 \exp \{ \beta \cdot r\tick \} $\\[1.5ex] %\sum \limits_{\pi_0}
% %     $\frac{1}{\beta}D_{KL}[\tpi:\tpi_0]$ & $\sum \limits_{a} \tpi \log \tpi/\tpi_0 - \sum \limits_{a} \tpi + \sum \limits_{a}\tpi_0$ & $\frac{1}{\beta} \sum \limits_{a} \tpi_0 \expof{\beta \cdot \dualvar} - \tpi_0$ & $\tpi_0 \exp\{\beta \cdot \dualvar \}$ & $\frac{1}{\beta} \log \frac{\pi}{\pi_0} $\\[1.5ex] % \mathbb{E}_{\pi_0}
% %     $\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $\frac{1}{\alpha(1-\alpha)}\big( 1 - \sum \limits_{a} \pi_0^{1-\alpha} \pi^{\alpha} \big)$ &  \tiny $\frac{\alpha-1}{\alpha} \sum \limits_a \pi_0 [ 1 + (\alpha-1) \beta \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}}$ & \tiny $\pi_0 [ 1 + (\alpha-1) \beta \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}} $ & \\
% %     & &  \qquad \tiny $\, + \frac{1}{\beta} \psi_{\alpha}(\beta)$&  &\\[1.5ex]
% %     $\frac{1}{\beta}D_{\alpha}[\tpi:\tpi_0]$ & \tiny $\frac{1}{\alpha(1-\alpha)}\big( \sum \limits_{a} (1-\alpha) \tpi_0 $ & \tiny $\frac{\alpha-1}{\alpha} \sum \limits_a \tpi_0 [ 1 + (\alpha-1) \beta \cdot \dualvar]_+^{\frac{1}{\alpha-1}}$ & \tiny $\tpi_0 [ 1 + (\alpha-1) \beta \cdot \dualvar]_+^{\frac{1}{\alpha-1}} $ & \\ 
% %     & $ \, \, +\sum \limits_{a} \alpha \tpi - \tpi_0^{1-\alpha} \tpi^{\alpha} \big)$ &  \tiny $\, \, + \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_a  (\tpi_0 [ 1 + (\alpha-1) \beta \cdot \dualvar]_+^{\frac{1}{\alpha-1}} - \tpi_0 \big)$&  &\\ \bottomrule
% % \end{tabular}
% \small
% \begin{tabular}{lll} %\pi_*= \tpi_*=
%   \multicolumn{1}{c}{$D[\pi||\pi_0]$} & \multicolumn{1}{c}{$\Omega(\pi)$} &  \multicolumn{1}{c}{$\Omega^{*}(\dualvar)$}  \\ \toprule
%     $\frac{1}{\beta} D_{KL}[\pi:\pi_0]$ & $\sum \limits_{a} \pi \log \pi/\pi_0 $& $\frac{1}{\beta} \log \sum \limits_{a} \pi_0  \expof{\beta \cdot \dualvar} := \psi_1(\beta) $ \\[1.5ex] %\sum \limits_{\pi_0}
%     $\frac{1}{\beta}D_{KL}[\tpi:\tpi_0]$ & $\sum \limits_{a} \tpi \log \tpi/\tpi_0 - \sum \limits_{a} \tpi + \sum \limits_{a}\tpi_0$ & $\frac{1}{\beta} \big( \sum \limits_{a} \tpi_0 \expof{\beta \cdot \dualvar} - \tpi_0 \big)$ \\[1.5ex] % \mathbb{E}_{\pi_0}
%     $\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $\frac{1}{\alpha(1-\alpha)}\big( 1 - \sum \limits_{a} \pi_0^{1-\alpha} \pi^{\alpha} \big)$ &  $\frac{\alpha-1}{\alpha} \sum \limits_a \pi_0 [ (\alpha-1) \beta \cdot \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}} \cdot \dualvar + \frac{1}{\alpha} \psi_{\alpha}(\beta)$ \\
%     %$\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $\frac{1}{\alpha(1-\alpha)}\big( 1 - \sum \limits_{a} \pi_0^{1-\alpha} \pi^{\alpha} \big)$ &  $\frac{\alpha-1}{\alpha} \sum \limits_a \pi_0 [ 1 + (\alpha-1) \beta \cdot \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}} \cdot \dualvar + \frac{1}{\beta} \psi_{\alpha}(\beta)$ \\
%     $\frac{1}{\beta}D_{\alpha}[\tpi:\tpi_0]$ & \footnotesize  $\frac{1}{\alpha(1-\alpha)}\big( \sum \limits_{a}  (1-\alpha) \tpi_0 + \alpha \tpi_1 - \tpi_0^{1-\alpha} \tpi^{\alpha} \big) $ & \tiny $\frac{\alpha-1}{\alpha}\bigg(  \sum \limits_a \tpi_0 [ 1 + (\alpha-1) \beta  \dualvar]_+^{\frac{1}{\alpha-1}} \dualvar \bigg) + \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_a  (\tpi_0 [ 1 + (\alpha-1) \beta  \dualvar]_+^{\frac{1}{\alpha-1}} - \tpi_0 \big)$\\[.1ex] \midrule
% \vspace*{.1cm}
% %& & & \linespread{0.5}  \\
% % \end{tabular}
% % \begin{tabular}{lll}
% \RB{Omit?}
% \multicolumn{1}{c}{$D[\pi||\pi_0]$} & \multicolumn{1}{c}{$\dualvar_*= \nabla \Omega(\pi)$} & \multicolumn{1}{c}{$\pi_* = \nabla \Omega^{*}( \dualvar )  $}  \\ \toprule
%  $\frac{1}{\beta} D_{KL}[\pi:\pi_0]$ & $\frac{1}{\beta} \log \frac{\pi}{\pi_0} + \frac{1}{\beta} \sum \limits_a \pi_0 \exp \{ \beta \cdot r\tick \} $  & $\pi_0 \exp\{\beta  \cdot \big( \dualvar - \psi(\beta) \big) \}$ \\
%  $\frac{1}{\beta}D_{KL}[\tpi:\tpi_0]$ & $\frac{1}{\beta} \log \frac{\pi}{\pi_0} $ & $\tpi_0 \exp\{\beta \cdot \dualvar \}$  \\
%  $\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $ \frac{1}{\beta} \frac{1}{\alpha-1} \left( \big(\frac{\tpi}{\tpi_0}\big)^{\alpha-1}\right) + \textcolor{red}{\psi_{\alpha}(\beta)}$ & $\pi_0 [ (\alpha-1) \beta \cdot \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}} $  \\ 
% %  $\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $ \frac{1}{\beta} \frac{1}{\alpha-1} \left( \big(\frac{\tpi}{\tpi_0}\big)^{1-\alpha}\right) $ & $\pi_0 [ 1 + (\alpha-1) \beta \cdot \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}} $  \\ 
%  $\frac{1}{\beta}D_{\alpha}[\tpi:\tpi_0]$ &$ \frac{1}{\beta}\ln_{\alpha} \big(\frac{\tpi}{\tpi_0}\big) := \frac{1}{\beta} \frac{1}{\alpha-1} \left( \big(\frac{\tpi}{\tpi_0}\big)^{\alpha-1} - 1\right)$ &  $\tpi_0 [ 1 + (\alpha-1) \beta \cdot \dualvar]_+^{\frac{1}{\alpha-1}} $ 
% \end{tabular}
% \captionof{table}{\centering Conjugate Functions for \textsc{kl} and $\alpha$-divergences over normalized $\pi$ and unnormalized $\tpi$.}\label{table:conjugates}
% \end{figure*}

\normalsize
\subsection{Primal Formulations}
We consider an \gls{MDP} as a tuple $\{ \mathcal{S}, \mathcal{A}, P, \nu_0, r, \gamma \}$ consisting of a state space $\mathcal{S}$, action space $\mathcal{A}$, transition dynamics $P(s\tick|s,a)$ for $s, s\tick \in \mathcal{S}$, $a \in \mathcal{A}$, initial state distribution $\nu_0(s) \in \Delta^{|\mathcal{S}|}$ in the probability simplex, and reward function $r(a,s):\mathcal{S} \times \mathcal{A} \mapsto \mathbb{R}$.   We use a discount factor $\gamma ~\in (0,1)$ 
% (\citet{puterman2014markov} Sec. 6)
, although this may also be handled by including a transition to an absorbing state into the \gls{MDP} (\citet{puterman2014markov} Sec. 5.3). 

\paragraph{Unregularized Case} %seeks %obtained 
%An agent seeks to maximize the expected discounted reward by acting according to a decision policy $\pi(a_t|s_t) \in \Delta^{|\mathcal{A}|}$, 
We consider an agent that seeks to maximize the expected discounted reward by acting according to a decision policy $\pi(a_t|s_t) \in \Delta^{|\mathcal{A}|}$ in each state of the \gls{MDP}. 
%which associates a distribution over actions to .    
We assume that the policy is stationary and Markovian, so that it is independent of both the timestep and trajectory history.


Most commonly, this optimization is written using expectations %are taken 
with respect to trajectories  $\tau$ which start from an initial state $s_0 \sim \nu_0(s)$ and evolve according to the policy $\pi(a|s)$ and dynamics $P(s\tick|s,a)$, with $ \tau \sim \pi(\tau):= \nu_0(s_0) \prod \pi(a_t | s_t) P(s_{t+1} | s_t, a_t)$.   Writing the objective $\mathcal{R}(r, \nu_0, P, \gamma)$ as $\mathcal{R}(r)$ for simplicity,
\begin{align}
   \mathcal{R}(r) := \max \limits_{\pi(a|s)} \, (1-\gamma) \, \mathbb{E}_{\tau \sim \pi(\tau)} \bigg[ \sum \limits_{t=0}^{\infty} \gamma^t \, r(s_t, a_t)  \bigg] \, . \label{eq:policy_only} 
\end{align}

%\subsubsection{Primal Optimization} 
%\paragraph{Primal Optimization} 
To highlight connections with literature on convex duality, we convert this optimization into a equivalent linear program, which we refer to as the \textit{primal}
%This learning problem may be also framed in terms of a linear program, which we will refer to as the \textit{primal}
\small
\begin{align}
   \hspace*{-.2cm} & \mathcal{R}(r) = \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \, \, \text{subj. to} \, \quad    \left( \forall s \in \mathcal{S} \right) \label{eq:primal_lp}\\
   &\sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \nonumber  \, .
   %\, \forall s \in \mathcal{S}\nonumber
\end{align}
\normalsize
where inner product notation $\langle \cdot, \cdot \rangle$ indicates summation or integration over the domain of $\mu$. %\RB{improve} %$\sum \mu \cdot \dualvar$
%The optimization is over state-action visitation distributions $\mu(a,s) \in \Delta^{|\mathcal{S}| \times |\mathcal{A}|} $, and a corresponding policy is obtained via $\pi(a|s) = \mu(a,s) / \sum_a \mu(a,s)$.   
We refer to the constraints as \textit{Bellman flow constraints} \citep{syed2008apprenticeship}, and denote
the set of feasible $\mu$ as $\mathcal{M}$. 
%the feasible set as $\mathcal{M}$. 
%~:=\{\mu(a,s) | \mu \in \Delta^{|\mathcal{S} \times \mathcal{A}|} , \sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick),  \forall s \}$.  

%As shown in \textcolor{red}{Appendix}, these constraints also enforce normalization of $\mu(a,s)$ for normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$.  Finally, the flow constraints reflect the familiar, undiscounted Markov stationarity condition $\sum_{a} \mu(a,s) = \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick)$ when $\gamma = 1$.

%\paragraph{} 
The equivalence between the \gls{LP} in \cref{eq:primal_lp} and the reward-maximization objective in \cref{eq:policy_only} can be seen by writing the marginal state-visitation distribution $\mu(s) \propto (1-\gamma) \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(s_t = s)$, which accounts for discounting and ensures the flow constraints are satisfied with $\mu(a,s) \in \mathcal{M}$. %\RB{Cite}
%that the joint $\mu(a,s) = \mu(s) \pi(a|s)$ factorizes into a marginal $\mu(s)$ which accounts for discounting, and a stationary policy $\pi(a|s)$. 
It can be shown that any stationary policy $\pi(a|s)$ induces a unique state-action 
visitation distribution $\mu(a,s)$, while, conversely, a feasible $\mu(a,s) \in \mathcal{M}$  is induced by some stationary $\pi(a|s)$ \citep{syed2008apprenticeship, agarwal2020rltheorybook}. % Sec. 1.5.2 % \citet{puterman2014markov} Sec. 8.9,
This result allows us to factorize the optimization in \cref{eq:primal_lp} into $\mu(s)\pi(a|s)$ for normalized $\pi(a|s) \in \Delta^{|\mathcal{A}|}$, which matches the optimization in \cref{eq:policy_only}.   Optimizing over $\mu(s)$ yields the unique marginal induced by $\pi(a|s)$.    %The optimal $\mu(s)$ corresponds to the unique marginal induced by $\pi(a|s)$ and ensures the flow constraints are satisfied with $\mu(a,s) \in \mathcal{M}$.
%to obtain a familiar state-wise policy optimization


% The equivalence between this \gls{LP} and the reward-maximization objective in \cref{eq:policy_only} can be seen by substituting the marginal state-visitation distribution $\mu(s) \propto (1-\gamma) \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(s_t = s)$ into \cref{eq:primal_lp}.  
% %, which accounts for discounting and ensures the flow constraints are satisfied with $\mu(a,s) \in \mathcal{M}$. \RB{Cite}
% %that the joint $\mu(a,s) = \mu(s) \pi(a|s)$ factorizes into a marginal $\mu(s)$ which accounts for discounting, and a stationary policy $\pi(a|s)$. 
% It can be shown that any stationary policy $\pi(a|s)$ induces a unique state-action visitation distribution $\mu(a,s)$, while, conversely, a feasible $\mu(a,s) \in \mathcal{M}$  is induced by some stationary $\pi(a|s)$ \citep{syed2008apprenticeship, agarwal2020rltheorybook}. % Sec. 1.5.2 % \citet{puterman2014markov} Sec. 8.9,
% This result allows us to factorize the optimization in \cref{eq:primal_lp} into $\mu(s)\pi(a|s)$ for normalized $\pi(a|s) \in \Delta^{|\mathcal{A}|}$, which matches the optimization in \cref{eq:policy_only}.   The optimization over $\mu(s)$ corresponds to the unique marginal induced by $\pi(a|s)$ and ensures the flow constraints are satisfied with $\mu(a,s) \in \mathcal{M}$.


\paragraph{Regularized Case}
We now consider regularizing the objective in \cref{eq:primal_lp} using a convex penalty function $\Omega$ with coefficient $1/\beta$.   
Letting $\Omega_{\pi_0}(\pi)$ be a statistical divergence between the policy and a reference distribution $\pi_0(a|s)$, we define the regularized $\mathcal{R}_{\Omega, \beta}(r)$~\footnote{We focus on policy regularization in this work, although similar reasoning may be applied to regularization of the joint-state action distribution $\mu(a,s)$ \citep{nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.} 
\begin{equation}
\resizebox{.9\columnwidth}{!}{\hspace*{-.2cm} $
   \mathcal{R}_{\Omega, \beta}(r) :=  \max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}} %\max \limits_{\pi(a|s) \in \Delta^{|A|}} 
   \blangle \mu(s)\pi(a|s), r(a,s) \brangle - \dfrac{1}{\beta}  \blangle \mu(s), \Omega_{\pi_0}(\pi) \brangle $  %\text{subj. to} \, \sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \, \forall s \in \mathcal{S} \label{eq:primal_lp}
   }\label{eq:primal_reg}
\end{equation}
%\normalsize
where we use $\mu(s) \rightarrow \mathcal{M}$ to indicate that $\mu(s)$ induces $\mu(a,s) \in \mathcal{M}$ for a given $\pi(a|s)$.    

% Comparing the form of \cref{eq:primal_reg} with the definition of $\Omega^{*}_{\pi_0,\beta}$ in \cref{eq:conjstar}, 
% we can recognize the regularized objective as corresponding to a conjugate optimization at each state
% %so that the value of the regularized objective 
% $ \mathcal{R}_{\Omega, \beta}(r) = \blangle \mu(s), \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(r) \brangle$, with the environment rewards $r(a,s)$ as the argument.   

%and an outer expectation over the discounted marginal visitation $\mu(s)$. 

%However, this expression is not useful in practice and an outer expectation with respect to the discounted marginal visitation $\mu(s)$. 
%However, this expression is not useful in practice, both because an agent must explore the environment without full knowledge of $r(a,s)$ and because the marginal $\mu(s)$ is intractable to sample.  
%We will observe more practical forms utilizing the conjugate in te
% \begin{align}
%     \mathcal{R}_{\Omega, \beta}(r) = \max \limits_{\mu(s) \rightarrow \mathcal{M}} \blangle \mu(s), \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(r) \brangle
% \end{align}
% where we include the constraint $\pi(a|s)\in \Delta^{|A|}$ in the definition of $\Omega^{*}_{\pi_0,\beta}$ (see \mysec{conj_examples}).
%$\langle \mu(s),  \frac{1}{\beta} \Omega^{*}_{\pi_0, \beta}(r) \rangle $


\subsection{Dual Formulations}\label{sec:dual}
\paragraph{Unregularized Case} 
The flow constraints in \cref{eq:primal_lp} are insightful, as they lead to a dual optimization reflecting the familiar Bellman equations \citep{bellman1957markovian}.    Introducing Lagrange multipliers $V(s)$ for each constraint, summing over $s \in \mathcal{S}$, and eliminating $\mu(a,s)$ by setting $d/d\mu(a,s) = 0$ yields the \textit{dual} %problem 
% Introducing Lagrange multipliers $V(s)$ for each constraint and summing over $s \in \mathcal{S}$, %we obtain the Lagrangian,
% \begin{align}
%     \max \limits_{\mu(a,s)} \min \limits_{V(s)} \, & \big \langle \mu(a,s), r(a,s) + \gamma \transitionv -V(s) \big \rangle \nonumber  \\
%     &+ (1-\gamma) \big\langle \nu_0, V(s) \big  \rangle \label{eq:dual_unreg}
% \end{align}
% where we have reindexed the transition tuple $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared with \cref{eq:primal_lp}.   Eliminating $\mu$ by setting $d/d\mu = 0$ yields a constraint in the \textit{dual} problem 
% %$\sum_{a\tick,s\tick} P(s|a\tick,s\tick) \mu(a,s)$ to $\sum_{a,s} P(s\tick|a,s) \mu(a,s)$
% % Indeed, this equivalence is supported by the result that each stationary policy $\pi(a|s)$ induces a unique $\mu(a,s)$ for a given $\nu_0(s)$ (\citet{puterman2014markov} Sec. 8.9, )
\begin{align}
  &\mathcal{R}^{*}(r):=\min \limits_{V(s)} \,  (1-\gamma) \big \langle \nu_0(s), V(s) \big \rangle \, \text{  subj to: }\, \label{eq:dual_lp} \\ %\quad \forall (s,a) \in \mathcal{S} \times \mathcal{A}
  & \, V(s) \geq r(s,a) + \gamma \transitionv  , \, \, \forall (s,a) \in \mathcal{S} \times \mathcal{A}  \nonumber \, ,
\end{align}
where $\transitionv$ is shorthand for $\mathbb{E}_{P(s\tick|a,s)}[ V(s\tick)]$, and we have reindexed the transition tuple $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared with \cref{eq:primal_lp}.
%See \citet{wang2007dual} for detailed discussion of algorithms solving the unregularized dual problem.

\paragraph{Regularized Case}
%convex conjugate function $\Omega^*_{\pi_0, \beta}(\dualvar)$, which we formally review in \mysec{conjugate} 
We can similarly derive dual versions of the regularized \gls{LP}, starting from a Lagrangian relaxation of \cref{eq:primal_reg}
%\max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}}
% \begin{align}
%     %\mathcal{L}(\mu, V, \Omega) := 
%     & \min \limits_{V(s)} \max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}} \, 
%      (1-\gamma) \big\langle \nu_0, V(s) \big  \rangle \\
%      + &\blangle \mu(s)\pi(a|s), r(a,s) +  \gamma \transitionv -V(s) \big \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \nonumber \\
%     &   \label{eq:lagrangian}\, ,
% \end{align}
\resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
\begin{align}
   &  \max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}} \min \limits_{V(s)}  \, 
     (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle  \label{eq:dual_lagrangian} \\
     + &\blangle \mu(s)\pi(a|s), r(a,s) +  \gamma \transitionv -V(s) - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \brangle \nonumber
\end{align}
}}
% \begin{equation}
%  \begin{array}{l}
%     \max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}} \min \limits_{V(s)}  \, 
%      (1-\gamma) \big\langle \nu_0, V(s) \big  \rangle  \label{eq:dual_lagrangian} \\[1.25ex]
%     \resizebox{\columnwidth}{!}{ + \blangle \mu(s)\pi(a|s), r(a,s) +  \gamma \transitionv -V(s)  - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \brangle } \nonumber
%     \end{array}
% \end{equation}
%We discuss two dual optimizations interpretations here, which will use similar analysis tools as used later in the paper. 
Swapping the order of optimization using strong duality \citep{agarwal2020rltheorybook}, we recognize the maximization over ${\pi(a|s)\in\Delta^{|A|}}$ as a conjugate function, leading to a regularized dual optimization
\resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
 \begin{align}
 \hspace*{-.2cm} &  \mathcal{R}_{\Omega, \beta}^{*}(r) = \min \limits_{V(s)} %\max \limits_{ \mu(s) \rightarrow \mathcal{M}}
 \,  (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle  \label{eq:dual_reg} \\ 
 &+ \mathbb{E}_{\mu(s)} \bigg[\, \frac{1}{\beta}\Omega^{*}_{\pi_0, \beta} \bigg(r(a,s) +  \gamma \transitionv -V(s) \bigg)  \bigg] \nonumber
\end{align}
}}
which is unconstrained, in contrast to \cref{eq:dual_lp}. %, and involves sampling under the induced marginal distribution $\mu(s)$. 
Dual objectives of this form appear variously in \citep{ying2020note,   nachum2020reinforcement, basserrano2021logistic, husain2021regularized, belousov2019entropic}, %although alternative choices must be made to avoid sampling from the intractable $\mu(s)$.
although it is often infeasible to sample from the induced marginal $\mu(s)$. % induced by $\pi(a|s)$.
In both cases, note that the optimization is over the dual variables $V(s)$ only.

\subsection{Soft Value Aggregation}\label{sec:valueaggregation}
%\RB{This is an optimization in terms of $\pi$, not $V(s)$}
Our main object of interest in the rest of the paper will be an alternative decomposition of the Lagrangian %dual 
in \cref{eq:dual_lagrangian}.
%mention a further decomposition the Lagrangian dual in \cref{eq:dual_lagrangian}.
%We mention a further decomposition of the Lagrangian dual to highlight an approach used later in the paper.  
% from \cref{eq:dual_lagrangian}
Eliminating $\mu(s)$ by setting $d/d\mu(s) = 0$, we obtain a condition known as the \textit{regularized Bellman operator} \citep{neu2017unified, geist2019theory}
%\resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
\small
\begin{align}
    V(s)  = \blangle \pi(a|s), \, r(s,a) + \gamma \transitionv \brangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \nonumber . % \label{eq:reg_bell}
\end{align}
\normalsize
%}}
% using fact that $V(s)$ is not a function of the action $a$. % $\pi(a|s)$.  
Eliminating $\mu(s)$ thus leads to a constraint on the form of $V(s)$, since both may be viewed as enforcing the Bellman flow constraints.  Plugging this expression back into the Lagrangian \cref{eq:dual_lagrangian} and removing the minimization over $V(s)$, we are left with only the initial state term and a maximization over $\pi(a|s) \in \Delta^{|\mathcal{A}|}$.
%, where the policy appears in the above expression for the value function $V(s)$.  

%This translates to a constraint of $V(s)$, so that we can remove minimization over the value function and plug this expression back into the Lagrangian \cref{eq:dual_lagrangian}.   We are left with only the initial state term and a maximization over $\pi(a|s) \in \Delta^{|\mathcal{A}|}$, where the policy appears in the above expression for the value function $V(s)$.  
%However, the above expression for the value function $V(s)$. %in \cref{eq:reg_bell} still depends on the policy, with a maximization over $\pi(a|s) \in \Delta^{|\mathcal{A}|}$.  

Recalling the definition of the state-action value, or $Q$ function, ${Q_V(s,a)= r(s,a) + \gamma \transitionv}$, which is recursively defined in terms of value function estimates $V(s\tick)$, we obtain the following optimization %\gamma \mathbb{E}_{P(s'|s,a)}[V(s')]
\resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
\begin{align}
    &\mathcal{R}_{\Omega, \beta}^{*}(r) = \, \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}} (1-\gamma) \, \blangle \nu_0(s) , V(s) \brangle \label{eq:bellman_reg} \\
    & \,\, \text{subj. \footnotesize $ V(s)= \blangle \pi(a|s), r(s,a) + \gamma \transitionv \brangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) $} \nonumber \\[1.25ex]
    &\text{\footnotesize$=(1-\gamma) \mathbb{E}_{\nu_0} \big[\max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \langle \pi(a|s), Q(s,a)  \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \big]$}  \label{eq:soft_bellman}
\end{align}
}}
\normalsize
This conveniently involves expectations under $\nu_0(s)$ only, and leads to `soft' versions of standard \gls{RL} algorithms such as value iteration (e.g. \citet{haarnoja17a, geist2019theory}).    
In the following sections, we interpret the regularized policy optimization in \cref{eq:soft_bellman}, which corresponds to the conjugate function $\frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$, as a two player game between an agent and an imagined adversary \citep{ortega2014adversarial}.
In \cref{fig:value_agga}, we visualize the optimal value function $V_*(s) = \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$, for \textsc{kl} or $\alpha$-divergence regularization and different choices of regularization strength $1/\beta$.   
The choice of divergence particularly affects the aggregated value for low regularization, although we do not observe a clear pattern with respect to $\alpha$.\footnote{See \citet{belousov2019entropic, lee2018sparse, lee2019tsallis}, or \cref{app:alpha_results} for additional discussion of the effect of $\alpha$-divergence regularization on learned policies.}
In all cases, the value function ranges between $\max_a Q(a,s)$ for an unregularized deterministic policy as $\beta \rightarrow \infty$, and the expectation under the reference policy $\mathbb{E}_{\pi_0}[Q(a,s)]$ for strong regularization as $\beta \rightarrow 0$.   We further discuss this property in Sec. \ref{sec:discussion}, and provide closed forms for $V_*(s)$ and the optimal policy below.   


% Recalling the definition of the state-action value, or $Q$ function $Q(s,a)= r(s,a) + \gamma \mathbb{E}_{P(s'|s,a)}[V(s')]$
% and plugging \cref{eq:reg_bell} back into the Lagrangian \cref{eq:lagrangian}, 

% The remaining optimization also corresponds to a conjugate optimization, so
% %We write the remaining optimization over $\pi(a|s)$, which must be normalized to satisfy the flow constraints, as
% % obtain a familiar optimization involving the initial state distribution
% \begin{align}
%     \mathcal{R}^{*}(r) = \, (1-\gamma) \, \mathbb{E}_{\nu_0(s)} \bigg[  \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}} \big\langle \pi(a|s), Q(s,a) \big \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi)  \bigg]  \,. \label{eq:bellman_reg}
% \end{align}
% where the term inside the expectation is 
% %which is the expected value of 
% the regularized Bellman \textit{optimality} operator $[\mathcal{T}_{*,\pi, \Omega_{\pi_0}, \beta} V](s) = \Omega^{*}_{\pi_0, \beta}(Q)$ \citep{neu2017unified, geist2019theory}, which is a contractive mapping and leads to various `soft' value iteration algorithms \citep{littman1996generalized, tishby2011information, fox2016taming, asadi2017alternative, haarnoja17a, lee2019tsallis}.



% \subsection{Convex Conjugate}\label{sec:conjugate}\label{sec:conj_examples}

% \paragraph{KL Divergence}

\subsection{Conjugate Function Examples}\label{sec:conj_examples}
% In this work, 
We consider regularization using the family of $\alpha$-divergences \citep{amari2016information, zhang2004divergence}, which includes both the forward and reverse \textsc{kl} divergences as special cases. 
We take the slightly non-standard step of writing divergences over unnormalized measures rather than probability distributions.  To see why this is useful, consider introducing a Lagrange multiplier to enforce the normalization constraint $\pi(a|s) \in \Delta^{|\mathcal{A}|}$ in \cref{eq:primal_reg}.   
In order to evaluate this relaxation,  the regularizer $\Omega_{\pi_0}(\pi)$ must be able to take unnormalized $\tpi(a|s) \not \in \Delta^{|\mathcal{A}|}$ as input. % in order to evaluate this expression.   

\paragraph{$\alpha$-Divergence} The $\alpha$-divergence over possibly unnormalized measures is defined as 
\small
\begin{align}
\hspace*{-.15cm} D_{\alpha}[\tpi_0:\tpi] = 
    \frac{1}{\alpha(1-\alpha)}\bigg( &  (1-\alpha) \sum \limits_{a \in \mathcal{A}}  \tpi_0(a|s) + \alpha \sum \limits_{a \in \mathcal{A}} \tpi(a|s) \nonumber \\
    &- \sum \limits_{a \in \mathcal{A}} \tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} \bigg) 
\end{align}
\normalsize
We distinguish between the conjugate function $\alphaconju$ and the conjugate with restriction to normalized distributions $\alphaconjn$  \citep{ruderman2012tighter}, with detailed discussion in \myapp{alpha_conj_all}.  The latter appears in defining the optimal value function in \cref{eq:primal_reg} and \cref{eq:soft_bellman}, 
\small
\begin{align}
    V_*(s) &= \alphaconjn(Q) = \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \blangle \pi(a|s), Q(a,s) \brangle -  \frac{1}{\beta}\Omega^{(\alpha)}_{\tpi_0,\beta}(\pi) \nonumber \\
    &= \frac{\alpha-1}{\alpha} \blangle \piopt(a|s), Q(a,s) \brangle + \frac{1}{\alpha} \normalizeralpha \label{eq:alpha_conj_norm_main}
\end{align}
\normalsize
where $\normalizeralpha$ is the normalization constant for the optimizing argument $\piopt(a|s)$ associated with $Q(a,s)$ %the dual variable 
\small
\begin{align}
   \hspace*{-.2cm} \piopt(a|s) = \pi_0(a|s) \, [1+(\alpha-1) \beta \cdot \big( Q(a,s) - \normalizeralpha \big) ]_+^{\frac{1}{\alpha-1}} \label{eq:alpha_opt_policy}
\end{align}
\normalsize
%See \myapp{alpha_conj_all} for derivations.  
The $\alpha$-divergence is also closely related to the Tsallis entropy \citep{lee2019tsallis}, as discussed in \ref{app:tsallis}.  
Unfortunately, the normalizer $\normalizeralpha$ appears inside the exponent and must be estimated numerically apart from special cases of $\alpha$ \citep{lee2019tsallis}.\footnote{\citet{wong2021tsallis} provide justification for a multiplicative normalization constant, but this is no longer directly related to the expected reward objective.}

We visualize the optimal value $V_*(s)$ and the normalization constant $\normalizeralpha$ as a function of $\alpha$ in \cref{fig:value_aggb}.   Apart from the case when $\alpha = 1$ as discussed below, we have $V_*(s) \neq \normalizeralpha$ in  \cref{eq:alpha_conj_norm_main}. 
% Also, notice that $V_*(s) \neq \normalizer$ except for when $\alpha = 1$, as discussed below and shown in \cref{fig:value_aggb}. 

\begin{figure}[t]
\begin{subfigure}{0.47\columnwidth}\includegraphics[width=\textwidth]{figs/value_agg/prior_uniform.pdf}
%\vspace*{.15cm}
\caption{$V(s)$ as a function of $\beta$}\label{fig:value_agga}\end{subfigure}\hspace*{.01\columnwidth}
\begin{subfigure}{0.52\columnwidth} 
% \vspace*{-.12cm}\includegraphics[scale=.3]{figs/conj_by_alpha/value_norm_beta1_vert.pdf}
\vspace*{-.1cm}\includegraphics[width=.96\textwidth]{figs/conj_by_alpha/value_norm_beta1_vert_thin.pdf}
\caption{$V(s)$ and $\psi_{\alpha}(s)$ as a function of $\alpha$ for $\beta=1$}\label{fig:value_aggb}\end{subfigure}
\caption{Optimal value function $V_*(s)$ and normalization constant $\psi_{\alpha}(s)$ as a function of $\beta$ (left) and $\alpha$ (right), using $Q(a,s)$ and $\pi_0(a|s)$ from the left inset.   See \cref{eq:alpha_conj_norm_main} and \cref{eq:kl_v} for closed forms. }\label{fig:value_agg_main}
\end{figure}


\paragraph{KL Divergence}
Taking the limit as $\alpha \rightarrow 1$, we obtain an extended version of the \textsc{kl} divergence commonly used as regularization for \gls{RL} 
% (\citet{tishby2011information, ortega2013thermodynamics, fox2016taming})
\small
\begin{align}
    \hspace*{-.15cm} D_{KL}[\tpi:\tpi_0] = \sum \limits_{a \in \mathcal{A}} \tpi(a|s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} - \tpi(a|s) + \tpi_0(a|s) \, . \nonumber
    %\sum \limits_{a \in \mathcal{A}} %\lim_{\alpha \rightarrow 1}
\end{align}
\normalsize
The value function, or conjugate $\frac{1}{\beta}\Omega^*_{\pi_0,\beta}(Q)$, as a function $Q$ and with restriction to normalized $\pi$ becomes
\small
\begin{align}
  \hspace*{-.2cm} V_*(s) = \frac{1}{\beta}\Omega^*_{\pi_0,\beta}(Q) = \frac{1}{\beta} \log \sum \limits_{a \in \mathcal{A}} \pi_0(a|s) \expof{\beta \cdot Q(a,s)}. \label{eq:kl_v}
\end{align}
\normalsize
%For the \textsc{kl} divergence, 
This matches the normalization constant for the optimal policy, with $V_*(s) = \psi(s;\beta)$ and
 \begin{align}
 \pi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s) -  \psi(s;\beta)\big)} \, ,\label{eq:kl_opt_policy}
 \end{align}
 This can also be seen by plugging $\alpha = 1$ into \cref{eq:alpha_conj_norm_main}.
 %after projection of unnormalized $\tpi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s)}$ onto the simplex $\Delta^{|\mathcal{A}|}$, with $\psi(s;\beta) = \frac{1}{\beta} \log \sum_a \pi_0(a|s) \expof{\beta \cdot Q(a,s)}$ enforcing normalization.

% \paragraph{$\alpha$-Divergence}
% \paragraph{Soft Value Aggregation}
% %\subsection{Soft Value Aggregation}\mysec{valueaggregation}
% In the following sections, we will interpret the regularized policy optimization in \cref{eq:primal_reg} or \cref{eq:soft_bellman} as a two player game between an agent and an imagined adversary \citep{ortega2014adversarial}.   
% We present this adversarial interpretation, which depends on the regularization function $\Omega_{\pi_0}(\pi)$ and strength $1/\beta$, in \mysec{adversarial_perturb}.
% %In \cref{fig:value_agg}, we visualize % and divergence 

% The value function $V(s)$, which measures the expected payoff for an agent with estimated values $\{Q(s,a), V(s)\}$ acting in a given \gls{MDP} starting from state $s \in \mathcal{S}$, depends on the strength and form of the regularization.  The value ranges between $\max_a Q(a,s)$ for a deterministic policy and weak adversaries as $\beta \rightarrow \infty$, and the expectation under the reference policy $\mathbb{E}_{\pi_0}[Q(a,s)]$ for strong adversaries as $\beta \rightarrow 0$.    In \cref{fig:value_agg}, we visualize $V(s) = \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ using the \textsc{kl} divergence or $\alpha$-divergence for regularization $\Omega_{\pi_0}(\pi)$ and different
% choices of regularization strength $1/\beta$.
% %$\beta$ and $\Omega_{\pi_0}(\pi)$ in  \cref{fig:value_agg}.

% %When viewing game theoretic terms, this is known as the \textit{certainty equivalent}

% %We will proceed to characterize this adversary in terms of  in terms of the regularization strength ($\beta$) and divergence $\Omega_{\pi_0}(\pi)$.
% %Note that high regularization or low $\beta$ indicates a weak adversary, so that the policy becomes increasingly greedily with respect to $Q(a,s)$. 


% Finally, the conjugacy conditions in \cref{eq:optimal_policy_as_grad} provide a closed form for the policy in terms of $Q(a,s)$ for each state in \cref{eq:soft_bellman}.   For \textsc{kl} divergence regularization,
%   \begin{align}
%  \pi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s) -  \psi(s;\beta)\big)} \label{eq:opt_policy}
%  \end{align}
%  after projection of unnormalized $\tpi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s)}$ onto the simplex $\Delta^{|\mathcal{A}|}$, with $\psi(s;\beta) = \frac{1}{\beta} \log \sum_a \pi_0(a|s) \expof{\beta \cdot Q(a,s)}$ enforcing normalization.
 
 


==> Reward Robustness TMLR (3)/old/2_perturbed.tex <==
\section{Adversarial Reward Perturbations}\label{sec:adversarial_perturb}
% Several previous works have leveraged the convex programming tools from the previous section to interpret regularized policies as being robust to adversarial perturbations of the reward function \citep{ortega2014adversarial, eysenbach2021maximum, husain2021regularized}. 
% Previous work \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum} has analyzed the robustness of regularized policies to adversarial perturbations to the environment reward function using convex duality.  We extend the analysis of \citet{ortega2014adversarial} to the sequential setting, and clarify the characterization of the feasible set of adversarial perturbations compared to \citep{eysenbach2021maximum}.      

In this section, we analyze the robustness of regularized policies to adversarial perturbations of the reward function, which arises from an alternative application of convex duality for regularized \gls{RL} objectives.    We draw connections with similar interpretations from \citet{ortega2014adversarial, eysenbach2021maximum, husain2021regularized} throughout our exposition, with additional discussion in \mysec{discussion}.
%Our analysis extends \citet{ortega2014adversarial} to the sequential setting and clarifies the feasible set of reward perturbations available to the adversary from \citet{eysenbach2021maximum}.  We discuss additional connections with related work in \mysec{discussion}.
%Building upon previous work, we extend the analysis of \citet{ortega2014adversarial} to the sequential setting, provide a precise characterization of the feasible set of reward perturbations available to the adversary \citep{eysenbach2021maximum},    

%We build upon previous work \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum} to characterize 
%, which suggests that stochastic policies are robust to adversarial perturbations of the environmental reward function.   
%We build upon previous work \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum} to characterize 
% which highlights the need for careful, game-theoretic analysis of reward robustness. % described in \citet{eysenbach2021maximum}.  
% %resolve counter-intuitive conclusions based on the
% Compared with \citet{eysenbach2021maximum}, we clarify the characterization of the feasible set of adversarial perturbations, resolve several unintuitive properties arising from entropy rather than divergence regularization,
% and provide further visualizations and derivations for the $\alpha$-divergence. 


% \paragraph{Conjugate Functions}
% Throughout this section, we utilize the conjugate of the \KL divergence over unnormalized measures \citep{zhang2004divergence} \footnote{\textcolor{red}{This extended \KL divergence matches the $\alpha$-divergence over unnormalized measures for $\alpha = \{0,1\}$.}} for simplicity.  
% \RB{Choose to enforce later}
% \begin{align}
%     &\Omega_{\tpi_0}(\tpi) = D_{KL}[\tpi(a|s):\tpi_0(a|s)] \\
%     &\phantom{\Omega_{\tpi}} :=  \sum \limits_{a} \tpi(a|s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} - \sum \limits_{a} \tpi(a|s) + \sum \limits_{a} \tpi_0(a|s) \nonumber
% \end{align}
% % \frac{1}{\beta} \sum \limits_{a} \tpi_0 \expof{\beta \cdot \dualvar} - \tpi_0
% with the conjugate of the scaled $\frac{1}{\beta} \Omega_{\tpi_0}(\tpi)$ equal to 
% \begin{align}
%   \frac{1}{\beta} \Omega^{*}_{\tpi_0,\beta}&(\dualvar) = \frac{1}{\beta} \sum \limits_{a} \tpi_0 \expof{\beta \cdot \dualvar} - \frac{1}{\beta} \sum \limits_{a} \tpi_0
% \end{align}
% See \myapp{kl_conj_all} for derivations.  We provide additional discussion of the $\alpha$-divergence, which is essentially identical to the Tsallis divergence used in \citep{lee2019tsallis}, in \myapp{alpha_conj_all}.  
% \footnote{Studying the $\alpha$-divergence allows disentangling the role of the conjugate function $\frac{1}{\beta}\Omega^{*}_{\tpi_0,\beta}$ and the policy normalization constant, which both match the value function $V(s)$ in the case of the \KL divergence. Compared with the Tsallis entropy \citep{lee2019tsallis}, the $\alpha$-divergence conveniently avoids a $1/\alpha$ factor in the solution to the conjugate optimization, with $\alpha = q$.}
% %and an interpretation of regularization and value aggregation.

%\paragraph{Conjugate Policy Representation}
\subsection{Policy-Based Interpretation}
We have seen that the conjugate optimization provides an alternative representation of a convex regularizer %$\frac{1}{\beta}\Omega_{\pi_0}(\pi)$.   
 \begin{align}
     \hspace*{-.2cm} \frac{1}{\beta} \Omega_{\tpi_0}(\tpi) = \max_{\pr} \big \langle \tpi(a|s), \pr(a,s) \big \rangle - \frac{1}{\beta}  \Omega^{*}(\pr) \, .\label{eq:conjomega2}
 \end{align}
Expanding the regularization term in \cref{eq:dual_lagrangian} using the conjugate function, we have %\cref{eq:conjomega} %$\Omega_{\pi_0}(\pi)$
\begin{align}
    \hspace*{-.2cm} & \quad \max \limits_{\mu(s) \rightarrow \mathcal{M}} \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s)} \min \limits_{\textcolor{\highlight}{\perturbr(a,s)}} \, \label{eq:pedro_form} \\
    & \big \langle {\mu(s)\pi(a|s)}, {r(a,s) +\gamma \transitionv - V(s) - \textcolor{\highlight}{\perturbr(a,s)}} \brangle  \nonumber  \\
    & \qquad + \frac{1}{\beta} \Omega^{*}_{\tpi_0, \beta} \big( \textcolor{\highlight}{\perturbr(a,s)} \big) + (1-\gamma) \blangle \nu_0(s), V(s) \brangle \, ,  \nonumber
\end{align}
where we change the maximization in \cref{eq:conjomega2} to a minimization since the \KL divergence is subtracted.
Optimizations over $\mu(s)$ or $V(s)$ enforce the Bellman flow constraints across states of the \gls{MDP}.

%This expression extends the single-step case in \citet{ortega2014adversarial} to the discounted, infinite-horizon setting.   
As in \citet{ortega2014adversarial}, we interpret this minmax optimization as a two player game in each state, between an agent which chooses a policy $\pi(a|s)$, and an imagined adversary which chooses a reward perturbation $\perturbr(a,s)$. %to minimize the objective.  
Notice that the adversary is penalized for large reward perturbations, with a cost measured by the conjugate function ${\Omega^{*}_{\tpi_0, \beta}(\perturbr)}$. %\geq 0 (only when $\pi$ is normalized)
%which is nonnegative and increasing in $\pr$ in our case.
%which we assume to be increasing and nonnegative \citep{husain2021regularized}. 

In the following proposition, we translate this cost function to a constraint on the feasible set of reward perturbations $\pr$ available to the adversary at a given regularization function $\Omega_{\tpi_0}$ with strength $1/\beta$. We also characterize the optimal adversarial reward perturbations, with detailed proofs in \myapp{kl_perturb_section} and \myapp{alpha_perturb}. 
% From this feasible set,
%dversarial %We solve for the optimal adversarial reward perturbations. 
\begin{proposition} \label{prop:perturbations}
Using \KL divergence regularization $\Omega_{\tpi_0} = D_{KL}[\tpi:\tpi_0]$, we have the following results:
\begin{enumerate}[label=(\alph*)]
% \item The unconstrained optimization in \cref{eq:pedro_form} corresponds to the following constrained optimization
% \small
% \begin{align}
%     %&\max \limits_{\mu(s) \rightarrow \mathcal{M}} \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s)} \min
%     &\hspace*{-.4cm} \max \limits_{\mu(s), \pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s),\perturbr(a,s)} (1-\gamma) \blangle \nu_0(s), V(s) \brangle \label{eq:constraint_set} \\[1.25ex]
%     & \scriptsize \hspace*{-.55cm} {+ \big \langle {\mu(s)\pi(a|s)}, {r(a,s) +\gamma \transitionv - V(s) - \perturbr(a,s)} \brangle  } \nonumber  \\[1.5ex]
%     & \hspace*{-.55cm} \text{subj.} \sum \limits_{a} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} \leq \sum \limits_{a} \pi(a|s)  \, \, \forall s \in \mathcal{S} \nonumber
%     %\frac{1}{\beta} \Omega^{*}_{\textcolor{red}{\tpi_0}, \beta} \big( \perturbr(a,s) \big)
% \end{align}
% \normalsize
% where the constraint arises from the conjugate function $\Omega^{*}_{\tpi_0,\beta}(\pr)$.% = \frac{1}{\beta} \sum \limits_{a} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} - \frac{1}{\beta}\sum \limits_{a} \pi_0(a|s)$.
\item 
For a given policy $\pi(a|s)$, the unconstrained optimization over $\pr(a,s)$ in \cref{eq:pedro_form} corresponds to the following constrained optimization
\small
\begin{align}
    %&\max \limits_{\mu(s) \rightarrow \mathcal{M}} \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s)} \min
    &\hspace*{-.4cm}  \min \limits_{\perturbr(a,s)} (1-\gamma) \blangle \nu_0(s), V(s) \brangle \label{eq:constraint_set} \\[1.25ex]
    & \scriptsize \hspace*{-.55cm} {+ \big \langle {\mu(s)\pi(a|s)}, {r(a,s) +\gamma \transitionv - V(s) - \perturbr(a,s)} \brangle  } \nonumber  \\[1.5ex]
    & \hspace*{-.55cm} \text{subj.} \sum \limits_{a} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} \leq \sum \limits_{a} \pi(a|s)  \, \, \forall s \in \mathcal{S} \nonumber
    %\frac{1}{\beta} \Omega^{*}_{\textcolor{red}{\tpi_0}, \beta} \big( \perturbr(a,s) \big)
\end{align}
\normalsize
where the constraint arises from the conjugate function $\Omega^{*}_{\tpi_0,\beta}(\pr)$.
\item The optimal strategy for the adversary is to choose reward perturbations equal to
\begin{align}
    \propt(a,s) = \frac{1}{\beta} \log \frac{\tpi(a|s)}{\tpi_0(a|s)} \label{eq:optimal_perturbed}
\end{align}
\end{enumerate}
\end{proposition}
% \begin{proof}
% See \myapp{kl_perturb_section}
% \end{proof}
\begin{proposition} \label{prop:perturbations_alpha}
Using $\alpha$-divergence regularization $\Omega_{\tpi_0} = D_{\alpha}[\tpi_0:\tpi]$, we have the following results:
\begin{enumerate}[label=(\alph*)]
\item For a given $\pi(a|s)$, the unconstrained optimization over $\pr(a,s)$ from \cref{eq:pedro_form} translates to the same minimization objective as in \myprop{perturbations}(a), with the following constraint 
\small
\begin{align}
      \hspace*{-.4cm} \sum \limits_{a \in \mathcal{A}} &\tpi_0(a|s) [1 + (\alpha-1) \beta \cdot \pr(a,s) ]_+^{\frac{\alpha}{\alpha-1}} \label{eq:constraint_set_alpha}  \\
      &\leq \sum \limits_{a \in \mathcal{A}} \tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} \quad \forall s \in \mathcal{S} \nonumber
      %\hspace*{-.5cm}\alphaconju(\pr) \leq  \, \frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a \in \mathcal{A}} \tpi_0(a|s) \left(\frac{\tpi(a|s)}{\tpi_0(a|s)}^{\alpha} -1 \right) \,\, \forall s \in \mathcal{S} \nonumber
      %\tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} - \frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a \in \mathcal{A}} \tpi_0(a|s) \quad \forall s \in \mathcal{S} 
\end{align}
\normalsize
where the constraint arises from the conjugate function $\Omega^{*(\alpha)}_{\tpi_0,\beta}(\pr)$.
\item The optimal strategy for the adversary is to choose reward perturbations equal to
\begin{align}
    \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \frac{\tpi(a|s)}{\tpi_0(a|s)} 
\end{align}
where %$\log_{\alpha}u:= \frac{1}{\alpha-1} \left( u^{\alpha-1} - 1\right)$.
$\log_{\alpha}\frac{\tpi(a|s)}{\tpi_0(a|s)}:= \frac{1}{\alpha-1} \left( \frac{\tpi(a|s)}{\tpi_0(a|s)}^{\alpha-1} - 1\right)$.
\end{enumerate}
\end{proposition}
% \begin{proof}
% See \myapp{alpha_perturb}.  \RB{Combine props?}
% \end{proof}
%We discuss these results in the rest of the section.

% \begin{proposition}
% For the \KL divergence over normalized distributions and the constrained conjugate optimization,
% %$\Omega^{*}_{\pi_0,\beta}(\pr) = \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \langle \pi, \pr \rangle - \Omega_{\pi_0}(\pi)$, 
% the optimal reward perturbations are defined in self-consistent fashion:
%  \begin{align}
%   \propt(a,s) =& \frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)} \label{eq:normalized_rewards} \\ 
%   &+ \frac{1}{\beta} \log \sum \limits_{a} \pi_0(a|s)  \expof{\beta \cdot \propt(a,s)} \nonumber
% \end{align}
% where $\frac{1}{\beta} \log \sum \limits_{a} \pi_0(a|s)  \expof{\beta \cdot \pr(a,s)}$ reflects the additive normalization constant of $\pi(a|s) \in \Delta^{|\mathcal{A}|}$.
% \normalsize
% \end{proposition}
% \begin{proof}
% See \myapp{kl_perturb_section}
% \end{proof}

% \begin{figure*}[t]
% \centering
% % \begin{minipage}{\textwidth}%{0.8\textwidth}
% % \centering
% \begin{center}
% \[\arraycolsep=.003\textwidth
% \begin{array}{cccccc} %[width=40mm]
%  \begin{subfigure}{0.07\textwidth} \vspace*{-.24cm} \includegraphics[width=\textwidth]
%  {figs/feasible/uniform_prior.png} \end{subfigure}& %\qquad  \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_01.png}
% {figs/feasible/kl/beta01alpha1uniform.pdf}
% \caption{\label{fig:taba} \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}& % \qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_1.png}
% {figs/feasible/kl/beta1alpha1uniform.pdf}
% \caption{\label{fig:tabb} \centering  $D_{KL}, \beta = 1$}\end{subfigure}& %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_10.png} 
% {figs/feasible/kl/beta10alpha1uniform.pdf}
% \caption{\label{fig:tabc} \centering \small $D_{KL}, \beta = 10$}\end{subfigure}& \rulesep
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
% % {figs/feasible/alpha-1/alpha_neg1_beta1_uniform.png} 
% {figs/feasible/alpha-1/alpha_neg1_beta1_uniform_redo.pdf} 
% \caption{\label{fig:tabd} \centering \small $\alpha = -1, \beta = 1$}\end{subfigure}&
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
% % {figs/feasible/alpha3/alpha3_beta1_uniform.png} 
% {figs/feasible/alpha3/alpha3_beta1_uniform_redo.pdf}
% \caption{\label{fig:tabe} \centering \small $\alpha = 3, \beta = 1$}\end{subfigure}
% \\ %&\hspace*{.2cm}\\
% \begin{subfigure}{0.07\textwidth}\vspace*{-.24cm} \includegraphics[width=\textwidth]{figs/feasible/nonuniform_prior.png}\end{subfigure}& %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_01.png}
% {figs/feasible/kl/beta01alpha1nonuniform.pdf}
% \caption{\label{fig:tabd} \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}& %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_1.png}
% {figs/feasible/kl/beta1alpha1nonuniform.pdf}
% \caption{\label{fig:tabe} \centering \small $D_{KL}, \beta = 1$}\end{subfigure}& %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_10.png} 
% {figs/feasible/kl/beta10alpha1nonuniform.pdf}
% \caption{\label{fig:tabf} \centering \small $D_{KL}, \beta = 10$}\end{subfigure}& \rulesep %\hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/alpha-1/alpha_neg1_beta1_nonuniform.png} 
% {figs/feasible/alpha-1/alpha_neg1_beta1_nonuniform_redo.pdf} 
% \caption{\label{fig:tabi} \centering \small $\alpha = -1, \beta = 1$}\end{subfigure}&
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip] 
% %{figs/feasible/alpha3/alpha3_beta1_nonuniform.png} 
% {figs/feasible/alpha3/alpha3_beta1_nonuniform_redo.pdf} 
% \caption{\label{fig:tabj} \centering \small $\alpha = 3, \beta = 1$}\end{subfigure}
% \end{array}
% \] 
% \end{center}
% % \end{minipage}
% \caption{Feasible Set (red region) for \textsc{kl} divergence (at various $\beta$) and $\alpha$-divergence ($\alpha=\{-1, 3\}, \beta =1$) regularization and fixed $Q(a,s)$ values (blue star).  Red star indicates optimal perturbed reward $\mr = r - \pr$, for optimal $\pi_*(a|s)$ associated with $Q$-values and regularization parameters $\alpha, \beta, \pi_0$ (\cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).  Top row:  $\pi_0=(\frac{1}{2},\frac{1}{2})$, Bottom row: $\pi_0 = (\frac{2}{3}, \frac{1}{3})$.  
% % Red dot indicates $Q(a,s)$ associated with policy $\pi(a|s)$
% }\label{fig:feasible_set_main}
% \end{figure*}
% \begin{figure}[t]
% \centering
% % \begin{minipage}{\textwidth}%{0.8\textwidth}
% % \centering
% % \[\arraycolsep=.003\textwidth
% % \begin{array}{cccccc} %[width=40mm]
%  \begin{subfigure}{0.07\textwidth} 
%  \vspace*{-.24cm} \includegraphics[width=\textwidth]
%  {figs/feasible/uniform_prior.png} 
%  \end{subfigure} % & \qquad  \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_01.png}
% {figs/feasible/kl/beta01alpha1uniform.pdf}
% \caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba} \end{subfigure} %& \qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_1.png}
% {figs/feasible/kl/beta1alpha1uniform.pdf}
% \caption{\label{fig:tabb} \centering  $D_{KL}, \beta = 1$}\end{subfigure} %& \qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_10.png} 
% {figs/feasible/kl/beta10alpha1uniform.pdf}
% \caption{\label{fig:tabc} \centering \small $D_{KL}, \beta = 10$}\end{subfigure}  
% % & 
% \rulesep
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
% % {figs/feasible/alpha-1/alpha_neg1_beta1_uniform.png} 
% {figs/feasible/alpha-1/alpha_neg1_beta1_uniform_redo.pdf} 
% \caption{\label{fig:tabd} \centering \small $\alpha = -1, \beta = 1$}\end{subfigure}
% % &
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
% % {figs/feasible/alpha3/alpha3_beta1_uniform.png} 
% {figs/feasible/alpha3/alpha3_beta1_uniform_redo.pdf}
% \caption{\label{fig:tabe} \centering \small $\alpha = 3, \beta = 1$}\end{subfigure}
% \\ %&\hspace*{.2cm}\\
% \begin{subfigure}{0.07\textwidth}\vspace*{-.24cm} \includegraphics[width=\textwidth]{figs/feasible/nonuniform_prior.png}\end{subfigure}
% % & %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_01.png}
% {figs/feasible/kl/beta01alpha1nonuniform.pdf}
% \caption{\label{fig:tabd} \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}
% % & %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_1.png}
% {figs/feasible/kl/beta1alpha1nonuniform.pdf}
% \caption{\label{fig:tabe} \centering \small $D_{KL}, \beta = 1$}\end{subfigure}
% % & %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_10.png} 
% {figs/feasible/kl/beta10alpha1nonuniform.pdf}
% \caption{\label{fig:tabf} \centering \small $D_{KL}, \beta = 10$}\end{subfigure}
% % & 
% \rulesep %\hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/alpha-1/alpha_neg1_beta1_nonuniform.png} 
% {figs/feasible/alpha-1/alpha_neg1_beta1_nonuniform_redo.pdf} 
% \caption{\label{fig:tabi} \centering \small $\alpha = -1, \beta = 1$}\end{subfigure}
% % &
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip] 
% %{figs/feasible/alpha3/alpha3_beta1_nonuniform.png} 
% {figs/feasible/alpha3/alpha3_beta1_nonuniform_redo.pdf} 
% \caption{\label{fig:tabj} \centering \small $\alpha = 3, \beta = 1$}\end{subfigure}
% % \end{array}
% % \]
% % \end{minipage}
% \caption{Feasible Set (red region) for \textsc{kl} divergence (at various $\beta$) and $\alpha$-divergence ($\alpha=\{-1, 3\}, \beta =1$) regularization and fixed $Q(a,s)$ values (blue star).  Red star indicates optimal perturbed reward $\mr = r - \pr$, for optimal $\pi_*(a|s)$ associated with $Q$-values and regularization parameters $\alpha, \beta, \pi_0$ (\cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).  Top row:  $\pi_0=(\frac{1}{2},\frac{1}{2})$, Bottom row: $\pi_0 = (\frac{2}{3}, \frac{1}{3})$.  
% % Red dot indicates $Q(a,s)$ associated with policy $\pi(a|s)$
% }\label{fig:feasible_set_main}
% \end{figure}

% Note that we have considered the conjugate derived from $\Omega(\tpi)$ over unnormalized density functions, so that normalization of $\pi(a|s)$ %\in \Delta^{|\mathcal{A}|}$ 
% is enforced when solving \cref{eq:pedro_form} for the policy rather than in the definition of the conjugate itself. %$\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}$ itself.  
% This allows us to avoid a self-referential definition of $\propt(a,s)$, which would include an additional $\frac{1}{\beta} \log \sum_{a} \pi_0 \expof{\beta \cdot \pr}$ on the right hand side of \cref{eq:optimal_perturbed}.   See \myapp{kl_perturb_section}.

 \paragraph{Conjugate Policy Representation}
Our derivations so far have only invoked the conjugate representation of the regularization function, which suggests that \textit{any} stochastic policy may be interpreted via an adversarial game once $\Omega, \tpi_0,$ and $\beta$ are known.  %$\frac{1}{\beta} \Omega_{\tpi_0}(\tpi)$ is known.      

By contrast, the analysis of \citet{eysenbach2021maximum} is framed in terms of the robustness associated with a given reward function and regularization scheme, rather than a policy.  While the feasible set for \KL divergence regularization in \cref{eq:constraint_set} can be characterized without reference to a particular policy assuming $\sum_a \pi(a|s) = 1$, %$\pi \in \Delta^{|\mathcal{A}|}$
the optimal reward perturbations and feasible set for the $\alpha$-divergence require knowledge of the policy.   
Unfortunately, associating a policy with a reward function $r(a,s)$ in a given (regularized) \gls{MDP} requires solving for the optimal policy in \cref{eq:primal_reg} or (\ref{eq:bellman_reg}). %in \cref{eq:reg_rl}  
%In order to associate a policy with a reward function and a given \gls{MDP} requires solving for the optimal policy in \cref{eq:reg_rl}.   
%using Shannon entropy regularization, a special case of the \KL divergence.  

% In this case, note that the feasible set can be characterized without reference to a particular policy, assuming $\pi \in \Delta^{|\mathcal{A}|}$.   However, this is not true of the constraint for the $\alpha$-divergence and, in both cases, the optimal reward perturbations depend directly on the policy.   
% Thus, solving for the optimal policy is necessary to fully characterize the robustness of 
% in an \gls{MDP} with reward $r(a,s)$ 
% in order to fully characterize the robustness associated with an \gls{MDP} with reward

% the optimal policy associated with an \gls{MDP} with reward 


% In the case of \KL divergence regularization, note the feasible set of reward functions does not depend on a particular policy and can be calculated directly assuming $\pi \in \Delta^{|\mathcal{A}|}$.   However, for the $\alpha$-divergence, the constraint depends on a particular policy.  

% %Our derivations involving the conjugate $\frac{1}{\beta} \Omega_{\tpi_0}(\tpi)$ in \cref{eq:conjomega2} suggest that any policy may . 
% analysis should begin with a particular policy rather than a given reward function.   To analyze robustness associated with a given reward function and regularization scheme, as in \citet{eysenbach2021maximum}, we would first need to solve for the optimal policy.

 \paragraph{Analyzing the Feasible Set}
In \cref{fig:feasible_set_main}, we visualize the feasible set of perturbed rewards in a two-dimensional action space for the \KL or $\alpha$-divergence, various $\beta$, and uniform or non-uniform priors.    
Since the optimal policy can be calculated easily in the single-step case, we consider $\pi_*(a|s)$ corresponding to fixed $Q(a,s) = [1.1, 0.8]$ for various regularization settings (see \cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).
We determine the feasible set of $\pr(a,s)$ according to the constraint in \cref{eq:constraint_set} or (\ref{eq:constraint_set_alpha}), and plot the modified reward $r\tick(a,s) = Q(a,s) - \pr(a,s)$ for 
 each action.
%  We then plot the modified reward $Q(a,s) - \pr(a,s)$ for each action and draw the feasible set according to \cref{eq:constraint_set}.
% We first fix a stochastic policy $\pi(a|s)$ and use \cref{eq:alpha_opt_policy} or (\ref{eq:kl_opt_policy}) to derive the corresponding $Q$-values, which we plot in blue and will discuss further in \mysec{value_based}.   We then plot the modified reward $Q(a,s) - \pr(a,s)$ for each action and draw the feasible set according to \cref{eq:constraint_set}.

 %reward perturbations should be analyzed with respect to a
%In the single step case, we have $Q(a,s) = r(a,s)$ and plot this as the reward function in blue.   
%We also plot the modified reward $r(a,s) - \pr(a,s)$ for each action and draw the feasible set according to \cref{eq:constraint_set}.   
%penalized for decreasing the reward while increasing both rewards is clearly feasible.  

Inspecting the constraints for the adversary in \cref{eq:constraint_set} and (\ref{eq:constraint_set_alpha}), note that both reward increases $\pr > 0$ and reward decreases $\pr < 0$ contribute non-negative terms which either up- or down-weight the reference policy $\pi_0(a|s)$.    The constraint on their summation forces the adversary to trade off between perturbing the reward at different actions in a particular state.

%  First, note that both reward increases $\pr > 0$ and reward decreases $\pr < 0$ provide a non-negative contribution to the adversary's constraint in \cref{eq:constraint_set}.
%  %at each action $a$.  
%  These terms either up- or down-weight the reference policy $\pi_0(a|s)$ with the resulting summation still equal to $1$, so that this constraint forces the adversary to trade off between perturbing the reward at different actions in a particular state.  % \RB{related to normalization}

For high regularization strength ($\beta=0.1$), we observe that the boundary is nearly linear, with slope $-\frac{\pi_0(a_2|s)}{\pi_0(a_1|s)}$ based on the ratio of each action in the prior.  The boundary steepens for lower regularization strength, with only small decreases in the reward function available.  In all cases, it is natural that increasing the reward in both actions is feasible for an adversary that seeks to minimize the objective in \cref{eq:pedro_form}.

Finally, we visualize the feasible set for the $\alpha$-divergence, with $\alpha \in \{-1, 3\}$ and $\beta = 1$, in \cref{fig:feasible_set_main} 
% \ref{fig:tabd}-\ref{fig:tabe} and \ref{fig:tabi}-\ref{fig:tabj} .  
(d)-(e) and (i)-(j).
For the optimal policy associated with a given reward function,  we see that the $\alpha = -1$ feasible set may not include this reward function.  
%Also note that, if we are given a reward function instead of a policy and are interested in characterizing the feasible set for the $\alpha$-divergence, 
% \RB{Move to discussion later?}
% While \citet{eysenbach2021maximum} display feasible sets arising from (negative) Shannon entropy regularization $\Omega(\pi) = - H(\pi)$, this approach leads to puzzling conclusion that \textit{lower} regularization strength $1/\beta$ leads to \textit{greater} adversarial robustness, with larger feasible sets.   
% In contrast to \cref{eq:optimal_perturbed}, the entropy-regularized policy is `robust' to only positive changes in the reward function $\pr(a,s) \geq 0$, with the optimal perturbed reward $\mr(a,s) = r(a,s) - \pr(a,s) = r(a,s) - \log \pi(a|s)$.   We also observe robustness to large positive reward perturbations for low regularization strength in \cref{fig:perturb_opt}, but the crucial negative reward perturbation arises for the action(s) in the support of the nearly deterministic policy.
% We prefer to characterize `robustness' in terms of \textit{reductions} to the reward function.    

%We also observe robustness to large 
%\RB{Best explanation as to why??}
%This suggests that \textit{all} perturbations contribute to the constraint 
%This interpretation arises from the fact that the entropy is pointwise non-negative
%proceed to characterize the feasible set of adversarial perturbations $\pr(a,s)$ using a constrained version of \cref{eq:pedro_form}, with visualizations in \cref{fig:feasible_set_main}. 

% \paragraph{Constrained Adversary}
% Notice that the adversary is penalized for large reward perturbations, with a cost measured by the conjugate function ${\Omega^{*}_{\tpi_0, \beta}(\perturbr)}$ \textcolor{red}{$\geq 0$}. %\geq 0 (only when $\pi$ is normalized)
% %which is nonnegative and increasing in $\pr$ in our case.
% %which we assume to be increasing and nonnegative \citep{husain2021regularized}. 
% We proceed to characterize the feasible set of reward perturbations $\pr(a,s)$ available to the adversary for a given regularization strength $1/\beta$, with detailed derivations in \myapp{kl_perturb_section}.
% Translating the unconstrained term $\frac{1}{\beta} \Omega^{*}_{\tpi_0, \beta}(\perturbr)$ to a constraint, we obtain
% %we show that a regularization strength of $\frac{1}{\beta}$ in the unconstrained adversarial optimization translates to a constraint
% \begin{align}
%     \hspace*{-.2cm}  \sum \limits_{a} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} \leq 1
% \end{align}
% with the remaining terms in \cref{eq:pedro_form} remaining unchanged.  Note that the adversary pays a non-negative penalty for both reward increases $\pr > 0$ and reward decreases $\pr < 0$ at each action $a$.  These terms either up- or down-weight the reference policy $\pi_0(a|s)$ with the resulting summation still summing to $1$, so we can already see that the adversary faces a tradeoff between perturbing the reward at different actions in a particular state.

% In \cref{fig:feasible_set_main}, we visualize the feasible set of perturbed rewards in a two-dimensional action space for the \KL divergence, various $\beta$, and uniform or non-uniform priors.    We plot the modified reward $r(a,s) - \pr(a,s)$ for each action and a fixed state.   
% %penalized for decreasing the reward while increasing both rewards is clearly feasible.  

% For high regularization strength ($\beta=0.1$), we observe that the boundary is nearly linear, with slope based on the ratio of each action in the prior. \RB{Check}   The boundary steepens for higher regularization strength, with only small decreases in the reward function available.  In all cases, note that increasing the reward in both actions is clearly feasible for an adversary minimizing the objective in \cref{eq:pedro_form}.

% %proceed to characterize the feasible set of adversarial perturbations $\pr(a,s)$ using a constrained version of \cref{eq:pedro_form}, with visualizations in \cref{fig:feasible_set_main}.



% % To derive the feasible set, we use the conjugate derived from $\Omega(\tpi)$ over unnormalized density functions, so that normalization of $\pi(a|s)$ %\in \Delta^{|\mathcal{A}|}$ 
% % is enforced when solving \cref{eq:pedro_form} for the policy rather than in the definition of $\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}$ itself.\footnote{See \myapp{kl_conj_all} for more detailed discussion.}



% \paragraph{Optimal Reward Perturbations}
% % Differentiating \cref{eq:pedro_form} with respect to $\perturbr$, we obtain the conjugate optimality conditions $\tpi(a|s) &= \nabla \frac{1}{\beta}\Omega^{*}_{\tpi_0, \beta}\big( \perturbr \big) = \big(\nabla \Omega_{\tpi_0}\big)^{-1}(\pr)$ from \cref{eq:optimal_policy_as_grad}, leading to %and solve for $\perturbr(a,s)$.   
% % %Alternatively, , leading to the condition for the optimal reward perturbations \citep{ortega2014adversarial}
% % \begin{align}
% %       \pr(a,s) = \frac{1}{\beta} \log \frac{\tpi(a|s)}{\tpi_0(a|s)} \,. \label{eq:optimal_perturbed}
% % %     \tpi(a|s) &= \nabla \frac{1}{\beta}\Omega^{*}_{\tpi_0, \beta}\big( \perturbr \big) \nonumber \\
% % %    \implies  & \pr(a,s) = \frac{1}{\beta} \log \frac{\tpi(a|s)}{\tpi_0(a|s)}
% % \end{align}
% In \myprop{perturbations} (b), we found that the optimal reward perturbations $\pr(a,s)$ correspond to the pointwise regularization $\ptReg(\tpi(a|s))$ at each action,  by using the optimality conditions 
% $\pr(a,s) &= \nabla \frac{1}{\beta}\Omega_{\tpi_0}\big( \tpi \big) = \big(\nabla \Omega^{*}_{\tpi_0,\beta}\big)^{-1}(\tpi)$ 
% %$\tpi(a|s) &= \nabla \frac{1}{\beta}\Omega^{*}_{\tpi_0, \beta}\big( \perturbr \big) = \big(\nabla \Omega_{\tpi_0}\big)^{-1}(\pr)$
% from \cref{eq:optimal_policy_as_grad}.   The $\alpha$-divergence may also be written with an outer expectation over $\tpi(a|s)$, $\Omega_{\tpi_0}(\tpi) = \mathbb{E}_{\tpi}[\ptReg(\tpi(a|s))]$, \RB{OMIT if keeping Prop}
% so that, as shown in \myapp{alpha_perturb} \myprop{perturbations_alpha}, we can similarly interpret the optimal reward perturbations as the pointwise regularizer
% \small
% \begin{align}
%     \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \frac{\tpi(a|s)}{\tpi_0(a|s)} := \frac{1}{\beta} \frac{1}{\alpha-1} \left( \frac{\tpi(a|s)}{\tpi_0(a|s)}^{\alpha-1} - 1\right)
% \end{align}
% \normalsize
% %\footnote{This assumption and point-wise regularization result similarly hold for the $\alpha$-divergence in \myapp{alpha_conj_all}.}
% Note that we have considered the conjugate derived from $\Omega(\tpi)$ over unnormalized density functions, so that normalization of $\pi(a|s)$ %\in \Delta^{|\mathcal{A}|}$ 
% is enforced when solving \cref{eq:pedro_form} for the policy rather than in the definition of $\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}$ itself.  
% This allows us to avoid a self-referential definition of $\propt(a,s)$ with an additional $\frac{1}{\beta} \log \sum_{a} \pi_0 \expof{\beta \cdot \pr}$ on the right hand side of \cref{eq:optimal_perturbed}.   See \myapp{kl_perturb_section}.
% %the conjugate function $\Omega^{*}_{\tpi_0, \beta}\big( \perturbr \big)$ over unnormalized density functions in \cref{eq:} and \cref{eq:}, so that normalization of $\pi(a|s)$ is enforced when solving for the policy rather than in the definition of the conjugate.   This allows us to avoid a self-referential definition of $\pr(a,s)$ with an additional $\frac{1}{\beta}\sum \limits_{a} \pi_0 \expof{\beta \cdot \pr}$ on the right hand side of \cref{eq:optimal_perturbed}   


\paragraph{Reward Perturbation as Pointwise Regularizer}
Note that both the \textsc{kl} and $\alpha$-divergences can be written with an outer expectation over $\tpi(a|s)$, with $\Omega_{\tpi_0}(\tpi) = \langle \tpi(a|s), \ptReg(\tpi(a|s)) \rangle$.   
With derivations in \myapp{tsallis}, we can see that the optimal reward perturbations in \myprop{perturbations} (b) and \ref{prop:perturbations_alpha}(b) correspond to the (scaled) pointwise regularization $\ptReg(\pi(a|s))$ for the divergence over normalized $\pi(a|s) \in \Delta^{|\mathcal{A}|}$
\begin{align}
   \ptReg(\pi(a|s)) = \frac{1}{\alpha} \propt(a,s) = \frac{1}{\alpha} \log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}
\end{align}
which may be further scaled by the regularization strength $1/\beta$.
This is a natural result, since the objective in \cref{eq:pedro_form} takes the outer expectation $\langle \pi(a|s), r(a,s) - \pr(a,s) \rangle$.  As an example, for the \KL divergence we have $\ptReg(\pi(a|s)) = \log \pi(a|s)/\pi_0(a|s) = \propt(a,s)$ with $\alpha = 1$. %and $D_{KL}[\pi:\pi_0] = \langle \pi(a|s),\ptReg(\pi(a|s))\rangle$.  
\RB{Unresolved... when $\alpha\neq 1$, objective value appears to change due to $\frac{1}{\alpha}$ factor}
% \begin{align}
%      \ptReg(\pi(a|s)) = \log \frac{\pi}{\pi_0} = \propt(a,s)
% \end{align}

Finally, note that we have considered the conjugate derived from $\Omega_{\tpi_0}(\tpi)$ over unnormalized density functions in deriving the optimal reward perturbations, so that normalization of $\pi(a|s)$ %\in \Delta^{|\mathcal{A}|}$ 
is enforced when solving \cref{eq:pedro_form} for the policy rather than in the definition of the conjugate itself. %$\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}$ itself.  
This allows us to avoid a self-referential definition of $\propt(a,s)$, which, for example, would include an additional $\frac{1}{\beta} \log \sum_{a} \pi_0 \expof{\beta \cdot \pr}$ on the right hand side of \cref{eq:optimal_perturbed}.   See \myapp{kl_perturb_section}.


% In \myprop{perturbations} (b) and \ref{prop:perturbations_alpha}(b), we can see that the optimal reward perturbations $\pr(a,s)$ correspond to the pointwise regularization $\ptReg(\tpi(a|s))$ at each action.   
% by using the optimality conditions 
% $\pr(a,s) &= \nabla \frac{1}{\beta}\Omega_{\tpi_0}\big( \tpi \big) = \big(\nabla \Omega^{*}_{\tpi_0,\beta}\big)^{-1}(\tpi)$ 
% %$\tpi(a|s) &= \nabla \frac{1}{\beta}\Omega^{*}_{\tpi_0, \beta}\big( \perturbr \big) = \big(\nabla \Omega_{\tpi_0}\big)^{-1}(\pr)$
% from \cref{eq:optimal_policy_as_grad}.   The $\alpha$-divergence may also be written with an outer expectation over $\tpi(a|s)$, $\Omega_{\tpi_0}(\tpi) = \mathbb{E}_{\tpi}[\ptReg(\tpi(a|s))]$, \RB{OMIT if keeping Prop}
% so that, as shown in \myapp{alpha_perturb} \myprop{perturbations_alpha}, we can similarly interpret the optimal reward perturbations as the pointwise regularizer
% \small
% \begin{align}
%     \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \frac{\tpi(a|s)}{\tpi_0(a|s)} := \frac{1}{\beta} \frac{1}{\alpha-1} \left( \frac{\tpi(a|s)}{\tpi_0(a|s)}^{\alpha-1} - 1\right)
% \end{align}
% \normalsize
% %\footnote{This assumption and point-wise regularization result similarly hold for the $\alpha$-divergence in \myapp{alpha_conj_all}.}


%This indicates that the optimal reward perturbations correspond to the point-wise regularization term at each $a|s$, assuming that the regularizer $\Omega_{\tpi_0}(\tpi) = \mathbb{E}_{\tpi}[\ptReg(\tpi(a|s))]$ can be written with an outer expectation over $\tpi(a|s)$.\footnote{This assumption and point-wise regularization result similarly hold for the $\alpha$-divergence in \myapp{alpha_conj_all}.}

% What are the implications of this result for our interpreting the adversarial reward robustness of regularized policies?
% \RB{save until discussion later, or briefly mention?}
% What implications does this result have for our adversarial reward robustness interpretation of regularized policies?
% %In light of this observation, how should we interpret the adversarial reward robustness?  
% The equivalence of the objectives in \cref{eq:reward_perturbation_stmt} \citep{eysenbach2021maximum} is trivially confirmed for the optimal $\dualvar(a,s) = r(a,s) - \ptReg(\tpi(a|s))$, which is not surprising given that our derivations only utilize an alternative representation of $\Omega_{\pi_0}(\pi)$ using convex duality.
% %aligns with our use of convex duality to obtain an alternative form for $\Omega_{\pi_0}(\pi)$.  %, so that the objectives match exactly.
% %The objective and reward perturbations are crucially sensitive to the  
% %Further, \cref{eq:reward_perturbation_stmt} and the perturbations in
%  %which are known to provide dual representations of a policy \citep{lee2019stochastic}.

% Nevertheless, the reward perturbations in \cref{eq:optimal_perturbed} indicate a very particular game-theoretic robustness \citep{ortega2014adversarial}, which may not directly align with notions of robustness as zero-shot generalization.   In the next section, we further discuss this robustness and explicitly relate the reward perturbations to dual representations of the policy in terms of $Q$-values and the value function $V(s)$ \citep{wang2007dual, lee2019stochastic}. %The adversarial reward perturbations are for each state-action pair, and the per-state normalization or feasible set constraints introduce competition among the perturbations for each action.   

% %\sout{This is in notable contrast to the experiments of \citet{eysenbach2021maximum}, in which the reward for \textit{an entire state}, chosen to be in the path of a deterministic policy, was modified.  While entropy-regularized policies performed better than a deterministic, unregularized policy in this environment, these results are more directly attributable to stochastic policies learning a \textit{diversity of solutions} \citep{haarnoja17a, haarnoja2018acquiring, kumar2020one}, rather than the \textit{reward robustness} suggested by convex duality. }

\subsection{Value-Based Interpretation}\label{sec:value_based} % of Reward Robustness}
In this subsection, we provide a complementary interpretation of adversarial reward robustness from a value perspective, which highlights the role of $\pr(a,s)$ as a dual variable related to $V(s)$ and $Q(a,s)$. % from \mysec{dual}.   %the results of the previous section, we  interpret strength and type of regularization as determining how an agent expresses uncertainty when aggregating state-action estimates $Q(a,s)$ into a per-state value function $V(s)$.
%leading to a known \textit{indifference} condition at optimal policy as in \citet{ortega2014adversarial}. 


\paragraph{Soft Value Aggregation \& Adversarial Hedging}
Using the results of the previous subsection, the value function $V_*(s) = \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ in \cref{eq:soft_bellman} and \cref{fig:value_agg_main} can be interpreted as the \textit{certainty equivalent} \citep{myerson2019probability, ortega2013thermodynamics}, %myerson2019probability,
which aggregates over actions $a \in \mathcal{A}$ to measure the payoff of a two-player game where the agent begins in state $s \in \mathcal{S}$ and plays against an adversary defined by the regularizer $\Omega_{\pi}(\pi)$ and strength $\beta$ as in \myprop{perturbations} \citep{ortega2014adversarial}.   % As shown in \cref{fig:value_agg}, for $\beta > 0$, this value ranges between the maximum reward over actions and the expected reward under the reference distribution.


%\paragraph{Soft Value Aggregation \& Adversarial Hedging}

% \paragraph{Soft Value Aggregation as Adversarial Hedge}
% % ********* Moved to Background ***********
%  We begin by imagining a single-step decision in a particular state $s \in \mathcal{S}$, for an agent with given $Q$-function estimates $Q(a,s) = r(a,s) + \gamma \transitionv$ in an \gls{MDP}.  
 
%  Instead of acting with deterministically with the greedy policy $\max_{\pi} \blangle\pi(a|s), Q(a,s)\brangle$,  %a \textbf{regularized} 
%  an agent \textcolor{red}{might express uncertainty in its $Q$-value estimates }by only allowing this information to induce a certain average deviation $R$ from a prior reference policy $\pi_0(a|s)$.
%  %the consideration of $Q$-value estimates to induce a certain average deviation $R$ from a prior reference policy $\pi_0(a|s)$.   
%  Measuring this average deviation using a convex divergence $\Omega_{\tpi_0} = R$ and introducing an appropriate Lagrange multiplier $1/\beta$ for the constraint, we are left with the conjugate optimization \citep{geist2019theory}
%  \begin{align}
%     V(s):= \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta} = \max_{\pi \in \Delta^{|\mathcal{A}|}} \blangle\pi(a|s), Q(a,s)\brangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) %\nonumber \label{eq:value_opt}
%  \end{align}
%  This expression matches \cref{eq:primal_reg} or \cref{eq:soft_bellman}, and \textit{soft}-value aggregation is indeed common in the literature \citep{ortega2013thermodynamics, fox2016taming, lee2019tsallis}.    However, the results of the previous section suggest an interpretation of soft-value aggregation as hedging against an \textit{imagined}, reward-perturbing adversary, where we use the conjugate representation of the regularizer  $\Omega_{\pi_0}(\pi) = \, \sup_{\perturbr} \langle \pi, \pr \brangle - \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(\pr)$ \citep{ortega2014adversarial}.   
%  The strength of the adversary is determined by $\beta$, with the feasible set determined by $\beta$ and the shape of the conjugate function $\Omega^{*}_{\pi_0,\beta}(\pr)$.
 
%  %Solving the conjugate optimization for the \textsc{kl} divergence, the optimizing policy becomes
 
%  %The resulting value function $V(s) = \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ reflects a \textit{soft}-aggregation of state-action estimates $Q(a,s)$ into a \textit{certainty equivalent} \citep{myerson2019probability}, which measures the agent's payoff for playing this two player game in a given state $s \in \mathcal{S}$ and against a particular adversary.   
% We visualize the value function $V(s) = \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$, which measures the agent's payoff for playing this two player game in a given state $s \in \mathcal{S}$ and against a particular adversary, for different adversary strengths ($\beta$) and divergences in \cref{fig:value_agg}.  The value ranges between $\max_a Q(a,s)$ for a deterministic policy as $\beta \rightarrow \infty$ or the expectation under the reference policy $\mathbb{E}_{\pi_0}[Q(a,s)]$ as $\beta \rightarrow 0$.    Note that high regularization or low $\beta$ indicates a weak adversary, so that the policy becomes increasingly greedily with respect to $Q(a,s)$. 

% Finally, the conjugacy conditions in \cref{eq:optimal_policy_as_grad} provide the optimizing policy in each state.   For \textsc{kl} divergence regularization, we have
%   \begin{align}
%  \pi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s) -  \psi_{\beta}(s)\big)} \label{eq:opt_policy}
%  \end{align}
%  where $\psi(s;\beta) = \frac{1}{\beta} \log \sum_a \pi_0(a|s) \expof{\beta \cdot Q(a,s)}$ enforces normalization.    While we always define the value function $V(s):= \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ using the conjugate as in \cref{eq:}
 
 
%  In the case of the \KL divergence, $\psi(s;\beta) = V(s)$, with $V(s):= \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ from \cref{eq:}, the subtractive normalization constant does not correspond to the value or conjugate function in general,  the $\alpha$-divergence in \myapp{alpha_conj_all} or \citet{lee2019tsallis}.
 
%  $V(s) := \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ for the \KL divergence, this is not true in general for the $\alpha$-divergence in \myapp{alpha_conj_all} or \citet{lee2019tsallis}.   We now proceed to discuss this policy in relation to the adversarial reward perturbations in \myprop{perturbations}
 
% %While soft value-aggregation is standard \citep{ortega2013thermodynamics, fox2016taming, lee2019tsallis}, we have emphasized its adversarial interpretation as in \citet{ortega2014adversarial}. 


%  %\textcolor{red}{While more complex techniques for expressing uncertainty exist \citep{duff2002optimal ,smirnova2019distributionally}, a simple strategy is to only allow these estimates to induce a certain average deviation $R$ from a prior reference policy $\pi_0(a|s)$.}   Deciding to measure this deviation using a convex statistical divergence $\Omega_{\tpi_0} = R$, we find that the agent will aggregate value in the state according to the conjugate function
%  %the agent will act according to a policy
% ******************************************               ***************************************


% Visualization:   Q values => policy at each α, 
% same policy, different Q values different value, different α
\paragraph{Reward Perturbations using $Q$-Values}
 %\paragraph{Reward Perturbations as \cancel{Advantage Function}}
 While a stochastic policy may be interpreted as hedging against an imagined adversary, we can also identify a given stochastic policy with an optimal adversarial reward perturbation. 
 %To further understand the nature of this adversary, we can also identify a given stochastic policy with an optimal adversarial reward perturbation.    
 %While a stochastic policy may be interpreted as hedging against an imagined adversary, we can also identify a given stochastic policy with an optimal adversarial reward perturbation.    
 Given a regularizer $\Omega_{\pi_0}(\pi) = D_{KL}[\pi:\pi_0]$, reference distribution $\pi_0(a|s)$, and regularization strength $1/\beta$, %simple algebraic rearrangement of \cref{eq:opt_policy} 
 we can simply rearrange \cref{eq:kl_opt_policy} to write  
\begin{align}
    \propt(a,s) = Q(a,s) - \normalizerexp =  \frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)} \label{eq:perturb_opt_q}
\end{align}
where the difference $Q(a,s) - \normalizerexp$ is uniquely determined from $\pi(a|s)$ and the assumed regularizer.   Note that the choice of $Q(a,s)$ and $\normalizerexp$ are not unique, as the normalization constant $\normalizerexp$ is determined from the choice of $Q(a,s)$ and may be intractable in practice.
%However, note that the choice of $Q(a,s)$ and $\normalizerexp$ are not unique, with $\normalizerexp$ chosen to enforce normalization for a given set of $Q(a,s)$.  %Furthermore, $\normalizerexp$ is often intractable in practice.
We obtain a similar expression for the $\alpha$-divergence, $Q(a,s) - \alphanorm =  \frac{1}{\beta} \ln_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}$, although the normalizer $\alphanorm$ is not equal to the conjugate $\alphaconjn(\pr)$ as in the case of the \KL divergence.

We visualize the optimal reward perturbations for the single step case in \cref{fig:perturb_opt}.   
Notice that the reward perturbations reflecting a given policy $\pi(a|s)$ can either be positive or negative, depending on the likelihood ratio $\frac{\pi(a|s)}{\pi_0(a|s)} \lessgtr 1$ or the difference $Q(a,s) - \alphanorm \lessgtr 0$.    We discuss this property in more detail in \mysec{discussion}.
%From \cref{eq:perturb_opt_q} or \cref{eq:optimal_perturbed}, we can see that the reward perturbations reflecting a given policy $\pi(a|s)$ can either be positive or negative, depending on the likelihood ratio between the policy the reference policy at each action.   
%This multiplicative factor can also be measured by a monotonic function of $Q(a,s) - \normalizerexp$, for example in the exponential family policy in \cref{eq:opt_policy}. 
 %To do so, we assume that the normalization constant for a given $\pi(a|s)$ is tractable.   With knowledge of $\pi_0(a|s)$
 
 
 \paragraph{Indifference Condition for Optimal Policy}
%In the previous sections, we have used convex duality to translate between expressions for the optimal reward perturbations in terms of the primal policy or dual value functions.    
For the optimal policy $\opt(a|s)$ in a given \gls{MDP}, we can additionally state an \textit{indifference condition} across actions, which is a well-known property of Nash equilibria in game theory \citep{osborne1994course, ortega2014adversarial}.   In particular, the adversarial objective
%For the optimal policy $\opt(a|s)$ in a given \gls{MDP}, the objective 
% \footnotesize
% \begin{align}
% \min \limits_{\pr(a,s)} &\blangle \opt(a|s), r(a,s) + \gamma \transitionv - V(s) - \pr(a,s) \brangle + \frac{1}{\beta} \Omega^{*}_{\tpi_0, \beta}(\pr) \nonumber \\
% &= V_{\beta}(s)
% \end{align}
has the same value for each action $a \in \mathcal{A}$ in state  $s \in \mathcal{S}$ (see \myapp{indifference}).   
We can see in \cref{fig:perturb_opt}(a) that the perturbed rewards for each action match the value function $V_*(s)$ in each state.   %This property also appears in \cref{fig:feasible_set_main}, with matching coordinates for the optimal perturbed $\mr(a,s)$. %with \KL divergence regularization.    
While it is possible to derive an adversarial interpretation for any $\pi(a|s)$ using \cref{eq:pedro_form}, we see in \cref{fig:perturb_opt}(b) that the indifference condition does not hold for suboptimal policies.  

% As the indifference condition for optimal policies highlights, the adversarial reward perturbations preserve the value of the objective in each state.   We further explore this sensitivity of the reward perturbations to the form of objective function below.

%in the single-step case, the $Q$-values do not match the environment rewards. %However, one can confirm algebraically or numerically that the value of the objective does not change.
%$Q(a,s) \neq r(a,s)$ for some $(a,s)$ in the single step case.  
%, where the single-step $Q$-values do not match the environment rewards.  

% While the indifference condition depends on the optimal policy arising from the $\max$ over $\pi(a|s)$, we can construct an adversarial interpretation in \cref{eq:pedro_form} for any $\pi(a|s)$ using the conjugate representation of the divergence $\Omega_{\pi_0}(\pi)$.   Visualizing the reward perturbations for both optimal and suboptimal policies for the single-step case in \cref{fig:indifference}, we observe that the indifference among actions does not occur for suboptimal policies.  
%Although the reward perturbations correspond to $Q(a,s) - \psi(s;\beta)$ despite the fact that the 


% \begin{figure}
% \begin{minipage}[b][6cm]{0.3\linewidth}
% \subfloat[A]{\includegraphics[width=3cm,height=2cm]{logo}}

% \vfill
% \subfloat[B]{\includegraphics[width=3cm,height=2cm]{logo}}
% \end{minipage}%
% \begin{minipage}[t][6cm]{0.3\linewidth}
% \subfloat[D]{\includegraphics[width=3cm,height=6cm]{logo}}
% \end{minipage}%
% \begin{minipage}[t][6cm]{0.3\linewidth}
% \subfloat[D]{\includegraphics[width=3cm,height=6cm]{logo}}
% \end{minipage}
% \caption{Many figures}\label{foo}
% \end{figure}

%%Our starting point in this section is the Lagrangian 
% \paragraph{Robustness to Reward Perturbations}
% To derive the adversarial robustness statement in \cref{eq:reward_perturbation_stmt} in terms of a constrained linear program, 
% \begin{align}
% &\max \limits_{\pi(a|s)} \mathbb{E}_{\tau \sim p^{\pi}(\tau)} \left[ \sum \limits_{t=0}^\infty \gamma^t \, \bigg( r(a_t, s_t) - \Omega\big(\pi(a_t | s_t)\big) \bigg) \right] \nonumber \\
% &= \max \limits_{\pi(a|s)} \min \limits_{r\tick(a,s) \in \mathcal{R}}  \mathbb{E}_{\tau \sim p^{\pi}(\tau)} \left[ \sum \limits_{t=0}^\infty \gamma^t \, r\tick(a_t,s_t) \right]
% \label{eq:reward_perturbation_stmt}
% \end{align}






% \newcommand{\WidthS}{.22\textwidth}
% \newcommand{\WidthM}{.25\textwidth}
% \newcommand{\WidthMM}{.27\textwidth}
% \newcommand{\HeightS}{30mm}
% \newcommand{\HeightM}{30mm}

\newcommand{\WidthS}{.2\textwidth}
\newcommand{\WidthM}{.22\textwidth}
\newcommand{\WidthMM}{.25\textwidth}
\newcommand{\HeightS}{20mm}
\newcommand{\HeightM}{20mm}

\hspace*{-.2cm}
\begin{figure*}[t]
\centering
\begin{minipage}{.48\textwidth}
% \begin{subfigure}
%\def\arraystretch{2.2}
%  \subcaptionbox{Optimal Policy \label{fig:perturb_opt_a}}{
\[\arraycolsep=.005\textwidth
\begin{array}{cccc} %[width=40mm]
%\begin{subfigure}{.16\columnwidth}
 & \multicolumn{3}{c}{\text{(i) }\beta = 0.1} \\[.5ex]
\multirow{3}{\WidthMM}{\includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/env.png} \\[4ex] \includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/opt_agent.png}} &
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta01policy_opt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta01perturb_opt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta01perturbed_opt.png}  \\[.25ex]
 & \multicolumn{3}{c}{\text{(ii) }\beta = 1.0} \\[.5ex]
%\caption{\centering \small $D_{KL}, \beta = 10$}\label{fig:tabc}\end{subfigure}&\hspace*{.2cm}\\
& % NEXT LINE for multi-row
%\includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/opt_agent.png} &
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta1policy_opt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta1perturb_opt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta1perturbed_opt.png} \\[.25ex]
 & \multicolumn{3}{c}{\text{(iii) } \beta = 10} \\[.25ex]
&
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta10policy_opt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta10perturb_opt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta10perturbed_opt.png} 
% \\[.25ex]
\end{array}
\]
 %\hspace*{0.25cm}
% \label{subfig:subfig}
% \caption{Optimal Policy }\label{fig:perturb_opt_a}
% \end{subfigure}
\end{minipage}\hspace{.02\textwidth} %{\quad \vline width 1pt}&
%&\\[2ex] \midrule
\begin{minipage}{.48\textwidth}
% \begin{subfigure}{.48\textwidth}
% \subcaptionbox{Suboptimal Policy \label{fig:perturb_subopt_b}}{
\[\arraycolsep=.005\textwidth
\begin{array}{cccc} %[width=40mm]
%\begin{subfigure}{.16\columnwidth}
 & \multicolumn{3}{c}{\text{(i) } \beta = 0.1} \\[.5ex]
\multirow{3}{\WidthMM}{\includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/env.png} \\[4ex] \includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/agent.png}} &
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta01policy_subopt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta01perturb_subopt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta01perturbed_subopt.png}  \\[.25ex]
 & \multicolumn{3}{c}{\text{(ii) } \beta = 1.0} \\[.5ex]
%\caption{\centering \small $D_{KL}, \beta = 10$}\label{fig:tabc}\end{subfigure}&\hspace*{.2cm}\\
& % NEXT LINE for multi-row
%\includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/agent.png} &
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta1policy_subopt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta1perturb_subopt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta1perturbed_subopt.png} \\[.25ex]
 & \multicolumn{3}{c}{\text{(iii) } \beta = 10} \\[.5ex]
&
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta10policy_subopt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta10perturb_subopt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta10perturbed_subopt.png} \\[.25ex]
\end{array}
\]
% }
\end{minipage}
\caption{Suboptimal Policy} \label{fig:perturb_subopt_b}
% \end{subfigure}
\caption{ Single-Step Reward Perturbations.  $Q$-values in leftmost columns are used for each $\beta$ in columns 2-4.  
We report the optimal $-\pr(a,s)$, so that values less than 0 are subtracted in the objective $\langle \pi_Q(a|s), r(a,s) - \pr(a,s) \rangle + \alphaconju(\pr)$.
In (a), we show the optimal policy ($Q(a,s) = r(a,s)$), where the  perturbed reward $r^{\prime}(a,s) = c \, \, \forall a$ reflects the indifference condition.  We also show a suboptimal policy in (b), where indifference does not hold.  In all cases, actions with high $Q(a,s)$ are robust to subtracted perturbations. }\label{fig:perturb_opt}
\end{figure*}



\section{Discussion}\label{sec:discussion}
%In light of the above results, 
What insights can be obtained from this adversarial interpretation of regularized policies?
%Ultimately, what insight is provided by this adversarial reward robustness interpretation of regularized policies?
%What implications do the above results have for our adversarial reward robustness interpretation of regularized policies?]
%Our results in the previous section indicate a very particular form of robustness, which has a natural game-theoretic interpretation. %\citep{ortega2014adversarial}.  
%The results of the previous section indicate a very particular form of robustness which has a natural game-theoretic interpretation \citep{ortega2014adversarial}.
In \ref{sec:generalization}, we discuss the generalization properties associated with this robustness, which we highlight is particularly sensitive to the form of the objective in \ref{sec:entropy_vs_div}.
%However, as we argue below, this may not directly align with desired notions of robustness as zero-shot generalization to unseen environments.
%However, this robustness is particularly sensitive to the form of the objective, as discussed in \mysec{entropy_vs_div}.   
%may not directly align with desirable notions of zero-shot generalization to unseen environments \TG{This needs a bit of unpacking - do you mean that we can't say anything about unseen environments because we don't know the dynamics/reward function? I would argue that we can at least say something about unseen environments where the reward has been perturbed according to the feasible set - which is actually quite a nice statement I think.} and, as we discuss in \mysec{entropy_vs_div}, is sensitive to the form of the objective.
%particularly sensitive to the form of the objective.
%and is particularly sensitive to the form of the objective, as discussed in \mysec{entropy_vs_div}.   
We draw connections with the notion of path consistency \citep{nachum2017bridging, chow2018path} in \ref{sec:modified}, and argue that  adversarial reward perturbations can provides a natural justification for including $Q$-values as dual variables in \gls{LP} formulations of \gls{MDP}s in \ref{sec:qlp}.
%\RB{Add generalization analysis}
%\RB{Add reward $\rightarrow$ robustness vs. policy $\rightarrow$ robustness}

\subsection{Relationship to Generalization}\label{sec:generalization}
%For our purposes, we consider `zero-shot generalization' of a given policy $\pi(a|s)$ to an environment with a modified reward function $\mr(a,s)$ to mean that
Our adversarial interpretations imply robustness or generalization of a given policy $\pi(a|s)$ to an environment with a modified reward $\mr(a,s)$ in the sense that, for given \gls{MDP} transition dynamics
\scriptsize
\begin{align}
  \hspace*{-.3cm} \langle \mu(s) \pi(a|s), \mr(a,s) \rangle \geq \langle \mu(s) \pi(a|s), r(a,s) \rangle - \langle \mu(s), \frac{1}{\beta} \Omega_{\pi_0}(\pi) \rangle \, \label{eq:robust_def}
   %\blangle \mu(s) \pi(a|s), \mr(a,s) \brangle \geq  \blangle \mu(s) \pi(a|s), r(a,s) - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \brangle \, . \label{eq:robust_def}
\end{align}
\normalsize
%Our adversarial interpretations imply robustness or generalization of a given policy $\pi(a|s)$ to a modified reward function in this particular sense.   
%Notice that 
where the right hand side corresponds to the full objective function, including regularization, whereas the left hand side is only the expected reward.
 %the regularized objective $\mathcal{R}_{\Omega, \beta}(r\tick) \geq \mathcal{R}_{\Omega, \beta}(r\tick)$
The constraints in \myprop{perturbations}-\ref{prop:perturbations_alpha} characterize the robust set of modified rewards to which a given policy can generalize, as visualized in \cref{fig:feasible_set_main}.   Since these constraints integrate over the action space, note that the rewards for all actions in a particular state must be perturbed together.

By running a fixed policy in an environment with higher rewards, we naturally expect the objective function to increase.   However, for useful zero-shot generalization, we might hope that a policy will still perform well when the reward function decreases in at least some states.    
%In the next subsection, we 
In the next subsection, we discuss how these qualitative properties can depend on the form of the regularization function $\frac{1}{\beta} \Omega_{\pi_0}(\pi)$ in \cref{eq:robust_def}. %can impact these qualitative.
%of the reward robustness \cref{eq:robust_def} and their sensitivity to the form of the regularization function .
%Using the expression in \cref{eq:perturb_opt_q}, we can see that a regularized policy will be robust to negative changes in the reward function when
%$\frac{\pi(a|s)}{\pi_0(a|s)} \lessgtr 1$ or difference $Q(a,s) - \alphanorm \lessgtr 0$.  


%As observed above, entropy regularization can only provide robustness to reward increases $-\pr \geq 0$ and objective values $\alphaconjn$ which are higher than the environment rewards.  
%For useful generalization to unseen environments, we are usually 



\subsection{Comparison with Entropy Regularization }\label{sec:entropy_vs_div}
% \paragraph{Dual Representations} The equivalence of the objectives in \cref{eq:reward_perturbation_stmt} %\citep{eysenbach2021maximum} 
% is trivially confirmed for the optimal $\dualvar_*(a,s) = r(a,s) - \frac{1}{\beta} \ptReg(\pi(a|s)) = r(a,s) - \frac{1}{\beta} \propt(a,s)$ (\RB{This is wrong and unresolved.  Only true of KL div, otherwise $\frac{1}{\beta} \ptReg(\pi(a|s)) = \frac{1}{\beta} \frac{1}{\alpha} \propt(a,s)$ factor}), which is not surprising given that our derivations only invoked an alternative representation of $\Omega_{\tpi_0}(\tpi)$ via convex duality.   This duality is also reflected in the fact that we can represent the optimal reward perturbations, or a stochastic policy itself, in terms of either probabilities $\pi(a|s)$ or dual variables $Q(a,s)$ for a given $\Omega$, $\pi_0$, and $\beta$.  
% %representations of a stochastic policy in terms of probabilities $\pi(a|s)$ or dual variables $Q(a,s)$
%As the indifference condition for optimal policies highlights, the adversarial reward perturbations preserve the value of the objective in each state.   We further explore this sensitivity of the reward perturbations to the form of objective function below.

%{\paragraph{Entropy vs. Divergence}}
%Our use of the \textsc{kl} and} $\alpha$-divergences, instead of the corresponding entropic quantities, resolves several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}.   Regularizing with the Tsallis or Shannon ($\alpha = 1$) entropy, the optimal perturbations are %perturbed reward is %reward
When regularizing with the Tsallis or Shannon ($\alpha = 1$) entropy, the optimal reward perturbations become %perturbed reward is %reward
\begin{align}
    \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \pi(a|s) \,. \label{eq:ptwise_perturb_ent}
\end{align}
%For entropy regularization, 
We argue the pointwise non-negative contribution of these perturbations to the objective $r(a,s) - \propt(a,s)$, with $-\propt(a,s) \geq 0$ for $\pi(a|s) \leq 1$, leads to several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}, which are resolved by our use of the \textsc{kl} and $\alpha$-divergences instead of the entropic quantities.   In particular, entropy regularization should be considered as a divergence to the uniform reference distribution $\pi_0(a|s)$ over actions.
%Our use of the \textsc{kl} and} $\alpha$-divergences, instead of the corresponding entropic quantities, resolves several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}.   

First, this means that an entropy regularized policy is only `robust' to \textit{increases} in the reward function.  
%This can be corrected when 
Including the reference distribution as in \myprop{perturbations}(b) and \cref{fig:perturb_opt} changes this property, so that the optimal reward perturbation $\propt(a,s) = \frac{1}{\beta}\log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}$ %\frac{\pi(a|s)}{ \pi_0(a|s)}$ %
yields robustness to reward \textit{decreases} when $\pi(a|s) > \pi_0(a|s)$ and reward increases otherwise.  

%After taking the expectation over actions, note that subtracting a non-negative \textsc{kl} divergence yields a smaller quantity than the unregularized objective, whereas subtracting the negative entropy yields a larger quantity.

%adding the entropy gives a larger quantity.

%The possibility of both reward increases and decreases also clarifies constraints on the feasible set.   
%Nevertheless, as the indifference condition for optimal policies suggests, the role of these perturbations is simply to re-express the value of the objective function in each state.

%which can be corrected by including the reference distribution $\pi_0(a|s)$ as in our results from the previous section.

%Although divergences and entropies are both non-negative in expectation, we argue that explicitly including the reference distribution is crucial to 
%which matches \cref{eq:optimal_perturbed} for uniform $\pi_0(a|s)$.   




% These observations stem from the fact that the Shannon or Tsallis entropy is a pointwise non-negative quantity.
Similarly, \citet{lee2019tsallis} note that %$\frac{1}{\beta}\Omega^{*}_{\pi_0}(\discussiondual) = \max_{\pi(a|s)} \langle \pi(a|s), \discussiondual(a,s) \rangle + \frac{1}{\beta} H_{\alpha}(\pi) \geq \discussiondual(a_{\max}, s) $
\small
\begin{align*}
    \frac{1}{\beta}\Omega^{*(H_{\alpha)}}_{\pi_0}(\discussiondual) = %\max_{\pi(a|s)}
    \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \langle \pi, \discussiondual \rangle - \left(-\frac{1}{\beta} H_{\alpha}(\pi)\right) \geq \discussiondual(a_{\max}, s) 
\end{align*}
\normalsize
where $a_{\max} = \argmax_a \discussiondual(a,s)$ and the Tsallis entropy $H_{\alpha}(\pi)$ equals the Shannon entropy for $\alpha = 1$.  
%Due to the non-negativity of the pointwise entropy, 
This soft value aggregation, using the negative (Tsallis) entropy as a regularizer,  yields a value which is \textit{larger} than any particular reward. 
%so that soft value aggregation yields a value which is \textit{larger} than any particular reward. 
% \begin{align}
%     \max_{\pi(a|s)} \langle \pi(a|s), \discussiondual(a,s) \rangle + \beta H_q(\pi) \geq \max_a \discussiondual(a,s)
% \end{align}
% where $H_q$ is the Tsallis entropy.
By contrast, for the $\alpha$-divergence, we show in \myapp{qmax} that
\small
\begin{align*}
   \discussiondual(a_{\max},s) + \frac{1}{\beta} \log_{\alpha} \frac{ \pi(a_{\max}| s)}{\pi_0( a_{\max}| s)} \leq \alphaconjn(\discussiondual) \leq  \discussiondual(a_{\max},s)
   %\leq  \alphaconjn(\discussiondual) \leq \max_a \discussiondual(a,s) % \max \limits_{a \in \mathcal{A}} \discussiondual(a_{\max},s)
%     \discussiondual(a_{\max},s) \geq \alphaconjn(\discussiondual) \geq \begin{cases}  \discussiondual(a_{\max},s) -  \frac{1}{\alpha-1} \big( \frac{\pi(a_{\max} | s)}{\pi_0(a_{\max}|s)}^{\frac{1}{\alpha-1}} - 1 \big) \hfill \alpha \neq 1 \\
%   \discussiondual(a_{\max},s) - \log \frac{ \pi(a_{\max}| s)}{\pi_0( a_{\max}| s)}  \hfill \alpha =1 \end{cases}  
%   %\leq  \alphaconjn(\discussiondual) \leq \max_a \discussiondual(a,s) % \max \limits_{a \in \mathcal{A}} \discussiondual(a_{\max},s)
\end{align*}
\normalsize
This provides a more natural interpretation of $V(s) =  \alphaconjn(Q)$ as a soft maximum function, with $ \mathbb{E}_{\pi_0}[\discussiondual(a_{\max},s)] \leq V(s) \leq \discussiondual(a_{\max},s)$ as in \cref{fig:perturb_opt}.


Finally, entropy regularization also affects interpretations of the feasible set.  %For entropy regularization,
\citet{eysenbach2021maximum} consider the same constraint as in \myprop{perturbations}, but without considering the reference distribution
\begin{align}
    \sum \limits_{a} \expof{\beta \cdot \pr(a,s)} \leq \sum \limits_{a} \pi(a|s)  \, \, \, \forall s \in \mathcal{S} \, . \label{eq:ent_constraint}
\end{align}
This constraint suggests that the original reward function ($\pr = 0$) is not feasible for the adversary, unless the policy is deterministic.  More surprisingly, \citet{eysenbach2021maximum} App. A5 argues that \textit{increasing} regularization strength may lead to \textit{less} robust policies based on the constraint in \cref{eq:ent_constraint}.    In \myapp{eysenbach}, we discuss how including $\pi_0(a|s)$ in the constraint via divergence regularization modifies this conclusion.   As expected, we observe in \cref{fig:feasible_set_main} that increasing regularization strength leads to more robust policies.


% \RB{Need to further investigate.  What is Fig. 7 (left) of \citet{eysenbach2021maximum} showing?  }
% Further, \citet{eysenbach2021maximum} App. A5 observe that \textit{increasing} the regularization strength leads to \textit{less} robust policies, with \textit{smaller} feasible sets for the adversary.  With Shannon entropy regularization, the constraint in \myprop{perturbations}(a) becomes
% %For Shannon entropy regularization, the analogous constraint to \myprop{perturbations}(a) is
% \begin{align}
%     \sum \limits_{a} \expof{\beta \cdot \pr(a,s)} \leq \sum \limits_{a} \pi(a|s)  \, \, \forall s \in \mathcal{S} 
% \end{align}
% Restricting attention to $\pr(a,s) < 0$ based on \cref{eq:ptwise_perturb_ent}, \citet{eysenbach2021maximum} conclude that the 

% %To understand this, note that the feasible constraint 

% This is a surprising conclusion, as we would expect regularization to improve robustness, and \cref{fig:feasible_set_main} shows that this is indeed the case when regularizing using divergences rather than entropies.   


% While \citet{eysenbach2021maximum} display feasible sets arising from (negative) Shannon entropy regularization $\Omega(\pi) = - H(\pi)$, this approach leads to puzzling conclusion that \textit{lower} regularization strength $1/\beta$ leads to \textit{greater} adversarial robustness, with larger feasible sets.   
% In contrast to \cref{eq:optimal_perturbed}, the entropy-regularized policy is `robust' to only positive changes in the reward function $\pr(a,s) \geq 0$, with the optimal perturbed reward $\mr(a,s) = r(a,s) - \pr(a,s) = r(a,s) - \log \pi(a|s)$.   We also observe robustness to large positive reward perturbations for low regularization strength in \cref{fig:perturb_opt}, but the crucial negative reward perturbation arises for the action(s) in the support of the nearly deterministic policy.
% We prefer to characterize `robustness' in terms of \textit{reductions} to the reward function

%sensitivity to the value of objective function


% 

==> Reward Robustness TMLR (3)/old/3_modified.tex <==
\subsection{Adversarial Modified Rewards}\label{sec:modified}
The adversarial interpretation in the previous sections may also be written directly using the modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$, which has been studied in a more general setting by \citet{husain2021regularized}.

%We briefly describe this perspective for the policy regularization case, drawing connections with path consistency learning \citep{nachum2017bridging, chow2018path} and logistic $Q$-learning \citep{basserrano2021logistic}.

%\paragraph{Modified Reward Interpretation}
\citet{husain2021regularized} consider maximizing an arbitrary concave objective $\concaveopt$, and proceed to derive its convex conjugate $(-\concaveopt)^*$.    Translated to our setting and notation,
this involves the conjugate expansion of the regularized objective $(-\mathcal{R}_{\Omega, \beta}(r))^*$ instead of the conjugate of the regularizer $ (\frac{1}{\beta} \Omega_{\pi_0}(\pi))^*$ only.  
With detailed derivations in \myapp{husain_conjugate}, this leads to the Lagrangian
\begin{align}
    \hspace*{-.2cm} & \quad \max \limits_{\mu(s) \rightarrow \mathcal{M}} \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s)} \min \limits_{\textcolor{\highlight}{\mr(a,s)}} \, \label{eq:husain_form} \\
    & \big \langle {\mu(s)\pi(a|s)}, {\textcolor{\highlight}{\mr(a,s)} +\gamma \transitionv - V(s) } \brangle  \nonumber  \\
    & \quad+ \frac{1}{\beta} \Omega^{*}_{\textcolor{red}{\tpi_0}, \beta} \big( r(a,s) - \textcolor{\highlight}{\mr(a,s)} \big) + (1-\gamma) \blangle \nu_0(s), V(s) \brangle \, ,  \nonumber
\end{align}
which matches \cref{eq:pedro_form} up to simple reparameterization of $\mr(a,s) = r(a,s) - \pr(a,s)$.

\paragraph{Optimal Modified Rewards}
%In \myapp{perturb_husain}, we show
Differentiating \cref{eq:husain_form} with respect to $\pi(a|s)$ and solving for the optimal modified rewards yields the result of \citet{husain2021regularized} that
\begin{align}
   \mropt(a,s) = V(s) - \gamma \transitionv  %\quad \forall (a,s) \in (\mathcal{A}, \mathcal{S})
\end{align}
%The optimal modified rewards from \citet{husain2021regularized} %match our \cref{eq:optimal_perturbed} up to reparameterization
%\citet{husain2021regularized} interpret this modified reward as `relating the rewards between states through the dynamics of $P(s\tick|s,a)$'.
%Consider the Bellman backup or \textsc{td}-0 error $r(s,a) + \gamma \transitionv - Q(a,s)$
Adding the environment reward, we can use the optimal reward perturbations $\propt(a,s) = r(a,s) - \mropt(a,s)$ to rewrite this expression
% \begin{align}
%   \hspace*{-.2cm} r(a,s) - \mr(a,s) &=  r(a,s) + \gamma \transitionv -  V(s) 
% \end{align}
% \RB{what about cases other than the KL divergence?  }
% which suggests
\begin{align}
\propt(a,s) &=  r(a,s) + \gamma \transitionv -  V(s) \label{eq:modified_reward_opt}
\end{align}
\normalsize
\textcolor{red}{This seems problematic because we would write $\pr(a,s) = Q(a,s) - \psi_{\alpha}(s;\beta)$ for $\alpha$-divergence minimization, with $\psi_{\alpha}(s;\beta) \neq V(s)$.  
}\RB{Think I can fix this}


\paragraph{Connection with Path Consistency}
For the \textsc{kl} divergence regularization, \citet{nachum2017bridging} use the \textsc{kkt} conditions to show that the optimal policy satisfies \textit{path consistency} equations, which follow directly from the adversarial rewards in \cref{eq:modified_reward_opt} using \myprop{perturbations}.   In particular,
\begin{align}
    r(a,s) - \underbrace{\frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)}}_{\propt(a,s)} = V(s) - \gamma \transitionv 
    %\, \, \forall s \in \mathcal{S}, a \in \mathcal{A}
\end{align}
for all $s \in \mathcal{S}, a \in \mathcal{A}$.

Generalizing the path consistency equation shown in \citet{chow2018path} for the Tsallis entropy with $\alpha =2$, we can write
% of \citet{chow2018path} for the Tsallis entropy with $\alpha = 2$ into our notation, the path consistency condition  corresponds to 
% Adapting the result of \citet{chow2018path} for the Tsallis entropy with $\alpha = 2$ into our notation, the path consistency condition  corresponds to 
%For the Tsallis entropy with $\alpha=2$, \citet{chow2018path} obtain the following path consistency equation
\begin{align}
r(a,s) - \underbrace{\frac{1}{\beta}\log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)}}_{\propt(a,s)} &= V(s) - \gamma \transitionv + \Lambda(s)  \label{eq:path1}
\end{align}
where $\Lambda(s) = \normalizerexp - V(s)$ is a Lagrange multiplier which can be seen as accounting for the fact that $\normalizerexp \neq V(s)$ for $\alpha \neq 1$.
Finally, we are left with
\begin{align}
    r(a,s) + \gamma \transitionv - \propt(a,s) = \normalizeralpha   \label{eq:path}
\end{align}
which matches our condition $\pr(a,s) = Q(a,s) - \normalizeralpha$. 
With detailed derivations in \cref{app:path_consistency}, we show that the optimal $\alpha$-divergence regularized policy satisfies the path consistency condition in \cref{eq:path1}, which generalizes the result of \citet{chow2018path} from $\alpha=2$ to general $\alpha$.


These optimality conditions mirror the equilibrium indifference condition from \cref{sec:value_based}, where the quantity $Q(a,s) - \propt(a,s) = r(a,s) + \transitionv -\propt(a,s) = c(s)$ equals a constant for all $a \in \mathcal{A}$.




==> Reward Robustness TMLR (3)/old/5_discussion.tex <==
\subsection{$Q$-Value Relaxations}\label{sec:qlp} \label{sec:logisticq}
\RB{Likely to be cut}
% \citet{husain2021regularized} suggest that a link between policy regularization and alternative Bellman aggregation errors.
% Similar observations have been made in the context of offline learning \citep{nachum2020reinforcement} and \gls{REPS} \citep{basserrano2021logistic}.

Among the most intriguing observations in \citet{husain2021regularized} is to relate the adversarial reward perturbation $\pr(a,s) = r(a,s) - \mr(a,s)$ to the \textsc{td}-\textsc{0} or Bellman backup error.   Similar observations have been made in the context of offline learning \citep{nachum2020reinforcement} and \gls{REPS} \citep{belousov2019entropic, basserrano2021logistic}.

However, these works require modifications to the \gls{LP} to incorporate $Q$-values, 
which is necessary since the objective in \cref{eq:dual_reg} involves $V(s)$ instead of $Q(a,s)$ as in the \textsc{td}-\textsc{0} error.
Previous work has considered a non-standard `$Q$-\textsc{lp}' \citep{nachum2020reinforcement} or introduced redundant constraints in a relaxed \gls{LP} \citep{mehta2009q, mehta2020convex, lee2019stochastic, basserrano2021logistic}. 
The latter approach considers augmenting the flow constraints with a second distribution $d(a,s)$
%One way to incorporate $Q$-values into linear or convex programming formulations of \gls{MDP}s is to consider augmenting the flow constraints with a second distribution $d(a,s)$
\begin{align}
   d(a,s) &= \mu(a,s) \label{eq:d_flow} \\
   \sum_{a} d(a,s) &= (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \nonumber
\end{align}

In \myapp{relaxed_lp}, we argue that the introduction of dual variables $\mr(a,s)$ or $\pr(a,s)$ via the convex conjugate function % of the regularizer, 
may provide an alternative justification for this relaxed \textsc{lp}.   In particular,  by further expanding the term $\Omega^{*}(\pr(a,s))$ in \cref{eq:pedro_form} using the conjugate optimization $ \max_d \langle d(a,s), \pr(a,s) \rangle - \Omega(d)$, we can obtain
%is a natural way to include 
a second state-action visitation distribution $d(a,s)$ or a second policy $d(a|s)$ with a fixed $\mu(s)$   
\small 
\begin{align}
    \hspace*{-.2cm} & \quad \max \limits_{\mu(s) \rightarrow \mathcal{M}} \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s)} \min \limits_{\textcolor{\highlight}{\perturbr(a,s)}} \max \limits_{\textcolor{\highlight}{d(a,s)}} \, \label{eq:relaxed_lp_form} \\
    & \big \langle {\mu(s)\pi(a|s)}, {r(a,s) +\gamma \transitionv - V(s) - \textcolor{\highlight}{\perturbr(a,s)}} \brangle  \nonumber  \\
    &+ (1-\gamma) \blangle \nu_0(s), V(s) \brangle + \blangle \mu(s) \textcolor{\highlight}{d(a|s)}, \textcolor{\highlight}{\pr(a,s)}- \frac{1}{\beta} \Omega_{\pi_0}(\textcolor{\highlight}{d})  \brangle \, .  \nonumber
\end{align}
\normalsize
We can make several observations from this objective.  First, differentiating with respect to $\pr(a,s)$ yields the condition that $d(a|s) = \pi(a|s)$ from \cref{eq:d_flow}, with the second constraint following directly.  
Further, for \textsc{kl} divergence regularization, substituting $\pr(a,s) = Q(a,s) - V(s)$ yields the desired \textsc{td-0} error $r(a,s) +\gamma \transitionv - Q(a,s)$.
%, which we have shown are related to $Q(a,s)$ value estimates, may provide more 
We provide an alternative derivation of the Lagrangian for Logistic $Q$-learning \citep{basserrano2021logistic} in \myapp{logistic_q}, but leave further exploration, such as extending the primal dual algorithm of \citet{lee2019stochastic} to the regularized case, for future work.  

%For example, the stochastic primal-dual algorithm of \citet{lee2019stochastic} might be extended to the regularized case.  
%However, note that policy regularization
%We do not expect the approach of Logistic $Q$-learning  \citep{basserrano2021logistic}, 
%\citet{lee2019stochastic} primal dual , working with the Lagrangian

==> Reward Robustness TMLR (3)/old/6_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this work, we have analyzed the robustness of convex-regularized \gls{RL} policies to adversarial perturbations of the reward function.   This robustness can be given a natural game-theoretic interpretation, in which the equilibrium indifference condition for the optimal policy highlights that the adversarial perturbations re-express the value of the objective function.  
Furthermore, policy regularization alone implies generalization to worst-case reward functions chosen within a particular robust set.
We have characterized the robust set of reward functions for \KL and $\alpha$-divergence regularization, and resolved apparent differences in robustness properties arising from entropy versus divergence regularization.   Our analysis integrates several existing works on adversarial robustness, and highlights how convex conjugate representations can provide additional insight into regularization in \gls{RL}.    


Among the most intriguing observations in \citet{husain2021regularized} is to relate the adversarial reward perturbation $\pr(a,s) = r(a,s) - \mr(a,s)$ to the \textsc{td}-\textsc{0} or Bellman backup error.   Similar observations have been made in the context of offline learning \citep{nachum2020reinforcement} and \gls{REPS} \citep{belousov2019entropic, basserrano2021logistic}.
%  Translating these insights into algorithmic improvements remains for future work. 
 Extending recent work on alternative Bellman error aggregation \citep{dai2018sbeed, nachum2020reinforcement, belousov2019entropic, basserrano2021logistic} to policy regularization settings, 
% \textcolor{red}{actor-critic / soft $Q$}
% or soft $Q$-learning
potentially using $\alpha$-divergence regularization or learned reference distributions \citep{grau2018soft, galashov2018information}, remains an intriguing direction for future work.

% Translating these insights into algorithmic improvements remains for future work.   Intruiging directions include adapting the primal-dual \gls{RL} algorithm of \citet{lee2019stochastic} to the regularized setting, or extending recent work on alternative Bellman error aggregation \citep{dai2018sbeed, nachum2020reinforcement, belousov2019entropic, basserrano2021logistic} to
% policy regularization settings, 
% % \textcolor{red}{actor-critic / soft $Q$}
% % or soft $Q$-learning
% potentially using learned reference distributions \citep{teh2017distral, grau2018soft} and $\alpha$-divergence regularization. %\citep{dai2018sbeed, nachum2020reinforcement, basserrano2021logistic}
%In particular, we have shown how stochastic policies %While the objective function for an unregularized, deterministic policy depends only on the value of the optimal action, stochastic policies crucially depend on $Q$ values across all actions and correspond to impli




% In this work, we have provided an integrated analysis of 
% previous work which interprets regularized policies as providing robustness to adversarial reward perturbations \TG{Don't put the emphasis on unifying previous work. Rather say that we provided an analysis of the robustness and generalization arising from regularized policies. Then mention and discuss the main findings. And then only say that this unifies/integrates previous work along the same interpretations.}.   These interpretations arise from dual representations of a convex regularization function $\Omega_{\pi_0}(\pi)$ in terms of its conjugate function $\Omega^{*}_{\pi_0}(\pi)$, with the reward perturbations $\pr(a,s)$ as dual variables.   
% For a given regularization function and strength, this matches the duality between a stochastic policy and the estimated $Q$-values of an agent, so that adversarial reward perturbations represent a natural justification for including $Q$-values in convex programming formulations of \gls{RL}.  
% We hope that these observations will be useful to further develop and understand \gls{RL} algorithms using convex duality. \TG{Ok, but the main findings/takeaways are missing! What do we conclude about the nature of the robustness that we get from policy regularization? How does it relate to the adversarial interpretation (and the indifference principle)? Comment on maxent vs. KL vs. alpha-div regulariztion. What have we seen from looking at the feasible set?}





==> Reward Robustness TMLR (3)/old/7_pyco.tex <==
\section{Visualizations}\label{sec:visualizations}
\begin{figure*}[t]
\begin{subfigure}{.2\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_world.pdf}\vspace*{.2cm}
\caption{Environment \\
($r(a,s) = -1$ for water, \\
$r(a,s) = 5$ for goal) \label{fig:pyco_env}}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta02_alpha1_gamma99.pdf}
\caption{$\beta = 0.2$ (High Reg.)}\label{fig:pyco_beta02}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta1_alpha1_gamma99.pdf}
\caption{$\beta = 1$}\label{fig:pyco_beta1}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta10_alpha1_gamma99.pdf}
\caption{$\beta = 10$ (Low Reg.)}\label{fig:pyco_beta02}
\end{subfigure} 
% \\
% \begin{subfigure}{.2\textwidth}
% \end{subfigure}
% \begin{subfigure}{.26\textwidth}
% \includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta02_alpha1_gamma99_perturbed.pdf}
% \caption{$\beta = 0.2$ (High Reg.)}\label{fig:pyco_beta02}
% \end{subfigure}
% \begin{subfigure}{.26\textwidth}
% \includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta1_alpha1_gamma99_perturbed.pdf}
% \caption{$\beta = 1$}\label{fig:pyco_beta1}
% \end{subfigure}
% \begin{subfigure}{.26\textwidth}
% \includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta10_alpha1_gamma99_perturbed.pdf}
% \caption{$\beta = 10$ (Low Reg.)}\label{fig:pyco_beta02}
% \end{subfigure}
\caption{\label{fig:pyco} Optimal adversarial reward perturbations $\propt(a,s) = \frac{1}{\beta}\log \frac{\pi(a|s)}{ \pi_0(a|s)}$ for a sequential setting. Policy trained with \textsc{kl} divergence regularization,  $\gamma$ = 0.99.  Red indicates robustness to negative reward perturbations.}
\end{figure*}

\begin{figure*}[t]
\begin{subfigure}{.2\textwidth}
\phantom{\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_world.pdf}\vspace*{.2cm}}
% \caption{\centering Environment \\
% ($r(a,s) = -1$ for water, \\
% $r(a,s) = 5$ for goal)}\label{fig:pyco_env}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta02_alpha1_gamma99_perturbed.pdf}
\caption{$\beta = 0.2$ (High Reg.)}\label{fig:pyco_beta02}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta1_alpha1_gamma99_perturbed.pdf}
\caption{$\beta = 1$}\label{fig:pyco_beta1}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta10_alpha1_gamma99_perturbed.pdf}
\caption{$\beta = 10$ (Low Reg.)}\label{fig:pyco_beta02}
\end{subfigure}
\caption{\label{fig:pyco} Perturbed rewards $\mr(a,s) = r(a,s) - \pr(a,s)$ for policies trained with \textsc{kl} divergence regularization.  The indifference condition holds in all cases, with $\mr(a,s) = c(s)$ for each action, and at each state and $c(s) = V(s)$ for \textsc{kl} regularization.  This confirms that the policy is optimal \citep{ortega2014adversarial, nachum2017bridging}.}
\end{figure*}

==> Reward Robustness TMLR (3)/sections/conj_table.tex <==
%%%%% Contains all possibilities
% \begin{figure*}[t]
% \resizebox{\textwidth}{!}{
% \centering
% \small

%         \begin{tabular}{lllll}
%     \toprule
%     %   \multicolumn{2}{c}{Regularization} &  \multicolumn{2}{c}{Conjugate} \\[0.25ex]
%     %   Notation &  Expression  &  Notation &  \multicolumn{1}{c}{Expression} \\
% %  \text{Regularizer} 
%  \multicolumn{2}{c}{  Divergence } & 
%   Conjugate & 
% \multicolumn{1}{c}{Conjugate Expression} 
%  & Optimizing $\pi_{\pr}(a|s)$ or $\mu_{\pr}(a,s)$
%  \\
% %   [1.5ex]
% %         % \multicolumn{2}{c}{Conjugate} \\
%         \midrule
%         % \frac{1}{\beta} \Omega_{\pi_0}(\mu) &
%     $\frac{1}{\beta} \Omega_{\pi_0}(\mu) 
%     % =$  
%      $&    
%     $\frac{1}{\beta} \KL[\pi:\pi_0]$ & $\frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(\pr)$ 
%     % $=$ 
%     & 
%         %  $\sum \limits_{a \in \mathcal{A}} 
%          $\frac{1}{\beta} \sum \limits_{a} 
%          \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} - 
%         %  \sum \limits_{a \in \mathcal{A}} 
%          \frac{1}{\beta} \sum \limits_{a} 
%          \pi_0(a|s)$ 
%          & $ \pi_0(a|s) \expof{\beta \cdot \pr(a,s)}$
%          \\[1.5ex]
%         % \frac{1}{\beta} \frac{1}{\beta} \Omega_{\mu_0}(\mu) &
%      $\frac{1}{\beta} \Omega_{\mu_0}(\mu)
%     %  =$
%      $ &    
%      $\frac{1}{\beta} \KL[\mu:\mu_0]$ & $\frac{1}{\beta} \Omega^{*}_{\mu_0,\beta}(\pr)$  
%       &
%     %  $=$
%      $\frac{1}{\beta} \sum \limits_{a,s}% \in \mathcal{A} 
%         %  \sum \limits_{a,s \in \mathcal{A}, \mathcal{S}}
%          \mu_0(a,s) \expof{\beta \cdot \pr(a,s)} - 
%         \frac{1}{\beta} \sum \limits_{a,s} 
%         %  \sum \limits_{a,s \in \mathcal{A}, \mathcal{S}}
%          \mu_0(a,s)$  
%           & $ \mu_0(a,s) \expof{\beta \cdot \pr(a,s)}$ 
%          \\[1.5ex]
%         %  \alphaomegapi & 
%          $\frac{1}{\beta} \Omega^{(\alpha)}_{\pi_0}(\mu)
%     %  =$
%       $ &   
%     $\frac{1}{\beta} D_{\alpha}[\pi_0:\pi]$ & $\frac{1}{\beta} \Omega^{*(\alpha)}_{\pi_0,\beta}(\pr)$  
%      &
%     %  $=$
%      \footnotesize $\frac{\alpha-1}{\alpha}\blangle \mu(s)\pi_{\pr}(a|s), \pr(a,s) \brangle + \frac{1}{\alpha} \psi_{\pr}$
%         &
%         $\pi_0(a|s) \exp_{\alpha} \big\{\beta \cdot \pr(a,s) - \psi_{\pr} \big\}$
%         \\[1.5ex] \midrule
%      $\frac{1}{\beta} \Omega^{(\alpha)}_{\pi_0}(\mu)
%     %  =$
%       $ &   
%     $\frac{1}{\beta} D_{\alpha}[\pi_0:\pi]$ & $\frac{1}{\beta} \Omega^{*(\alpha)}_{\pi_0,\beta}(\pr)$  
%      &
%     %  $=$
%     \footnotesize $ \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \mu(s) \pi_0(a|s)^{1-\alpha}\pi_{\pr}(a|s)^{\alpha} -  \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \mu(s) \pi_0(a|s) $ 
%     %  \footnotesize $\frac{\alpha-1}{\alpha}\blangle \mu(s)\pi_{\pr}(a|s), \pr(a,s) \brangle + 
%     %     \textcolor{red}{\frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \pi_0 \exp_\alpha{\beta \pr} -  \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \pi_0 }$        
%         %  \frac{1}{\beta} (1-\alpha) D_{\alpha}[\pi_0:\pi_{\pr}]$ 
%         &
%         $\pi_0(a|s) \exp_{\alpha} \big\{\beta \cdot \pr(a,s)\big\}$
%         \\
%         & & & $\frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \mu_{\pr}(s) \pi_0(a|s) \big[1+\beta (\alpha-1)\pr(a,s)\big]^{\frac{\alpha}{\alpha-1}} -  \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \mu_{\pr}(s) \pi_0(a|s)$ & \\
%         & & & $\frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \mu_{\pr}(s) \pi_0(a|s) \exp_{\alpha} \big\{\beta \cdot \pr(a,s)\big\}^{\alpha} -  \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \mu_{\pr}(s) \pi_0(a|s)$ & 
%         \\[1.5ex] \midrule
%         %  \frac{1}{\alpha} \psi_{\pr} $ \\
%         %  \alphaomegamu & 
%       $\frac{1}{\beta} \Omega^{(\alpha)}_{\mu_0}(\mu) 
%     %   =$
%     $ &  
%       $\frac{1}{\beta} D_{\alpha}[\mu_0:\mu]$ & $\frac{1}{\beta} \Omega^{*(\alpha)}_{\mu_0,\beta}(\pr)
%     %   =$ 
%      $ & 
%       \footnotesize $\frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s) \big[ 1+ \beta(\alpha-1)\pr(a,s) \big]^{\frac{\alpha}{\alpha-1}} - \frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s) $ 
%     %   $\textcolor{red}{\frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s)^{1-\alpha} \mu(a,s)^{\alpha} - \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s)} $ 
%      & $ \mu_0(a,s) \exp_{\alpha} \big\{\beta \cdot \pr(a,s) \big\} $ \\
%      & & &  $\frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s) \exp_{\alpha}\big\{ \beta \cdot \pr(a,s) \big\}^{\alpha} - \frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s) $ & \\
%          \bottomrule
%     \end{tabular}
% }
    
    
%     \captionof{table}{See \myapp{alpha_conj_all} and \ref{app:kl_conj_all} for derivations.}\label{tab:my_label}
% % \end{table}
% \end{figure*}
  


\begin{figure*}[t]
% \begin{table}
\vspace*{-1cm}
\resizebox{\textwidth}{!}{%
\centering
% \small
% \begin{table}[]
    % \centering
    % \begin{tabular}{ccc}
    %    \toprule
    %     Divergence  & Conjugate Notation & Conjugate Expression \\
    %     % \multicolumn{2}{c}{Conjugate} \\
    %     \midrule
    %     % \frac{1}{\beta} \Omega_{\pi_0}(\mu) &
    %      $\KL[\pi:\pi_0]$ & $\Omega^{*}_{\pi_0,\beta}(\pr)$& 
    %     %  $\sum \limits_{a \in \mathcal{A}} 
    %      $\sum \limits_{a} 
    %      \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} - 
    %     %  \sum \limits_{a \in \mathcal{A}} 
    %      \sum \limits_{a} 
    %      \pi_0(a|s)$  \\[1.5ex]
    %     % \frac{1}{\beta} \Omega_{\mu_0}(\mu) &
    %      $\KL[\mu:\mu_0]$ & $\Omega^{*}_{\mu_0,\beta}(\pr)$  & $
    %     \sum \limits_{a,s}% \in \mathcal{A} 
    %     %  \sum \limits_{a,s \in \mathcal{A}, \mathcal{S}}
    %      \mu_0(a,s) \expof{\beta \cdot \pr(a,s)} - 
    %     \sum \limits_{a,s} 
    %     %  \sum \limits_{a,s \in \mathcal{A}, \mathcal{S}}
    %      \mu_0(a,s)$  \\[1.5ex]
    %     %  \alphaomegapi & 
    %      $D_{\alpha}[\pi_0:\pi]$ & $\Omega^{*(\alpha)}_{\pi_0,\beta}(\pr)$  & $\frac{\alpha-1}{\alpha}\blangle \mu(a,s), \pr(a,s) \brangle + 
    %     (1-\alpha) D_{\alpha}[\pi_0:\pi]$ \\[1.5ex]
    %     %  \frac{1}{\alpha} \psi_{\pr} $ \\
    %     %  \alphaomegamu & 
    %     $D_{\mu}[\mu_0:\mu]$ & $\Omega^{*(\alpha)}_{\mu_0,\beta}(\pr)$ & $ \textcolor{red}{\frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s)^{1-\alpha} \mu(a,s)^{\alpha} - \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s)}$ \\
    %      \bottomrule
    % \end{tabular}
    
    
%     \begin{tabular}{cll}
%     \toprule
%     %   \multicolumn{2}{c}{Regularization} &  \multicolumn{2}{c}{Conjugate} \\[0.25ex]
%     %   Notation &  Expression  &  Notation &  \multicolumn{1}{c}{Expression} \\
% %  \text{Regularizer} 
%  \multicolumn{1}{c}{  Divergence } & 
% %  Conjugate & 
% \multicolumn{1}{c}{Conjugate Expression} 
%  & Optimizing Argument
%  \\
% %   [1.5ex]
% %         % \multicolumn{2}{c}{Conjugate} \\
%         \midrule
%         % \frac{1}{\beta} \Omega_{\pi_0}(\mu) &
%     $\Omega_{\pi_0}(\mu) =$  
%     % $&    
%     $\KL[\pi:\pi_0]$ & $\Omega^{*}_{\pi_0,\beta}(\pr)$ $=$ 
%     %& 
%         %  $\sum \limits_{a \in \mathcal{A}} 
%          $\sum \limits_{a} 
%          \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} - 
%         %  \sum \limits_{a \in \mathcal{A}} 
%          \sum \limits_{a} 
%          \pi_0(a|s)$ 
%          & $\pi(a|s) = \pi_0(a|s) \expof{\beta \cdot \pr(a,s)}$
%          \\[1.5ex]
%         % \frac{1}{\beta} \Omega_{\mu_0}(\mu) &
%      $\Omega_{\mu_0}(\mu)=$
%      %$ &    
%      $\KL[\mu:\mu_0]$ & $\Omega^{*}_{\mu_0,\beta}(\pr)$  
%     %  &
%      $=$
%      $\sum \limits_{a,s}% \in \mathcal{A} 
%         %  \sum \limits_{a,s \in \mathcal{A}, \mathcal{S}}
%          \mu_0(a,s) \expof{\beta \cdot \pr(a,s)} - 
%         \sum \limits_{a,s} 
%         %  \sum \limits_{a,s \in \mathcal{A}, \mathcal{S}}
%          \mu_0(a,s)$  
%           & $\mu(a,s) = \mu_0(a,s) \expof{\beta \cdot \pr(a,s)}$ 
%          \\[1.5ex]
%         %  \alphaomegapi & 
%      $\Omega^{(\alpha)}_{\pi_0}(\mu)=$
%     %  $ &   
%     $D_{\alpha}[\pi_0:\pi]$ & $\Omega^{*(\alpha)}_{\pi_0,\beta}(\pr)$  
%     %  &
%      $=$
%      $\frac{\alpha-1}{\alpha}\blangle \mu(a,s), \pr(a,s) \brangle + 
%         (1-\alpha) D_{\alpha}[\pi_0:\pi]$ 
%         &
%         $\pi(a|s) = \pi_0(a|s) \exp_{\alpha} \big\{\beta \cdot \pr(a,s)\big\}$
%         \\[1.5ex]
%         %  \frac{1}{\alpha} \psi_{\pr} $ \\
%         %  \alphaomegamu & 
%       $\Omega^{(\alpha)}_{\mu_0}(\mu) =$
%     %   $ &  
%       $D_{\mu}[\mu_0:\mu]$ & $\Omega^{*(\alpha)}_{\mu_0,\beta}(\pr)=$ 
%     %  $ & 
%       $\textcolor{red}{\frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s)^{1-\alpha} \mu(a,s)^{\alpha} - \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s)} $ 
%      & $\mu(a,s) = \mu_0(a,s) \exp_{\alpha} \big\{\beta \cdot \pr(a,s)\big\}$ 
%       \\
%          \bottomrule
%     \end{tabular}
%     \normalsize
        \begin{tabular}{llll}
    \toprule
    %   \multicolumn{2}{c}{Regularization} &  \multicolumn{2}{c}{Conjugate} \\[0.25ex]
    %   Notation &  Expression  &  Notation &  \multicolumn{1}{c}{Expression} \\
%  \text{Regularizer} 
 \multicolumn{1}{c}{  Divergence } & 
  Conjugate & 
\multicolumn{1}{c}{Conjugate Expression} 
 & Optimizing Argument ($\pi_{\pr}$ or $\mu_{\pr}$)
%  Conjugate $\pi_{\pr}(a|s)$ or $\mu_{\pr}(a,s)$
 \\
%   [1.5ex]
%         % \multicolumn{2}{c}{Conjugate} \\
        \midrule
        % \frac{1}{\beta} \Omega_{\pi_0}(\mu) &
    $\frac{1}{\beta} \KL[\pi:\pi_0]$ & $\frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(\pr)$ 
    % $=$ 
    & 
        %  $\sum \limits_{a \in \mathcal{A}} 
         $\frac{1}{\beta} \sum \limits_{a} 
         \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} - 
        %  \sum \limits_{a \in \mathcal{A}} 
         \frac{1}{\beta} $
        %  \sum \limits_{a} \pi_0(a|s)$ %% NORMALIZED REF
         & $ \pi_0(a|s) \expof{\beta \cdot \pr(a,s)}$
         \\[1.5ex]
        % \frac{1}{\beta} \frac{1}{\beta} \Omega_{\mu_0}(\mu) &
     $\frac{1}{\beta} \KL[\mu:\mu_0]$ & $\frac{1}{\beta} \Omega^{*}_{\mu_0,\beta}(\pr)$  
      &
     $\frac{1}{\beta} \sum \limits_{a,s}
        % \in \mathcal{A} 
        %  \sum \limits_{a,s \in \mathcal{A}, \mathcal{S}}
         \mu_0(a,s) \expof{\beta \cdot \pr(a,s)} - 
        \frac{1}{\beta} $
        % \sum \limits_{a,s}  \mu_0(a,s)$  %% NORMALIZED REF
        %  \sum \limits_{a,s \in \mathcal{A}, \mathcal{S}}
          & $ \mu_0(a,s) \expof{\beta \cdot \pr(a,s)}$ 
         \\[1.5ex] \midrule
        %  \alphaomegapi & 
    $\frac{1}{\beta} D_{\alpha}[\pi_0:\pi]$ & $\frac{1}{\beta} \Omega^{*(\alpha)}_{\pi_0,\beta}(\pr)$  
     &
   {\footnotesize $\frac{1}{\beta} \frac{1}{\alpha}  \sum \limits_{a} \pi_0(a|s) \exp_{\alpha}\big\{ \beta \cdot \big( \pr(a,s) - \myconst \big) \big\}^{\alpha} - \frac{1}{\beta} \frac{1}{\alpha} +   \psi_{\pr}(s;\beta)  $}
    &
        $\pi_0(a|s) \exp_{\alpha} \big\{\beta \cdot \left(  \pr(a,s) - \psi_{\pr}(s;\beta)  \right) \big\}$
        \\[1.5ex]
    % $\frac{1}{\beta} D_{\alpha}[\pi_0:\pi]$ & $\frac{1}{\beta} \Omega^{*(\alpha)}_{\pi_0,\beta}(\pr)$  
    %  &
    %   $\frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \textcolor{red}{\mu(s) \pi_0(a|s)} \exp_{\alpha} \big\{\beta \cdot \pr(a,s)\big\}^{\alpha} -  \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \mu(s) \pi_0(a|s)$  
    %     %  \frac{1}{\beta} (1-\alpha) D_{\alpha}[\pi_0:\pi_{\pr}]$ 
    %     &
    %     $\pi_0(a|s) \exp_{\alpha} \big\{\beta \cdot \pr(a,s)\big\}$
    %     \\[1.5ex] 
        % \midrule
        %  \frac{1}{\alpha} \psi_{\pr} $ \\
        %  \alphaomegamu & 
      $\frac{1}{\beta} D_{\alpha}[\mu_0:\mu]$ & $\frac{1}{\beta} \Omega^{*(\alpha)}_{\mu_0,\beta}(\pr)
     $ & 
    $\frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s) \exp_{\alpha}\big\{ \beta \cdot \pr(a,s) \big\}^{\alpha} - \frac{1}{\beta} \frac{1}{\alpha}$ 
    %   \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s) $  %% NORMALIZED REF
     & $\mu_0(a,s) \exp_{\alpha} \big\{ \beta \cdot \pr(a,s) \big\} $ 
    %  \\
    %  & &        ${\frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s)^{1-\alpha} \mu_{\pr}(a,s)^{\alpha} - \frac{1}{\beta} \frac{1}{\alpha}}$ 
    %  \sum \limits_{a,s} \mu_0(a,s)} $  %% NORMALIZED REF
  
    %  COMMENT BACK IN FOR 1-α vs. α FORM
    % $\frac{1}{\beta} D_{\alpha}[\pi_0:\pi]$ & $\frac{1}{\beta} \Omega^{*(\alpha)}_{\pi_0,\beta}(\pr)$  
    %  &
    % $\frac{1}{\beta} \frac{1}{\alpha}  \sum \limits_{a} \pi_0(a|s)^{1-\alpha} \pi_{\pr}(a|s)^{\alpha} - \frac{1}{\beta} \frac{1}{\alpha} +   \psi_{\pr}(s;\beta)  $
    % %  $\frac{\alpha-1}{\alpha}\blangle {\mu(s)\pi_{\pr}(a|s)}, \pr(a,s) \brangle +  \frac{1}{\alpha} \psi_{\pr}(s;\beta)  $
    % &
    %     $\pi_0(a|s) \exp_{\alpha} \big\{\beta \cdot \left(  \pr(a,s) - \psi_{\pr}(s;\beta)  \right) \big\}$
    %     \\[1.5ex]
    % % $\frac{1}{\beta} D_{\alpha}[\pi_0:\pi]$ & $\frac{1}{\beta} \Omega^{*(\alpha)}_{\pi_0,\beta}(\pr)$  
    % %  &
    % %   $\frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \textcolor{red}{\mu(s) \pi_0(a|s)} \exp_{\alpha} \big\{\beta \cdot \pr(a,s)\big\}^{\alpha} -  \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a,s} \mu(s) \pi_0(a|s)$  
    % %     %  \frac{1}{\beta} (1-\alpha) D_{\alpha}[\pi_0:\pi_{\pr}]$ 
    % %     &
    % %     $\pi_0(a|s) \exp_{\alpha} \big\{\beta \cdot \pr(a,s)\big\}$
    % %     \\[1.5ex] 
    %     % \midrule
    %     %  \frac{1}{\alpha} \psi_{\pr} $ \\
    %     %  \alphaomegamu & 
    %   $\frac{1}{\beta} D_{\alpha}[\mu_0:\mu]$ & $\frac{1}{\beta} \Omega^{*(\alpha)}_{\mu_0,\beta}(\pr)
    %  $ & 
    % %   $\frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s) \exp_{\alpha}\big\{ \beta \cdot \pr(a,s) \big\}^{\alpha} - \frac{1}{\beta} \frac{1}{\alpha}$ 
    %   ${\frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s)^{1-\alpha} \mu_{\pr}(a,s)^{\alpha} - \frac{1}{\beta} \frac{1}{\alpha}}$
    % %   \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s) $  %% NORMALIZED REF
    %  & $\mu_0(a,s) \exp_{\alpha} \big\{ \beta \cdot \pr(a,s) \big\} $ 
    % %  \\
    % %  & &        ${\frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a,s} \mu_0(a,s)^{1-\alpha} \mu_{\pr}(a,s)^{\alpha} - \frac{1}{\beta} \frac{1}{\alpha}}$ 
    % %  \sum \limits_{a,s} \mu_0(a,s)} $  %% NORMALIZED REF
    % & \\
        \\   \bottomrule
    \end{tabular}%
    }
    %  \captionof{table}
     \captionof{table}{Conjugate Function expressions for \textsc{kl} and $\alpha$-divergence regularization of either the policy $\pi(a|s)$ or occupancy $\mu(a,s)$.  See \myapp{conj1}-\ref{app:conj4} for derivations.  The final column shows the optimizing argument in the definition of the conjugate function $\frac{1}{\beta}\Omega^{*}(\pr)$, for example 
     $\mu_{\pr} \coloneqq \argmax_{\mu} \langle \mu, \pr \rangle -\frac{1}{\beta}\Omega_{\mu_0}(\mu)$.
    %  $\mu_{\pr}(a,s) \coloneqq \argmax_{\mu} \langle \mu(a,s), \pr(a,s) \rangle -\frac{1}{\beta}\Omega_{\mu_0}(\mu)$.  
    Note that each conjugate expression for $\pi(a|s)$ regularization also contains an outer expectation over $\mu(s)$.}
    \label{table:conj_table}
% \end{table}
\end{figure*}

% we can derive Δr_V = r + γ V' - V for suboptimal V, but this != Δr_π (in previous sections), unless we are at optimal policy & value

% i've written some experimentation below the blog post and outline here https://docs.google.com/document/d/19NjndpIiuljRxNuGdTspwuo5lJEpMztZ-m6RdTLfdVQ/edit




==> Reward Robustness TMLR (3)/sections/feasible_fig.tex <==
\begin{figure*}[!t]
\vspace*{-1.5cm}
\centering
% \begin{minipage}{\textwidth}%{0.8\textwidth}
%\centering
\begin{center}
\[\arraycolsep=.003\textwidth
\begin{array}{cccccc} %[width=40mm]
 \begin{subfigure}{0.07\textwidth} \vspace*{-.24cm} \includegraphics[width=\textwidth]
 {figs/feasible/uniform_prior.png} \end{subfigure}& %\qquad  \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_uniform_01.png}
{figs/feasible/kl/beta01alpha1uniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}& % \qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_uniform_1.png}
{figs/feasible/kl/beta1alpha1uniform.pdf}
\caption{ \centering  $D_{KL}, \beta = 1$}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_uniform_10.png} 
{figs/feasible/kl/beta10alpha1uniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 10$}\end{subfigure}& \rulesep
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
% {figs/feasible/alpha-1_no_lambda/alpha_neg1_beta1_uniform.png} 
{figs/feasible/alpha-1/alpha_neg1_beta10uniform.pdf}
\caption{\centering \small $\alpha = -1, \beta = 10$}\end{subfigure}&
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
{figs/feasible/alpha3/alpha3_beta10uniform.pdf}
% {figs/feasible/alpha3_no_lambda/alpha3_beta10_uniform_redo.pdf}
\caption{ \centering \small $\alpha = 3, \beta = 10$}\end{subfigure}
\\ %&\hspace*{.2cm}\\
\begin{subfigure}{0.07\textwidth}\vspace*{-.24cm} \includegraphics[width=\textwidth]{figs/feasible/nonuniform_prior.png}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_73_01.png}
{figs/feasible/kl/beta01alpha1nonuniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_73_1.png}
{figs/feasible/kl/beta1alpha1nonuniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 1$}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_73_10.png} 
{figs/feasible/kl/beta10alpha1nonuniform.pdf}
\caption{\centering \small $D_{KL}, \beta = 10$}\end{subfigure}& \rulesep %\hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/alpha-1_no_lambda/alpha_neg1_beta1_nonuniform.png} 
% {figs/feasible/alpha-1_no_lambda/alpha_neg1_beta1_nonuniform_redo.pdf}
{figs/feasible/alpha-1/alpha_neg1_beta10nonuniform.pdf}
\caption{\centering \small $\alpha = -1, \beta = 10$}\end{subfigure}&
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip] 
{figs/feasible/alpha3/alpha3_beta10nonuniform.pdf}
% {figs/feasible/alpha3_no_lambda/alpha3_beta10_nonuniform_redo.pdf}
\caption{ \centering \small $\alpha = 3, \beta = 10$}\end{subfigure}
\end{array}
\] 
\end{center}
% \end{minipage}
\vspace*{-.28cm}
\caption{\textbf{Robust Set} (red region) of perturbed reward functions to which a stochastic policy generalizes, in the sense that the policy is guaranteed to achieve an expected modified reward greater than or equal to the value of the regularized objective (\cref{eq:generalization}).  
The robust set characterizes the perturbed rewards achievable by the adversary. Red stars indicate the worst-case perturbed reward $\mr_{\piopt} = r - \pr_{\piopt}$ (\myprop{optimal_perturbations}).
We show feasible sets 
% for \textsc{kl} divergence (at various $\beta$) and $\alpha$-divergence ($\alpha=\{-1, 3\}, \beta =10$) regularization, 
% \TG{Do we need the two statements in brackets? It's obvious from the figure.}
 for the optimal $\pi_*(a|s)$ associated with fixed $Q(a,s)=r(a,s)$ values (blue star), where the policy differs based on the regularization parameters $\alpha, \beta, \pi_0$--- see \cref{eq:optimal_policy}.  The robust set becomes more restricted with decreasing regularization strength (increasing $\beta$), implying decreased generalization.
Importantly, the slope of the boundary of the robust set can be directly linked to the action probabilities under the given policy (see \mysec{visualizations_feasible}). 
% become more axis-aligned with decreasing regularization strength, which c
The shape of the robust set is affected by the choice of $\alpha$-divergence and reference $\pi_0$.
% \TG{This last sentence is also obvious from the figure and we have it in the main text.}.
% stochasticity of the optimal policy (see \mysec{generalization})
% of less regularized policies. choice
% The particular shape of the feasible set is affected by the choice of $\alpha$-divergence and reference $\pi_0$. Importantly, the slopes of the boundaries of the feasible set become more axis-aligned with decreasing regularization strength, which can be directly linked to the stochasticity of the optimal policy (see \mysec{generalization}).
% Top row:  reference distribution $\pi_0=(\frac{1}{2},\frac{1}{2})$, bottom row: $\pi_0 = (\frac{2}{3}, \frac{1}{3})$. 
% \TG{Missing: describe the results (size and shape of the set in relation to regularization strength).} 
% Red dot indicates $Q(a,s)$ associated with policy $\pi(a|s)$
}\label{fig:feasible_set_main}
\end{figure*}
\headerv




==> Reward Robustness TMLR (3)/sections/feasible_fig_no_lambda.tex <==
%%%%%%%%%%%%% NO LAMBDA VERSION &&&&&&&&&&&&&&&&&&&&
\begin{figure*}[!t]
\vspace*{-1.6cm}
\centering
% \begin{minipage}{\textwidth}%{0.8\textwidth}
%\centering
\begin{center}
\[\arraycolsep=.003\textwidth
\begin{array}{cccccc} %[width=40mm]
 \begin{subfigure}{0.07\textwidth} \vspace*{-.24cm} \includegraphics[width=\textwidth]
 {figs/feasible/uniform_prior.png} \end{subfigure}& %\qquad  \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_uniform_01.png}
{figs/feasible/kl/beta01alpha1uniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}& % \qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_uniform_1.png}
{figs/feasible/kl/beta1alpha1uniform.pdf}
\caption{ \centering  $D_{KL}, \beta = 1$}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_uniform_10.png} 
{figs/feasible/kl/beta10alpha1uniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 10$}\end{subfigure}& \rulesep
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
% {figs/feasible/alpha-1_no_lambda/alpha_neg1_beta1_uniform.png} 
{figs/feasible/alpha-1_no_lambda/alpha_neg1_beta10uniform.pdf}
\caption{\centering \small $\alpha = -1, \beta = 10$}\end{subfigure}&
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
{figs/feasible/alpha3_no_lambda/alpha3_beta10uniform.pdf}
% {figs/feasible/alpha3_no_lambda/alpha3_beta10_uniform_redo.pdf}
\caption{ \centering \small $\alpha = 3, \beta = 10$}\end{subfigure}
\\ %&\hspace*{.2cm}\\
\begin{subfigure}{0.07\textwidth}\vspace*{-.24cm} \includegraphics[width=\textwidth]{figs/feasible/nonuniform_prior.png}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_73_01.png}
{figs/feasible/kl/beta01alpha1nonuniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_73_1.png}
{figs/feasible/kl/beta1alpha1nonuniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 1$}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_73_10.png} 
{figs/feasible/kl/beta10alpha1nonuniform.pdf}
\caption{\centering \small $D_{KL}, \beta = 10$}\end{subfigure}& \rulesep %\hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/alpha-1_no_lambda_no_lambda/alpha_neg1_beta1_nonuniform.png} 
% {figs/feasible/alpha-1_no_lambda_no_lambda/alpha_neg1_beta1_nonuniform_redo.pdf}
{figs/feasible/alpha-1_no_lambda/alpha_neg1_beta10nonuniform.pdf}
\caption{\centering \small $\alpha = -1, \beta = 10$}\end{subfigure}&
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip] 
{figs/feasible/alpha3_no_lambda/alpha3_beta10nonuniform.pdf}
% {figs/feasible/alpha3_no_lambda/alpha3_beta10_nonuniform_redo.pdf}
\caption{ \centering \small $\alpha = 3, \beta = 10$}\end{subfigure}
\end{array}
\] 
\end{center}
% \end{minipage}
\vspace*{-.38cm}
\caption{\textbf{Robust Set} (red region) of perturbed reward functions to which a stochastic policy generalizes, in the sense that the policy is guaranteed to achieve an expected modified reward greater than or equal to the value of the regularized objective (\cref{eq:generalization}).  
The robust set characterizes the perturbed rewards which are feasible for the adversary. Red stars indicate the worst-case perturbed reward $\mr_{\piopt} = r - \pr_{\piopt}$ (\myprop{optimal_perturbations}).
We show robust sets 
% for \textsc{kl} divergence (at various $\beta$) and $\alpha$-divergence ($\alpha=\{-1, 3\}, \beta =10$) regularization, 
% \TG{Do we need the two statements in brackets? It's obvious from the figure.}
 for the optimal $\pi_*(a|s)$ with fixed $Q(a,s)=r(a,s)$ values (blue star), where the optimal policy differs based on the regularization parameters $\alpha, \beta, \pi_0$ (see \cref{eq:optimal_policy}).  The robust set is more restricted with decreasing regularization strength (increasing $\beta$), implying decreased generalization.
Importantly, the slope of the robust set boundary can be linked to the action probabilities under the policy (see \mysec{visualizations_feasible}). 
% become more axis-aligned with decreasing regularization strength, which c
% The shape of the robust set is affected by the choice of $\alpha$-divergence and reference $\pi_0$.
% \TG{This last sentence is also obvious from the figure and we have it in the main text.}.
% stochasticity of the optimal policy (see \mysec{generalization})
% of less regularized policies. choice
% The particular shape of the feasible set is affected by the choice of $\alpha$-divergence and reference $\pi_0$. Importantly, the slopes of the boundaries of the feasible set become more axis-aligned with decreasing regularization strength, which can be directly linked to the stochasticity of the optimal policy (see \mysec{generalization}).
% Top row:  reference distribution $\pi_0=(\frac{1}{2},\frac{1}{2})$, bottom row: $\pi_0 = (\frac{2}{3}, \frac{1}{3})$. 
% \TG{Missing: describe the results (size and shape of the set in relation to regularization strength).} 
% Red dot indicates $Q(a,s)$ associated with policy $\pi(a|s)$
}\label{fig:feasible_set_main}
\vspace*{-.1cm}
\end{figure*}


==> Reward Robustness TMLR (3)/sections/new/0_intro.tex <==
\headerv
\section{Introduction}\label{sec:intro}
\headerv
% \textcolor{red}{Submission version can be found here:  }\href{https://ol.deepmind.host/project/61ae907d5ff66355dd683052}{https://ol.deepmind.host/project/61ae907d5ff66355dd683052}

% \RB{Intro has been written carefully.   comments and/or suggestions for abstract and conclusion welcomed!}
%While \gls{RL} algorithms have achieved remarkable success in challenging domains \citep{mnih2015human,silver2016mastering}, questions of optimization, exploration, and safe generalization remain activate areas of research.   
Regularization plays a crucial role in various settings across \gls{RL}, 
% Regularization plays a prominent role in \gls{RL} across various algorithmic settings 
such as trust-region methods \citep{peters2010relative, schulman2015trust, schulman2017proximal, basserrano2021logistic}, offline learning \citep{levine2020offline, nachum2019dualdice, nachum2019algaedice, nachum2020reinforcement}, multi-task learning \citep{teh2017distral, igl2020multitask}, and soft 
$Q$-learning or actor-critic methods
% actor-critic methods 
\citep{fox2016taming, nachum2017bridging, haarnoja17a, haarnoja2018soft, grau2018soft}. 
% \textcolor{red}{SAC? Soft Q?}
%with stochastic policies 
Various justifications have been given for policy regularization, %the benefits of
such as improved optimization \citep{ahmed2019understanding},  
% implicit averaging of $Q$-values, \citep{viellard},
connections with probabilistic inference \citep{levine2018reinforcement, 
% dayan1997using, 
kappen2012optimal, rawlik2013stochastic, wang2021variational}, 
 %with purported benefits including X, Y, Z , 
 and robustness to perturbations in the environmental rewards or dynamics \citep{derman2021twice, eysenbach2021maximum, husain2021regularized}.
%  The latter benefits may be particularly relevant for safety considerations \citep{amodei2016concrete, everitt2018agi}, where we are interested in agents which can generalize or adapt to new environments or distribution shift.

% The latter 
% is critical in \textsc{ai} safety, where
% % plays a crucial role in \textsc{ai} safety, where 
% % a primary goal
% the goal 
% is to design agents that generalize and adapt safely to new situations or distributional shift.
% % \citep{amodei2016concrete, everitt2018agi}.

% In this work, we provide a unified discussion of several recent works that interpret policy regularization as providing robustness to perturbations in the environmental rewards \TG{Suggestion: ``In this work we theoretically analyze the robustness-properties that arise form policy regularization in RL.'' Then skip to the next sentence (For a policy...) and mention the unified view later.} \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}.

In this work, we use convex duality to 
% highlight that 
analyze the reward robustness which naturally arises from policy regularization in \gls{RL}.
% analyze the reward robustness which naturally arises from policy regularization in \gls{RL}.
% In this work, 
% we analyze robustness properties that naturally arise 
% % we analyze the robustness properties which arise
% from policy regularization in \gls{RL}.  
In particular, we interpret regularized reward maximization as a two-player game between the agent and an imagined adversary that modifies the reward function.  For a policy $\pi(a|s)$ regularized with a convex function $\Omega(\pi) = \mathbb{E}_{\pi}[\ptReg(\pi)]$ 
% such as the \textsc{kl} or $\alpha$-divergence 
and regularization strength $1/\beta$,
% $\frac{1}{\beta}$, 
we 
% define robustness to adversarial modifications of the reward function using
investigate statements of the form %\citep{eysenbach2021maximum}
% {\tau \sim p_{\pi}(\tau)}
% {p_{\pi}(\tau)}
\begin{align}
\hspace*{-.3cm} \max \limits_{\pi(a|s)} \text{\small $(1-\gamma)$} 
% \mathbb{E}_{\tau \sim p_\pi(\tau)} 
\mathbb{E}_{\taunotation}
\left[ \sum \limits_{t=0}^\infty \gamma^t \bigg( r(a_t, s_t) -  {\frac{1}{\beta}} \ptReg \big(\pi(a_t | s_t)\big) \bigg) \right] = \max \limits_{\pi(a|s)} \min \limits_{r\tick(a,s) \in \feasibleset}  \text{\small $(1-\gamma)$} \mathbb{E}_{\taunotation} \left[ \sum \limits_{t=0}^\infty \gamma^t r\tick(a_t,s_t) \right],
\label{eq:reward_perturbation_stmt} 
% 
\end{align}
% \RB{Do we need the maximization??}\\
\normalsize
%%%%%% AISTATS PARAGRAPH %%%%%
% where $r\tick(a,s)$ 
% % is the worst-case reward function 
% indicates a modified reward chosen
% from an appropriate feasible set $\feasibleset$. %which depends on the policy $\pi$.
% This robustness is intriguing, as it suggests regularized policies achieve a form of `zero-shot' generalization to new environments where the reward has been adversarially chosen. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where 
$r\tick(a,s)$ 
% $r\tick$
% is the worst-case reward function 
indicates a modified reward function chosen
from an appropriate robust set $\feasibleset$ (see \myfig{related}-\ref{fig:feasible_set_main}). %which depends on the policy $\pi$.
% \textcolor{red}{We refer to \cref{eq:reward_perturbation_stmt} as showing the robustness of the policy $\pi(a|s)$ to adversarial modifications of the reward function.}
% \textcolor{red}{We define the robustness of a policy to adversarial modifications of the reward function according to \cref{eq:reward_perturbation_stmt}.}
\cref{eq:reward_perturbation_stmt} suggests that an agent may translate uncertainty in its estimate of the reward function into regularization of a learned policy, which is particularly relevant in applications such as inverse \gls{RL} \citep{ng2000algorithms, arora2021survey} or learning from human preferences \citep{christiano2017deep}.

% \textcolor{red}{
% % When learning a reward function $r(a,s)$ from observed behavior \citep{ng2000algorithms, arora2021survey} or human preferences \citep{christiano2017deep}, 
% For inverse \gls{RL} \citep{ng2000algorithms, arora2021survey} or learning from human preferences \citep{christiano2017deep},
% \cref{eq:reward_perturbation_stmt} suggests that an agent may translate uncertainty in its estimate of the reward function into regularization of a subsequently learned policy, which automatically hedges against a set of reward modifications.}
% % \cref{eq:reward_perturbation_stmt} suggests that the agent tasked with learning a reward function $r(a,s)$ from observed behavior \citep{ng2000algorithms, arora2021survey} or human preferences \citep{christiano2017deep} may translate uncertainty in its estimate of the reward function into regularization of a subsequently learned policy, by automatically hedging against a set of reward modifications which depends on the regularizer. (\cref{fig:feasible_set_main}). 
% % may translate uncertainty in its estimate of the reward function into regularization of a subsequently learned policy.
% % By automatically hedging against a set of reward modifications (\cref{fig:feasible_set_main}), \cref{eq:reward_perturbation_stmt} suggests that an agent tasked with learning a reward function $r(a,s)$ from observed behavior \citep{ng2000algorithms, arora2021survey} or human preferences \citep{christiano2017deep} may translate uncertainty in its estimate of the reward function into regularization of a subsequently learned policy. 

% % policy regularization allows an agent to encode uncertainty about its value estimates, By automatically hedging against a  set of reward perturbations (\cref{fig:feasible_set_main}) that depends on the choice of $\alpha$-divergence and regularization strength. 
% % and performing optimization on this reward 

\begin{figure}[t]
% {.3\textwidth}
\centering
% \vspace*{-1.8cm}
% \includegraphics[width=.34\textwidth]{figs/feasible/kl/beta1alpha1uniform_adj.pdf}
\vspace*{-1.1cm}
% \vspace*{-.2cm}
\includegraphics[width=.35\textwidth]{figs/feasible/kl/robust_set_fig1.pdf}
% \includegraphics[width=.4\textwidth]{figs/feasible/kl/beta1alpha1uniform_adj2.pdf}
% \caption{}\label{fig:derman}
\vspace*{-.05cm}
\caption{
\textbf{Robust set} $\feasibleset$ (red region) of perturbed reward functions to which a stochastic policy generalizes, in the sense of \cref{eq:generalization}.
% that the policy is guaranteed to achieve expected perturbed reward greater than or equal to the value of the regularized objective (\cref{eq:generalization}).
Red star indicates the worst-case perturbed reward $\mroptpi = r - \proptpi$ (\myprop{optimal_perturbations}) chosen by the adversary.
The robust set also characterizes the set of reward perturbations $\pr(a,s)$ that are feasible for the adversary, which differs based on the choice of regularization function, regularization strength $\beta$, and reference distribution $\pi_0$ (see \mysec{visualizations_feasible} and \myfig{feasible_set_main}).  We show the robust set for the optimal single-step policy with value estimates $Q(a,s) = r(a,s)$ and \textsc{kl} divergence regularization to a uniform $\pi_0$, with $\beta = 1$.
% Note that 
Our robust set is larger and has a 
qualitatively 
different shape 
% than
compared to the 
%{rectangular} 
robust set of \citet{derman2021twice} (dotted lines, see \mysec{related}). %see
% We show feasible sets 
% % for \textsc{kl} divergence (at various $\beta$) and $\alpha$-divergence ($\alpha=\{-1, 3\}, \beta =10$) regularization, 
% % \TG{Do we need the two statements in brackets? It's obvious from the figure.}
%  for the optimal $\pi_*(a|s)$ associated with fixed $Q(a,s)=r(a,s)$ values (blue star), where the policy differs based on the regularization parameters $\alpha, \beta, \pi_0$--- see \cref{eq:alpha_opt_policy} and (\ref{eq:kl_opt_policy}).  The feasible set becomes more restricted with decreasing regularization strength (increasing $\beta$), implying decreased generalization.
% Importantly, the slope of the boundary of the feasible set can be directly linked to the action probabilities for the optimal policy (see \mysec{generalization}).  
% % become more axis-aligned with decreasing regularization strength, which c
% The particular shape of the feasible set is affected by the choice of $\alpha$-divergence and reference $\pi_0$.
}\label{fig:related}
% \captionof{figure}{\text{\small \citet{derman2021twice}}}\label{fig:derman}
% \end{minipage}
% \end{minipage}
% \end{center}
\vspace*{-.3cm}
\end{figure}

% This robustness is intriguing, as it suggests 
% This robustness also suggests that
% More formally,
% Further, 
This reward robustness further implies that
regularized policies achieve a form of `zero-shot' generalization to new environments where the reward is adversarially chosen.   
% While the adversary does not modify the optimal policy in a fixed \textsc{mdp} or the regret of a particular policy, we obtain the following performance guarantee for any given $\pi(a|s)$ and a modified reward $\mr(a,s) \in \feasibleset$ within the corresponding robust set.
In particular, for any given $\pi(a|s)$ and a modified reward $\mr \in \feasibleset$ 
within the corresponding robust set,
% \textcolor{red}{since equality is achieved in \cref{eq:reward_perturbation_stmt},} 
we obtain the following performance guarantee 
% In particular, 
% % \textcolor{red}{since equality is achieved in \cref{eq:reward_perturbation_stmt},} 
% we obtain the following performance guarantee on the expected modified reward.   For \textit{any} given $\pi(a|s)$ and a modified reward $\mr(a,s) \in \feasibleset$ 
% within the corresponding robust set,
% In particular, for $\mr(a,s) \in \mathcal{R}$ and a given $\pi(a|s)$, we obtain the following performance guarantee on the expected modified reward
% \small
% \begin{align}
% %   \hspace*{-.2cm} 
% %   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) \rangle - \omegamu \, . \label{eq:robust_def} \\
% %   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) \rangle - \omegamu \, . \label{eq:robust_def} \\
%   \mathbb{E}_{\mu(s)\pi(a|s)}\big[ \mr(a,s) \big]  &\geq   \mathbb{E}_{\mu(s)}\left[\mathbb{E}_{\pi(a|s)}\big[r(a,s)\big] - \frac{1}{\beta} \Omega\big(\pi(a|s)\big) \right]
%  \nonumber
% \end{align}
% \normalsize
% \footnotesize
% \begin{align}
\begin{equation}
 \hspace*{-.2cm} 
    %  \text{\small $(1-\gamma)$} 
    %  \resizebox{.925\columnwidth}{!}{$
     \mathbb{E}
    %  _{\pi(\tau)}
     _{\taunotation} 
     \left[ \sum \limits_{t=0}^\infty \gamma^t r\tick(a_t,s_t) \right] \geq 
    %  \text{\small $(1-\gamma)$}
     \mathbb{E}
    %  _{\pi(\tau)}
    _{\taunotation} 
     \left[ \sum \limits_{t=0}^\infty \gamma^t \bigg( r(a_t, s_t) - {\frac{1}{\beta}} \ptReg 
     \big(\pi_t \big) \bigg) \right] .
    %  \big(\pi(a_t | s_t)\big) \bigg) \right]
    % $
    \label{eq:generalization}
    % }
\end{equation}
% \end{align}
\normalsize
% where $\mu(s)$ is the state-occupancy distribution induced by the policy (see \mysec{mdp_background}).
\cref{eq:generalization} states that the expected modified reward under $\pi(a|s)$, with $\mr \in \feasibleset$ as in \myfig{related}, will be greater than the value of the regularized objective with the original, unmodified reward.  
It is in this particular sense that we 
make claims about robustness and zero-shot generalization throughout the paper.   
% It is in this particular sense that we make claims about robustness and zero-shot generalization throughout this paper.   
%Among our primary contributions is to characterize the robust set of modified rewards $\feasibleset$, based on the regularization function $\Omega(\pi)$ and strength $\beta$, with a formal statement in \myprop{feasible} and example visualizations in \myfig{feasible_set_main}.

% We visualize example robust sets in \myfig{feasible_set_main}.


% provide robustness or zero-shot generalization guarantees for a regularized policy.

% We also notice that this form of robustness is sensitive to the exact value of the regularized objective function, which we discuss in further detail in \mysec{entropy_vs_div}.

% It is in this precise sense that we are able to make generalization 

Our analysis unifies 
%\textcolor{\shiehl}{\sout{and extends}} 
recent work exploring similar interpretations \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum, derman2021twice} %\textcolor{\shiehl}{\citet{derman2021twice}}, 
% and our further contributions include
as summarized in \mysec{discussion} and \mytab{novelty}.  
% Under this adversarial interpretation, policy regularization allows an agent to encode uncertainty about its value estimates, by automatically hedging against a  set of reward perturbations (\cref{fig:feasible_set_main}) that depends on the choice of $\alpha$-divergence and regularization strength. 
Our contributions include
\setlength\itemsep{0.025em}
\begin{itemize}
% \item A thorough analysis of the robustness associated with \kl and $\alpha$-divergence regularization of \gls{RL} policies, which includes popular Shannon \citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum} and Tsallis entropy \citep{lee2019tsallis} entropy regularization as a special cases.    We argue that using divergence regularization instead of entropy regularization avoids several unsatisfying conclusions from previous work. %\citep{lee2019tsallis, eysenbach2021maximum}.
% %Our derivations for $\alpha$-divergence regularization extend the Tsallis entropy \citep{lee2019tsallis}
\item A thorough analysis of the robustness associated with \kl and $\alpha$-divergence policy regularization, which includes popular Shannon entropy regularization
% schemes 
% \citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum} 
as a special case.  Our derivations for the $\alpha$-divergence generalize the Tsallis entropy \gls{RL} framework of \citet{lee2019tsallis}.
% and shed light on properties of soft-value aggregation.   
% \TG{``a general relationship'' is too vague for the reader. Either leave that part of the sentence out, or formulate as simple/clear as possible.} 
% Our analysis covers popular Shannon entropy regularization schemes \citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum}, while our derivations for the $\alpha$-divergence extend the Tsallis entropy \gls{RL} framework of \citep{lee2019tsallis}.    
% but not for the $\alpha$-divergence. 
% We argue that using divergence regularization instead of entropy regularization avoids several unsatisfying conclusions from previous work. %\citep{lee2019tsallis, eysenbach2021maximum}.
% \item In \cref{fig:feasible_set_main}, we compute and visualize the feasible set  $\mathcal{R}$  of adversarial rewards against which a regularized policy is robust, with further detail in \myprop{feasible}. 
\item We derive the worst-case reward perturbations $\prpi = r - \mr_{\pi}$ corresponding to any stochastic policy $\pi$ and a fixed regularization scheme (\myprop{optimal_perturbations}). 
% For the $\alpha$-divergence regularization,  
% \textcolor{red}{Our $\alpha$-divergence derivations highlight distinct roles for the value function and policy normalization constant, which coincide only in the case of \textsc{kl} divergence regularization (\myapp{soft_value}).}
% \textcolor{red}{We also observe differences between using $\alpha$-divergence regularization for the policy $\pi(a|s)$ and joint occupancy distribution $\mu(a,s)$.}

\item For the optimal regularized policy in a given environment, we show that the corresponding worst-case reward perturbations 
% $\propt = r - r_*\tick$ 
match the advantage function for \textit{any} $\alpha$-divergence.   
We relate this finding to the path consistency optimality condition, which has been used to construct learning objectives in \citep{nachum2017bridging, chow2018path}, and a game-theoretic indifference condition, 
which occurs at a Nash equilibrium between the agent and adversary \citep{ortega2014adversarial}.   
% In contrast to previous work, our results in \mysec{visualizations} explicitly visualize the reward robustness of regularized policies in a simple sequential setting, where we can use the path consistency or indifference conditions to confirm the optimality of the policy.  
% \item For a sequential setting \TG{Maybe: ``We perform experiments on a sequential grid-world task where we explicitly ...''}, we explicitly visualize the reward robustness and adversarial strategies associated with regularized policies in \mysec{visualizations}. 
\item  We visualize the set  $\feasibleset$ of adversarially perturbed rewards against which a regularized policy is robust in \myfig{related}-\ref{fig:feasible_set_main}, with details in \myprop{feasible}.
% In addition to \myprop{feasible} and \myfig{feasible_set_main}, our 
% Our robust set is different than that in \citet{derman2021twice}, and 
Our use of divergence instead of entropy regularization to analyze the robust set 
%$\feasibleset$  
clarifies several unexpected conclusions from previous work.   In particular, 
similar plots in 
\citet{eysenbach2021maximum} 
suggest that
% indicate that 
MaxEnt \textsc{rl} is not robust to the reward function of the training environment, and that increased regularization strength may hurt robustness.  Our analysis in \mysec{entropy_vs_div} and  \myapp{eysenbach} establishes the expected, \textcolor{black}{opposite} results.
%\textcolor{\shiehl}{\sout{Our robust set 
%for divergence regularization 
%also differs from the more general approach of \citet{derman2021twice} (\myfig{related}).}}


% \begin{figure*}[t]
% \vspace*{-1cm}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccc}
%     &  \text{ \citet{ortega2014adversarial}} & \text{\citet{eysenbach2021maximum}} &  \text{ \citet{husain2021regularized}} & Ours \\ \toprule
%     \bullets{Multi-Step Analysis} & \tcminus{\xmark} & \tcplus{\cmark} & \tcplus{\cmark} & \tcplus{\cmark} \\ 
%     \bullets{Worst-Case $\pr(a,s)$} & \tcminus{policy form} & \tcminus{policy form} & \tcminus{value form} & \tcplus{policy $\&$ value forms} \\ 
%   \bullets{Robust Set} & \tcminus{\xmark} & 
%     \tcplus{\cmark}  \tcminus{(see our \myapp{eysenbach})} & \tcminus{\xmark} & \tcplus{\cmark}  \\ 
%   \bullets{Divergence Used} & \tcminus{KL ($\alpha = 1$)} & \tcminus{\text{ Shannon entropy (see \mysec{entropy_vs_div})}} & \tcplus{any convex $\Omega$} & \tcplus{$\alpha$-Divergence}  \\ 
%     \bullets{$\mu(a,s)$ or $\pi(a|s)$ Reg.?} & 
%      $\pi(a|s)$ & 
%     % (= in single step) & 
%     $\pi(a|s)$ & \tcplus{Both} & \tcplus{Both}  \\
%     \bullets{Indifference} & \tcplus{\cmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}   \\ 
%     \bullets{Path Consistency} & \tcminus{\xmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}  \\ 
%     \bottomrule
% \end{tabular}%
% }
% \vspace*{-.25cm}
% \captionof{table}{Comparison with related work. }\label{table:novelty}
% \headerv
% \headerv
% \end{figure*}

\item We perform experiments for a sequential grid-world task in \mysec{visualizations} where, in contrast to previous work, we explicitly visualize the reward robustness and adversarial strategies resulting from our theory.
% associated with a regularized policy.   
We use the path consistency or indifference conditions to certify optimality of the policy.
% We perform experiments on a sequential grid-world task in \mysec{visualizations}, where we explicitly visualize the reward robustness and adversarial strategies associated a regularized policy, 
% and use the path consistency or indifference conditions to confirm the optimality of the policy.
% can use the path consistency or indifference conditions to confirm the optimality of the policy.
% We explicitly visualize the reward robustness and adversarial strategies of regularized policies for a simple sequential setting in \mysec{visualizations}, where we can use the path consistency or indifference conditions to confirm the optimality of the policy. To the best of our knowledge this has not been shown before. 
% compute and \TG{Maybe a bit too strong? The bullet point used to start with: ``In contrast to previous work'' which I thought was not ideal.}
\end{itemize}
% In contrast to previous work, we explicitly visualize the reward robustness of regularized policies for a simple sequential setting in \mysec{visualizations}, where we can use the path consistency or indifference conditions to confirm the optimality of the policy.   While these conditions hold only for the optimal policy, we emphasize that our analysis provides an adversarial robustness interpretation for \textit{any} stochastic policy under a given regularization scheme.
% While the latter observation holds only for the optimal policy, we emphasize that our results provide a reward robustness interpretation for \textit{any} stochastic policy under a given regularization scheme.
%  of an optimal policy 
%\RB{Still needed?}
% Under this adversarial interpretation, policy regularization allows an agent to encode uncertainty about its value estimates, by automatically hedging against a  set of reward perturbations (\cref{fig:feasible_set_main}) that depends on the choice of $\alpha$-divergence and regularization strength. 

% \begin{figure*}[t]
% \vspace*{-1cm}
% \begin{minipage}{.44\textwidth}
% \centering
% \includegraphics[width=.95\textwidth, trim=5 0 0 0, clip]{figs/feasible/kl/robust_set_fig1.pdf} 
% \end{minipage}\hspace*{.03cm}
% \begin{minipage}{.56\textwidth}
% % \vspace*{-.1cm}
% \captionof{figure}{\label{fig:related}
% \textbf{Robust set} $\feasibleset$ (red region) of perturbed reward functions to which a stochastic policy generalizes, in the sense of \cref{eq:generalization}.
% % that the policy is guaranteed to achieve expected perturbed reward greater than or equal to the value of the regularized objective (\cref{eq:generalization}).
% Red star indicates the worst-case perturbed reward $\mroptpi = r - \proptpi$ (\myprop{optimal_perturbations}) chosen by the adversary.
% The robust set also characterizes the set of reward perturbations $\pr(a,s)$ that are feasible for the adversary, which differs based on the choice of regularization function, regularization strength $\beta$, and reference distribution $\pi_0$ (see \mysec{visualizations_feasible}, \myfig{feasible_set_main}).  We show the robust set for the optimal single-step policy with value estimates $Q(a,s) = r(a,s)$ and \textsc{kl} divergence regularization to a uniform $\pi_0$, and $\beta = 1$.
% % Note that 
% Our robust set is larger, with qualitatively different shape compared to the {rectangular} robust set analyzed by \citet{derman2021twice} (dotted lines, see \mysec{related}).
% }
% % \vspace*{-.3cm} 
% \end{minipage}
% % \vspace*{-.2cm}
% \end{figure*}%







%%%%%%%%%%%%%%%%%%%%%%%%% PREV BULLET POINTS AI STATS SUBMISSION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Using tools from convex duality, we characterize this reward robustness and discuss its implications for generalization. 
% % via the the feasible set of perturbations. 
% % \RB{modify? we characterize the worst-case rewards using tools from convex duality and discuss implications for generalization using the the feasible set of perturbations.}
% % In particular, we show that policy regularization implies robustness to the feasible set $\mathcal{R}$ of perturbed rewards visualized in \cref{fig:feasible_set_main}. 
% Our analysis unifies and extends several recent works exploring similar interpretations \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}, and our main contributions are
% % We find that the optimal modified reward $r_{*}\tick$ in \cref{eq:reward_perturbation_stmt} re-expresses the value of the objective for a given policy, which places restrictions on the set $\mathcal{R}$.  
% %which leads to a game-theoretic interpretation of soft value aggregation as hedging against adversarial perturbations which tend to equalize the reward function across actions in a particular state \citep{ortega2014adversarial}.
% %and provide a unified discussion of several recent works that explore similar interpretations \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}
% % We discuss the implications of this particular form of robustness for generalization, along with a game-theoretic interpretation of soft value aggregation as hedging against adversarial perturbations that seek to 
% % equalize the reward obtained for each action in a particular state \citep{ortega2014adversarial}.
% % We find that the optimal modified reward $r_{*}\tick$ in \cref{eq:reward_perturbation_stmt} re-expresses the value of the objective for a given policy, which places restrictions on the set $\mathcal{R}$.  
% % how this impacts the nature of the robustness or `zero-shot' generalization induced by policy regularization
% % Our analysis unifies several recent works that explore similar interpretations \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}, and our main contributions include
% % \TG{Alternative for the previous para: ``Using tools from convex duality, we precisely characterize the `zero-shot' generalization regime and relate it to a game-theoretic interpretation where robustness arises from `hedging' against adversarial perturbations to the reward function \citep{ortega2014adversarial}. We find that the optimal modified reward $r\tick$ in \cref{eq:reward_perturbation_stmt} re-expresses the value of the objective for a given policy, which restricts the set $\mathcal{R}$. We discuss how this impacts the nature of the robustness or `zero-shot' generalization induced by policy regularization and provide a unified discussion of several recent works that explore similar interpretations \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}. Our main contributions are:}
% \setlength\itemsep{0.1em}
% \begin{itemize}
% % \item A thorough analysis of the robustness associated with \kl and $\alpha$-divergence regularization of \gls{RL} policies, which includes popular Shannon \citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum} and Tsallis entropy \citep{lee2019tsallis} entropy regularization as a special cases.    We argue that using divergence regularization instead of entropy regularization avoids several unsatisfying conclusions from previous work. %\citep{lee2019tsallis, eysenbach2021maximum}.
% % %Our derivations for $\alpha$-divergence regularization extend the Tsallis entropy \citep{lee2019tsallis}
% \item A thorough analysis of the robustness associated with \kl and $\alpha$-divergence policy regularization, which includes popular Shannon entropy regularization
% % schemes 
% % \citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum} 
% as a special case.  Our derivations for the $\alpha$-divergence generalize the Tsallis entropy \gls{RL} framework of \citep{lee2019tsallis} and 
% % show a general relationship between the value function and the policy normalization constant, 
% highlight distinct roles for the value function and normalization constant of the optimal policy,
% which coincide only in the case of \textsc{kl} divergence regularization. 
% % \TG{``a general relationship'' is too vague for the reader. Either leave that part of the sentence out, or formulate as simple/clear as possible.} 
% % Our analysis covers popular Shannon entropy regularization schemes \citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum}, while our derivations for the $\alpha$-divergence extend the Tsallis entropy \gls{RL} framework of \citep{lee2019tsallis}.    
% % but not for the $\alpha$-divergence. 
% % We argue that using divergence regularization instead of entropy regularization avoids several unsatisfying conclusions from previous work. %\citep{lee2019tsallis, eysenbach2021maximum}.
% \item In \cref{fig:feasible_set_main}, we compute and visualize the feasible set  $\mathcal{R}$  of adversarial rewards against which a regularized policy is robust, with further detail in \myprop{feasible}.  
% % We compute and visualize the feasible set  $\mathcal{R}$  of adversarial rewards against which a regularized policy is robust in \cref{fig:feasible_set_main}, with details in \myprop{feasible}.
% Our use of divergence instead of entropy regularization to define the feasible set clarifies
% several unsatisfying interpretations from previous work (\mysec{entropy_vs_div}).
% \item For the optimal regularized policy in a given environment, we show that the corresponding reward perturbations $\propt = r - r_*\tick$ match the advantage function for \textit{any} $\alpha$-divergence.   
% We relate this finding to the path consistency optimality condition, which has been used to construct learning objectives in \citep{nachum2017bridging, chow2018path}, and a game-theoretic indifference condition, which occurs at a Nash equilibrium between the agent and adversary \citep{ortega2014adversarial}.   
% % In contrast to previous work, our results in \mysec{visualizations} explicitly visualize the reward robustness of regularized policies in a simple sequential setting, where we can use the path consistency or indifference conditions to confirm the optimality of the policy.  
% % \item For a sequential setting \TG{Maybe: ``We perform experiments on a sequential grid-world task where we explicitly ...''}, we explicitly visualize the reward robustness and adversarial strategies associated with regularized policies in \mysec{visualizations}. 
% \item  We perform experiments on a sequential grid-world task in \mysec{visualizations}, where we explicitly visualize the reward robustness and adversarial strategies associated a regularized policy, 
% and use the path consistency or indifference conditions to confirm the optimality of the policy.
% % can use the path consistency or indifference conditions to confirm the optimality of the policy.
% % We explicitly visualize the reward robustness and adversarial strategies of regularized policies for a simple sequential setting in \mysec{visualizations}, where we can use the path consistency or indifference conditions to confirm the optimality of the policy. To the best of our knowledge this has not been shown before. 
% % compute and \TG{Maybe a bit too strong? The bullet point used to start with: ``In contrast to previous work'' which I thought was not ideal.}
% \end{itemize}
% % In contrast to previous work, we explicitly visualize the reward robustness of regularized policies for a simple sequential setting in \mysec{visualizations}, where we can use the path consistency or indifference conditions to confirm the optimality of the policy.   While these conditions hold only for the optimal policy, we emphasize that our analysis provides an adversarial robustness interpretation for \textit{any} stochastic policy under a given regularization scheme.
% % While the latter observation holds only for the optimal policy, we emphasize that our results provide a reward robustness interpretation for \textit{any} stochastic policy under a given regularization scheme.
% %  of an optimal policy 
% Under this adversarial interpretation, policy regularization allows an agent to encode uncertainty about its value estimates, by automatically hedging against a  set of reward perturbations (\cref{fig:feasible_set_main}) that depends on the choice of $\alpha$-divergence and regularization strength. % $\beta$.
% % This robust set follows from the choice of $\alpha$-divergence and regularization strength $\beta$..
% % dding a policy regularizer corresponds to hedgin
% % training with a policy regularizer corresponds to assuming that the rewards observed might not be entirely reliable or might change in the future, and taking these assumptions into account such that the learned policy automatically hedges (is robust against) a set of such reward perturbations.





\begin{figure*}[t]
\vspace*{-1cm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccc}
    &  \text{ \citet{ortega2014adversarial}} & \text{\citet{eysenbach2021maximum}} &  \text{ \citet{husain2021regularized}}  & \citet{derman2021twice} & Ours \\ \toprule
    \bullets{Multi-Step Analysis} & \tcminus{\xmark} & \tcplus{\cmark} & \tcplus{\cmark} & \tcplus{\cmark} & \tcplus{\cmark} \\ 
    \bullets{Worst-Case $\pr(a,s)$} & \tcminus{policy form} & \tcminus{policy form} & \tcminus{value form} & \tcminus{policy} (via dual \textsc{lp} \cref{eq:dual_lp}) & \tcplus{policy $\&$ value forms}  \\ 
  \bullets{Robust Set} & \tcminus{\xmark} & 
    \tcplus{\cmark}  \tcminus{(see our \myapp{eysenbach})} & \tcminus{\xmark} & \tcplus{\cmark (flexible specification)} & \tcplus{\cmark}  \\ 
  \bullets{Divergence Used} & \tcminus{KL ($\alpha = 1$)} & \tcminus{\text{ Shannon entropy (\mysec{entropy_vs_div})}} & \tcplus{any convex $\Omega$} & \tcplus{derived from robust set}  & 
  %\begin{tabular}{@{}c@{}} \tcplus{any convex $\Omega$} \\ \tcplus{$\alpha$-Div examples} \end{tabular}
  \tcplus{any convex $\Omega$, $\alpha$-Div examples}  
  \\ 
    \bullets{$\mu(a,s)$ or $\pi(a|s)$ Reg.?} & 
     $\pi(a|s)$ & 
    % (= in single step) & 
    $\pi(a|s)$ & \tcplus{Both}  & $\pi(a|s)$ & \tcplus{Both} \\
    \bullets{Indifference} & \tcplus{\cmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcminus{\xmark} & \tcplus{\cmark} \\ 
    \bullets{Path Consistency} & \tcminus{\xmark} & \tcminus{\xmark}  & \tcminus{\xmark}  &\tcminus{\xmark} & \tcplus{\cmark}   \\ 
    \bottomrule
\end{tabular}%
}
\vspace*{-.3cm}
\captionof{table}{Comparison to related work. }\label{table:novelty}
\headerv
\end{figure*}

==> Reward Robustness TMLR (3)/sections/new/1_tmlr_submit_prelim.tex <==
\headerv
\headerv
\section{Preliminaries}\label{sec:prelim}
\headerv

In this section, we review
% provide background on 
\gls{LP} formulations of %fully observed, 
discounted \gls{MDP} and extensions to convex policy regularization.
We begin by reviewing the convex conjugate function, also known as the Legendre-Fenchel transform, which will play a crucial role throughout our paper.

\headerv
\subsection{Convex Conjugate Function}\label{sec:conj_intro}
\headerv

% Before describing analogous primal and dual optimizations for regularized \gls{MDP}s, we review the convex conjugate function, or Legendre-Fenchel transform, which will play a crucial role throughout our paper.
%First,
For any convex function $\Omega(\primalvar)$ with domain $\primalvar \in \mathcal{D}$, 
%, where $\mathcal{D}$ may indicate the probability simplex $\Delta^{|A|}$ with possible additional constraints, such as $\mu_{\pi}(a,s) \in \mathcal{M}$
%over domain $\pi \in \Delta^{|\mathcal{A}|}$, possibly , 
%the Legendre-Fenchel transform or 
the conjugate function $\Omega^{*}$ is defined via the optimization
% \RB{what choice of primal variable? $\tpi$ is in function space in general, but will end up being a distribution}
% \RB{explain inner product notation here? what choice of primal variable $\primalvar$?} \TG{Yes both, but brief.}
\begin{align}
    \Omega^{*}( \dualvar ) = \sup \limits_{\primalvar \in \mathcal{D}} \, \big \langle \primalvar, \dualvar \big \rangle - \Omega(\primalvar) \label{eq:conjstar}
\end{align} 
where $\dualvar \in \dualdomain$ is 
% a function 
in the 
% continuous 
dual space of $\primalvar$ and $\langle \cdot, \cdot \rangle$ indicates the inner product.
% summation or integration over the dimensionality of the domain.  \RB{awkward?}
% $\mathcal{D}$ or $\dualdomain$. %continuous function in the topological dual space of $\pi$. %arbitrary function whose domain has the same dimension as $\mathcal{D}$.  
 %The conjugate function 
 The conjugate operation is an involution for proper, lower semi-continuous, convex $\Omega$ \citep{boyd2004convex},
 %(\citet{borwein2010convex} Sec. 4.3), 
 so that $(\Omega^{*})^{*} = \Omega$ and $\Omega^{*}$ is also convex.  
 We can thus represent $\Omega(\primalvar)$ via a conjugate optimization
 \begin{align}
     \Omega(\primalvar) = \sup_{\dualvar \in \dualdomain} \big \langle \primalvar, \dualvar \big \rangle - \Omega^{*}(\dualvar). \label{eq:conjomega}
 \end{align}
  %   Solving for the $\arg \sup$ in either \cref{eq:conjstar} or \cref{eq:conjomega} suggests optimality conditions for $\pi_*$ and $\dualvar$
  Differentiating with respect to the optimization variable in \cref{eq:conjstar} or (\ref{eq:conjomega}) suggests the optimality conditions 
%  \begin{align}
%      \primalvar(a,s) = \nabla \Omega^{*}( \dualvar )   \quad \qquad \dualvar(a,s) = \nabla \Omega(\primalvar) \, .     \label{eq:optimal_policy_as_grad}
%  \end{align}
% From the above, conjugacy also implies relationships of the form $\primalvar(a,s) = (\nabla \Omega)^{-1}(\dualvar(a,s))$, for example, when $\primalvar$ and $\dualvar$ are in dual correspondence.
% We provide examples of the convex conjugate for common divergence functions in \mytab{conj_table}.
  \begin{align}
     \primalvar_{\dualvar} = \nabla \Omega^{*}( \dualvar )   \quad \qquad \dualvar_{\primalvar} = \nabla \Omega(\primalvar) \, .     \label{eq:optimal_policy_as_grad}
 \end{align}
 Note that the above conditions also imply relationships of the form $\primalvar_{\dualvar} = (\nabla \Omega)^{-1}(\dualvar)$.   This dual correspondence between 
%  particular 
 values of $\primalvar$ and $\dualvar$ will form the basis of our adversarial interpretation in \mysec{adversarial_perturb}.
 
%  From the above, conjugacy also implies relationships of the form $\primalvar = (\nabla \Omega)^{-1}(\dualvar)$ when $\primalvar$ and $\dualvar$ are in dual correspondence.  
%  This correspondence will form the basis of our adversarial interpretation in \mysec{adversarial_perturb}.
%  We will make use of these conditions to associate 
%  , for example,

\headerv
\subsection{Divergence Functions}\label{sec:divergence_intro}
\headerv
% The family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases, 
% We will consider regularization using 
We are interested in the conjugate duality associated with 
policy regularization, which is often expressed using a
statistical divergence $\Omega(\mu)$ over a joint density $\mu(a,s) = \mu(s) \pi(a|s)$ (see \mysec{mdp_background}).  %commonly-used 
% where 
% The notation $\mu(a,s) = \mu(s) \pi(a|s)$ indicates a joint density
% which we will describe 
% whose meaning is described
% in \mysec{mdp_background}.
% which are used as regularization for \gls{RL} policies in \mysec{mdp_background}.   
In particular, we consider
the family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases.    
In the following, we consider extended divergences that accept unnormalized density functions as input \citep{zhu1995information} 
so that we may
% in order to 
 analyze function space dualities and evaluate Lagrangian relaxations without
%  , for example, 
projection
%the need to project 
 onto the probability simplex.
% so that Lagrangian relaxations in later sections will be well-defined even if normalization constraints are not satisfied.   

% \textcolor{red}{so that Lagrangian relaxations such as \cref{eq:dual_lagrangian} are well defined even when normalization constraints are not satisfied.}
% $\mu(a,s)$ is not normalized.}
% \textcolor{blue}{$\mu(a,s) \not \in \Delta^{|\mathcal{A}| \times |\mathcal{S}|}$.}

%  We primarily focus on policy regularization using a conditional divergence $\Omega^{(\alpha)}_{\pi_0}(\mu)$ to a reference policy $\pi_0(a|s)$.
% % but we also discuss regularization of the joint state-action occupancy to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$, in \textcolor{blue}{in \mysec{?}}.   
% Note that we consider the regularizer to be a function of $\mu(a,s)$, since it is applied 
% % in 
% across
% each 
% % $s \in \mathcal{S}$ 
% state
% % $s \sim \mu_\pi(s)$
% % \textcolor{red}{$s \sim \mu_\pi(s)$} 
% visited by the agent.
% \textcolor{blue}{In \mysec{?}}, we also discuss regularizing the joint state-action occupancy to be close to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$. 
% % \citep{nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.

% \RB{Need 2nd paragraph??  Smoother intro?}

% \RB{Remove all $\mu(s)$ below?}
% % \RB{REMOVE ALL THE $\mu(s)$ in Divergence derivations?}

\paragraph{KL Divergence}
% Taking the limit as $\alpha \rightarrow 1$, we obtain
% an (extended version of) 
The `forward' \textsc{kl} divergence to a reference policy $\pi_0(a|s)$ is commonly used for policy regularization in \gls{RL}.  
Extending the input domain to unnormalized measures, we write the divergence as
% \citep{zhu1995information},
% \citep{cichocki2010families}, 
%  (\citet{tishby2011information, ortega2013thermodynamics, fox2016taming})
\begin{align}
        &\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\Big[D_{KL}[\pi:\pi_0]\Big] = \sum \limits_{s \in \mathcal{S}} \mu(s) \sum \limits_{a \in \mathcal{A}}  \left(\pi(a|s)  \log \frac{\pi(a|s)}{\pi_0(a|s)} -  
        % \sum \limits_{a, s} 
      \pi(a|s) 
        + 
        % \sum \limits_{a,s} 
      \pi_0(a|s)\right). \label{eq:kl_def} 
\end{align}
\normalsize
Using a uniform reference  $\pi_0(a|s) = 1$ $\forall 
\, (a,s)$, we recover the Shannon entropy up to an additive constant.
%Up to an additive constant, we recover the Shannon entropy using a uniform reference, $\pi_0(a|s) = 1$ $\forall \, (a,s).$ 
% \in \mathcal{A} \times \mathcal{S}$.
% \, a \in \mathcal{A}, s \in \mathcal{S}$. 
% the final terms cancel if both $\pi$ and $\pi_0$ are normalized.


\paragraph{$\alpha$-Divergence} The $\alpha$-divergence $\mathbb{E}_{\mu(s)}\big[D_{\alpha}[\pi_0:\pi]\big]$ over possibly unnormalized measures
%$\omegamu &= \mathbb{E}_{\mu(s)}\big[D_{\alpha}[\pi_0:\pi]\big]$, 
is defined as 
% \footnotesize
\begin{align}
\hspace*{-.1cm} 
\Omega^{(\alpha)}_{\pi_0}(\mu)& =
% \mathbb{E}_{\mu(s)}\big[
% D_{\alpha}[\pi_0:\pi]
% \big]
% &= 
\frac{1}{\alpha(1-\alpha)} 
% \sum \limits_{s \in \mathcal{S}}
\sum \limits_{s \in \mathcal{S}}
\mu(s)
    \bigg( (1-\alpha) 
    % \sum \limits_{a \in \mathcal{A}} 
    \sum \limits_{a \in \mathcal{A}}
    \pi_0(a|s) 
    %+\alpha 
    % \\ &\phantom{\sum \limits_{s \in \mathcal{S}}\mu(s)} 
    + \alpha 
    % \sum \limits_{a \in \mathcal{A}} 
    \sum \limits_{a \in \mathcal{A}}
    \pi(a|s) 
    % \nonumber 
    % &- \sum \limits_{a \in \mathcal{A}} 
    % \\ &\phantom{\sum \limits_{s} \mu(s)} 
    - \sum \limits_{a \in \mathcal{A}} 
    \pi_0(a|s)^{1-\alpha} \pi(a|s)^{\alpha} \bigg)  
    % \label{eq:alpha_def}
    \label{eq:alpha_def} 
\end{align}
\normalsize
Taking the limiting behavior, we recover the `forward' \textsc{kl} divergence $D_{KL}[\pi:\pi_0]$ as $\alpha \rightarrow 1$ or the `reverse' \textsc{kl} divergence $D_{KL}[\pi_0:\pi]$ as $\alpha \rightarrow 0$.


To provide intuition for 
% for?  contextualize?  understand?}
the $\alpha$-divergence, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential, with
\begin{align}
    \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , 
    % \label{eq:qlog}  
    \qquad \qquad 
    \exp_{\alpha}(u) = [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, . \label{eq:qexp}
    % \hfill \, \,  \alpha \neq 1 \
\end{align}
\textcolor{black}{where $[\cdot]_+ = \max(\cdot,0)$ ensures fractional powers can be taken and suggests that $\exp_{\alpha}(u)=0$ for $u \leq 1/(1-\alpha)$.}
% Using $\log_{\alpha}$, 
Using the $\alpha$-logarithm, we can rewrite the $\alpha$-divergence 
% in similar fashion to
similarly to
the \kl divergence in 
\cref{eq:kl_def}
% \scriptsize
\resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
\begin{align}
  \Omega^{(\alpha)}_{\pi_0}(\mu) &= \frac{1}{\alpha} \sum \limits_{s \in \mathcal{S}} \mu(s) \bigg( \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)} - \pi(a|s) + \pi_0(a|s) \bigg) \nonumber.
\end{align}
}}
\normalsize
For a uniform reference $\pi_0$, the $\alpha$-divergence 
differs from the Tsallis entropy by only the $1/\alpha$ factor and an additive constant (see \myapp{tsallis}).

\headerv
\subsection{Unregularized MDPs}\label{sec:mdp_background}
% \subsection{MDPs as Linear or Convex Programs}\label{sec:mdp_background}
% \subsection{Linear $\&$ Convex Programming Formulations of MDPs}
\headerv
% \vspace*{\header}

% \paragraph{Unregularized Case}
A discounted \gls{MDP} is a tuple $\{ \mathcal{S}, \mathcal{A}, P, \nu_0, r, \gamma \}$ consisting of a state space $\mathcal{S}$, action space $\mathcal{A}$, transition dynamics $P(s\tick|s,a)$ for $s, s\tick \in \mathcal{S}$, $a \in \mathcal{A}$, initial state distribution $\nu_0(s) \in \Delta^{|\mathcal{S}|}$ in the probability simplex, and reward function $r(a,s):\mathcal{S} \times \mathcal{A} \mapsto \mathbb{R}$.   We also use a discount factor $\gamma\in (0,1)$ 
(\citet{puterman2014markov} Sec 6).
% , although discounting may also be handled by including a transition to an absorbing state in the \gls{MDP} (\citet{puterman2014markov} Sec. 5.3). 
% in the \gls{MDP}

% \paragraph{Unregularized Case}
We consider an agent that seeks to maximize the expected discounted reward by acting according to a decision policy 
% $\{ \pi(a|s) \in \Delta^{|\mathcal{A}|} \}_{s \in \mathcal{S}}$.
$\pi(a_t|s_t) \in \Delta^{|\mathcal{A}|}$. %\, \,\, {\forall s_t \in \mathcal{S}}  
The expected reward is calculated over trajectories ${\tau \sim \pi(\tau):= \nu_0(s_0) \prod \pi(a_t | s_t) P(s_{t+1} | s_t, a_t)}$, which begin from an initial $s_0 \sim \nu_0(s)$ and evolve according to the policy and \gls{MDP} dynamics $P(s\tick|s,a)$  
% We consider an agent that acts according to a decision policy $\pi(a_t|s_t) \in \Delta^{|\mathcal{A}|}$, seeking to maximize the expected discounted reward over trajectories ${\tau \sim \pi(\tau):= \nu_0(s_0) \prod \pi(a_t | s_t) P(s_{t+1} | s_t, a_t)}$ which start from $s_0 \sim \nu_0(s)$ and evolve according to the policy and \gls{MDP} dynamics $P(s\tick|s,a)$.  
% Thus, the objective in \cref{eq:primal_lp} can be rewritten in similar fashion to \cref{eq:reward_perturbation_stmt}
% This leads to the objective function
\small
\begin{align}
  \hspace*{-.2cm}
  \obj(r) := 
   \max \limits_{\pi(a|s)} \, (1-\gamma) \, \mathbb{E}_{\tau \sim \pi(\tau)} \bigg[ \sum \limits_{t=0}^{\infty} \gamma^t \, r(s_t, a_t)  \bigg] \, . \label{eq:policy_only} 
\end{align}
\normalsize
We assume that the policy is stationary and Markovian, and thus independent of both the timestep and trajectory history.  

% \paragraph{MDPs as Linear Programs}
\paragraph{Linear Programming Formulation}
% % \RB{We adopt notation, For the remainder of the paper, heavy use}
% % To highlight connections with the literature on convex duality, we consider 
% For the remainder of the paper, we will consider
% an equivalent \gls{LP} formulation in which optimization is performed over the discounted 
% % joint 
% state-action occupancy measure 
% $\mu(a,s) \coloneqq (1-\gamma) \mathbb{E}_{\tau\sim \pi(\tau)} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$,
% % with
% For the remainder of this work, 
In what follows, we will focus on 
a linear programming (\gls{LP}) form for the objective in \cref{eq:policy_only}, which is common in the literature on convex duality.
% an equivalent \gls{LP} formulation which is common in the literature on convex duality.   
With optimization over the discounted 
state-action occupancy measure, 
% ${\mu(a,s) \coloneqq (1-\gamma)} \mathbb{E} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$, we have
${\mu(a,s) \coloneqq (1-\gamma)} \mathbb{E}_{\tau\sim \pi(\tau)} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$, the objective can be rewritten
% becomes
% With optimization over the discounted 
% state-action occupancy measure 
% ${\mu(a,s) \coloneqq (1-\gamma)} \mathbb{E}_{\tau\sim \pi(\tau)} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$, 
% \small
% \begin{align}
%   \hspace*{-.2cm} &  
%   \obj(r) :=
%   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \, \, \text{subj. to} \, \quad    \left( \forall s \in \mathcal{S} \right) \label{eq:primal_lp}\\[1.25ex]
%   &\sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \nonumber  \, ,
%   %\, \forall s \in \mathcal{S}\nonumber
% \end{align}
\small
\begin{align}
   \hspace*{-.23cm}  
   \obj(r) \coloneqq
   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \qquad \text{subject to } \quad \mu(a,s) &\geq 0 \qquad \forall (a,s) \in \mathcal{A} \times \mathcal{S},   \quad  \label{eq:primal_lp} \\
    \sum_{a} \mu(a,s)& = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \qquad \forall s \in \mathcal{S}, \nonumber 
   %\left( \forall s \in \mathcal{S} \right) 
   %\, \forall s \in \mathcal{S}\nonumber
\end{align}
% \small
% \begin{align}
%   \hspace*{-.23cm}  
%   \obj(r) \coloneqq
%   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \qquad \text{subject to } \quad \forall (a,s) \in \mathcal{A} \times \mathcal{S}:&   \quad  \mu(a,s) \geq 0  \label{eq:primal_lp} \\
%     \quad \forall s \in \mathcal{S}:& \quad \sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick)  \nonumber 
%   %\left( \forall s \in \mathcal{S} \right) 
%   %\, \forall s \in \mathcal{S}\nonumber
% \end{align}
% \footnotesize
% \begin{align}
%   \hspace*{-.2cm} &  
%   \obj(r) :=
%   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \, \, \label{eq:primal_lp} \\
%   &\phantom{ \obj(r) :=} \text{subj. to} \, \,\mu(a,s) \geq 0 \quad \forall (a, s) \in \mathcal{A} \times \mathcal{S}   \nonumber  \\[1.25ex] %
%   &\sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \, \,  \forall s \in \mathcal{S}  \nonumber  \, , %\left( \forall s \in \mathcal{S} \right)
%   %\, \forall s \in \mathcal{S}\nonumber
% \end{align}
\normalsize
% \RB{$\mu(a,s) \geq 0 $ leads to $V \geq r + \gamma\transitionv$ \textit{inequality} constraint}
where inner product notation 
% $\langle \cdot, \cdot \rangle$ 
indicates summation or integration over the domain of $\mu$. 
% and nonnegativity constraints apply for each $(a, s) \in \mathcal{A} \times \mathcal{S}$. %\RB{improve} %$\sum \mu \cdot \dualvar$
%The optimization is over state-action visitation distributions $\mu(a,s) \in \Delta^{|\mathcal{S}| \times |\mathcal{A}|} $, and a corresponding policy is obtained via $\pi(a|s) = \mu(a,s) / \sum_a \mu(a,s)$.   
We refer to the constraints in the second line of \cref{eq:primal_lp} as the \textit{Bellman flow constraints}, which force $\mu(a,s)$ to respect the \gls{MDP} dynamics.
%and denote the set of feasible $\mu$ as $\mathcal{M}$. For normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$, we show in \myapp{normalized_mu} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized.
We denote the set of feasible $\mu$ as $\mathcal{M}$.    For normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$,   we show in \myapp{optimal_policy} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s)$
% \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ 
is normalized. 
% we show in \myapp{normalized_mu} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized. 
% We denote the set of feasible $\mu$ as $\mathcal{M}$
% % For normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$, we show in \myapp{normalized_mu} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized. 
% and in \myapp{normalized_mu}, show that $\mu(a,s) \in \mathcal{M}$ implies that $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized for normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$.
% % assuming $\nu_0(s)$ and $P(s|a\tick, s\tick)$ are normalized.

% \RB{Flow constraints force $\mu$ to respect dynamics}
% \RB{Mention that $\nu_0(s), P(s\tick|s,a)$ normalized implies $\mu(a,s) \in \mathcal{M}$ normalized} 
\input{sections/conj_table}

It can be shown that any feasible $\mu(a,s) \in \mathcal{M}$  induces a stationary $\pi(a|s) = \mu(a,s) / 
\mu(s)$, 
% \sum_{a\tick} \mu(a\tick,s)
where  $\mu(s) \coloneqq \sum_{a\tick} \mu(a\tick,s)$ and $\pi(a|s) \in \Delta^{|\mathcal{A}|}$ is normalized by definition.
% \footnote{To see this, since $\sum_a \frac{\mu(a,s)}{\sum_{a'} \mu(s)}= \frac{\sum_a \mu(a,s)}{\mu(s)} = 1$.} 
% \footnote{The policy is always normalized 
% % even if $\mu(a,s)$ is not, 
% since $\sum_a \frac{\mu(a,s)}{\sum_{a'} \mu(s)}= \frac{\sum_a \mu(a,s)}{\mu(s)} = 1$.}$
Conversely, any stationary policy $\pi(a|s)$ induces a unique state-action visitation distribution $\mu(a,s)$ (\citet{syed2008apprenticeship},
\citet{feinberg2012handbook} Sec. 6.3).
%\citet{puterman2014markov} Sec. ??).
 Along with the definition of $\mu(a,s)$ above, 
%  this demonstrates 
this result demonstrates
 the equivalence of the optimizations in \cref{eq:policy_only} and \cref{eq:primal_lp}.  We will proceed with the \gls{LP} notation from \cref{eq:primal_lp} and assume $\mu(s)$ is induced by
%the corresponding 
$\pi(a|s)$ whenever the two appear together in an expression.
% It can be shown that any stationary policy $\pi(a|s)$ induces a unique state-action 
% visitation distribution $\mu(a,s)$, while, conversely, a feasible $\mu(a,s) \in \mathcal{M}$  is induced by some stationary $\pi(a|s) = \mu(a,s) / \mu(s)$ (\citep{syed2008apprenticeship}, \citet{feinberg2012handbook} Sec. 6.3).   

% where the marginal state-visitation distribution $\mu(s) \propto (1-\gamma) \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(s_t = s)$ a
% The flow constraints in \cref{eq:primal_lp} are insightful, as they lead to a dual optimization reflecting the familiar Bellman equations \citep{bellman1957markovian}. 
Importantly, the flow constraints in \cref{eq:primal_lp} lead to a dual optimization which reflects the familiar Bellman equations \citep{bellman1957markovian}. 
To see this, we introduce Lagrange multipliers $V(s)$ for each flow constraint and $\lambdaplus \geq 0$ for the nonnegativity constraints.  Summing over $s \in \mathcal{S}$, and eliminating $\mu(a,s)$ by setting $d/d\mu(a,s) = 0$ yields the \textit{dual} \gls{LP}
% Introducing Lagrange multipliers $V(s)$ for each flow constraint, summing over $s \in \mathcal{S}$, and eliminating $\mu(a,s)$ by setting $d/d\mu(a,s) = 0$ yields the \textit{dual} \gls{LP}
% \begin{align}
%   &\obj^{*}(r):=\min \limits_{V(s)} \,  (1-\gamma) \big \langle \nu_0(s), V(s) \big \rangle \, \text{  subj to: }\, \label{eq:dual_lp} \\ %\quad \forall (a,s) \in \mathcal{S} \times \mathcal{A}
%   & \, V(s) = r(a,s) + \gamma \transitionv + \lambdaplus 
% %   \,\, \forall (a,s) \in \mathcal{A} \times \mathcal{S}  
%  \nonumber \, ,
% \end{align}
% \small
\begin{align}
 \hspace*{-.2cm} \obj^{*}(r)&\coloneqq
  \min \limits_{V(s), \lambdaplus} \,
%   \min \limits_{V(s)} \,  
  (1-\gamma) \big \langle \nu_0(s), V(s) \big \rangle  
%   \\
%   \text{  subj to: }\label{eq:dual_lp} \\ %\quad \forall (a,s) \in \mathcal{S} \times \mathcal{A}
 \quad \text{  subject to } \,\,\, V(s) = r(a,s) + \gamma \transitionv + \lambdaplus 
%  \quad \forall (a,s) \in \mathcal{A} \times \mathcal{S}  
 \label{eq:dual_lp} , 
%  \nonumber \, ,
\end{align}
\normalsize
% where the constraint applies for all $(a,s) \in \mathcal{A} \times \mathcal{S}$ and $\lambdaplus \geq 0$.  By complementary slackness \citep{boyd2004convex}, we know that $\lambdaplus =0$ for $\mu(a,s) > 0$.
% Finally,  we use $\transitionv$ as shorthand for $\mathbb{E}_{P(s\tick|a,s)}[ V(s\tick)]$ and have reindexed the transition tuple from $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared to \cref{eq:primal_lp}. 
where we have used $\transitionv$ as shorthand for $\mathbb{E}_{P(s\tick|a,s)}[ V(s\tick)]$ and reindexed the transition tuple from $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared to \cref{eq:primal_lp}.   Note that the constraint applies for all $(a,s) \in \mathcal{A} \times \mathcal{S}$ and that $\lambdaplus \geq 0$.  By complementary slackness, 
% \citep{boyd2004convex}, 
we know that $\lambdaplus =0$ for $(a,s)$ such that $\mu(a,s) > 0$.

% In similar fashion to the conjugate optimizations in \cref{eq:conjstar}-\ref{eq:conjomega}, these dual objectives have the same solution under strong duality, despite optimizing over different variables.

% where the constraint applies for all $(a,s) \in \mathcal{A} \times \mathcal{S}$ and $\lambdaplus \geq 0$.  By complementary slackness, 
% % \citep{boyd2004convex}, 
% we know that $\lambdaplus =0$ for $(a,s)$ such that $\mu(a,s) > 0$.
% Finally, we have used $\transitionv$ as shorthand for $\mathbb{E}_{P(s\tick|a,s)}[ V(s\tick)]$ and reindexed the transition tuple from $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared to \cref{eq:primal_lp}. 

% By complementary slackness \citep{boyd2004convex}, we know that $\lambdaplus =0$ for $(a,s)$ such that $\mu(a,s) > 0$.
% It is easy to show that the optimal policy is deterministic if $a_{\text{max}} \coloneqq \arg \max_a r(a,s) + \gamma \transitionv$ is unique, with $\pi_*(a_{\text{max}}|s) = 1$ and $V(s) = r(a_{\text{max}},s) + \gamma 
% \mathbb{E}_{a_{\text{max}},s}^{s\tick}\left[V(s\tick)\right]$.
% % \transitionv$
% $\lambda(a_{\text{max}}, s) = V(s) - r(a,s) - \gamma \transitionv > 0$.

% \paragraph{Regularized Case}
\headerv
\subsection{Regularized MDPs}\label{sec:mdp_regularized}
\headerv
We now consider regularizing the objective in \cref{eq:primal_lp} using a convex penalty function $\Omega(\mu)$ with coefficient $1/\beta$.   
We primarily focus on regularization using a conditional divergence $\Omega_{\pi_0}(\mu) \coloneqq \mathbb{E}_{\mu(s)\pi(a|s)}[\ptReg(\pi)]$ between the policy and a normalized reference distribution $\pi_0(a|s)$, as in \mysec{divergence_intro} and \citep{ortega2013thermodynamics,fox2016taming,haarnoja17a,haarnoja2018soft}.   
We also use the notation $\Omega_{\mu_0}(\mu) = \mathbb{E}_{\mu(a,s)}[\ptReg(\mu)]$ to indicate regularization of the full state-action occupancy measure to a normalized reference $\mu_0(a,s)$,  which appears, for example, in \gls{REPS} \citep{peters2010relative, belousov2019entropic}.   
% We assume the reference is normalized, either $\sum_a \pi_0(a|s) =1$ or $\sum_{a,s} \mu_0(a,s)=1$.
% We will also consider regularization of the full state-action occupancy measure to a reference $\mu_0(a,s)$, using the notation $\Omega_{\mu_0}(\mu) = \mathbb{E}_{\mu(a,s)}[\ptReg(\mu)]$ \citep{peters2010relative, belousov2019entropic, basserrano2021logistic}.
% The regularizer may be either a conditional divergence $\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)\pi(a|s)}[\ptReg(\pi)]$ between the policy and a reference distribution $\pi_0(a|s)$, or a divergence $\Omega_{\mu_0}(\mu) = \mathbb{E}_{\mu(a,s)}[\ptReg(\mu)]$ over the joint state-action occupancy measure with reference $\mu_0(a,s)$. \RB{?? Later.  reference \mysec{divergence_intro}}
% % We will consider $\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)\pi(a|s)}[\ptReg(\pi)]$ to be a conditional divergence between the policy and a reference distribution $\pi_0(a|s)$ that can be written with an outer expectation over $\mu(a,s)$.~\footnote{We focus on policy regularization \citep{neu2017unified} in this work, but similar reasoning may be applied for regularizing the joint state-action occupancy $\mu(a,s)$ \citep{nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.} 
% Letting $\Omega_{\pi_0}(\pi)$ be a statistical divergence between the policy and a reference distribution $\pi_0(a|s)$, 
% We define the regularized objective as 
The regularized objective $\obj_{\Omega, \beta}(r)$ is then defined as
% $\obj_{\Omega, \beta}(r)$
\begin{equation}
% \resizebox{.87\columnwidth}{!}{ \hspace*{-.2cm}   $
\obj_{\Omega, \beta}(r) :=  \max \limits_{\mu(a,s) \in \mathcal{M} } %\max \limits_{\pi(a|s) \in \Delta^{|A|}} 
   \blangle \mu(a,s), r(a,s) \brangle - \dfrac{1}{\beta}   \Omega_{\pi_0}(\mu) 
%   $ 
%   }
  \label{eq:primal_reg}
\end{equation}
where $\Omega_{\pi_0}(\mu)$ contains an expectation under $\mu(a,s)$ as in \cref{eq:kl_def}-(\ref{eq:alpha_def}).
We can also derive a dual version of the regularized \gls{LP}, 
by first writing the Lagrangian relaxation of \cref{eq:primal_reg}
% starting from a Lagrangian relaxation of \cref{eq:primal_reg}
%\max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}}
% \begin{align}
%     %\mathcal{L}(\mu, V, \Omega) := 
%     & \min \limits_{V(s)} \max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}} \, 
%      (1-\gamma) \big\langle \nu_0, V(s) \big  \rangle \\
%      + &\blangle \mu(s)\pi(a|s), r(a,s) +  \gamma \transitionv -V(s) \big \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \nonumber \\
%     &   \label{eq:lagrangian}\, ,
% \end{align}
% \resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
% \scriptsize
\begin{align}
%   \mathcal{L}:= 
  \max \limits_{\mu(a,s)} \min \limits_{V(s), \lambdaplus}  \, 
     (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle 
     + &\langle \mu(a,s), r(a,s) + \gamma \transitionv -V(s) + \lambdaplus \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\mu)  \label{eq:dual_lagrangian} 
\end{align}
\normalsize
% }}
% \resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
% \begin{align}
%   & 
% %   \mathcal{L}:= 
%   \max \limits_{\mu(a,s)} \min \limits_{V(s)}  \, 
%      (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle  \label{eq:dual_lagrangian} \\
%      + &\blangle \mu(a,s), r(a,s) +  \gamma \transitionv -V(s)\brangle - \frac{1}{\beta} \Omega_{\pi_0}(\mu)  \nonumber
% \end{align}
% }}
Swapping the order of optimization 
% using
under 
strong duality, we can recognize the 
maximization over ${\mu(a,s)}$ as a conjugate function $\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}$, as in \cref{eq:conjstar}, leading to a regularized dual optimization
% \resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
 \begin{align}
 \hspace*{-.2cm} &  \obj_{\Omega, \beta}^{*}(r) = 
%  \min \limits_{V(s)} 
 \min \limits_{V(s), \lambdaplus}
 %\max \limits_{ \mu(s) \rightarrow \mathcal{M}}
 \,  (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle  + \frac{1}{\beta}\Omega^{*}_{\pi_0, \beta} \bigg(r(a,s) +  \gamma \transitionv -V(s) + \lambdaplus \bigg)\label{eq:dual_reg} 
%  &+ \mathbb{E}_{\mu(s)} \bigg[\, \frac{1}{\beta}\Omega^{*}_{\pi_0, \beta} \bigg(r(a,s) +  \gamma \transitionv -V(s) \bigg)  \bigg] \nonumber
\end{align}
% }}
% \RB{Omit this, instead consider soft value aggregation? }
which involves optimization over dual variables $V(s)$ only and is unconstrained, in contrast to \cref{eq:dual_lp}. %, and involves sampling under the induced marginal distribution $\mu(s)$. 
% Similar dual objectives
Dual objectives of this form 
% have been considered 
appear 
in \citep{nachum2020reinforcement, belousov2019entropic, basserrano2021logistic, neu2017unified}.
\textcolor{black}{We emphasize the need to include the Lagrange multiplier $\lambdaplus$, with $\lambdaplus > 0$ when the optimal policy has $\piopt(a|s) = 0$, since an important motivation for $\alpha$-divergence regularization is to encourage sparsity in the policy (see \cref{eq:qexp}, \citet{lee2018sparse, lee2019tsallis, chow2018path}).}


\paragraph{Soft Value Aggregation}
In iterative algorithms such as (regularized) modified policy iteration \citep{puterman1978modified, scherrer15a}, it is useful to consider the \textit{regularized Bellman optimality operator} \citep{geist2019theory}.   For given estimates of the state-action value $Q(a,s) \coloneqq r(a,s) + \gamma \transitionv$, the operator $\mathcal{T}^{*}_{\Omega_{\pi_0, \beta}}$ updates $V(s)$ as
% \scriptsize
\begin{align} 
\hspace*{-.2cm} V(s)  \leftarrow \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(Q) = \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \blangle \pi(a|s), Q(a,s) \brangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \label{eq:soft_value}
\end{align}
\normalsize
Note that this conjugate optimization is performed in each state $s \in \mathcal{S}$ and explicitly constrains each $\pi(a|s)$ to be normalized.
Although we proceed with the notation of \cref{eq:primal_reg} and \cref{eq:dual_reg}, our later developments 
% for conditional policy regularization 
are compatible with the
% the regularized Bellman operator or 
`soft-value aggregation' perspective above.  See \myapp{soft_value} for detailed discussion.
% We provide detailed discussion in \myapp{soft_value}.
% We provide a detailed discussion of this `soft-value aggregation' operator in \myapp{soft_value}.   While we proceed with the notation of \cref{eq:dual_reg}
% While our developments in later sections focus on
% Our developments in later sections are compatible with this approach,

%%%%%%%%%%%%%%%%%%%%%%%%%% Prev Divergence Functions Paragraph %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Divergence Functions}\label{sec:divergence_intro}
% \RB{MOVE and modify this intro to fit?}

% % The family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases, 
% We consider regularization using the family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases.    
% We extend these divergences to accept unnormalized density functions as input \citep{zhu1995information}, \textcolor{red}{so that Lagrangian relaxations such as \cref{eq:dual_lagrangian} are well defined even when 
% normalization constraints are not satisfied.}
% % $\mu(a,s)$ is not normalized.}
% % \textcolor{blue}{$\mu(a,s) \not \in \Delta^{|\mathcal{A}| \times |\mathcal{S}|}$.}

%  We primarily focus on policy regularization using a conditional divergence $\Omega^{(\alpha)}_{\pi_0}(\mu)$ to a reference policy $\pi_0(a|s)$.
% % but we also discuss regularization of the joint state-action occupancy to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$, in \textcolor{blue}{in \mysec{?}}.   
% Note that we consider the regularizer to be a function of $\mu(a,s)$, since it is applied 
% % in 
% across
% each 
% % $s \in \mathcal{S}$ 
% state
% % $s \sim \mu_\pi(s)$
% % \textcolor{red}{$s \sim \mu_\pi(s)$} 
% visited by the agent.
% \textcolor{blue}{In \mysec{?}}, we also discuss regularizing the joint state-action occupancy to be close to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$. 
% % \citep{nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.

% \RB{Need 2nd paragraph??  Smoother intro?}

% \RB{Remove all $\mu(s)$ below?}
% % \RB{REMOVE ALL THE $\mu(s)$ in Divergence derivations?}

% \paragraph{KL Divergence}
% % Taking the limit as $\alpha \rightarrow 1$, we obtain
% % an (extended version of) 
% The forward \textsc{kl} divergence is commonly used for policy regularization in \gls{RL}.  Extending to unnormalized measures 
% \citep{zhu1995information},
% % \citep{cichocki2010families}, 
% %  (\citet{tishby2011information, ortega2013thermodynamics, fox2016taming})
% \footnotesize
% \begin{align}
%         &\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\bigg[D_{KL}[\tpi:\tpi_0]\bigg] \label{eq:kl_def} \\
%         &\phantom{\Omega} = \sum \limits_{s \in \mathcal{S}} \mu(s) \sum \limits_{a \in \mathcal{A}}  \left(\tpi(a|s)  \log \frac{\tpi(a|s)}{\tpi_0(a|s)} -  
%         % \sum \limits_{a, s} 
%       \tpi(a|s) 
%         + 
%         % \sum \limits_{a,s} 
%       \tpi_0(a|s)\right). \nonumber
% \end{align}
% % \begin{align}
% %     % \hspace*{-.15cm} D_{KL}[\tpi:\tpi_0] = \sum \limits_{a \in \mathcal{A}} \tpi(a|s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} - \tpi(a|s) + \tpi_0(a|s) \, . \nonumber
% %         % \hspace*{-.2cm}  
% %         \Omega&_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\bigg[D_{KL}[\tpi:\tpi_0]\bigg] \label{eq:kl_def} \\
% %         &= \sum \limits_{a, s} \mu(a,s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} -  
% %         % \sum \limits_{a, s} 
% %         \mu(s) \tpi(a|s) 
% %         + 
% %         % \sum \limits_{a,s} 
% %         \mu(s) \tpi_0(a|s)
% %       . \nonumber
% %         % \sum \limits_{a, s} \mu(a,s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
% %         % \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
% %         % \textcolor{red}{ -\sum \limits_{a \in \mathcal{A}} \tpi(a|s) +\sum \limits_{a \in \mathcal{A}} \tpi_0(a|s) } 
% %     %\sum \limits_{a \in \mathcal{A}} %\lim_{\alpha \rightarrow 1}
% % \end{align}
% \normalsize
% Up to an additive constant, we recover the Shannon entropy using a uniform reference, $\pi_0(a|s) = 1$ $\forall 
% \, (a,s).$ 
% % \in \mathcal{A} \times \mathcal{S}$.
% % \, a \in \mathcal{A}, s \in \mathcal{S}$. 
% % the final terms cancel if both $\tpi$ and $\tpi_0$ are normalized.


% \paragraph{$\alpha$-Divergence} The $\alpha$-divergence $\mathbb{E}_{\mu(s)}\big[D_{\alpha}[\tpi_0:\tpi]\big]$ over possibly unnormalized measures
% %$\omegamu &= \mathbb{E}_{\mu(s)}\big[D_{\alpha}[\tpi_0:\tpi]\big]$, 
% is defined as 
% \footnotesize
% \begin{align}
% \hspace*{-.1cm} 
% \Omega^{(\alpha)}_{\pi_0}(\mu)&=
% % \mathbb{E}_{\mu(s)}\big[
% % D_{\alpha}[\tpi_0:\tpi]
% % \big]
% % &= 
% \frac{1}{\alpha(1-\alpha)} 
% % \sum \limits_{s \in \mathcal{S}}
% \sum \limits_{s \in \mathcal{S}}
% \mu(s)
%     \bigg( (1-\alpha) 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a \in \mathcal{A}}
%     \tpi_0(a|s) 
%     %+\alpha 
%     \\ &\phantom{\sum \limits_{s \in \mathcal{S}}
% \mu(s)} + \alpha 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a \in \mathcal{A}}
%     \tpi(a|s) \nonumber 
%     % &- \sum \limits_{a \in \mathcal{A}} 
%     % \\ &\phantom{\sum \limits_{s} \mu(s)} 
%     - \sum \limits_{a \in \mathcal{A}} 
%     \tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} \bigg)  \label{eq:alpha_def}
% \end{align}
% \normalsize
% To provide intuition for 
% % for?  contextualize?  understand?}
% the $\alpha$-divergence, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential, with
% \begin{align}
%     \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , \\
%     \exp_{\alpha}(u) &= [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, .
%     % \hfill \, \,  \alpha \neq 1 \
% \end{align}
% % Using $\log_{\alpha}$, 
% Using the $\alpha$-logarithm, we can rewrite the $\alpha$-divergence 
% % in a form similar to 
% similarly to
% the \kl divergence in 
% \cref{eq:kl_def}.
% \scriptsize
% \begin{align}
%   \Omega^{(\alpha)}_{\pi_0}(\mu) &= \frac{1}{\alpha} \sum \limits_{s \in \mathcal{S}} \mu(s) \bigg( \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)} - \pi(a|s) + \pi_0(a|s) \bigg) \nonumber
% \end{align}
% \normalsize
% For a uniform reference, the $\alpha$-divergence 
% differs from the Tsallis entropy by only the $1/\alpha$ factor and an additive constant (see \myapp{tsallis}).


% \RB{Bridge}





%%%%%%%%%%%%%%%%%%%%%%%%%% END OF Prev Divergence Functions Paragraph %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





% As discussed in \myapp{tsallis}, the $\alpha$-divergence is closely related to the Tsallis entropy. \RB{Introduce $\log_{\alpha}$ first? (with the goal of reaching this insight)}
% \citep{lee2019tsallis}, as we discuss in detail in \myapp{tsallis}.  
% To see this, 

% For later convenience, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential,
% % \small
% % \begin{align}
% %     \log_{\alpha}(u) &= \begin{cases} \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \hfill \, \, \alpha \neq 1 \\
% %     \log(u) \hfill \, \, \alpha =1 \end{cases} \\
% %     \exp_{\alpha}(u) &= \begin{cases} [1 + (\alpha-1) \cdot u ]_+^{\frac{1}{\alpha-1}} \hfill \, \,  \alpha \neq 1 \\
% %     \exp(u) \hfill \, \, \alpha =1 \end{cases} \, .
% % \end{align}
% \begin{align}
%     \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , \\
%     \exp_{\alpha}(u) &= [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, .
%     % \hfill \, \,  \alpha \neq 1 \
% \end{align}
% \begin{equation}
% \resizebox{.87\columnwidth}{!}{\hspace*{-.36cm}
%     $\log_{\alpha}(u) &= \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \\
%     \quad 
%     \exp_{\alpha}(u) = [1 + (\alpha-1) u ]_+^{\frac{1}{\alpha-1}}$
% }
% \end{equation}
% \normalsize
% and we recover the natural logarithm and exponential in the limit as $\alpha \rightarrow 1$.


% \textcolor{blue}{
% We consider regularization of the policy $\pi(a|s)$ to a reference $\pi_0(a|s)$, with analogous derivations for  regularization of $\mu(a,s)$ to a reference $\mu_0(a,s)$ in \myapp{mu_results}.}
% \RB{Decide how to handle $\mu$ vs. $\pi$ regularization.  Difference is insightful for $\alpha$-divergence}

% \paragraph{KL Divergence}
% % Taking the limit as $\alpha \rightarrow 1$, we obtain
% % an (extended version of) 
% The forward \textsc{kl} divergence commonly used as regularization in \gls{RL} is defined as
% %  (\citet{tishby2011information, ortega2013thermodynamics, fox2016taming})
% \footnotesize
% \begin{align}
%     % \hspace*{-.15cm} D_{KL}[\tpi:\tpi_0] = \sum \limits_{a \in \mathcal{A}} \tpi(a|s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} - \tpi(a|s) + \tpi_0(a|s) \, . \nonumber
%         % \hspace*{-.2cm}  
%         \Omega&_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\bigg[D_{KL}[\tpi:\tpi_0]\bigg] \label{eq:kl_def} \\
%         &= \sum \limits_{a, s} \mu(a,s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} -  
%         % \sum \limits_{a, s} 
%         \mu(s) \tpi(a|s) 
%         + 
%         % \sum \limits_{a,s} 
%         \mu(s) \tpi_0(a|s)
%       . \nonumber
%         % \sum \limits_{a, s} \mu(a,s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
%         % \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
%         % \textcolor{red}{ -\sum \limits_{a \in \mathcal{A}} \tpi(a|s) +\sum \limits_{a \in \mathcal{A}} \tpi_0(a|s) } 
%     %\sum \limits_{a \in \mathcal{A}} %\lim_{\alpha \rightarrow 1}
% \end{align}
% \normalsize
% \RB{$\tpi$ or $\pi$?}
% To derive a closed form for the convex conjugate function, we consider the conditional \kl divergence as a function of $\mu(a,s)$ in the following conjugate optimization
% \footnotesize
% \begin{align}
%   \hspace*{-.25cm}  &\klconjpii(\dualvar) = \max \limits_{\mu(a,s)} \blangle 
%     \mu(a,s), \dualvar(a,s)
%     % \mu(a,s), \dualvar(a,s)
%     \brangle - \klomegamu \label{eq:kl_conj} \\
%   &= \frac{1}{\beta} \sum \limits_s \mu(s) 
%   \left(
%   \sum \limits_{a} \pi_0(a|s) \expof{\beta \cdot \dualvar(a,s)} - \sum \limits_{a} \pi_0(a|s) 
%   \right)
%   \nonumber
% %   &= \frac{1}{\beta} \log \sum \limits_{a,s} \mu(s) \pi_0(a|s) \expof{\beta \cdot \dualvar(a,s)}
%     % - \blangle \lambda , \mu(a,s) - 1\brangle
% \end{align}
% \normalsize
% where the \textcolor{red}{optimizing argument is 
% the occupancy measure
% induced by } $\pir(a|s) = \pi_0(a|s)\exp\{\beta \cdot \dualvar(a,s)\} $.
% See \myapp{kl_conj_all} for detailed derivations.  Note that the log-sum-exp form of the conjugate function arises from enforcing a normalization constraint on the optimization variable \citep{ruderman2012tighter}.   
% % $\mu(a,s) \in \Delta^{\mathcal{A} \times \mathcal{S}}$.

% % Finally, note that the optimizing argument for the conjugate in \cref{eq:kl_conj} is given by 
% % \begin{align}
% %     \piopt(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( \dualvar(a,s) \big) } 
% % \end{align}
% % where $\muopt(a,s) = \muopt(s) \piopt(a|s)$ is induced from $\piopt(a|s)$.

% % With detailed derivations in \myapp{kl_conj_all}, the solution to the conjugate optimization is
% % Considering this conditional \kl divergence as a function of $\mu(a,s)$ and enforcing normalization, we obtain the following conjugate optimization.   With detailed derivations in \myapp{kl_conj_all}, 

% % normalized mu conjugate with log-sum-exp solution
% % \footnotesize
% % \begin{align}
% %   \hspace*{-.25cm}   \klconjpii(\dualvar) &= \max \limits_{\mu(a,s) \in \Delta^{|\mathcal{A}| \times |\mathcal{S}|}} \blangle 
% %     \mu, \dualvar 
% %     % \mu(a,s), \dualvar(a,s)
% %     \brangle - \klomegamu \\
% %   &= \frac{1}{\beta} \log \sum \limits_{a,s} \mu(s) \pi_0(a|s) \expof{\beta \cdot \dualvar(a,s)}
% %     % - \blangle \lambda , \mu(a,s) - 1\brangle
% % \end{align}
% % \normalsize

% % \RB{Emphasize derivation of $\pi_* = \nabla \Omega^{*}(Q)$}
% % The value function, or conjugate $\alphaconjn(Q)$, as a function $Q$ and with restriction to normalized $\pi$, is

% %For the \textsc{kl} divergence, 
% % This matches the normalization constant for the optimal policy, with $V_*(s) = \psi(s;\beta)$ and
% %  \begin{align}
% %  \pi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s) -  \psi(s;\beta)\big)} \, ,\label{eq:kl_opt_policy}
% %  \end{align}
% % This can also be seen by plugging $\alpha = 1$ into \cref{eq:alpha_conj_norm_main}.
% % Apart from the case of $\alpha=1$, we can see from \cref{eq:alpha_conj_norm_main} that $V_*(s) \neq \normalizeralpha$.
% % We discuss the relationship between $V_*(s)$ and $\normalizeralpha$ for general $\alpha$ in more detail in \mysec{optimal_policy}, while the optimal policy expressions in \cref{eq:alpha_opt_policy} and (\ref{eq:kl_opt_policy}) will also play a central role.


% \paragraph{$\alpha$-Divergence} The $\alpha$-divergence over possibly unnormalized measures,  $\omegamu &=
% \mathbb{E}_{\mu(s)}\big[
% D_{\alpha}[\tpi_0:\tpi]
% \big]$, is defined as 
% \footnotesize
% \begin{align}
% \hspace*{-.15cm} 
% \omegamu &=
% % \mathbb{E}_{\mu(s)}\big[
% % D_{\alpha}[\tpi_0:\tpi]
% % \big]
% % &= 
% \frac{1}{\alpha(1-\alpha)} 
% % \sum \limits_{s \in \mathcal{S}}
% \sum \limits_{s}
% \mu(s)
%     \bigg( (1-\alpha) 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a} 
%     \tpi_0(a|s) 
%     %+\alpha 
%     \\ \phantom{\sum \limits_{s}
% \mu(s)} + \alpha 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a} 
%     \tpi(a|s) \nonumber 
%     % &- \sum \limits_{a \in \mathcal{A}} 
%     % \\ &\phantom{\sum \limits_{s} \mu(s)} 
%     - \sum \limits_{a} 
%     \tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} \bigg)  \label{eq:alpha_def}
% \end{align}
% \normalsize
% with the forward \kl divergence $D_{KL}[\tpi:\tpi_0]$ in \cref{eq:kl_def}
% % in \cref{eq:kl_def}
% % , \textcolor{red}{extended to take unnormalized densities as input, }
% recovered in the limit as $\alpha \rightarrow 1$.  
% As discussed in \myapp{tsallis}, the $\alpha$-divergence is closely related to the Tsallis entropy. \RB{Introduce $\log_{\alpha}$ first? (with the goal of reaching this insight)}
% % \citep{lee2019tsallis}, as we discuss in detail in \myapp{tsallis}.  
% % To see this, 

% For later convenience, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential,
% % \small
% % \begin{align}
% %     \log_{\alpha}(u) &= \begin{cases} \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \hfill \, \, \alpha \neq 1 \\
% %     \log(u) \hfill \, \, \alpha =1 \end{cases} \\
% %     \exp_{\alpha}(u) &= \begin{cases} [1 + (\alpha-1) \cdot u ]_+^{\frac{1}{\alpha-1}} \hfill \, \,  \alpha \neq 1 \\
% %     \exp(u) \hfill \, \, \alpha =1 \end{cases} \, .
% % \end{align}
% \begin{align}
%     \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , \\
%     \exp_{\alpha}(u) &= [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, .
%     % \hfill \, \,  \alpha \neq 1 \
% \end{align}
% % \begin{equation}
% % \resizebox{.87\columnwidth}{!}{\hspace*{-.36cm}
% %     $\log_{\alpha}(u) &= \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \\
% %     \quad 
% %     \exp_{\alpha}(u) = [1 + (\alpha-1) u ]_+^{\frac{1}{\alpha-1}}$
% % }
% % \end{equation}
% % \normalsize
% and we recover the natural logarithm and exponential in the limit as $\alpha \rightarrow 1$.

% With detailed derivations in \myapp{alpha_conj_norm}, the conjugate function for conditional divergence regularization takes the form
% \footnotesize
% \begin{align}
%      \hspace*{-.2cm} &\alphaconj(\dualvar) = \max \limits_{\mu(a,s)} \blangle \mu(a|s), \dualvar(a,s) \brangle -  \omegamu \label{eq:alpha_conj_norm_main} \\
%     &\phantom{=}= \frac{\alpha-1}{\alpha} \blangle \mu(s) \pi_{\dualvar}(a|s), \dualvar(a,s) \brangle + \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi_{\dualvar}] \nonumber
% %   \frac{1}{\alpha}  \normalizeralpha 
%     % \label{eq:alpha_conj_norm_main}
% \end{align}
% \normalsize
% As we discuss in \mysec{adversarial_perturb} or \myapp{alpha_conj_norm}, the final term $\frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi_{\dualvar}]$ 
% % plays the role of the normalization constant for 
% normalizes
% the policy in the optimizing argument $\pi_{\dualvar}(a|s) = \mu_{\dualvar}(a,s)/ \mu(s)$.   In particular, the policy has the form
% \footnotesize
% \begin{align}
%     \pi_{\dualvar}(a|s) = \pi_0(a|s) \exp_{\alpha} \big\{\beta \cdot \big( \dualvar(a,s) - \frac{1}{\beta}(1-\alpha)D_{\alpha}[\pi_0:\pi_{\dualvar}] \big)  \big\}
% \end{align}
% \normalsize
% \textcolor{blue}{wrap up / transition sentence}

% \RB{Introduce notation for normalizer / $D_{\alpha}$?}
% \RB{Inspect.  Reference App. and \textbf{optimal policy expression}}


==> Reward Robustness TMLR (3)/sections/new/1b_new_prelim.tex <==
\headerv
\headerv
\section{Preliminaries}\label{sec:prelim}
\headerv




In this section, we review
% provide background on 
\gls{LP} formulations of %fully observed, 
discounted \gls{MDP} and extensions to convex policy regularization.

\newcommand{\myset}{X}
\paragraph{Notation} \revhl{For a finite set $\mathcal{\myset}$, let $\mathbb{R}^{\mathcal{\myset}}$ denote the space of real-valued functions over $\mathcal{\myset}$, with $\mathbb{R}_+^{\mathcal{\myset}}$ indicating restriction to non-negative functions.  We let $\Delta^{|\mathcal{\myset}|}$ denote the probability simplex with dimension equal to the cardinality of $\mathcal{\myset}$.
% $|\mathcal{\myset}|$.   
For $ \mu, q \in \mathbb{R}^{\mathcal{\myset}}$, 
% we use 
$\langle \mu , q \rangle = \sum_{x \in \mathcal{\myset}} \mu(x) q(x)$ indicates the inner product in Euclidean space. }
% We abbreviate $\mathcal{X} \coloneqq \mathcal{A} \times \mathcal{S}$ for an action space $\mathcal{A}$ and state space $\mathcal{S}$.}
% For a finite set $\mathcal{A}$, we let $\mathcal{F}^{\mathcal{A}}$ denote the space of bounded, measurable functions over $\mathcal{A}$,  and use $\mathcal{F}_+^{\mathcal{A}}$ to indicate restriction to nonnegative functions.   We let $\Delta^{|\mathcal{A}|}$ indicate the probability simplex with dimension equal to the cardinality of the set $|\mathcal{A}|$.  
% We let $\Delta^{|\mathcal{A}|}$ indicate the probability simplex with dimension equal to the cardinality of the set $|\mathcal{A}|$.  
% We use subscripts $\pi_*$ or $V_*$ indicate values of variables at optimality, while superscripts $\Omega^*$ indicate the convex conjugate function.     

% We will use subscripts, $\mu_{\Delta_r}$ to indicate correspondence under conjugate duality when $\mu \in \mathcal{D}$ and $\Delta_r \in \mathcal{D}^*$ are elements of mutually dual spaces.   We will also use subscript notation $\pi_{\mu}$ to indicate the policy $\pi$ induced from a joint state-action occupancy $\mu$.

\headerv
\subsection{Convex Conjugate Function}\label{sec:conj_intro}
\headerv
We begin by reviewing the convex conjugate function, also known as the Legendre-Fenchel transform, which will play a crucial role throughout our paper.
% Before describing analogous primal and dual optimizations for regularized \gls{MDP}s, we review the convex conjugate function, or Legendre-Fenchel transform, which will play a crucial role throughout our paper.
%First,
For a convex function $\Omega(\primalvar)$ which, in our context, has domain $\primalvar \in \mudomainconj$,
%, where $\mathcal{D}$ may indicate the probability simplex $\Delta^{|A|}$ with possible additional constraints, such as $\mu_{\pi}(a,s) \in \mathcal{M}$
%over domain $\pi \in \Delta^{|\mathcal{A}|}$, possibly , 
%the Legendre-Fenchel transform or 
the conjugate function $\Omega^{*}$ is defined via the optimization
% \RB{what choice of primal variable? $\tpi$ is in function space in general, but will end up being a distribution}
% \RB{explain inner product notation here? what choice of primal variable $\primalvar$?} \TG{Yes both, but brief.}
\begin{align}
    \Omega^{*}( \dualvar ) = \sup \limits_{\primalvar \in 
    \mudomainconj
    % \mathcal{D}
    } \, \big \langle \primalvar, \dualvar \big \rangle - \Omega(\primalvar), \label{eq:conjstar}
\end{align} 
where $\dualvar \in \rprimedomainconj$.
% where $\dualvar \in \dualdomain$ is in the % continuous dual space of $\primalvar$ and $\langle \cdot, \cdot \rangle$ indicates the inner product.
% summation or integration over the dimensionality of the domain.  \RB{awkward?}
% $\mathcal{D}$ or $\dualdomain$. %continuous function in the topological dual space of $\pi$. %arbitrary function whose domain has the same dimension as $\mathcal{D}$.  
 %The conjugate function 
 The conjugate operation is an involution for proper, lower semi-continuous, convex $\Omega$ \citep{boyd2004convex},
 %(\citet{borwein2010convex} Sec. 4.3), 
 so that $(\Omega^{*})^{*} = \Omega$ and $\Omega^{*}$ is also convex.  
 We can thus represent $\Omega(\primalvar)$ via a conjugate optimization
 \begin{align}
     \Omega(\primalvar) = \sup_{\dualvar \in 
     \rprimedomainconj}
    %  \dualdomain} 
     \big \langle \primalvar, \dualvar \big \rangle - \Omega^{*}(\dualvar). \label{eq:conjomega}
 \end{align}
  %   Solving for the $\arg \sup$ in either \cref{eq:conjstar} or \cref{eq:conjomega} suggests optimality conditions for $\pi_*$ and $\dualvar$
  Differentiating with respect to the optimization variable in \cref{eq:conjstar} or (\ref{eq:conjomega}) suggests the optimality conditions 
%  \begin{align}
%      \primalvar(a,s) = \nabla \Omega^{*}( \dualvar )   \quad \qquad \dualvar(a,s) = \nabla \Omega(\primalvar) \, .     \label{eq:optimal_policy_as_grad}
%  \end{align}
% From the above, conjugacy also implies relationships of the form $\primalvar(a,s) = (\nabla \Omega)^{-1}(\dualvar(a,s))$, for example, when $\primalvar$ and $\dualvar$ are in dual correspondence.
% We provide examples of the convex conjugate for common divergence functions in \mytab{conj_table}.
  \begin{align}
     \primalvar_{\dualvar} = \nabla \Omega^{*}( \dualvar )   \quad \qquad \dualvar_{\primalvar} = \nabla \Omega(\primalvar) \, .     \label{eq:optimal_policy_as_grad}
 \end{align}
 Note that the above conditions also imply relationships of the form $\primalvar_{\dualvar} = (\nabla \Omega)^{-1}(\dualvar)$.   This dual correspondence between 
%  particular 
 values of $\primalvar$ and $\dualvar$ will form the basis of our adversarial interpretation in \mysec{adversarial_perturb}.
 
%  From the above, conjugacy also implies relationships of the form $\primalvar = (\nabla \Omega)^{-1}(\dualvar)$ when $\primalvar$ and $\dualvar$ are in dual correspondence.  
%  This correspondence will form the basis of our adversarial interpretation in \mysec{adversarial_perturb}.
%  We will make use of these conditions to associate 
%  , for example,

\headerv
\subsection{Divergence Functions}\label{sec:divergence_intro}
\headerv
% The family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases, 
% We will consider regularization using 
We are interested in the conjugate duality associated with 
policy regularization, which is often expressed using a
statistical divergence $\Omega(\mu)$ over a joint density $\mu(a,s) = \mu(s) \pi(a|s)$ (see \mysec{mdp_background}).  %commonly-used 
% where 
% The notation $\mu(a,s) = \mu(s) \pi(a|s)$ indicates a joint density
% which we will describe 
% whose meaning is described
% in \mysec{mdp_background}.
% which are used as regularization for \gls{RL} policies in \mysec{mdp_background}.   
In particular, we consider
the family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases.    
In the following, we consider extended divergences that accept unnormalized density functions as input \citep{zhu1995information} 
so that we may
% in order to 
 analyze function space dualities and evaluate Lagrangian relaxations without
%  , for example, 
projection
%the need to project 
 onto the probability simplex.
% so that Lagrangian relaxations in later sections will be well-defined even if normalization constraints are not satisfied.   

% \textcolor{red}{so that Lagrangian relaxations such as \cref{eq:dual_lagrangian} are well defined even when normalization constraints are not satisfied.}
% $\mu(a,s)$ is not normalized.}
% \textcolor{blue}{$\mu(a,s) \not \in \Delta^{|\mathcal{A}| \times |\mathcal{S}|}$.}

%  We primarily focus on policy regularization using a conditional divergence $\Omega^{(\alpha)}_{\pi_0}(\mu)$ to a reference policy $\pi_0(a|s)$.
% % but we also discuss regularization of the joint state-action occupancy to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$, in \textcolor{blue}{in \mysec{?}}.   
% Note that we consider the regularizer to be a function of $\mu(a,s)$, since it is applied 
% % in 
% across
% each 
% % $s \in \mathcal{S}$ 
% state
% % $s \sim \mu_\pi(s)$
% % \textcolor{red}{$s \sim \mu_\pi(s)$} 
% visited by the agent.
% \textcolor{blue}{In \mysec{?}}, we also discuss regularizing the joint state-action occupancy to be close to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$. 
% % \citep{nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.

% \RB{Need 2nd paragraph??  Smoother intro?}

% \RB{Remove all $\mu(s)$ below?}
% % \RB{REMOVE ALL THE $\mu(s)$ in Divergence derivations?}

\paragraph{KL Divergence}
% Taking the limit as $\alpha \rightarrow 1$, we obtain
% an (extended version of) 
The `forward' \textsc{kl} divergence to a reference policy $\pi_0(a|s)$ is commonly used for policy regularization in \gls{RL}.  
Extending the input domain to unnormalized measures, we write the divergence as
% \citep{zhu1995information},
% \citep{cichocki2010families}, 
%  (\citet{tishby2011information, ortega2013thermodynamics, fox2016taming})
\begin{align}
        &\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\Big[D_{KL}[\pi:\pi_0]\Big] = \sum \limits_{s \in \mathcal{S}} \mu(s) \sum \limits_{a \in \mathcal{A}}  \left(\pi(a|s)  \log \frac{\pi(a|s)}{\pi_0(a|s)} -  
        % \sum \limits_{a, s} 
      \pi(a|s) 
        + 
        % \sum \limits_{a,s} 
      \pi_0(a|s)\right). \label{eq:kl_def} 
\end{align}
\normalsize
Using a uniform reference  $\pi_0(a|s) = 1$ $\forall 
\, (a,s)$, we recover the Shannon entropy up to an additive constant.
%Up to an additive constant, we recover the Shannon entropy using a uniform reference, $\pi_0(a|s) = 1$ $\forall \, (a,s).$ 
% \in \mathcal{A} \times \mathcal{S}$.
% \, a \in \mathcal{A}, s \in \mathcal{S}$. 
% the final terms cancel if both $\pi$ and $\pi_0$ are normalized.


\paragraph{$\alpha$-Divergence} The $\alpha$-divergence $\mathbb{E}_{\mu(s)}\big[D_{\alpha}[\pi_0:\pi]\big]$ over possibly unnormalized measures
%$\omegamu &= \mathbb{E}_{\mu(s)}\big[D_{\alpha}[\pi_0:\pi]\big]$, 
is defined as 
% \footnotesize
\begin{align}
\hspace*{-.1cm} 
\Omega^{(\alpha)}_{\pi_0}(\mu)& =
% \mathbb{E}_{\mu(s)}\big[
% D_{\alpha}[\pi_0:\pi]
% \big]
% &= 
\frac{1}{\alpha(1-\alpha)} 
% \sum \limits_{s \in \mathcal{S}}
\sum \limits_{s \in \mathcal{S}}
\mu(s)
    \bigg( (1-\alpha) 
    % \sum \limits_{a \in \mathcal{A}} 
    \sum \limits_{a \in \mathcal{A}}
    \pi_0(a|s) 
    %+\alpha 
    % \\ &\phantom{\sum \limits_{s \in \mathcal{S}}\mu(s)} 
    + \alpha 
    % \sum \limits_{a \in \mathcal{A}} 
    \sum \limits_{a \in \mathcal{A}}
    \pi(a|s) 
    % \nonumber 
    % &- \sum \limits_{a \in \mathcal{A}} 
    % \\ &\phantom{\sum \limits_{s} \mu(s)} 
    - \sum \limits_{a \in \mathcal{A}} 
    \pi_0(a|s)^{1-\alpha} \pi(a|s)^{\alpha} \bigg)  
    % \label{eq:alpha_def}
    \label{eq:alpha_def} 
\end{align}
\normalsize
Taking the limiting behavior, we recover the `forward' \textsc{kl} divergence $D_{KL}[\pi:\pi_0]$ as $\alpha \rightarrow 1$ or the `reverse' \textsc{kl} divergence $D_{KL}[\pi_0:\pi]$ as $\alpha \rightarrow 0$.


To provide intuition for 
% for?  contextualize?  understand?}
the $\alpha$-divergence, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential, with
\begin{align}
    \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , 
    % \label{eq:qlog}  
    \qquad \qquad 
    \exp_{\alpha}(u) = [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, . \label{eq:qexp}
    % \hfill \, \,  \alpha \neq 1 \
\end{align}
\textcolor{black}{where $[\cdot]_+ = \max(\cdot,0)$ ensures fractional powers can be taken and suggests that $\exp_{\alpha}(u)=0$ for $u \leq 1/(1-\alpha)$.}
% Using $\log_{\alpha}$, 
Using the $\alpha$-logarithm, we can rewrite the $\alpha$-divergence 
% in similar fashion to
similarly to
the \kl divergence in 
\cref{eq:kl_def}
% \scriptsize
\resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
\begin{align}
  \Omega^{(\alpha)}_{\pi_0}(\mu) &= \frac{1}{\alpha} \sum \limits_{s \in \mathcal{S}} \mu(s) \bigg( \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)} - \pi(a|s) + \pi_0(a|s) \bigg) \nonumber.
\end{align}
}}
\normalsize
For a uniform reference $\pi_0$, the $\alpha$-divergence 
differs from the Tsallis entropy by only the $1/\alpha$ factor and an additive constant (see \myapp{tsallis}).

\input{sections/conj_table}

\headerv
\subsection{Unregularized MDPs}\label{sec:mdp_background}
% \subsection{MDPs as Linear or Convex Programs}\label{sec:mdp_background}
% \subsection{Linear $\&$ Convex Programming Formulations of MDPs}
\headerv
% \vspace*{\header}

% \paragraph{Unregularized Case}
A discounted \gls{MDP} is a tuple $\{ \mathcal{S}, \mathcal{A}, P, \nu_0, r, \gamma \}$ consisting of a state space $\mathcal{S}$, action space $\mathcal{A}$, transition dynamics $P(s\tick|s,a)$ for $s, s\tick \in \mathcal{S}$, $a \in \mathcal{A}$, initial state distribution $\nu_0(s) \in \Delta^{|\mathcal{S}|}$ in the probability simplex, and reward function $r(a,s):\mathcal{S} \times \mathcal{A} \mapsto \mathbb{R}$.   We also use a discount factor $\gamma\in (0,1)$ 
(\citet{puterman2014markov} Sec 6).
% , although discounting may also be handled by including a transition to an absorbing state in the \gls{MDP} (\citet{puterman2014markov} Sec. 5.3). 
% in the \gls{MDP}

% \paragraph{Unregularized Case}
We consider an agent that seeks to maximize the expected discounted reward by acting according to a decision policy 
% $\{ \pi(a|s) \in \Delta^{|\mathcal{A}|} \}_{s \in \mathcal{S}}$.
$\pi(a|s) \in \Delta^{|\mathcal{A}|}$  for each $ s \in \mathcal{S}$.  
The expected reward is calculated over trajectories ${\tau \sim \pi(\tau):= \nu_0(s_0) \prod \pi(a_t | s_t) P(s_{t+1} | s_t, a_t)}$, which begin from an initial $s_0 \sim \nu_0(s)$ and evolve according to the policy $\pi(a|s)$ and \gls{MDP} dynamics $P(s\tick|s,a)$  
% We consider an agent that acts according to a decision policy $\pi(a_t|s_t) \in \Delta^{|\mathcal{A}|}$, seeking to maximize the expected discounted reward over trajectories ${\tau \sim \pi(\tau):= \nu_0(s_0) \prod \pi(a_t | s_t) P(s_{t+1} | s_t, a_t)}$ which start from $s_0 \sim \nu_0(s)$ and evolve according to the policy and \gls{MDP} dynamics $P(s\tick|s,a)$.  
% Thus, the objective in \cref{eq:primal_lp} can be rewritten in similar fashion to \cref{eq:reward_perturbation_stmt}
% This leads to the objective function
% \small
\begin{align}
  \hspace*{-.2cm}
  \obj(r) := 
   \max \limits_{\pi(a|s)} \, (1-\gamma) \, \mathbb{E}_{\tau \sim \pi(\tau)} \bigg[ \sum \limits_{t=0}^{\infty} \gamma^t \, r(s_t, a_t)  \bigg] \, . \label{eq:policy_only} 
\end{align}
\normalsize
We assume that the policy is stationary and Markovian, and thus independent of both the timestep and trajectory history.  


% \paragraph{MDPs as Linear Programs}
\paragraph{Linear Programming Formulation}
% % \RB{We adopt notation, For the remainder of the paper, heavy use}
% % To highlight connections with the literature on convex duality, we consider 
% For the remainder of the paper, we will consider
% an equivalent \gls{LP} formulation in which optimization is performed over the discounted 
% % joint 
% state-action occupancy measure 
% $\mu(a,s) \coloneqq (1-\gamma) \mathbb{E}_{\tau\sim \pi(\tau)} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$,
% % with
% For the remainder of this work, 
% In what follows, 
We will focus on 
a linear programming (\gls{LP}) form for the objective in \cref{eq:policy_only}, which is common in the literature on convex duality.
% an equivalent \gls{LP} formulation which is common in the literature on convex duality.   
With optimization over the discounted 
state-action occupancy measure, 
% ${\mu(a,s) \coloneqq (1-\gamma)} \mathbb{E} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$, we have
${\mu(a,s) \coloneqq (1-\gamma)} \mathbb{E}_{\tau\sim \pi(\tau)} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$, 
we rewrite 
% \cref{eq:policy_only} as
the objective as
% the objective can be rewritten
% becomes
% With optimization over the discounted 
% state-action occupancy measure 
% ${\mu(a,s) \coloneqq (1-\gamma)} \mathbb{E}_{\tau\sim \pi(\tau)} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$, 
% \small
% \begin{align}
%   \hspace*{-.2cm} &  
%   \obj(r) :=
%   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \, \, \text{subj. to} \, \quad    \left( \forall s \in \mathcal{S} \right) \label{eq:primal_lp}\\[1.25ex]
%   &\sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \nonumber  \, ,
%   %\, \forall s \in \mathcal{S}\nonumber
% \end{align}
\ifx\omitindices\undefined
\small
\begin{align}
   \hspace*{-.23cm}  
   \obj(r) \coloneqq
   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \qquad \text{subject to } \quad \mu(a,s) &\geq 0 \qquad \forall (a,s) \in \mathcal{A} \times \mathcal{S},   \quad  \label{eq:primal_lp} \\
    \sum_{a} \mu(a,s)& = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \qquad \forall s \in \mathcal{S}, \nonumber 
   %\left( \forall s \in \mathcal{S} \right) 
   %\, \forall s \in \mathcal{S}\nonumber
\end{align}
\else
\begin{align}
   \hspace*{-.23cm}  
   \obj(r) \coloneqq
   \max \limits_{\mu} \big \langle {\mu, r} \big \rangle \qquad \text{subject to } \quad \mu(a,s) &\geq 0 \qquad \forall (a,s) \in \mathcal{A} \times \mathcal{S},   \quad  \label{eq:primal_lp} \\
    \sum_{a} \mu(a,s)& = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \qquad \forall s \in \mathcal{S} \nonumber.
   %\left( \forall s \in \mathcal{S} \right) 
   %\, \forall s \in \mathcal{S}\nonumber
\end{align}
\fi
% \small
% \begin{align}
%   \hspace*{-.23cm}  
%   \obj(r) \coloneqq
%   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \qquad \text{subject to } \quad \forall (a,s) \in \mathcal{A} \times \mathcal{S}:&   \quad  \mu(a,s) \geq 0  \label{eq:primal_lp} \\
%     \quad \forall s \in \mathcal{S}:& \quad \sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick)  \nonumber 
%   %\left( \forall s \in \mathcal{S} \right) 
%   %\, \forall s \in \mathcal{S}\nonumber
% \end{align}
% \footnotesize
% \begin{align}
%   \hspace*{-.2cm} &  
%   \obj(r) :=
%   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \, \, \label{eq:primal_lp} \\
%   &\phantom{ \obj(r) :=} \text{subj. to} \, \,\mu(a,s) \geq 0 \quad \forall (a, s) \in \mathcal{A} \times \mathcal{S}   \nonumber  \\[1.25ex] %
%   &\sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \, \,  \forall s \in \mathcal{S}  \nonumber  \, , %\left( \forall s \in \mathcal{S} \right)
%   %\, \forall s \in \mathcal{S}\nonumber
% \end{align}
\normalsize
% \RB{$\mu(a,s) \geq 0 $ leads to $V \geq r + \gamma\transitionv$ \textit{inequality} constraint}
% \textcolor{red}{where inner product notation indicates summation or integration over the domain of $\mu$. }
% and nonnegativity constraints apply for each $(a, s) \in \mathcal{A} \times \mathcal{S}$. %\RB{improve} %$\sum \mu \cdot \dualvar$
%The optimization is over state-action visitation distributions $\mu(a,s) \in \Delta^{|\mathcal{S}| \times |\mathcal{A}|} $, and a corresponding policy is obtained via $\pi(a|s) = \mu(a,s) / \sum_a \mu(a,s)$.   
We refer to the constraints in the second line of \cref{eq:primal_lp} as the \textit{Bellman flow constraints}, which force $\mu(a,s)$ to respect the \gls{MDP} dynamics.
%and denote the set of feasible $\mu$ as $\mathcal{M}$. For normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$, we show in \myapp{normalized_mu} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized.
We denote the set of feasible $\mu$ as $\mathcal{M} \subset \mudomainfn$.    For normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$,   we show in \myapp{optimal_policy} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s)$
% \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ 
is normalized. 
% we show in \myapp{normalized_mu} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized. 
% We denote the set of feasible $\mu$ as $\mathcal{M}$
% % For normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$, we show in \myapp{normalized_mu} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized. 
% and in \myapp{normalized_mu}, show that $\mu(a,s) \in \mathcal{M}$ implies that $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized for normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$.
% % assuming $\nu_0(s)$ and $P(s|a\tick, s\tick)$ are normalized.

% \RB{Flow constraints force $\mu$ to respect dynamics}
% \RB{Mention that $\nu_0(s), P(s\tick|s,a)$ normalized implies $\mu(a,s) \in \mathcal{M}$ normalized} 


It can be shown that any feasible $\mu(a,s) \in \mathcal{M}$  induces a stationary $\pi(a|s) = \mu(a,s) / 
\mu(s)$, 
% \sum_{a\tick} \mu(a\tick,s)
where  $\mu(s) \coloneqq \sum_{a\tick} \mu(a\tick,s)$ and $\pi(a|s) \in \Delta^{|\mathcal{A}|}$ is normalized by definition.
% \footnote{To see this, since $\sum_a \frac{\mu(a,s)}{\sum_{a'} \mu(s)}= \frac{\sum_a \mu(a,s)}{\mu(s)} = 1$.} 
% \footnote{The policy is always normalized 
% % even if $\mu(a,s)$ is not, 
% since $\sum_a \frac{\mu(a,s)}{\sum_{a'} \mu(s)}= \frac{\sum_a \mu(a,s)}{\mu(s)} = 1$.}$
Conversely, any stationary policy $\pi(a|s)$ induces a unique state-action visitation distribution $\mu(a,s)$ (\citet{syed2008apprenticeship},
\citet{feinberg2012handbook} Sec. 6.3).
%\citet{puterman2014markov} Sec. ??).
 Along with the definition of $\mu(a,s)$ above, 
%  this demonstrates 
this result demonstrates
 the equivalence of the optimizations in \cref{eq:policy_only} and \cref{eq:primal_lp}.  We will proceed with the \gls{LP} notation from \cref{eq:primal_lp} and assume $\mu(s)$ is induced by
%the corresponding 
$\pi(a|s)$ whenever the two appear together in an expression.
% It can be shown that any stationary policy $\pi(a|s)$ induces a unique state-action 
% visitation distribution $\mu(a,s)$, while, conversely, a feasible $\mu(a,s) \in \mathcal{M}$  is induced by some stationary $\pi(a|s) = \mu(a,s) / \mu(s)$ (\citep{syed2008apprenticeship}, \citet{feinberg2012handbook} Sec. 6.3).   

% where the marginal state-visitation distribution $\mu(s) \propto (1-\gamma) \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(s_t = s)$ a
% The flow constraints in \cref{eq:primal_lp} are insightful, as they lead to a dual optimization reflecting the familiar Bellman equations \citep{bellman1957markovian}. 
Importantly, the flow constraints in \cref{eq:primal_lp} lead to a dual optimization which reflects the familiar Bellman equations \citep{bellman1957markovian}. 
To see this, we introduce Lagrange multipliers 
\ifx\omitindices\undefined
$V(s)$ for each flow constraint and $\lambdaplus \geq 0$ for the nonnegativity constraints.
\else
$V \in \mathbb{R}^{\mathcal{S}}$ for each flow constraint and $\lambdaplus \in \mathbb{R}_+^{\mathcal{A} \times \mathcal{S}}$ for the nonnegativity constraints.
\fi
  Summing over $s \in \mathcal{S}$, and eliminating $\mu(a,s)$ by setting $d/d\mu(a,s) = 0$ yields the \textit{dual} \gls{LP}
% Introducing Lagrange multipliers $V(s)$ for each flow constraint, summing over $s \in \mathcal{S}$, and eliminating $\mu(a,s)$ by setting $d/d\mu(a,s) = 0$ yields the \textit{dual} \gls{LP}
% \begin{align}
%   &\obj^{*}(r):=\min \limits_{V(s)} \,  (1-\gamma) \big \langle \nu_0(s), V(s) \big \rangle \, \text{  subj to: }\, \label{eq:dual_lp} \\ %\quad \forall (a,s) \in \mathcal{S} \times \mathcal{A}
%   & \, V(s) = r(a,s) + \gamma \transitionv + \lambdaplus 
% %   \,\, \forall (a,s) \in \mathcal{A} \times \mathcal{S}  
%  \nonumber \, ,
% \end{align}
% \small
\ifx\omitindices\undefined
\begin{align}
 \hspace*{-.2cm} \obj^{*}(r)&\coloneqq
  \min \limits_{V(s), \lambdaplus} \,
%   \min \limits_{V(s)} \,  
  (1-\gamma) \big \langle \nu_0(s), V(s) \big \rangle  
%   \\
%   \text{  subj to: }\label{eq:dual_lp} \\ %\quad \forall (a,s) \in \mathcal{S} \times \mathcal{A}
 \quad \text{  subject to } \,\,\, V(s) = r(a,s) + \gamma \transitionv + \lambdaplus 
%  \quad \forall (a,s) \in \mathcal{A} \times \mathcal{S}  
 \label{eq:dual_lp} , 
%  \nonumber \, ,
\end{align}
\else
\begin{align}
 \hspace*{-.2cm} \obj^{*}(r)&\coloneqq
  \min \limits_{V, \lambda} \,
%   \min \limits_{V(s)} \,  
  (1-\gamma) \big \langle \nu_0, V \big \rangle  
%   \\
%   \text{  subj to: }\label{eq:dual_lp} \\ %\quad \forall (a,s) \in \mathcal{S} \times \mathcal{A}
 \quad \text{  subject to } \,\,\, V(s) = r(a,s) + \gamma \transitionv + \lambdaplus 
\quad \forall (a,s) \in \mathcal{A} \times \mathcal{S}  
 \label{eq:dual_lp} , 
%  \nonumber \, ,
\end{align}
\fi
\normalsize
% where the constraint applies for all $(a,s) \in \mathcal{A} \times \mathcal{S}$ and $\lambdaplus \geq 0$.  By complementary slackness \citep{boyd2004convex}, we know that $\lambdaplus =0$ for $\mu(a,s) > 0$.
% Finally,  we use $\transitionv$ as shorthand for $\mathbb{E}_{P(s\tick|a,s)}[ V(s\tick)]$ and have reindexed the transition tuple from $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared to \cref{eq:primal_lp}. 
where we have used $\transitionv$ as shorthand for $\mathbb{E}_{P(s\tick|a,s)}[ V(s\tick)]$ and reindexed the transition tuple from $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared to \cref{eq:primal_lp}.   Note that the constraint applies for all $(a,s) \in \mathcal{A} \times \mathcal{S}$ and that $\lambdaplus \geq 0$.  By complementary slackness, 
% \citep{boyd2004convex}, 
we know that $\lambdaplus =0$ for $(a,s)$ such that $\mu(a,s) > 0$.

% In similar fashion to the conjugate optimizations in \cref{eq:conjstar}-\ref{eq:conjomega}, these dual objectives have the same solution under strong duality, despite optimizing over different variables.

% where the constraint applies for all $(a,s) \in \mathcal{A} \times \mathcal{S}$ and $\lambdaplus \geq 0$.  By complementary slackness, 
% % \citep{boyd2004convex}, 
% we know that $\lambdaplus =0$ for $(a,s)$ such that $\mu(a,s) > 0$.
% Finally, we have used $\transitionv$ as shorthand for $\mathbb{E}_{P(s\tick|a,s)}[ V(s\tick)]$ and reindexed the transition tuple from $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared to \cref{eq:primal_lp}. 

% By complementary slackness \citep{boyd2004convex}, we know that $\lambdaplus =0$ for $(a,s)$ such that $\mu(a,s) > 0$.
% It is easy to show that the optimal policy is deterministic if $a_{\text{max}} \coloneqq \arg \max_a r(a,s) + \gamma \transitionv$ is unique, with $\pi_*(a_{\text{max}}|s) = 1$ and $V(s) = r(a_{\text{max}},s) + \gamma 
% \mathbb{E}_{a_{\text{max}},s}^{s\tick}\left[V(s\tick)\right]$.
% % \transitionv$
% $\lambda(a_{\text{max}}, s) = V(s) - r(a,s) - \gamma \transitionv > 0$.

% \paragraph{Regularized Case}
\headerv
\subsection{Regularized MDPs}\label{sec:mdp_regularized}
\headerv
We now consider regularizing the objective in \cref{eq:primal_lp} using a convex penalty function $\Omega(\mu)$ with coefficient $1/\beta$.   
We primarily focus on regularization using a conditional divergence $\Omega_{\pi_0}(\mu) \coloneqq \mathbb{E}_{\mu(s)\pi(a|s)}[\ptReg(\pi)]$ between the policy and a normalized reference distribution $\pi_0(a|s)$, as in \mysec{divergence_intro} and \citep{ortega2013thermodynamics,fox2016taming,haarnoja17a,haarnoja2018soft}.   
We also use the notation $\Omega_{\mu_0}(\mu) = \mathbb{E}_{\mu(a,s)}[\ptReg(\mu)]$ to indicate regularization of the full state-action occupancy measure to a normalized reference $\mu_0(a,s)$,  which appears, for example, in \gls{REPS} \citep{peters2010relative, belousov2019entropic}.   
% We assume the reference is normalized, either $\sum_a \pi_0(a|s) =1$ or $\sum_{a,s} \mu_0(a,s)=1$.
% We will also consider regularization of the full state-action occupancy measure to a reference $\mu_0(a,s)$, using the notation $\Omega_{\mu_0}(\mu) = \mathbb{E}_{\mu(a,s)}[\ptReg(\mu)]$ \citep{peters2010relative, belousov2019entropic, basserrano2021logistic}.
% The regularizer may be either a conditional divergence $\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)\pi(a|s)}[\ptReg(\pi)]$ between the policy and a reference distribution $\pi_0(a|s)$, or a divergence $\Omega_{\mu_0}(\mu) = \mathbb{E}_{\mu(a,s)}[\ptReg(\mu)]$ over the joint state-action occupancy measure with reference $\mu_0(a,s)$. \RB{?? Later.  reference \mysec{divergence_intro}}
% % We will consider $\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)\pi(a|s)}[\ptReg(\pi)]$ to be a conditional divergence between the policy and a reference distribution $\pi_0(a|s)$ that can be written with an outer expectation over $\mu(a,s)$.~\footnote{We focus on policy regularization \citep{neu2017unified} in this work, but similar reasoning may be applied for regularizing the joint state-action occupancy $\mu(a,s)$ \citep{nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.} 
% Letting $\Omega_{\pi_0}(\pi)$ be a statistical divergence between the policy and a reference distribution $\pi_0(a|s)$, 
% We define the regularized objective as 
The regularized objective $\obj_{\Omega, \beta}(r)$ is then defined as
% $\obj_{\Omega, \beta}(r)$
\ifx\omitindices\undefined
\begin{equation}
% \resizebox{.87\columnwidth}{!}{ \hspace*{-.2cm}   $
\obj_{\Omega, \beta}(r) :=  \max \limits_{\mu(a,s) \in \mathcal{M} } %\max \limits_{\pi(a|s) \in \Delta^{|A|}} 
   \blangle \mu(a,s), r(a,s) \brangle - \dfrac{1}{\beta}   \Omega_{\pi_0}(\mu) 
%   $ 
%   }
  \label{eq:primal_reg}
\end{equation}
\else
\begin{equation}
% \resizebox{.87\columnwidth}{!}{ \hspace*{-.2cm}   $
\obj_{\Omega, \beta}(r) :=  \max \limits_{\mu \in \mathcal{M} } %\max \limits_{\pi(a|s) \in \Delta^{|A|}} 
   \blangle \mu, r \brangle - \dfrac{1}{\beta}   \Omega_{\pi_0}(\mu) 
%   $ 
%   }
  \label{eq:primal_reg}
\end{equation}
\fi
where $\Omega_{\pi_0}(\mu)$ contains an expectation under $\mu(a,s)$ as in \cref{eq:kl_def}-(\ref{eq:alpha_def}).
We can also derive a dual version of the regularized \gls{LP}, 
by first writing the Lagrangian relaxation of \cref{eq:primal_reg}
% starting from a Lagrangian relaxation of \cref{eq:primal_reg}
%\max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}}
% \begin{align}
%     %\mathcal{L}(\mu, V, \Omega) := 
%     & \min \limits_{V(s)} \max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}} \, 
%      (1-\gamma) \big\langle \nu_0, V(s) \big  \rangle \\
%      + &\blangle \mu(s)\pi(a|s), r(a,s) +  \gamma \transitionv -V(s) \big \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \nonumber \\
%     &   \label{eq:lagrangian}\, ,
% \end{align}
% \resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
% \scriptsize
\ifx\omitindices\undefined
\begin{align}
%   \mathcal{L}:= 
  \max \limits_{\mu(a,s)} \min \limits_{V(s), \lambdaplus}  \, 
     (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle 
     + &\langle \mu(a,s), r(a,s) + \gamma \transitionv -V(s) + \lambdaplus \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\mu)  \label{eq:dual_lagrangian} 
\end{align}
\else
\begin{align}
%   \mathcal{L}:= 
  \max \limits_{\mu} \min \limits_{V, \lambda}  \, 
     (1-\gamma) \big\langle \nu_0, V \big  \rangle 
     + &\, \langle \mu, r + \gamma \transitionvinds -V + \lambda \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\mu) . \label{eq:dual_lagrangian} 
\end{align}
\fi
\normalsize
% }}
% \resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
% \begin{align}
%   & 
% %   \mathcal{L}:= 
%   \max \limits_{\mu(a,s)} \min \limits_{V(s)}  \, 
%      (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle  \label{eq:dual_lagrangian} \\
%      + &\blangle \mu(a,s), r(a,s) +  \gamma \transitionv -V(s)\brangle - \frac{1}{\beta} \Omega_{\pi_0}(\mu)  \nonumber
% \end{align}
% }}
Swapping the order of optimization 
% using
under 
strong duality, we can recognize the 
maximization over ${\mu(a,s)}$ as a conjugate function $\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}$, as in \cref{eq:conjstar}, leading to a regularized dual optimization
% \resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
\ifx\omitindices\undefined
 \begin{align}
 \hspace*{-.2cm} &  \obj_{\Omega, \beta}^{*}(r) = 
%  \min \limits_{V(s)} 
 \min \limits_{V(s), \lambdaplus}
 %\max \limits_{ \mu(s) \rightarrow \mathcal{M}}
 \,  (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle  + \frac{1}{\beta}\Omega^{*}_{\pi_0, \beta} \bigg(r(a,s) +  \gamma \transitionv -V(s) + \lambdaplus \bigg)\label{eq:dual_reg} 
%  &+ \mathbb{E}_{\mu(s)} \bigg[\, \frac{1}{\beta}\Omega^{*}_{\pi_0, \beta} \bigg(r(a,s) +  \gamma \transitionv -V(s) \bigg)  \bigg] \nonumber
\end{align}
\else
 \begin{align}
 \hspace*{-.2cm} &  \obj_{\Omega, \beta}^{*}(r) = 
%  \min \limits_{V(s)} 
 \min \limits_{V, \lambda}
 %\max \limits_{ \mu(s) \rightarrow \mathcal{M}}
 \,  (1-\gamma) \big\langle \nu_0, V \big  \rangle  + \frac{1}{\beta}\Omega^{*}_{\pi_0, \beta} \Big(r  +  \gamma \transitionvinds -V + \lambda \Big)\label{eq:dual_reg} 
%  &+ \mathbb{E}_{\mu(s)} \bigg[\, \frac{1}{\beta}\Omega^{*}_{\pi_0, \beta} \bigg(r(a,s) +  \gamma \transitionv -V(s) \bigg)  \bigg] \nonumber
\end{align}
\fi
% }}
% \RB{Omit this, instead consider soft value aggregation? }
which involves optimization over dual variables $V(s)$ only and is unconstrained, in contrast to \cref{eq:dual_lp}. %, and involves sampling under the induced marginal distribution $\mu(s)$. 
% Similar dual objectives
Dual objectives of this form 
% have been considered 
appear 
in \citep{nachum2020reinforcement, belousov2019entropic, basserrano2021logistic, neu2017unified}.
\textcolor{black}{We emphasize the need to include the Lagrange multiplier $\lambdaplus$, with $\lambdaplus > 0$ when the optimal policy has $\piopt(a|s) = 0$, since an important motivation for $\alpha$-divergence regularization is to encourage sparsity in the policy (see \cref{eq:qexp}, \citet{lee2018sparse, lee2019tsallis, chow2018path}).}


\paragraph{Soft Value Aggregation}
In iterative algorithms such as (regularized) modified policy iteration \citep{puterman1978modified, scherrer15a}, it is useful to consider the \textit{regularized Bellman optimality operator} \citep{geist2019theory}.   For given estimates of the state-action value $Q(a,s) \coloneqq r(a,s) + \gamma \transitionv$, the operator $\mathcal{T}^{*}_{\Omega_{\pi_0, \beta}}$ updates $V(s)$ as
% \scriptsize
\ifx\omitindices\undefined
\begin{align} 
\hspace*{-.2cm} V(s)  \leftarrow \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(Q) = \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \blangle \pi(a|s), Q(a,s) \brangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \label{eq:soft_value}
\end{align}
\else
\begin{align} 
\hspace*{-.2cm} V(s)  \leftarrow \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(Q) = \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \blangle \pi, Q \brangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \label{eq:soft_value} .
\end{align}
\fi
\normalsize
Note that this conjugate optimization is performed in each state $s \in \mathcal{S}$ and explicitly constrains each $\pi(a|s)$ to be normalized.
Although we proceed with the notation of \cref{eq:primal_reg} and \cref{eq:dual_reg}, our later developments 
% for conditional policy regularization 
are compatible with the
% the regularized Bellman operator or 
`soft-value aggregation' perspective above.  See \myapp{soft_value} for detailed discussion.
% We provide detailed discussion in \myapp{soft_value}.
% We provide a detailed discussion of this `soft-value aggregation' operator in \myapp{soft_value}.   While we proceed with the notation of \cref{eq:dual_reg}
% While our developments in later sections focus on
% Our developments in later sections are compatible with this approach,

%%%%%%%%%%%%%%%%%%%%%%%%%% Prev Divergence Functions Paragraph %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Divergence Functions}\label{sec:divergence_intro}
% \RB{MOVE and modify this intro to fit?}

% % The family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases, 
% We consider regularization using the family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases.    
% We extend these divergences to accept unnormalized density functions as input \citep{zhu1995information}, \textcolor{red}{so that Lagrangian relaxations such as \cref{eq:dual_lagrangian} are well defined even when 
% normalization constraints are not satisfied.}
% % $\mu(a,s)$ is not normalized.}
% % \textcolor{blue}{$\mu(a,s) \not \in \Delta^{|\mathcal{A}| \times |\mathcal{S}|}$.}

%  We primarily focus on policy regularization using a conditional divergence $\Omega^{(\alpha)}_{\pi_0}(\mu)$ to a reference policy $\pi_0(a|s)$.
% % but we also discuss regularization of the joint state-action occupancy to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$, in \textcolor{blue}{in \mysec{?}}.   
% Note that we consider the regularizer to be a function of $\mu(a,s)$, since it is applied 
% % in 
% across
% each 
% % $s \in \mathcal{S}$ 
% state
% % $s \sim \mu_\pi(s)$
% % \textcolor{red}{$s \sim \mu_\pi(s)$} 
% visited by the agent.
% \textcolor{blue}{In \mysec{?}}, we also discuss regularizing the joint state-action occupancy to be close to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$. 
% % \citep{nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.

% \RB{Need 2nd paragraph??  Smoother intro?}

% \RB{Remove all $\mu(s)$ below?}
% % \RB{REMOVE ALL THE $\mu(s)$ in Divergence derivations?}

% \paragraph{KL Divergence}
% % Taking the limit as $\alpha \rightarrow 1$, we obtain
% % an (extended version of) 
% The forward \textsc{kl} divergence is commonly used for policy regularization in \gls{RL}.  Extending to unnormalized measures 
% \citep{zhu1995information},
% % \citep{cichocki2010families}, 
% %  (\citet{tishby2011information, ortega2013thermodynamics, fox2016taming})
% \footnotesize
% \begin{align}
%         &\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\bigg[D_{KL}[\tpi:\tpi_0]\bigg] \label{eq:kl_def} \\
%         &\phantom{\Omega} = \sum \limits_{s \in \mathcal{S}} \mu(s) \sum \limits_{a \in \mathcal{A}}  \left(\tpi(a|s)  \log \frac{\tpi(a|s)}{\tpi_0(a|s)} -  
%         % \sum \limits_{a, s} 
%       \tpi(a|s) 
%         + 
%         % \sum \limits_{a,s} 
%       \tpi_0(a|s)\right). \nonumber
% \end{align}
% % \begin{align}
% %     % \hspace*{-.15cm} D_{KL}[\tpi:\tpi_0] = \sum \limits_{a \in \mathcal{A}} \tpi(a|s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} - \tpi(a|s) + \tpi_0(a|s) \, . \nonumber
% %         % \hspace*{-.2cm}  
% %         \Omega&_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\bigg[D_{KL}[\tpi:\tpi_0]\bigg] \label{eq:kl_def} \\
% %         &= \sum \limits_{a, s} \mu(a,s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} -  
% %         % \sum \limits_{a, s} 
% %         \mu(s) \tpi(a|s) 
% %         + 
% %         % \sum \limits_{a,s} 
% %         \mu(s) \tpi_0(a|s)
% %       . \nonumber
% %         % \sum \limits_{a, s} \mu(a,s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
% %         % \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
% %         % \textcolor{red}{ -\sum \limits_{a \in \mathcal{A}} \tpi(a|s) +\sum \limits_{a \in \mathcal{A}} \tpi_0(a|s) } 
% %     %\sum \limits_{a \in \mathcal{A}} %\lim_{\alpha \rightarrow 1}
% % \end{align}
% \normalsize
% Up to an additive constant, we recover the Shannon entropy using a uniform reference, $\pi_0(a|s) = 1$ $\forall 
% \, (a,s).$ 
% % \in \mathcal{A} \times \mathcal{S}$.
% % \, a \in \mathcal{A}, s \in \mathcal{S}$. 
% % the final terms cancel if both $\tpi$ and $\tpi_0$ are normalized.


% \paragraph{$\alpha$-Divergence} The $\alpha$-divergence $\mathbb{E}_{\mu(s)}\big[D_{\alpha}[\tpi_0:\tpi]\big]$ over possibly unnormalized measures
% %$\omegamu &= \mathbb{E}_{\mu(s)}\big[D_{\alpha}[\tpi_0:\tpi]\big]$, 
% is defined as 
% \footnotesize
% \begin{align}
% \hspace*{-.1cm} 
% \Omega^{(\alpha)}_{\pi_0}(\mu)&=
% % \mathbb{E}_{\mu(s)}\big[
% % D_{\alpha}[\tpi_0:\tpi]
% % \big]
% % &= 
% \frac{1}{\alpha(1-\alpha)} 
% % \sum \limits_{s \in \mathcal{S}}
% \sum \limits_{s \in \mathcal{S}}
% \mu(s)
%     \bigg( (1-\alpha) 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a \in \mathcal{A}}
%     \tpi_0(a|s) 
%     %+\alpha 
%     \\ &\phantom{\sum \limits_{s \in \mathcal{S}}
% \mu(s)} + \alpha 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a \in \mathcal{A}}
%     \tpi(a|s) \nonumber 
%     % &- \sum \limits_{a \in \mathcal{A}} 
%     % \\ &\phantom{\sum \limits_{s} \mu(s)} 
%     - \sum \limits_{a \in \mathcal{A}} 
%     \tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} \bigg)  \label{eq:alpha_def}
% \end{align}
% \normalsize
% To provide intuition for 
% % for?  contextualize?  understand?}
% the $\alpha$-divergence, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential, with
% \begin{align}
%     \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , \\
%     \exp_{\alpha}(u) &= [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, .
%     % \hfill \, \,  \alpha \neq 1 \
% \end{align}
% % Using $\log_{\alpha}$, 
% Using the $\alpha$-logarithm, we can rewrite the $\alpha$-divergence 
% % in a form similar to 
% similarly to
% the \kl divergence in 
% \cref{eq:kl_def}.
% \scriptsize
% \begin{align}
%   \Omega^{(\alpha)}_{\pi_0}(\mu) &= \frac{1}{\alpha} \sum \limits_{s \in \mathcal{S}} \mu(s) \bigg( \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)} - \pi(a|s) + \pi_0(a|s) \bigg) \nonumber
% \end{align}
% \normalsize
% For a uniform reference, the $\alpha$-divergence 
% differs from the Tsallis entropy by only the $1/\alpha$ factor and an additive constant (see \myapp{tsallis}).


% \RB{Bridge}





%%%%%%%%%%%%%%%%%%%%%%%%%% END OF Prev Divergence Functions Paragraph %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





% As discussed in \myapp{tsallis}, the $\alpha$-divergence is closely related to the Tsallis entropy. \RB{Introduce $\log_{\alpha}$ first? (with the goal of reaching this insight)}
% \citep{lee2019tsallis}, as we discuss in detail in \myapp{tsallis}.  
% To see this, 

% For later convenience, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential,
% % \small
% % \begin{align}
% %     \log_{\alpha}(u) &= \begin{cases} \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \hfill \, \, \alpha \neq 1 \\
% %     \log(u) \hfill \, \, \alpha =1 \end{cases} \\
% %     \exp_{\alpha}(u) &= \begin{cases} [1 + (\alpha-1) \cdot u ]_+^{\frac{1}{\alpha-1}} \hfill \, \,  \alpha \neq 1 \\
% %     \exp(u) \hfill \, \, \alpha =1 \end{cases} \, .
% % \end{align}
% \begin{align}
%     \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , \\
%     \exp_{\alpha}(u) &= [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, .
%     % \hfill \, \,  \alpha \neq 1 \
% \end{align}
% \begin{equation}
% \resizebox{.87\columnwidth}{!}{\hspace*{-.36cm}
%     $\log_{\alpha}(u) &= \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \\
%     \quad 
%     \exp_{\alpha}(u) = [1 + (\alpha-1) u ]_+^{\frac{1}{\alpha-1}}$
% }
% \end{equation}
% \normalsize
% and we recover the natural logarithm and exponential in the limit as $\alpha \rightarrow 1$.


% \textcolor{blue}{
% We consider regularization of the policy $\pi(a|s)$ to a reference $\pi_0(a|s)$, with analogous derivations for  regularization of $\mu(a,s)$ to a reference $\mu_0(a,s)$ in \myapp{mu_results}.}
% \RB{Decide how to handle $\mu$ vs. $\pi$ regularization.  Difference is insightful for $\alpha$-divergence}

% \paragraph{KL Divergence}
% % Taking the limit as $\alpha \rightarrow 1$, we obtain
% % an (extended version of) 
% The forward \textsc{kl} divergence commonly used as regularization in \gls{RL} is defined as
% %  (\citet{tishby2011information, ortega2013thermodynamics, fox2016taming})
% \footnotesize
% \begin{align}
%     % \hspace*{-.15cm} D_{KL}[\tpi:\tpi_0] = \sum \limits_{a \in \mathcal{A}} \tpi(a|s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} - \tpi(a|s) + \tpi_0(a|s) \, . \nonumber
%         % \hspace*{-.2cm}  
%         \Omega&_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\bigg[D_{KL}[\tpi:\tpi_0]\bigg] \label{eq:kl_def} \\
%         &= \sum \limits_{a, s} \mu(a,s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} -  
%         % \sum \limits_{a, s} 
%         \mu(s) \tpi(a|s) 
%         + 
%         % \sum \limits_{a,s} 
%         \mu(s) \tpi_0(a|s)
%       . \nonumber
%         % \sum \limits_{a, s} \mu(a,s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
%         % \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
%         % \textcolor{red}{ -\sum \limits_{a \in \mathcal{A}} \tpi(a|s) +\sum \limits_{a \in \mathcal{A}} \tpi_0(a|s) } 
%     %\sum \limits_{a \in \mathcal{A}} %\lim_{\alpha \rightarrow 1}
% \end{align}
% \normalsize
% \RB{$\tpi$ or $\pi$?}
% To derive a closed form for the convex conjugate function, we consider the conditional \kl divergence as a function of $\mu(a,s)$ in the following conjugate optimization
% \footnotesize
% \begin{align}
%   \hspace*{-.25cm}  &\klconjpii(\dualvar) = \max \limits_{\mu(a,s)} \blangle 
%     \mu(a,s), \dualvar(a,s)
%     % \mu(a,s), \dualvar(a,s)
%     \brangle - \klomegamu \label{eq:kl_conj} \\
%   &= \frac{1}{\beta} \sum \limits_s \mu(s) 
%   \left(
%   \sum \limits_{a} \pi_0(a|s) \expof{\beta \cdot \dualvar(a,s)} - \sum \limits_{a} \pi_0(a|s) 
%   \right)
%   \nonumber
% %   &= \frac{1}{\beta} \log \sum \limits_{a,s} \mu(s) \pi_0(a|s) \expof{\beta \cdot \dualvar(a,s)}
%     % - \blangle \lambda , \mu(a,s) - 1\brangle
% \end{align}
% \normalsize
% where the \textcolor{red}{optimizing argument is 
% the occupancy measure
% induced by } $\pir(a|s) = \pi_0(a|s)\exp\{\beta \cdot \dualvar(a,s)\} $.
% See \myapp{kl_conj_all} for detailed derivations.  Note that the log-sum-exp form of the conjugate function arises from enforcing a normalization constraint on the optimization variable \citep{ruderman2012tighter}.   
% % $\mu(a,s) \in \Delta^{\mathcal{A} \times \mathcal{S}}$.

% % Finally, note that the optimizing argument for the conjugate in \cref{eq:kl_conj} is given by 
% % \begin{align}
% %     \piopt(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( \dualvar(a,s) \big) } 
% % \end{align}
% % where $\muopt(a,s) = \muopt(s) \piopt(a|s)$ is induced from $\piopt(a|s)$.

% % With detailed derivations in \myapp{kl_conj_all}, the solution to the conjugate optimization is
% % Considering this conditional \kl divergence as a function of $\mu(a,s)$ and enforcing normalization, we obtain the following conjugate optimization.   With detailed derivations in \myapp{kl_conj_all}, 

% % normalized mu conjugate with log-sum-exp solution
% % \footnotesize
% % \begin{align}
% %   \hspace*{-.25cm}   \klconjpii(\dualvar) &= \max \limits_{\mu(a,s) \in \Delta^{|\mathcal{A}| \times |\mathcal{S}|}} \blangle 
% %     \mu, \dualvar 
% %     % \mu(a,s), \dualvar(a,s)
% %     \brangle - \klomegamu \\
% %   &= \frac{1}{\beta} \log \sum \limits_{a,s} \mu(s) \pi_0(a|s) \expof{\beta \cdot \dualvar(a,s)}
% %     % - \blangle \lambda , \mu(a,s) - 1\brangle
% % \end{align}
% % \normalsize

% % \RB{Emphasize derivation of $\pi_* = \nabla \Omega^{*}(Q)$}
% % The value function, or conjugate $\alphaconjn(Q)$, as a function $Q$ and with restriction to normalized $\pi$, is

% %For the \textsc{kl} divergence, 
% % This matches the normalization constant for the optimal policy, with $V_*(s) = \psi(s;\beta)$ and
% %  \begin{align}
% %  \pi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s) -  \psi(s;\beta)\big)} \, ,\label{eq:kl_opt_policy}
% %  \end{align}
% % This can also be seen by plugging $\alpha = 1$ into \cref{eq:alpha_conj_norm_main}.
% % Apart from the case of $\alpha=1$, we can see from \cref{eq:alpha_conj_norm_main} that $V_*(s) \neq \normalizeralpha$.
% % We discuss the relationship between $V_*(s)$ and $\normalizeralpha$ for general $\alpha$ in more detail in \mysec{optimal_policy}, while the optimal policy expressions in \cref{eq:alpha_opt_policy} and (\ref{eq:kl_opt_policy}) will also play a central role.


% \paragraph{$\alpha$-Divergence} The $\alpha$-divergence over possibly unnormalized measures,  $\omegamu &=
% \mathbb{E}_{\mu(s)}\big[
% D_{\alpha}[\tpi_0:\tpi]
% \big]$, is defined as 
% \footnotesize
% \begin{align}
% \hspace*{-.15cm} 
% \omegamu &=
% % \mathbb{E}_{\mu(s)}\big[
% % D_{\alpha}[\tpi_0:\tpi]
% % \big]
% % &= 
% \frac{1}{\alpha(1-\alpha)} 
% % \sum \limits_{s \in \mathcal{S}}
% \sum \limits_{s}
% \mu(s)
%     \bigg( (1-\alpha) 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a} 
%     \tpi_0(a|s) 
%     %+\alpha 
%     \\ \phantom{\sum \limits_{s}
% \mu(s)} + \alpha 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a} 
%     \tpi(a|s) \nonumber 
%     % &- \sum \limits_{a \in \mathcal{A}} 
%     % \\ &\phantom{\sum \limits_{s} \mu(s)} 
%     - \sum \limits_{a} 
%     \tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} \bigg)  \label{eq:alpha_def}
% \end{align}
% \normalsize
% with the forward \kl divergence $D_{KL}[\tpi:\tpi_0]$ in \cref{eq:kl_def}
% % in \cref{eq:kl_def}
% % , \textcolor{red}{extended to take unnormalized densities as input, }
% recovered in the limit as $\alpha \rightarrow 1$.  
% As discussed in \myapp{tsallis}, the $\alpha$-divergence is closely related to the Tsallis entropy. \RB{Introduce $\log_{\alpha}$ first? (with the goal of reaching this insight)}
% % \citep{lee2019tsallis}, as we discuss in detail in \myapp{tsallis}.  
% % To see this, 

% For later convenience, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential,
% % \small
% % \begin{align}
% %     \log_{\alpha}(u) &= \begin{cases} \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \hfill \, \, \alpha \neq 1 \\
% %     \log(u) \hfill \, \, \alpha =1 \end{cases} \\
% %     \exp_{\alpha}(u) &= \begin{cases} [1 + (\alpha-1) \cdot u ]_+^{\frac{1}{\alpha-1}} \hfill \, \,  \alpha \neq 1 \\
% %     \exp(u) \hfill \, \, \alpha =1 \end{cases} \, .
% % \end{align}
% \begin{align}
%     \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , \\
%     \exp_{\alpha}(u) &= [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, .
%     % \hfill \, \,  \alpha \neq 1 \
% \end{align}
% % \begin{equation}
% % \resizebox{.87\columnwidth}{!}{\hspace*{-.36cm}
% %     $\log_{\alpha}(u) &= \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \\
% %     \quad 
% %     \exp_{\alpha}(u) = [1 + (\alpha-1) u ]_+^{\frac{1}{\alpha-1}}$
% % }
% % \end{equation}
% % \normalsize
% and we recover the natural logarithm and exponential in the limit as $\alpha \rightarrow 1$.

% With detailed derivations in \myapp{alpha_conj_norm}, the conjugate function for conditional divergence regularization takes the form
% \footnotesize
% \begin{align}
%      \hspace*{-.2cm} &\alphaconj(\dualvar) = \max \limits_{\mu(a,s)} \blangle \mu(a|s), \dualvar(a,s) \brangle -  \omegamu \label{eq:alpha_conj_norm_main} \\
%     &\phantom{=}= \frac{\alpha-1}{\alpha} \blangle \mu(s) \pi_{\dualvar}(a|s), \dualvar(a,s) \brangle + \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi_{\dualvar}] \nonumber
% %   \frac{1}{\alpha}  \normalizeralpha 
%     % \label{eq:alpha_conj_norm_main}
% \end{align}
% \normalsize
% As we discuss in \mysec{adversarial_perturb} or \myapp{alpha_conj_norm}, the final term $\frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi_{\dualvar}]$ 
% % plays the role of the normalization constant for 
% normalizes
% the policy in the optimizing argument $\pi_{\dualvar}(a|s) = \mu_{\dualvar}(a,s)/ \mu(s)$.   In particular, the policy has the form
% \footnotesize
% \begin{align}
%     \pi_{\dualvar}(a|s) = \pi_0(a|s) \exp_{\alpha} \big\{\beta \cdot \big( \dualvar(a,s) - \frac{1}{\beta}(1-\alpha)D_{\alpha}[\pi_0:\pi_{\dualvar}] \big)  \big\}
% \end{align}
% \normalsize
% \textcolor{blue}{wrap up / transition sentence}

% \RB{Introduce notation for normalizer / $D_{\alpha}$?}
% \RB{Inspect.  Reference App. and \textbf{optimal policy expression}}


==> Reward Robustness TMLR (3)/sections/new/2_adv_interp.tex <==
\headerv
\section{Adversarial Interpretation}\label{sec:adversarial_perturb}
\headerv
\normalsize
% In this section, we leverage tools from convex duality to interpret regularization as implicitly providing robustness to adversarial perturbations of the reward function.
% % $\alpha$-divergence regularized policies to adversarial perturbations of the reward function.  
% % In this section, we show that policy regularization can be understood as a game against an imaginary, reward-perturbing adversary.  
% % We analyze the limited feasible set of perturbations available to the adversary for a given regularization scheme, and relate this to zero-shot generalization of the policy.  
% % \TG{Maybe even simpler / clearer: ``In this section we show precisely how policy regularization can be interpreted as as an imaginary game against a reward-perturbing adversary. We analyze the adversary and its limitations (through the feasible set) and relate it to zero-shot robustness of the policy.'' (or something along these lines).}
% Our contributions include characterizing the 
% robust set of adversarial perturbations 
% in \cref{fig:feasible_set_main} and \myprop{feasible}, 
% with additional discussion in \mysec{entropy_vs_div}-\ref{sec:related} 
% %and \myapp{eysenbach}.
% %in relation to related work 
% We analyze the worst-case reward perturbations associated with an arbitrary stochastic policy in \mysec{any_policy}, which extends \citet{ortega2014adversarial} to multi-step \gls{MDP}s with $\alpha$-divergence regularization.   Finally, in \mysec{optimal_policy} we 
% % provide a unified discussion of \citet{eysenbach2021maximum, } and
% \textcolor{red}{follow \citet{husain2021regularized} in showing that,} for the \textit{optimal} policy in a given \gls{MDP}, the worst-case adversarial perturbations correspond to the advantage function.
% \RB{New Intro section.  Shorten?  Rewrite? Previous version commented out}
% % chosen by the adversary.   First, we consider arbitrary stochastic polic
% % for arbitrary stochastic policies.
% % in two different cases.   We consider 
% % Our analysis unifies and extends similar interpretations from \citep{ortega2014adversarial, eysenbach2021maximum, husain2021regularized}. 
% % PREVIOUS AI STATS
% % \RB{Previous}
% % In the following two sections, we leverage tools from convex duality to analyze the robustness of regularized policies to adversarial perturbations of the reward function. 
% % Our contributions include characterizing the 
% % robust set of adversarial reward perturbations 
% % in \cref{fig:feasible_set_main} and \myprop{feasible}, providing derivations for the $\alpha$-divergence, and connecting the worst-case adversarial perturbations with the advantage function for the optimal policy.  Our analysis unifies and extends similar interpretations from \citep{ortega2014adversarial, eysenbach2021maximum, husain2021regularized}.  
% To derive an adversarial interpretation of regularized policies, 
% \RB{More intro necessary?  e.g. Section outlines, emphasis on contributions?  Prev versions commented out}
In this section, we interpret regularization as implicitly providing robustness to adversarial perturbations of the reward function.  To derive our adversarial interpretation, recall from \cref{eq:conjomega} that conjugate duality yields an alternative representation of the regularizer 
% function $\Omega(\mu)$
%we use tools from convex duality to
% regularization function
% To derive an adversarial interpretation of regularized policies, we recall from \cref{eq:conjomega} that the convex conjugate provides an alternative representation of the regularization function
% \RB{Clarify relationship to \cref{eq:conjomega}}
% function.  
% We denote this conjugate as $\alphaconjmu$ and, using \cref{eq:conjomega},
% Using \cref{eq:conjomega}, we have %$\frac{1}{\beta}\Omega_{\pi_0}(\pi)$.   
% \scriptsize
% \begin{align}
\ifx\omitindices\undefined
\begin{equation}
\hspace*{-.2cm}
% \resizebox{.9\columnwidth}{!}{
% $
%       $\omegamu = \max \limits_{\prpi(a,s)} \langle \mu(a,s), \prpi(a,s) \rangle - \alphaconj(\prpi) .$ 
%      \label{eq:conjomega2} }
     \omegamu = \max \limits_{\prinit(a,s)} \langle \mu(a,s), \prinit(a,s) \rangle - \alphaconj(\prinit) . \label{eq:conjomega2} 
    %  $}
 \end{equation}
%  \end{align}
 \else
 \begin{equation}
\hspace*{-.2cm}
     \omegamu = \max \limits_{\prinit \in \rprimedomain} \, \langle \mu, \prinit \rangle - \alphaconj(\prinit) . \label{eq:conjomega2} 
    %  $}
 \end{equation}
 \fi
 \normalsize
 
% In contrast to \mysec{conj_examples}, we consider the conjugate $\omegamu$ derived using optimization over the full state-action occupancy measure $\mu(a,s)$.  
% Note that we optimize over $\mu(a,s)$ as in \cref{eq:dual_lagrangian}, instead of $\pi(a|s)$ as in \cref{eq:alpha_conj_norm_main}.
% Expanding the regularization term in the primal objective (\cref{eq:primal_reg}) using this conjugate optimization, we obtain 
Using this conjugate optimization to expand the regularization term in the primal objective of \cref{eq:primal_reg}, 
% we obtain
% Expanding the regularization term in the primal objective (\cref{eq:primal_reg}) with this conjugate optimization, we obtain
% \footnotesize
% \resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
% \begin{align}
\ifx\omitindices\undefined
\begin{equation}
\hspace*{-.2cm} 
% \resizebox{.9\columnwidth}{!}{$
\obj_{\Omega, \beta}(r) = \max \limits_{\mu \in \mathcal{M}}  \min \limits_{\textcolor{\highlight}{\prinit(a,s)}} 
  \langle {\mu(a,s)}, {r(a,s) - \textcolor{\highlight}{\prinit(a,s)}} \rangle  + \alphaconj \big( \textcolor{\highlight}{\prinit} \big) . 
% $
%   \nonumber 
% }
\label{eq:pedro_form} 
\end{equation}
\else
\begin{equation}
\hspace*{-.2cm} 
% \resizebox{.9\columnwidth}{!}{$
\obj_{\Omega, \beta}(r) = \max  \limits_{\mu \in \mathcal{M}}  \min \limits_{\textcolor{\highlight}{\prinit \in \rprimedomain}} 
  \, \langle {\mu}, {r - \textcolor{\highlight}{\prinit}} \rangle  + \alphaconj \big( \textcolor{\highlight}{\prinit} \big) . 
% $
%   \nonumber 
% }
\label{eq:pedro_form} 
\end{equation}
\fi
% \end{align}
% }}
\normalsize
We interpret 
\cref{eq:pedro_form}
% this optimization 
as a two-player minimax game between an agent and an implicit adversary, where the agent chooses an occupancy measure $\mu(a,s) \in \mathcal{M}$ or its corresponding policy $\pi(a|s)$,
% \textcolor{red}{subject to $\mu(a,s) \in \mathcal{M}$}, 
% while 
and 
the adversary chooses reward perturbations $\prinit(a,s)$ 
% with the
subject to the convex
conjugate $\alphaconj(\prinit)$ as a penalty function \citep{ortega2014adversarial}.

% Expanding the regularization term in the Lagrangian (\cref{eq:dual_lagrangian}) with this conjugate optimization, we obtain
% % , for all $a \in \mathcal{A}, s \in \mathcal{S}$, %\cref{eq:conjomega} %$\Omega_{\pi_0}(\pi)$
% \RB{Will omit in favor of Eq. 17 above?}
% \footnotesize
% \textcolor{red}{
% \begin{align}
%     \hspace*{-.2cm} & \quad \max \limits_{\mu(a,s)} \min \limits_{V(s), \lambdaplus} \min \limits_{\textcolor{\highlight}{\perturbr(a,s)}} \, \label{eq:pedro_form} \\
%     & \big \langle {\mu(a,s)}, {r(a,s) +\gamma \transitionv - V(s) + \lambdaplus - \textcolor{\highlight}{\perturbr(a,s)}} \brangle  \nonumber  \\
%     & \qquad + \alphaconjm \big( \textcolor{\highlight}{\perturbr} \big) + (1-\gamma) \blangle \nu_0(s), V(s) \brangle \, ,  \nonumber
% \end{align}
%     }
% \normalsize

% % where we have changed the maximization in \cref{eq:conjomega2} to a minimization since $\omegamu$ is subtracted. 
% We interpret this optimization as a two-player \textcolor{red}{minimax} game between an agent and an implicit adversary.   The agent chooses a policy $\pi(a|s)$ or occupancy measure $\mu(a,s)$, \textcolor{red}{subject to the flow constraints enforced by the Lagrange multipliers $V(s)$}.  The adversary chooses a reward perturbation $\perturbr(a,s)$, with the convex conjugate $\alphaconjm(\perturbr)$ as a penalty function \citep{ortega2014adversarial}.
% \RB{Experimenting with shoving $V(s)$ into constraint on $\mu$. This emphasizes 2 player game, primal view.   We might be concerned about the constraint, but we can induce $\mu(s)$ and $\mu(a,s) \in \mathcal{M}$ by running any policy to $\infty$.}



% \RB{Clarify 2-player nature, not 3 (what does focus on $\mu(a,s)$ say about role of $V(s)$?)}
% For a fixed value function $V(s)$, we interpret this minmax optimization as a two player game between an agent, which chooses a policy $\pi(a|s)$ or occupancy measure $\mu(a,s)$, and an implicit adversary, which chooses a reward perturbation $\perturbr(a,s)$ with the conjugate $\alphaconjmu(\perturbr)$ as a penalty function \citep{ortega2014adversarial}. 
% % To understand this adversary, we first derive the worst-case perturbation strategy for the adversary.
% To understand the limitations this penalty imposes on the adversary, we first derive the worst-case reward perturbations $\prpi(a,s)$, before characterizing the feasible set \textcolor{blue}{of reward perturbations in \mysec{feasible}.}



% with the Lagrange multipliers $V(s)$ enforcing the flow constraints of the \gls{MDP}.  
To understand the limitations this penalty imposes on the adversary, we transform the optimization over $\pr$ 
in \cref{eq:pedro_form} 
to a constrained optimization in \mysec{generalization}.  This allows us to characterize the feasible set of
% strategies 
reward perturbations
available to the adversary or, equivalently, the set of modified rewards $\mr(a,s) \in \feasibleset$ to which a particular stochastic policy is robust.
In \mysec{any_policy} and \ref{sec:optimal_policy}, we 
interpret the worst-case adversarial perturbations corresponding to an arbitrary stochastic policy and the optimal policy, respectively.
% provide two interpretations of the worst-case reward perturbations, which describe the optimal strategy for the adversary in response to a given policy.
% \RB{Sentence referencing worst case}

% To understand the limitations this penalty imposes on the adversary, we first derive the optimal worst-case reward perturbations $\prpi(a,s)$, before characterizing the feasible set \textcolor{blue}{available to the adversary in \mysec{feasible}.}

% In \mysec{any_policy} and \ref{sec:optimal_policy}, we analyze the optimal worst-case reward perturbations $\prpi(a,s)$ associated with a given stochastic policy or regularized \gls{MDP}.
% derive the optimal worst-case reward perturbations $\prpi(a,s)$, before characterizing the feasible set \textcolor{blue}{available to the adversary in \mysec{feasible}.}


\headerv
\subsection{Robust Set of Modified Rewards}\label{sec:feasible}\label{sec:generalization}
\headerv

% We characterize the feasible set in the following proposition, with visualizations in \cref{fig:feasible_set_main}.
In order to link our adversarial interpretation to robustness and zero-shot generalization as in 
\cref{eq:reward_perturbation_stmt}-(\ref{eq:generalization}),
% \mysec{intro},
we characterize the feasible set of reward perturbations in the following proposition.
We state our proposition for policy regularization, and discuss differences for $\mu(a,s)$ regularization in \myapp{mu_feasible}.
% \RB{Holds for \textit{policy} regularization, not necessarily $\alpha$-divergence $\mu$ regularization}
% \subsection{Feasible Set}\label{sec:feasible}
% \TG{I like this section. Maybe worth spending one, two sentences re-iterating that we have established the adversarial interpretation, but we also know that the adversary is limited. The most important missing bit then is: the characterization of the adversary via this limitedness (the feasible set), which we're going to show now.}
% \RB{Although the feasible set is general (any $\pi$), the plot is for the case of an optimal policy and is identical to the setting of \citet{eysenbach2021maximum} referenced previously}
% In order to link our adversarial interpretation to robustness and zero-shot generalization, we characterize the feasible set of reward perturbations in the following proposition.
% In the previous section, we have established an adversarial interpretation of regularized policies.   However, we have not 
% which suggests that regularized policies are robust to worst-case reward perturbations.   However, we have not discussed implications for zero-shot generalization or understood the limitations of this adversary.

% robustness to worst-case reward perturbations 
% The adversarial interpretation in  suggests that regularized policies are robust to worst-case reward perturbations.   
%  In particular, it is not clear how the cost function $\alphaconjmu(\pr)$ in \cref{eq:pedro_form} restricts the feasible set $\mathcal{R}$ of perturbations from which the adversary can select.  
%  We characterize the feasible set in the following proposition, with visualizations in \cref{fig:feasible_set_main}.
%  In the following proposition, we provide a simple constraint to characterize the feasible set, with visualizations in \cref{fig:feasible_set_main}.
%  The optimal $\prpi$ in \myprop{optimal_perturbations} suggest a simple constraint to characterize the feasible set in the following proposition.
\begin{restatable}[]{proposition}{feasible}\label{prop:feasible} 
Assume a normalized policy $\pi(a|s)$ for the agent is given, with $\sum_a \pi(a|s) = 1 \, \forall s \in \mathcal{S}$.   Under $\alpha$-divergence policy regularization to a normalized reference $\pi_0(a|s)$, 
% for any value of $\alpha$,
% with $\sum_a \pi_0(a|s) = 1 \, \forall s \in \mathcal{S}$), 
% the feasible set of reward perturbations available to the adversary takes the form 
% \textcolor{\revhl}
\revhl{the optimization over $\pr(a,s)$ in \cref{eq:pedro_form} can be written in the following constrained form}
\ifx\omitindices\undefined
\begin{align}
\min \limits_{\pr(a,s) \in \mathcal{R}^{\Delta}_{\pi}} \blangle \mu(a,s), r(a,s) - \pr(a,s)\brangle \qquad \text{where} \quad
% \alphaconjmu(\pr) 
\mathcal{R}^{\Delta}_{\pi} \coloneqq \left\{ \prrob(a,s) \in  \textcolor{red}{\mathcal{F}} \, \bigg| \, 
\Omega^{*(\alpha)}_{\pi_0,\beta}(\prrob) \leq 0 \right\} ,
% \alphaconj(\prrob) \leq 0 \right\} ,
% \alphaconj(\pr)\leq 0
\label{eq:alpha_feasible} 
% \\\frac{\alpha-1}{\alpha} \langle \mu(s) \pi^{(\pr)}_*(a|s), \pr \rangle - \frac{1}{\alpha}(V^{\pr}_*(s)  \leq 0 \label{eq:alpha_feasible}
\end{align}
\else
\begin{align}
\min \limits_{\pr \in \mathcal{R}^{\Delta}_{\pi}} \blangle \mu, r - \pr \brangle \qquad \text{where} \quad
% \alphaconjmu(\pr) 
\mathcal{R}^{\Delta}_{\pi} \coloneqq \left\{ \prrob \in \rprimedomain  \, \bigg| \, 
\Omega^{*(\alpha)}_{\pi_0,\beta}(\prrob) \leq 0 \right\} ,
% \alphaconj(\prrob) \leq 0 \right\} ,
% \alphaconj(\pr)\leq 0
\label{eq:alpha_feasible} 
% \\\frac{\alpha-1}{\alpha} \langle \mu(s) \pi^{(\pr)}_*(a|s), \pr \rangle - \frac{1}{\alpha}(V^{\pr}_*(s)  \leq 0 \label{eq:alpha_feasible}
\end{align}
\fi
% \textcolor{red}{and where $\mathcal{F}$ is the set of bounded, measurable functions on $\mathcal{A} \times \mathcal{S}$.}
We refer to $\mathcal{R}^{\Delta}_{\pi} \subset \rprimedomain$ as the feasible set of reward perturbations available to the adversary.   This translates to a robust set $\feasibleset$ of modified rewards $\mr(a,s) = r(a,s) - \prrob(a,s)$ 
for the given policy.
% to which the policy is robust.   
These sets depend on the $\alpha$-divergence and regularization strength $\beta$ via the conjugate function.
%%%%%%%%%%%%%%%%%%%%%%%%%%% PREV THM &&&&&&&&&&&&
% the feasible set of 
% adversarial reward perturbations 
% % reward perturbations available to the adversary
% is defined by the constraint
% % and $\sum_a \pi_0(a|s) = 1$, $\forall s \in \mathcal{S}$.
% % For a given policy $\pi(a|s)$ and 
% % % For regularization using any $\alpha$-divergence, the feasible set of reward perturbations 
% % available to the adversary
% % % for the implicit adversary 
% % is defined by the constraint
% \begin{align}
% % \alphaconjmu(\pr) 
% \mathcal{R}^{\Delta}_{\pi} \coloneqq \left\{ \prrob(a,s) \in \mathcal{F} \, \bigg| \, \alphaconj(\prrob) \leq 0 \right\} ,
% % \alphaconj(\pr)\leq 0
% \label{eq:alpha_feasible} 
% % \\\frac{\alpha-1}{\alpha} \langle \mu(s) \pi^{(\pr)}_*(a|s), \pr \rangle - \frac{1}{\alpha}(V^{\pr}_*(s)  \leq 0 \label{eq:alpha_feasible}
% \end{align}
% {where $\mathcal{F}$ is the space of bounded, measurable functions on $\mathcal{A} \times \mathcal{S}$.}
% This translates to the set $\feasibleset$ of modified rewards $\mr(a,s) = r(a,s) - \prrob(a,s)$ to which the policy is robust, and depends on the $\alpha$-divergence and regularization strength $\beta$ via the conjugate function.
% % in \cref{eq:alpha_feasible}. 
% % % via using $\mr(a,s) = r(a,s) - \prrob(a,s)$.
% % This translates to a robust set of modified rewards $\mr(a,s) \in \feasibleset$ using $\mr(a,s) = r(a,s) - \prrob(a,s)$.
% % This translates to a robust set of modified rewards $\mr(a,s) \in \feasibleset$ using $\mr(a,s) = r(a,s) - \prrob(a,s)$.
% % \textcolor{red}{\text{clarify function space for $\mathcal{R}$, e.g. $\textcolor{red}{\pr(a,s) \in \mathcal{F}}$}}

For \textsc{kl} divergence regularization, the constraint is
% this translates to
\begin{align}
   \sum\limits_{a \in \mathcal{A}} \pi_0(a|s) \expof{\beta \cdot \prrob(a,s)} \leq 1 \, . \label{eq:kl_feasible}
\end{align}
\end{restatable}
% \textcolor{red}{We note that this result does not apply for $\alpha$-divergence regularization of $\mu(a,s)$, with detailed discussion in App. \cref{app:}}
% \begin{proof} 
\vspace*{-.2cm}
See \myapp{pf_feasible} for proof, and \mytab{conj_table} for the convex conjugate function $\alphaconj(\prrob)$ associated with various regularization schemes.
\revhl{The proof proceeds by evaluating the conjugate function at the minimizing argument $\prpi$ in \cref{eq:pedro_form} (see \mysec{any_policy}), with $\Omega^{*(\alpha)}_{\pi_0,\beta}(\propt)=0 \, \forall \alpha$ for normalized $\pi(a|s)$ and $\pi_0(a|s)$.  
The constraint 
% for the minimization problem in \cref{eq:pedro_form} 
then follows from the fact that $\Omega^{*(\alpha)}_{\pi_0,\beta}(\propt)$ is convex and increasing in $\pr$ \citep{husain2021regularized}.}
%worst-case $\prpi$ (see \mysec{any_policy}),
% We provide expressionsfor the convex conjugate $\alphaconj$ for various 
% $\alpha$-divergence 
% regularization schemes in \mytab{conj_table}.    }.
We visualize the robust set for a two-dimensional action space in \myfig{feasible_set_main}, with additional discussion in \mysec{visualizations_feasible}. 
% , and provide full discussion in \mysec{visualizations}.



% \textcolor{red}{which proceeds by evaluating the conjugate function at the worst-case $\prpi$, with $\alphaconjn(\prpi)=0 \, \forall \alpha$.  
% % Since $\alphaconjn(\pr)$ is increasing in $\pr$ and the $-\pr(a,s)$ term in \cref{eq:pedro_form} is decreasing, the constraint follows.
% The constraint for the minimization problem in \cref{eq:pedro_form} then follows from the fact that $\alphaconjn(\pr)$ is increasing in $\pr$. \RB{\textbf{no longer holds}: alternative proof given in the appendix}}
% % \RB{improve}
% \end{proof}





% \begin{restatable}[]{proposition}{feasible}\label{prop:feasible} For a given policy $\pi(a|s)$ and any $\alpha$-divergence, the feasible set of reward perturbations $\pr(a,s)$ available to the adversary is defined by the constraint
% \begin{align}
% % \alphaconjmu(\pr) 
% \alphaconj(\pr)
% \leq 0 \label{eq:alpha_feasible} 
% % \\\frac{\alpha-1}{\alpha} \langle \mu(s) \pi^{(\pr)}_*(a|s), \pr \rangle - \frac{1}{\alpha}(V^{\pr}_*(s)  \leq 0 \label{eq:alpha_feasible}
% \end{align}
% For \textsc{kl} divergence regularization, we obtain
% % this translates to
% \begin{align}
%   \sum\limits_{a \in \mathcal{A}} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} \leq 1 \, . \label{eq:kl_feasible}
% \end{align}
% \end{restatable}
% \begin{proof} See \myapp{feasible_pf} for proof. 
% We provide expressions for the convex conjugate $\alphaconj$ for various $\alpha$-divergence regularization schemes in \mytab{conj_table}.
% % \textcolor{red}{which proceeds by evaluating the conjugate function at the worst-case $\prpi$, with $\alphaconjn(\prpi)=0 \, \forall \alpha$.  
% % % Since $\alphaconjn(\pr)$ is increasing in $\pr$ and the $-\pr(a,s)$ term in \cref{eq:pedro_form} is decreasing, the constraint follows.
% % The constraint for the minimization problem in \cref{eq:pedro_form} then follows from the fact that $\alphaconjn(\pr)$ is increasing in $\pr$. \RB{\textbf{no longer holds}: alternative proof given in the appendix}}
% % % \RB{improve}
% \end{proof}


% The above feasible set of perturbations $\pr(a,s)$ translates to a robust set of modified rewards $\mr(a,s) \in \feasibleset$ using $\mr(a,s) = r(a,s) - \pr(a,s)$.   
% % For this set of modified rewards,

% For this set of modified rewards $\feasibleset$,
As in \cref{eq:generalization},
we can provide `zero-shot' performance guarantees using this set of modified rewards.
% $\feasibleset$.
% in the sense of \cref{eq:generalization}.   
% In particular, for $\mr(a,s) \in \feasibleset$, 
% we have that $\langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) \rangle - \omegamu$.
\ifx\omitindices\undefined
For any perturbed reward in the robust set $\mr(a,s) \in \feasibleset$, 
we have $\langle \mu(a,s), \mr(a,s) \rangle \geq \langle \mu(a,s), r(a,s) \rangle - \omegamu$, 
\else
For any perturbed reward in the robust set $\mr \in \feasibleset$, 
we have $\langle \mu, \mr \rangle \geq \langle \mu, r \rangle - \omegamu$,
\fi
so that the policy achieves an expected modified reward which is at least as large as the regularized objective. %the value of
% for $\mr(a,s) \in \feasibleset$.   
However, notice that this 
form of robustness is sensitive to the exact value of the 
% regularized objective function, which we discuss in further detail in \mysec{entropy_vs_div}.
% in \cref{eq:robust_def}, 
%  \RB{More here?}
regularized objective function.
% For example, 
Although entropy regularization and divergence regularization with a uniform reference
induce the same optimal $\mu(a,s)$,
% for a uniform reference distribution, 
we highlight crucial differences in their reward robustness interpretations in \mysec{entropy_vs_div}.




% % The above constraints characterize the robust set of modified reward functions for which we can provide performance guarantees, in the sense of \cref{eq:generalization}.   In particular, 
% The above constraints characterize the robust set of modified reward functions for which we can provide performance guarantees.
% % , given a particular stochastic policy and regularized objective.
% % for a particular stochastic policy and regularized objective.
% More precisely, for given \gls{MDP} transition dynamics, we say that a policy trained with reward $r(a,s)$ and 
% % and regularization based on $\Omega, \pi_0, $  
% regularized objective $\obj_{\Omega,\beta}(r)$ 
% \textit{generalizes} to an environment with a modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$ if 
% % , as in \cref{eq:reward_perturbation_stmt},
% \small
% \begin{align}
%   \hspace*{-.2cm} 
% %   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) \rangle - \omegamu \, . \label{eq:robust_def} \\
%   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) \rangle - \omegamu \, . \label{eq:robust_def}
% %   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(s)\pi(a|s), r(a,s) - \ptReg(\pi) \rangle \\
% %   \langle \mu(a,s), \mr(a,s) \rangle &\geq \obj_{\Omega, \beta}(r) = \alphaconjmu \\
% %   \alphaconjmu \text{vs.} \alphaconjmuu \\
% %   \alphaconjn \text{vs.} \alphaconjnn \\
% %   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(s), V_*(s; \beta) \rangle = \langle \mu(s),\alphaconjn \rangle \\
% %   \obj_{\Omega, \beta}(r)  = \alphaconjmu &= \frac{\alpha-1}{\alpha} \langle \mu(s), \alphaconjn \rangle 
% %   \langle \mu(a,s), r(a,s) - \pr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) - \ptReg(\pi) \rangle  %\blangle \mu(s) \pi(a|s), \mr(a,s) \brangle \geq  \blangle \mu(s) \pi(a|s), r(a,s) - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \brangle \, . \label{eq:robust_def}
% \end{align}
% \normalsize
% % \JG{Ok, I think you need to say a couple of sentences here. I was initially confused by this thinking that it was trivial but it is not at all. I think one expects something of the form: $ \langle \mu(a,s), r(s,a) + \Delta r(s,a) \rangle \geq \langle \mu(a,s), r(a,s) \rangle $ for $\Delta r(s,a) \in Z$ where $r(s,a) + \Delta r(s,a) = r'(s,a)$ and $Z$ is the set of allowed perturbations. In its current form with the regularizer it is not clear what this implies for generalization right?. Sorry if this question is too complicated, It could also be that I need more time to understand this. I think its important to get the explanation right though.} 
% In other words, the expected reward using the modified $\mr(a,s)$ is greater than or equal to the value of the regularized objective $\obj_{\Omega,\beta}(r)$ using the original $r(a,s)$. 
% %  on the left side on the right side.  
% Note that \cref{eq:robust_def} holds with equality for the worst-case modified reward $\mropt(a,s)$ (\mysec{optimal_perturb} or \myapp{preserve}). 
% \textcolor{red}{The feasible set in \myfig{feasible_set_main} shows other rewards for which the inequality holds, with equality 
% % holding 
% at the boundary.} \RB{Is this true?  Otherwise, why would we pick out the particular $\Delta r^{*}$ that we do?  Further, the original $r(a,s)$ is at the boundary, and this does not hold with equality.}
% % While it is clear that increasing the reward in both actions preserves the inequality in \cref{eq:robust_def},  
% % % is feasible for an adversary that minimizes \cref{eq:pedro_form}, 
% % \cref{fig:feasible_set_main} also includes regions where one reward decreases.

% % while the feasible set in \myfig{feasible_set_main} shows the other rewards for which the inequality holds. \TG{Shall we mention that the boundary of the feasible set corresponds to the equality?}

% It is in this particular sense that we can claim zero-shot generalization for a regularized policy.
% We also notice that this form of robustness is sensitive to the value of the regularized objective function in \cref{eq:robust_def}, which we discuss in further detail in \mysec{entropy_vs_div}.
% % Note that the expected reward under the worst-case modified reward $\mropt(a,s)$ matches the value of the regularized objective, as we have reasoned in \mysec{optimal_perturb} or \myapp{preserve}, while the feasible set in \myfig{feasible_set_main} shows the other rewards for which \cref{eq:robust_def} holds.
% % Note that the right hand side corresponds to the full objective function, including regularization, whereas the left hand side is only the expected reward.  
% % .regularization, as we further discuss in \mysec{entropy_vs_div}.
% % the other reward functions for a stochastic policy is robust 
% % The feasible set characterizes the other reward functions for which a stochastic policy achieves an expected reward greater than or equal to the value of the regularized objective. \TG{This is very important (for the reader) - make sure to emphasize the ``robustness'' and generalization-guarantee (in terms of performance) we get exactly from this fact.}
% % to which a stochastic policy is robust.

% \headerv
% \paragraph{Visualizing the Feasible Set} \RB{Moved to \cref{sec:visualizations_feasible}}

% In \myfig{feasible_set_main}, we visualize the feasible set of perturbed rewards in a two-dimensional action space for the \kl or $\alpha$-divergence, various $\beta$, and a uniform or non-uniform prior policy $\pi_0$.
% Since the optimal policy can be calculated easily in the single-step case, we consider fixed $Q(a,s) = r(a,s) = \{1.1, 0.8\}$ and show the robustness of the optimal $\pi_*(a|s)$, which differs based on the regularization scheme (see \cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).
% We determine the feasible set of $\pr$ using the constraint in \myprop{feasible} (see \myapp{feasible_plot} for details), and plot the modified reward $r\tick(a,s) = Q(a,s) - \pr(a,s)$ for each action.  
% %  For clarify of exposition, we focus on the \KL divergence constraint in \cref{eq:kl_feasible}.

% Inspecting the constraint for the adversary in \cref{eq:kl_feasible}, note that both reward increases $\pr(a,s) < 0$ and reward decreases $\pr(a,s) > 0$ contribute non-negative terms at each action, which either up- or down-weight the reference policy $\pi_0(a|s)$.  The constraint on their summation forces the adversary to trade off between perturbations of different actions in a particular state.   
% Further, since the constraints in \myprop{feasible} integrate over the action space, the rewards for \textit{all} actions in a particular state must be perturbed together.  
% While it is clear that increasing the reward in both actions preserves the inequality in \cref{eq:robust_def},  
% % is feasible for an adversary that minimizes \cref{eq:pedro_form}, 
% \cref{fig:feasible_set_main} also includes regions where one reward decreases.
% % While it is natural that increasing the reward in both actions is feasible for an adversary that minimizes \cref{eq:pedro_form}, \cref{fig:feasible_set_main} also includes regions where one reward decreases.
% % In all cases, it is natural that increasing the reward in both actions is feasible for an adversary seeking to minimize the objective in \cref{eq:pedro_form}.

% For high regularization strength ($\beta=0.1$), we observe that the boundary of the feasible set is nearly linear, with the slope $-\frac{\pi_0(a_1|s)}{\pi_0(a_2|s)}$ based on the ratio of each action in the prior.  The boundary steepens for lower regularization strength.  We can use the indifference condition to provide further geometric insight.   First, drawing a line from the origin with slope $1$ will intersect the feasible set at the worst-case modified reward (red star) in each panel, with $\mropt(a_1,s) = \mropt(a_2,s)$.  At this point, the slope of the tangent line yields the ratio of action probabilities, as we saw for the $\beta = 0.1$ case.  With decreasing regularization as $\beta \rightarrow \infty$, the slope approaches $0$ or $-\infty$ for a nearly deterministic policy and a rectangular feasible region.
% % ince we have plotted the optimal policy $\piopt(a|s)$ corresponding to the reward function $r(a,s)$, we can see that the indifference condition holds, with $\mropt(a_1,s) = \mropt(a_2,s)$ for the red star in each panel.   In this case, we ca  

% Finally, we show the feasible set for the $\alpha$-divergence with $\alpha \in \{-1, 3\}$ and $\beta = 10$ in \cref{fig:feasible_set_main} (d)-(e) and (i)-(j), with further visualizations in \myapp{additional_feasible}.   Compared with the \textsc{kl} divergence,
% we observe a wider feasible set boundary for $\alpha =-1$, whereas $\alpha = 3$ \textcolor{red}{
% induces a steeper boundary with smaller worst-case perturbations. }
% % \RB{Update the discussion here to reflect modified plots}
% % for the $\alpha = 3$ case, corresponding to a steeper boundary of the feasible set.   
% % \ref{fig:tabd}-\ref{fig:tabe} and \ref{fig:tabi}-\ref{fig:tabj} .  
% % For the optimal policy associated with a given reward function,  we see that the $\alpha = -1$ feasible set may not include this reward function.  





% % , which chooses a policy $\pi(a|s)$ or occupancy measure $\mu(a,s)$, and an implicit adversary, which chooses a reward perturbation $\perturbr(a,s)$ with the conjugate $\alphaconjmu(\perturbr)$ as a penalty function \citep{ortega2014adversarial}.   
% % To understand the limitations this penalty imposes on the adversary, we first derive the optimal worst-case reward perturbations $\prpi(a,s)$, before characterizing the feasible set \textcolor{blue}{available to the adversary in \mysec{feasible}.}



\headerv
\subsection{Worst-Case Perturbations: Policy Form}
% \subsection{Worst-Case Reward Perturbations: Arbitrary Policy}
% % \subsection{Worst-Case Perturbations: Optimal Policy}
% \subsection{Worst-Case $\prpi(a,s)$: Arbitrary Policies}
% % \subsection{Analysis for Arbitrary Stochastic Policies}
\label{sec:any_policy}
\headerv
From the feasible set in \myprop{feasible}, how should the adversary select its reward perturbations?
% For an arbitrary, fixed stochastic policy, 
In the following proposition,
we use the optimality conditions in \cref{eq:optimal_policy_as_grad}
to solve for the \textit{worst-case} reward perturbations $\prpi(a,s)$ which minimize \cref{eq:pedro_form} for an fixed but arbitrary stochastic policy $\pi(a|s)$.   
% This leads to the
% in the 
% following proposition.
% \footnote{We use optimality notation for the worst-case reward perturbations $\propt(a,s)$, since they are optimal in the sense of \cref{eq:conjomega2}.   These perturbations are associated with a given, possibly suboptimal $\pi(a|s)$ or $\mu(a,s)$. }
% Using the optimality condition for the conjugate optimization in \cref{eq:optimal_policy_as_grad}, we can solve for the worst-case reward perturbations $\proptpi(a,s)$ in the following proposition.
% = \nabla \omegamu = (\nabla \alphaconjmu)^{-1}(\mu)$
% \footnote{Note that we use the notation $\proptpi(a,s)$ to refer to the worst-case or `optimal' reward perturbations associated with a given, \textit{possibly suboptimal} $\pi(a|s)$ or $\mu(a,s)$.}  

% \footnote{We use the notation $\proptpi(a,s)$ to refer to the worst-case reward perturbations, which are optimal in the sense of \cref{eq:conjomega2}, but are associated with a given, possibly \textit{suboptimal} $\pi(a|s)$ or $\mu(a,s)$.}  

% \RB{Change $\propt$ notation based on footnote?}
\begin{restatable}[]{proposition}{optimalperturbations}
\label{prop:optimal_perturbations} 
For a given policy $\pi(a|s)$ or state-action occupancy $\mu(a,s)$, 
the worst-case adversarial reward perturbations $\prpi$ or $\prmu$ associated with a 
% $\alpha$-divergence 
convex function $\Omega(\mu)$ and regularization strength $1/\beta$ 
are
% are given by
\ifx\omitindices\undefined
\begin{align}
    \hspace*{-.23cm} \prpi(a,s) = \nabla_{\mu} \frac{1}{\beta} \Omega(\mu) \, .
    % - \lambdaplus  
    \label{eq:prop1}
\end{align}
\else
\begin{align}
    \hspace*{-.23cm} \prpi = \nabla_{\mu} \frac{1}{\beta} \Omega(\mu) \, .
    % - \lambdaplus  
    \label{eq:prop1}
\end{align}
\fi
% where the Lagrange multiplier $\lambdaplus$ enforces $\mu(a,s) \geq 0$.
% where $\lambdaplus$ is a Lagrange multiplier enforcing $\mu(a,s) \geq 0$.
\end{restatable}
See \myapp{prop2} for proof. %\myapp{joint_derivation} 
We now provide example closed form expressions for the worst-case reward perturbations under common regularization schemes.
We emphasize that the same stochastic policy $\pi(a|s)$ or joint occupancy measure $\mu(a,s)$ can be associated with different adversarial perturbations depending on the choice of $\alpha$-divergence and strength $\beta$.\footnote{One exception is that a policy with $a\tick$ s.t. $\pi(a\tick|s)=0$ can only be represented using \textsc{kl} regularization if $\pi_0(a\tick|s) = 0$.}
\headerv
\paragraph{KL Divergence} For \kl divergence policy regularization, the worst-case reward perturbations 
are
% take the form 
% \small
\begin{align}
    \prpi(a,s) = \frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)} \, , \label{eq:kl_perturbations}
\end{align}
\normalsize
which 
corresponds to the pointwise regularization $\prpi(a,s)=\ptReg_{\pi_0}(\pi(a|s)$ for each state-action pair, with $\Omega_{\pi_0}(\mu)= \mathbb{E}_{\mu(a,s)}[\ptReg_{\pi_0}(\pi(a|s)]$.   
% \textcolor{blue}{Note that the ratio $\frac{\pi(a|s)}{\pi_0(a|s)}$ appears naturally after differentiating with respect to $\mu(a,s)$ as in \cref{eq:prop1}.}
% Note that we can ignore $\lambdaplus$ since 
{See \myapp{conj1}}.
% for derivations.
% We discuss the role of the Lagrange multiplier $\lambdaplus$ in \mysec{value_form}.}
% Note that we omit $\lambdaplus$, since a policy with $a_0$ such that $\pi(a_0|s) = 0$ can only be represented using \textsc{kl} divergence regularization if $\pi_0(a_0 | s) = 0$.
% We provide detailed derivations in \myapp{kl_conj_all}.
% In \mytab{conj_table} and  
We show an analogous result in \myapp{conj2}
% can be shown
for 
%joint
state-action occupancy regularization $\KL[\mu:\mu_0]$, where $\prmu(a,s) = \frac{1}{\beta} \log 
% \mu(a|s)/\mu_0(a,s)= \ptReg_{\mu_0}(\mu)$.
 \frac{\mu(a,s)}{\mu_0(a,s)}= \ptReg_{\mu_0}(\mu(a,s))$.
 
% For \kl divergence regularization, the worst-case reward perturbations directly correspond to the pointwise regularization term.  For example, 
% for conditional policy regularization % $\ptReg(\pi) = \log \pi(a|s)/\pi_0(a|s)$
% \begin{align}
%     \prpi(a,s) = \frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)} \, ,
% \end{align}
% which corresponds to the pointw


% \RB{Need to actually have the $\lambdaplus$ correction...}
% \headerv
\paragraph{$\alpha$-Divergence} For \kl divergence regularization, the worst-case reward perturbations had a similar expression for conditional and joint regularization.   However, we observe notable differences 
% notable differences 
for the $\alpha$-divergence in general.  For policy regularization to a reference $\pi_0$,
% While the reward perturbations had analogous expressions for conditional and joint regularization using the \kl divergence,  we notice differences for the $\alpha$-divergence. 
% \small
\begin{align}
    \hspace*{-.23cm} \prpi(a,s) = \frac{1}{\beta} \log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)} + 
    % \underbrace{
    \psipr ,
    % \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi]
    % }_{\textcolor{red}{\psi_{\pr}(s)}} 
    % - {\lambdaplus} 
    \label{eq:optimal_perturbations}
\end{align}
\normalsize
where we define $\psipr$ as
\small
\begin{equation}
%   \hspace*{-.3cm}  \resizebox{.91\columnwidth}{!}{
    \psipr \coloneqq \frac{1}{\beta}\frac{1}{\alpha} \left( \sum \limits_{a \in \mathcal{A}} \pi_0(a|s)- \sum \limits_{a \in \mathcal{A}} \pi_0(a|s)^{1-\alpha} \pi(a|s)^\alpha \right).
    % $ . 
    % }
    \label{eq:pr_normalizer}
\end{equation}
\normalsize
As we discuss in \myapp{conj3}, $\psipr$ plays the role of a normalization constant for the optimizing argument $\pir(a|s)$ in the definition of $\alphaconjn(\pr)$ (see \cref{eq:conjstar}, \mytab{conj_table}).  This term arises from differentiating $\Omega^{(\alpha)}_{\pi_0}(\mu)$ with respect to $\mu(a,s)$ instead of from an explicit constraint.
% This normalization term naturally arises from differentiating 
% % the conditional regularization 
% $\Omega^{(\alpha)}_{\pi_0}(\mu)$
% % =\mathbb{E}_{\mu(a,s)}[\ptReg_{\pi_0}^{(\alpha)}(\pi(a|s))]$
% with respect to $\mu(a,s)$, rather than using an explicit constraint.
Assuming the given $\pi(a|s)$ and reference $\pi_0(a|s)$ are normalized, note that $\psipr = \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi]$.   
With normalization, we also observe that $\psipr = 0$ for \kl divergence regularization ($\alpha=1$), which confirms \cref{eq:kl_perturbations} is a special case of \cref{eq:optimal_perturbations}. 

%%%%%%%%%%%%%%%%%%% PREV $$$$$$$$$$$$$$$$$$$$$$$$$
% where $\psi_{\pr}(s)$ 
% % plays the role of 
% is a normalization constant 
% % in the conjugate optimization 
% % for $\pi$
% % for $\pir(a|s) \coloneqq \pi(a|s)$, 
% which naturally appears from differentiating the conditional regularization $\Omega^{(\alpha)}_{\pi_0}(\mu)$
% % =\mathbb{E}_{\mu(a,s)}[\ptReg_{\pi_0}^{(\alpha)}(\pi(a|s))]$
% with respect to $\mu(a,s)$.   In particular,  we can write $\psi_{\pr}(s)$ in self-consistent fashion as
% % $\psi_{\pr}(s)= \frac{1}{\beta}\frac{1}{\alpha}( \sum \pi_0(a|s)- \sum \pi_0(a|s)^{1-\alpha} \pi(a|s)^\alpha$ 
% \footnotesize
% \begin{equation}
%   \resizebox{.9\columnwidth}{!}{
%      \hspace*{-.3cm} $\psipr = \frac{1}{\beta}\frac{1}{\alpha} \left( \sum \limits_{a \in \mathcal{A}} \pi_0(a|s)- \sum \limits_{a \in \mathcal{A}} \pi_0(a|s)^{1-\alpha} \pi(a|s)^\alpha \right)$ %_{\pr}
%  }\label{eq:pr_normalizer}
% \end{equation}
% % \begin{align}
% %   \hspace*{-.3cm} \psi_{\pr}(s)= \frac{1}{\beta}\frac{1}{\alpha} \left( \sum \limits_{a \in \mathcal{A}} \pi_0(a|s)- \sum \limits_{a \in \mathcal{A}} \pi_0(a|s)^{1-\alpha} \pi_{\pr}(a|s)^\alpha \right)
% % \label{eq:pr_normalizer}
% % \end{align}
% \normalsize
% % \RB{Mention that this looks like a $D_{\alpha}$?}
% % where $\pir(a|s)$ is 
% with 
% % detailed 
% derivations in \myapp{conj3}. 
% % and additional discussion in \myapp{advantage_confirm}. 
% % Note that $\psipr = \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi]$ for normalized $\pi$, $\pi_0$. 
% % \RB{Check:  Should be $\pi_\pr$ notation?}
% Assuming that the given $\pi(a|s)$ and reference $\pi_0(a|s)$ are normalized, note that $\psipr = \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi]$.   
% With normalization, we also observe that $\psipr = 0$ for \kl divergence regularization ($\alpha=1$), which confirms that \cref{eq:kl_perturbations} is a special case of \cref{eq:optimal_perturbations}. 

%%%%%%%%%%%%%%%%%%% PREV $$$$$$$$$$$$$$$$$$$$$$$$$


% In this case, we also observe that $\psi_{\pr}(s) = 0$ for \kl divergence regularization ($\alpha=1$), which confirms that \cref{eq:kl_perturbations} is a special case of \cref{eq:optimal_perturbations}. 
% Assuming the given $\pir(a|s)$ and reference $\pi_0(a|s)$ are normalized, note that 
% we note that $\psi_{\pr}(s) = 0$ for \kl divergence regularization ($\alpha=1$), which confirms that \cref{eq:kl_perturbations} is a special case of \cref{eq:optimal_perturbations}. 
%In \myapp{soft_value}, we further discuss this normalization constant in the context of soft value aggregation and regularized Bellman optimality operators \citep{lee2019tsallis, geist2019theory} using $\alpha$-divergence regularization.  
% In particular, we distinguish between the policy normalization constant $\psi_{Q_*}(s)$ and the value or conjugate function $V_*(s) =  \alphaconj(Q_*)$ \citep{geist2019theory}, which match only in the case of \textsc{kl} divergence regularization.
% We can thus recognize the expression  as a special case of  since $\psi_{\pr}(s) = 0$. 

% Assuming that $\pi_0(a|s)$ is normalized and using that $\sum_a \pi(a|s) = \frac_a \frac{\mu(a,s)}{\mu(s)}=  \frac{\frac_a \mu(a,s)}{\mu(s)}= 1$

% Indeed, the expression for $\psi_\pr(s)$ in \cref{eq:pr_normalizer} vanishes for $\alpha =1$ and normalized $\pi_0(a|s)$ and $\pi_\pr(a|s)$, so that $\psi_Q(s) = V(s)$ for \kl divergence regularization.


% We provide additional discussion of this normalization constant in \mysec{optimal_policy}, with detailed derivations in \myapp{perturb_pf}.
% % \textcolor{red}{ See \myapp{alpha_conj_all} for derivations.}

For any given state-action occupancy measure $\mu(a,s)$ and joint $\alpha$-divergence regularization 
% with strength $1/\beta$ and 
to a reference $\mu_0(a|s)$, the worst-case perturbations become
% For joint $\mu(a,s)$ regularization, we obtain
% \small
\begin{align}
    \prmu(a,s) = \frac{1}{\beta} \log_{\alpha}\frac{\mu(a,s)}{\mu_0(a,s)}, \label{eq:pr_mu}
    % - \lambdaplus \, ,
\end{align}
\normalsize
with detailed derivations in \myapp{mu_results}.   
In contrast to \cref{eq:optimal_perturbations}, this expression lacks an explicit normalization constant, as this constraint is enforced by the Lagrange multipliers $V(s)$ and $\mu(a,s) \in \mathcal{M}$ (\myapp{optimal_policy}).
% a normalization constant does not appear in this expression, with normalization enforced by the Lagrange multipliers $V(s)$ and $\mu(a,s) \in \mathcal{M}$ (\myapp{normalized_mu}).


% which matches the pointwise regularization $\ptReg_{\mu_0}(\mu(a,s))$. 
% \begin{restatable}[]{proposition}{optimalperturbations}
% \label{prop:optimal_perturbations} 
% For a given policy $\pi(a|s)$ and conditional $\alpha$-divergence regularization with strength $1/\beta$ and reference $\pi_0(a|s)$, the worst-case adversarial reward perturbations are 
% % \TG{(do we need to add ``policy regularized with alpha-divergence'' to Prop. 1?)}
% \footnotesize
% \begin{align}
%     \hspace*{-.23cm} \prpi(a,s) = \frac{1}{\beta} \log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)} + 
%     % \underbrace{
%     \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi]
%     % }_{\textcolor{red}{\psi_{\pr}(s)}} 
%     - {\lambdaplus} \label{eq:optimal_perturbations}
% \end{align}
% \normalsize
% (b) For any given state-action occupancy measure $\mu(a,s)$ and conditional $\alpha$-divergence regularization with strength $1/\beta$ and reference $\mu_0(a|s)$, the worst-case adversarial reward perturbations are 
% % For joint $\mu(a,s)$ regularization, we obtain
% \normalsize
% \begin{align}
%   \hspace*{-.2cm} \prpi(a,s) = \frac{1}{\beta} \log_{\alpha}\frac{\mu(a,s)}{\mu_0(a,s)} - \lambdaplus
% \end{align}
%  \textcolor{red}{where, in both cases, $\lambdaplus$ is a Lagrange multiplier enforcing $\mu(a,s) > 0$.}
% \end{restatable}
 





% \begin{restatable}[]{proposition}{optimalperturbations}
% \label{prop:optimal_perturbations} 
% (a) For any given policy $\pi(a|s)$ and conditional $\alpha$-divergence regularization with strength $1/\beta$ and reference $\pi_0(a|s)$, the worst-case adversarial reward perturbations are 
% % \TG{(do we need to add ``policy regularized with alpha-divergence'' to Prop. 1?)}
% \footnotesize
% \begin{align}
%     \hspace*{-.23cm} \prpi(a,s) = \frac{1}{\beta} \log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)} + 
%     % \underbrace{
%     \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi]
%     % }_{\textcolor{red}{\psi_{\pr}(s)}} 
%     - {\lambdaplus} \label{eq:optimal_perturbations}
% \end{align}
% \normalsize
% (b) For any given state-action occupancy measure $\mu(a,s)$ and conditional $\alpha$-divergence regularization with strength $1/\beta$ and reference $\mu_0(a|s)$, the worst-case adversarial reward perturbations are 
% % For joint $\mu(a,s)$ regularization, we obtain
% \normalsize
% \begin{align}
%     \prpi(a,s) = \frac{1}{\beta} \log_{\alpha}\frac{\mu(a,s)}{\mu_0(a,s)} - \lambdaplus
% \end{align}
%  \textcolor{red}{where, in both cases, $\lambdaplus$ is a Lagrange multiplier enforcing $\mu(a,s) \geq 0$.}
% \end{restatable}
 
 
 
%  See \myapp{perturb_pf_sub}
% %  \myapp{joint_derivation} 
%  for proof. 
% In \myapp{preserve}, we confirm the identity in \cref{eq:conjomega2} for these worst-case reward perturbations
% % , so that 
% .  This shows that
% our adversarial interpretation 
% % of the Lagrangian in \cref{eq:dual_lagrangian}
% does not change the value of the overall objective in \cref{eq:dual_lagrangian}.   
% For the \textsc{kl} divergence ($\alpha =1$), we directly obtain the pointwise regularization term $\prpi(a,s) = \frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)}$ when $\pi(a|s) > 0$.
























% \subsection{Worst-Case Perturbations: Value Form}
% % \subsection{Analysis for the Optimal Policy}
% % \subsection{Worst-Case Reward Perturbations: Optimal Policy}
% % \subsection{Worst-Case $\proptv(a,s)$: Optimal Policy}
% \label{sec:optimal_policy}
% \headerv
% % In the previous section, we showed that \textit{any} stochastic policy may be interpreted via an adversarial game for given $\Omega, \pi_0,$ and $\beta$.  
% In the previous section, we analyzed the implicit adversary corresponding to \textit{any} stochastic policy $\pi(a|s)$ for a given  $\Omega, \pi_0,$ and $\beta$.
% We now take a dual perspective, where the adversary is given access to 
% \textcolor{red}{the value function $V_{\pi}(s)$ of the agent }
% in each state, and the value is calculated with respect to a particular regularized objective (\citet{geist2019theory} Def. 2).
% % (\textcolor{red}{see \myapp{soft_value}}).

% % % \paragraph{Modified Reward Intepretation}
% % Our starting point is Theorem 3 of \citet{husain2021regularized} which, adapted to our setting and notation, expands the regularized dual optimization in \cref{eq:dual_reg} to include a minimization over the modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$

% % \begin{restatable}[{Theorem 3 \citep{husain2021regularized}}]{theorem}{husain}
% % \label{thm:husain}
% % %  \begin{restatable}{proposition}{husain}
% % % [\textbf{Advantage Function}]
% % The optimal value of the regularized objective $\obj_{\Omega, \beta}(r)$ in \cref{eq:primal_reg}, or its dual $\obj^{*}_{\Omega, \beta}(r)$ in \cref{eq:dual_reg}, 
% % is equal to
% % \footnotesize
% % \begin{align}
% %   \hspace*{-.2cm} \inf \limits_{V(s)} &\inf \limits_{\mr(a,s)}   
% %     %&
% %   (1-\gamma) \blangle \nu_0(s), V(s) \brangle 
% %     % \\ & 
% %     + \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left( 
% %     % \pr(a,s)
% %     % \pr(a,s)
% %     r(a,s) - \mr(a,s)
% %     % r(a,s) + \gamma \transitionvpi - \vpi 
% %     \right) \nonumber \\
% %     &\text{subj. to  } V(s) \geq \mr(a,s) + \gamma \transitionv \quad
% %     \forall (a,s)
% %     % \in \mathcal{A} \times \mathcal{S}
% %     \label{eq:husain_constrain}
% % \end{align}
% % \normalsize
% % \end{restatable}
% % \begin{proof} 
% % Note that this optimization may be obtained by eliminating $\mu(a,s)$ from the Lagrangian in \cref{eq:pedro_form}.   When the constraint is satisfied with equality, we recover the regularized dual objective in \cref{eq:dual_reg}.
% % We rewrite an alternative proof from \citet{husain2021regularized} using our notation in \myapp{husain_conjugate}.
% % \end{proof}
% % % Note that, instead of expanding the conjugate of the regularization function as in \cref{eq:conjomega2}, \citet{husain2021regularized} consider the convex conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} regularized optimization,
% % % $\obj_{\Omega,\beta}(r)$, which is a concave function of $\mu$ by \cref{eq:primal_reg}.
% % % \footnote{From \cref{eq:primal_reg}, we see that $\obj_{\Omega,\beta}(r)$ is a concave function of $\mu$.}   

% % It is insightful to compare \cref{eq:husain_constrain} to the unregularized dual objective in \cref{eq:dual_lp}, which has a constraint involving the unmodified reward function and does not include the adversarial cost $\frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left(r -\mr \right)$.   
% % As in \mysec{any_policy}, the adversary incorporates the effect of policy regularization by modifying the reward function, subject to a penalty on $\pr(a,s) = r(a,s) -\mr(a,s)$.


%  \begin{restatable}{proposition}{advantage} 
% % [\textbf{Advantage Function}]
% \label{prop:advantage} Consider the value function $V_\pi(s)$ associated with a given policy $\pi(a|s)$.   For $\alpha$-divergence regularization with any $\alpha$, the worst-case adversarial reward perturbations $r_V(a,s)$ correspond to the advantage function
% % can be expressed as
% \begin{align}
%     %  \proptv(a,s) &= Q_{*}(a,s) - V_*(s) \, . \label{eq:advantage} \\
%      \proptv(a,s) &= r(a,s) + \gamma \transitionv- V(s)\, .
% \end{align}
% \end{restatable}
% \begin{proof}
% Differentiating \cref{eq:pedro_form} with respect to $\mu(a,s)$, we obtain the optimality condition that $\pr(a,s) = r(a,s) + \gamma \transitionv - V(s)$.    Plugging this expression back into \cref{eq:pedro_form}, we obtain the regularized dual objective \cref{eq:dual_reg}.
% \end{proof}
% %%% OPTIMAL POLICY section intro
% %  \RB{No longer focusing on optimal}  Our derivations so far have only invoked the conjugate representation of the regularization function, which suggests that \textit{any} stochastic policy may be interpreted via an adversarial game for given $\Omega, \pi_0,$ and $\beta$.    We now analyse the adversarial reward perturbations associated with the \textit{optimal} policy $\pi_*(a|s)$ for a given regularized \gls{MDP}.   
% %  The uniqueness of the optimal policy allows us to associate its robustness with a given environment reward function, which is the focus of discussion in \citet{eysenbach2021maximum}.    
% % % Note that these statements rely on our ability to solve for the optimal policy in \cref{eq:primal_reg}.
% % %  We emphasize that the worst-case perturbations in the previous section apply for arbitrary policies, whereas the analysis in this section relies on first solving for the optimal policy according to \cref{eq:primal_reg}.


% % %   \textcolor{red}{While we are able to obtain additional insight for the optimal policy, this comes at the cost of having to solve for the unique optimal policy in \cref{eq:primal_reg}. }
% % %  which is defined via a reward function $r(a,s)$ in a given (regularized) \gls{MDP}. 
% % %  We will see that we can make stronger statements for the conjugate expansion of the optimal policy $\pi_*(a|s)$, which comes at the cost of having to solve for the optimal policy in \cref{eq:primal_reg}. 
% % % We will see that we can make stronger statements in this case, albeit at the cost of having to solve for the unique optimal policy in \cref{eq:primal_reg}. 
% % %  Note that 
% % % For a given regularization scheme and the unique optimal policy $\pi_*(a|s)$, 
% % % we can frame our analysis in terms of robustness associated 
% % %  Note that this allows us to frame the analysis in terms of the robustness associated with a given reward function and regularization scheme, rather than a particular policy \citep{eysenbach2021maximum}.
% % % Note that the uniqueness of the optimal policy $\pi_*(a|s)$ for a chosen regularization scheme allows us to associate its robustness with a given reward function and \gls{MDP}, as in \citet{eysenbach2021maximum}.
 
% %  \begin{restatable}{proposition}{advantage} 
% % % [\textbf{Advantage Function}]
% % \label{prop:advantage} For the optimal policy $\pi_*(a|s)$ and $\alpha$-divergence regularization with any $\alpha$, the worst-case adversarial reward perturbations correspond to the advantage function
% % % can be expressed as
% % \begin{align}
% %     %  \proptv(a,s) &= Q_{*}(a,s) - V_*(s) \, . \label{eq:advantage} \\
% %      \proptv(a,s) &= r(a,s) + \gamma \transitionv- V(s)
% % \end{align}
% % \end{restatable}
% %  \begin{proof}
% %  \RB{Proof is the same as Modified Reward Dual}
% %  Differentiating \cref{eq:pedro_form} with respect to $\mu(a,s)$, we obtain the optimality condition that $\pr(a,s) = r(a,s) + \gamma \transitionv - V(s)$.    Plugging this expression back into \cref{eq:pedro_form}, we obtain the regularized dual objective \cref{eq:dual_reg}.
% %  \RB{Husain citation and mention here}
% %  \end{proof}
% %  \RB{Why wouldn't this hold for any $V(s)$ (not just $V_*$)?   To argue for optimal only, the below derivations imply we need $\pi(a|s) = \pi_0(a|s) \exp_{\alpha}{ \beta (r(a,s) + \gamma \transitionv - V(s)}$ $(\forall s \in \mathcal{S})$. } 
% % %  Also, as a sanity check, we know that we can induce $\mu(a,s) \in \mathcal{M}$ from any $\pi(a|s)$ by running .}

 
%  \paragraph{Optimal Policy}
% We first consider the form of the optimal policy in a regularized \gls{MDP}, which corresponds to the conjugate optimality condition $\primalvar(a,s) = (\nabla \Omega)^{-1}\big(\pr(a,s) \big)$ in \mysec{conj_intro} and \mytab{conj_table}.   For policy regularization using the $\alpha$-divergence, we obtain
% \footnotesize
% \begin{align}
%       \hspace*{-.2cm} &\piopt(a|s)= \label{eq:alpha_opt_policy} \\
%       & \pi_0(a|s) \exp_{\alpha}\bigg\{ \beta \cdot \big( 
%     %   \underbrace{ 
%       r(a,s) + \gamma \transitionv
%     %   \nonumber \\
%     %   & \phantom{= \pi_0(a|s) \exp_{\alpha}\bigg\{} 
%       - V(s)
%     %   }_{\Delta r_*(a,s)}
%       - \psi_{\pr}(s) \big) \bigg\}. \nonumber
% \end{align}
% \normalsize
% We can confirm that $\piopt(a|s)$ is normalized in two different ways.   Using \myprop{advantage}, note that $\psi_{\pr}(s)$ is the appropriate normalization constant for \textcolor{red}{$\pr(a,s) =  r(a,s) + \gamma \transitionv - V(s)$} \RB{Should be $\prpi?$. Is this actually normalized?}.  However, it is more common to treat the optimal regularized policy as a function of the $Q$-values, with $Q(a,s) = r(a,s) + \gamma \transitionv$ and  $\psi_Q(s)$ as the corresponding normalization constant. 
% In \myapp{advantage_pf}, we use similar derivations as \citet{lee2019tsallis} to show that
% \begin{align}
%     \psi_{Q}(s) = V(s) + \psi_{\pr}(s) . \label{eq:q_normalizer} 
% \end{align}
% This identity highlights distinct roles for the policy normalization constant $\psi_Q(s)$ and the value function $V(s)$, which coincide only in the case of the \kl divergence regularization.  
% Indeed, we have argued below \cref{eq:pr_normalizer} that $\psi_{\pr}(s) = 0$ and $\psi_Q(s) = V(s)$ for $\alpha=1$, which does not hold for general $\alpha$ in \cref{eq:q_normalizer}.
% % As discussed in \citet{geist2019theory} and \myapp{soft_value}, the value function for a regularized policy matches the conjugate function $V_{\pi}(s)$


% Finally, we can confirm \myprop{advantage} by plugging either
% the optimal policy \cref{eq:alpha_opt_policy} into the worst-case reward perturbations in \cref{eq:kl_perturbations} or \cref{eq:optimal_perturbations}.

% % the arguments below \cref{eq:pr_normalizer} show that $\psi_{\pr}(s) = 0$ and $\psi_Q(s) = V(s)$, which is not true for general $\alpha$.
% % In the latter case, the discussion below \cref{eq:pr_normalizer} for $\alpha=1$

% % To understand this expression, we can see $\piopt(a|s) \in \Delta^{|\mathcal{A}|}$ using \myprop{advantage}, since $\psi_{\pr(a,s)}(s)$ is the appropriate normalization constant for $\pr(a,s) =  r(a,s) + \gamma \transitionv - V(s)$.  However, it is more common to treat the optimal regularized policy as a function of the $Q$-values, with $Q(a,s) = r(a,s) + \gamma \transitionv$ and  $\psi_Q(s)$ as the corresponding normalization constant.   
% %Using $\psi_Q(s)$ to indicate the normalization constant with respect to the $Q$-values as input,
  
% % Indeed, the expression for $\psi_\pr(s)$ in \cref{eq:pr_normalizer} vanishes for $\alpha =1$ and normalized $\pi_0(a|s)$ and $\pi_\pr(a|s)$, so that $\psi_Q(s) = V(s)$ for \kl divergence regularization.

% % show that this $\piopt(a|s)$ is normalized using similar derivations as \citet{lee2019tsallis}.  

% % Indeed, 
% % when differentiating the Lagrangian in \cref{eq:dual_lagrangian} 
% % % to obtain the dual optimization in \cref{eq:dual_reg}, 
% % we see that the optimal $\mu(a,s)$ satisfies
% % \begin{align}
% %     r(a,s) + \gamma \transitionv - V(s) = \nabla_{\mu}\frac{1}{\beta}\Omega_{\pi_0}(\mu)  \label{eq:opt_policy}
% % \end{align}
% % where $\dualvar(a,s) \leftarrow r(a,s) + \gamma \transitionv - V(s)$ plays the role of the dual variable.   We note the similarity with \myprop{optimal_perturbations}, and 
% % , as in \myprop{optimal_perturbations}.   

% %  We begin by recalling the expression for the optimal policy in a regularized \gls{MDP}, which is obtained by differentiating with respect to $\mu(a,s)$ in \cref{eq:lagrangian}.   
% %  \RB{Does eliminating $\mu(a,s)$ automatically specify the Value function?   In theory (i.e. run the policy for time $\infty$), but possibly not with function approximation...}
 
% %  \RB{Only need Value function for optimal policy}
% % \paragraph{Optimal Policy for KL Divergence}
% %  \paragraph{KL Divergence}
% %  \scriptsize
% % \begin{align}
% % %   \hspace*{-.2cm} \piopt(a|s) = \pi_0(a|s) \, [1+(\alpha-1) \beta \cdot \big( Q(a,s) - \normalizeralpha \big) ]_+^{\frac{1}{\alpha-1}} \label{eq:alpha_opt_policy}
% %   \hspace*{-.2cm} \piopt(a|s) &= \pi_0(a|s) \exp_{\alpha}\bigg\{ \beta \cdot \big( \underbrace{ r(a,s) + \transitionvstar - V_*(s)}_{\Delta r_*(a,s)}- \psi_{\pr}(s) \big) \bigg\}. \label{eq:alpha_opt_policy} \\
% %   \hspace*{-.2cm} \piopt(a|s) &= \pi_0(a|s) \exp_{\alpha}\left\{ \beta \cdot \big( \underbrace{ r(a,s) + \transitionvstar}_{Q_*(a,s)} \underbrace{- V_*(s)- \psi_{\pr}(s)}_{-\psi_Q^{\alpha} = V_*(s)} \big) \right\}. \label{eq:alpha_opt_policy}
% % \end{align}
% % \normalsize

% % \\
% % \textcolor{red}{Check notation of $\normalizeralpha$ over $Q$ values vs. $\Delta r$ as inputs to $\alphaconjmu$}

 
% % For joint $\mu$ regularization,
% %  \scriptsize
% % \begin{align}
% % %   \hspace*{-.2cm} \piopt(a|s) = \pi_0(a|s) \, [1+(\alpha-1) \beta \cdot \big( Q(a,s) - \normalizeralpha \big) ]_+^{\frac{1}{\alpha-1}} \label{eq:alpha_opt_policy}
% %   \hspace*{-.2cm} \mu_*(a,s) = \mu_0(a,s) \exp_{\alpha}\left\{ \beta \cdot \big( r(a,s) + \transitionvstar - V_*(s)- \psi_{\pr} \big) \right\}. \label{eq:alpha_opt_policy}
% % \end{align}
% % \normalsize

% %%%%%%%%%%%%%%%%%%%% HUSAIN MODIFIED REWARD %%%%%%%%%%%%%%%%%%%%%%%%%
% %  \paragraph{Modified Reward Interpretation}
% %  Adapting the dual
% % %  The results of \citet{husain2021regularized}, which apply in a more general setting of arbitrary convex objective functions, match our \myprop{advantage} for the case of regularized \gls{MDP}s.    
% %   While \citet{husain2021regularized} consider a more general setting of arbitrary convex objective functions, their results match our \myprop{advantage} for the case of regularized \gls{MDP}s.
% %   In particular, 
% % instead of expanding the conjugate of the regularization function as in \cref{eq:conjomega2}, \citet{husain2021regularized} consider the convex conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} concave optimization problem $\obj_{\Omega,\beta}(r)$ in \cref{eq:primal_reg}.   This approach yields the modified reward
% % \begin{align}
% % \mropt(a,s) = V_*(s) - \gamma \transitionvstar \, , \label{eq:modified_reward_husain}  %\quad \forall (a,s) \in (\mathcal{A}, \mathcal{S})
% % \end{align}
% % which matches \myprop{advantage} for $\mropt(a,s) = r(a,s) - \proptv(a,s)$.
% % We repeat the derivations of \citet{husain2021regularized} in our notation in \myapp{husain_conjugate}.
% % % We begin by recalling the reward robustness result of \citet{husain2021regularized} in terms of the worst-case modified rewards $\mropt(a,s) = r(a,s) - \propt(a,s)$.   
% % % Instead of expanding the conjugate of the regularization function, \citet{husain2021regularized} consider the conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} concave optimization problem in \cref{eq:primal_reg}.
% % % With detailed derivations in \myapp{husain_conjugate}, th


% % % %  \RB{Optimal POLICY = conjugate applied to optimal Q values}
% % % \paragraph{Modified Reward Interpretation}
% % % We begin by recalling the reward robustness result of \citet{husain2021regularized} in terms of the worst-case modified rewards $\mropt(a,s) = r(a,s) - \propt(a,s)$.   
% % % Instead of expanding the conjugate of the regularization function as in \cref{eq:conjomega2}, \citet{husain2021regularized} consider the conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} concave optimization problem in \cref{eq:primal_reg}.
% % % With detailed derivations in \myapp{husain_conjugate}, this leads to
% % % % We begin by recalling the reward robustness result of \citet{husain2021regularized} in terms of the worst-case modified rewards $\mropt(a,s) = r(a,s) - \propt(a,s)$.   
% % % % Instead of expanding the conjugate of the regularization function, \citet{husain2021regularized} consider the conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} concave optimization problem in \cref{eq:primal_reg}.
% % % % With detailed derivations in \myapp{husain_conjugate}, this leads to 
% % % % % the result
% % % % \begin{restatable}[\citet{husain2021regularized}]{lemma}{husain} 
% % % % % [\textbf{Advantage Function}]
% % % % \label{prop:husain}
% % % % Suppose $(-\obj_{\Omega,\beta}(r))^*$ is increasing and $V_*(s)$ is the optimal solution to 
% % % % For the optimal policy $\pi_*(a|s)$ and any $\alpha$, the worst-case adversarial reward perturbations can be re-expressed as
% % % % \begin{align}
% % % %      \propt(a,s) = Q_{*}(a,s) - V_*(s) \, . \label{eq:advantage}
% % % % \end{align}
% % % % \end{restatable}
% % % % \begin{align}
% % % %   \mropt(a,s) = V_*(s) - \gamma \transitionvstar \, , \label{eq:modified_reward_husain}  %\quad \forall (a,s) \in (\mathcal{A}, \mathcal{S})
% % % % \end{align}
% % % % \JG{I think you can remove this equation and directly talk about \eqref{eq:modified_reward_opt}}
% % % % Adding the environment reward, we can use the worst-case reward perturbations $\propt(a,s) = r(a,s) - \mropt(a,s)$ to rewrite this expression as
% % % \begin{align}
% % % \propt(a,s) &=  r(a,s) + \gamma \transitionvstar -  V_*(s) \label{eq:modified_reward_opt} \, ,
% % % \end{align}
% % % which holds for the optimal value $V_*(s)$ in \cref{eq:dual_reg}.
% % % We can also obtain this result by eliminating $\mu(a,s)$ from the Lagrangian in either \cref{eq:dual_lagrangian} or (\ref{eq:pedro_form}), which are equivalent when $\propt(a,s)= \nabla \omegamu$ as in \mysec{optimal_perturb}.  

% % % % \JG{These two following paragraphs are good. Even better would be to point out more what we are trying to do. E.g. something like: ``Therefore, their result (using the conjugate of entire concave optimization) makes it obvious that the optimal adversarial reward perturbation corresponds to the advantage function. A intriguing question is whether this is also the case when only using the conjugate of the regularizer which is our central tool of analysis)." Or something similar.}
% % % % the approach of \citet{husain2021regularized} and 
% % % From \cref{eq:modified_reward_opt}, we see that the worst-case reward perturbations match the advantage function $\propt(a,s) = r(a,s) + \gamma \transitionvstar -  V_*(s) = Q_{*}(a,s) - V_*(s)$ at optimality. 
% % % % as in  \cref{eq:modified_reward_opt}
% % % However, it is not clear how our expression for $\propt(a,s)$ as a function of $\pi_*(a|s)$ in \cref{eq:optimal_perturbations} would correspond to the advantage function.
% % % % that our expression for $\propt(a,s)$ as a function of $\pi_*(a|s)$ in \cref{eq:optimal_perturbations} corresponds to the advantage function.
% % % % $Q_{*}(a,s) - V_*(s) = r(a,s) + \gamma \transitionvstar -  V_*(s)$ as in  \cref{eq:modified_reward_opt}.  
% % % In \myapp{advantage_pf}, we prove the following proposition from \cref{eq:optimal_perturbations}  directly.
% % % % \paragraph{Relationship to Advantage Function}
% % % \begin{restatable}{proposition}{advantage} 
% % % % [\textbf{Advantage Function}]
% % % \label{prop:advantage} For the optimal policy $\pi_*(a|s)$ and any value of $\alpha$, the worst-case adversarial reward perturbations can be re-expressed as
% % % \begin{align}
% % %      \propt(a,s) = Q_{*}(a,s) - V_*(s) \, . \label{eq:advantage}
% % % \end{align}
% % % \end{restatable}
% % % % \begin{proof}
% % % The proof relies on the following identity (\citet{lee2019tsallis}, \myapp{advantage_pf}), which relates the normalization constant $\normalizeralpha$ of the optimal policy in \cref{eq:alpha_opt_policy}, to the optimal value function $V_*(s)$ in \cref{eq:alpha_conj_norm_main}.
% % % \begin{align}
% % %     \normalizeralpha - V_*(s)=  \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi_*] \label{eq:psidentity} \\
% % %      \textcolor{red}{\psi_{Q}^{\alpha}(s) = V_*(s) + \underbrace{\frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi_*]}_{\psi_{\pr}} }
% % % \end{align}
% % % % Using the optimal policy in \cref{eq:alpha_opt_policy}, we have
% % % % \begin{align}
% % % %     \frac{1}{\beta} \log_{\alpha} \frac{\pi_*(a|s)}{\pi_0(a|s)} = Q(a,s) - \normalizeralpha \, .\label{eq:opt}
% % % % \end{align}
% % % % Combining \cref{eq:psidentity} and \cref{eq:opt}, 
% % % For the optimal policy in \cref{eq:alpha_opt_policy}, we also have $\frac{1}{\beta} \log_{\alpha} \frac{\pi_*(a|s)}{\pi_0(a|s)} = Q_*(a,s) - \normalizeralpha $.   Plugging these into \cref{eq:optimal_perturbations} yields the desired result $\propt(a,s) =Q_*(a,s) - \normalizeralpha +  \normalizeralpha- V_*(s) = Q_*(a,s) - V_*(s)$.  
% % % % From \cref{eq:psidentity}, we can see that $\psi(s;\beta) = V_*(s)$ for the \textsc{kl} divergence at $\alpha =1$.
% % % % $\propt(a,s) &= \frac{1}{\beta} \log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)} + \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi]$ 
% % % % \small 
% % % % \begin{align*}
% % % %     &\propt(a,s) = \frac{1}{\beta} \log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)} + \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi] \\
% % % %     &= Q_*(a,s) - \normalizeralpha +  \normalizeralpha- V_*(s) = Q_*(a,s)- V_*(s)
% % % % \end{align*}
% % % % \normalsize
% % % % \end{proof}

% \subsection{Analysis of the Optimal Policy}
% % \paragraph{Modified Reward Intepretation}
% \textcolor{red}{Our starting point} is Theorem 3 of \citet{husain2021regularized} which, adapted to our setting and notation, expands the regularized dual optimization in \cref{eq:dual_reg} to include a minimization over the modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$

% \begin{restatable}[{Theorem 3 \citep{husain2021regularized}}]{theorem}{husain}
% \label{thm:husain}
% %  \begin{restatable}{proposition}{husain}
% % [\textbf{Advantage Function}]
% The optimal value of the regularized objective $\obj_{\Omega, \beta}(r)$ in \cref{eq:primal_reg}, or its dual $\obj^{*}_{\Omega, \beta}(r)$ in \cref{eq:dual_reg}, 
% is equal to
% \footnotesize
% \begin{align}
%   \hspace*{-.2cm} \inf \limits_{V(s)} &\inf \limits_{\mr(a,s)}   
%     %&
%   (1-\gamma) \blangle \nu_0(s), V(s) \brangle 
%     % \\ & 
%     + \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left( 
%     % \pr(a,s)
%     % \pr(a,s)
%     r(a,s) - \mr(a,s)
%     % r(a,s) + \gamma \transitionvpi - \vpi 
%     \right) \nonumber \\
%     &\text{subj. to  } V(s) \geq \mr(a,s) + \gamma \transitionv \quad
%     \forall (a,s)
%     % \in \mathcal{A} \times \mathcal{S}
%     \label{eq:husain_constrain}
% \end{align}
% \normalsize
% \end{restatable}
% % \begin{proof} 
% % Note that this optimization may be obtained by eliminating $\mu(a,s)$ from the Lagrangian in \cref{eq:pedro_form}.   When the constraint is satisfied with equality, we recover the regularized dual objective in \cref{eq:dual_reg}.
% % We rewrite an alternative proof from \citet{husain2021regularized} using our notation in \myapp{husain_conjugate}.
% % \end{proof}
% % % Note that, instead of expanding the conjugate of the regularization function as in \cref{eq:conjomega2}, \citet{husain2021regularized} consider the convex conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} regularized optimization,
% % % $\obj_{\Omega,\beta}(r)$, which is a concave function of $\mu$ by \cref{eq:primal_reg}.
% % % \footnote{From \cref{eq:primal_reg}, we see that $\obj_{\Omega,\beta}(r)$ is a concave function of $\mu$.}   

% It is insightful to compare \cref{eq:husain_constrain} to the unregularized dual objective in \cref{eq:dual_lp}, which has a constraint involving the unmodified reward function and does not include the adversarial cost $\frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left(r -\mr \right)$.   
% As in \mysec{any_policy}, the adversary incorporates the effect of policy regularization by modifying the reward function, subject to a penalty on $\pr(a,s) = r(a,s) -\mr(a,s)$.
% \citet{husain2021regularized} Lemma 1 shows that the constraint is tight at optimality, with $\mr_{V^*}(a,s) = V^{*}(s) - \gamma \transitionvstar$ and $\pr_{V^*}(a,s)= r(a,s) + \gamma \transitionvstar - V^{*}(s)$ as in \myprop{advantage}.




% % \subsubsection{Equilibrium Properties}
% \subsection{Optimality Conditions}

% % \subsubsection{Conditions on the Optimal Policy}
% % \subsubsection{Nash Equilibrium Conditions}
% % \subsubsection{Properties of the Worst-Case Perturbations for Optimal Policy}
% % \subsubsection{Properties of the Optimal Policy}
% \RB{To further contextualize our adversarial interpretation of the \textit{optimal} policy}

% \input{sections/feasible_fig}

% \paragraph{Path Consistency Condition}
% \vspace*{\header}
% We can further show that the \textit{path consistency} optimality conditions from \citep{nachum2017bridging, chow2018path} 
% are related to the reward perturbation expression in \cref{eq:modified_reward_opt}.  Indeed, by substituting \cref{eq:optimal_perturbations} and (\ref{eq:psidentity}) into \cref{eq:modified_reward_opt}, we obtain
% \small
% \begin{align}
%   \hspace*{-.2cm}  r(a,s) + \gamma \transitionvstar - \frac{1}{\beta} \log_{\alpha}\frac{\pi_*(a|s)}{\pi_0(a|s)} = \normalizeralpha  \, , \label{eq:path}
% \end{align}
% \normalsize
% for all $s \in \mathcal{S}$ and all $a \in \mathcal{A}$ such that $\piopt(a|s) > 0$.
% Note that $\normalizeralpha = V_*(s)$ for \textsc{kl} divergence regularization.

% % We emphasize that 
% This is a natural result, since path consistency is obtained using the \textsc{kkt} conditions and we have seen that $\propt(a,s) = \nabla \omegamu$.
% Path consistency conditions were previously derived for the Shannon entropy \citep{nachum2017bridging} and Tsallis entropy with $\alpha=2$ \citep{chow2018path}, but our expression in \cref{eq:path} provides a generalization to $\alpha$-divergences with arbitrary reference policies.  We provide more detailed discussion in \myapp{path_consistency}.

% % Our expression in \cref{eq:path} generalizes the path consistency conditions, previously derived for the Shannon entropy \citep{nachum2017bridging} and Tsallis entropy with $\alpha=2$ \citep{chow2018path}, to general $\alpha$-divergences and arbitrary reference policies.  We provide more detailed discussion in \myapp{path_consistency}.

% % For the \textsc{kl} divergence regularization, \citet{nachum2017bridging} use the \textsc{kkt} conditions to show that the optimal policy satisfies \textit{path consistency} equations, which follow directly from the adversarial rewards in \cref{eq:modified_reward_opt} using \myprop{perturbations}.   In particular,
% % \begin{align}
% %     r(a,s) - \underbrace{\frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)}}_{\propt(a,s)} = V(s) - \gamma \transitionv 
% %     %\, \, \forall s \in \mathcal{S}, a \in \mathcal{A}
% % \end{align}
% % for all $s \in \mathcal{S}, a \in \mathcal{A}$.
% % \citet{chow2018path} derive a path consistency equation for the Tsallis entropy with $\alpha =2$ which, generalized to the arbitrary $\alpha$-divergences and using our notation, becomes
% % \begin{align}
% % r(a,s) &- \underbrace{\frac{1}{\beta}\log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)} - \frac{1}{\beta}(1-\alpha)D_{\alpha}[\pi_0:\pi]}_{\propt(a,s)} \\
% % &= V(s) - \gamma \transitionv  + \Lambda(s) \label{eq:path1}
% % \end{align}
% % where $\Lambda(s) = \normalizerexp - V(s)$.   Using \eqref{eq:psidentity}, we can see that this Lagrange multiplier is equal to $\normalizerexp - V(s)= - \frac{1}{\beta}(1-\alpha)D_{\alpha}[\pi_0:\pi]$, so that we finally obtain
% % % is a Lagrange multiplier which can be seen as accounting for the fact that $\normalizerexp \neq V(s)$ for $\alpha \neq 1$.
% % % Finally, we are left with
% % \begin{align}
% %     r(a,s) + \gamma \transitionv - \propt(a,s) = \normalizeralpha   \label{eq:path}
% % \end{align}
% % \RB{Will change to reflect $\pr(a,s) = Q(a,s) - V(s)$}
% % which matches our condition $\pr(a,s) = Q(a,s) - \normalizeralpha$. 
% % With detailed derivations in \cref{app:path_consistency}, we show that the optimal $\alpha$-divergence regularized policy satisfies the path consistency condition in \cref{eq:path1}, which generalizes the result of \citet{chow2018path} from $\alpha=2$ to general $\alpha$.

% \paragraph{Indifference Condition} 
% As \citet{ortega2014adversarial} discuss for the single step case, the saddle point of the minmax optimization in \cref{eq:pedro_form} reflects an \textit{indifference} which is a well-known property of Nash equilibria in game theory \citep{osborne1994course}.  In particular, for the optimal policy and corresponding worst-case reward perturbations, 
% % we confirm in \myapp{indifference} that the modified reward $r\tick(a,s)$
% we confirm using \cref{eq:advantage} that the pointwise objective $r(a,s) + \transitionvstar - \propt(a,s) = V_*(s)$ equals a constant across all actions $a \in \mathcal{A}$ in 
% % $a \in \mathcal{A}$ 
% a particular state.  
% % value across all actions $a \in \mathcal{A}$ for a particular state.  
% % \RB{Is this the expression we should write for the multi-step case?   Haven't stated that $\omegamu = 0$ yet in \cref{eq:pedro_form})}
% The value  $V_*(s)$  is also known as the \textit{certainty equivalent} \citep{fishburn1988nonlinear, ortega2013thermodynamics}, 
% which measures the payoff of a two-player game where the agent begins in state $s \in \mathcal{S}$ and plays against an adversary defined by the regularizer $\Omega$ with strength $\beta$.
% We confirm this indifference condition empirically in \cref{fig:perturb_opt} and \cref{fig:pyco_indifference}. 




\input{sections/new/2a_optimal_value}

==> Reward Robustness TMLR (3)/sections/new/2a_optimal_value.tex <==
\headerv
\subsection{Worst-Case Perturbations: Value Form}
% \subsection{Analysis for the Optimal Policy}
% \subsection{Worst-Case Reward Perturbations: Optimal Policy}
% \subsection{Worst-Case $\proptv(a,s)$: Optimal Policy}
\label{sec:value_form}

% In the previous section, we analyzed the implicit adversary corresponding to \textit{any} stochastic policy $\pi(a|s)$ for a given  $\Omega, \pi_0,$ and $\beta$. We now take a dual perspective, where the adversary is given access to a set of dual variables $V(s)$ across states $s \in \mathcal{S}$.   Although this leads to an alternative definition of the reward perturbations $\prv$ and modified rewards $\mrv$, we will see in \mysec{optimal_policy} that these notions match the policy form $\prpi$ for the optimal policy $\pi_*$ and value function $V_*$.   


In the previous section, we analyzed the implicit adversary corresponding to \textit{any} stochastic policy $\pi(a|s)$ for a given  $\Omega, \pi_0,$ and $\beta$. We now take a dual perspective, where the adversary is given access to a set of dual variables $V(s)$ across states $s \in \mathcal{S}$ and selects reward perturbations $\prv(a,s)$.    We will eventually show in \mysec{optimal_policy} that these perturbations match the policy-form perturbations at optimality.
% from the previous section.

% Our starting point is Theorem 3 of \citet{husain2021regularized} which, adapted to our notation in \myapp{husain_conjugate}, 
% % can be viewed as incorporating 
% incorporates
% an optimization over adversarial reward perturbations $\prv(a,s)$
% % modified reward $\mrv(a,s) = r(a,s) - \prv(a,s)$ 
% into the regularized Lagrangian (\cref{eq:dual_lagrangian}). 
Our starting point is Theorem 3 of \citet{husain2021regularized}, which arises from taking the convex conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} regularized objective $\obj_{\Omega,\beta}(r)$, which is concave in $\mu(a,s)$.  See \myapp{husain}.
% instead of the only .
\begin{restatable}[{\citet{husain2021regularized}}]{theorem}{husain}
\label{thm:husain}
%  \begin{restatable}{proposition}{husain}
% [\textbf{Advantage Function}]
The optimal value of the regularized objective $\obj_{\Omega, \beta}(r)$ in \cref{eq:primal_reg}, or its dual $\obj^{*}_{\Omega, \beta}(r)$ in \cref{eq:dual_reg}, 
is equal to
\ifx\omitindices\undefined
\begin{align}
% \vspace*{-.1cm}
   \hspace*{-.3cm} \inf \limits_{V(s), \lambdaplus} \inf \limits_{\textcolor{\highlight}{\prv(a,s)}}   
    %&
   & (1-\gamma) \blangle \nu_0(s), V(s) \brangle 
    % \\ & 
    + \frac{1}{\beta} \Omega^{*(\alpha)}_{\pi_0,\beta}\left( 
    % \pr(a,s)
    \textcolor{\highlight}{\prv}
    % r - \mrv
    % r(a,s) - \mrv(a,s)
    % r(a,s) + \gamma \transitionvpi - \vpi 
    \right)  \quad
    \label{eq:husain_constrain} \\
    % \nonumber \\
    \text{subject to }\quad
    V(s) &= r(a,s) + \gamma \transitionv - \textcolor{\highlight}{\prv(a,s)} + \lambdaplus \quad \forall (a,s) \in \mathcal{A} \times \mathcal{S}.
    % V(s) \geq \mrv(a,s) + \gamma \transitionv \quad
    % \forall (a,s)
    % \in \mathcal{A} \times \mathcal{S}
    \nonumber
    % \label{eq:husain_constrain}
\end{align}
\else
\begin{align}
% \vspace*{-.1cm}
   \hspace*{-.3cm} \inf \limits_{V, \lambda} \inf \limits_{\textcolor{\highlight}{\prv}}   
    %&
   \, & \, (1-\gamma) \blangle \nu_0, V \brangle 
    % \\ & 
    + \frac{1}{\beta} \Omega^{*(\alpha)}_{\pi_0,\beta}\left( 
    % \pr(a,s)
    \textcolor{\highlight}{\prv}
    % r - \mrv
    % r(a,s) - \mrv(a,s)
    % r(a,s) + \gamma \transitionvpi - \vpi 
    \right)  
    \quad
    \label{eq:husain_constrain} \\
    % \nonumber \\
    \text{subject to }\,\,\,
    V(s) &= r(a,s) + \gamma \transitionv - \textcolor{\highlight}{\prv(a,s)} + \lambdaplus \quad \forall (a,s) \in \mathcal{A} \times \mathcal{S}.
    % V(s) \geq \mrv(a,s) + \gamma \transitionv \quad
    % \forall (a,s)
    % \in \mathcal{A} \times \mathcal{S}
    \nonumber
    % \label{eq:husain_constrain}
\end{align}
\fi

\normalsize
% \scriptsize
% \begin{align}
%   \hspace*{-.2cm} &\inf \limits_{V(s), \lambdaplus} \inf \limits_{\mrv(a,s)}   
%     %&
%   (1-\gamma) \blangle \nu_0(s), V(s) \brangle 
%     % \\ & 
%     + \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left( 
%     % \pr(a,s)
%     % \pr(a,s)
%     r - \mrv
%     % r(a,s) - \mrv(a,s)
%     % r(a,s) + \gamma \transitionvpi - \vpi 
%     \right) \nonumber \\
%     &\text{subj. to  } 
%     V(s) = \mrv(a,s) + \gamma \transitionv + \lambdaplus \,\,.
%     % V(s) \geq \mrv(a,s) + \gamma \transitionv \quad
%     % \forall (a,s)
%     % \in \mathcal{A} \times \mathcal{S}
%     \label{eq:husain_constrain}
% \end{align}
% \normalsize
\end{restatable}
% See \myapp{husain_conjugate} for proof.   
Rearranging the equality constraint to solve for $\prv(a,s)$ and substituting into the objective, this optimization recovers the regularized dual problem in \cref{eq:dual_reg}.   
We can also compare \cref{eq:husain_constrain} to the \textit{unregularized} dual problem in \cref{eq:dual_lp}, which does not include an adversarial cost and whose constraint 
$V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$ implies an \textit{unmodified} reward, or $\prv(a,s) = 0$. 
Similarly to \mysec{any_policy}, the adversary incorporates the effect of policy regularization via the reward perturbations $\prv(a,s)$.
%in \cref{eq:husain_constrain}.    
% See \myapp{husain_conjugate}.
% Substituting the equality constraint for $\prv(a,s)$ into the objective, we see that this optimization recovers the regularized dual problem in \cref{eq:dual_reg}.   See \myapp{husain_conjugate}.   
% \begin{proof} 
%  See \myapp{husain_conjugate} for proof.   Note that this optimization may be obtained by eliminating $\mu(a,s)$ from the Lagrangian in \cref{eq:pedro_form}.   
% For a fixed, possibly suboptimal set of dual variables $V(s)$, it can be shown that the constraint is tight, with $\mrv(a,s) = V(s) - \transitionv$ (\citet{husain2021regularized}, \myapp{husain_conjugate}).
% Using this expression to eliminate $\mrv(a,s)$ in \cref{eq:husain_constrain}, we are left with the regularized dual objective in \cref{eq:dual_reg}.   
% % although the constraint is tight $\mrv(a,s) = V(s) - \transitionv$ for a fixed, suboptimal set of dual variables \citep{husain2021regularized}
% % When the constraint is satisfied with equality, we recover the regularized dual objective in \cref{eq:dual_reg}.
% % We rewrite an alternative proof from \citet{husain2021regularized} using our notation in \myapp{husain_conjugate}.
% \end{proof}
% % % Note that, instead of expanding the conjugate of the regularization function as in \cref{eq:conjomega2}, \citet{husain2021regularized} consider the convex conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} regularized optimization,
% % % $\obj_{\Omega,\beta}(r)$, which is a concave function of $\mu$ by \cref{eq:primal_reg}.
% % % \footnote{From \cref{eq:primal_reg}, we see that $\obj_{\Omega,\beta}(r)$ is a concave function of $\mu$.}   
% % We provide a proof in \myapp{app:husain_conjugate}, and note that this optimization may be obtained by eliminating $\mu(a,s)$ from the Lagrangian in \cref{eq:pedro_form}.  

% However, although the constraint is tight $\mrv(a,s) = V(s) - \transitionv$ for a fixed, suboptimal set of dual variables \citep{husain2021regularized}, we have 

% , and note that this optimization may be obtained by eliminating $\mu(a,s)$ from the Lagrangian in \cref{eq:pedro_form}.
% It is insightful to compare \cref{eq:husain_constrain} to the \textit{unregularized} dual in \cref{eq:dual_lp}, where
% the objective does not include the adversarial cost $\frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left(\prv \right)$  
% and the constraint $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$ 
% corresponds to an unmodified reward function $\prv(a,s)=0$.
% \paragraph{Comparison with Unregularized Case} 
% It is insightful to compare \cref{eq:husain_constrain} to the \textit{unregularized} dual in \cref{eq:dual_lp}, where
% the objective does not include the adversarial cost and the
% constraint $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$ 
% corresponds to an unmodified reward function $\prv(a,s)=0$.   
% Similarly to \mysec{any_policy}, the adversary incorporates the effect of policy regularization via the 
% reward perturbations 
% % dual variables
% $\prv(a,s)$.    
% Although the regularized policy is generally stochastic, the Lagrange multipliers $\lambdaplus$ may additionally force action probabilities to be zero.



% as dual variables.
% , subject to a penalty on the perturbation $\prv = r-\mrv$.
% The reward perturbations arising from regularization also affect the value constraint, where \cref{eq:husain_constrain} contains an additional $\prv$ term compared with the unregularized constraint $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$.   In this sense, the 


% to highlight the role of $\prv(a,s)$ as a dual variable,


% It is also insightful to compare \cref{eq:husain_constrain} to the \textit{unregularized} dual objective in \cref{eq:dual_lp}, which has a constraint involving the unmodified reward function $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$ and does not include the adversarial cost $\frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left(r -\mrv \right)$.   Similarly to \mysec{any_policy}, the adversary incorporates the effect of policy regularization by modifying the reward function, subject to a penalty on the perturbation $\prv = r-\mrv$.

% $\pr(a,s) = r(a,s) -\mr(a,s)$.



% \paragraph{Comparison with Unregularized Case} 
% It is insightful to compare \mythm{husain} with the \textit{unregularized} dual objective in \cref{eq:dual_lp} to highlight the distinct roles of the Lagrange multipliers $\lambdaplus$ and reward perturbations $\pr(a,s)$.
% The unregularized objective does not include an adversarial cost, and the constraint $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$ corresponds to an \textit{unmodified} reward, $\prv(a,s)=0$.   


% In particular, $\lambdaplus = V(s) - r(a,s) - \gamma \transitionv \geq 0 $ equals the negative advantage function and sets action probabilities to zero in the 
% % deterministic 
% optimal policy $\piopt(a|s) = \text{uniform}(\argmax_a r(a,s) + \gamma \transitionvstar )$.  


% % It is insightful to compare \mythm{husain} with the \textit{unregularized} dual objective in \cref{eq:dual_lp}.  
% It is insightful to compare \mythm{husain} with the \textit{unregularized} dual objective in \cref{eq:dual_lp} to highlight the distinct roles of the Lagrange multipliers $\lambdaplus$ and reward perturbations $\pr(a,s)$.
% The unregularized objective does not include an adversarial cost, and the constraint $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$ corresponds to an \textit{unmodified} reward, $\prv(a,s)=0$.   In particular, $\lambdaplus = V(s) - r(a,s) - \gamma \transitionv \geq 0 $ equals the (negative) advantage function and sets action probabilities to zero in the 
% % deterministic 
% optimal policy.  
% % when $\lambdaplus > 0$ 
% % when $Q(a,s) < \arg\max_{a\tick} Q(a\tick,s)$. 
% % sets action probabilities to zero in the deterministic optimal policy.
% % At optimality, we use \myprop{advantage} to confirm that $\lambdaplus = V_*(s) - Q_*(a,s)$ reflects the advantage function and $\prpiopt(a,s)=0$.


% Similarly to \mysec{any_policy}, 
% the adversary in \cref{eq:husain_constrain} incorporates the effect of policy regularization via the reward perturbations $\prv(a,s)$.  
% We will show below that $\prv(a,s)$ rather than $\lambdaplus$ reflects the advantage function in the regularized case, and further compare the role of $\lambdaplus$ and $\pr(a,s)$ in an example in \mysec{visualizations_worst_case}.
% In the next subsection, we show that $\prv(a,s)$ rather than $\lambdaplus$ matches the advantage function in the regularized case. We further discuss the role of $\lambdaplus$ and $\pr(a,s)$ in an example in \mysec{visualizations_worst_case}.

% In contrast to the unregularized case, we will show in the next subsection that $\prv(a,s)$ matches the advantage function for actions with nonzero probability ($\lambdaplus=0$) under the optimal regularized policy.


% In \myprop{advantage} below, we will see that $\prv(a,s)$ matches the advantage function for actions with nonzero probability in the optimal policy ($\lambdaplus=0$)
% In \myprop{advantage} below, we will see that $\prv(a,s)$ matches the advantage function for actions with nonzero probability in the optimal policy ($\lambdaplus=0$).  
% Depending on the regularization parameters $\alpha$ and $\beta$, the Lagrange multipliers $\lambdaplus$ may additionally force some action probabilities to zero due to the cutoff behavior of $\exp_{\alpha}$ (see \cref{eq:qexp} and (\ref{eq:optimal_policy}), \citet{lee2018sparse, lee2019tsallis}).
% We compare the role of $\lambdaplus$ and $\pr(a,s)$ in an example in \mysec{visualizations_worst_case}.

% Depending on the regularization parameters $\alpha$ and $\beta$, Lagrange multipliers with $\lambdaplus > 0$ may additionally force some action probabilities to zero due to the cutoff behavior of $\exp_{\alpha}$ (see \cref{eq:qexp} and (\ref{eq:optimal_policy}), \citet{lee2018sparse, lee2019tsallis}).
% We compare the role of $\lambdaplus$ and $\pr(a,s)$ in an example in \mysec{visualizations_worst_case}.



% The optimal regularized policy is stochastic in general, which implies that $\prv(a,s)$ matches the advantage function when $\piopt(a|s)=0$.
% Depending on the regularization parameters $\alpha$ and $\beta$, Lagrange multipliers with $\lambdaplus > 0$ may additionally force some action probabilities to zero due to the cutoff behavior of $\exp_{\alpha}$ (see \cref{eq:qexp} and (\ref{eq:optimal_policy}), \citet{lee2018sparse, lee2019tsallis}).
% We compare the role of $\lambdaplus$ and $\pr(a,s)$ in an example in \mysec{visualizations_worst_case}.


% For actions with nonzero probability in the optimal policy, $\lambdaplus=0$ implies that $\prv(a,s)$ reflects the advantage function.
% % In this case, \myprop{advantage} suggests that the reward perturbations reflect the advantage function.
% Although the optimal regularized policy is stochastic in general, the Lagrange multipliers $\lambdaplus > 0$ may, depending on the regularization parameters $\alpha$ and $\beta$, additionally force some action probabilities to zero due to the cutoff behavior of $\exp_{\alpha}$ (see \cref{eq:qexp} and (\ref{eq:optimal_policy}), \citet{lee2018sparse, lee2019tsallis}).
% We compare the role of $\lambdaplus$ and $\pr(a,s)$ in an example in \mysec{visualizations_worst_case}.
% % $\prv(a,s)=0$.   

% \headerv
\subsection{Policy Form $=$ Value Form at Optimality}\label{sec:optimal_policy}
% \headerv
In the following proposition, we provide a link between the policy and value forms of the adversarial reward perturbations, showing that $\proptpi(a,s)=\proptv(a,s)$ for the optimal policy $\piopt(a|s)$ and value $V_*(s)$.
%for a given \gls{MDP} and regularization scheme.
% For the optimal policy $\piopt(a|s)$ and value $V_*(s)$, we show in the following proposition that the policy and value forms of the adversarial reward perturbations are equal, with $\proptpi(a,s)=\proptv(a,s)$.
% In the following proposition that the policy and value forms of the adversarial reward perturbations match, $\proptv = \proptpi$, at optimality in a regularized \gls{MDP}.
% Only at optimality in the regularized \gls{MDP}
% However, as we show in the following proposition, the adversarial reward perturbations associated with a value function $V(s)$ (\mysec{value_form}) and policy $\pi(a|s)$ (\mysec{any_policy}) align \textcolor{red}{only at optimality} in the regularized \gls{MDP}, with $\proptv = \proptpi$. 
% form for the adversarial reward perturbations only matches the policy form in \mysec{any_policy} at optimality in the regularized \gls{MDP}, with $\proptv = \proptpi$.
% \citet{husain2021regularized} Lemma 1 shows that the constraint is tight at optimality, with $\mr_{V^*}(a,s) = V^{*}(s) - \gamma \transitionvstar$ and $\pr_{V^*}(a,s)= r(a,s) + \gamma \transitionvstar - V^{*}(s)$ as in \myprop{advantage}.
% now analyse the adversarial reward perturbations associated with the \textit{optimal} policy $\pi_*(a|s)$ for a given regularized \gls{MDP}.   
% In the following proposition, we relate the policy and value forms of the adversarial reward perturbations for the optimal policy and value function.
% using the \textsc{kkt} conditions.
% For a given \gls{MDP} and regularization scheme, 
% As is the focus of discussion 
As in \citet{eysenbach2021maximum}, the uniqueness of the optimal policy 
% $\piopt(a|s)$ 
implies that its robustness may be associated with an environmental reward $r(a,s)$ for a given
regularized \gls{MDP}.
% environmental reward $r(a,s)$, 
% Further, as in \citet{eysenbach2021maximum}, the uniqueness of the optimal policy $\piopt(a|s)$ for a fixed \gls{MDP} and regularization scheme implies that its robustness may be associated with a given environmental reward $r(a,s)$.
% and regularization scheme.
% Further, as is the focus of discussion in \citet{eysenbach2021maximum}, the uniqueness of the optimal policy $\piopt$ for a given \gls{MDP} allows us to associate its robustness with a given environmental reward $r(a,s)$.
 \begin{restatable}{proposition}{advantage} 
% [\textbf{Advantage Function}]
\label{prop:advantage} For the optimal policy $\pi_*(a|s)$ and value function $V_*(s)$ corresponding to $\alpha$-divergence policy regularization with strength $\beta$, 
% any $\alpha$,
the policy and value forms of the worst-case adversarial reward perturbations match, $\proptpi=\proptv$, and are related to the advantage function via
% the worst-case policy-form of the adversarial reward perturbations is related to the {advantage function}
% can be expressed as
% \small
% \begin{align}
%     % \proptv(a,s) &= Q_{*}(a,s) - V_*(s) \, .  \\
% \hspace*{-.2cm}
% \proptpi(a,s)
% % = \proptv(a,s) 
% &= r(a,s) + \gamma \transitionvstar - V_*(s) + \lambdaplus \label{eq:advantage}
% \end{align}
\normalsize
\begin{align}
    % \proptv(a,s) &= Q_{*}(a,s) - V_*(s) \, .  \\
\hspace*{-.2cm}
\proptpi(a,s)
% = \proptv(a,s) 
&= Q_*(a,s) - V_*(s) + \lambdaopt ,\label{eq:advantage}
\end{align}
where we define $Q_*(a,s) \coloneqq r(a,s) + \gamma \transitionvstar$ and recall $\lambdaopt \pi_*(a|s) = 0$ by complementary slackness.
Note that $V_*(s)$ depends on the regularization scheme via the conjugate function $\alphaconj(\prv)$ in \cref{eq:husain_constrain}.   
% Note that \cref{eq:advantage} omits the dependence of the optimal value function $V_*(s)$ on the regularization scheme, via the conjugate function $\alphaconj(\prv)$ in \cref{eq:husain_constrain}.   
% Note, our notation omits the dependence of optimal value $V_*(s)$ on $\beta$ and $\alpha$ via the conjugate $\alphaconj(\prv)$ in \cref{eq:husain_constrain}.    
% as in \cref{eq:husain_constrain}.
\end{restatable}
\normalsize
%  \RB{Proof is the same as Modified Reward Dual}
%  Differentiating \cref{eq:pedro_form} with respect to $\mu(a,s)$, we obtain the optimality condition that $\pr(a,s) = r(a,s) + \gamma \transitionv - V(s)$.    Plugging this expression back into \cref{eq:pedro_form}, we obtain the regularized dual objective \cref{eq:dual_reg}.
%  \end{proof}
%   Also, as a sanity check, we know that we can induce $\mu(a,s) \in \mathcal{M}$ from any $\pi(a|s)$ by running .}
% %  We emphasize that the worst-case perturbations in the previous section apply for arbitrary policies, whereas the analysis in this section relies on first solving for the optimal policy according to \cref{eq:primal_reg}.
% In the previous section, we analyzed the implicit adversary corresponding to \textit{any} stochastic policy $\pi(a|s)$ for a given  $\Omega, \pi_0,$ and $\beta$.
% We now take a dual perspective, where the adversary is given access to 
% \textcolor{red}{the value function $V_{\pi}(s)$ of the agent }
% in each state, and the value is calculated with respect to a particular regularized objective (\citet{geist2019theory} Def. 2).
% (\textcolor{red}{see \myapp{soft_value}}).
% % \paragraph{Modified Reward Intepretation}
% Our starting point is Theorem 3 of \citet{husain2021regularized} which, adapted to our setting and notation, expands the regularized dual optimization in \cref{eq:dual_reg} to include a minimization over the modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$
% \begin{restatable}[{Theorem 3 \citep{husain2021regularized}}]{theorem}{husain}
% \label{thm:husain}
% %  \begin{restatable}{proposition}{husain}
% % [\textbf{Advantage Function}]
% The optimal value of the regularized objective $\obj_{\Omega, \beta}(r)$ in \cref{eq:primal_reg}, or its dual $\obj^{*}_{\Omega, \beta}(r)$ in \cref{eq:dual_reg}, 
% is equal to
% \footnotesize
% \begin{align}
%   \hspace*{-.2cm} \inf \limits_{V(s)} &\inf \limits_{\mr(a,s)}   
%     %&
%   (1-\gamma) \blangle \nu_0(s), V(s) \brangle 
%     % \\ & 
%     + \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left( 
%     % \pr(a,s)
%     % \pr(a,s)
%     r(a,s) - \mr(a,s)
%     % r(a,s) + \gamma \transitionvpi - \vpi 
%     \right) \nonumber \\
%     &\text{subj. to  } V(s) \geq \mr(a,s) + \gamma \transitionv \quad
%     \forall (a,s)
%     % \in \mathcal{A} \times \mathcal{S}
%     \label{eq:husain_constrain}
% \end{align}
% \normalsize
% \end{restatable}
% \begin{proof} 
% Note that this optimization may be obtained by eliminating $\mu(a,s)$ from the Lagrangian in \cref{eq:pedro_form}.   When the constraint is satisfied with equality, we recover the regularized dual objective in \cref{eq:dual_reg}.
% We rewrite an alternative proof from \citet{husain2021regularized} using our notation in \myapp{husain_conjugate}.
% \end{proof}
% % Note that, instead of expanding the conjugate of the regularization function as in \cref{eq:conjomega2}, \citet{husain2021regularized} consider the convex conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} regularized optimization,
% % $\obj_{\Omega,\beta}(r)$, which is a concave function of $\mu$ by \cref{eq:primal_reg}.
% % \footnote{From \cref{eq:primal_reg}, we see that $\obj_{\Omega,\beta}(r)$ is a concave function of $\mu$.}   
% It is insightful to compare \cref{eq:husain_constrain} to the unregularized dual objective in \cref{eq:dual_lp}, which has a constraint involving the unmodified reward function and does not include the adversarial cost $\frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left(r -\mr \right)$.   
% As in \mysec{any_policy}, the adversary incorporates the effect of policy regularization by modifying the reward function, subject to a penalty on $\pr(a,s) = r(a,s) -\mr(a,s)$.
%%% OPTIMAL POLICY section intro
%  \RB{No longer focusing on optimal}  Our derivations so far have only invoked the conjugate representation of the regularization function, which suggests that \textit{any} stochastic policy may be interpreted via an adversarial game for given $\Omega, \pi_0,$ and $\beta$.    We now analyse the adversarial reward perturbations associated with the \textit{optimal} policy $\pi_*(a|s)$ for a given regularized \gls{MDP}.   
%  The uniqueness of the optimal policy allows us to associate its robustness with a given environment reward function, which is the focus of discussion in \citet{eysenbach2021maximum}.  
% % Note that these statements rely on our ability to solve for the optimal policy in \cref{eq:primal_reg}.
% %  We emphasize that the worst-case perturbations in the previous section apply for arbitrary policies, whereas the analysis in this section relies on first solving for the optimal policy according to \cref{eq:primal_reg}.
% %   \textcolor{red}{While we are able to obtain additional insight for the optimal policy, this comes at the cost of having to solve for the unique optimal policy in \cref{eq:primal_reg}. }
% %  which is defined via a reward function $r(a,s)$ in a given (regularized) \gls{MDP}. 
% %  We will see that we can make stronger statements for the conjugate expansion of the optimal policy $\pi_*(a|s)$, which comes at the cost of having to solve for the optimal policy in \cref{eq:primal_reg}. 
% % We will see that we can make stronger statements in this case, albeit at the cost of having to solve for the unique optimal policy in \cref{eq:primal_reg}. 
% %  Note that 
% % For a given regularization scheme and the unique optimal policy $\pi_*(a|s)$, 
% % we can frame our analysis in terms of robustness associated 
% %  Note that this allows us to frame the analysis in terms of the robustness associated with a given reward function and regularization scheme, rather than a particular policy \citep{eysenbach2021maximum}.
% % Note that the uniqueness of the optimal policy $\pi_*(a|s)$ for a chosen regularization scheme allows us to associate its robustness with a given reward function and \gls{MDP}, as in \citet{eysenbach2021maximum}.
%  \paragraph{Optimal Policy}
% We first consider the form of the optimal policy in a regularized \gls{MDP}, which corresponds to the conjugate optimality condition $\primalvar(a,s) = (\nabla \Omega)^{-1}\big(\pr(a,s) \big)$ in \mysec{conj_intro} and \mytab{conj_table}.   For policy regularization using the $\alpha$-divergence, we obtain
 \begin{proof}
See \myapp{advantage_pf}.  We consider the optimal policy in an \gls{MDP} with $\alpha$-divergence policy regularization $\frac{1}{\beta}\Omega^{(\alpha)}_{\pi_0}(\mu)$, which is derived via similar derivations as \citet{lee2019tsallis} or by eliminating $\mu(a,s)$ in \cref{eq:dual_lagrangian}.
% \scriptsize
%   \begin{minipage}{\linewidth}
%   \begin{equation}\label{eq:alpha_opt_policy} 
%   \begin{aligned}
\small
\begin{align}
      &\piopt(a|s)=  
        %   \resizebox{1.0\linewidth}{!}{ 
          \, \pi_0(a|s) \exp_{\alpha}\big\{ \beta \cdot \big( 
    %   \underbrace{ 
    %   r(a,s) + \gamma \transitionvstar
    Q_*(a,s)
    %   \nonumber \\
    %   & \phantom{= \pi_0(a|s) \exp_{\alpha}\bigg\{} 
      - V_*(s) + \lambdaplus
    %   }_{\Delta r_*(a,s)}
      - \psipropt  \big) \big\}. \label{eq:optimal_policy} 
        %  }
        %  \end{aligned}
\end{align}
% \begin{align}
% \hspace*{-.2cm} 
% \resizebox{.9\columnwidth}{!}{
%          $\piopt(a|s)=  \pi_0(a|s) \exp_{\alpha}\big\{ \beta \cdot \big( 
%     %   \underbrace{ 
%     %   r(a,s) + \gamma \transitionvstar
%       Q_*(a,s) 
%     %   \nonumber \\
%     %   & \phantom{= \pi_0(a|s) \exp_{\alpha}\bigg\{} 
%       - V_*(s)
%     %   }_{\Delta r_*(a,s)}
%         + \lambdaplus - \psipropt \big) \big\}. 
%         $ } \label{eq:optimal_policy}  
%         %  \end{aligned}
% \end{align}
\normalsize
% \RB{REDO This?  }
% Clarify role of $\psi_{\propt}(s;\beta)$ as not being specific to $\pr$ and rather being the normalizer for any $\pi$.}
% Note that $\psi_{\propt}(s)$ appears from differentiating $\nabla_{\mu}\Omega(\mu)$ as in \myprop{optimal_perturbations} and \cref{eq:}
We prove \myprop{advantage} by plugging 
this optimal policy into the worst-case reward perturbations from \cref{eq:optimal_perturbations}, $\proptpi(a,s) = \frac{1}{\beta}\log_{\alpha}\frac{\piopt(a|s)}{\pi_0(a|s)} + \psipropt$.
We can also use \cref{eq:advantage} to verify 
% $\piopt(a|s) \in \Delta^{|\mathcal{A}|}$ 
$\piopt(a|s)$ is normalized,
since 
$\psi_{\pr_{\piopt}}$
% $\psipropt$ 
% is the normalization constant for 
% appropriate 
% correct
ensures normalization for
the policy corresponding to $\prpiopt$.
% $\pi_{\propt}(a|s)$.   
% Equivalently, using \cref{eq:soft_value}, we can relate 
In \myapp{advantage_confirm}, we also show $\psiqopt = V_*(s) + \psipropt$, where $\psiqopt$ is a Lagrange multiplier enforcing normalization in \cref{eq:soft_value}.
% However, using $Q(a,s) \coloneqq  r(a,s) + \gamma \transitionv$, it is also common to consider the regularized Bellman optimality operator 
\end{proof}

% \paragraph{Comparison to the Unregularized Case}
% It is insightful to compare \mythm{husain} and \myprop{advantage} to the \textit{unregularized} dual objective in \cref{eq:dual_lp}.   The unregularized objective does not include an adversarial cost, and the constraint $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$ corresponds to an \textit{unmodified} reward, or $\prv(a,s)=0$.
% At optimality, 

% $\lambdaplus =  V_*(s) - Q_*(a,s) = 0$
 
 
%  $\lambdaplus =  V_*(s) - Q_*(a,s) > 0$ for actions with zero probability under the deterministic unregularized policy, whereas $V_*(s) = Q_*(a_\text{max}, s)$ and $\lambda(a_{\text{max}}, s) = 0$ for $a_{\text{max}} = \arg\max_a Q_*(a,s)$.}
%%%%%%%%% THIS REASONING MADE ME OMIT THIS DETAILED COMPARISON %%%%%%%
% \paragraph{Comparison to the Unregularized Case}
% To highlight the distinct roles of the Lagrange multipliers $\lambdaplus$ and reward perturbations $\pr(a,s)$, we compare  \mythm{husain} and \myprop{advantage} to the \textit{unregularized} dual objective in \cref{eq:dual_lp}.   The unregularized objective does not include an adversarial cost, and the constraint $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$ corresponds to an \textit{unmodified} reward or $\prv(a,s)=0$.    For the optimal values, we see that $\lambdaplus = V_*(s) - Q_*(a,s)$ is equal to the negative advantage function and the optimal policy places nonzero probability ($\lambdaplus=0$) only on actions with $Q_*(a,s) = V_*(s) \coloneqq \max_{a\tick} Q_*(a\tick,s)$.

%  By contrast, in the regularized case, \myprop{advantage} shows that $\pr_{V_*}(a,s)$ is equal to the advantage function for actions with nonzero probability 
% under the stochastic optimal policy.   Depending on the regularization parameters $\alpha$ and $\beta$, the Lagrange multipliers $\lambdaplus$ may
% % additionally 
% force some action probabilities to zero via the cutoff behavior of $\exp_{\alpha}$ in \cref{eq:optimal_policy} (see \cref{eq:qexp}, \citet{lee2018sparse, lee2019tsallis}).  
% % We compare the role of $\lambdaplus$ and $\pr(a,s)$ in an example in \mysec{visualizations_worst_case}.
 
 
%%%%%%%%% PREVIOUS %%%%%%%%
% It is insightful to compare \mythm{husain} with the \textit{unregularized} dual objective in \cref{eq:dual_lp} to highlight the distinct roles of the Lagrange multipliers $\lambdaplus$ and reward perturbations $\pr(a,s)$.
% The unregularized objective does not include an adversarial cost, and the constraint $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$ corresponds to an \textit{unmodified} reward, $\prv(a,s)=0$.   At optimality, we use \myprop{advantage} to confirm that $\lambdaplus = V_*(s) - Q_*(a,s)$ reflects the advantage function and $\prpiopt(a,s)=0$.
% Further,
% the constraint $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$ 
% corresponds to an \textit{unmodified} reward function and $\prpi(a,s) = 0$.   
% \textcolor{red}{
% % To confirm this using \myprop{advantage}, 
% To confirm this using \myprop{advantage},
% note that $\lambdaplus =  V_*(s) - Q_*(a,s) > 0$ for actions with zero probability under the deterministic unregularized policy, whereas $V_*(s) = Q_*(a_\text{max}, s)$ and $\lambda(a_{\text{max}}, s) = 0$ for $a_{\text{max}} = \arg\max_a Q_*(a,s)$.}


% We consider an example in \mysec{visualizations_worst_case}.
% \textcolor{red}{To confirm this using \myprop{advantage}, note that the optimal policy is deterministic 
% % with 
% % deterministically selects $a_{\text{max}}$, with
% $\pi_*(a_{\text{max}}|s) = 1$, provided $a_{\text{max}} \coloneqq \arg\max_a Q_*(a,s)$ is unique.  This implies that $\proptpi(a_{\text{max}}, s) = 0$, since $V_*(s) = Q_*(a_{\text{max}},s)$ and $\lambda(a_{\text{max}}, s) = 0$.
% For $a \neq a_{\text{max}}$, the Lagrange multipliers $\lambdaplus = V_*(s) -  Q_*(a,s)> 0$  enforce $\piopt(a|s)=0$, which implies $\proptpi(a,s) = 0$ via \cref{eq:advantage}.}

% \textcolor{red}{For $a \neq a_{\text{max}}$, $\piopt(a|s)=0$ and $\lambdaplus = V_*(s) -  Q_*(a,s)> 0$ implies $\proptpi(a,s) = 0$ using \cref{eq:advantage}.}
% % ensures that $\pi(a|s)=0$ and $\proptpi(a,s) = 0$ using \cref{eq:advantage}.   
% Similarly to \mysec{any_policy}, 
% the adversary incorporates the effect of policy regularization via the reward perturbations 
% $\prv(a,s)$ in \cref{eq:husain_constrain}.    
% % In this case, \myprop{advantage} suggests that the reward perturbations reflect the advantage function.
% Although the optimal regularized policy is stochastic in general, the Lagrange multipliers $\lambdaplus$ may, depending on the regularization parameters $\alpha$ and $\beta$, additionally force some action probabilities to zero due to the cutoff behavior of $\exp_{\alpha}$ in the optimal policy (see \cref{eq:qexp} and (\ref{eq:optimal_policy}), \citet{lee2018sparse, lee2019tsallis}).
% % (see \cref{eq:adv}, \citet{lee2018sparse, lee2019tsallis}).
% \textcolor{red}{We compare the role of $\lambdaplus$ and $\pr(a,s)$ in an example in \mysec{visualizations_worst_case}.}



%  \paragraph{Comparison with }
% % \paragraph{Soft Value Aggregation}
% \paragraph{Normalization of Optimal Policy}
% % This also 
% \myprop{advantage} allows us to 
% % We further 
% verify that $\piopt(a|s)$ is normalized,
% since $\psi_{\propt}(s)$ is the appropriate normalization constant for $\proptpi(a,s)$ in \cref{eq:advantage}.
% However, using $Q(a,s) \coloneqq  r(a,s) + \gamma \transitionv$, it is also common to consider the regularized Bellman optimality operator 
% % $V(s) \leftarrow \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q) = \max_\pi \langle \pi(a|s), r(a,s) + \gamma \transitionv \rangle - \frac{1}{\beta}\Omega_{\pi_0}(\pi)$ 
% $V(s) \leftarrow \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q) = \max_\pi \langle \pi(a|s), Q(a,s)  \rangle - \frac{1}{\beta}\Omega_{\pi_0}(\pi)$ 
% \citep{geist2019theory}.   In this case, the appropriate normalization constant is $\psi_{Q_*}(s) = V_*(s) + \psi_{\propt}(s)$ \citep{lee2019tsallis}.   Using \cref{eq:pr_normalizer}, this normalizer $\psi_{Q_*}(s)$ matches the optimal value function $V_*(s) = \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q_*)$ only for \textsc{kl} divergence regularization ($\alpha =1$).
% In \myapp{soft_value}, we describe how this normalization constant $\psi_{\propt}(s)$ relates to soft value aggregation and regularized Bellman optimality operators \citep{lee2019tsallis, geist2019theory} under $\alpha$-divergence regularization.  In particular, we distinguish between the policy normalization constant $\psi_{Q_*}(s)$ and the value or conjugate function $V_*(s) =  \alphaconj(Q_*)$ \citep{geist2019theory}, which match only in the case of \textsc{kl} divergence regularization.
% \end{proof} 


% Finally, we can confirm that $\piopt(a|s)$ is normalized using \myprop{advantage}, 
% We can further use \myprop{advantage} to confirm $\piopt(a|s)$ is normalized,
% since $\psi_{\propt}(s)$ is the appropriate normalization constant for $\proptpi(a,s)$ in \cref{eq:advantage}.
% % $\proptpi(a,s) =  r(a,s) + \gamma \transitionvstar - V_*(s) + \lambdaplus$.  
% In \myapp{soft_value}, we describe how this normalization constant $\psi_{\propt}(s)$ relates to soft value aggregation and regularized Bellman optimality operators \citep{lee2019tsallis, geist2019theory} under $\alpha$-divergence regularization.  In particular, we distinguish between the policy normalization constant $\psi_{Q_*}(s)$ and the value or conjugate function $V_*(s) =  \alphaconj(Q_*)$ \citep{geist2019theory}, which match only in the case of \textsc{kl} divergence regularization.

% Recalling the unregularized dual objective \cref{eq:dual_unreg}, note that the corresponding optimal policy is deterministic with $\piopt(a_{\text{max}}|s) = 1$ for $a_{\text{max}}= \arg \max_{a} r(a,s) + \gamma \transitionvstar$. and $V_*(s) = r(a_{\text{max}},s) + \gamma \transitionvstar$. }
% and $\lambda(a,s) >0$

% In \myapp{soft_value}, we highlight distinct roles for the policy normalization $\psi_{\propt}(s)$ and value function $V_*(s) = \frac{1}{\beta} \alphaconj$ \citep{geist2019theory} in the context of soft value aggregation with the $\alpha$-divergence \citep{lee2019tsallis}.
% % provide detailed discussion of soft value aggregation using the $\alpha$-divergence \citep{lee2019tsallis}, which 

% % we provide detailed discussion relating this normalization condition to soft value aggregation with the $\alpha$-divergence \citep{geist2019theory, lee2019tsallis}. 
% % \RB{Should be $\prpi?$. Is this actually normalized?}.  

% \RB{Too much detail?}
% However, it is more common to treat the optimal regularized policy as a function of the $Q$-values, with $Q_*(a,s) = r(a,s) + \gamma \transitionvstar$.   Letting $\psi_{Q_*}(s)$ denote the corresponding normalization constant, it is clear that
% % As in \citet{lee2019tsallis}, this suggests the identity
% % In \myapp{advantage_pf}, we use similar derivations as \citet{lee2019tsallis} to show that
% \begin{align}
%     \psi_{Q_*}(s) = V_*(s) + \psi_{\propt}(s) . \label{eq:q_normalizer} 
% \end{align}
% This identity \citep{lee2019tsallis} highlights distinct roles for the policy normalization constant $\psi_{Q_*}(s)$ and the value function $V_*(s)$, which coincide only in the case of the \kl divergence regularization.  
% Indeed, we have argued below \cref{eq:pr_normalizer} that for $\alpha = 1$, we have $\psi_{\propt}(s) = 0$ and $\psi_{Q_*}(s) = V_*(s)$ 
% for $\alpha=1$, which does not hold for general $\alpha$ in \cref{eq:q_normalizer}.
% % As discussed in \citet{geist2019theory} and \myapp{soft_value}, the value function for a regularized policy matches the conjugate function $V_{\pi}(s)$

% \RB{Defer to appendix?}
% In \myapp{soft_value}, we provide detailed discussion relating this normalization condition to soft value aggregation with the $\alpha$-divergence \citep{geist2019theory, lee2019tsallis}. 

% % Finally, we can confirm \myprop{advantage} by plugging either the optimal policy \cref{eq:alpha_opt_policy} into the worst-case reward perturbations in \cref{eq:kl_perturbations} or \cref{eq:optimal_perturbations}.

% % the arguments below \cref{eq:pr_normalizer} show that $\psi_{\pr}(s) = 0$ and $\psi_Q(s) = V(s)$, which is not true for general $\alpha$.
% % In the latter case, the discussion below \cref{eq:pr_normalizer} for $\alpha=1$

% % To understand this expression, we can see $\piopt(a|s) \in \Delta^{|\mathcal{A}|}$ using \myprop{advantage}, since $\psi_{\pr(a,s)}(s)$ is the appropriate normalization constant for $\pr(a,s) =  r(a,s) + \gamma \transitionv - V(s)$.  However, it is more common to treat the optimal regularized policy as a function of the $Q$-values, with $Q(a,s) = r(a,s) + \gamma \transitionv$ and  $\psi_Q(s)$ as the corresponding normalization constant.   
% %Using $\psi_Q(s)$ to indicate the normalization constant with respect to the $Q$-values as input,
  
% % Indeed, the expression for $\psi_\pr(s)$ in \cref{eq:pr_normalizer} vanishes for $\alpha =1$ and normalized $\pi_0(a|s)$ and $\pi_\pr(a|s)$, so that $\psi_Q(s) = V(s)$ for \kl divergence regularization.

% % show that this $\piopt(a|s)$ is normalized using similar derivations as \citet{lee2019tsallis}.  

% % Indeed, 
% % when differentiating the Lagrangian in \cref{eq:dual_lagrangian} 
% % % to obtain the dual optimization in \cref{eq:dual_reg}, 
% % we see that the optimal $\mu(a,s)$ satisfies
% % \begin{align}
% %     r(a,s) + \gamma \transitionv - V(s) = \nabla_{\mu}\frac{1}{\beta}\Omega_{\pi_0}(\mu)  \label{eq:opt_policy}
% % \end{align}
% % where $\dualvar(a,s) \leftarrow r(a,s) + \gamma \transitionv - V(s)$ plays the role of the dual variable.   We note the similarity with \myprop{optimal_perturbations}, and 
% % , as in \myprop{optimal_perturbations}.   

% %  We begin by recalling the expression for the optimal policy in a regularized \gls{MDP}, which is obtained by differentiating with respect to $\mu(a,s)$ in \cref{eq:lagrangian}.   
% %  \RB{Does eliminating $\mu(a,s)$ automatically specify the Value function?   In theory (i.e. run the policy for time $\infty$), but possibly not with function approximation...}
 
% %  \RB{Only need Value function for optimal policy}
% % \paragraph{Optimal Policy for KL Divergence}
% %  \paragraph{KL Divergence}
% %  \scriptsize
% % \begin{align}
% % %   \hspace*{-.2cm} \piopt(a|s) = \pi_0(a|s) \, [1+(\alpha-1) \beta \cdot \big( Q(a,s) - \normalizeralpha \big) ]_+^{\frac{1}{\alpha-1}} \label{eq:alpha_opt_policy}
% %   \hspace*{-.2cm} \piopt(a|s) &= \pi_0(a|s) \exp_{\alpha}\bigg\{ \beta \cdot \big( \underbrace{ r(a,s) + \transitionvstar - V_*(s)}_{\Delta r_*(a,s)}- \psi_{\pr}(s) \big) \bigg\}. \label{eq:alpha_opt_policy} \\
% %   \hspace*{-.2cm} \piopt(a|s) &= \pi_0(a|s) \exp_{\alpha}\left\{ \beta \cdot \big( \underbrace{ r(a,s) + \transitionvstar}_{Q_*(a,s)} \underbrace{- V_*(s)- \psi_{\pr}(s)}_{-\psi_Q^{\alpha} = V_*(s)} \big) \right\}. \label{eq:alpha_opt_policy}
% % \end{align}
% % \normalsize

% % \\
% % \textcolor{red}{Check notation of $\normalizeralpha$ over $Q$ values vs. $\Delta r$ as inputs to $\alphaconjmu$}

 
% % For joint $\mu$ regularization,
% %  \scriptsize
% % \begin{align}
% % %   \hspace*{-.2cm} \piopt(a|s) = \pi_0(a|s) \, [1+(\alpha-1) \beta \cdot \big( Q(a,s) - \normalizeralpha \big) ]_+^{\frac{1}{\alpha-1}} \label{eq:alpha_opt_policy}
% %   \hspace*{-.2cm} \mu_*(a,s) = \mu_0(a,s) \exp_{\alpha}\left\{ \beta \cdot \big( r(a,s) + \transitionvstar - V_*(s)- \psi_{\pr} \big) \right\}. \label{eq:alpha_opt_policy}
% % \end{align}
% % \normalsize

% %%%%%%%%%%%%%%%%%%%% HUSAIN MODIFIED REWARD %%%%%%%%%%%%%%%%%%%%%%%%%
% %  \paragraph{Modified Reward Interpretation}
% %  Adapting the dual
% % %  The results of \citet{husain2021regularized}, which apply in a more general setting of arbitrary convex objective functions, match our \myprop{advantage} for the case of regularized \gls{MDP}s.    
% %   While \citet{husain2021regularized} consider a more general setting of arbitrary convex objective functions, their results match our \myprop{advantage} for the case of regularized \gls{MDP}s.
% %   In particular, 
% % instead of expanding the conjugate of the regularization function as in \cref{eq:conjomega2}, \citet{husain2021regularized} consider the convex conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} concave optimization problem $\obj_{\Omega,\beta}(r)$ in \cref{eq:primal_reg}.   This approach yields the modified reward
% % \begin{align}
% % \mropt(a,s) = V_*(s) - \gamma \transitionvstar \, , \label{eq:modified_reward_husain}  %\quad \forall (a,s) \in (\mathcal{A}, \mathcal{S})
% % \end{align}
% % which matches \myprop{advantage} for $\mropt(a,s) = r(a,s) - \proptv(a,s)$.
% % We repeat the derivations of \citet{husain2021regularized} in our notation in \myapp{husain_conjugate}.
% % % We begin by recalling the reward robustness result of \citet{husain2021regularized} in terms of the worst-case modified rewards $\mropt(a,s) = r(a,s) - \propt(a,s)$.   
% % % Instead of expanding the conjugate of the regularization function, \citet{husain2021regularized} consider the conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} concave optimization problem in \cref{eq:primal_reg}.
% % % With detailed derivations in \myapp{husain_conjugate}, th


% % % %  \RB{Optimal POLICY = conjugate applied to optimal Q values}
% % % \paragraph{Modified Reward Interpretation}
% % % We begin by recalling the reward robustness result of \citet{husain2021regularized} in terms of the worst-case modified rewards $\mropt(a,s) = r(a,s) - \propt(a,s)$.   
% % % Instead of expanding the conjugate of the regularization function as in \cref{eq:conjomega2}, \citet{husain2021regularized} consider the conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} concave optimization problem in \cref{eq:primal_reg}.
% % % With detailed derivations in \myapp{husain_conjugate}, this leads to
% % % % We begin by recalling the reward robustness result of \citet{husain2021regularized} in terms of the worst-case modified rewards $\mropt(a,s) = r(a,s) - \propt(a,s)$.   
% % % % Instead of expanding the conjugate of the regularization function, \citet{husain2021regularized} consider the conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} concave optimization problem in \cref{eq:primal_reg}.
% % % % With detailed derivations in \myapp{husain_conjugate}, this leads to 
% % % % % the result
% % % % \begin{restatable}[\citet{husain2021regularized}]{lemma}{husain} 
% % % % % [\textbf{Advantage Function}]
% % % % \label{prop:husain}
% % % % Suppose $(-\obj_{\Omega,\beta}(r))^*$ is increasing and $V_*(s)$ is the optimal solution to 
% % % % For the optimal policy $\pi_*(a|s)$ and any $\alpha$, the worst-case adversarial reward perturbations can be re-expressed as
% % % % \begin{align}
% % % %      \propt(a,s) = Q_{*}(a,s) - V_*(s) \, . \label{eq:advantage}
% % % % \end{align}
% % % % \end{restatable}
% % % % \begin{align}
% % % %   \mropt(a,s) = V_*(s) - \gamma \transitionvstar \, , \label{eq:modified_reward_husain}  %\quad \forall (a,s) \in (\mathcal{A}, \mathcal{S})
% % % % \end{align}
% % % % \JG{I think you can remove this equation and directly talk about \eqref{eq:modified_reward_opt}}
% % % % Adding the environment reward, we can use the worst-case reward perturbations $\propt(a,s) = r(a,s) - \mropt(a,s)$ to rewrite this expression as
% % % \begin{align}
% % % \propt(a,s) &=  r(a,s) + \gamma \transitionvstar -  V_*(s) \label{eq:modified_reward_opt} \, ,
% % % \end{align}
% % % which holds for the optimal value $V_*(s)$ in \cref{eq:dual_reg}.
% % % We can also obtain this result by eliminating $\mu(a,s)$ from the Lagrangian in either \cref{eq:dual_lagrangian} or (\ref{eq:pedro_form}), which are equivalent when $\propt(a,s)= \nabla \omegamu$ as in \mysec{optimal_perturb}.  

% % % % \JG{These two following paragraphs are good. Even better would be to point out more what we are trying to do. E.g. something like: ``Therefore, their result (using the conjugate of entire concave optimization) makes it obvious that the optimal adversarial reward perturbation corresponds to the advantage function. A intriguing question is whether this is also the case when only using the conjugate of the regularizer which is our central tool of analysis)." Or something similar.}
% % % % the approach of \citet{husain2021regularized} and 
% % % From \cref{eq:modified_reward_opt}, we see that the worst-case reward perturbations match the advantage function $\propt(a,s) = r(a,s) + \gamma \transitionvstar -  V_*(s) = Q_{*}(a,s) - V_*(s)$ at optimality. 
% % % % as in  \cref{eq:modified_reward_opt}
% % % However, it is not clear how our expression for $\propt(a,s)$ as a function of $\pi_*(a|s)$ in \cref{eq:optimal_perturbations} would correspond to the advantage function.
% % % % that our expression for $\propt(a,s)$ as a function of $\pi_*(a|s)$ in \cref{eq:optimal_perturbations} corresponds to the advantage function.
% % % % $Q_{*}(a,s) - V_*(s) = r(a,s) + \gamma \transitionvstar -  V_*(s)$ as in  \cref{eq:modified_reward_opt}.  
% % % In \myapp{advantage_pf}, we prove the following proposition from \cref{eq:optimal_perturbations}  directly.
% % % % \paragraph{Relationship to Advantage Function}
% % % \begin{restatable}{proposition}{advantage} 
% % % % [\textbf{Advantage Function}]
% % % \label{prop:advantage} For the optimal policy $\pi_*(a|s)$ and any value of $\alpha$, the worst-case adversarial reward perturbations can be re-expressed as
% % % \begin{align}
% % %      \propt(a,s) = Q_{*}(a,s) - V_*(s) \, . \label{eq:advantage}
% % % \end{align}
% % % \end{restatable}
% % % % \begin{proof}
% % % The proof relies on the following identity (\citet{lee2019tsallis}, \myapp{advantage_pf}), which relates the normalization constant $\normalizeralpha$ of the optimal policy in \cref{eq:alpha_opt_policy}, to the optimal value function $V_*(s)$ in \cref{eq:alpha_conj_norm_main}.
% % % \begin{align}
% % %     \normalizeralpha - V_*(s)=  \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi_*] \label{eq:psidentity} \\
% % %      \textcolor{red}{\psi_{Q}^{\alpha}(s) = V_*(s) + \underbrace{\frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi_*]}_{\psi_{\pr}} }
% % % \end{align}
% % % % Using the optimal policy in \cref{eq:alpha_opt_policy}, we have
% % % % \begin{align}
% % % %     \frac{1}{\beta} \log_{\alpha} \frac{\pi_*(a|s)}{\pi_0(a|s)} = Q(a,s) - \normalizeralpha \, .\label{eq:opt}
% % % % \end{align}
% % % % Combining \cref{eq:psidentity} and \cref{eq:opt}, 
% % % For the optimal policy in \cref{eq:alpha_opt_policy}, we also have $\frac{1}{\beta} \log_{\alpha} \frac{\pi_*(a|s)}{\pi_0(a|s)} = Q_*(a,s) - \normalizeralpha $.   Plugging these into \cref{eq:optimal_perturbations} yields the desired result $\propt(a,s) =Q_*(a,s) - \normalizeralpha +  \normalizeralpha- V_*(s) = Q_*(a,s) - V_*(s)$.  
% % % % From \cref{eq:psidentity}, we can see that $\psi(s;\beta) = V_*(s)$ for the \textsc{kl} divergence at $\alpha =1$.
% % % % $\propt(a,s) &= \frac{1}{\beta} \log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)} + \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi]$ 
% % % % \small 
% % % % \begin{align*}
% % % %     &\propt(a,s) = \frac{1}{\beta} \log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)} + \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi] \\
% % % %     &= Q_*(a,s) - \normalizeralpha +  \normalizeralpha- V_*(s) = Q_*(a,s)- V_*(s)
% % % % \end{align*}
% % % % \normalsize
% % % % \end{proof}

% % \subsection{Analysis of the Optimal Policy}
% % % \paragraph{Modified Reward Intepretation}
% % \textcolor{red}{Our starting point} is Theorem 3 of \citet{husain2021regularized} which, adapted to our setting and notation, expands the regularized dual optimization in \cref{eq:dual_reg} to include a minimization over the modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$

% % \begin{restatable}[{Theorem 3 \citep{husain2021regularized}}]{theorem}{husain}
% % \label{thm:husain}
% % %  \begin{restatable}{proposition}{husain}
% % % [\textbf{Advantage Function}]
% % The optimal value of the regularized objective $\obj_{\Omega, \beta}(r)$ in \cref{eq:primal_reg}, or its dual $\obj^{*}_{\Omega, \beta}(r)$ in \cref{eq:dual_reg}, 
% % is equal to
% % \footnotesize
% % \begin{align}
% %   \hspace*{-.2cm} \inf \limits_{V(s)} &\inf \limits_{\mr(a,s)}   
% %     %&
% %   (1-\gamma) \blangle \nu_0(s), V(s) \brangle 
% %     % \\ & 
% %     + \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left( 
% %     % \pr(a,s)
% %     % \pr(a,s)
% %     r(a,s) - \mr(a,s)
% %     % r(a,s) + \gamma \transitionvpi - \vpi 
% %     \right) \nonumber \\
% %     &\text{subj. to  } V(s) \geq \mr(a,s) + \gamma \transitionv \quad
% %     \forall (a,s)
% %     % \in \mathcal{A} \times \mathcal{S}
% %     \label{eq:husain_constrain}
% % \end{align}
% % \normalsize
% % \end{restatable}
% % % \begin{proof} 
% % % Note that this optimization may be obtained by eliminating $\mu(a,s)$ from the Lagrangian in \cref{eq:pedro_form}.   When the constraint is satisfied with equality, we recover the regularized dual objective in \cref{eq:dual_reg}.
% % % We rewrite an alternative proof from \citet{husain2021regularized} using our notation in \myapp{husain_conjugate}.
% % % \end{proof}
% % % % Note that, instead of expanding the conjugate of the regularization function as in \cref{eq:conjomega2}, \citet{husain2021regularized} consider the convex conjugate $(-\obj_{\Omega,\beta}(r))^*$ of the \textit{entire} regularized optimization,
% % % % $\obj_{\Omega,\beta}(r)$, which is a concave function of $\mu$ by \cref{eq:primal_reg}.
% % % % \footnote{From \cref{eq:primal_reg}, we see that $\obj_{\Omega,\beta}(r)$ is a concave function of $\mu$.}   

% % It is insightful to compare \cref{eq:husain_constrain} to the unregularized dual objective in \cref{eq:dual_lp}, which has a constraint involving the unmodified reward function and does not include the adversarial cost $\frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left(r -\mr \right)$.   
% % As in \mysec{any_policy}, the adversary incorporates the effect of policy regularization by modifying the reward function, subject to a penalty on $\pr(a,s) = r(a,s) -\mr(a,s)$.
% % \citet{husain2021regularized} Lemma 1 shows that the constraint is tight at optimality, with $\mr_{V^*}(a,s) = V^{*}(s) - \gamma \transitionvstar$ and $\pr_{V^*}(a,s)= r(a,s) + \gamma \transitionvstar - V^{*}(s)$ as in \myprop{advantage}.




% % \subsubsection{Equilibrium Properties}
% % \subsection{Optimality Conditions}

% % \subsubsection{Conditions on the Optimal Policy}
% % \subsubsection{Nash Equilibrium Conditions}
% % \subsubsection{Properties of the Worst-Case Perturbations for Optimal Policy}
% % \subsubsection{Properties of the Optimal Policy}
% % \RB{To further contextualize our adversarial interpretation of the \textit{optimal} policy}


\paragraph{Path Consistency Condition}
\vspace*{\header}
The equivalence between $\proptpi(a,s)$ and $\proptv(a,s)$ at optimality matches the \textit{path consistency} conditions from \citep{nachum2017bridging, chow2018path} and suggests generalizations to general $\alpha$-divergence regularization.
% We can further show that the \textit{path consistency} optimality conditions from \citep{nachum2017bridging, chow2018path} are related to the reward perturbation expression in \cref{eq:modified_reward_opt}.  
Indeed, combining \cref{eq:optimal_perturbations} and (\ref{eq:advantage}) and rearranging,
% \begin{equation}
% \hspace*{-.3cm} \resizebox{.91\linewidth}{!}{ $  r(a,s) + \gamma \transitionvstar - \frac{1}{\beta} \log_{\alpha}\frac{\pi_*(a|s)}{\pi_0(a|s)} -  \psipiopt = V_*(s) - \lambdaplus$
% %   V_*(s) -  \gamma \transitionvstar  = r(a,s) - \frac{1}{\beta} \log_{\alpha}\frac{\pi_*(a|s)}{\pi_0(a|s)} + \psi_{\propt}(s) = 
% %   \normalizeralpha  
% }
% \label{eq:path}
% \end{equation}
% \scriptsize
\small
\begin{align}
 r(a,s) + \gamma \transitionvstar - \frac{1}{\beta} \log_{\alpha}\frac{\pi_*(a|s)}{\pi_0(a|s)} & - \psipiopt  =  V_*(s) - \lambdaopt \label{eq:path}
\end{align}
\normalsize
for all $s \in \mathcal{S}$ and $a \in \mathcal{A}$.
%such that $\piopt(a|s) > 0$.
% Note that $\normalizeralpha = V_*(s)$ for \textsc{kl} divergence regularization.
% We emphasize that 
This is a natural result, since path consistency is obtained using the \textsc{kkt} optimality condition involving the gradient with respect to $\mu$ of the Lagrangian relaxation in \cref{eq:dual_lagrangian}.   Similarly, we have seen in \myprop{optimal_perturbations} that 
\ifx\omitindices\undefined
$\prpi(a,s) = \nabla_{\mu} \omegamu$.   
\else
$\prpi = \nabla_{\mu} \omegamu$.  
\fi
See \myapp{path_consistency}.

Path consistency conditions were previously derived for the Shannon entropy \citep{nachum2017bridging} and Tsallis entropy with $\alpha=2$ \citep{chow2018path}, but our expression in \cref{eq:path} provides a generalization to $\alpha$-divergences with arbitrary reference policies.  We provide more detailed discussion in \myapp{indifference_all}.

% Our expression in \cref{eq:path} generalizes the path consistency conditions, previously derived for the Shannon entropy \citep{nachum2017bridging} and Tsallis entropy with $\alpha=2$ \citep{chow2018path}, to general $\alpha$-divergences and arbitrary reference policies.  We provide more detailed discussion in \myapp{path_consistency}.

% For the \textsc{kl} divergence regularization, \citet{nachum2017bridging} use the \textsc{kkt} conditions to show that the optimal policy satisfies \textit{path consistency} equations, which follow directly from the adversarial rewards in \cref{eq:modified_reward_opt} using \myprop{perturbations}.   In particular,
% \begin{align}
%     r(a,s) - \underbrace{\frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)}}_{\propt(a,s)} = V(s) - \gamma \transitionv 
%     %\, \, \forall s \in \mathcal{S}, a \in \mathcal{A}
% \end{align}
% for all $s \in \mathcal{S}, a \in \mathcal{A}$.
% \citet{chow2018path} derive a path consistency equation for the Tsallis entropy with $\alpha =2$ which, generalized to the arbitrary $\alpha$-divergences and using our notation, becomes
% \begin{align}
% r(a,s) &- \underbrace{\frac{1}{\beta}\log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)} - \frac{1}{\beta}(1-\alpha)D_{\alpha}[\pi_0:\pi]}_{\propt(a,s)} \\
% &= V(s) - \gamma \transitionv  + \Lambda(s) \label{eq:path1}
% \end{align}
% where $\Lambda(s) = \normalizerexp - V(s)$.   Using \eqref{eq:psidentity}, we can see that this Lagrange multiplier is equal to $\normalizerexp - V(s)= - \frac{1}{\beta}(1-\alpha)D_{\alpha}[\pi_0:\pi]$, so that we finally obtain
% % is a Lagrange multiplier which can be seen as accounting for the fact that $\normalizerexp \neq V(s)$ for $\alpha \neq 1$.
% % Finally, we are left with
% \begin{align}
%     r(a,s) + \gamma \transitionv - \propt(a,s) = \normalizeralpha   \label{eq:path}
% \end{align}
% \RB{Will change to reflect $\pr(a,s) = Q(a,s) - V(s)$}
% which matches our condition $\pr(a,s) = Q(a,s) - \normalizeralpha$. 
% With detailed derivations in \cref{app:path_consistency}, we show that the optimal $\alpha$-divergence regularized policy satisfies the path consistency condition in \cref{eq:path1}, which generalizes the result of \citet{chow2018path} from $\alpha=2$ to general $\alpha$.



\headerv
\paragraph{Indifference Condition} 
As \citet{ortega2014adversarial} discuss for the single step case, the saddle point of the minmax optimization in \cref{eq:pedro_form} reflects an \textit{indifference} condition which is a well-known property of Nash equilibria in game theory \citep{osborne1994course}.  
Consider $Q(a,s) = r(a,s) + \gamma \transitionv$ to be the agent's estimated payoff for each action in a particular state.  For the optimal policy, value, and worst-case reward perturbations, \cref{eq:path} shows that the pointwise modified reward $Q_*(a,s) - \proptpi(a,s) = V_*(s)$ is equal to a constant.\footnote{This holds for actions with $\piopt(a|s)>0$ and $\small \lambdaplus = 0$.   
Note that we treat $Q(a,s)$ as the reward in the sequential case.}   
% for actions with $\piopt(a|s)>0$ and $\small \lambdaplus = 0$.
Against the optimal strategy of the adversary, the agent becomes indifferent between the actions in its mixed strategy.
The value or conjugate function $V_*(s) = \klconjpii(Q_*)$ (see \myapp{soft_value}) is known as the \textit{certainty equivalent} \citep{fishburn1988nonlinear, ortega2013thermodynamics}, 
which measures the total expected utility for an agent starting in state $s$, in a two-player game 
against an adversary defined by the regularizer $\Omega$ with strength $\beta$.
% where the agent starts in state 
% $s$
% % $s \in \mathcal{S}$ 
% and plays against an adversary defined by the regularizer $\Omega$ with strength $\beta$.
We empirically confirm the indifference condition in \myfig{perturb_opt} and 
% \myfig{pyco_indifference}.
\ref{fig:pyco_indifference}.
% and provide further discussion of the soft aggregation perspective in \myapp{soft_value}. 

% In particular, for the optimal policy and corresponding worst-case reward perturbations, 
% % we confirm in \myapp{indifference} that the modified reward $r\tick(a,s)$
% we confirm using \cref{eq:path} that the 
% % modified payoff for the agent,
% pointwise regularized objective 
% % $r(a,s) + \transitionvstar - \frac{1}{\beta}\log_{\alpha}\frac{\pi^*(a|s)}{\pi_0(a|s)} $
% $r(a,s) + \gamma \transitionvstar - \proptpi(a,s) = V_*(s)$,
% equals a constant across actions where $\piopt(a|s) > 0$, which implies $\lambdaplus = 0$.
% % $a \in \mathcal{A}$ . 
% % where $\pi_*(a|s) > 0$.\footnote{This implies $\lambdaplus=0$ by complementary slackness.}
% % we confirm using \cref{eq:advantage} that the pointwise objective $r(a,s) + \transitionvstar - \propt(a,s) = V_*(s)$ equals a constant across all actions $a \in \mathcal{A}$ in 
% % % $a \in \mathcal{A}$ 
% % a particular state.  
% % % value across all actions $a \in \mathcal{A}$ for a particular state.  
% % % \RB{Is this the expression we should write for the multi-step case?   Haven't stated that $\omegamu = 0$ yet in \cref{eq:pedro_form})}
% The value or conjugate function $V_*(s) = \klconjpii(Q_*)$ is also known as the \textit{certainty equivalent} \citep{fishburn1988nonlinear, ortega2013thermodynamics}, 
% which measures the expected payoff of a two-player game where the agent begins in state 
% $s$
% % $s \in \mathcal{S}$ 
% and plays against an adversary defined by the regularizer $\Omega$ with strength $\beta$.
% We confirm this indifference condition empirically in \cref{fig:perturb_opt} and \cref{fig:pyco_indifference}. 




% \paragraph{Advantage Function Interpretation}
% %From the soft-value aggregation perspective, we can also consider the Lagrange multiplier enforcing normalization $\psi_Q(s)$ in \cref{eq:soft_value}

% % We can use \mythm{husain} and \myprop{advantage} to highlight the complementary roles played by the reward perturbations $\proptv(a,s)$ and Lagrange multiplier $\lambdaplus$ as dual variables.
%  \mythm{husain} and \myprop{advantage} provide further insight into the relationship between the optimal advantage function $Q_*(a,s) - V_*(s)$, the Lagrange multiplier $\lambdaplus$, and the reward perturbations $\proptv(a,s)$.  First, in the unregularized case, note that the optimal policy is deterministic with $\piopt(a_{\text{max}}|s) = 1$,  $V_*(s) = Q_*(a_{\text{max}}, s)$, and $\lambda(a_{\text{max}},s)=0$.
% %  $r(a_{\text{max}},s) + \gamma \mathbb{E}_{a_{\text{max}}, s}^{s\tick}\left[ V_*(s\tick)\right]$.
%  For $a \neq a_{\text{max}}$, the constraint in \cref{eq:dual_lp} is enforced by $\lambdaplus = V_*(s)-Q_*(a,s)>0$.   For all $a \in \mathcal{A}$, \cref{eq:advantage} confirms that $\prpiopt(a,s) = 0$ since there is no regularization.
% %  adversarial interpretation due to regularization.
 
 
% Since the optimal policy is no longer deterministic in a regularized \gls{MDP}, \myprop{advantage} shows that the reward perturbations $\proptpi(a,s)$ need to account for both for the relative value $Q_*(a,s) - V_*(s)$ , and the 
% % depend on both the value estimates $ $
% % shows that $\prpiopt(a,s)$ must account for 
 
%  In the regularized dual optimization in \cref{eq:husain_constrain}, 
 
 
 
 
 
 

% It is common to rewrite \cref{eq:advantage} using the (optimal) state-action values $Q(a,s) = r(a,s) + \gamma \transitionv$


% We can use \mythm{husain} and \myprop{advantage} to further analyze the relationship between $\pr(a,s)$, and the advantage function $Q_*(a,s) =$ act as a dual variable, we can use our advantage function interpretation in \myprop{advantage} to distinguish the role of 


% \paragraph{Comparison to Unregularized Case}
% Finally, it is insightful to compare \cref{eq:husain_constrain} to the \textit{unregularized} dual objective in \cref{eq:dual_lp} in order to highlight the role of the reward perturbations $\proptpi(a,s)$, Lagrange multipliers $\lambdaplus$, and advantage $Q(a,s) - V(s)$.

% First, note that if 

% optimal policy is deterministic with $\piopt(a_{\text{max}}|s) = 1$,  $V_*(s) = Q_*(a_{\text{max}}, s)$, and $\lambda(a_{\text{max}},s)=0$.



% optimal policy is deterministic with $\piopt(a_{\text{max}}|s) = 1$,  $V_*(s) = Q_*(a_{\text{max}}, s)$, and $\lambda(a_{\text{max}},s)=0$.
% It is also insightful to compare \cref{eq:husain_constrain} to the \textit{unregularized} dual objective in \cref{eq:dual_lp}, where the constraint is $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$.  

% does not include the perturbation term $\prv(a,s)$.   


% It is also insightful to compare \cref{eq:husain_constrain} to the \textit{unregularized} dual objective in \cref{eq:dual_lp}, which has a constraint involving the unmodified reward function $V(s) = r(a,s) + \gamma \transitionv + \lambdaplus$ and does not include the adversarial cost $\frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}\left(r -\mrv \right)$.   
% Similarly to \mysec{any_policy}, the adversary incorporates the effect of policy regularization by modifying the reward function, subject to a penalty on the perturbation $\prv = r-\mrv$.
% In \myapp{soft_value}, we further discuss this normalization constant in the context of soft value aggregation and regularized Bellman optimality operators \citep{lee2019tsallis, geist2019theory} using $\alpha$-divergence regularization.


% \textcolor{red}{Finally, \myprop{advantage} reveals a similar role for the Lagrange multiplier $\lambdaplus$ and reward perturbations $\prpi$ as dual variables.  For the \textit{unregularized} dual objective \cref{eq:dual_unreg}, note that the corresponding optimal policy is deterministic with $\piopt(a_{\text{max}}|s) = 1$ and $V_*(s) = r(a_{\text{max}},s) + \gamma \mathbb{E}_{a_{\text{max}}, s}^{s\tick}\left[ V_*(s\tick)\right] \transitionvstar$.
% % $\piopt(a_{\text{max}}|s) = 1$
% % $V_*(s) = r(a_{\text{max}},s) + \gamma \mathbb{E}_{a_{\text{max}}, s}^{s\tick}\left[ V_*(s\tick)\right] \transitionvstar$
% }


==> Reward Robustness TMLR (3)/sections/new/2b_generalization.tex <==
% \section{Relationship with Generalization}\label{sec:feasible}\label{sec:generalization}
\headerv
\section{Visualizing the Feasible Set}\label{sec:feasible}\label{sec:generalization}
\headerv
% \subsection{Feasible Set}\label{sec:feasible}
% \TG{I like this section. Maybe worth spending one, two sentences re-iterating that we have established the adversarial interpretation, but we also know that the adversary is limited. The most important missing bit then is: the characterization of the adversary via this limitedness (the feasible set), which we're going to show now.}
% \RB{Although the feasible set is general (any $\pi$), the plot is for the case of an optimal policy and is identical to the setting of \citet{eysenbach2021maximum} referenced previously}
In the previous section, we have established an adversarial interpretation which suggests that regularized policies are robust to worst-case reward perturbations.   However, we have not discussed implications for zero-shot generalization or understood the limitations of this adversary.
% robustness to worst-case reward perturbations 
% The adversarial interpretation in  suggests that regularized policies are robust to worst-case reward perturbations.   
 In particular, it is not clear how the cost function $\alphaconjmu(\pr)$ in \cref{eq:pedro_form} restricts the feasible set $\mathcal{R}$ of perturbations from which the adversary can select.  
 We characterize the feasible set in the following proposition, with visualizations in \cref{fig:feasible_set_main}.
%  In the following proposition, we provide a simple constraint to characterize the feasible set, with visualizations in \cref{fig:feasible_set_main}.
%  The optimal $\propt$ in \myprop{optimal_perturbations} suggest a simple constraint to characterize the feasible set in the following proposition.
\begin{restatable}[]{proposition}{feasible}\label{prop:feasible} For a given policy $\pi(a|s)$ and any $\alpha$-divergence, the feasible set of reward perturbations available to the adversary is defined by the constraint
\begin{align}
\alphaconjmu(\pr) \leq 0 \label{eq:alpha_feasible} 
% \\\frac{\alpha-1}{\alpha} \langle \mu(s) \pi^{(\pr)}_*(a|s), \pr \rangle - \frac{1}{\alpha}(V^{\pr}_*(s)  \leq 0 \label{eq:alpha_feasible}
\end{align}
For \textsc{kl} divergence regularization, we obtain
% this translates to
\begin{align}
   \sum\limits_{a \in \mathcal{A}} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} \leq 1 \, . \label{eq:kl_feasible}
\end{align}
\end{restatable}
\begin{proof} See \myapp{feasible_pf} for proof. 
\textcolor{red}{which proceeds by evaluating the conjugate function at the worst-case $\propt$, with $\alphaconjn(\propt)=0 \, \forall \alpha$.  
% Since $\alphaconjn(\pr)$ is increasing in $\pr$ and the $-\pr(a,s)$ term in \cref{eq:pedro_form} is decreasing, the constraint follows.
The constraint for the minimization problem in \cref{eq:pedro_form} then follows from the fact that $\alphaconjn(\pr)$ is increasing in $\pr$. \RB{\textbf{no longer holds}: alternative proof given in the appendix}}
% \RB{improve}
\end{proof}
The above constraints characterize the robust set of modified reward functions for which we can provide performance guarantees.
% , given a particular stochastic policy and regularized objective.
% for a particular stochastic policy and regularized objective.
More precisely, for given \gls{MDP} transition dynamics, we say that a policy trained with reward $r(a,s)$ and 
% and regularization based on $\Omega, \pi_0, $  
regularized objective $\obj_{\Omega,\beta}(r)$ 
\textit{generalizes} to an environment with a modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$ if 
% , as in \cref{eq:reward_perturbation_stmt},
\small
\begin{align}
  \hspace*{-.2cm} 
%   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) \rangle - \omegamu \, . \label{eq:robust_def} \\
  \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) \rangle - \omegamu \, . \label{eq:robust_def}
%   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(s)\pi(a|s), r(a,s) - \ptReg(\pi) \rangle \\
%   \langle \mu(a,s), \mr(a,s) \rangle &\geq \obj_{\Omega, \beta}(r) = \alphaconjmu \\
%   \alphaconjmu \text{vs.} \alphaconjmuu \\
%   \alphaconjn \text{vs.} \alphaconjnn \\
%   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(s), V_*(s; \beta) \rangle = \langle \mu(s),\alphaconjn \rangle \\
%   \obj_{\Omega, \beta}(r)  = \alphaconjmu &= \frac{\alpha-1}{\alpha} \langle \mu(s), \alphaconjn \rangle 
%   \langle \mu(a,s), r(a,s) - \pr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) - \ptReg(\pi) \rangle  %\blangle \mu(s) \pi(a|s), \mr(a,s) \brangle \geq  \blangle \mu(s) \pi(a|s), r(a,s) - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \brangle \, . \label{eq:robust_def}
\end{align}
\normalsize
% \JG{Ok, I think you need to say a couple of sentences here. I was initially confused by this thinking that it was trivial but it is not at all. I think one expects something of the form: $ \langle \mu(a,s), r(s,a) + \Delta r(s,a) \rangle \geq \langle \mu(a,s), r(a,s) \rangle $ for $\Delta r(s,a) \in Z$ where $r(s,a) + \Delta r(s,a) = r'(s,a)$ and $Z$ is the set of allowed perturbations. In its current form with the regularizer it is not clear what this implies for generalization right?. Sorry if this question is too complicated, It could also be that I need more time to understand this. I think its important to get the explanation right though.} 
In other words, the expected reward using the modified $\mr(a,s)$ is greater than or equal to the value of the regularized objective $\obj_{\Omega,\beta}(r)$ using the original $r(a,s)$. 
%  on the left side on the right side.  
Note that \cref{eq:robust_def} holds with equality for the worst-case modified reward $\mropt(a,s)$ (\mysec{optimal_perturb} or \myapp{preserve}). 
\textcolor{red}{The feasible set in \myfig{feasible_set_main} shows other rewards for which the inequality holds, with equality 
% holding 
at the boundary.} \RB{Is this true?  Otherwise, why would we pick out the particular $\Delta r^{*}$ that we do?  Further, the original $r(a,s)$ is at the boundary, and this does not hold with equality.}
% While it is clear that increasing the reward in both actions preserves the inequality in \cref{eq:robust_def},  
% % is feasible for an adversary that minimizes \cref{eq:pedro_form}, 
% \cref{fig:feasible_set_main} also includes regions where one reward decreases.

% while the feasible set in \myfig{feasible_set_main} shows the other rewards for which the inequality holds. \TG{Shall we mention that the boundary of the feasible set corresponds to the equality?}

It is in this particular sense that we can claim zero-shot generalization for a regularized policy.
We also notice that this form of robustness is sensitive to the value of the regularized objective function in \cref{eq:robust_def}, which we discuss in further detail in \mysec{entropy_vs_div}.
% Note that the expected reward under the worst-case modified reward $\mropt(a,s)$ matches the value of the regularized objective, as we have reasoned in \mysec{optimal_perturb} or \myapp{preserve}, while the feasible set in \myfig{feasible_set_main} shows the other rewards for which \cref{eq:robust_def} holds.
% Note that the right hand side corresponds to the full objective function, including regularization, whereas the left hand side is only the expected reward.  
% .regularization, as we further discuss in \mysec{entropy_vs_div}.
% the other reward functions for a stochastic policy is robust 
% The feasible set characterizes the other reward functions for which a stochastic policy achieves an expected reward greater than or equal to the value of the regularized objective. \TG{This is very important (for the reader) - make sure to emphasize the ``robustness'' and generalization-guarantee (in terms of performance) we get exactly from this fact.}
% to which a stochastic policy is robust.

\headerv
\paragraph{Visualizing the Feasible Set} 
In \myfig{feasible_set_main}, we visualize the feasible set of perturbed rewards in a two-dimensional action space for the \KL or $\alpha$-divergence, various $\beta$, and a uniform or non-uniform prior policy $\pi_0$.
\textcolor{red}{Since the optimal policy can be calculated easily in the single-step case}, we consider fixed $Q(a,s) = r(a,s) = \{1.1, 0.8\}$ and show the robustness of the optimal $\pi_*(a|s)$, which differs based on the regularization scheme (see \cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).
We determine the feasible set of $\pr$ using the constraint in \myprop{feasible} (see \myapp{feasible_plot} for details), and plot the modified reward $r\tick(a,s) = Q(a,s) - \pr(a,s)$ for each action.  
%  For clarify of exposition, we focus on the \KL divergence constraint in \cref{eq:kl_feasible}.

Inspecting the constraint for the adversary in \cref{eq:kl_feasible}, note that both reward increases $\pr(a,s) < 0$ and reward decreases $\pr(a,s) > 0$ contribute non-negative terms at each action, which either up- or down-weight the reference policy $\pi_0(a|s)$.  The constraint on their summation forces the adversary to trade off between perturbations of different actions in a particular state.   
Further, since the constraints in \myprop{feasible} integrate over the action space, the rewards for \textit{all} actions in a particular state must be perturbed together.  
While it is clear that increasing the reward in both actions preserves the inequality in \cref{eq:robust_def},  
% is feasible for an adversary that minimizes \cref{eq:pedro_form}, 
\cref{fig:feasible_set_main} also includes regions where one reward decreases.
% While it is natural that increasing the reward in both actions is feasible for an adversary that minimizes \cref{eq:pedro_form}, \cref{fig:feasible_set_main} also includes regions where one reward decreases.
% In all cases, it is natural that increasing the reward in both actions is feasible for an adversary seeking to minimize the objective in \cref{eq:pedro_form}.

For high regularization strength ($\beta=0.1$), we observe that the boundary of the feasible set is nearly linear, with the slope $-\frac{\pi_0(a_1|s)}{\pi_0(a_2|s)}$ based on the ratio of each action in the prior.  The boundary steepens for lower regularization strength.  \textcolor{red}{We can use the indifference condition to provide further geometric insight.   First, drawing a line from the origin with slope $1$ will intersect the feasible set at the worst-case modified reward (red star) in each panel, with $\mropt(a_1,s) = \mropt(a_2,s)$.  At this point, the slope of the tangent line yields the ratio of action probabilities, as we saw for the $\beta = 0.1$ case.  With decreasing regularization as $\beta \rightarrow \infty$, the slope approaches $0$ or $-\infty$ for a nearly deterministic policy and a rectangular feasible region.} \RB{Where does InDifference go?}
% ince we have plotted the optimal policy $\piopt(a|s)$ corresponding to the reward function $r(a,s)$, we can see that the indifference condition holds, with $\mropt(a_1,s) = \mropt(a_2,s)$ for the red star in each panel.   In this case, we ca  

Finally, we show the feasible set for the $\alpha$-divergence with $\alpha \in \{-1, 3\}$ and $\beta = 10$ in \cref{fig:feasible_set_main} (d)-(e) and (i)-(j), with further visualizations in \myapp{additional_feasible}.   Compared with the \textsc{kl} divergence,
we observe a wider feasible set boundary for $\alpha =-1$, whereas $\alpha = 3$ \textcolor{red}{}
% induces a steeper boundary with smaller worst-case perturbations. 
% \RB{Update the discussion here to reflect modified plots}
% for the $\alpha = 3$ case, corresponding to a steeper boundary of the feasible set.   
% \ref{fig:tabd}-\ref{fig:tabe} and \ref{fig:tabi}-\ref{fig:tabj} .  
% For the optimal policy associated with a given reward function,  we see that the $\alpha = -1$ feasible set may not include this reward function.  
% \input{sections/single_step_fig}
%%%%%%%%%%%%%%%%%%%%% PRE-move to "GENERALIZATION" Section %%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Feasible Set}\label{sec:feasible}
% % \TG{I like this section. Maybe worth spending one, two sentences re-iterating that we have established the adversarial interpretation, but we also know that the adversary is limited. The most important missing bit then is: the characterization of the adversary via this limitedness (the feasible set), which we're going to show now.}
% % \RB{Although the feasible set is general (any $\pi$), the plot is for the case of an optimal policy and is identical to the setting of \citet{eysenbach2021maximum} referenced previously}

% The adversarial interpretation in \cref{eq:pedro_form} suggests that regularized policies are robust to worst-case reward perturbations.   However, it is not clear how the cost function $\alphaconjn(\pr)$ restricts the set of perturbations available to the adversary.
%  In particular, it is not clear how the cost function $\alphaconjn(\pr)$ in \cref{eq:pedro_form} restricts the set of perturbations available to the adversary.
%  The optimal $\propt$ in \myprop{optimal_perturbations} suggest a simple constraint to characterize the feasible set in the following proposition.
% \begin{restatable}[]{proposition}{feasible}\label{prop:feasible} For a given policy $\pi(a|s)$ and any $\alpha$-divergence, the feasible set of reward perturbations is defined by the constraint
% \begin{align}
% \alphaconjn(\pr) \leq 0 \label{eq:alpha_feasible}
% \end{align}
% For \textsc{kl} divergence regularization, this translates to
% \begin{align}
%   \sum\limits_{a \in \mathcal{A}} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} \leq 1 \, . \label{eq:kl_feasible}
% \end{align}
% \end{restatable}
% \begin{proof} See \myapp{feasible_pf} for proof, which proceeds by evaluating the conjugate function at the optimal $\propt$, with $\alphaconjn(\propt)=0 \, \forall \alpha$.  
% % Since $\alphaconjn(\pr)$ is increasing in $\pr$ and the $-\pr(a,s)$ term in \cref{eq:pedro_form} is decreasing, the constraint follows.
% The constraint for the minimization problem in \cref{eq:pedro_form} then follows from the fact that $\alphaconjn(\pr)$ is increasing in $\pr$.\RB{improve}
% \end{proof}
% \vspace*{-.1cm}

% These constraints precisely characterize the robust set of modified reward functions, for which we can guarantee zero-shot generalization of a particular stochastic policy and regularized objective.\TG{This is very important (for the reader)}
% % the other reward functions for a stochastic policy is robust 
% % The feasible set characterizes the other reward functions for which a stochastic policy achieves an expected reward greater than or equal to the value of the regularized objective. \TG{This is very important (for the reader) - make sure to emphasize the ``robustness'' and generalization-guarantee (in terms of performance) we get exactly from this fact.}
% % to which a stochastic policy is robust.
% In \myfig{feasible_set_main}, we visualize the feasible set of perturbed rewards in a two-dimensional action space for the \KL or $\alpha$-divergence, various $\beta$, and uniform or non-uniform prior policy $\pi_0$.
% Since the optimal policy can be calculated easily in the single-step case, we consider $\pi_*(a|s)$ corresponding to fixed $Q(a,s) = r(a,s) = \{1.1, 0.8\}$, which differ based on the regularization scheme (see \cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).
% We determine the feasible set of $\pr$ according to the constraint in \myprop{feasible} (see \myapp{feasible_plot} for details), and plot the modified reward $r\tick(a,s) = Q(a,s) - \pr(a,s)$ for 
%  each action.  
% %  For clarify of exposition, we focus on the \KL divergence constraint in \cref{eq:kl_feasible}.

% Inspecting the constraints for the adversary in \cref{eq:kl_feasible}, note that both reward increases $\pr(a,s) > 0$ and reward decreases $\pr(a,s) < 0$ contribute non-negative terms at each action, which either up- or down-weight the reference policy $\pi_0(a|s)$.  The constraint on their summation forces the adversary to trade off between perturbations of different actions in a particular state.   In all cases, it is natural that increasing the reward in both actions is feasible for an adversary seeking to minimize the objective in \cref{eq:pedro_form}.

% For high regularization strength ($\beta=0.1$), we observe that the boundary of the feasible set is nearly linear, with the slope $-\frac{\pi_0(a_2|s)}{\pi_0(a_1|s)}$ based on the ratio of each action in the prior.  The boundary steepens for lower regularization strength.  However, since we have expanded the optimal policy $\piopt(a|s)$ for the reward $r(a,s)$, we can use the indifference condition provide further geometric insight.   First, drawing a line from the origin with slope $1$ will intersect the feasible set at the worst-case modified reward (red star) in each panel, with $\mropt(a_1,s) = \mropt(a_2,s)$.  At this point, the slope of the tangent line yields the ratio of action probabilities, as we saw for the $\beta = 0.1$ case.  With decreasing regularization as $\beta \rightarrow \infty$, the slope approaches $0$ or $\infty$, with a deterministic policy and rectangular feasible region.
% % ince we have plotted the optimal policy $\piopt(a|s)$ corresponding to the reward function $r(a,s)$, we can see that the indifference condition holds, with $\mropt(a_1,s) = \mropt(a_2,s)$ for the red star in each panel.   In this case, we ca  

% Finally, we show the feasible set for the $\alpha$-divergence with $\alpha \in \{-1, 3\}$ and $\beta = 10$ in \cref{fig:feasible_set_main} (d)-(e) and (i)-(j), with further visualizations in \cref{app:additional_feasible}.   Compared with the \textsc{kl} divergence,
% we observe a wider boundary of the feasible set for $\alpha =-1$, whereas $\alpha = 3$ induces a steeper boundary with smaller worst-case reward perturbations.
% % for the $\alpha = 3$ case, corresponding to a steeper boundary of the feasible set.   
% % \ref{fig:tabd}-\ref{fig:tabe} and \ref{fig:tabi}-\ref{fig:tabj} .  
% % For the optimal policy associated with a given reward function,  we see that the $\alpha = -1$ feasible set may not include this reward function.  

==> Reward Robustness TMLR (3)/sections/new/3_entropy_reg.tex <==
% \section{Discussion}\label{sec:discussion}
% \vspace*{\header}
% % What insights \TG{What are the main insights (sounds less defensive) :))))} 
% What are the main insights that can be obtained from this adversarial interpretation of regularized policies?
% In \mysec{generalization}, we discuss the generalization properties associated with this robustness, which we highlight is particularly sensitive to the form of the objective in \mysec{entropy_vs_div}.  We highlight an additional connection with the notion of path consistency \citep{nachum2017bridging, chow2018path} in \mysec{path}.
% % For the optimal policy, we show that our interpretation is compatible with the modified reward interpretation of \citet{husain2021regularized} in \ref{sec:husain}.  This directly leads to connections with the notion of path consistency \citep{nachum2017bridging, chow2018path} in \ref{sec:path} and the game-theoretic interpretation of \citet{ortega2014adversarial} in \ref{sec:indifference}. 
% % \RB{seems long, is this all necessary?}
% % We
% % connections with the notion of path consistency \citep{nachum2017bridging, chow2018path} in \ref{sec:modified} and , and argue that  adversarial reward perturbations can provides a natural justification for including $Q$-values as dual variables in \gls{LP} formulations of \gls{MDP}s in \ref{sec:qlp}.
% %\RB{Add generalization analysis}
% %\RB{Add reward $\rightarrow$ robustness vs. policy $\rightarrow$ robustness}

% \subsection{Relationship to Generalization}\label{sec:generalization}
% %For our purposes, we consider `zero-shot generalization' of a given policy $\pi(a|s)$ to an environment with a modified reward function $\mr(a,s)$ to mean that
% Our adversarial interpretations imply robustness or generalization of a given policy $\pi(a|s)$ to an environment with a modified reward $\mr(a,s)$ in the sense that, for given \gls{MDP} transition dynamics
% \small
% \begin{align}
%   \hspace*{-.2cm} \langle \mu(a,s), \mr(a,s) \rangle \geq \langle \mu(a,s), r(a,s) \rangle - \omegamu \, \label{eq:robust_def}
%   %\blangle \mu(s) \pi(a|s), \mr(a,s) \brangle \geq  \blangle \mu(s) \pi(a|s), r(a,s) - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \brangle \, . \label{eq:robust_def}
% \end{align}
% \normalsize
% %Our adversarial interpretations imply robustness or generalization of a given policy $\pi(a|s)$ to a modified reward function in this particular sense.   
% %Notice that 
% where the right hand side corresponds to the full objective function, including regularization, whereas the left hand side is only the expected reward.
%  %the regularized objective $\mathcal{R}_{\Omega, \beta}(r\tick) \geq \mathcal{R}_{\Omega, \beta}(r\tick)$
% The constraints in \myprop{feasible} characterize the robust set of modified rewards to which a given policy can generalize, as visualized in \cref{fig:feasible_set_main}.   Since these constraints integrate over the action space, the rewards for all actions in a particular state must be perturbed together.   
% % As we see in \cref{fig:perturb_opt} and \ref{fig:pyco}, this often corresponds to 
% % Due to these constraints on the adversarym we see in \cref{fig:perturb_opt} and \ref{fig:pyco} that 
% % \TG{Maybe we can comment here directly that this typically corresponds to reward-decreases for some actions but (adversarial!) reward increases for other actions of the same state.}

% By running a fixed policy in an environment with higher rewards, we naturally expect the objective function to increase.   However, for useful zero-shot generalization, we might hope that a policy will still perform well when the reward function decreases in at least some states.   We observe in \cref{fig:perturb_opt} and \ref{fig:pyco} that the adversary typically chooses reward decreases in some actions and increases in others, and proceed to further investigate this property in the next subsection.
% % However, we next discuss how
% In the next subsection, we discuss how 
% these qualitative properties can be sensitive to the form of the regularization function $\omegamu$.
% in \cref{eq:robust_def}.

% \section{Divergence vs. Entropy}\label{sec:entropy_vs_div}
\headerv
\section{Comparison with Entropy Regularization}\label{sec:entropy_vs_div}
% \subsection{Comparison with Entropy Regularization }\label{sec:entropy_vs_div}
\vspace*{\header}
% \JG{This whole section is absolutely amazing. Thanks!} 
As argued in \mysec{optimal_perturb}, the worst-case reward perturbations preserve the value of the regularized objective function.  Thus, we should expect our robustness conclusions to depend on the exact form of the regularizer.

When regularizing with the Tsallis or Shannon ($\alpha = 1$) entropy, the worst-case reward perturbations become %perturbed reward is %reward
\small
\begin{align}
    % \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \pi(a|s) \,. \label{eq:ptwise_perturb_ent}
    \hspace*{-.2cm} \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \pi(a|s) + \frac{1}{\beta} \frac{1}{\alpha} \big(1 - \sum 
    % \limits
    _{a \in \mathcal{A}} \pi(a|s)^{\alpha} \big) \,. \label{eq:ptwise_perturb_ent}
\end{align}
\normalsize
% \RB{Change with new $\propt$}
%For entropy regularization,
In \myapp{entropy_nonnegative}, we show that these perturbations yield a pointwise non-negative contribution to the objective $r(a,s) - \propt(a,s)$, with $-\propt(a,s) \geq 0$ when $\pi(a|s) \leq 1$, for $0 < \alpha \leq 1$.   
% \RB{Why does Lee result hold for any $\alpha$?}
%  ONLY} 
% In the following, 
We argue that this property leads to several unsatisfying conclusions in previous work \citep{lee2019tsallis, eysenbach2021maximum}, which are resolved by using the \textsc{kl} and $\alpha$-divergence for analysis instead of the corresponding entropic quantities.\footnote{Entropy regularization corresponds to divergence regularization with the uniform reference distribution $\pi_0(a|s)$.}

% We argue the pointwise non-negative contribution of these perturbations to the objective $r(a,s) - \propt(a,s)$, with $-\propt(a,s) \geq 0$ for $\pi(a|s) \leq 1$, leads to several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}.   As we discuss in the following, this is resolved by using the \textsc{kl} and $\alpha$-divergence instead of the corresponding entropic quantities for the analysis. \footnote{Entropy regularization corresponds to the divergence to the uniform reference distribution $\pi_0(a|s)$ over actions.}
% In particular, entropy regularization should be considered as a divergence to the uniform reference distribution $\pi_0(a|s)$ over actions.
%Our use of the \textsc{kl} and} $\alpha$-divergences, instead of the corresponding entropic quantities, resolves several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}.   

First, this means that an entropy-regularized policy appears to only be `robust' to \textit{increases} in the reward function.   However, for useful generalization, we might hope that a policy will still perform well when the reward function decreases in at least some state-action pairs. 
 Including the reference distribution $\pi_0$ via divergence regularization resolves this issue,
%  changes this property, 
 and we observe in \cref{fig:feasible_set_main}-\ref{fig:pyco} that the adversary typically chooses reward decreases in some actions and increases in others.  For example, for the \textsc{kl} divergence, $\propt(a,s) = \frac{1}{\beta}\log \frac{\pi(a|s)}{\pi_0(a|s)}$ implies robustness to reward decreases when $\pi(a|s) > \pi_0(a|s)$.
 
%  so that the worst-case perturbation $\propt(a,s) = \frac{1}{\beta}\log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}$ %\frac{\pi(a|s)}{ \pi_0(a|s)}$ % yields robustness to reward \textit{decreases} when $\pi(a|s) > \pi_0(a|s)$ and reward increases otherwise.  
% Indeed, using divergence regularization, we observe in \cref{fig:perturb_opt} and \ref{fig:pyco} that the adversary typically chooses reward decreases in some actions and increases in others.  
% , and proceed to further investigate this property in the next subsection.
% For useful zero-shot generalization


% Including the reference distribution as in \myprop{feasible} changes this property, so that the worst-case perturbation $\propt(a,s) = \frac{1}{\beta}\log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}$ %\frac{\pi(a|s)}{ \pi_0(a|s)}$ % yields robustness to reward \textit{decreases} when $\pi(a|s) > \pi_0(a|s)$ and reward increases otherwise.  
% \RB{Include that we would like to be robust to decreases for useful generalization}

Similarly, \citet{lee2019tsallis} note that \textcolor{red}{, for any $\alpha$,}%$\frac{1}{\beta}\Omega^{*}_{\pi_0}(\discussiondual) = \max_{\pi(a|s)} \langle \pi(a|s), \discussiondual(a,s) \rangle + \frac{1}{\beta} H_{\alpha}(\pi) \geq \discussiondual(a_{\max}, s) $
\small
\begin{align*}
    \frac{1}{\beta}\Omega^{*(H_{\alpha})}_{\pi_0,\beta,\pi}(\discussiondual) = %\max_{\pi(a|s)}
    \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \langle \pi, \discussiondual \rangle + \frac{1}{\beta} H_{\alpha}(\pi) \geq \discussiondual(a_{\max}, s) 
    % \left(-\frac{1}{\beta} H_{\alpha}(\pi)\right)
\end{align*}
\normalsize
\normalsize
where $a_{\max} = \argmax_a \discussiondual(a,s)$ and Tsallis entropy $H_{\alpha}(\pi)$ equals Shannon entropy for $\alpha = 1$. 
% \RB{Soft Value, $\pi$ optimization}
% \textcolor{red}{Due to the pointwise non-negativity of $-\log_{\alpha}\pi(a|s)$ in the (Tsallis) entropy,  this soft value aggregation 
% % with the negative Tsallis entropy as a regularizer,  
% yields a result that is \textit{larger} than any particular $Q$-value. }
\textcolor{red}{This soft value aggregation yields a result that is \textit{larger} than any particular $Q$-value.}
% Due to the pointwise non-negativity of the 
%so that soft value aggregation yields a value which is \textit{larger} than any particular reward. 
% \begin{align}
%     \max_{\pi(a|s)} \langle \pi(a|s), \discussiondual(a,s) \rangle + \beta H_q(\pi) \geq \max_a \discussiondual(a,s)
% \end{align}
% where $H_q$ is the Tsallis entropy.
By contrast, for the $\alpha$-divergence, we show in \myapp{qmax} that
% \footnotesize
% \begin{align*}
%   \hspace*{-.1cm} \discussiondual(a_{\max},s) + \frac{1}{\beta}\frac{1}{\alpha} \log_{\alpha} \pi(a_{\max}| s) \leq \alphaconjn(\discussiondual) \leq  \discussiondual(a_{\max},s)
% \end{align*}
\begin{equation}
\resizebox{\columnwidth}{!}{ $\discussiondual(a_{\max},s) + \frac{1}{\beta}\frac{1}{\alpha} \log_{\alpha} \pi(a_{\max}| s) \leq \alphaconjn(\discussiondual) \leq  \discussiondual(a_{\max},s) $ 
  } \nonumber
\end{equation}
\normalsize
This provides a more natural interpretation of $V_*(s) =  \alphaconjn(Q)$ as a soft maximum function, with $ \mathbb{E}_{\pi_0}[\discussiondual(a_{\max},s)] \leq V_*(s) \leq \discussiondual(a_{\max},s)$, as in \myapp{soft_value}.
% \cref{fig:perturb_opt}.

Finally, entropy regularization also affects interpretations of the feasible set.  %For entropy regularization,
\citet{eysenbach2021maximum} consider the same constraint as in \cref{eq:kl_feasible}, but without the reference distribution
\begin{align}
    \sum \limits_{a} \expof{\beta \cdot \pr(a,s)} \leq 1  \, \, \, \forall s \in \mathcal{S} \, . \label{eq:ent_constraint}
\end{align}
This constraint suggests that the original reward function ($\pr = 0$) is not feasible for the adversary.  
% , unless the policy is deterministic
More surprisingly, \citet{eysenbach2021maximum} App. A5 argues that \textit{increasing} regularization strength (with lower $\beta$) may lead to \textit{less} robust policies based on the constraint in \cref{eq:ent_constraint}.    In \myapp{eysenbach}, we discuss how including $\pi_0(a|s)$ in the constraint via divergence regularization avoids this conclusion.   As expected, 
we observe in 
\cref{fig:feasible_set_main} that increasing regularization strength leads to more robust policies.


% \subsection{Adversarial Modified Rewards}\label{sec:husain}
% \vspace*{\header}
% The adversarial interpretation in the previous sections may also be written directly using the modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$, which has been studied in a more general setting by \citet{husain2021regularized}.

% \citet{husain2021regularized} consider maximizing an arbitrary concave objective $\concaveopt$, and proceed to derive its convex conjugate $(-\concaveopt)^*$.    Translated to our setting and notation,
% this involves the conjugate expansion of the regularized objective $(-\obj_{\Omega, \beta}(r))^*$ instead of the conjugate of the regularizer only, $ (\omegamu)^*$.  
% With detailed derivations in \myapp{husain_conjugate}, this leads to the Lagrangian
% \begin{align}
%     \hspace*{-.2cm} & \quad \max \limits_{\mu(a,s)} \min \limits_{V(s)} \min \limits_{\textcolor{\highlight}{\mr(a,s)}} \, \label{eq:husain_form} \\
%     & \big \langle {\mu(s)\pi(a|s)}, {\textcolor{\highlight}{\mr(a,s)} +\gamma \transitionv - V(s) } \brangle  \nonumber  \\
%     & \quad+ \alphaconjn \big( r(a,s) - \textcolor{\highlight}{\mr(a,s)} \big) + (1-\gamma) \blangle \nu_0(s), V(s) \brangle \, ,  \nonumber
% \end{align}
% which matches \cref{eq:pedro_form} up to simple reparameterization of $\mr(a,s) = r(a,s) - \pr(a,s)$.

% Differentiating \cref{eq:husain_form} with respect to $\pi(a|s)$ and solving for the optimal modified rewards yields the result of \citet{husain2021regularized} that
% \begin{align}
%   \mropt(a,s) = V(s) - \gamma \transitionv  %\quad \forall (a,s) \in (\mathcal{A}, \mathcal{S})
% \end{align}
% Adding the environment reward, we can use the optimal reward perturbations $\propt(a,s) = r(a,s) - \mropt(a,s)$ to rewrite this expression
% \begin{align}
% \propt(a,s) &=  r(a,s) + \gamma \transitionv -  V(s) \label{eq:modified_reward_opt}
% \end{align}
% which matches our advantage function interpretation in 
% % \mysec{advantage} 
% \myprop{advantage}.


\input{sections/pyco_fig}

% \subsection{Connection with Path Consistency}\label{sec:path}
% \vspace*{\header}
% For the \textsc{kl} divergence regularization, \citet{nachum2017bridging} use the \textsc{kkt} conditions to show that the optimal policy satisfies \textit{path consistency} equations, which follow directly from the adversarial rewards in \cref{eq:modified_reward_opt} using \myprop{perturbations}.   In particular,
% \begin{align}
%     r(a,s) - \underbrace{\frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)}}_{\propt(a,s)} = V(s) - \gamma \transitionv 
%     %\, \, \forall s \in \mathcal{S}, a \in \mathcal{A}
% \end{align}
% for all $s \in \mathcal{S}, a \in \mathcal{A}$.
% \citet{chow2018path} derive a path consistency equation for the Tsallis entropy with $\alpha =2$ which, generalized to the arbitrary $\alpha$-divergences and using our notation, becomes
% \begin{align}
% r(a,s) &- \underbrace{\frac{1}{\beta}\log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)} - \frac{1}{\beta}(1-\alpha)D_{\alpha}[\pi_0:\pi]}_{\propt(a,s)} \\
% &= V(s) - \gamma \transitionv  + \Lambda(s) \label{eq:path1}
% \end{align}
% where $\Lambda(s) = \normalizerexp - V(s)$.   Using \eqref{eq:psidentity}, we can see that this Lagrange multiplier is equal to $\normalizerexp - V(s)= - \frac{1}{\beta}(1-\alpha)D_{\alpha}[\pi_0:\pi]$, so that we finally obtain
% % is a Lagrange multiplier which can be seen as accounting for the fact that $\normalizerexp \neq V(s)$ for $\alpha \neq 1$.
% % Finally, we are left with
% \begin{align}
%     r(a,s) + \gamma \transitionv - \propt(a,s) = \normalizeralpha   \label{eq:path}
% \end{align}
% \RB{Will change to reflect $\pr(a,s) = Q(a,s) - V(s)$}
% which matches our condition $\pr(a,s) = Q(a,s) - \normalizeralpha$. 
% With detailed derivations in \cref{app:path_consistency}, we show that the optimal $\alpha$-divergence regularized policy satisfies the path consistency condition in \cref{eq:path1}, which generalizes the result of \citet{chow2018path} from $\alpha=2$ to general $\alpha$.


% \subsection{Indifference Condition}\label{sec:indifference}
% For the optimal policy $\opt(a|s)$ in a given \gls{MDP}, \citet{ortega2014adversarial} additionally state an \textit{indifference condition} across actions, which is a well-known property of Nash equilibria in game theory \citep{osborne1994course}.   
% In particular, the adversarial objective has the same value for each action $a \in \mathcal{A}$ in state  $s \in \mathcal{S}$ (see \myapp{indifference}).   
% We can see in \cref{fig:perturb_opt}(a) that the perturbed rewards for each action match the value function $V_*(s)$ in each state.     
% While it is possible to derive an adversarial interpretation for any $\pi(a|s)$ using \cref{eq:pedro_form}, we see in \cref{fig:perturb_opt}(b) that the indifference condition does not hold for suboptimal policies.  

% can be interpreted as the \textit{certainty equivalent} \citep{myerson2019probability, ortega2013thermodynamics}, %myerson2019probability,
% which aggregates over actions $a \in \mathcal{A}$ to measure the payoff of a two-player game where the agent begins in state $s \in \mathcal{S}$ and plays against an adversary defined by the regularizer $\Omega_{\pi}(\pi)$ and strength $\beta$ as in \myprop{perturbations} \citep{ortega2014adversarial}.

==> Reward Robustness TMLR (3)/sections/new/4_entropy_related.tex <==
\headerv
\section{Discussion}\label{sec:entropy_vs_div} \label{sec:discussion}
\headerv
Our analysis in \mysec{adversarial_perturb}
% -\ref{sec:visualizations} 
unifies and extends several previous works analyzing the reward robustness of regularized policies \citep{ortega2014adversarial, eysenbach2021maximum, husain2021regularized}, as summarized in \mytab{novelty}.   \revhl{We highlight differences in the analysis of 
entropy-regularized policies 
% \citep{eysenbach2021maximum, lee2019tsallis} 
in \mysec{entropy_vs_div}, and provide additional discussion of the closely-related work of \citet{derman2021twice} in \mysec{related}.
}
% We summarize our contributions with respect 
% these works in \mytab{novelty}, with additional discussion in relation to the related work of \citet{derman2021twice} in \mysec{related}.
% Our analysis in \mysec{adversarial_perturb}
% % -\ref{sec:visualizations} 
% unifies and extends several previous works which analyze the reward robustness of regularized policies \citep{ortega2014adversarial, eysenbach2021maximum, husain2021regularized}.    We summarize our contributions with respect 
% these works in \mytab{novelty}, with additional discussion in relation to the related work of \citet{derman2021twice} in \mysec{related}.
% to previous work in \mytab{novelty}, with additional discussion below.
% and additionally discuss relationships with \citet{derman2021twice} in \mysec{related}.
% Several previous works have analyzed the reward robustness of regularized policies, and we summarize our contributions with respect to these works in \cref{table:novelty}.  

% First, our analysis extends \citet{ortega2014adversarial} to the sequential case and alternative regularizers.
% Compared with \citet{eysenbach2021maximum}, we \textcolor{red}{correct} the feasible set of perturbations $\mathcal{R}$ (see \myapp{eysenbach}), and associate robustness properties with a particular, possibly suboptimal policy rather than an environmental reward.  We emphasize this `policy form' of the worst-case reward perturbations in \myprop{optimal_perturbations}, and note that our robustness corresponds with a given reward function only in the case of the \textit{optimal} policy.  \citet{husain2021regularized} provide results for general convex regularization which mirror the `value form' of the worst-case perturbations in \myprop{advantage}, but these also hold only at optimality in a given \textsc{mdp}.   Our focus on specific policy regularization objectives and the robust set $\mathcal{R}$ extends the analysis of \citet{husain2021regularized}, while our experiments in \mysec{visualizations} reflect the theoretical results more directly than previous works.

\headerv
 \subsection{Comparison with Entropy Regularization }\label{sec:entropy_vs_div}
 \headerv
% \vspace*{\header}
% \paragraph{Comparison with Entropy Regularization} 
% \RB{Paragraph or Section?}
% \JG{This whole section is absolutely amazing. Thanks!} 
As argued in \mysec{adversarial_perturb}, the worst-case reward perturbations preserve the value of the regularized objective function.  Thus, we should expect our robustness conclusions to depend on the exact form of the regularizer.

% \input{sections/related_work_table}

% \headerv
% \begin{figure*}[t]
% \vspace*{-.2cm}
% \centering
% \resizebox{\textwidth}{!}
% {
% \begin{tabular}{lcccc}
%     &  \text{ \citet{ortega2014adversarial}} & \text{\citet{eysenbach2021maximum}} &  \text{ \citet{husain2021regularized}} & Ours \\ \toprule
%     \bullets{Multi-Step Analysis} & \tcminus{\xmark} & \tcplus{\cmark} & \tcplus{\cmark} & \tcplus{\cmark} \\ 
%     \bullets{Worst-Case $\propt(a,s)$} & \tcminus{policy form} & \tcminus{policy form} & \tcminus{value form} & \tcplus{policy \& value forms} \\ 
%   \bullets{Feasible Set} & \tcminus{\xmark} & 
%     \tcplus{\cmark} \, \,  \tcminus{(see our App G)} & \tcminus{\xmark} & \tcplus{\cmark} \\ 
%   \bullets{Divergence Used} & \tcminus{KL ($\alpha = 1$)} & \tcminus{\text{ Shannon entropy (see Sec  5.1)}} & \tcplus{any convex $\Omega$} & \tcplus{$\alpha$-Div.} \\ 
%     \bullets{$\mu(a,s)$ or $\pi(a|s)$ Reg.?} & (= in single step) & $\pi(a|s)$ & \tcplus{Both} & \tcplus{Both} \\
%     \bullets{Indifference} & \tcplus{\cmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}  \\ 
%     \bullets{Path Consistency} & \tcminus{\xmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}  \\ 
%     \bottomrule
% \end{tabular}
% }
% \vspace*{-.3cm}
% \caption{Comparison to related work. }\label{table:novelty}
% \end{figure*}


When regularizing with the Tsallis or Shannon ($\alpha = 1$) entropy, the worst-case reward perturbations become %perturbed reward is %reward
\small
\begin{align}
    % \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \pi(a|s) \,. \label{eq:ptwise_perturb_ent}
    \hspace*{-.2cm} \prpi(a,s) = \frac{1}{\beta} \log_{\alpha} \pi(a|s) + \frac{1}{\beta} \frac{1}{\alpha} \Big(1 - 
    \sum_{a \in \mathcal{A}} \pi(a|s)^{\alpha} \Big) \,. \label{eq:ptwise_perturb_ent}
\end{align}
\normalsize
% \RB{Change with new $\propt$}
%For entropy regularization,
See \myapp{entropy_nonnegative}, we also show that for $0 < \alpha \leq 1$,
% , which includes the Shannon entropy,
these perturbations cannot decrease the reward, with $-\prpi(a,s) \geq 0$ and $\mr_{\pi}(a,s) \geq r(a,s)$.
% these reward perturbations are nonpositive in each state action pair and lead to increased modified rewards $\mrpi(a,s) \geq r(a,s)$.
% In \myapp{entropy_nonnegative}, we show that these perturbations yield a pointwise non-negative contribution to the objective $r(a,s) - \prpi(a,s)$, with $-\prpi(a,s) \geq 0$ for $0 < \alpha \leq 1$.    %$\pi(a|s) \leq 1$, f
% % \RB{Why does Lee result hold for any $\alpha$?}
%  ONLY} 
% In the following,
In the rest of this section, we
% We
argue that this property leads to several unsatisfying conclusions in previous work \citep{lee2019tsallis, eysenbach2021maximum}, which are resolved by using the \textsc{kl} and $\alpha$-divergence for analysis instead of the corresponding entropic quantities.\footnote{Entropy regularization corresponds to divergence regularization with the uniform reference distribution $\pi_0(a|s)$.}

% We argue the pointwise non-negative contribution of these perturbations to the objective $r(a,s) - \propt(a,s)$, with $-\propt(a,s) \geq 0$ for $\pi(a|s) \leq 1$, leads to several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}.   As we discuss in the following, this is resolved by using the \textsc{kl} and $\alpha$-divergence instead of the corresponding entropic quantities for the analysis. \footnote{Entropy regularization corresponds to the divergence to the uniform reference distribution $\pi_0(a|s)$ over actions.}
% In particular, entropy regularization should be considered as a divergence to the uniform reference distribution $\pi_0(a|s)$ over actions.
%Our use of the \textsc{kl} and} $\alpha$-divergences, instead of the corresponding entropic quantities, resolves several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}.   
First, 
% analysis in terms of Shannon entropy regularization suggests that the policy is only
this means that a Shannon entropy-regularized policy is only
% appears to only be 
`robust' to \textit{increases} in the reward function.   However, for useful generalization, we might hope that a policy still performs well when the reward function decreases in at least some states. 
 Including the reference distribution via divergence regularization resolves this issue,
%  changes this property, 
 and we observe in \myfig{feasible_set_main} and \myfig{pyco} that the adversary 
%  typically 
 chooses reward decreases in some actions and increases in others.  For example, for the \textsc{kl} divergence, $\prpiopt(a,s) = \frac{1}{\beta}\log \frac{\piopt(a|s)}{\pi_0(a|s)} = Q_*(a,s) - V_*(s)$ implies robustness to reward decreases when $\piopt(a|s) > \pi_0(a|s)$ or $Q_*(a,s) > V_*(s)$.
 
%  so that the worst-case perturbation $\propt(a,s) = \frac{1}{\beta}\log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}$ %\frac{\pi(a|s)}{ \pi_0(a|s)}$ % yields robustness to reward \textit{decreases} when $\pi(a|s) > \pi_0(a|s)$ and reward increases otherwise.  
% Indeed, using divergence regularization, we observe in \cref{fig:perturb_opt} and \ref{fig:pyco} that the adversary typically chooses reward decreases in some actions and increases in others.  
% , and proceed to further investigate this property in the next subsection.
% For useful zero-shot generalization


% Including the reference distribution as in \myprop{feasible} changes this property, so that the worst-case perturbation $\propt(a,s) = \frac{1}{\beta}\log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}$ %\frac{\pi(a|s)}{ \pi_0(a|s)}$ % yields robustness to reward \textit{decreases} when $\pi(a|s) > \pi_0(a|s)$ and reward increases otherwise.  
% \RB{Include that we would like to be robust to decreases for useful generalization}

Similarly, \citet{lee2019tsallis} note that for any $\alpha$,%$\frac{1}{\beta}\Omega^{*}_{\pi_0}(\discussiondual) = \max_{\pi(a|s)} \langle \pi(a|s), \discussiondual(a,s) \rangle + \frac{1}{\beta} H_{\alpha}(\pi) \geq \discussiondual(a_{\max}, s) $
\small
\begin{align*}
    \frac{1}{\beta}\Omega^{*(H_{\alpha})}_{\beta}(\discussiondual) = %\max_{\pi(a|s)}
    \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \langle \pi, \discussiondual \rangle + \frac{1}{\beta} H_{\alpha}(\pi) \geq \discussiondual(a_{\max}, s) 
    % \left(-\frac{1}{\beta} H_{\alpha}(\pi)\right)
\end{align*}
\normalsize
\normalsize
where $a_{\max} = \argmax_a \discussiondual(a,s)$ and the Tsallis entropy $H_{\alpha}(\pi)$ equals the Shannon entropy for $\alpha = 1$. 
% \RB{Soft Value, $\pi$ optimization}
% \textcolor{red}{Due to the pointwise non-negativity of $-\log_{\alpha}\pi(a|s)$ in the (Tsallis) entropy,  this soft value aggregation 
% % with the negative Tsallis entropy as a regularizer,  
% yields a result that is \textit{larger} than any particular $Q$-value. }
This soft value aggregation yields a result that is \textit{larger} than any particular $Q$-value. 
% Due to the pointwise non-negativity of the 
%so that soft value aggregation yields a value which is \textit{larger} than any particular reward. 
% \begin{align}
%     \max_{\pi(a|s)} \langle \pi(a|s), \discussiondual(a,s) \rangle + \beta H_q(\pi) \geq \max_a \discussiondual(a,s)
% \end{align}
% where $H_q$ is the Tsallis entropy.
By contrast, for the $\alpha$-divergence, we show in \myapp{qmax} that for fixed $\beta$ and $\alpha > 0$,
% \footnotesize
% \begin{align*}
%   \hspace*{-.1cm} \discussiondual(a_{\max},s) + \frac{1}{\beta}\frac{1}{\alpha} \log_{\alpha} \pi(a_{\max}| s) \leq \alphaconjn(\discussiondual) \leq  \discussiondual(a_{\max},s)
% \end{align*}
 \small
\begin{equation}
% \resizebox{\columnwidth}{!}{ $
\discussiondual(a_{\max},s) + \frac{1}{\beta}\frac{1}{\alpha} \log_{2-\alpha} \pi(a_{\max}| s) \leq \alphaconj(\discussiondual) \leq  \discussiondual(a_{\max},s) 
% $ } 
.
\end{equation}
\normalsize
This provides a more natural interpretation of the Bellman optimality operator $V(s) \leftarrow \alphaconj(Q)$ as a soft maximum operation.   As a function of $\beta$, we see in \myapp{alpha_results} and \ref{app:qmax} that the conjugate ranges between $\mathbb{E}_{\pi_0}[\discussiondual(a_{\max},s)] \leq \alphaconj(Q) \leq \discussiondual(a_{\max},s)$.
% \cref{fig:perturb_opt}.

Finally, using entropy instead of divergence regularization also affects interpretations of the feasible set.  %For entropy regularization,
\citet{eysenbach2021maximum} consider the same constraint as in \cref{eq:kl_feasible}, but without the reference $\pi_0(a|s)$
% distribution
\small
\begin{align}
    \sum \limits_{a \in \mathcal{A}} \expof{\beta \cdot \pr(a,s)} \leq 1  \, \quad \forall s \in \mathcal{S} \, . \label{eq:ent_constraint}
\end{align}
\normalsize
This constraint suggests that the original reward function ($\pr = 0$) is not feasible for the adversary.  
% , unless the policy is deterministic
More surprisingly, \citet{eysenbach2021maximum} App. A8 argues that \textit{increasing} regularization strength (with lower $\beta$) may lead to \textit{less} robust policies based on the constraint in \cref{eq:ent_constraint}.    In \myapp{eysenbach}, we discuss how including $\pi_0(a|s)$ in the constraint via divergence regularization (\myprop{feasible}) avoids this conclusion.   As expected, 
% we observe in 
% \cref{fig:feasible_set_main} that increasing regularization strength leads to more robust policies.
\cref{fig:feasible_set_main} shows that increasing regularization strength leads to more robust policies.

% \subsection{Adversarial Modified Rewards}\label{sec:husain}
% \vspace*{\header}
% The adversarial interpretation in the previous sections may also be written directly using the modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$, which has been studied in a more general setting by \citet{husain2021regularized}.

% \citet{husain2021regularized} consider maximizing an arbitrary concave objective $\concaveopt$, and proceed to derive its convex conjugate $(-\concaveopt)^*$.    Translated to our setting and notation,
% this involves the conjugate expansion of the regularized objective $(-\obj_{\Omega, \beta}(r))^*$ instead of the conjugate of the regularizer only, $ (\omegamu)^*$.  
% With detailed derivations in \myapp{husain_conjugate}, this leads to the Lagrangian
% \begin{align}
%     \hspace*{-.2cm} & \quad \max \limits_{\mu(a,s)} \min \limits_{V(s)} \min \limits_{\textcolor{\highlight}{\mr(a,s)}} \, \label{eq:husain_form} \\
%     & \big \langle {\mu(s)\pi(a|s)}, {\textcolor{\highlight}{\mr(a,s)} +\gamma \transitionv - V(s) } \brangle  \nonumber  \\
%     & \quad+ \alphaconjn \big( r(a,s) - \textcolor{\highlight}{\mr(a,s)} \big) + (1-\gamma) \blangle \nu_0(s), V(s) \brangle \, ,  \nonumber
% \end{align}
% which matches \cref{eq:pedro_form} up to simple reparameterization of $\mr(a,s) = r(a,s) - \pr(a,s)$.

% Differentiating \cref{eq:husain_form} with respect to $\pi(a|s)$ and solving for the optimal modified rewards yields the result of \citet{husain2021regularized} that
% \begin{align}
%   \mropt(a,s) = V(s) - \gamma \transitionv  %\quad \forall (a,s) \in (\mathcal{A}, \mathcal{S})
% \end{align}
% Adding the environment reward, we can use the optimal reward perturbations $\propt(a,s) = r(a,s) - \mropt(a,s)$ to rewrite this expression
% \begin{align}
% \propt(a,s) &=  r(a,s) + \gamma \transitionv -  V(s) \label{eq:modified_reward_opt}
% \end{align}
% which matches our advantage function interpretation in 
% % \mysec{advantage} 
% \myprop{advantage}.

% \input{sections/related_work_table_no_derman}
% \subsection{Relation to Existing Algorithms}
% \vspace*{-.05cm}
\headerv
\subsection{Related Algorithms}\label{sec:related}
\headerv
% \subsection{Algorithmic Implications}\label{sec:related}
% \subsection{Related Work}\label{sec:related}
% \paragraph{Related Work / Algorithmic Implications}
% directly reflect theoretical findings.
% our theoretical results.
% \RB{Experiments match theory}
% Finally, the experimental validation in \citet{husain2021regularized}
Several recent works provide algorithmic insights which build upon convex duality 
and complement or extend our analysis.  
%nicely 
\revhl{\citet{derman2021twice} 
derive practical iterative algorithms based on a general equivalence between robustness and regularization, which can be used to enforce
% both reward robustness and dynamics robustness.  
robustness to \textit{both} reward perturbations (through policy regularization) and changes in environment dynamics (through value regularization).
%  The approach of \citet{derman2021twice} translates the definition of a desired robust set into a regularization function using the conjugate function of the set indicator function.
%   Starting from a desired robust set, \citet{derman2021twice} use the support function (as the conjugate of the set indicator function) to translate 
%   into a regularization function.
 For policy regularization, \citet{derman2021twice} translate
%   \citet{derman2021twice} translate from 
  the specification of a desired robust set 
 % translates to 
  into
  a regularizer using the convex conjugate of the set indicator function.   In particular, \citet{derman2021twice} associate \textsc{kl} divergence or (scaled) Tsallis entropy policy regularization with the robust set $\mathcal{R}^{\Delta}_{\pi} \coloneqq \{ 
% \prrob \in \rprimedomain  \, | \, 
\prrob \, | \,
\prrob(a,s) \in [\frac{1}{\beta} \frac{1}{\alpha} \log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}, \infty) \, \, \forall \,  (a,s) \in  \mathcal{A} \times \mathcal{S}\}$.
% For \textsc{kl} divergence and Tsallis entropy regularization, \citet{derman2021twice} consider the robust set $\mathcal{R}^{\Delta}_{\pi} \coloneqq \{ 
% % \prrob \in \rprimedomain  \, | \, 
% \prrob \in (\frac{1}{\alpha} \log_{\alpha} \pi(a|s), \infty) \, \, \forall \, \, (a,s) \in  \mathcal{A} \times \mathcal{S}\}$, which is translated to a regularization using the support function, or convex conjugate of the indicator function of this set.
% For \textsc{kl} divergence and Tsallis entropy regularization, the approach of \citet{derman2021twice} yields a robust set whose boundary is based on each conditional action probability $\pi(a|s)$, as shown in \myfig{related}. 
% In particular, \citet{derman2021twice} analyze a \textit{rectangular} robust set whose boundary is based on each conditional action probability $\pi(a|s)$, as shown in \myfig{related}. 
% \cref{fig:derman}.
Our analysis proceeds in the opposite direction, from regularization to robustness, 
using the conjugate of the divergence.    While the worst-case perturbations 
result in the same modified objective, 
our approach
% using the conjugate of the divergence function
% based on the conjugate of the divergence 
yields a larger robust set with qualitatively different shape (see \myfig{related}).}
%Depending on the problem setting, it may be more natural to think about robustness or regularization first.
%\textcolor{\shiehl}{
%Our approaches are complementary, in the sense that starting from robustness or regularization may be more insightful depending on the problem setting.}
%Depending on the problem setting, it may be more insightful to specify the desired robustness
%Depending on the setting, starting from regularization or insightful for deriving new analysis tools or algorithms.}
%textcolor{\shiehl}{In the end, either direction may be insightful for deriving new analysis tools or algorithms.}
% % which is defined based on each individual state-action pair. 
% % Further, 
% Our constraint defining the robust set in \myprop{optimal_perturbations} is based on the conjugate function of the regularizer itself, which \textit{jointly} considers all actions in particular state.  
% % By contrast,   
% In \cref{fig:feasible_set_main}, we can see that our robust set is in fact larger than \citet{derman2021twice} and has a qualitatively different shape.
% \sout{Starting with a desired robust set of reward perturbations, the convex conjugate of the 
% indicator 
% % or characteristic 
% function is used to derive an appropriate regularized Bellman operator and modified policy iteration algorithm \citep{geist2019theory}.  
% %  While this approach allows for flexible specification of robust sets, it leads to 
% %  our \myprop{optimal_perturbations} 
% Our analysis proceeds in the opposite direction, from regularization to robustness.  Notably, this approach yields a larger robust set with qualitatively different shape.    
% In particular, \citet{derman2021twice} obtain a \textit{rectangular} robust set which is defined based on each individual state-action pair. }
% % Furthermore, our definition of the robust set is related to the conjugate function of the regularizer itself, instead of the conjugate of the set indicator function as in \citet{derman2021twice}.


% has several notable differences. In particular, our definition of the robust set in \myprop{optimal_perturbations} involves the conjugate function of the regularizer itself, and the constraint is calculated for each state, 
% .  As shown in \myfig{feasible_set_main}, this leads to a different robust set
% even in special cases

% rather than for each state-action pair in . 

% \RB{are our robust sets larger?  Actually do differ}
% %The latter observation appears to arise from the normalization constraint of the policy $\pi(a|s)$ (see \cref{sec:conj_examples}).
% Our constraints defined using the conjugate function of the regularizer itself.
% While this approach allows for flexible specification of robust sets, our \myprop{optimal_perturbations} 
% This approach allows for efficient algorithms with flexible specification of robust sets    


% \citet{derman2021twice} must specify the 
% \citet{derman2021twice} construct the the sets corresponding to common policy regularizers in bespoke fashion without the generality or conjugate perspective from our \myprop{optimal_perturbations} and \myprop{feasible}.


\citet{zahavy2021reward} analyze a general `meta-algorithm' which alternates between updates of the occupancy measure $\mu(a,s)$ and modified reward $\mr(a,s)$ in online fashion.
This approach highlights the fact that the modified reward $\mr_{\pi}$ or worst-case perturbations $\prpi$ change as the policy or occupancy measure is optimized.  
The results of \citet{zahavy2021reward} and \citet{husain2021regularized} hold for general convex \gls{MDP}s, which encompass common exploration and imitation learning objectives beyond the policy regularization setting
we consider.
% ed here.
% The convex \gls{MDP} setting of \citet{zahavy2021reward} matches \citet{husain2021regularized}, encompassing common exploration and imitation learning objectives as special cases in addition to the standard regularized \textsc{rl} problems considered here.
% The results of \citet{zahavy2021reward} encompass numerous common algorithms as special cases, including standard regularized \textsc{rl} problems discussed here.

As discussed in \mysec{optimal_policy}, path consistency conditions have been used to derive practical learning objectives in \citep{nachum2017bridging, chow2018path}.   These algorithms might be extended to general $\alpha$-divergence regularization via \cref{eq:path}, which involves an arbitrary reference policy $\pi_0(a|s)$ that can be learned adaptively as in \citep{teh2017distral, grau2018soft}.


Finally, previous work has used dual optimizations similar to \cref{eq:dual_reg} to derive alternative Bellman error losses \citep{dai2018sbeed, belousov2019entropic, nachum2020reinforcement, basserrano2021logistic}, highlighting how convex duality can be used to bridge between policy regularization and Bellman error aggregation \citep{belousov2019entropic, husain2021regularized}.




% We leave exploring the implicia
% and a full exploration of the relationship between alternative Bellman error losses and policy regularization \citep{husain2021regularized}.

% Finally, we note that previous work \citep{lee2019stochastic, basserrano2021logistic} has considered relaxed \gls{LP} formulations of \gls{MDP}s involving redundant constraints on an auxiliary, or `mirror-image' state-occupancy measure $d(a,s)$.   This conveniently allows for the introduction of state-action $Q$-values as Lagrange multipliers to enforce the constraint that $\mu(a,s) = d(a,s)$ and has been used to derive alternative Bellman error losses \citep{dai2018sbeed, nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.   In \myapp{logistic_q}, we show a similar formulation may be obtained using a further conjugate expansion of $\alphaconjmu$ in \cref{eq:pedro_form}, so that our conjugate duality approach may provide an alternative perspective on these \gls{LP} relaxations. 

% and may be useful in \textcolor{red}{xyz....} 
% \textcolor{red}{and may be useful in analyzing practical deep $Q$-learning algorithms such as \textsc{dqn} \citep{mnih2015human} and \textsc{a3c} \citep{mnih2016asynchronous}, whose convergence properties are not well understood.} (\RB{CHECK})


% in \myapp{logistic_q}, 
% Finally, our advantage function interpretation suggests conjugate representations may provide justification for including learned $Q$-values as dual variables in convex programming forms of \gls{MDP}s.

% The regret bounds and sample complexity results 
% The convex \textsc{mdp} framework of \citet{zahavy2021reward} includes numerous common algorithms as special cases, including standard regularized \textsc{rl} problems 
% and \citet{husain2021regularized}.
% considered here.  Indeed, the results of \citet{husain2021regularized} hold for a general convex \textsc{mdp}s (see \myapp{husain_conjugate}).   

% Their framework contains numerous common algorithms as special cases, but should also include the standard convex-regularized \textsc{rl} problems considered here and in \citet{husain2021regularized}.

% `policy form' for the worst-case reward perturbations in \myprop{optimal_perturbations} with \textit{any} stochastic policy.   The robustness associated with the feasbile  

% While \citet{husain2021regularized}

% \citet{husain2021regularized, zahavy2021reward} provide results for the case of maximizing a general concave function of the joint state-action occupancy distribution $\mu(a,s)$, which includes the (linear) expected reward with convex regularization as a special case.   
% However, \citet{husain2021regularized} do not include detailed discussion of policy regularization schemes, 
% % $\pi(a|s)$ schemes most widely used in practice.





==> Reward Robustness TMLR (3)/sections/new/4_vis_feasible.tex <==
In \myfig{feasible_set_main}, we visualize the robust set of perturbed rewards for the optimal policy in a two-dimensional action space for the \textsc{kl} or $\alpha$-divergence, various $\beta$, and a uniform or non-uniform prior policy $\pi_0$.
Since the optimal policy can be easily calculated in the single-step case, we consider fixed $Q_*(a,s) = r(a,s) = \{1.1, 0.8\}$ and show the robustness of the optimal $\pi_*(a|s)$, which differs based on the choice of regularization scheme using \cref{eq:optimal_policy}.
% (see \cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).
We determine the feasible set of $\prrobust$ using the constraint in \myprop{feasible} (see \myapp{feasible_plot} for details), and plot the modified reward $\mr_{\piopt}(a,s) = Q_*(a,s) - \proptpi(a,s)$ for each action.  
%  For clarify of exposition, we focus on the \KL divergence constraint in \cref{eq:kl_feasible}.

Inspecting the constraint for the adversary 
in \cref{eq:kl_feasible}, note that both reward increases $\prrobust(a,s) < 0$ and reward decreases $\prrobust(a,s) > 0$ contribute non-negative terms at each action, which either up- or down-weight the reference policy $\pi_0(a|s)$.  The constraint on their summation forces the adversary to trade off between perturbations of different actions in a particular state.   
Further, since the constraints in \myprop{feasible} integrate over the action space, the rewards for \textit{all} actions in a particular state must be perturbed together.  
While it is clear that increasing the reward in both actions preserves the inequality in \cref{eq:generalization},  
% is feasible for an adversary that minimizes \cref{eq:pedro_form}, 
\cref{fig:feasible_set_main} also includes regions where one reward decreases.
% While it is natural that increasing the reward in both actions is feasible for an adversary that minimizes \cref{eq:pedro_form}, \cref{fig:feasible_set_main} also includes regions where one reward decreases.
% In all cases, it is natural that increasing the reward in both actions is feasible for an adversary seeking to minimize the objective in \cref{eq:pedro_form}.

For high regularization strength ($\beta=0.1$), we observe that the boundary of the feasible set is nearly linear, with the slope $-\frac{\pi_0(a_1|s)}{\pi_0(a_2|s)}$ based on the ratio of 
action probabilities in a policy that matches the prior.  
The boundary steepens for lower regularization strength.  {We can use the indifference condition to provide further geometric insight.   First, drawing a line from the origin with slope $1$ will intersect the feasible set at the worst-case modified reward (red star) in each panel, with $\mrrobust(a_1,s) = \mrrobust(a_2,s)$.  At this point, the slope of the tangent line yields the ratio of action probabilities in the regularized policy, as we saw for the $\beta = 0.1$ case.  With decreasing regularization as $\beta \rightarrow \infty$, the slope approaches $0$ or $-\infty$ for a nearly deterministic policy and a rectangular feasible region.} 
% \RB{Where does InDifference go?}
% ince we have plotted the optimal policy $\piopt(a|s)$ corresponding to the reward function $r(a,s)$, we can see that the indifference condition holds, with $\mropt(a_1,s) = \mropt(a_2,s)$ for the red star in each panel.   In this case, we ca  

Finally, we show the $\alpha$-divergence robust set with $\alpha \in \{-1, 3\}$ and $\beta = 10$ in \cref{fig:feasible_set_main} (d)-(e) and (i)-(j), with further visualizations in \myapp{additional_feasible}.  
%%%%%%%%%%%%% WITH LAMBDA for INDIFFERENCE %%%%%%%%%%%%%
% Compared to the \textsc{kl} divergence, we find a wider robust set boundary for $\alpha =-1$ and a more strict boundary for $\alpha = 3$.
%%%%%%%%%%%%% WITHOUT LAMBDA / Without INDIFFERENCE %%%%%%%%%%%%%
Compared to the \textsc{kl} divergence, we find a wider robust set boundary for $\alpha =-1$.   For $\alpha = 3$ and $\beta=10$, the boundary is more strict and we observe much smaller reward perturbations as the optimal policy becomes deterministic ($\pi(a_1|s) = 1$) for both reference distributions.    
However, in contrast to the unregularized deterministic policy, the reward perturbations $\proptpi(a,s) \neq 0$ are nonzero.
% as we confirm with a worked example in \myapp{deterministic_alpha},
We provide a worked example in \myapp{deterministic_alpha}, and note that 
indifference does not hold in this case, $\mr_{\piopt}(a_1,s) \neq \mr_{\piopt}(a_2,s)$, due to the Lagrange multiplier $\lambda_*(a_2,s)>0$. % (see \mysec{value_form})
% the optimal policy sets $\pi_*(a_2,s)=0$ for both reference distributions.   
% However, $V_*(s) \neq \max_a Q_*(a,s) = 1.1$ in this case.   Instead, $V_*(s) = \psiq - \psipi = 0.95 + .10$
% This leads to smaller worst-case reward perturbations

==> Reward Robustness TMLR (3)/sections/new/4_visualizations.tex <==
% \section{Visualizations}\label{sec:visualizations}
%  \headerv


\headerv
\section{Experiments}\label{sec:visualizations}
\headerv
In this section, we visualize the robust set and worst-case reward perturbations associated with policy regularization, using intuitive examples to highlight theoretical properties of our adversarial interpretation.  
% Our experiments more directly reflect the theoretical properties of 
% % this robustness
% our adversarial robustness
% compared to previous work \citep{husain2021regularized, eysenbach2021maximum}.

\input{sections/feasible_fig_no_lambda}
% \input{sections/feasible_fig}

\headerv
\subsection{Visualizing the Robust Set}\label{sec:visualizations_feasible}
% \vspace*{-.1cm}
\headerv

\input{sections/new/4_vis_feasible}
\input{sections/single_step_fig}

% \headerv
% \headerv
\subsection{Visualizing the Worst-Case Reward Perturbations}\label{sec:visualizations_worst_case}
\headerv
% For the experiments 
In this section, we consider \textsc{kl} divergence regularization to a uniform reference policy, which is equivalent to Shannon entropy regularization but more appropriate for analysis, as we discuss in \mysec{entropy_vs_div}. 
% maximum Shannon entropy regularization with various regularization strength $\beta$.   However, for the purposes of analysis, we
\headerv
\paragraph{Single Step Case}
In \cref{fig:perturb_opt}, we plot the \textit{negative} worst-case reward perturbations $-\pr_{\pi}(a,s)$ and modified reward for a single step decision-making case.   For the optimal policy in \cref{fig:perturb_opt}(a), the perturbations match the advantage function as in \cref{eq:advantage} and the perturbed reward for all actions matches the value function $V_*(s)$. 
While we have shown in \mysec{any_policy} that any stochastic policy may be given an adversarial interpretation, we see in \cref{fig:perturb_opt}(b) that the indifference condition does not hold for suboptimal policies.  

The nearly-deterministic policy in \myfig{perturb_opt}(a)(ii) also provides intuition for the unregularized case as {$\beta \rightarrow \infty$}. 
Although we saw in \mysec{value_form} that $\pr_{\piopt}(a,s) = 0 \,\, \forall a$ 
% for all $a$
% \, \forall a$
in the unregularized case,  \cref{eq:dual_lp} and (\ref{eq:advantage}) suggest that $\lambdaplus = V_*(s) - Q_*(a,s)$ plays a similar role to the (negative) reward perturbations in \myfig{perturb_opt}(a)(ii), with $\lambda(a_1,s)=0$ and $\lambda(a,s)>0$ for all other actions. 


% Although we saw in \mysec{value_form} that $\pr_{\piopt}(a,s) = 0$ for all $a$ in the unregularized case,  \cref{eq:dual_lp} and (\ref{eq:advantage}) suggest that $\lambdaplus = V_*(s) - Q_*(a,s)$, with $\lambda(a_1,s)=0$ and $\lambda(a,s)>0$ for all other actions.  Thus, in the limit as $\beta \rightarrow \infty$, the role of the  may be viewed as the limiting behavior of $\pr_{\piopt}(a,s)$
% First, since \textsc{kl} regularization with finite $\beta$ and bounded advantages cannot set $\piopt(a|s) = 0$ in \cref{eq:optimal_policy}, we have $\lambdaplus = 0$ for all $a$ in the regularized case.  \myprop{advantage} thus implies that $-\pr_{\piopt}(a,s) = V_*(s) - Q_*(a,s)$.
% With $\beta=10$, 
% For $a_1= \argmax_a  Q_*(a,s)$, $\lambdaplus =0$.
% we can compare the nearly deterministic policy in \myfig{perturb_opt}(a)(ii) with the unregularized case ($\beta \rightarrow \infty$)
% provides valuable intuition for the unregularized case ($\beta \rightarrow \infty$).  
% % provides intuition for the limiting behavior of our analysis as $\beta \rightarrow \infty$. 
% With \textsc{kl} divergence regularization and finite $\beta$, $\lambdaplus = 0$ since the exponential function cannot set action probabilities to 0 unless $V_*(s) - Q_*(a,s) \rightarrow \infty$ (see \cref{eq:optimal_policy}).  By \myprop{advantage}, this implies $-\pr_{\piopt}(a,s) = V_*(s)-Q_*(a,s)$



% Although $\prv(a,s) = 0$ for all $(a,s)$ in the unregularized case (see \mysec{value_form}), we can view the Lagrange multipliers $\lambdaplus = V_*(s)-Q_*(a,s) \geq 0$ as playing a similar role as $-\prv(a,s)$ (.  In particular,  $\lambdaplus = V_*(s)-Q_*(a,s) \geq 0$ for the optimal unregularized value $V_*(s) \coloneq \argmax_a Q(a,s)$.   In the \myfig{perturb_opt} example, this implies $\piopt(a_1|s)=1$ and $\lambdaplus(a_1, s)=0$ for the optimal action, whereas $\lambdaplus = V_*(s)-Q_*(a,s)$


% Recall from \cref{eq:dual_lp} that $\lambdaplus = V_*(s)-Q_*(a,s) \geq 0$ for the optimal unregularized value $V_*(s) \coloneq \argmax_a Q(a,s)$. 


% Nevertheless, we will see that   




% In the \myfig{perturb_opt} example, this implies $\piopt(a_1|s)=1$ and $\lambdaplus(a_1, s)=0$



% Finally, we compare the role of $\lambdaplus$ and $\pr(a,s)$ for the nearly deterministic policy in \myfig{perturb_opt}(a)(ii).  
% Recall from \cref{eq:dual_lp} and \mysec{optimal_policy} that, for an optimal \textit{unregularized} policy, we have $\lambdaplus = V_*(s)-Q_*(a,s) > 0$ for actions $a_{2:6}$.   With \textsc{kl} divergence regularization and finite $\beta$, $\lambdaplus = 0$ since the exponential function cannot set action probabilities to 0 unless $V_*(s) - Q_*(a,s) \rightarrow \infty$ (see \cref{eq:optimal_policy}).   
% From \myfig{perturb_opt}(a)(ii) and \myprop{advantage}, we can see that $-\pr_{\piopt}(a,s) = V_*(s) - Q_*(a,s)$ captures the advantage function in the low regularization regime.
% % In  \cref{fig:perturb_opt}(a)(ii), 


% Since the exponential function cannot set actions to 0 unless $Q_*(a,s) -V_*(s) \rightarrow -\infty$, the perturbations $\pr(a,s)$ from 

% 

% \RB{Add reference to Unregularized Case / Lagrange multiplier}
% While it is possible to derive an adversarial interpretation for any $\pi(a|s)$ using \cref{eq:pedro_form}, we see in \cref{fig:perturb_opt}(b) that the indifference condition does not hold for suboptimal policies.  
% (max Shannon entropy regularization) (max Shannon entropy regularization) 
\headerv
\paragraph{Sequential Setting}
% \headerv
In \cref{fig:pyco}(a), we consider a grid world where the agent receives $+5$ for picking up the reward pill, $-1$ for stepping in water, and zero reward otherwise.  We train an agent 
% \RB{to convergence? no need to mention $\epsilon$-greedy?}   with \textsc{kl} divergence regularization to a uniform reference policy 
using tabular $Q$-learning and a discount factor $\gamma = 0.99$. 
We visualize the worst-case reward perturbations $\prpi(a,s) = \frac{1}{\beta}\log \frac{\pi(a|s)}{\pi_0(a|s)}$ 
in each state-action pair for policies trained with various regularization strengths in \cref{fig:pyco}(b)-(d).  While it is well-known that there exists a unique optimal policy for a given regularized \gls{MDP}, 
our results 
% in \cref{fig:pyco} 
additionally display the adversarial strategies and resulting Nash equilibria which can be associated with a regularization scheme specified by $\Omega$, $\pi_0$, $\alpha$, and $\beta$ in a given \gls{MDP}.

Each policy implicitly hedges against an adversary that perturbs the rewards according to the values and colormap shown.  For example, inspecting the state to the left of the goal state in panel \cref{fig:pyco}(b)-(c), we see that the adversary reduces the immediate reward for moving right (in red, $\proptpi > 0$). 
 Simultaneously, the adversary raises the reward for moving up or down towards the water (in blue).
%  the agent to move up or down towards the water (in blue).  
% Simultaneously, the adversary incentivises the agent to move up or down towards the water and (with weaker strength) further away from the goal, by increasing the rewards for the actions not leading into the goal state (in blue).
This is in line with the constraints on the feasible set, which imply that the adversary must balance reward decreases with reward increases in each state. 
% In general, the adversary increases the rewards for actions leading away from the goal state. 
% not leading into the goal state
% forcing the optimal policy to become indifferent between actions.
% such that the policy tends to become indifferent between the actions.  
In \myapp{optimal_policy_confirm} \cref{fig:pyco_indifference}, we certify the optimality of each policy using the path consistency conditions, which also confirms that the adversarial perturbations have rendered the agent indifferent across actions in each state.
% , satisfying the indifference condition). In \myapp{additional_results} \cref{fig:pyco_indifference}, we confirm the optimality of each policy using the indifference condition.

Although we observe that the agent with high regularization in \cref{fig:pyco}(b) is robust to a strong adversary, the value 
% obtained for the regularized objective 
% , and thus the expected reward of the policy
of the regularized objective is also lower in this case.   As expected, lower regularization strength reduces robustness to negative reward perturbations.
With low regularization in \cref{fig:pyco}(d), 
% the weaker implicit adversary 
% cannot compel 
the behavior of the agent barely deviates from the deterministic policy in the face of the weaker adversary.
% the agent to deviate far from the deterministic policy by modifying the rewards.
% significantly alter the behavior of the agent compared with the deterministic policy.
% cause the agent to significantly deviate from the deterministic optimal policy by modifying the rewards.
% affect the behavior of the agent
%  . significantly  
% Dually, we can say that weakly regularized policies are robust to a smaller set of adversarial reward perturbations. 
% JG{maybe: "Thus for a fixed external adversary, regularized policies will perform better" or similar.}
% (via changing the rewards). 
% Or, expressed dually, the set of reward perturbations to which the policy is robust against is much smaller for weakly regularized policies.  

% Note that Red indicates robustness to negative reward perturbations


% based on $\Omega$, $\pi_0$, and $\beta$.

% \TG{Tabular q-learning, $epsilon$-greedy ($epsilon=0.25$), $\gamma=0.99$, rewarad=1 for picking up the pill, -1 for stepping into the water, and -0.1 otherwise?}

% \myapp{additional_results} \cref{fig:pyco_indifference}

\input{sections/pyco_fig}

==> Reward Robustness TMLR (3)/sections/new/5_conclusion.tex <==
% \vspace*{-.125cm}
\headerv
\section{Conclusion}\label{sec:conclusion}
\headerv
% \vspace*{-.125cm}

In this work, we analyzed the robustness of convex-regularized \gls{RL} policies to worst-case perturbations of the reward function,
which implies generalization to adversarially chosen reward functions from within a particular robust set. 
% From this perspective, policy regularization implies generalization to worst-case reward functions chosen within a particular feasible set. 
% This robustness can be given a natural game-theoretic interpretation, in which the equilibrium indifference condition for the optimal policy highlights that the adversarial perturbations re-express the value of the objective function.  
% The generalization guarantee we get is that for any perturbation to the rewards from the robust set the (fixed) policy is guaranteed to achieve expected rewards that are equal to or higher than the value of the regularized objective.
We have characterized this robust set of reward functions for \textsc{kl} and $\alpha$-divergence regularization, provided a unified discussion of existing works on reward robustness, and clarified apparent differences in robustness arising from entropy versus divergence regularization.
%visualized the strategy of the adversary in a sequential setting,
{Our advantage function interpretation of the worst-case reward perturbations provides a complementary perspective on how $Q$-values appear as dual variables in convex programming forms of regularized \gls{MDP}s.  Compared to a deterministic, unregularized policy, 
% whose value function depends on a single action,
% which considers only $V(s) = \argmax_a Q(a,s)$, 
a stochastic, regularized policy 
places probability mass on a wider set of actions and 
% .   This
% which 
requires state-action value adjustments via the advantage function or adversarial reward perturbations. }
Conversely, a regularized agent, acting based on given $Q$-value estimates, implicitly hedges against the anticipated perturbations of an appropriate adversary.
% we can interpret an agent acting based on $Q$-value estimates and a given regularization scheme to 

% chosen by an implicit adversary.
% We have shown that this behavior may also be interpreted as implicitly hedging against the reward perturbations imposed by an adversary.
% adjustments may also be viewed as implicitly hedging 
% % necessitates per-action value adjustments via the advantage function, which can also be viewed as 
% reward perturbations selected by an implicit adversary.
% Finally, our advantage function interpretation suggests an alternative 
% % justification for
% perspective on 
% including learned $Q$-values as dual variables in convex programming forms of \gls{MDP}s.   Compared to a deterministic, unregularized policy which considers only $V(s) = \argmax_a Q(a,s)$, a stochastic, regularized policy 
% places probability mass on a wider set of actions, which 
% necessitates per-action value adjustments via the advantage function or adversarial reward perturbations.
% % \RB{(Variational optimization)}
% % an provide additional insight into the role of regularization in \gls{RL}.   
% % In particular, our interpretation of the advantage function $Q(a,s)-V(s)$ as a dual variable $\pr(a,s)$ may provide alternative justification for including $Q$-values in regularized \gls{MDP} formulations.
% % Translating these insights into algorithmic improvements, such as policy-regularization versions of alternative Bellman error aggregation \citep{dai2018sbeed, nachum2020reinforcement, belousov2019entropic, basserrano2021logistic} methods derived from convex duality, remains an intriguing direction for future work.
% Translating these insights into algorithmic improvements, 
% % \RB{such as policy-regularization versions of \gls{REPS} and offline learning methods that derive}
% such as extending recent methods that use convex duality to derive alternative Bellman error aggregation objectives \citep{basserrano2021logistic, dai2018sbeed, belousov2019entropic,nachum2020reinforcement} or implementing path consistency objectives beyond \citet{nachum2017bridging, chow2018path}, remains an intriguing direction for future work.
% % by modifying \cref{eq:dual_reg} 

% \RB{some of this included in discussion}

% % Recent work has proposed alternative Bellman error aggregation \citep{dai2018sbeed, nachum2020reinforcement, belousov2019entropic, basserrano2021logistic} using dual optimizations resembling \cref{eq:dual_reg}, but these approaches often incorporate $Q$-values using redundant \gls{LP} constraints \citep{mehta2009q, mehta2020convex, lee2019stochastic, basserrano2021logistic}.  Our interpretation of the advantage function as a dual variable $\pr(a,s)$ may provide alternative justification for including $Q$-values in regularized \gls{MDP} formulations. 
% % Extending these methods to policy regularization settings, potentially using $\alpha$-divergence regularization or learned reference distributions \citep{grau2018soft, galashov2018information}, remains an intriguing direction for future work.

% %  Extending recent work on alternative Bellman error aggregation \citep{dai2018sbeed, nachum2020reinforcement, belousov2019entropic, basserrano2021logistic} to policy regularization settings, 
% % potentially using $\alpha$-divergence regularization or learned reference distributions \citep{grau2018soft, galashov2018information}, remains an intriguing direction for future work.


% At a high level, 
% Our analysis of the reward perturbations $\prpi(a,s)$ provides new perspective on the convex duality relationships underlying regularized \gls{RL} objectives.    Previous work introduces $Q$-values into \gls{LP} forms of regularized \gls{MDP}s using redundant state-action occupancy distributions or constraints \citep{mehta2009q, mehta2020convex, lee2019stochastic, nachum2020reinforcement, basserrano2021logistic} 





==> Reward Robustness TMLR (3)/sections/pyco_fig.tex <==
\begin{figure*}[t]
\vspace*{-1.2cm}
\begin{subfigure}{.2\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_world.pdf} 
% \vspace*{.2cm}
\caption{Environment \\
\small (uniform $\nu_0(s)$, \\
% initial state \\
$r(a,s) = -1$ for water, \\
$r(a,s) = 5$ for goal) \label{fig:pycoa}}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta02_alpha1_gamma99.pdf}
\caption{$\beta = 0.2$ (High Reg.)}\label{fig:pyco_beta02m}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta1_alpha1_gamma99.pdf}
\caption{$\beta = 1$}\label{fig:pyco_beta1m}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta10_alpha1_gamma99.pdf}
\caption{$\beta = 10$ (Low Reg.)}\label{fig:pyco_beta10m}
\end{subfigure} 
\caption{\label{fig:pyco} \textbf{Grid-World Reward Perturbations.} \textbf{(a)} Sequential task. \textbf{(b)-(d)} Policies trained with Shannon entropy regularization of different strength. Action probabilities are indicated via relative arrow lengths; the goal-state is gray and without annotations. Colors indicate worst-case adversarial reward perturbations $\prpi(a,s) = \frac{1}{\beta}\log \frac{\pi(a|s)}{ \pi_0(a|s)}$ for each state and action (up, down, left, right) against which the policy is 
robust. 
% guaranteed to be robust.
Red (or positive $\prpi(a,s)$) implies that the policy is robust to reward decreases (up to the value shown) imposed by the adversary. These decreases are balanced by adversarial reward increases (blue) for other actions in the same state. 
% While the highly regularized policy in (b) is robust against stronger perturbations in the sense of \cref{eq:robust_def}, it obtains a lower overall expected reward due to its increased stochasticity.
% ---which is, however, guaranteed to be larger or equal to the value of the regularized objective (\cref{eq:robust_def})  
We confirm the optimality of each policy using path consistency in \myapp{additional_results} \cref{fig:pyco_indifference}.}
% \RB{This is post-perturbation, I think I just meant that the regularized objective was worse} \TG{Yes, important to point out that the statements are post-perturbation, also in intro and conclusions where I left similar statements}.
% \TG{A bit more explanation - what is the reader supposed to see, what are the main takeaways? }}
\vspace*{-.1cm}
\end{figure*}


% \begin{figure*}[t]
% \begin{subfigure}{.2\textwidth}
% \phantom{\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_world.pdf}\vspace*{.2cm}}
% % \caption{\centering Environment \\
% % ($r(a,s) = -1$ for water, \\
% % $r(a,s) = 5$ for goal)}\label{fig:pyco_env}
% \end{subfigure}
% \begin{subfigure}{.26\textwidth}
% \includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta02_alpha1_gamma99_perturbed.pdf}
% \caption{$\beta = 0.2$ (High Reg.)}\label{fig:pyco_beta02}
% \end{subfigure}
% \begin{subfigure}{.26\textwidth}
% \includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta1_alpha1_gamma99_perturbed.pdf}
% \caption{$\beta = 1$}\label{fig:pyco_beta1}
% \end{subfigure}
% \begin{subfigure}{.26\textwidth}
% \includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta10_alpha1_gamma99_perturbed.pdf}
% \caption{$\beta = 10$ (Low Reg.)}\label{fig:pyco_beta02}
% \end{subfigure}
% \caption{\label{fig:pyco} Perturbed rewards $\mr(a,s) = r(a,s) - \pr(a,s)$ for policies trained with \textsc{kl} divergence regularization.  The indifference condition holds in all cases, with $\mr(a,s) = c(s)$ for each action, and at each state and $c(s) = V(s)$ for \textsc{kl} regularization.  This confirms that the policy is optimal \citep{ortega2014adversarial, nachum2017bridging}.}
% \end{figure*}

==> Reward Robustness TMLR (3)/sections/related_work_table.tex <==

\begin{figure*}[t]
\vspace*{-.2cm}
% \begin{minipage}{\pagewidth}
% \begin{minipage}{.7\textwidth}
\begin{subfigure}{.7\textwidth}
\centering
% \begin{center*}{\textwidth}
% \begin{table*}[t]
% % {\textwidth}
% \centering
% \caption{Comparison of Contributions}\label{table:novelty}
% \vspace*{-.2cm}
\resizebox{\textwidth}{!}
{
\begin{tabular}{lcccc}
    &  \text{\footnotesize \citet{ortega2014adversarial}} & \text{\footnotesize \citet{eysenbach2021maximum}} &  \text{\footnotesize \citet{husain2021regularized}} & Ours \\ \toprule
    \bullets{Multi-Step Analysis} & \tcminus{\xmark} & \tcplus{\cmark} & \tcplus{\cmark} & \tcplus{\cmark} \\ 
%   \bullets{Experiments match Theory} 
% %   \footnote{Our Fig. 3 displays the worst-case reward perturbations, and Fig. 6 confirms the optimality of the policy using the indifference and path consistency conditions. By contrast, \citet{husain2021regularized} evaluate using perturbations which do not match the theory, namely choosing $r\tick(a,s)= r(a,s) + \delta$ with $\delta \sim \mathcal{N}(5,.1)$ for $r(a,s) \leq \epsilon$. Fig. 6 and 9 in \citet{eysenbach2021maximum} lack detail.}
%     % Fig. 6 and 9 in \citet{eysenbach2021maximum} are not discussed in detail.   Our theory would predict that the MaxEnt \textsc{rl} objective with standard rewards matches the 
%     % % It is not appropriate to use the worst-case reward perturbations of MaxEnt \textsc{rl} to train .
%      & \tcminus{single step only} & \tcminus{\xmark} & \tcminus{\xmark} & \tcplus{\cmark} \\
    \bullets{Worst-Case $\propt(a,s)$} & \tcminus{policy form} & \tcminus{policy form} & \tcminus{value form} & \tcplus{policy \& value forms} \\ 
  \bullets{Feasible Set} & \tcminus{\xmark} & \tcminus{
    \cmark \, \,  (see our App G)} & \tcminus{\xmark} & \tcplus{\cmark} \\ 
  \bullets{Divergence Used} & \tcminus{KL ($\alpha = 1$)} & \tcminus{\text{ Shannon entropy (see Sec  5.1)}} & \tcplus{any convex $\Omega$} & \tcplus{$\alpha$-Div.} \\ 
    \bullets{$\mu(a,s)$ or $\pi(a|s)$ Reg.?} & (= in single step) & $\pi(a|s)$ & \tcplus{Both} & \tcplus{Both} \\
    \bullets{Indifference} & \tcplus{\cmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}  \\ 
    \bullets{Path Consistency} & \tcminus{\xmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}  \\ 
    \bottomrule
\end{tabular}
}
% \vspace*{.2cm}
\caption{}\label{table:novelty}
\end{subfigure}
% \captionof{table}{Comparison of Contributions}\label{table:novelty}
% \end{minipage}%
% \begin{minipage}{.3\textwidth}
\begin{subfigure}{.3\textwidth}
\centering
\vspace*{-0.5cm}
\includegraphics[width=.68\textwidth]{figs/feasible/kl/beta1alpha1uniform_adj.pdf}
\vspace*{-1.2cm}
\caption{}\label{fig:derman}
\end{subfigure}
\vspace*{-.3cm}
\caption{(a) Comparison to related work. (b) Comparison to rectangular robust set of \citet{derman2021twice}.  }\label{fig:related}
% \captionof{figure}{\text{\small \citet{derman2021twice}}}\label{fig:derman}
% \end{minipage}
% \end{minipage}
% \end{center}
\end{figure*}


==> Reward Robustness TMLR (3)/sections/related_work_table_no_derman.tex <==
\begin{figure*}[t]
\vspace*{-1cm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc}
    &  \text{ \citet{ortega2014adversarial}} & \text{\citet{eysenbach2021maximum}} &  \text{ \citet{husain2021regularized}} & Ours \\ \toprule
    \bullets{Multi-Step Analysis} & \tcminus{\xmark} & \tcplus{\cmark} & \tcplus{\cmark} & \tcplus{\cmark} \\ 
    \bullets{Worst-Case $\pr(a,s)$} & \tcminus{policy form} & \tcminus{policy form} & \tcminus{value form} & \tcplus{policy $\&$ value forms} \\ 
  \bullets{Robust Set} & \tcminus{\xmark} & 
    \tcplus{\cmark}  \tcminus{(see our \myapp{eysenbach})} & \tcminus{\xmark} & \tcplus{\cmark} \\ 
  \bullets{Divergence Used} & \tcminus{KL ($\alpha = 1$)} & \tcminus{\text{ Shannon entropy (see \mysec{entropy_vs_div})}} & \tcplus{any convex $\Omega$} & \tcplus{$\alpha$-Divergence} \\ 
    \bullets{$\mu(a,s)$ or $\pi(a|s)$ Reg.?} & 
     $\pi(a|s)$ & 
    % (= in single step) & 
    $\pi(a|s)$ & \tcplus{Both} & \tcplus{Both} \\
    \bullets{Indifference} & \tcplus{\cmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}  \\ 
    \bullets{Path Consistency} & \tcminus{\xmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}  \\ 
    \bottomrule
\end{tabular}%
}
\vspace*{-.3cm}
\captionof{table}{Comparison to related work. }\label{table:novelty}
\headerv
\end{figure*}

==> Reward Robustness TMLR (3)/sections/single_step_fig.tex <==
\newcommand{\WidthS}{.2\textwidth}
\newcommand{\WidthM}{.22\textwidth}
\newcommand{\WidthMM}{.22\textwidth}
\newcommand{\WidthMMM}{.23\textwidth}
\newcommand{\HeightS}{22mm}
\newcommand{\HeightSS}{22mm}
\newcommand{\HeightM}{22mm}


% \begin{figure*}[t]
% \vspace*{-1.5cm}
% % \vspace*{-0.5cm}
% \centering
% \subcaptionbox{Optimal Policy \label{fig:perturb_opt_a}}{
% \begin{minipage}{.48\textwidth}
% % \begin{subfigure}
% %\def\arraystretch{2.2}
% %  \subcaptionbox{Optimal Policy \label{fig:perturb_opt_a}}{
% \[\arraycolsep=.005\textwidth
% \begin{array}{cccc} %[width=40mm]
% %\begin{subfigure}{.16\columnwidth}
% %  & \multicolumn{3}{c}{\text{(i) }\beta = 0.1} \\[.5ex]
% %\end{subfigure}&\qquad  \hspace*{.2cm}
% %\begin{subfigure}{0.33\columnwidth} 
%   & \multicolumn{3}{c}{\text{(i) }\beta = 1.0} \\[.25ex]
% %  \vspace{-.26ex}\multirow{2}{\WidthMM}{\includegraphics[width=\WidthM, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/env.pdf} \\[.25ex] \includegraphics[width=\WidthM, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/opt_agent.pdf}} & \rulesep
% \includegraphics[width=\WidthM, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/env.pdf}  & \rulesep
% %\caption{\centering \small $D_{KL}, \beta = 10$}\label{fig:tabc}\end{subfigure}&\hspace*{.2cm}\\
% \includegraphics[width=\WidthS, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/beta1policy_opt.pdf} & 
% %\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
% %\begin{subfigure}{0.33\columnwidth} 
% \includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta1perturb_opt.pdf} & 
% %\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
% %\begin{subfigure}{0.33\columnwidth} 
% \includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta1perturbed_opt.pdf} \\[.25ex]
%  & \multicolumn{3}{c}{\text{(ii) } \beta = 10} \\[.25ex]
% \includegraphics[width=\WidthM, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/opt_agent.pdf} &\rulesep 
% %\end{subfigure}&\qquad  \hspace*{.2cm}
% %\begin{subfigure}{0.33\columnwidth} 
% \includegraphics[width=\WidthS, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/beta10policy_opt.pdf} & 
% %\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
% %\begin{subfigure}{0.33\columnwidth} 
% \includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta10perturb_opt.pdf} & 
% %\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
% %\begin{subfigure}{0.33\columnwidth} 
% \includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta10perturbed_opt.pdf} 
% % \\[.25ex]
% \end{array}
% \]
%  %\hspace*{0.25cm}
% % \label{subfig:subfig}
% % \caption{Optimal Policy }\label{fig:perturb_opt_a}
% % \end{subfigure}
% \end{minipage}\hspace{.02\textwidth} %{\quad \vline width 1pt}&
% }% 
% \subcaptionbox{Suboptimal Policy \label{fig:perturb_opt_a}}{
% \begin{minipage}{.48\textwidth}
% % \begin{subfigure}{.48\textwidth}
% % \subcaptionbox{Suboptimal Policy \label{fig:perturb_subopt_b}}{
% \[\arraycolsep=.005\textwidth
% \begin{array}{cccc} %[width=40mm]
% %\begin{subfigure}{.16\columnwidth}
%  & \multicolumn{3}{c}{\text{(i) } \beta = 1.0} \\[.25ex]
% %\caption{\centering \small $D_{KL}, \beta = 10$}\label{fig:tabc}\end{subfigure}&\hspace*{.2cm}\\
% \includegraphics[width=\WidthM, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/env.pdf}  & \rulesep
% \includegraphics[width=\WidthS, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/beta1policy_subopt.pdf} & 
% %\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
% %\begin{subfigure}{0.33\columnwidth} 
% \includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta1perturb_subopt.pdf} & 
% %\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
% %\begin{subfigure}{0.33\columnwidth} 
% \includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta1perturbed_subopt.pdf} \\[.25ex]
%  &  \multicolumn{3}{c}{\text{(ii) } \beta = 10} \\[.25ex]
%  \includegraphics[width=\WidthM, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/subopt_agent.pdf}  &\rulesep
% %\end{subfigure}&\qquad  \hspace*{.2cm}
% %\begin{subfigure}{0.33\columnwidth} 
% \includegraphics[width=\WidthS, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/beta10policy_subopt.pdf} & 
% %\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
% %\begin{subfigure}{0.33\columnwidth} 
% \includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta10perturb_subopt.pdf} & 
% %\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
% %\begin{subfigure}{0.33\columnwidth} 
% \includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta10perturbed_subopt.pdf} \\[.25ex]
% \end{array}
% \]
% \end{minipage}
% }
% % \caption{Suboptimal Policy} \label{fig:perturb_subopt_b}
% % \end{subfigure}
% \vspace*{-0.2cm}
% \caption{ \textbf{Single-Step Reward Perturbations} for \textsc{kl}~regularization to uniform reference policy $\pi_0(a|s)$.  $Q$-values in leftmost columns are used for each $\beta$ in columns 2-4.  We report the worst-case $-\proptpi(a,s)$ from \cref{eq:optimal_perturbations}, so that negative values correspond to reward decreases. 
% % Note that the adversary cannot selectively perturb a single action, and instead must apply both negative and positive perturbations. 
% % \TG{We have this in the main text, maybe axe it here.} 
% \textbf{(a)} Optimal policy ($Q_*(a,s) = r(a,s)$), where the perturbed reward $r^{\prime}(a,s) = c \, \, \forall a$ reflects the indifference condition. \textbf{(b)} Suboptimal policy where indifference does not hold.  In all cases, actions with high $Q(a,s)$ are robust to reward decreases. }\label{fig:perturb_opt}
% % (we only consider a single state $s$ but keep it in the notation for consistency)
% \vspace*{-0.2cm}
% \end{figure*}


\begin{figure*}[t]
\vspace*{-1.65cm}
% \vspace*{-0.5cm}
\centering
\subcaptionbox{Optimal Policy \label{fig:perturb_opt_a}}{
\begin{minipage}{.485\textwidth}
% \begin{subfigure}
%\def\arraystretch{2.2}
%  \subcaptionbox{Optimal Policy \label{fig:perturb_opt_a}}{
\[\arraycolsep=.0025\textwidth
\begin{array}{cccc} %[width=40mm]
%\begin{subfigure}{.16\columnwidth}
%  & \multicolumn{3}{c}{\text{(i) }\beta = 0.1} \\[.5ex]
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
  & \multicolumn{3}{c}{\text{(i) }\beta = 1.0} \\[.25ex]
%  \vspace{-.26ex}\multirow{2}{\WidthMM}{\includegraphics[width=\WidthM, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/env.pdf} \\[.25ex] \includegraphics[width=\WidthM, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/opt_agent.pdf}} & \rulesep
\multirow{2}{*}[.25cm]{ \includegraphics[width=\WidthM,height=\HeightSS, trim=0 0 0 0, clip]{figs/perturbed/env_qopt.pdf} } & \rulesep
%\caption{\centering \small $D_{KL}, \beta = 10$}\label{fig:tabc}\end{subfigure}&\hspace*{.2cm}\\
\includegraphics[width=\WidthS, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/beta1policy_opt.pdf} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta1perturb_opt.pdf} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta1perturbed_opt.pdf} \\[.25ex]
 & \multicolumn{3}{c}{\text{(ii) } \beta = 10} \\[.25ex]
% \includegraphics[width=\WidthM, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/opt_agent.pdf} 
&\rulesep 
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/beta10policy_opt.pdf} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta10perturb_opt.pdf} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta10perturbed_opt.pdf} 
% \\[.25ex]
\end{array}
\]
 %\hspace*{0.25cm}
% \label{subfig:subfig}
% \caption{Optimal Policy }\label{fig:perturb_opt_a}
% \end{subfigure}
\end{minipage}\hspace{.02\textwidth} %{\quad \vline width 1pt}&
}% 
\subcaptionbox{Suboptimal Policy \label{fig:perturb_opt_a}}{
\begin{minipage}{.485\textwidth}
% \begin{subfigure}{.48\textwidth}
% \subcaptionbox{Suboptimal Policy \label{fig:perturb_subopt_b}}{
\[\arraycolsep=.005\textwidth
\begin{array}{cccc} %[width=40mm]
%\begin{subfigure}{.16\columnwidth}
 & \multicolumn{3}{c}{\text{(i) } \beta = 1.0} \\[.25ex]
%\caption{\centering \small $D_{KL}, \beta = 10$}\label{fig:tabc}\end{subfigure}&\hspace*{.2cm}\\
 \multirow{2}{*}[.075cm]{
\includegraphics[width=\WidthM, height=\HeightSS, trim=0 0 0 0, clip]{figs/perturbed/subopt_agent.pdf}}  & \rulesep
\includegraphics[width=\WidthS, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/beta1policy_subopt.pdf} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta1perturb_subopt.pdf} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta1perturbed_subopt.pdf} \\[.25ex]
 &  \multicolumn{3}{c}{\text{(ii) } \beta = 10} \\[.25ex]
%  \includegraphics[width=\WidthM, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/subopt_agent.pdf}  
 &\rulesep
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=0 0 0 0, clip]{figs/perturbed/beta10policy_subopt.pdf} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta10perturb_subopt.pdf} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=0 0 0 0, clip]{figs/perturbed/beta10perturbed_subopt.pdf} \\[.25ex]
\end{array}
\]
\end{minipage}
}
% \caption{Suboptimal Policy} \label{fig:perturb_subopt_b}
% \end{subfigure}
\vspace*{-0.15cm}
\caption{ \textbf{Single-Step Reward Perturbations} for \textsc{kl}~regularization to uniform reference policy $\pi_0(a|s)$.  $Q$-values in left columns are used for each $\beta$ in columns 2-4.  We report the worst-case $-\proptpi(a,s)$ (\cref{eq:optimal_perturbations}), so negative values correspond to reward decreases. 
% Note that the adversary cannot selectively perturb a single action, and instead must apply both negative and positive perturbations. 
% \TG{We have this in the main text, maybe axe it here.} 
\textbf{(a)} Optimal policy ($Q_*(a,s) = r(a,s)$) using the environment reward, where the perturbed $r^{\prime}(a,s) = c \, \, \forall a$ reflects the indifference condition. \textbf{(b)} Suboptimal policy where indifference does not hold.  In all cases, actions with high $Q(a,s)$ are robust to reward decreases. }\label{fig:perturb_opt}
% (we only consider a single state $s$ but keep it in the notation for consistency)
\vspace*{-0.1cm}
\end{figure*}

==> old/0_intro.tex <==
\section{Introduction}\label{sec:intro}
%\TG{Not very urgent, but I think the title of the paper can be improved - ideally it's catchy and summarizes the main finding/message of the paper. E.g. ``Meta-trained agents implement Bayes-optimal agents'' was a winner :)}
% While \gls{RL} algorithms have achieved remarkable success in challenging domains \citep{mnih2015human,silver2016mastering}, questions of optimization, exploration, and safe generalization remain activate areas of research.   
Regularization plays a crucial role in various settings across \gls{RL}, such as trust-region methods \citep{peters2010relative, schulman2015trust, schulman2017proximal, basserrano2021logistic}, offline learning \citep{levine2020offline, nachum2019dualdice, nachum2019algaedice, nachum2020reinforcement}, multi-task learning \citep{teh2017distral, galashov2020importance}, and soft 
$Q$-learning or actor-critic methods
% actor-critic methods 
\citep{fox2016taming, nachum2017bridging, haarnoja17a, haarnoja2018soft, grau2018soft}. 
% \textcolor{red}{SAC? Soft Q?}
%with stochastic policies 
Various justifications have been given for policy regularization, %the benefits of
such as improved optimization \citep{ahmed2019understanding},  
% implicit averaging of $Q$-values, \citep{viellard},
connections with probabilistic inference \citep{levine2018reinforcement, galashov2018information}, 
 %with purported benefits including X, Y, Z , 
 and robustness to perturbations in environment rewards or dynamics \citep{eysenbach2021maximum, husain2021regularized}.
%  The latter benefits may be particularly relevant for safety considerations \citep{amodei2016concrete, everitt2018agi}, where we are interested in agents which can generalize or adapt to new environments or distribution shift.
The latter 
is crucial in \textsc{ai} safety, where
% plays a crucial role in \textsc{ai} safety, where 
a primary goal
% the goal 
is to design agents that generalize and adapt safely to new situations or distributional shift.
% \citep{amodei2016concrete, everitt2018agi}.

% In this work, we provide a unified discussion of several recent works that interpret policy regularization as providing robustness to perturbations in the environmental rewards \TG{Suggestion: ``In this work we theoretically analyze the robustness-properties that arise form policy regularization in RL.'' Then skip to the next sentence (For a policy...) and mention the unified view later.} \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}.

In this work, we analyze the robustness properties which arise from policy regularization in \gls{RL}.
For a policy $\pi(a|s)$ regularized using a convex function $\Omega(\pi) = \mathbb{E}_{\pi}[\ptReg(\pi)]$ such as a statistical divergence, we investigate statements of the form %\citep{eysenbach2021maximum}
\begin{align}
\hspace*{-.2cm} &\max \limits_{\pi(a|s)} (1-\gamma) \mathbb{E}_{\tau \sim p^{\pi}(\tau)} \left[ \sum \limits_{t=0}^\infty \gamma^t \bigg( r(a_t, s_t) - \ptReg \big(\pi(a_t | s_t)\big) \bigg) \right] \nonumber \\
&= \max \limits_{\pi(a|s)} \min \limits_{r\tick(a,s) \in \feasibleset}  \mathbb{E}_{\tau \sim p^{\pi}(\tau)} \left[ \sum \limits_{t=0}^\infty \gamma^t \, r\tick(a_t,s_t) \right]
\label{eq:reward_perturbation_stmt}
\end{align}
where $r\tick(a,s)$ is the worst-case reward function chosen from an appropriate feasible set $\feasibleset$. %which depends on the policy $\pi$.
This robustness is intriguing, as it suggests regularized policies achieve a form of `zero-shot' generalization to new environments where the reward has been adversarially chosen. %of a policy

Using tools from convex duality, we provide a precise characterization of this reward robustness,
%which leads to a game-theoretic interpretation of soft value aggregation as hedging against adversarial perturbations which tend to equalize the reward function across actions in a particular state \citep{ortega2014adversarial}.
%and provide a unified discussion of several recent works that explore similar interpretations \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}
We find that the optimal modified reward $r_{*}\tick$ in \cref{eq:reward_perturbation_stmt} re-expresses the value of the objective for a given policy, which places restrictions on the set $\mathcal{R}$.  We discuss the implications of this particular form of robustness for generalization, along with a game-theoretic interpretation of soft value aggregation as hedging against adversarial perturbations that seek to 
equalize the reward obtained for each action in a particular state \citep{ortega2014adversarial}.
% how this impacts the nature of the robustness or `zero-shot' generalization induced by policy regularization
Our analysis unifies several recent works that explore similar interpretations \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}, and our main contributions include
%Our main contributions are:
% Using tools from convex duality, we show that adversarial reward interpretations may not align with this desired robustness. Instead, we find that the optimal modified reward $r\tick$ in \cref{eq:reward_perturbation_stmt} simply re-expresses the value of the objective for a given policy, with the minimax optimization corresponding to a particular game-theoretic interpretation \citep{ortega2014adversarial}. We make the following additional contributions
% \TG{Alternative for the previous para: ``Using tools from convex duality, we precisely characterize the `zero-shot' generalization regime and relate it to a game-theoretic interpretation where robustness arises from `hedging' against adversarial perturbations to the reward function \citep{ortega2014adversarial}. We find that the optimal modified reward $r\tick$ in \cref{eq:reward_perturbation_stmt} re-expresses the value of the objective for a given policy, which restricts the set $\mathcal{R}$. We discuss how this impacts the nature of the robustness or `zero-shot' generalization induced by policy regularization and provide a unified discussion of several recent works that explore similar interpretations \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum}. Our main contributions are:}
\begin{itemize}
% \item A thorough analysis of the robustness associated with \KL and $\alpha$-divergence regularization of \gls{RL} policies, which includes popular Shannon \citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum} and Tsallis entropy \citep{lee2019tsallis} entropy regularization as a special cases.    We argue that using divergence regularization instead of entropy regularization avoids several unsatisfying conclusions from previous work. %\citep{lee2019tsallis, eysenbach2021maximum}.
% %Our derivations for $\alpha$-divergence regularization extend the Tsallis entropy \citep{lee2019tsallis}
\item A thorough analysis of the robustness associated with \KL and $\alpha$-divergence regularization of \gls{RL} policies.  This includes popular Shannon entropy regularization  
%schemes 
\citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum} as a special case, and our derivations for the $\alpha$-divergence generalize the Tsallis entropy \gls{RL} framework of \citep{lee2019tsallis}.  
% Our analysis covers popular Shannon entropy regularization schemes \citep{haarnoja17a,haarnoja2018soft, eysenbach2021maximum}, while our derivations for the $\alpha$-divergence extend the Tsallis entropy \gls{RL} framework of \citep{lee2019tsallis}.    
\item Our analysis of the $\alpha$-divergence highlights distinct roles for the value function and policy normalization constant, which coincide in the case of the \textsc{kl} divergence. 
% but not for the $\alpha$-divergence. 
% We argue that using divergence regularization instead of entropy regularization avoids several unsatisfying conclusions from previous work. %\citep{lee2019tsallis, eysenbach2021maximum}.
\item A precise characterization of the feasible set $\mathcal{R}$ of adversarial rewards against which a regularized policy is robust, as visualized in \cref{fig:feasible_set_main} and shown in \myprop{perturbations}-\ref{prop:perturbations_alpha}.
% which improves upon the analysis of \citet{eysenbach2021maximum}.  
Our use of divergence regularization instead of entropy regularization clarifies 
several unsatisfying conclusions from previous work.
% the analysis of \citet{eysenbach2021maximum}.
\item We link a game-theoretic `indifference condition', which occurs at an equilibrium between the agent and adversary \citep{ortega2014adversarial}, to the `path consistency' optimality condition, which has been used to construct learning objectives in \citep{nachum2017bridging, chow2018path}.  
% % for the optimal policy and reward perturbations  with notion of path consistency \citep{nachum2017bridging, chow2018path}.  
% \item \textcolor{red}{to be cut} A comparison of regularization of the joint state-action distribution and conditional policy distribution. 
% % with connections between adversarial reward perturbations and the notion of path consistency \citep{nachum2017bridging, chow2018path}.  
% \item An alternative derivation of the objective function used in Logistic $Q$-learning \citep{basserrano2021logistic}, in which adversarial reward perturbations provide a natural justification for including $Q$-values in convex programming formulations of \textsc{rl}. \RB{likely only one of these, derivation needs to be checked to prioritize this}
\end{itemize}
While the latter observations hold only for the optimal policy, we emphasize that our results provide a reward robustness interpretation for \textit{any} stochastic policy under a given regularization scheme.
%After interpreting the optimal adversarial rewards in terms of both the policy and $Q$-values of the agent, we argue that adversarial reward perturbation interpretations %of stochastic policies provide a natural way to include $Q$-values in \gls{LP} formulations of \gls{RL} and lead to an alternative derivation of the objective function used in Logistic $Q$-learning \citep{basserrano2021logistic}. 
%     \item \TG{Precise characterization of the robustness induced via policy regularization in RL. In particular we theoretically analyze KL- and alpha-divergence regularization, which includes the popular maximum entropy regularization (TODO: citation) as a special case.}
%     \item \TG{Theoretical and empirical analysis of the feasible set $\mathcal{R}$, which is the set of adversarial reward perturbations to which the regularized policy is `zero-shot' robust against.}
%     \item %We clarify the feasible set of adversarial rewards associated with a particular policy compared with \citet{eysenbach2021maximum}, 
%     Compared with \TG{Maybe better: ``Following up on''} \citet{eysenbach2021maximum}, we clarify the feasible set of adversarial rewards associated with a particular policy
%     and argue that using divergence regularization instead of entropy regularization avoids several unsatisfying conclusions.
%     %leads to several unsatisfying interpretations compared with divergence regularization.
%     %correct several unintuitive conclusions which arise from entropy regularization rather than divergence regularization.
%     \item We provide derivations and analysis for $\alpha$-divergence regularization, which generalizes the Tsallis entropy framework of \citet{lee2019tsallis}.    This provides insight into the distinct role of the value function and normalization constant of the policy, which coincide for the case of the \textsc{kl} divergence or Shannon entropy.   %and provides insight into the distinct role of the value function and normalization constant of the policy, which coincide for the case of the \textsc{kl} divergence or Shannon entropy.
%     \item After interpreting the optimal adversarial rewards in terms of both the policy and $Q$-values of the agent, 
%     we argue that adversarial reward perturbation interpretations %of stochastic policies
%     provide a natural way to include $Q$-values in \gls{LP} formulations of \gls{RL} and lead to an alternative derivation of the objective function used in Logistic $Q$-learning \citep{basserrano2021logistic}.   %To this end, %we provide an alternative derivation of the objective function in Logistic $Q$-learning.  %which does not rely on a relaxed \gls{LP}.
% \end{itemize}
% %Compared with previous works, we clarify the feasible set of adversarial rewards and correct several surprising conclusions which arise from entropy regularization rather than divergence regularization.  Finally, we provide additional derivations and analysis for $\alpha$-divergence regularization, which extends the Tsallis entropy \textsc{rl} framework of \citet{lee2019tsallis}.



% \textbf{Contributions}
% \begin{itemize}
%     \item  We extend the analysis of \citet{ortega2014adversarial} to the sequential setting using the convex programming tools, which leads to more extensive, game-theoretic analysis of the reward robustness described in \citet{eysenbach2021maximum}.    We also discuss connections with the more general results of \citet{husain2021regularized}, and clarify the feasible set of reward perturbations compared with \citep{eysenbach2021maximum}.
%     %provide a more precise characterization of the
%     %Further, the use of entropy regularization in \citet{eysenbach2021maximum} leads to the counter-intuitive conclusion that increasing regularization strength leads to \textit{less} robust agents.   
%     \item We extend derivations using the \textsc{kl} divergence to the $\alpha$-divergence, which includes the Tsallis entropy as a special case.  With detailed convex conjugacy derivations, we highlight distinct roles for the value function and policy normalization constant, which coincide in the case of the \textsc{kl} divergence but not for the $\alpha$-divergence. 
    
%     % \item We provide a more detailed amore precise characterization of the feasible set of perturbations
    
%     \item Finally, our reward robustness interpretations using convex duality suggest connections with the notion of path consistency \citep{nachum2017bridging, chow2018path} and may provide additional insight into a relaxed \textsc{lp} formulation from \citep{mehta2009q, lee2019stochastic, basserrano2021logistic}. 
%     %\item  We provide a more precise characterization of the feasible set of perturbations
%     %\item  We visualize the optimal perturbed rewards in a single step (\cref{fig:perturb_opt}) and \textcolor{red}{multi-step} setting 
%     %\item  We analysis applies similarly to the derivations of \citet{husain2021regularized}
% \end{itemize}

==> old/1_prelim.tex <==
\section{Preliminaries}\label{sec:prelim}
% In this section, we provide background on primal and dual \gls{LP} formulations of %fully observed, 
% discounted \gls{MDP}, along with extensions using convex policy regularization.
% We begin by reviewing the convex conjugate function, %or Legendre-Fenchel transform, 
% which will play a crucial role throughout our paper.
In this section, we review
% provide background on 
\gls{LP} formulations of %fully observed, 
discounted \gls{MDP}, along with extensions to convex policy regularization.
We begin by reviewing the convex conjugate, %or Legendre-Fenchel transform, 
which will play a crucial role throughout our paper.


\subsection{Convex Conjugate}\label{sec:conj_intro}
% Before describing analogous primal and dual optimizations for regularized \gls{MDP}s, we review the convex conjugate function, or Legendre-Fenchel transform, which will play a crucial role throughout our paper.
%First,
For any convex function $\Omega(\pi)$ with domain $\pi \in \mathcal{D}$, 
%, where $\mathcal{D}$ may indicate the probability simplex $\Delta^{|A|}$ with possible additional constraints, such as $\mu_{\pi}(a,s) \in \mathcal{M}$
%over domain $\pi \in \Delta^{|\mathcal{A}|}$, possibly , 
%the Legendre-Fenchel transform or 
the conjugate function $\Omega^{*}$ is defined via the optimization
\begin{align}
    \Omega^{*}( \dualvar ) = \sup \limits_{\pi \in \mathcal{D}} \, \big \langle \pi, \dualvar \big \rangle - \Omega(\pi) \label{eq:conjstar}
\end{align} 
where $\dualvar \in \dualdomain$ is a function in the continuous dual space of $\pi$. %continuous function in the topological dual space of $\pi$. %arbitrary function whose domain has the same dimension as $\mathcal{D}$.  
 %The conjugate function 
 The conjugate operation is an involution for proper, lower semi-continuous, and convex $\Omega$ \citep{boyd2004convex},
 %(\citet{borwein2010convex} Sec. 4.3), 
 so that $(\Omega^{*})^{*} = \Omega$ and $\Omega^{*}$ is also convex.  
 We can thus represent $\Omega(\pi)$ via a conjugate optimization
 \begin{align}
     \Omega(\pi) = \sup_{\dualvar \in \dualdomain} \big \langle \pi, \dualvar \big \rangle - \Omega^{*}(\dualvar) \label{eq:conjomega}
 \end{align}
  Differentiating with respect to optimization variable in either \cref{eq:conjstar} or \cref{eq:conjomega} suggests optimality conditions for $\pi_*$ and $\dualvar$
%   Solving for the $\arg \sup$ in either \cref{eq:conjstar} or \cref{eq:conjomega} suggests optimality conditions for $\pi_*$ and $\dualvar$
% \begin{align}
%     \pi_*(a|s) = \big(\nabla \Omega(\pi) \big)^{-1}(\dualvar) \qquad \qquad \dualvar_*(a,s) = \big(\nabla \Omega^{*}(\dualvar) \big)^{-1}(\pi)
% \end{align}
 \begin{align}
     \pi_*(a|s) = \nabla \Omega^{*}( \dualvar )   \quad \qquad \dualvar_*(a,s) = \nabla \Omega(\pi)     \label{eq:optimal_policy_as_grad}
 \end{align}
From the above, conjugacy also implies relationships of the form $\pi_*(a|s) = (\nabla \Omega)^{-1}(\dualvar_*(a,s))$ when $\pi_*$ and $\dualvar_*$ are in dual correspondence.


%We show concrete examples of the conjugate function in \cref{table:conjugates}\footnote{Note, we distinguish between conjugate functions $\Omega_{\pi}(\pi)$ and $\Omega_{\tpi}(\tpi)$, where $\pi$ is explicitly constrained to be normalized while  $\tpi$  is not.}, with derivations in \myapp{kl_conj_all}-\ref{app:alpha_conj_all}, %and discussion in \mysec{conj_examples}
We proceed to describe how the conjugate arises in convex programming formulations of regularized \gls{MDP}s, before describing examples in \mysec{conj_examples}. %concrete


% \small
% \begin{figure*}[t]
% \centering
% % \begin{tabular}{ccc}
% %   \multicolumn{1}{c}{$\Omega(\pi)$} & \multicolumn{1}{c}{Definition of $D[\pi||\pi_0]$} & \multicolumn{1}{c}{Conjugate $\Omega^{*}(\dualvar)$} \\ \toprule
% %     $\frac{1}{\beta} D_{KL}[\pi:\pi_0]$ & $\sum \limits_{a} \pi \log \pi/\pi_0 $& $\frac{1}{\beta} \log \sum \limits_{a} \pi_0  \expof{\beta \cdot \dualvar} $ \\[1.25ex] %\sum \limits_{\pi_0}
% %     $\frac{1}{\beta}D_{KL}[\tpi:\tpi_0]$ & $\sum \limits_{a} \tpi \log \tpi/\tpi_0 - \sum \limits_{a} \tpi + \sum \limits_{a}\tpi_0$ & $\frac{1}{\beta} \sum \limits_{a} \tpi_0 \expof{\beta \cdot \dualvar} - \frac{1}{\beta} \sum \limits_{a} \tpi_0$  \\[1.25ex] % \mathbb{E}_{\pi_0}
% %     $\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $\frac{1}{\alpha(1-\alpha)}\big( 1 - \sum \limits_{a} \pi_0^{1-\alpha} \pi^{\alpha} \big)$ & \\[1.25ex]
% %     $\frac{1}{\beta}D_{\alpha}[\tpi:\tpi_0]$ & $\frac{1}{\alpha(1-\alpha)}\big( (1-\alpha) \sum \limits_{a} \tpi_0 + \alpha \sum \limits_{a} \tpi - \sum \limits_{a} \tpi_0^{1-\alpha} \tpi^{\alpha} \big)$ & $\frac{1}{\beta}\frac{1}{\alpha} \sum \limits_{a} \tpi_0^{1-\alpha} \tpi^{\alpha} - \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_a \tpi$ \\ \bottomrule
% % \end{tabular
% %\tiny
% % \begin{tabular}{lllll} %\pi_*= \tpi_*=
% %   \multicolumn{1}{c}{$D[\pi||\pi_0]$} & \multicolumn{1}{c}{$\Omega(\pi)$} &  \multicolumn{1}{c}{$\Omega^{*}(\dualvar)$} & $\pi_* = \nabla \Omega^{*}( \dualvar )  $ & $\dualvar_*= \nabla \Omega(\pi)$  \\ \toprule
% %     $\frac{1}{\beta} D_{KL}[\pi:\pi_0]$ & $\sum \limits_{a} \pi \log \pi/\pi_0 $& $\frac{1}{\beta} \log \sum \limits_{a} \pi_0  \expof{\beta \cdot \dualvar} $ & $\pi_0 \exp\{\beta  \big( \dualvar - \psi(\beta) \big) \}$ & \tiny $\frac{1}{\beta} \log \frac{\pi}{\pi_0} + \frac{1}{\beta} \sum \limits_a \pi_0 \exp \{ \beta \cdot r\tick \} $\\[1.5ex] %\sum \limits_{\pi_0}
% %     $\frac{1}{\beta}D_{KL}[\tpi:\tpi_0]$ & $\sum \limits_{a} \tpi \log \tpi/\tpi_0 - \sum \limits_{a} \tpi + \sum \limits_{a}\tpi_0$ & $\frac{1}{\beta} \sum \limits_{a} \tpi_0 \expof{\beta \cdot \dualvar} - \tpi_0$ & $\tpi_0 \exp\{\beta \cdot \dualvar \}$ & $\frac{1}{\beta} \log \frac{\pi}{\pi_0} $\\[1.5ex] % \mathbb{E}_{\pi_0}
% %     $\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $\frac{1}{\alpha(1-\alpha)}\big( 1 - \sum \limits_{a} \pi_0^{1-\alpha} \pi^{\alpha} \big)$ &  \tiny $\frac{\alpha-1}{\alpha} \sum \limits_a \pi_0 [ 1 + (\alpha-1) \beta \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}}$ & \tiny $\pi_0 [ 1 + (\alpha-1) \beta \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}} $ & \\
% %     & &  \qquad \tiny $\, + \frac{1}{\beta} \psi_{\alpha}(\beta)$&  &\\[1.5ex]
% %     $\frac{1}{\beta}D_{\alpha}[\tpi:\tpi_0]$ & \tiny $\frac{1}{\alpha(1-\alpha)}\big( \sum \limits_{a} (1-\alpha) \tpi_0 $ & \tiny $\frac{\alpha-1}{\alpha} \sum \limits_a \tpi_0 [ 1 + (\alpha-1) \beta \cdot \dualvar]_+^{\frac{1}{\alpha-1}}$ & \tiny $\tpi_0 [ 1 + (\alpha-1) \beta \cdot \dualvar]_+^{\frac{1}{\alpha-1}} $ & \\ 
% %     & $ \, \, +\sum \limits_{a} \alpha \tpi - \tpi_0^{1-\alpha} \tpi^{\alpha} \big)$ &  \tiny $\, \, + \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_a  (\tpi_0 [ 1 + (\alpha-1) \beta \cdot \dualvar]_+^{\frac{1}{\alpha-1}} - \tpi_0 \big)$&  &\\ \bottomrule
% % \end{tabular}
% \small
% \begin{tabular}{lll} %\pi_*= \tpi_*=
%   \multicolumn{1}{c}{$D[\pi||\pi_0]$} & \multicolumn{1}{c}{$\Omega(\pi)$} &  \multicolumn{1}{c}{$\Omega^{*}(\dualvar)$}  \\ \toprule
%     $\frac{1}{\beta} D_{KL}[\pi:\pi_0]$ & $\sum \limits_{a} \pi \log \pi/\pi_0 $& $\frac{1}{\beta} \log \sum \limits_{a} \pi_0  \expof{\beta \cdot \dualvar} := \psi_1(\beta) $ \\[1.5ex] %\sum \limits_{\pi_0}
%     $\frac{1}{\beta}D_{KL}[\tpi:\tpi_0]$ & $\sum \limits_{a} \tpi \log \tpi/\tpi_0 - \sum \limits_{a} \tpi + \sum \limits_{a}\tpi_0$ & $\frac{1}{\beta} \big( \sum \limits_{a} \tpi_0 \expof{\beta \cdot \dualvar} - \tpi_0 \big)$ \\[1.5ex] % \mathbb{E}_{\pi_0}
%     $\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $\frac{1}{\alpha(1-\alpha)}\big( 1 - \sum \limits_{a} \pi_0^{1-\alpha} \pi^{\alpha} \big)$ &  $\frac{\alpha-1}{\alpha} \sum \limits_a \pi_0 [ (\alpha-1) \beta \cdot \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}} \cdot \dualvar + \frac{1}{\alpha} \psi_{\alpha}(\beta)$ \\
%     %$\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $\frac{1}{\alpha(1-\alpha)}\big( 1 - \sum \limits_{a} \pi_0^{1-\alpha} \pi^{\alpha} \big)$ &  $\frac{\alpha-1}{\alpha} \sum \limits_a \pi_0 [ 1 + (\alpha-1) \beta \cdot \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}} \cdot \dualvar + \frac{1}{\beta} \psi_{\alpha}(\beta)$ \\
%     $\frac{1}{\beta}D_{\alpha}[\tpi:\tpi_0]$ & \footnotesize  $\frac{1}{\alpha(1-\alpha)}\big( \sum \limits_{a}  (1-\alpha) \tpi_0 + \alpha \tpi_1 - \tpi_0^{1-\alpha} \tpi^{\alpha} \big) $ & \tiny $\frac{\alpha-1}{\alpha}\bigg(  \sum \limits_a \tpi_0 [ 1 + (\alpha-1) \beta  \dualvar]_+^{\frac{1}{\alpha-1}} \dualvar \bigg) + \frac{1}{\beta}\frac{1}{\alpha} \sum \limits_a  (\tpi_0 [ 1 + (\alpha-1) \beta  \dualvar]_+^{\frac{1}{\alpha-1}} - \tpi_0 \big)$\\[.1ex] \midrule
% \vspace*{.1cm}
% %& & & \linespread{0.5}  \\
% % \end{tabular}
% % \begin{tabular}{lll}
% \RB{Omit?}
% \multicolumn{1}{c}{$D[\pi||\pi_0]$} & \multicolumn{1}{c}{$\dualvar_*= \nabla \Omega(\pi)$} & \multicolumn{1}{c}{$\pi_* = \nabla \Omega^{*}( \dualvar )  $}  \\ \toprule
%  $\frac{1}{\beta} D_{KL}[\pi:\pi_0]$ & $\frac{1}{\beta} \log \frac{\pi}{\pi_0} + \frac{1}{\beta} \sum \limits_a \pi_0 \exp \{ \beta \cdot r\tick \} $  & $\pi_0 \exp\{\beta  \cdot \big( \dualvar - \psi(\beta) \big) \}$ \\
%  $\frac{1}{\beta}D_{KL}[\tpi:\tpi_0]$ & $\frac{1}{\beta} \log \frac{\pi}{\pi_0} $ & $\tpi_0 \exp\{\beta \cdot \dualvar \}$  \\
%  $\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $ \frac{1}{\beta} \frac{1}{\alpha-1} \left( \big(\frac{\tpi}{\tpi_0}\big)^{\alpha-1}\right) + \textcolor{red}{\psi_{\alpha}(\beta)}$ & $\pi_0 [ (\alpha-1) \beta \cdot \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}} $  \\ 
% %  $\frac{1}{\beta}D_{\alpha}[\pi:\pi_0]$ & $ \frac{1}{\beta} \frac{1}{\alpha-1} \left( \big(\frac{\tpi}{\tpi_0}\big)^{1-\alpha}\right) $ & $\pi_0 [ 1 + (\alpha-1) \beta \cdot \big( \dualvar - \psi_{\alpha}(\beta) \big)]_+^{\frac{1}{\alpha-1}} $  \\ 
%  $\frac{1}{\beta}D_{\alpha}[\tpi:\tpi_0]$ &$ \frac{1}{\beta}\ln_{\alpha} \big(\frac{\tpi}{\tpi_0}\big) := \frac{1}{\beta} \frac{1}{\alpha-1} \left( \big(\frac{\tpi}{\tpi_0}\big)^{\alpha-1} - 1\right)$ &  $\tpi_0 [ 1 + (\alpha-1) \beta \cdot \dualvar]_+^{\frac{1}{\alpha-1}} $ 
% \end{tabular}
% \captionof{table}{\centering Conjugate Functions for \textsc{kl} and $\alpha$-divergences over normalized $\pi$ and unnormalized $\tpi$.}\label{table:conjugates}
% \end{figure*}

\normalsize
\subsection{Primal Formulations}
We consider an \gls{MDP} as a tuple $\{ \mathcal{S}, \mathcal{A}, P, \nu_0, r, \gamma \}$ consisting of a state space $\mathcal{S}$, action space $\mathcal{A}$, transition dynamics $P(s\tick|s,a)$ for $s, s\tick \in \mathcal{S}$, $a \in \mathcal{A}$, initial state distribution $\nu_0(s) \in \Delta^{|\mathcal{S}|}$ in the probability simplex, and reward function $r(a,s):\mathcal{S} \times \mathcal{A} \mapsto \mathbb{R}$.   We use a discount factor $\gamma ~\in (0,1)$ 
% (\citet{puterman2014markov} Sec. 6)
, although this may also be handled by including a transition to an absorbing state into the \gls{MDP} (\citet{puterman2014markov} Sec. 5.3). 

\paragraph{Unregularized Case} %seeks %obtained 
%An agent seeks to maximize the expected discounted reward by acting according to a decision policy $\pi(a_t|s_t) \in \Delta^{|\mathcal{A}|}$, 
We consider an agent that seeks to maximize the expected discounted reward by acting according to a decision policy $\pi(a_t|s_t) \in \Delta^{|\mathcal{A}|}$ in each state of the \gls{MDP}. 
%which associates a distribution over actions to .    
We assume that the policy is stationary and Markovian, so that it is independent of both the timestep and trajectory history.


Most commonly, this optimization is written using expectations %are taken 
with respect to trajectories  $\tau$ which start from an initial state $s_0 \sim \nu_0(s)$ and evolve according to the policy $\pi(a|s)$ and dynamics $P(s\tick|s,a)$, with $ \tau \sim \pi(\tau):= \nu_0(s_0) \prod \pi(a_t | s_t) P(s_{t+1} | s_t, a_t)$.   Writing the objective $\mathcal{R}(r, \nu_0, P, \gamma)$ as $\mathcal{R}(r)$ for simplicity,
\begin{align}
   \mathcal{R}(r) := \max \limits_{\pi(a|s)} \, (1-\gamma) \, \mathbb{E}_{\tau \sim \pi(\tau)} \bigg[ \sum \limits_{t=0}^{\infty} \gamma^t \, r(s_t, a_t)  \bigg] \, . \label{eq:policy_only} 
\end{align}

%\subsubsection{Primal Optimization} 
%\paragraph{Primal Optimization} 
To highlight connections with literature on convex duality, we convert this optimization into a equivalent linear program, which we refer to as the \textit{primal}
%This learning problem may be also framed in terms of a linear program, which we will refer to as the \textit{primal}
\small
\begin{align}
   \hspace*{-.2cm} & \mathcal{R}(r) = \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \, \, \text{subj. to} \, \quad    \left( \forall s \in \mathcal{S} \right) \label{eq:primal_lp}\\
   &\sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \nonumber  \, .
   %\, \forall s \in \mathcal{S}\nonumber
\end{align}
\normalsize
where inner product notation $\langle \cdot, \cdot \rangle$ indicates summation or integration over the domain of $\mu$. %\RB{improve} %$\sum \mu \cdot \dualvar$
%The optimization is over state-action visitation distributions $\mu(a,s) \in \Delta^{|\mathcal{S}| \times |\mathcal{A}|} $, and a corresponding policy is obtained via $\pi(a|s) = \mu(a,s) / \sum_a \mu(a,s)$.   
We refer to the constraints as \textit{Bellman flow constraints} \citep{syed2008apprenticeship}, and denote
the set of feasible $\mu$ as $\mathcal{M}$. 
%the feasible set as $\mathcal{M}$. 
%~:=\{\mu(a,s) | \mu \in \Delta^{|\mathcal{S} \times \mathcal{A}|} , \sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick),  \forall s \}$.  

%As shown in \textcolor{red}{Appendix}, these constraints also enforce normalization of $\mu(a,s)$ for normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$.  Finally, the flow constraints reflect the familiar, undiscounted Markov stationarity condition $\sum_{a} \mu(a,s) = \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick)$ when $\gamma = 1$.

%\paragraph{} 
The equivalence between the \gls{LP} in \cref{eq:primal_lp} and the reward-maximization objective in \cref{eq:policy_only} can be seen by writing the marginal state-visitation distribution $\mu(s) \propto (1-\gamma) \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(s_t = s)$, which accounts for discounting and ensures the flow constraints are satisfied with $\mu(a,s) \in \mathcal{M}$. %\RB{Cite}
%that the joint $\mu(a,s) = \mu(s) \pi(a|s)$ factorizes into a marginal $\mu(s)$ which accounts for discounting, and a stationary policy $\pi(a|s)$. 
It can be shown that any stationary policy $\pi(a|s)$ induces a unique state-action 
visitation distribution $\mu(a,s)$, while, conversely, a feasible $\mu(a,s) \in \mathcal{M}$  is induced by some stationary $\pi(a|s)$ \citep{syed2008apprenticeship, agarwal2020rltheorybook}. % Sec. 1.5.2 % \citet{puterman2014markov} Sec. 8.9,
This result allows us to factorize the optimization in \cref{eq:primal_lp} into $\mu(s)\pi(a|s)$ for normalized $\pi(a|s) \in \Delta^{|\mathcal{A}|}$, which matches the optimization in \cref{eq:policy_only}.   Optimizing over $\mu(s)$ yields the unique marginal induced by $\pi(a|s)$.    %The optimal $\mu(s)$ corresponds to the unique marginal induced by $\pi(a|s)$ and ensures the flow constraints are satisfied with $\mu(a,s) \in \mathcal{M}$.
%to obtain a familiar state-wise policy optimization


% The equivalence between this \gls{LP} and the reward-maximization objective in \cref{eq:policy_only} can be seen by substituting the marginal state-visitation distribution $\mu(s) \propto (1-\gamma) \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(s_t = s)$ into \cref{eq:primal_lp}.  
% %, which accounts for discounting and ensures the flow constraints are satisfied with $\mu(a,s) \in \mathcal{M}$. \RB{Cite}
% %that the joint $\mu(a,s) = \mu(s) \pi(a|s)$ factorizes into a marginal $\mu(s)$ which accounts for discounting, and a stationary policy $\pi(a|s)$. 
% It can be shown that any stationary policy $\pi(a|s)$ induces a unique state-action visitation distribution $\mu(a,s)$, while, conversely, a feasible $\mu(a,s) \in \mathcal{M}$  is induced by some stationary $\pi(a|s)$ \citep{syed2008apprenticeship, agarwal2020rltheorybook}. % Sec. 1.5.2 % \citet{puterman2014markov} Sec. 8.9,
% This result allows us to factorize the optimization in \cref{eq:primal_lp} into $\mu(s)\pi(a|s)$ for normalized $\pi(a|s) \in \Delta^{|\mathcal{A}|}$, which matches the optimization in \cref{eq:policy_only}.   The optimization over $\mu(s)$ corresponds to the unique marginal induced by $\pi(a|s)$ and ensures the flow constraints are satisfied with $\mu(a,s) \in \mathcal{M}$.


\paragraph{Regularized Case}
We now consider regularizing the objective in \cref{eq:primal_lp} using a convex penalty function $\Omega$ with coefficient $1/\beta$.   
Letting $\Omega_{\pi_0}(\pi)$ be a statistical divergence between the policy and a reference distribution $\pi_0(a|s)$, we define the regularized $\mathcal{R}_{\Omega, \beta}(r)$~\footnote{We focus on policy regularization in this work, although similar reasoning may be applied to regularization of the joint-state action distribution $\mu(a,s)$ \citep{nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.} 
\begin{equation}
\resizebox{.9\columnwidth}{!}{\hspace*{-.2cm} $
   \mathcal{R}_{\Omega, \beta}(r) :=  \max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}} %\max \limits_{\pi(a|s) \in \Delta^{|A|}} 
   \blangle \mu(s)\pi(a|s), r(a,s) \brangle - \dfrac{1}{\beta}  \blangle \mu(s), \Omega_{\pi_0}(\pi) \brangle $  %\text{subj. to} \, \sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \, \forall s \in \mathcal{S} \label{eq:primal_lp}
   }\label{eq:primal_reg}
\end{equation}
%\normalsize
where we use $\mu(s) \rightarrow \mathcal{M}$ to indicate that $\mu(s)$ induces $\mu(a,s) \in \mathcal{M}$ for a given $\pi(a|s)$.    

% Comparing the form of \cref{eq:primal_reg} with the definition of $\Omega^{*}_{\pi_0,\beta}$ in \cref{eq:conjstar}, 
% we can recognize the regularized objective as corresponding to a conjugate optimization at each state
% %so that the value of the regularized objective 
% $ \mathcal{R}_{\Omega, \beta}(r) = \blangle \mu(s), \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(r) \brangle$, with the environment rewards $r(a,s)$ as the argument.   

%and an outer expectation over the discounted marginal visitation $\mu(s)$. 

%However, this expression is not useful in practice and an outer expectation with respect to the discounted marginal visitation $\mu(s)$. 
%However, this expression is not useful in practice, both because an agent must explore the environment without full knowledge of $r(a,s)$ and because the marginal $\mu(s)$ is intractable to sample.  
%We will observe more practical forms utilizing the conjugate in te
% \begin{align}
%     \mathcal{R}_{\Omega, \beta}(r) = \max \limits_{\mu(s) \rightarrow \mathcal{M}} \blangle \mu(s), \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(r) \brangle
% \end{align}
% where we include the constraint $\pi(a|s)\in \Delta^{|A|}$ in the definition of $\Omega^{*}_{\pi_0,\beta}$ (see \mysec{conj_examples}).
%$\langle \mu(s),  \frac{1}{\beta} \Omega^{*}_{\pi_0, \beta}(r) \rangle $


\subsection{Dual Formulations}\label{sec:dual}
\paragraph{Unregularized Case} 
The flow constraints in \cref{eq:primal_lp} are insightful, as they lead to a dual optimization reflecting the familiar Bellman equations \citep{bellman1957markovian}.    Introducing Lagrange multipliers $V(s)$ for each constraint, summing over $s \in \mathcal{S}$, and eliminating $\mu(a,s)$ by setting $d/d\mu(a,s) = 0$ yields the \textit{dual} %problem 
% Introducing Lagrange multipliers $V(s)$ for each constraint and summing over $s \in \mathcal{S}$, %we obtain the Lagrangian,
% \begin{align}
%     \max \limits_{\mu(a,s)} \min \limits_{V(s)} \, & \big \langle \mu(a,s), r(a,s) + \gamma \transitionv -V(s) \big \rangle \nonumber  \\
%     &+ (1-\gamma) \big\langle \nu_0, V(s) \big  \rangle \label{eq:dual_unreg}
% \end{align}
% where we have reindexed the transition tuple $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared with \cref{eq:primal_lp}.   Eliminating $\mu$ by setting $d/d\mu = 0$ yields a constraint in the \textit{dual} problem 
% %$\sum_{a\tick,s\tick} P(s|a\tick,s\tick) \mu(a,s)$ to $\sum_{a,s} P(s\tick|a,s) \mu(a,s)$
% % Indeed, this equivalence is supported by the result that each stationary policy $\pi(a|s)$ induces a unique $\mu(a,s)$ for a given $\nu_0(s)$ (\citet{puterman2014markov} Sec. 8.9, )
\begin{align}
  &\mathcal{R}^{*}(r):=\min \limits_{V(s)} \,  (1-\gamma) \big \langle \nu_0(s), V(s) \big \rangle \, \text{  subj to: }\, \label{eq:dual_lp} \\ %\quad \forall (s,a) \in \mathcal{S} \times \mathcal{A}
  & \, V(s) \geq r(s,a) + \gamma \transitionv  , \, \, \forall (s,a) \in \mathcal{S} \times \mathcal{A}  \nonumber \, ,
\end{align}
where $\transitionv$ is shorthand for $\mathbb{E}_{P(s\tick|a,s)}[ V(s\tick)]$, and we have reindexed the transition tuple $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared with \cref{eq:primal_lp}.
%See \citet{wang2007dual} for detailed discussion of algorithms solving the unregularized dual problem.

\paragraph{Regularized Case}
%convex conjugate function $\Omega^*_{\pi_0, \beta}(\dualvar)$, which we formally review in \mysec{conjugate} 
We can similarly derive dual versions of the regularized \gls{LP}, starting from a Lagrangian relaxation of \cref{eq:primal_reg}
%\max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}}
% \begin{align}
%     %\mathcal{L}(\mu, V, \Omega) := 
%     & \min \limits_{V(s)} \max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}} \, 
%      (1-\gamma) \big\langle \nu_0, V(s) \big  \rangle \\
%      + &\blangle \mu(s)\pi(a|s), r(a,s) +  \gamma \transitionv -V(s) \big \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \nonumber \\
%     &   \label{eq:lagrangian}\, ,
% \end{align}
\resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
\begin{align}
   &  \max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}} \min \limits_{V(s)}  \, 
     (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle  \label{eq:dual_lagrangian} \\
     + &\blangle \mu(s)\pi(a|s), r(a,s) +  \gamma \transitionv -V(s) - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \brangle \nonumber
\end{align}
}}
% \begin{equation}
%  \begin{array}{l}
%     \max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}} \min \limits_{V(s)}  \, 
%      (1-\gamma) \big\langle \nu_0, V(s) \big  \rangle  \label{eq:dual_lagrangian} \\[1.25ex]
%     \resizebox{\columnwidth}{!}{ + \blangle \mu(s)\pi(a|s), r(a,s) +  \gamma \transitionv -V(s)  - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \brangle } \nonumber
%     \end{array}
% \end{equation}
%We discuss two dual optimizations interpretations here, which will use similar analysis tools as used later in the paper. 
Swapping the order of optimization using strong duality \citep{agarwal2020rltheorybook}, we recognize the maximization over ${\pi(a|s)\in\Delta^{|A|}}$ as a conjugate function, leading to a regularized dual optimization
\resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
 \begin{align}
 \hspace*{-.2cm} &  \mathcal{R}_{\Omega, \beta}^{*}(r) = \min \limits_{V(s)} %\max \limits_{ \mu(s) \rightarrow \mathcal{M}}
 \,  (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle  \label{eq:dual_reg} \\ 
 &+ \mathbb{E}_{\mu(s)} \bigg[\, \frac{1}{\beta}\Omega^{*}_{\pi_0, \beta} \bigg(r(a,s) +  \gamma \transitionv -V(s) \bigg)  \bigg] \nonumber
\end{align}
}}
which is unconstrained, in contrast to \cref{eq:dual_lp}. %, and involves sampling under the induced marginal distribution $\mu(s)$. 
Dual objectives of this form appear variously in \citep{ying2020note,   nachum2020reinforcement, basserrano2021logistic, husain2021regularized, belousov2019entropic}, %although alternative choices must be made to avoid sampling from the intractable $\mu(s)$.
although it is often infeasible to sample from the induced marginal $\mu(s)$. % induced by $\pi(a|s)$.
In both cases, note that the optimization is over the dual variables $V(s)$ only.

\subsection{Soft Value Aggregation}\label{sec:valueaggregation}
%\RB{This is an optimization in terms of $\pi$, not $V(s)$}
Our main object of interest in the rest of the paper will be an alternative decomposition of the Lagrangian %dual 
in \cref{eq:dual_lagrangian}.
%mention a further decomposition the Lagrangian dual in \cref{eq:dual_lagrangian}.
%We mention a further decomposition of the Lagrangian dual to highlight an approach used later in the paper.  
% from \cref{eq:dual_lagrangian}
Eliminating $\mu(s)$ by setting $d/d\mu(s) = 0$, we obtain a condition known as the \textit{regularized Bellman operator} \citep{neu2017unified, geist2019theory}
%\resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
\small
\begin{align}
    V(s)  = \blangle \pi(a|s), \, r(s,a) + \gamma \transitionv \brangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \nonumber . % \label{eq:reg_bell}
\end{align}
\normalsize
%}}
% using fact that $V(s)$ is not a function of the action $a$. % $\pi(a|s)$.  
Eliminating $\mu(s)$ thus leads to a constraint on the form of $V(s)$, since both may be viewed as enforcing the Bellman flow constraints.  Plugging this expression back into the Lagrangian \cref{eq:dual_lagrangian} and removing the minimization over $V(s)$, we are left with only the initial state term and a maximization over $\pi(a|s) \in \Delta^{|\mathcal{A}|}$.
%, where the policy appears in the above expression for the value function $V(s)$.  

%This translates to a constraint of $V(s)$, so that we can remove minimization over the value function and plug this expression back into the Lagrangian \cref{eq:dual_lagrangian}.   We are left with only the initial state term and a maximization over $\pi(a|s) \in \Delta^{|\mathcal{A}|}$, where the policy appears in the above expression for the value function $V(s)$.  
%However, the above expression for the value function $V(s)$. %in \cref{eq:reg_bell} still depends on the policy, with a maximization over $\pi(a|s) \in \Delta^{|\mathcal{A}|}$.  

Recalling the definition of the state-action value, or $Q$ function, ${Q_V(s,a)= r(s,a) + \gamma \transitionv}$, which is recursively defined in terms of value function estimates $V(s\tick)$, we obtain the following optimization %\gamma \mathbb{E}_{P(s'|s,a)}[V(s')]
\resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
\begin{align}
    &\mathcal{R}_{\Omega, \beta}^{*}(r) = \, \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}} (1-\gamma) \, \blangle \nu_0(s) , V(s) \brangle \label{eq:bellman_reg} \\
    & \,\, \text{subj. \footnotesize $ V(s)= \blangle \pi(a|s), r(s,a) + \gamma \transitionv \brangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) $} \nonumber \\[1.25ex]
    &\text{\footnotesize$=(1-\gamma) \mathbb{E}_{\nu_0} \big[\max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \langle \pi(a|s), Q(s,a)  \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \big]$}  \label{eq:soft_bellman}
\end{align}
}}
\normalsize
This conveniently involves expectations under $\nu_0(s)$ only, and leads to `soft' versions of standard \gls{RL} algorithms such as value iteration (e.g. \citet{haarnoja17a, geist2019theory}).    
In the following sections, we interpret the regularized policy optimization in \cref{eq:soft_bellman}, which corresponds to the conjugate function $\frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$, as a two player game between an agent and an imagined adversary \citep{ortega2014adversarial}.
In \cref{fig:value_agga}, we visualize the optimal value function $V_*(s) = \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$, for \textsc{kl} or $\alpha$-divergence regularization and different choices of regularization strength $1/\beta$.   
The choice of divergence particularly affects the aggregated value for low regularization, although we do not observe a clear pattern with respect to $\alpha$.\footnote{See \citet{belousov2019entropic, lee2018sparse, lee2019tsallis}, or \cref{app:alpha_results} for additional discussion of the effect of $\alpha$-divergence regularization on learned policies.}
In all cases, the value function ranges between $\max_a Q(a,s)$ for an unregularized deterministic policy as $\beta \rightarrow \infty$, and the expectation under the reference policy $\mathbb{E}_{\pi_0}[Q(a,s)]$ for strong regularization as $\beta \rightarrow 0$.   We further discuss this property in Sec. \ref{sec:discussion}, and provide closed forms for $V_*(s)$ and the optimal policy below.   


% Recalling the definition of the state-action value, or $Q$ function $Q(s,a)= r(s,a) + \gamma \mathbb{E}_{P(s'|s,a)}[V(s')]$
% and plugging \cref{eq:reg_bell} back into the Lagrangian \cref{eq:lagrangian}, 

% The remaining optimization also corresponds to a conjugate optimization, so
% %We write the remaining optimization over $\pi(a|s)$, which must be normalized to satisfy the flow constraints, as
% % obtain a familiar optimization involving the initial state distribution
% \begin{align}
%     \mathcal{R}^{*}(r) = \, (1-\gamma) \, \mathbb{E}_{\nu_0(s)} \bigg[  \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}} \big\langle \pi(a|s), Q(s,a) \big \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi)  \bigg]  \,. \label{eq:bellman_reg}
% \end{align}
% where the term inside the expectation is 
% %which is the expected value of 
% the regularized Bellman \textit{optimality} operator $[\mathcal{T}_{*,\pi, \Omega_{\pi_0}, \beta} V](s) = \Omega^{*}_{\pi_0, \beta}(Q)$ \citep{neu2017unified, geist2019theory}, which is a contractive mapping and leads to various `soft' value iteration algorithms \citep{littman1996generalized, tishby2011information, fox2016taming, asadi2017alternative, haarnoja17a, lee2019tsallis}.



% \subsection{Convex Conjugate}\label{sec:conjugate}\label{sec:conj_examples}

% \paragraph{KL Divergence}

\subsection{Conjugate Function Examples}\label{sec:conj_examples}
% In this work, 
We consider regularization using the family of $\alpha$-divergences \citep{amari2016information, zhang2004divergence}, which includes both the forward and reverse \textsc{kl} divergences as special cases. 
We take the slightly non-standard step of writing divergences over unnormalized measures rather than probability distributions.  To see why this is useful, consider introducing a Lagrange multiplier to enforce the normalization constraint $\pi(a|s) \in \Delta^{|\mathcal{A}|}$ in \cref{eq:primal_reg}.   
In order to evaluate this relaxation,  the regularizer $\Omega_{\pi_0}(\pi)$ must be able to take unnormalized $\tpi(a|s) \not \in \Delta^{|\mathcal{A}|}$ as input. % in order to evaluate this expression.   

\paragraph{$\alpha$-Divergence} The $\alpha$-divergence over possibly unnormalized measures is defined as 
\small
\begin{align}
\hspace*{-.15cm} D_{\alpha}[\tpi_0:\tpi] = 
    \frac{1}{\alpha(1-\alpha)}\bigg( &  (1-\alpha) \sum \limits_{a \in \mathcal{A}}  \tpi_0(a|s) + \alpha \sum \limits_{a \in \mathcal{A}} \tpi(a|s) \nonumber \\
    &- \sum \limits_{a \in \mathcal{A}} \tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} \bigg) 
\end{align}
\normalsize
We distinguish between the conjugate function $\alphaconju$ and the conjugate with restriction to normalized distributions $\alphaconjn$  \citep{ruderman2012tighter}, with detailed discussion in \myapp{alpha_conj_all}.  The latter appears in defining the optimal value function in \cref{eq:primal_reg} and \cref{eq:soft_bellman}, 
\small
\begin{align}
    V_*(s) &= \alphaconjn(Q) = \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \blangle \pi(a|s), Q(a,s) \brangle -  \frac{1}{\beta}\Omega^{(\alpha)}_{\tpi_0,\beta}(\pi) \nonumber \\
    &= \frac{\alpha-1}{\alpha} \blangle \piopt(a|s), Q(a,s) \brangle + \frac{1}{\alpha} \normalizeralpha \label{eq:alpha_conj_norm_main}
\end{align}
\normalsize
where $\normalizeralpha$ is the normalization constant for the optimizing argument $\piopt(a|s)$ associated with $Q(a,s)$ %the dual variable 
\small
\begin{align}
   \hspace*{-.2cm} \piopt(a|s) = \pi_0(a|s) \, [1+(\alpha-1) \beta \cdot \big( Q(a,s) - \normalizeralpha \big) ]_+^{\frac{1}{\alpha-1}} \label{eq:alpha_opt_policy}
\end{align}
\normalsize
%See \myapp{alpha_conj_all} for derivations.  
The $\alpha$-divergence is also closely related to the Tsallis entropy \citep{lee2019tsallis}, as discussed in \ref{app:tsallis}.  
Unfortunately, the normalizer $\normalizeralpha$ appears inside the exponent and must be estimated numerically apart from special cases of $\alpha$ \citep{lee2019tsallis}.\footnote{\citet{wong2021tsallis} provide justification for a multiplicative normalization constant, but this is no longer directly related to the expected reward objective.}

We visualize the optimal value $V_*(s)$ and the normalization constant $\normalizeralpha$ as a function of $\alpha$ in \cref{fig:value_aggb}.   Apart from the case when $\alpha = 1$ as discussed below, we have $V_*(s) \neq \normalizeralpha$ in  \cref{eq:alpha_conj_norm_main}. 
% Also, notice that $V_*(s) \neq \normalizer$ except for when $\alpha = 1$, as discussed below and shown in \cref{fig:value_aggb}. 

\begin{figure}[t]
\begin{subfigure}{0.47\columnwidth}\includegraphics[width=\textwidth]{figs/value_agg/prior_uniform.pdf}
%\vspace*{.15cm}
\caption{$V(s)$ as a function of $\beta$}\label{fig:value_agga}\end{subfigure}\hspace*{.01\columnwidth}
\begin{subfigure}{0.52\columnwidth} 
% \vspace*{-.12cm}\includegraphics[scale=.3]{figs/conj_by_alpha/value_norm_beta1_vert.pdf}
\vspace*{-.1cm}\includegraphics[width=.96\textwidth]{figs/conj_by_alpha/value_norm_beta1_vert_thin.pdf}
\caption{$V(s)$ and $\psi_{\alpha}(s)$ as a function of $\alpha$ for $\beta=1$}\label{fig:value_aggb}\end{subfigure}
\caption{Optimal value function $V_*(s)$ and normalization constant $\psi_{\alpha}(s)$ as a function of $\beta$ (left) and $\alpha$ (right), using $Q(a,s)$ and $\pi_0(a|s)$ from the left inset.   See \cref{eq:alpha_conj_norm_main} and \cref{eq:kl_v} for closed forms. }\label{fig:value_agg_main}
\end{figure}


\paragraph{KL Divergence}
Taking the limit as $\alpha \rightarrow 1$, we obtain an extended version of the \textsc{kl} divergence commonly used as regularization for \gls{RL} 
% (\citet{tishby2011information, ortega2013thermodynamics, fox2016taming})
\small
\begin{align}
    \hspace*{-.15cm} D_{KL}[\tpi:\tpi_0] = \sum \limits_{a \in \mathcal{A}} \tpi(a|s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} - \tpi(a|s) + \tpi_0(a|s) \, . \nonumber
    %\sum \limits_{a \in \mathcal{A}} %\lim_{\alpha \rightarrow 1}
\end{align}
\normalsize
The value function, or conjugate $\frac{1}{\beta}\Omega^*_{\pi_0,\beta}(Q)$, as a function $Q$ and with restriction to normalized $\pi$ becomes
\small
\begin{align}
  \hspace*{-.2cm} V_*(s) = \frac{1}{\beta}\Omega^*_{\pi_0,\beta}(Q) = \frac{1}{\beta} \log \sum \limits_{a \in \mathcal{A}} \pi_0(a|s) \expof{\beta \cdot Q(a,s)}. \label{eq:kl_v}
\end{align}
\normalsize
%For the \textsc{kl} divergence, 
This matches the normalization constant for the optimal policy, with $V_*(s) = \psi(s;\beta)$ and
 \begin{align}
 \pi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s) -  \psi(s;\beta)\big)} \, ,\label{eq:kl_opt_policy}
 \end{align}
 This can also be seen by plugging $\alpha = 1$ into \cref{eq:alpha_conj_norm_main}.
 %after projection of unnormalized $\tpi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s)}$ onto the simplex $\Delta^{|\mathcal{A}|}$, with $\psi(s;\beta) = \frac{1}{\beta} \log \sum_a \pi_0(a|s) \expof{\beta \cdot Q(a,s)}$ enforcing normalization.

% \paragraph{$\alpha$-Divergence}
% \paragraph{Soft Value Aggregation}
% %\subsection{Soft Value Aggregation}\mysec{valueaggregation}
% In the following sections, we will interpret the regularized policy optimization in \cref{eq:primal_reg} or \cref{eq:soft_bellman} as a two player game between an agent and an imagined adversary \citep{ortega2014adversarial}.   
% We present this adversarial interpretation, which depends on the regularization function $\Omega_{\pi_0}(\pi)$ and strength $1/\beta$, in \mysec{adversarial_perturb}.
% %In \cref{fig:value_agg}, we visualize % and divergence 

% The value function $V(s)$, which measures the expected payoff for an agent with estimated values $\{Q(s,a), V(s)\}$ acting in a given \gls{MDP} starting from state $s \in \mathcal{S}$, depends on the strength and form of the regularization.  The value ranges between $\max_a Q(a,s)$ for a deterministic policy and weak adversaries as $\beta \rightarrow \infty$, and the expectation under the reference policy $\mathbb{E}_{\pi_0}[Q(a,s)]$ for strong adversaries as $\beta \rightarrow 0$.    In \cref{fig:value_agg}, we visualize $V(s) = \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ using the \textsc{kl} divergence or $\alpha$-divergence for regularization $\Omega_{\pi_0}(\pi)$ and different
% choices of regularization strength $1/\beta$.
% %$\beta$ and $\Omega_{\pi_0}(\pi)$ in  \cref{fig:value_agg}.

% %When viewing game theoretic terms, this is known as the \textit{certainty equivalent}

% %We will proceed to characterize this adversary in terms of  in terms of the regularization strength ($\beta$) and divergence $\Omega_{\pi_0}(\pi)$.
% %Note that high regularization or low $\beta$ indicates a weak adversary, so that the policy becomes increasingly greedily with respect to $Q(a,s)$. 


% Finally, the conjugacy conditions in \cref{eq:optimal_policy_as_grad} provide a closed form for the policy in terms of $Q(a,s)$ for each state in \cref{eq:soft_bellman}.   For \textsc{kl} divergence regularization,
%   \begin{align}
%  \pi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s) -  \psi(s;\beta)\big)} \label{eq:opt_policy}
%  \end{align}
%  after projection of unnormalized $\tpi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s)}$ onto the simplex $\Delta^{|\mathcal{A}|}$, with $\psi(s;\beta) = \frac{1}{\beta} \log \sum_a \pi_0(a|s) \expof{\beta \cdot Q(a,s)}$ enforcing normalization.
 
 


==> old/2_perturbed.tex <==
\section{Adversarial Reward Perturbations}\label{sec:adversarial_perturb}
% Several previous works have leveraged the convex programming tools from the previous section to interpret regularized policies as being robust to adversarial perturbations of the reward function \citep{ortega2014adversarial, eysenbach2021maximum, husain2021regularized}. 
% Previous work \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum} has analyzed the robustness of regularized policies to adversarial perturbations to the environment reward function using convex duality.  We extend the analysis of \citet{ortega2014adversarial} to the sequential setting, and clarify the characterization of the feasible set of adversarial perturbations compared to \citep{eysenbach2021maximum}.      

In this section, we analyze the robustness of regularized policies to adversarial perturbations of the reward function, which arises from an alternative application of convex duality for regularized \gls{RL} objectives.    We draw connections with similar interpretations from \citet{ortega2014adversarial, eysenbach2021maximum, husain2021regularized} throughout our exposition, with additional discussion in \mysec{discussion}.
%Our analysis extends \citet{ortega2014adversarial} to the sequential setting and clarifies the feasible set of reward perturbations available to the adversary from \citet{eysenbach2021maximum}.  We discuss additional connections with related work in \mysec{discussion}.
%Building upon previous work, we extend the analysis of \citet{ortega2014adversarial} to the sequential setting, provide a precise characterization of the feasible set of reward perturbations available to the adversary \citep{eysenbach2021maximum},    

%We build upon previous work \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum} to characterize 
%, which suggests that stochastic policies are robust to adversarial perturbations of the environmental reward function.   
%We build upon previous work \citep{ortega2014adversarial, husain2021regularized, eysenbach2021maximum} to characterize 
% which highlights the need for careful, game-theoretic analysis of reward robustness. % described in \citet{eysenbach2021maximum}.  
% %resolve counter-intuitive conclusions based on the
% Compared with \citet{eysenbach2021maximum}, we clarify the characterization of the feasible set of adversarial perturbations, resolve several unintuitive properties arising from entropy rather than divergence regularization,
% and provide further visualizations and derivations for the $\alpha$-divergence. 


% \paragraph{Conjugate Functions}
% Throughout this section, we utilize the conjugate of the \KL divergence over unnormalized measures \citep{zhang2004divergence} \footnote{\textcolor{red}{This extended \KL divergence matches the $\alpha$-divergence over unnormalized measures for $\alpha = \{0,1\}$.}} for simplicity.  
% \RB{Choose to enforce later}
% \begin{align}
%     &\Omega_{\tpi_0}(\tpi) = D_{KL}[\tpi(a|s):\tpi_0(a|s)] \\
%     &\phantom{\Omega_{\tpi}} :=  \sum \limits_{a} \tpi(a|s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} - \sum \limits_{a} \tpi(a|s) + \sum \limits_{a} \tpi_0(a|s) \nonumber
% \end{align}
% % \frac{1}{\beta} \sum \limits_{a} \tpi_0 \expof{\beta \cdot \dualvar} - \tpi_0
% with the conjugate of the scaled $\frac{1}{\beta} \Omega_{\tpi_0}(\tpi)$ equal to 
% \begin{align}
%   \frac{1}{\beta} \Omega^{*}_{\tpi_0,\beta}&(\dualvar) = \frac{1}{\beta} \sum \limits_{a} \tpi_0 \expof{\beta \cdot \dualvar} - \frac{1}{\beta} \sum \limits_{a} \tpi_0
% \end{align}
% See \myapp{kl_conj_all} for derivations.  We provide additional discussion of the $\alpha$-divergence, which is essentially identical to the Tsallis divergence used in \citep{lee2019tsallis}, in \myapp{alpha_conj_all}.  
% \footnote{Studying the $\alpha$-divergence allows disentangling the role of the conjugate function $\frac{1}{\beta}\Omega^{*}_{\tpi_0,\beta}$ and the policy normalization constant, which both match the value function $V(s)$ in the case of the \KL divergence. Compared with the Tsallis entropy \citep{lee2019tsallis}, the $\alpha$-divergence conveniently avoids a $1/\alpha$ factor in the solution to the conjugate optimization, with $\alpha = q$.}
% %and an interpretation of regularization and value aggregation.

%\paragraph{Conjugate Policy Representation}
\subsection{Policy-Based Interpretation}
We have seen that the conjugate optimization provides an alternative representation of a convex regularizer %$\frac{1}{\beta}\Omega_{\pi_0}(\pi)$.   
 \begin{align}
     \hspace*{-.2cm} \frac{1}{\beta} \Omega_{\tpi_0}(\tpi) = \max_{\pr} \big \langle \tpi(a|s), \pr(a,s) \big \rangle - \frac{1}{\beta}  \Omega^{*}(\pr) \, .\label{eq:conjomega2}
 \end{align}
Expanding the regularization term in \cref{eq:dual_lagrangian} using the conjugate function, we have %\cref{eq:conjomega} %$\Omega_{\pi_0}(\pi)$
\begin{align}
    \hspace*{-.2cm} & \quad \max \limits_{\mu(s) \rightarrow \mathcal{M}} \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s)} \min \limits_{\textcolor{\highlight}{\perturbr(a,s)}} \, \label{eq:pedro_form} \\
    & \big \langle {\mu(s)\pi(a|s)}, {r(a,s) +\gamma \transitionv - V(s) - \textcolor{\highlight}{\perturbr(a,s)}} \brangle  \nonumber  \\
    & \qquad + \frac{1}{\beta} \Omega^{*}_{\tpi_0, \beta} \big( \textcolor{\highlight}{\perturbr(a,s)} \big) + (1-\gamma) \blangle \nu_0(s), V(s) \brangle \, ,  \nonumber
\end{align}
where we change the maximization in \cref{eq:conjomega2} to a minimization since the \KL divergence is subtracted.
Optimizations over $\mu(s)$ or $V(s)$ enforce the Bellman flow constraints across states of the \gls{MDP}.

%This expression extends the single-step case in \citet{ortega2014adversarial} to the discounted, infinite-horizon setting.   
As in \citet{ortega2014adversarial}, we interpret this minmax optimization as a two player game in each state, between an agent which chooses a policy $\pi(a|s)$, and an imagined adversary which chooses a reward perturbation $\perturbr(a,s)$. %to minimize the objective.  
Notice that the adversary is penalized for large reward perturbations, with a cost measured by the conjugate function ${\Omega^{*}_{\tpi_0, \beta}(\perturbr)}$. %\geq 0 (only when $\pi$ is normalized)
%which is nonnegative and increasing in $\pr$ in our case.
%which we assume to be increasing and nonnegative \citep{husain2021regularized}. 

In the following proposition, we translate this cost function to a constraint on the feasible set of reward perturbations $\pr$ available to the adversary at a given regularization function $\Omega_{\tpi_0}$ with strength $1/\beta$. We also characterize the optimal adversarial reward perturbations, with detailed proofs in \myapp{kl_perturb_section} and \myapp{alpha_perturb}. 
% From this feasible set,
%dversarial %We solve for the optimal adversarial reward perturbations. 
\begin{proposition} \label{prop:perturbations}
Using \KL divergence regularization $\Omega_{\tpi_0} = D_{KL}[\tpi:\tpi_0]$, we have the following results:
\begin{enumerate}[label=(\alph*)]
% \item The unconstrained optimization in \cref{eq:pedro_form} corresponds to the following constrained optimization
% \small
% \begin{align}
%     %&\max \limits_{\mu(s) \rightarrow \mathcal{M}} \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s)} \min
%     &\hspace*{-.4cm} \max \limits_{\mu(s), \pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s),\perturbr(a,s)} (1-\gamma) \blangle \nu_0(s), V(s) \brangle \label{eq:constraint_set} \\[1.25ex]
%     & \scriptsize \hspace*{-.55cm} {+ \big \langle {\mu(s)\pi(a|s)}, {r(a,s) +\gamma \transitionv - V(s) - \perturbr(a,s)} \brangle  } \nonumber  \\[1.5ex]
%     & \hspace*{-.55cm} \text{subj.} \sum \limits_{a} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} \leq \sum \limits_{a} \pi(a|s)  \, \, \forall s \in \mathcal{S} \nonumber
%     %\frac{1}{\beta} \Omega^{*}_{\textcolor{red}{\tpi_0}, \beta} \big( \perturbr(a,s) \big)
% \end{align}
% \normalsize
% where the constraint arises from the conjugate function $\Omega^{*}_{\tpi_0,\beta}(\pr)$.% = \frac{1}{\beta} \sum \limits_{a} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} - \frac{1}{\beta}\sum \limits_{a} \pi_0(a|s)$.
\item 
For a given policy $\pi(a|s)$, the unconstrained optimization over $\pr(a,s)$ in \cref{eq:pedro_form} corresponds to the following constrained optimization
\small
\begin{align}
    %&\max \limits_{\mu(s) \rightarrow \mathcal{M}} \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s)} \min
    &\hspace*{-.4cm}  \min \limits_{\perturbr(a,s)} (1-\gamma) \blangle \nu_0(s), V(s) \brangle \label{eq:constraint_set} \\[1.25ex]
    & \scriptsize \hspace*{-.55cm} {+ \big \langle {\mu(s)\pi(a|s)}, {r(a,s) +\gamma \transitionv - V(s) - \perturbr(a,s)} \brangle  } \nonumber  \\[1.5ex]
    & \hspace*{-.55cm} \text{subj.} \sum \limits_{a} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} \leq \sum \limits_{a} \pi(a|s)  \, \, \forall s \in \mathcal{S} \nonumber
    %\frac{1}{\beta} \Omega^{*}_{\textcolor{red}{\tpi_0}, \beta} \big( \perturbr(a,s) \big)
\end{align}
\normalsize
where the constraint arises from the conjugate function $\Omega^{*}_{\tpi_0,\beta}(\pr)$.
\item The optimal strategy for the adversary is to choose reward perturbations equal to
\begin{align}
    \propt(a,s) = \frac{1}{\beta} \log \frac{\tpi(a|s)}{\tpi_0(a|s)} \label{eq:optimal_perturbed}
\end{align}
\end{enumerate}
\end{proposition}
% \begin{proof}
% See \myapp{kl_perturb_section}
% \end{proof}
\begin{proposition} \label{prop:perturbations_alpha}
Using $\alpha$-divergence regularization $\Omega_{\tpi_0} = D_{\alpha}[\tpi_0:\tpi]$, we have the following results:
\begin{enumerate}[label=(\alph*)]
\item For a given $\pi(a|s)$, the unconstrained optimization over $\pr(a,s)$ from \cref{eq:pedro_form} translates to the same minimization objective as in \myprop{perturbations}(a), with the following constraint 
\small
\begin{align}
      \hspace*{-.4cm} \sum \limits_{a \in \mathcal{A}} &\tpi_0(a|s) [1 + (\alpha-1) \beta \cdot \pr(a,s) ]_+^{\frac{\alpha}{\alpha-1}} \label{eq:constraint_set_alpha}  \\
      &\leq \sum \limits_{a \in \mathcal{A}} \tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} \quad \forall s \in \mathcal{S} \nonumber
      %\hspace*{-.5cm}\alphaconju(\pr) \leq  \, \frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a \in \mathcal{A}} \tpi_0(a|s) \left(\frac{\tpi(a|s)}{\tpi_0(a|s)}^{\alpha} -1 \right) \,\, \forall s \in \mathcal{S} \nonumber
      %\tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} - \frac{1}{\beta} \frac{1}{\alpha} \sum \limits_{a \in \mathcal{A}} \tpi_0(a|s) \quad \forall s \in \mathcal{S} 
\end{align}
\normalsize
where the constraint arises from the conjugate function $\Omega^{*(\alpha)}_{\tpi_0,\beta}(\pr)$.
\item The optimal strategy for the adversary is to choose reward perturbations equal to
\begin{align}
    \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \frac{\tpi(a|s)}{\tpi_0(a|s)} 
\end{align}
where %$\log_{\alpha}u:= \frac{1}{\alpha-1} \left( u^{\alpha-1} - 1\right)$.
$\log_{\alpha}\frac{\tpi(a|s)}{\tpi_0(a|s)}:= \frac{1}{\alpha-1} \left( \frac{\tpi(a|s)}{\tpi_0(a|s)}^{\alpha-1} - 1\right)$.
\end{enumerate}
\end{proposition}
% \begin{proof}
% See \myapp{alpha_perturb}.  \RB{Combine props?}
% \end{proof}
%We discuss these results in the rest of the section.

% \begin{proposition}
% For the \KL divergence over normalized distributions and the constrained conjugate optimization,
% %$\Omega^{*}_{\pi_0,\beta}(\pr) = \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \langle \pi, \pr \rangle - \Omega_{\pi_0}(\pi)$, 
% the optimal reward perturbations are defined in self-consistent fashion:
%  \begin{align}
%   \propt(a,s) =& \frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)} \label{eq:normalized_rewards} \\ 
%   &+ \frac{1}{\beta} \log \sum \limits_{a} \pi_0(a|s)  \expof{\beta \cdot \propt(a,s)} \nonumber
% \end{align}
% where $\frac{1}{\beta} \log \sum \limits_{a} \pi_0(a|s)  \expof{\beta \cdot \pr(a,s)}$ reflects the additive normalization constant of $\pi(a|s) \in \Delta^{|\mathcal{A}|}$.
% \normalsize
% \end{proposition}
% \begin{proof}
% See \myapp{kl_perturb_section}
% \end{proof}

% \begin{figure*}[t]
% \centering
% % \begin{minipage}{\textwidth}%{0.8\textwidth}
% % \centering
% \begin{center}
% \[\arraycolsep=.003\textwidth
% \begin{array}{cccccc} %[width=40mm]
%  \begin{subfigure}{0.07\textwidth} \vspace*{-.24cm} \includegraphics[width=\textwidth]
%  {figs/feasible/uniform_prior.png} \end{subfigure}& %\qquad  \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_01.png}
% {figs/feasible/kl/beta01alpha1uniform.pdf}
% \caption{\label{fig:taba} \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}& % \qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_1.png}
% {figs/feasible/kl/beta1alpha1uniform.pdf}
% \caption{\label{fig:tabb} \centering  $D_{KL}, \beta = 1$}\end{subfigure}& %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_10.png} 
% {figs/feasible/kl/beta10alpha1uniform.pdf}
% \caption{\label{fig:tabc} \centering \small $D_{KL}, \beta = 10$}\end{subfigure}& \rulesep
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
% % {figs/feasible/alpha-1/alpha_neg1_beta1_uniform.png} 
% {figs/feasible/alpha-1/alpha_neg1_beta1_uniform_redo.pdf} 
% \caption{\label{fig:tabd} \centering \small $\alpha = -1, \beta = 1$}\end{subfigure}&
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
% % {figs/feasible/alpha3/alpha3_beta1_uniform.png} 
% {figs/feasible/alpha3/alpha3_beta1_uniform_redo.pdf}
% \caption{\label{fig:tabe} \centering \small $\alpha = 3, \beta = 1$}\end{subfigure}
% \\ %&\hspace*{.2cm}\\
% \begin{subfigure}{0.07\textwidth}\vspace*{-.24cm} \includegraphics[width=\textwidth]{figs/feasible/nonuniform_prior.png}\end{subfigure}& %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_01.png}
% {figs/feasible/kl/beta01alpha1nonuniform.pdf}
% \caption{\label{fig:tabd} \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}& %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_1.png}
% {figs/feasible/kl/beta1alpha1nonuniform.pdf}
% \caption{\label{fig:tabe} \centering \small $D_{KL}, \beta = 1$}\end{subfigure}& %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_10.png} 
% {figs/feasible/kl/beta10alpha1nonuniform.pdf}
% \caption{\label{fig:tabf} \centering \small $D_{KL}, \beta = 10$}\end{subfigure}& \rulesep %\hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/alpha-1/alpha_neg1_beta1_nonuniform.png} 
% {figs/feasible/alpha-1/alpha_neg1_beta1_nonuniform_redo.pdf} 
% \caption{\label{fig:tabi} \centering \small $\alpha = -1, \beta = 1$}\end{subfigure}&
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip] 
% %{figs/feasible/alpha3/alpha3_beta1_nonuniform.png} 
% {figs/feasible/alpha3/alpha3_beta1_nonuniform_redo.pdf} 
% \caption{\label{fig:tabj} \centering \small $\alpha = 3, \beta = 1$}\end{subfigure}
% \end{array}
% \] 
% \end{center}
% % \end{minipage}
% \caption{Feasible Set (red region) for \textsc{kl} divergence (at various $\beta$) and $\alpha$-divergence ($\alpha=\{-1, 3\}, \beta =1$) regularization and fixed $Q(a,s)$ values (blue star).  Red star indicates optimal perturbed reward $\mr = r - \pr$, for optimal $\pi_*(a|s)$ associated with $Q$-values and regularization parameters $\alpha, \beta, \pi_0$ (\cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).  Top row:  $\pi_0=(\frac{1}{2},\frac{1}{2})$, Bottom row: $\pi_0 = (\frac{2}{3}, \frac{1}{3})$.  
% % Red dot indicates $Q(a,s)$ associated with policy $\pi(a|s)$
% }\label{fig:feasible_set_main}
% \end{figure*}
% \begin{figure}[t]
% \centering
% % \begin{minipage}{\textwidth}%{0.8\textwidth}
% % \centering
% % \[\arraycolsep=.003\textwidth
% % \begin{array}{cccccc} %[width=40mm]
%  \begin{subfigure}{0.07\textwidth} 
%  \vspace*{-.24cm} \includegraphics[width=\textwidth]
%  {figs/feasible/uniform_prior.png} 
%  \end{subfigure} % & \qquad  \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_01.png}
% {figs/feasible/kl/beta01alpha1uniform.pdf}
% \caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba} \end{subfigure} %& \qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_1.png}
% {figs/feasible/kl/beta1alpha1uniform.pdf}
% \caption{\label{fig:tabb} \centering  $D_{KL}, \beta = 1$}\end{subfigure} %& \qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_uniform_10.png} 
% {figs/feasible/kl/beta10alpha1uniform.pdf}
% \caption{\label{fig:tabc} \centering \small $D_{KL}, \beta = 10$}\end{subfigure}  
% % & 
% \rulesep
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
% % {figs/feasible/alpha-1/alpha_neg1_beta1_uniform.png} 
% {figs/feasible/alpha-1/alpha_neg1_beta1_uniform_redo.pdf} 
% \caption{\label{fig:tabd} \centering \small $\alpha = -1, \beta = 1$}\end{subfigure}
% % &
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
% % {figs/feasible/alpha3/alpha3_beta1_uniform.png} 
% {figs/feasible/alpha3/alpha3_beta1_uniform_redo.pdf}
% \caption{\label{fig:tabe} \centering \small $\alpha = 3, \beta = 1$}\end{subfigure}
% \\ %&\hspace*{.2cm}\\
% \begin{subfigure}{0.07\textwidth}\vspace*{-.24cm} \includegraphics[width=\textwidth]{figs/feasible/nonuniform_prior.png}\end{subfigure}
% % & %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_01.png}
% {figs/feasible/kl/beta01alpha1nonuniform.pdf}
% \caption{\label{fig:tabd} \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}
% % & %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_1.png}
% {figs/feasible/kl/beta1alpha1nonuniform.pdf}
% \caption{\label{fig:tabe} \centering \small $D_{KL}, \beta = 1$}\end{subfigure}
% % & %\qquad \hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/kl_73_10.png} 
% {figs/feasible/kl/beta10alpha1nonuniform.pdf}
% \caption{\label{fig:tabf} \centering \small $D_{KL}, \beta = 10$}\end{subfigure}
% % & 
% \rulesep %\hspace*{.2cm}
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip]
% % {figs/feasible/alpha-1/alpha_neg1_beta1_nonuniform.png} 
% {figs/feasible/alpha-1/alpha_neg1_beta1_nonuniform_redo.pdf} 
% \caption{\label{fig:tabi} \centering \small $\alpha = -1, \beta = 1$}\end{subfigure}
% % &
% \begin{subfigure}{0.18\textwidth}\includegraphics[width=\textwidth, trim= 5 0 5 0, clip] 
% %{figs/feasible/alpha3/alpha3_beta1_nonuniform.png} 
% {figs/feasible/alpha3/alpha3_beta1_nonuniform_redo.pdf} 
% \caption{\label{fig:tabj} \centering \small $\alpha = 3, \beta = 1$}\end{subfigure}
% % \end{array}
% % \]
% % \end{minipage}
% \caption{Feasible Set (red region) for \textsc{kl} divergence (at various $\beta$) and $\alpha$-divergence ($\alpha=\{-1, 3\}, \beta =1$) regularization and fixed $Q(a,s)$ values (blue star).  Red star indicates optimal perturbed reward $\mr = r - \pr$, for optimal $\pi_*(a|s)$ associated with $Q$-values and regularization parameters $\alpha, \beta, \pi_0$ (\cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).  Top row:  $\pi_0=(\frac{1}{2},\frac{1}{2})$, Bottom row: $\pi_0 = (\frac{2}{3}, \frac{1}{3})$.  
% % Red dot indicates $Q(a,s)$ associated with policy $\pi(a|s)$
% }\label{fig:feasible_set_main}
% \end{figure}

% Note that we have considered the conjugate derived from $\Omega(\tpi)$ over unnormalized density functions, so that normalization of $\pi(a|s)$ %\in \Delta^{|\mathcal{A}|}$ 
% is enforced when solving \cref{eq:pedro_form} for the policy rather than in the definition of the conjugate itself. %$\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}$ itself.  
% This allows us to avoid a self-referential definition of $\propt(a,s)$, which would include an additional $\frac{1}{\beta} \log \sum_{a} \pi_0 \expof{\beta \cdot \pr}$ on the right hand side of \cref{eq:optimal_perturbed}.   See \myapp{kl_perturb_section}.

 \paragraph{Conjugate Policy Representation}
Our derivations so far have only invoked the conjugate representation of the regularization function, which suggests that \textit{any} stochastic policy may be interpreted via an adversarial game once $\Omega, \tpi_0,$ and $\beta$ are known.  %$\frac{1}{\beta} \Omega_{\tpi_0}(\tpi)$ is known.      

By contrast, the analysis of \citet{eysenbach2021maximum} is framed in terms of the robustness associated with a given reward function and regularization scheme, rather than a policy.  While the feasible set for \KL divergence regularization in \cref{eq:constraint_set} can be characterized without reference to a particular policy assuming $\sum_a \pi(a|s) = 1$, %$\pi \in \Delta^{|\mathcal{A}|}$
the optimal reward perturbations and feasible set for the $\alpha$-divergence require knowledge of the policy.   
Unfortunately, associating a policy with a reward function $r(a,s)$ in a given (regularized) \gls{MDP} requires solving for the optimal policy in \cref{eq:primal_reg} or (\ref{eq:bellman_reg}). %in \cref{eq:reg_rl}  
%In order to associate a policy with a reward function and a given \gls{MDP} requires solving for the optimal policy in \cref{eq:reg_rl}.   
%using Shannon entropy regularization, a special case of the \KL divergence.  

% In this case, note that the feasible set can be characterized without reference to a particular policy, assuming $\pi \in \Delta^{|\mathcal{A}|}$.   However, this is not true of the constraint for the $\alpha$-divergence and, in both cases, the optimal reward perturbations depend directly on the policy.   
% Thus, solving for the optimal policy is necessary to fully characterize the robustness of 
% in an \gls{MDP} with reward $r(a,s)$ 
% in order to fully characterize the robustness associated with an \gls{MDP} with reward

% the optimal policy associated with an \gls{MDP} with reward 


% In the case of \KL divergence regularization, note the feasible set of reward functions does not depend on a particular policy and can be calculated directly assuming $\pi \in \Delta^{|\mathcal{A}|}$.   However, for the $\alpha$-divergence, the constraint depends on a particular policy.  

% %Our derivations involving the conjugate $\frac{1}{\beta} \Omega_{\tpi_0}(\tpi)$ in \cref{eq:conjomega2} suggest that any policy may . 
% analysis should begin with a particular policy rather than a given reward function.   To analyze robustness associated with a given reward function and regularization scheme, as in \citet{eysenbach2021maximum}, we would first need to solve for the optimal policy.

 \paragraph{Analyzing the Feasible Set}
In \cref{fig:feasible_set_main}, we visualize the feasible set of perturbed rewards in a two-dimensional action space for the \KL or $\alpha$-divergence, various $\beta$, and uniform or non-uniform priors.    
Since the optimal policy can be calculated easily in the single-step case, we consider $\pi_*(a|s)$ corresponding to fixed $Q(a,s) = [1.1, 0.8]$ for various regularization settings (see \cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).
We determine the feasible set of $\pr(a,s)$ according to the constraint in \cref{eq:constraint_set} or (\ref{eq:constraint_set_alpha}), and plot the modified reward $r\tick(a,s) = Q(a,s) - \pr(a,s)$ for 
 each action.
%  We then plot the modified reward $Q(a,s) - \pr(a,s)$ for each action and draw the feasible set according to \cref{eq:constraint_set}.
% We first fix a stochastic policy $\pi(a|s)$ and use \cref{eq:alpha_opt_policy} or (\ref{eq:kl_opt_policy}) to derive the corresponding $Q$-values, which we plot in blue and will discuss further in \mysec{value_based}.   We then plot the modified reward $Q(a,s) - \pr(a,s)$ for each action and draw the feasible set according to \cref{eq:constraint_set}.

 %reward perturbations should be analyzed with respect to a
%In the single step case, we have $Q(a,s) = r(a,s)$ and plot this as the reward function in blue.   
%We also plot the modified reward $r(a,s) - \pr(a,s)$ for each action and draw the feasible set according to \cref{eq:constraint_set}.   
%penalized for decreasing the reward while increasing both rewards is clearly feasible.  

Inspecting the constraints for the adversary in \cref{eq:constraint_set} and (\ref{eq:constraint_set_alpha}), note that both reward increases $\pr > 0$ and reward decreases $\pr < 0$ contribute non-negative terms which either up- or down-weight the reference policy $\pi_0(a|s)$.    The constraint on their summation forces the adversary to trade off between perturbing the reward at different actions in a particular state.

%  First, note that both reward increases $\pr > 0$ and reward decreases $\pr < 0$ provide a non-negative contribution to the adversary's constraint in \cref{eq:constraint_set}.
%  %at each action $a$.  
%  These terms either up- or down-weight the reference policy $\pi_0(a|s)$ with the resulting summation still equal to $1$, so that this constraint forces the adversary to trade off between perturbing the reward at different actions in a particular state.  % \RB{related to normalization}

For high regularization strength ($\beta=0.1$), we observe that the boundary is nearly linear, with slope $-\frac{\pi_0(a_2|s)}{\pi_0(a_1|s)}$ based on the ratio of each action in the prior.  The boundary steepens for lower regularization strength, with only small decreases in the reward function available.  In all cases, it is natural that increasing the reward in both actions is feasible for an adversary that seeks to minimize the objective in \cref{eq:pedro_form}.

Finally, we visualize the feasible set for the $\alpha$-divergence, with $\alpha \in \{-1, 3\}$ and $\beta = 1$, in \cref{fig:feasible_set_main} 
% \ref{fig:tabd}-\ref{fig:tabe} and \ref{fig:tabi}-\ref{fig:tabj} .  
(d)-(e) and (i)-(j).
For the optimal policy associated with a given reward function,  we see that the $\alpha = -1$ feasible set may not include this reward function.  
%Also note that, if we are given a reward function instead of a policy and are interested in characterizing the feasible set for the $\alpha$-divergence, 
% \RB{Move to discussion later?}
% While \citet{eysenbach2021maximum} display feasible sets arising from (negative) Shannon entropy regularization $\Omega(\pi) = - H(\pi)$, this approach leads to puzzling conclusion that \textit{lower} regularization strength $1/\beta$ leads to \textit{greater} adversarial robustness, with larger feasible sets.   
% In contrast to \cref{eq:optimal_perturbed}, the entropy-regularized policy is `robust' to only positive changes in the reward function $\pr(a,s) \geq 0$, with the optimal perturbed reward $\mr(a,s) = r(a,s) - \pr(a,s) = r(a,s) - \log \pi(a|s)$.   We also observe robustness to large positive reward perturbations for low regularization strength in \cref{fig:perturb_opt}, but the crucial negative reward perturbation arises for the action(s) in the support of the nearly deterministic policy.
% We prefer to characterize `robustness' in terms of \textit{reductions} to the reward function.    

%We also observe robustness to large 
%\RB{Best explanation as to why??}
%This suggests that \textit{all} perturbations contribute to the constraint 
%This interpretation arises from the fact that the entropy is pointwise non-negative
%proceed to characterize the feasible set of adversarial perturbations $\pr(a,s)$ using a constrained version of \cref{eq:pedro_form}, with visualizations in \cref{fig:feasible_set_main}. 

% \paragraph{Constrained Adversary}
% Notice that the adversary is penalized for large reward perturbations, with a cost measured by the conjugate function ${\Omega^{*}_{\tpi_0, \beta}(\perturbr)}$ \textcolor{red}{$\geq 0$}. %\geq 0 (only when $\pi$ is normalized)
% %which is nonnegative and increasing in $\pr$ in our case.
% %which we assume to be increasing and nonnegative \citep{husain2021regularized}. 
% We proceed to characterize the feasible set of reward perturbations $\pr(a,s)$ available to the adversary for a given regularization strength $1/\beta$, with detailed derivations in \myapp{kl_perturb_section}.
% Translating the unconstrained term $\frac{1}{\beta} \Omega^{*}_{\tpi_0, \beta}(\perturbr)$ to a constraint, we obtain
% %we show that a regularization strength of $\frac{1}{\beta}$ in the unconstrained adversarial optimization translates to a constraint
% \begin{align}
%     \hspace*{-.2cm}  \sum \limits_{a} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} \leq 1
% \end{align}
% with the remaining terms in \cref{eq:pedro_form} remaining unchanged.  Note that the adversary pays a non-negative penalty for both reward increases $\pr > 0$ and reward decreases $\pr < 0$ at each action $a$.  These terms either up- or down-weight the reference policy $\pi_0(a|s)$ with the resulting summation still summing to $1$, so we can already see that the adversary faces a tradeoff between perturbing the reward at different actions in a particular state.

% In \cref{fig:feasible_set_main}, we visualize the feasible set of perturbed rewards in a two-dimensional action space for the \KL divergence, various $\beta$, and uniform or non-uniform priors.    We plot the modified reward $r(a,s) - \pr(a,s)$ for each action and a fixed state.   
% %penalized for decreasing the reward while increasing both rewards is clearly feasible.  

% For high regularization strength ($\beta=0.1$), we observe that the boundary is nearly linear, with slope based on the ratio of each action in the prior. \RB{Check}   The boundary steepens for higher regularization strength, with only small decreases in the reward function available.  In all cases, note that increasing the reward in both actions is clearly feasible for an adversary minimizing the objective in \cref{eq:pedro_form}.

% %proceed to characterize the feasible set of adversarial perturbations $\pr(a,s)$ using a constrained version of \cref{eq:pedro_form}, with visualizations in \cref{fig:feasible_set_main}.



% % To derive the feasible set, we use the conjugate derived from $\Omega(\tpi)$ over unnormalized density functions, so that normalization of $\pi(a|s)$ %\in \Delta^{|\mathcal{A}|}$ 
% % is enforced when solving \cref{eq:pedro_form} for the policy rather than in the definition of $\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}$ itself.\footnote{See \myapp{kl_conj_all} for more detailed discussion.}



% \paragraph{Optimal Reward Perturbations}
% % Differentiating \cref{eq:pedro_form} with respect to $\perturbr$, we obtain the conjugate optimality conditions $\tpi(a|s) &= \nabla \frac{1}{\beta}\Omega^{*}_{\tpi_0, \beta}\big( \perturbr \big) = \big(\nabla \Omega_{\tpi_0}\big)^{-1}(\pr)$ from \cref{eq:optimal_policy_as_grad}, leading to %and solve for $\perturbr(a,s)$.   
% % %Alternatively, , leading to the condition for the optimal reward perturbations \citep{ortega2014adversarial}
% % \begin{align}
% %       \pr(a,s) = \frac{1}{\beta} \log \frac{\tpi(a|s)}{\tpi_0(a|s)} \,. \label{eq:optimal_perturbed}
% % %     \tpi(a|s) &= \nabla \frac{1}{\beta}\Omega^{*}_{\tpi_0, \beta}\big( \perturbr \big) \nonumber \\
% % %    \implies  & \pr(a,s) = \frac{1}{\beta} \log \frac{\tpi(a|s)}{\tpi_0(a|s)}
% % \end{align}
% In \myprop{perturbations} (b), we found that the optimal reward perturbations $\pr(a,s)$ correspond to the pointwise regularization $\ptReg(\tpi(a|s))$ at each action,  by using the optimality conditions 
% $\pr(a,s) &= \nabla \frac{1}{\beta}\Omega_{\tpi_0}\big( \tpi \big) = \big(\nabla \Omega^{*}_{\tpi_0,\beta}\big)^{-1}(\tpi)$ 
% %$\tpi(a|s) &= \nabla \frac{1}{\beta}\Omega^{*}_{\tpi_0, \beta}\big( \perturbr \big) = \big(\nabla \Omega_{\tpi_0}\big)^{-1}(\pr)$
% from \cref{eq:optimal_policy_as_grad}.   The $\alpha$-divergence may also be written with an outer expectation over $\tpi(a|s)$, $\Omega_{\tpi_0}(\tpi) = \mathbb{E}_{\tpi}[\ptReg(\tpi(a|s))]$, \RB{OMIT if keeping Prop}
% so that, as shown in \myapp{alpha_perturb} \myprop{perturbations_alpha}, we can similarly interpret the optimal reward perturbations as the pointwise regularizer
% \small
% \begin{align}
%     \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \frac{\tpi(a|s)}{\tpi_0(a|s)} := \frac{1}{\beta} \frac{1}{\alpha-1} \left( \frac{\tpi(a|s)}{\tpi_0(a|s)}^{\alpha-1} - 1\right)
% \end{align}
% \normalsize
% %\footnote{This assumption and point-wise regularization result similarly hold for the $\alpha$-divergence in \myapp{alpha_conj_all}.}
% Note that we have considered the conjugate derived from $\Omega(\tpi)$ over unnormalized density functions, so that normalization of $\pi(a|s)$ %\in \Delta^{|\mathcal{A}|}$ 
% is enforced when solving \cref{eq:pedro_form} for the policy rather than in the definition of $\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}$ itself.  
% This allows us to avoid a self-referential definition of $\propt(a,s)$ with an additional $\frac{1}{\beta} \log \sum_{a} \pi_0 \expof{\beta \cdot \pr}$ on the right hand side of \cref{eq:optimal_perturbed}.   See \myapp{kl_perturb_section}.
% %the conjugate function $\Omega^{*}_{\tpi_0, \beta}\big( \perturbr \big)$ over unnormalized density functions in \cref{eq:} and \cref{eq:}, so that normalization of $\pi(a|s)$ is enforced when solving for the policy rather than in the definition of the conjugate.   This allows us to avoid a self-referential definition of $\pr(a,s)$ with an additional $\frac{1}{\beta}\sum \limits_{a} \pi_0 \expof{\beta \cdot \pr}$ on the right hand side of \cref{eq:optimal_perturbed}   


\paragraph{Reward Perturbation as Pointwise Regularizer}
Note that both the \textsc{kl} and $\alpha$-divergences can be written with an outer expectation over $\tpi(a|s)$, with $\Omega_{\tpi_0}(\tpi) = \langle \tpi(a|s), \ptReg(\tpi(a|s)) \rangle$.   
With derivations in \myapp{tsallis}, we can see that the optimal reward perturbations in \myprop{perturbations} (b) and \ref{prop:perturbations_alpha}(b) correspond to the (scaled) pointwise regularization $\ptReg(\pi(a|s))$ for the divergence over normalized $\pi(a|s) \in \Delta^{|\mathcal{A}|}$
\begin{align}
   \ptReg(\pi(a|s)) = \frac{1}{\alpha} \propt(a,s) = \frac{1}{\alpha} \log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}
\end{align}
which may be further scaled by the regularization strength $1/\beta$.
This is a natural result, since the objective in \cref{eq:pedro_form} takes the outer expectation $\langle \pi(a|s), r(a,s) - \pr(a,s) \rangle$.  As an example, for the \KL divergence we have $\ptReg(\pi(a|s)) = \log \pi(a|s)/\pi_0(a|s) = \propt(a,s)$ with $\alpha = 1$. %and $D_{KL}[\pi:\pi_0] = \langle \pi(a|s),\ptReg(\pi(a|s))\rangle$.  
\RB{Unresolved... when $\alpha\neq 1$, objective value appears to change due to $\frac{1}{\alpha}$ factor}
% \begin{align}
%      \ptReg(\pi(a|s)) = \log \frac{\pi}{\pi_0} = \propt(a,s)
% \end{align}

Finally, note that we have considered the conjugate derived from $\Omega_{\tpi_0}(\tpi)$ over unnormalized density functions in deriving the optimal reward perturbations, so that normalization of $\pi(a|s)$ %\in \Delta^{|\mathcal{A}|}$ 
is enforced when solving \cref{eq:pedro_form} for the policy rather than in the definition of the conjugate itself. %$\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}$ itself.  
This allows us to avoid a self-referential definition of $\propt(a,s)$, which, for example, would include an additional $\frac{1}{\beta} \log \sum_{a} \pi_0 \expof{\beta \cdot \pr}$ on the right hand side of \cref{eq:optimal_perturbed}.   See \myapp{kl_perturb_section}.


% In \myprop{perturbations} (b) and \ref{prop:perturbations_alpha}(b), we can see that the optimal reward perturbations $\pr(a,s)$ correspond to the pointwise regularization $\ptReg(\tpi(a|s))$ at each action.   
% by using the optimality conditions 
% $\pr(a,s) &= \nabla \frac{1}{\beta}\Omega_{\tpi_0}\big( \tpi \big) = \big(\nabla \Omega^{*}_{\tpi_0,\beta}\big)^{-1}(\tpi)$ 
% %$\tpi(a|s) &= \nabla \frac{1}{\beta}\Omega^{*}_{\tpi_0, \beta}\big( \perturbr \big) = \big(\nabla \Omega_{\tpi_0}\big)^{-1}(\pr)$
% from \cref{eq:optimal_policy_as_grad}.   The $\alpha$-divergence may also be written with an outer expectation over $\tpi(a|s)$, $\Omega_{\tpi_0}(\tpi) = \mathbb{E}_{\tpi}[\ptReg(\tpi(a|s))]$, \RB{OMIT if keeping Prop}
% so that, as shown in \myapp{alpha_perturb} \myprop{perturbations_alpha}, we can similarly interpret the optimal reward perturbations as the pointwise regularizer
% \small
% \begin{align}
%     \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \frac{\tpi(a|s)}{\tpi_0(a|s)} := \frac{1}{\beta} \frac{1}{\alpha-1} \left( \frac{\tpi(a|s)}{\tpi_0(a|s)}^{\alpha-1} - 1\right)
% \end{align}
% \normalsize
% %\footnote{This assumption and point-wise regularization result similarly hold for the $\alpha$-divergence in \myapp{alpha_conj_all}.}


%This indicates that the optimal reward perturbations correspond to the point-wise regularization term at each $a|s$, assuming that the regularizer $\Omega_{\tpi_0}(\tpi) = \mathbb{E}_{\tpi}[\ptReg(\tpi(a|s))]$ can be written with an outer expectation over $\tpi(a|s)$.\footnote{This assumption and point-wise regularization result similarly hold for the $\alpha$-divergence in \myapp{alpha_conj_all}.}

% What are the implications of this result for our interpreting the adversarial reward robustness of regularized policies?
% \RB{save until discussion later, or briefly mention?}
% What implications does this result have for our adversarial reward robustness interpretation of regularized policies?
% %In light of this observation, how should we interpret the adversarial reward robustness?  
% The equivalence of the objectives in \cref{eq:reward_perturbation_stmt} \citep{eysenbach2021maximum} is trivially confirmed for the optimal $\dualvar(a,s) = r(a,s) - \ptReg(\tpi(a|s))$, which is not surprising given that our derivations only utilize an alternative representation of $\Omega_{\pi_0}(\pi)$ using convex duality.
% %aligns with our use of convex duality to obtain an alternative form for $\Omega_{\pi_0}(\pi)$.  %, so that the objectives match exactly.
% %The objective and reward perturbations are crucially sensitive to the  
% %Further, \cref{eq:reward_perturbation_stmt} and the perturbations in
%  %which are known to provide dual representations of a policy \citep{lee2019stochastic}.

% Nevertheless, the reward perturbations in \cref{eq:optimal_perturbed} indicate a very particular game-theoretic robustness \citep{ortega2014adversarial}, which may not directly align with notions of robustness as zero-shot generalization.   In the next section, we further discuss this robustness and explicitly relate the reward perturbations to dual representations of the policy in terms of $Q$-values and the value function $V(s)$ \citep{wang2007dual, lee2019stochastic}. %The adversarial reward perturbations are for each state-action pair, and the per-state normalization or feasible set constraints introduce competition among the perturbations for each action.   

% %\sout{This is in notable contrast to the experiments of \citet{eysenbach2021maximum}, in which the reward for \textit{an entire state}, chosen to be in the path of a deterministic policy, was modified.  While entropy-regularized policies performed better than a deterministic, unregularized policy in this environment, these results are more directly attributable to stochastic policies learning a \textit{diversity of solutions} \citep{haarnoja17a, haarnoja2018acquiring, kumar2020one}, rather than the \textit{reward robustness} suggested by convex duality. }

\subsection{Value-Based Interpretation}\label{sec:value_based} % of Reward Robustness}
In this subsection, we provide a complementary interpretation of adversarial reward robustness from a value perspective, which highlights the role of $\pr(a,s)$ as a dual variable related to $V(s)$ and $Q(a,s)$. % from \mysec{dual}.   %the results of the previous section, we  interpret strength and type of regularization as determining how an agent expresses uncertainty when aggregating state-action estimates $Q(a,s)$ into a per-state value function $V(s)$.
%leading to a known \textit{indifference} condition at optimal policy as in \citet{ortega2014adversarial}. 


\paragraph{Soft Value Aggregation \& Adversarial Hedging}
Using the results of the previous subsection, the value function $V_*(s) = \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ in \cref{eq:soft_bellman} and \cref{fig:value_agg_main} can be interpreted as the \textit{certainty equivalent} \citep{myerson2019probability, ortega2013thermodynamics}, %myerson2019probability,
which aggregates over actions $a \in \mathcal{A}$ to measure the payoff of a two-player game where the agent begins in state $s \in \mathcal{S}$ and plays against an adversary defined by the regularizer $\Omega_{\pi}(\pi)$ and strength $\beta$ as in \myprop{perturbations} \citep{ortega2014adversarial}.   % As shown in \cref{fig:value_agg}, for $\beta > 0$, this value ranges between the maximum reward over actions and the expected reward under the reference distribution.


%\paragraph{Soft Value Aggregation \& Adversarial Hedging}

% \paragraph{Soft Value Aggregation as Adversarial Hedge}
% % ********* Moved to Background ***********
%  We begin by imagining a single-step decision in a particular state $s \in \mathcal{S}$, for an agent with given $Q$-function estimates $Q(a,s) = r(a,s) + \gamma \transitionv$ in an \gls{MDP}.  
 
%  Instead of acting with deterministically with the greedy policy $\max_{\pi} \blangle\pi(a|s), Q(a,s)\brangle$,  %a \textbf{regularized} 
%  an agent \textcolor{red}{might express uncertainty in its $Q$-value estimates }by only allowing this information to induce a certain average deviation $R$ from a prior reference policy $\pi_0(a|s)$.
%  %the consideration of $Q$-value estimates to induce a certain average deviation $R$ from a prior reference policy $\pi_0(a|s)$.   
%  Measuring this average deviation using a convex divergence $\Omega_{\tpi_0} = R$ and introducing an appropriate Lagrange multiplier $1/\beta$ for the constraint, we are left with the conjugate optimization \citep{geist2019theory}
%  \begin{align}
%     V(s):= \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta} = \max_{\pi \in \Delta^{|\mathcal{A}|}} \blangle\pi(a|s), Q(a,s)\brangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) %\nonumber \label{eq:value_opt}
%  \end{align}
%  This expression matches \cref{eq:primal_reg} or \cref{eq:soft_bellman}, and \textit{soft}-value aggregation is indeed common in the literature \citep{ortega2013thermodynamics, fox2016taming, lee2019tsallis}.    However, the results of the previous section suggest an interpretation of soft-value aggregation as hedging against an \textit{imagined}, reward-perturbing adversary, where we use the conjugate representation of the regularizer  $\Omega_{\pi_0}(\pi) = \, \sup_{\perturbr} \langle \pi, \pr \brangle - \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(\pr)$ \citep{ortega2014adversarial}.   
%  The strength of the adversary is determined by $\beta$, with the feasible set determined by $\beta$ and the shape of the conjugate function $\Omega^{*}_{\pi_0,\beta}(\pr)$.
 
%  %Solving the conjugate optimization for the \textsc{kl} divergence, the optimizing policy becomes
 
%  %The resulting value function $V(s) = \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ reflects a \textit{soft}-aggregation of state-action estimates $Q(a,s)$ into a \textit{certainty equivalent} \citep{myerson2019probability}, which measures the agent's payoff for playing this two player game in a given state $s \in \mathcal{S}$ and against a particular adversary.   
% We visualize the value function $V(s) = \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$, which measures the agent's payoff for playing this two player game in a given state $s \in \mathcal{S}$ and against a particular adversary, for different adversary strengths ($\beta$) and divergences in \cref{fig:value_agg}.  The value ranges between $\max_a Q(a,s)$ for a deterministic policy as $\beta \rightarrow \infty$ or the expectation under the reference policy $\mathbb{E}_{\pi_0}[Q(a,s)]$ as $\beta \rightarrow 0$.    Note that high regularization or low $\beta$ indicates a weak adversary, so that the policy becomes increasingly greedily with respect to $Q(a,s)$. 

% Finally, the conjugacy conditions in \cref{eq:optimal_policy_as_grad} provide the optimizing policy in each state.   For \textsc{kl} divergence regularization, we have
%   \begin{align}
%  \pi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s) -  \psi_{\beta}(s)\big)} \label{eq:opt_policy}
%  \end{align}
%  where $\psi(s;\beta) = \frac{1}{\beta} \log \sum_a \pi_0(a|s) \expof{\beta \cdot Q(a,s)}$ enforces normalization.    While we always define the value function $V(s):= \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ using the conjugate as in \cref{eq:}
 
 
%  In the case of the \KL divergence, $\psi(s;\beta) = V(s)$, with $V(s):= \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ from \cref{eq:}, the subtractive normalization constant does not correspond to the value or conjugate function in general,  the $\alpha$-divergence in \myapp{alpha_conj_all} or \citet{lee2019tsallis}.
 
%  $V(s) := \frac{1}{\beta}\Omega^{*}_{\pi_0,\beta}(Q)$ for the \KL divergence, this is not true in general for the $\alpha$-divergence in \myapp{alpha_conj_all} or \citet{lee2019tsallis}.   We now proceed to discuss this policy in relation to the adversarial reward perturbations in \myprop{perturbations}
 
% %While soft value-aggregation is standard \citep{ortega2013thermodynamics, fox2016taming, lee2019tsallis}, we have emphasized its adversarial interpretation as in \citet{ortega2014adversarial}. 


%  %\textcolor{red}{While more complex techniques for expressing uncertainty exist \citep{duff2002optimal ,smirnova2019distributionally}, a simple strategy is to only allow these estimates to induce a certain average deviation $R$ from a prior reference policy $\pi_0(a|s)$.}   Deciding to measure this deviation using a convex statistical divergence $\Omega_{\tpi_0} = R$, we find that the agent will aggregate value in the state according to the conjugate function
%  %the agent will act according to a policy
% ******************************************               ***************************************


% Visualization:   Q values => policy at each α, 
% same policy, different Q values different value, different α
\paragraph{Reward Perturbations using $Q$-Values}
 %\paragraph{Reward Perturbations as \cancel{Advantage Function}}
 While a stochastic policy may be interpreted as hedging against an imagined adversary, we can also identify a given stochastic policy with an optimal adversarial reward perturbation. 
 %To further understand the nature of this adversary, we can also identify a given stochastic policy with an optimal adversarial reward perturbation.    
 %While a stochastic policy may be interpreted as hedging against an imagined adversary, we can also identify a given stochastic policy with an optimal adversarial reward perturbation.    
 Given a regularizer $\Omega_{\pi_0}(\pi) = D_{KL}[\pi:\pi_0]$, reference distribution $\pi_0(a|s)$, and regularization strength $1/\beta$, %simple algebraic rearrangement of \cref{eq:opt_policy} 
 we can simply rearrange \cref{eq:kl_opt_policy} to write  
\begin{align}
    \propt(a,s) = Q(a,s) - \normalizerexp =  \frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)} \label{eq:perturb_opt_q}
\end{align}
where the difference $Q(a,s) - \normalizerexp$ is uniquely determined from $\pi(a|s)$ and the assumed regularizer.   Note that the choice of $Q(a,s)$ and $\normalizerexp$ are not unique, as the normalization constant $\normalizerexp$ is determined from the choice of $Q(a,s)$ and may be intractable in practice.
%However, note that the choice of $Q(a,s)$ and $\normalizerexp$ are not unique, with $\normalizerexp$ chosen to enforce normalization for a given set of $Q(a,s)$.  %Furthermore, $\normalizerexp$ is often intractable in practice.
We obtain a similar expression for the $\alpha$-divergence, $Q(a,s) - \alphanorm =  \frac{1}{\beta} \ln_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}$, although the normalizer $\alphanorm$ is not equal to the conjugate $\alphaconjn(\pr)$ as in the case of the \KL divergence.

We visualize the optimal reward perturbations for the single step case in \cref{fig:perturb_opt}.   
Notice that the reward perturbations reflecting a given policy $\pi(a|s)$ can either be positive or negative, depending on the likelihood ratio $\frac{\pi(a|s)}{\pi_0(a|s)} \lessgtr 1$ or the difference $Q(a,s) - \alphanorm \lessgtr 0$.    We discuss this property in more detail in \mysec{discussion}.
%From \cref{eq:perturb_opt_q} or \cref{eq:optimal_perturbed}, we can see that the reward perturbations reflecting a given policy $\pi(a|s)$ can either be positive or negative, depending on the likelihood ratio between the policy the reference policy at each action.   
%This multiplicative factor can also be measured by a monotonic function of $Q(a,s) - \normalizerexp$, for example in the exponential family policy in \cref{eq:opt_policy}. 
 %To do so, we assume that the normalization constant for a given $\pi(a|s)$ is tractable.   With knowledge of $\pi_0(a|s)$
 
 
 \paragraph{Indifference Condition for Optimal Policy}
%In the previous sections, we have used convex duality to translate between expressions for the optimal reward perturbations in terms of the primal policy or dual value functions.    
For the optimal policy $\opt(a|s)$ in a given \gls{MDP}, we can additionally state an \textit{indifference condition} across actions, which is a well-known property of Nash equilibria in game theory \citep{osborne1994course, ortega2014adversarial}.   In particular, the adversarial objective
%For the optimal policy $\opt(a|s)$ in a given \gls{MDP}, the objective 
% \footnotesize
% \begin{align}
% \min \limits_{\pr(a,s)} &\blangle \opt(a|s), r(a,s) + \gamma \transitionv - V(s) - \pr(a,s) \brangle + \frac{1}{\beta} \Omega^{*}_{\tpi_0, \beta}(\pr) \nonumber \\
% &= V_{\beta}(s)
% \end{align}
has the same value for each action $a \in \mathcal{A}$ in state  $s \in \mathcal{S}$ (see \myapp{indifference}).   
We can see in \cref{fig:perturb_opt}(a) that the perturbed rewards for each action match the value function $V_*(s)$ in each state.   %This property also appears in \cref{fig:feasible_set_main}, with matching coordinates for the optimal perturbed $\mr(a,s)$. %with \KL divergence regularization.    
While it is possible to derive an adversarial interpretation for any $\pi(a|s)$ using \cref{eq:pedro_form}, we see in \cref{fig:perturb_opt}(b) that the indifference condition does not hold for suboptimal policies.  

% As the indifference condition for optimal policies highlights, the adversarial reward perturbations preserve the value of the objective in each state.   We further explore this sensitivity of the reward perturbations to the form of objective function below.

%in the single-step case, the $Q$-values do not match the environment rewards. %However, one can confirm algebraically or numerically that the value of the objective does not change.
%$Q(a,s) \neq r(a,s)$ for some $(a,s)$ in the single step case.  
%, where the single-step $Q$-values do not match the environment rewards.  

% While the indifference condition depends on the optimal policy arising from the $\max$ over $\pi(a|s)$, we can construct an adversarial interpretation in \cref{eq:pedro_form} for any $\pi(a|s)$ using the conjugate representation of the divergence $\Omega_{\pi_0}(\pi)$.   Visualizing the reward perturbations for both optimal and suboptimal policies for the single-step case in \cref{fig:indifference}, we observe that the indifference among actions does not occur for suboptimal policies.  
%Although the reward perturbations correspond to $Q(a,s) - \psi(s;\beta)$ despite the fact that the 


% \begin{figure}
% \begin{minipage}[b][6cm]{0.3\linewidth}
% \subfloat[A]{\includegraphics[width=3cm,height=2cm]{logo}}

% \vfill
% \subfloat[B]{\includegraphics[width=3cm,height=2cm]{logo}}
% \end{minipage}%
% \begin{minipage}[t][6cm]{0.3\linewidth}
% \subfloat[D]{\includegraphics[width=3cm,height=6cm]{logo}}
% \end{minipage}%
% \begin{minipage}[t][6cm]{0.3\linewidth}
% \subfloat[D]{\includegraphics[width=3cm,height=6cm]{logo}}
% \end{minipage}
% \caption{Many figures}\label{foo}
% \end{figure}

%%Our starting point in this section is the Lagrangian 
% \paragraph{Robustness to Reward Perturbations}
% To derive the adversarial robustness statement in \cref{eq:reward_perturbation_stmt} in terms of a constrained linear program, 
% \begin{align}
% &\max \limits_{\pi(a|s)} \mathbb{E}_{\tau \sim p^{\pi}(\tau)} \left[ \sum \limits_{t=0}^\infty \gamma^t \, \bigg( r(a_t, s_t) - \Omega\big(\pi(a_t | s_t)\big) \bigg) \right] \nonumber \\
% &= \max \limits_{\pi(a|s)} \min \limits_{r\tick(a,s) \in \mathcal{R}}  \mathbb{E}_{\tau \sim p^{\pi}(\tau)} \left[ \sum \limits_{t=0}^\infty \gamma^t \, r\tick(a_t,s_t) \right]
% \label{eq:reward_perturbation_stmt}
% \end{align}






% \newcommand{\WidthS}{.22\textwidth}
% \newcommand{\WidthM}{.25\textwidth}
% \newcommand{\WidthMM}{.27\textwidth}
% \newcommand{\HeightS}{30mm}
% \newcommand{\HeightM}{30mm}

\newcommand{\WidthS}{.2\textwidth}
\newcommand{\WidthM}{.22\textwidth}
\newcommand{\WidthMM}{.25\textwidth}
\newcommand{\HeightS}{20mm}
\newcommand{\HeightM}{20mm}

\hspace*{-.2cm}
\begin{figure*}[t]
\centering
\begin{minipage}{.48\textwidth}
% \begin{subfigure}
%\def\arraystretch{2.2}
%  \subcaptionbox{Optimal Policy \label{fig:perturb_opt_a}}{
\[\arraycolsep=.005\textwidth
\begin{array}{cccc} %[width=40mm]
%\begin{subfigure}{.16\columnwidth}
 & \multicolumn{3}{c}{\text{(i) }\beta = 0.1} \\[.5ex]
\multirow{3}{\WidthMM}{\includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/env.png} \\[4ex] \includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/opt_agent.png}} &
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta01policy_opt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta01perturb_opt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta01perturbed_opt.png}  \\[.25ex]
 & \multicolumn{3}{c}{\text{(ii) }\beta = 1.0} \\[.5ex]
%\caption{\centering \small $D_{KL}, \beta = 10$}\label{fig:tabc}\end{subfigure}&\hspace*{.2cm}\\
& % NEXT LINE for multi-row
%\includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/opt_agent.png} &
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta1policy_opt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta1perturb_opt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta1perturbed_opt.png} \\[.25ex]
 & \multicolumn{3}{c}{\text{(iii) } \beta = 10} \\[.25ex]
&
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta10policy_opt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta10perturb_opt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta10perturbed_opt.png} 
% \\[.25ex]
\end{array}
\]
 %\hspace*{0.25cm}
% \label{subfig:subfig}
% \caption{Optimal Policy }\label{fig:perturb_opt_a}
% \end{subfigure}
\end{minipage}\hspace{.02\textwidth} %{\quad \vline width 1pt}&
%&\\[2ex] \midrule
\begin{minipage}{.48\textwidth}
% \begin{subfigure}{.48\textwidth}
% \subcaptionbox{Suboptimal Policy \label{fig:perturb_subopt_b}}{
\[\arraycolsep=.005\textwidth
\begin{array}{cccc} %[width=40mm]
%\begin{subfigure}{.16\columnwidth}
 & \multicolumn{3}{c}{\text{(i) } \beta = 0.1} \\[.5ex]
\multirow{3}{\WidthMM}{\includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/env.png} \\[4ex] \includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/agent.png}} &
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta01policy_subopt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta01perturb_subopt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta01perturbed_subopt.png}  \\[.25ex]
 & \multicolumn{3}{c}{\text{(ii) } \beta = 1.0} \\[.5ex]
%\caption{\centering \small $D_{KL}, \beta = 10$}\label{fig:tabc}\end{subfigure}&\hspace*{.2cm}\\
& % NEXT LINE for multi-row
%\includegraphics[width=\WidthM, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/agent.png} &
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta1policy_subopt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta1perturb_subopt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta1perturbed_subopt.png} \\[.25ex]
 & \multicolumn{3}{c}{\text{(iii) } \beta = 10} \\[.5ex]
&
%\end{subfigure}&\qquad  \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthS, height=\HeightS, trim=5 0 5 0, clip]{figs/perturbed/beta10policy_subopt.png} & 
%\caption{\centering \small $D_{KL}, \beta = 0.1$}\label{fig:taba}\end{subfigure}& \qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta10perturb_subopt.png} & 
%\caption{\centering  $D_{KL}, \beta = 1.0$}\label{fig:tabb}\end{subfigure}&\qquad \hspace*{.2cm}
%\begin{subfigure}{0.33\columnwidth} 
\includegraphics[width=\WidthM, height=\HeightM, trim=5 0 5 0, clip]{figs/perturbed/beta10perturbed_subopt.png} \\[.25ex]
\end{array}
\]
% }
\end{minipage}
\caption{Suboptimal Policy} \label{fig:perturb_subopt_b}
% \end{subfigure}
\caption{ Single-Step Reward Perturbations.  $Q$-values in leftmost columns are used for each $\beta$ in columns 2-4.  
We report the optimal $-\pr(a,s)$, so that values less than 0 are subtracted in the objective $\langle \pi_Q(a|s), r(a,s) - \pr(a,s) \rangle + \alphaconju(\pr)$.
In (a), we show the optimal policy ($Q(a,s) = r(a,s)$), where the  perturbed reward $r^{\prime}(a,s) = c \, \, \forall a$ reflects the indifference condition.  We also show a suboptimal policy in (b), where indifference does not hold.  In all cases, actions with high $Q(a,s)$ are robust to subtracted perturbations. }\label{fig:perturb_opt}
\end{figure*}



\section{Discussion}\label{sec:discussion}
%In light of the above results, 
What insights can be obtained from this adversarial interpretation of regularized policies?
%Ultimately, what insight is provided by this adversarial reward robustness interpretation of regularized policies?
%What implications do the above results have for our adversarial reward robustness interpretation of regularized policies?]
%Our results in the previous section indicate a very particular form of robustness, which has a natural game-theoretic interpretation. %\citep{ortega2014adversarial}.  
%The results of the previous section indicate a very particular form of robustness which has a natural game-theoretic interpretation \citep{ortega2014adversarial}.
In \ref{sec:generalization}, we discuss the generalization properties associated with this robustness, which we highlight is particularly sensitive to the form of the objective in \ref{sec:entropy_vs_div}.
%However, as we argue below, this may not directly align with desired notions of robustness as zero-shot generalization to unseen environments.
%However, this robustness is particularly sensitive to the form of the objective, as discussed in \mysec{entropy_vs_div}.   
%may not directly align with desirable notions of zero-shot generalization to unseen environments \TG{This needs a bit of unpacking - do you mean that we can't say anything about unseen environments because we don't know the dynamics/reward function? I would argue that we can at least say something about unseen environments where the reward has been perturbed according to the feasible set - which is actually quite a nice statement I think.} and, as we discuss in \mysec{entropy_vs_div}, is sensitive to the form of the objective.
%particularly sensitive to the form of the objective.
%and is particularly sensitive to the form of the objective, as discussed in \mysec{entropy_vs_div}.   
We draw connections with the notion of path consistency \citep{nachum2017bridging, chow2018path} in \ref{sec:modified}, and argue that  adversarial reward perturbations can provides a natural justification for including $Q$-values as dual variables in \gls{LP} formulations of \gls{MDP}s in \ref{sec:qlp}.
%\RB{Add generalization analysis}
%\RB{Add reward $\rightarrow$ robustness vs. policy $\rightarrow$ robustness}

\subsection{Relationship to Generalization}\label{sec:generalization}
%For our purposes, we consider `zero-shot generalization' of a given policy $\pi(a|s)$ to an environment with a modified reward function $\mr(a,s)$ to mean that
Our adversarial interpretations imply robustness or generalization of a given policy $\pi(a|s)$ to an environment with a modified reward $\mr(a,s)$ in the sense that, for given \gls{MDP} transition dynamics
\scriptsize
\begin{align}
  \hspace*{-.3cm} \langle \mu(s) \pi(a|s), \mr(a,s) \rangle \geq \langle \mu(s) \pi(a|s), r(a,s) \rangle - \langle \mu(s), \frac{1}{\beta} \Omega_{\pi_0}(\pi) \rangle \, \label{eq:robust_def}
   %\blangle \mu(s) \pi(a|s), \mr(a,s) \brangle \geq  \blangle \mu(s) \pi(a|s), r(a,s) - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \brangle \, . \label{eq:robust_def}
\end{align}
\normalsize
%Our adversarial interpretations imply robustness or generalization of a given policy $\pi(a|s)$ to a modified reward function in this particular sense.   
%Notice that 
where the right hand side corresponds to the full objective function, including regularization, whereas the left hand side is only the expected reward.
 %the regularized objective $\mathcal{R}_{\Omega, \beta}(r\tick) \geq \mathcal{R}_{\Omega, \beta}(r\tick)$
The constraints in \myprop{perturbations}-\ref{prop:perturbations_alpha} characterize the robust set of modified rewards to which a given policy can generalize, as visualized in \cref{fig:feasible_set_main}.   Since these constraints integrate over the action space, note that the rewards for all actions in a particular state must be perturbed together.

By running a fixed policy in an environment with higher rewards, we naturally expect the objective function to increase.   However, for useful zero-shot generalization, we might hope that a policy will still perform well when the reward function decreases in at least some states.    
%In the next subsection, we 
In the next subsection, we discuss how these qualitative properties can depend on the form of the regularization function $\frac{1}{\beta} \Omega_{\pi_0}(\pi)$ in \cref{eq:robust_def}. %can impact these qualitative.
%of the reward robustness \cref{eq:robust_def} and their sensitivity to the form of the regularization function .
%Using the expression in \cref{eq:perturb_opt_q}, we can see that a regularized policy will be robust to negative changes in the reward function when
%$\frac{\pi(a|s)}{\pi_0(a|s)} \lessgtr 1$ or difference $Q(a,s) - \alphanorm \lessgtr 0$.  


%As observed above, entropy regularization can only provide robustness to reward increases $-\pr \geq 0$ and objective values $\alphaconjn$ which are higher than the environment rewards.  
%For useful generalization to unseen environments, we are usually 



\subsection{Comparison with Entropy Regularization }\label{sec:entropy_vs_div}
% \paragraph{Dual Representations} The equivalence of the objectives in \cref{eq:reward_perturbation_stmt} %\citep{eysenbach2021maximum} 
% is trivially confirmed for the optimal $\dualvar_*(a,s) = r(a,s) - \frac{1}{\beta} \ptReg(\pi(a|s)) = r(a,s) - \frac{1}{\beta} \propt(a,s)$ (\RB{This is wrong and unresolved.  Only true of KL div, otherwise $\frac{1}{\beta} \ptReg(\pi(a|s)) = \frac{1}{\beta} \frac{1}{\alpha} \propt(a,s)$ factor}), which is not surprising given that our derivations only invoked an alternative representation of $\Omega_{\tpi_0}(\tpi)$ via convex duality.   This duality is also reflected in the fact that we can represent the optimal reward perturbations, or a stochastic policy itself, in terms of either probabilities $\pi(a|s)$ or dual variables $Q(a,s)$ for a given $\Omega$, $\pi_0$, and $\beta$.  
% %representations of a stochastic policy in terms of probabilities $\pi(a|s)$ or dual variables $Q(a,s)$
%As the indifference condition for optimal policies highlights, the adversarial reward perturbations preserve the value of the objective in each state.   We further explore this sensitivity of the reward perturbations to the form of objective function below.

%{\paragraph{Entropy vs. Divergence}}
%Our use of the \textsc{kl} and} $\alpha$-divergences, instead of the corresponding entropic quantities, resolves several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}.   Regularizing with the Tsallis or Shannon ($\alpha = 1$) entropy, the optimal perturbations are %perturbed reward is %reward
When regularizing with the Tsallis or Shannon ($\alpha = 1$) entropy, the optimal reward perturbations become %perturbed reward is %reward
\begin{align}
    \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \pi(a|s) \,. \label{eq:ptwise_perturb_ent}
\end{align}
%For entropy regularization, 
We argue the pointwise non-negative contribution of these perturbations to the objective $r(a,s) - \propt(a,s)$, with $-\propt(a,s) \geq 0$ for $\pi(a|s) \leq 1$, leads to several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}, which are resolved by our use of the \textsc{kl} and $\alpha$-divergences instead of the entropic quantities.   In particular, entropy regularization should be considered as a divergence to the uniform reference distribution $\pi_0(a|s)$ over actions.
%Our use of the \textsc{kl} and} $\alpha$-divergences, instead of the corresponding entropic quantities, resolves several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}.   

First, this means that an entropy regularized policy is only `robust' to \textit{increases} in the reward function.  
%This can be corrected when 
Including the reference distribution as in \myprop{perturbations}(b) and \cref{fig:perturb_opt} changes this property, so that the optimal reward perturbation $\propt(a,s) = \frac{1}{\beta}\log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}$ %\frac{\pi(a|s)}{ \pi_0(a|s)}$ %
yields robustness to reward \textit{decreases} when $\pi(a|s) > \pi_0(a|s)$ and reward increases otherwise.  

%After taking the expectation over actions, note that subtracting a non-negative \textsc{kl} divergence yields a smaller quantity than the unregularized objective, whereas subtracting the negative entropy yields a larger quantity.

%adding the entropy gives a larger quantity.

%The possibility of both reward increases and decreases also clarifies constraints on the feasible set.   
%Nevertheless, as the indifference condition for optimal policies suggests, the role of these perturbations is simply to re-express the value of the objective function in each state.

%which can be corrected by including the reference distribution $\pi_0(a|s)$ as in our results from the previous section.

%Although divergences and entropies are both non-negative in expectation, we argue that explicitly including the reference distribution is crucial to 
%which matches \cref{eq:optimal_perturbed} for uniform $\pi_0(a|s)$.   




% These observations stem from the fact that the Shannon or Tsallis entropy is a pointwise non-negative quantity.
Similarly, \citet{lee2019tsallis} note that %$\frac{1}{\beta}\Omega^{*}_{\pi_0}(\discussiondual) = \max_{\pi(a|s)} \langle \pi(a|s), \discussiondual(a,s) \rangle + \frac{1}{\beta} H_{\alpha}(\pi) \geq \discussiondual(a_{\max}, s) $
\small
\begin{align*}
    \frac{1}{\beta}\Omega^{*(H_{\alpha)}}_{\pi_0}(\discussiondual) = %\max_{\pi(a|s)}
    \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \langle \pi, \discussiondual \rangle - \left(-\frac{1}{\beta} H_{\alpha}(\pi)\right) \geq \discussiondual(a_{\max}, s) 
\end{align*}
\normalsize
where $a_{\max} = \argmax_a \discussiondual(a,s)$ and the Tsallis entropy $H_{\alpha}(\pi)$ equals the Shannon entropy for $\alpha = 1$.  
%Due to the non-negativity of the pointwise entropy, 
This soft value aggregation, using the negative (Tsallis) entropy as a regularizer,  yields a value which is \textit{larger} than any particular reward. 
%so that soft value aggregation yields a value which is \textit{larger} than any particular reward. 
% \begin{align}
%     \max_{\pi(a|s)} \langle \pi(a|s), \discussiondual(a,s) \rangle + \beta H_q(\pi) \geq \max_a \discussiondual(a,s)
% \end{align}
% where $H_q$ is the Tsallis entropy.
By contrast, for the $\alpha$-divergence, we show in \myapp{qmax} that
\small
\begin{align*}
   \discussiondual(a_{\max},s) + \frac{1}{\beta} \log_{\alpha} \frac{ \pi(a_{\max}| s)}{\pi_0( a_{\max}| s)} \leq \alphaconjn(\discussiondual) \leq  \discussiondual(a_{\max},s)
   %\leq  \alphaconjn(\discussiondual) \leq \max_a \discussiondual(a,s) % \max \limits_{a \in \mathcal{A}} \discussiondual(a_{\max},s)
%     \discussiondual(a_{\max},s) \geq \alphaconjn(\discussiondual) \geq \begin{cases}  \discussiondual(a_{\max},s) -  \frac{1}{\alpha-1} \big( \frac{\pi(a_{\max} | s)}{\pi_0(a_{\max}|s)}^{\frac{1}{\alpha-1}} - 1 \big) \hfill \alpha \neq 1 \\
%   \discussiondual(a_{\max},s) - \log \frac{ \pi(a_{\max}| s)}{\pi_0( a_{\max}| s)}  \hfill \alpha =1 \end{cases}  
%   %\leq  \alphaconjn(\discussiondual) \leq \max_a \discussiondual(a,s) % \max \limits_{a \in \mathcal{A}} \discussiondual(a_{\max},s)
\end{align*}
\normalsize
This provides a more natural interpretation of $V(s) =  \alphaconjn(Q)$ as a soft maximum function, with $ \mathbb{E}_{\pi_0}[\discussiondual(a_{\max},s)] \leq V(s) \leq \discussiondual(a_{\max},s)$ as in \cref{fig:perturb_opt}.


Finally, entropy regularization also affects interpretations of the feasible set.  %For entropy regularization,
\citet{eysenbach2021maximum} consider the same constraint as in \myprop{perturbations}, but without considering the reference distribution
\begin{align}
    \sum \limits_{a} \expof{\beta \cdot \pr(a,s)} \leq \sum \limits_{a} \pi(a|s)  \, \, \, \forall s \in \mathcal{S} \, . \label{eq:ent_constraint}
\end{align}
This constraint suggests that the original reward function ($\pr = 0$) is not feasible for the adversary, unless the policy is deterministic.  More surprisingly, \citet{eysenbach2021maximum} App. A5 argues that \textit{increasing} regularization strength may lead to \textit{less} robust policies based on the constraint in \cref{eq:ent_constraint}.    In \myapp{eysenbach}, we discuss how including $\pi_0(a|s)$ in the constraint via divergence regularization modifies this conclusion.   As expected, we observe in \cref{fig:feasible_set_main} that increasing regularization strength leads to more robust policies.


% \RB{Need to further investigate.  What is Fig. 7 (left) of \citet{eysenbach2021maximum} showing?  }
% Further, \citet{eysenbach2021maximum} App. A5 observe that \textit{increasing} the regularization strength leads to \textit{less} robust policies, with \textit{smaller} feasible sets for the adversary.  With Shannon entropy regularization, the constraint in \myprop{perturbations}(a) becomes
% %For Shannon entropy regularization, the analogous constraint to \myprop{perturbations}(a) is
% \begin{align}
%     \sum \limits_{a} \expof{\beta \cdot \pr(a,s)} \leq \sum \limits_{a} \pi(a|s)  \, \, \forall s \in \mathcal{S} 
% \end{align}
% Restricting attention to $\pr(a,s) < 0$ based on \cref{eq:ptwise_perturb_ent}, \citet{eysenbach2021maximum} conclude that the 

% %To understand this, note that the feasible constraint 

% This is a surprising conclusion, as we would expect regularization to improve robustness, and \cref{fig:feasible_set_main} shows that this is indeed the case when regularizing using divergences rather than entropies.   


% While \citet{eysenbach2021maximum} display feasible sets arising from (negative) Shannon entropy regularization $\Omega(\pi) = - H(\pi)$, this approach leads to puzzling conclusion that \textit{lower} regularization strength $1/\beta$ leads to \textit{greater} adversarial robustness, with larger feasible sets.   
% In contrast to \cref{eq:optimal_perturbed}, the entropy-regularized policy is `robust' to only positive changes in the reward function $\pr(a,s) \geq 0$, with the optimal perturbed reward $\mr(a,s) = r(a,s) - \pr(a,s) = r(a,s) - \log \pi(a|s)$.   We also observe robustness to large positive reward perturbations for low regularization strength in \cref{fig:perturb_opt}, but the crucial negative reward perturbation arises for the action(s) in the support of the nearly deterministic policy.
% We prefer to characterize `robustness' in terms of \textit{reductions} to the reward function

%sensitivity to the value of objective function


% 

==> old/3_modified.tex <==
\subsection{Adversarial Modified Rewards}\label{sec:modified}
The adversarial interpretation in the previous sections may also be written directly using the modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$, which has been studied in a more general setting by \citet{husain2021regularized}.

%We briefly describe this perspective for the policy regularization case, drawing connections with path consistency learning \citep{nachum2017bridging, chow2018path} and logistic $Q$-learning \citep{basserrano2021logistic}.

%\paragraph{Modified Reward Interpretation}
\citet{husain2021regularized} consider maximizing an arbitrary concave objective $\concaveopt$, and proceed to derive its convex conjugate $(-\concaveopt)^*$.    Translated to our setting and notation,
this involves the conjugate expansion of the regularized objective $(-\mathcal{R}_{\Omega, \beta}(r))^*$ instead of the conjugate of the regularizer $ (\frac{1}{\beta} \Omega_{\pi_0}(\pi))^*$ only.  
With detailed derivations in \myapp{husain_conjugate}, this leads to the Lagrangian
\begin{align}
    \hspace*{-.2cm} & \quad \max \limits_{\mu(s) \rightarrow \mathcal{M}} \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s)} \min \limits_{\textcolor{\highlight}{\mr(a,s)}} \, \label{eq:husain_form} \\
    & \big \langle {\mu(s)\pi(a|s)}, {\textcolor{\highlight}{\mr(a,s)} +\gamma \transitionv - V(s) } \brangle  \nonumber  \\
    & \quad+ \frac{1}{\beta} \Omega^{*}_{\textcolor{red}{\tpi_0}, \beta} \big( r(a,s) - \textcolor{\highlight}{\mr(a,s)} \big) + (1-\gamma) \blangle \nu_0(s), V(s) \brangle \, ,  \nonumber
\end{align}
which matches \cref{eq:pedro_form} up to simple reparameterization of $\mr(a,s) = r(a,s) - \pr(a,s)$.

\paragraph{Optimal Modified Rewards}
%In \myapp{perturb_husain}, we show
Differentiating \cref{eq:husain_form} with respect to $\pi(a|s)$ and solving for the optimal modified rewards yields the result of \citet{husain2021regularized} that
\begin{align}
   \mropt(a,s) = V(s) - \gamma \transitionv  %\quad \forall (a,s) \in (\mathcal{A}, \mathcal{S})
\end{align}
%The optimal modified rewards from \citet{husain2021regularized} %match our \cref{eq:optimal_perturbed} up to reparameterization
%\citet{husain2021regularized} interpret this modified reward as `relating the rewards between states through the dynamics of $P(s\tick|s,a)$'.
%Consider the Bellman backup or \textsc{td}-0 error $r(s,a) + \gamma \transitionv - Q(a,s)$
Adding the environment reward, we can use the optimal reward perturbations $\propt(a,s) = r(a,s) - \mropt(a,s)$ to rewrite this expression
% \begin{align}
%   \hspace*{-.2cm} r(a,s) - \mr(a,s) &=  r(a,s) + \gamma \transitionv -  V(s) 
% \end{align}
% \RB{what about cases other than the KL divergence?  }
% which suggests
\begin{align}
\propt(a,s) &=  r(a,s) + \gamma \transitionv -  V(s) \label{eq:modified_reward_opt}
\end{align}
\normalsize
\textcolor{red}{This seems problematic because we would write $\pr(a,s) = Q(a,s) - \psi_{\alpha}(s;\beta)$ for $\alpha$-divergence minimization, with $\psi_{\alpha}(s;\beta) \neq V(s)$.  
}\RB{Think I can fix this}


\paragraph{Connection with Path Consistency}
For the \textsc{kl} divergence regularization, \citet{nachum2017bridging} use the \textsc{kkt} conditions to show that the optimal policy satisfies \textit{path consistency} equations, which follow directly from the adversarial rewards in \cref{eq:modified_reward_opt} using \myprop{perturbations}.   In particular,
\begin{align}
    r(a,s) - \underbrace{\frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)}}_{\propt(a,s)} = V(s) - \gamma \transitionv 
    %\, \, \forall s \in \mathcal{S}, a \in \mathcal{A}
\end{align}
for all $s \in \mathcal{S}, a \in \mathcal{A}$.

Generalizing the path consistency equation shown in \citet{chow2018path} for the Tsallis entropy with $\alpha =2$, we can write
% of \citet{chow2018path} for the Tsallis entropy with $\alpha = 2$ into our notation, the path consistency condition  corresponds to 
% Adapting the result of \citet{chow2018path} for the Tsallis entropy with $\alpha = 2$ into our notation, the path consistency condition  corresponds to 
%For the Tsallis entropy with $\alpha=2$, \citet{chow2018path} obtain the following path consistency equation
\begin{align}
r(a,s) - \underbrace{\frac{1}{\beta}\log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)}}_{\propt(a,s)} &= V(s) - \gamma \transitionv + \Lambda(s)  \label{eq:path1}
\end{align}
where $\Lambda(s) = \normalizerexp - V(s)$ is a Lagrange multiplier which can be seen as accounting for the fact that $\normalizerexp \neq V(s)$ for $\alpha \neq 1$.
Finally, we are left with
\begin{align}
    r(a,s) + \gamma \transitionv - \propt(a,s) = \normalizeralpha   \label{eq:path}
\end{align}
which matches our condition $\pr(a,s) = Q(a,s) - \normalizeralpha$. 
With detailed derivations in \cref{app:path_consistency}, we show that the optimal $\alpha$-divergence regularized policy satisfies the path consistency condition in \cref{eq:path1}, which generalizes the result of \citet{chow2018path} from $\alpha=2$ to general $\alpha$.


These optimality conditions mirror the equilibrium indifference condition from \cref{sec:value_based}, where the quantity $Q(a,s) - \propt(a,s) = r(a,s) + \transitionv -\propt(a,s) = c(s)$ equals a constant for all $a \in \mathcal{A}$.




==> old/5_discussion.tex <==
\subsection{$Q$-Value Relaxations}\label{sec:qlp} \label{sec:logisticq}
\RB{Likely to be cut}
% \citet{husain2021regularized} suggest that a link between policy regularization and alternative Bellman aggregation errors.
% Similar observations have been made in the context of offline learning \citep{nachum2020reinforcement} and \gls{REPS} \citep{basserrano2021logistic}.

Among the most intriguing observations in \citet{husain2021regularized} is to relate the adversarial reward perturbation $\pr(a,s) = r(a,s) - \mr(a,s)$ to the \textsc{td}-\textsc{0} or Bellman backup error.   Similar observations have been made in the context of offline learning \citep{nachum2020reinforcement} and \gls{REPS} \citep{belousov2019entropic, basserrano2021logistic}.

However, these works require modifications to the \gls{LP} to incorporate $Q$-values, 
which is necessary since the objective in \cref{eq:dual_reg} involves $V(s)$ instead of $Q(a,s)$ as in the \textsc{td}-\textsc{0} error.
Previous work has considered a non-standard `$Q$-\textsc{lp}' \citep{nachum2020reinforcement} or introduced redundant constraints in a relaxed \gls{LP} \citep{mehta2009q, mehta2020convex, lee2019stochastic, basserrano2021logistic}. 
The latter approach considers augmenting the flow constraints with a second distribution $d(a,s)$
%One way to incorporate $Q$-values into linear or convex programming formulations of \gls{MDP}s is to consider augmenting the flow constraints with a second distribution $d(a,s)$
\begin{align}
   d(a,s) &= \mu(a,s) \label{eq:d_flow} \\
   \sum_{a} d(a,s) &= (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \nonumber
\end{align}

In \myapp{relaxed_lp}, we argue that the introduction of dual variables $\mr(a,s)$ or $\pr(a,s)$ via the convex conjugate function % of the regularizer, 
may provide an alternative justification for this relaxed \textsc{lp}.   In particular,  by further expanding the term $\Omega^{*}(\pr(a,s))$ in \cref{eq:pedro_form} using the conjugate optimization $ \max_d \langle d(a,s), \pr(a,s) \rangle - \Omega(d)$, we can obtain
%is a natural way to include 
a second state-action visitation distribution $d(a,s)$ or a second policy $d(a|s)$ with a fixed $\mu(s)$   
\small 
\begin{align}
    \hspace*{-.2cm} & \quad \max \limits_{\mu(s) \rightarrow \mathcal{M}} \max \limits_{\pi(a|s) \in \Delta^{|\mathcal{A}|}}  \min \limits_{V(s)} \min \limits_{\textcolor{\highlight}{\perturbr(a,s)}} \max \limits_{\textcolor{\highlight}{d(a,s)}} \, \label{eq:relaxed_lp_form} \\
    & \big \langle {\mu(s)\pi(a|s)}, {r(a,s) +\gamma \transitionv - V(s) - \textcolor{\highlight}{\perturbr(a,s)}} \brangle  \nonumber  \\
    &+ (1-\gamma) \blangle \nu_0(s), V(s) \brangle + \blangle \mu(s) \textcolor{\highlight}{d(a|s)}, \textcolor{\highlight}{\pr(a,s)}- \frac{1}{\beta} \Omega_{\pi_0}(\textcolor{\highlight}{d})  \brangle \, .  \nonumber
\end{align}
\normalsize
We can make several observations from this objective.  First, differentiating with respect to $\pr(a,s)$ yields the condition that $d(a|s) = \pi(a|s)$ from \cref{eq:d_flow}, with the second constraint following directly.  
Further, for \textsc{kl} divergence regularization, substituting $\pr(a,s) = Q(a,s) - V(s)$ yields the desired \textsc{td-0} error $r(a,s) +\gamma \transitionv - Q(a,s)$.
%, which we have shown are related to $Q(a,s)$ value estimates, may provide more 
We provide an alternative derivation of the Lagrangian for Logistic $Q$-learning \citep{basserrano2021logistic} in \myapp{logistic_q}, but leave further exploration, such as extending the primal dual algorithm of \citet{lee2019stochastic} to the regularized case, for future work.  

%For example, the stochastic primal-dual algorithm of \citet{lee2019stochastic} might be extended to the regularized case.  
%However, note that policy regularization
%We do not expect the approach of Logistic $Q$-learning  \citep{basserrano2021logistic}, 
%\citet{lee2019stochastic} primal dual , working with the Lagrangian

==> old/6_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this work, we have analyzed the robustness of convex-regularized \gls{RL} policies to adversarial perturbations of the reward function.   This robustness can be given a natural game-theoretic interpretation, in which the equilibrium indifference condition for the optimal policy highlights that the adversarial perturbations re-express the value of the objective function.  
Furthermore, policy regularization alone implies generalization to worst-case reward functions chosen within a particular robust set.
We have characterized the robust set of reward functions for \KL and $\alpha$-divergence regularization, and resolved apparent differences in robustness properties arising from entropy versus divergence regularization.   Our analysis integrates several existing works on adversarial robustness, and highlights how convex conjugate representations can provide additional insight into regularization in \gls{RL}.    


Among the most intriguing observations in \citet{husain2021regularized} is to relate the adversarial reward perturbation $\pr(a,s) = r(a,s) - \mr(a,s)$ to the \textsc{td}-\textsc{0} or Bellman backup error.   Similar observations have been made in the context of offline learning \citep{nachum2020reinforcement} and \gls{REPS} \citep{belousov2019entropic, basserrano2021logistic}.
%  Translating these insights into algorithmic improvements remains for future work. 
 Extending recent work on alternative Bellman error aggregation \citep{dai2018sbeed, nachum2020reinforcement, belousov2019entropic, basserrano2021logistic} to policy regularization settings, 
% \textcolor{red}{actor-critic / soft $Q$}
% or soft $Q$-learning
potentially using $\alpha$-divergence regularization or learned reference distributions \citep{grau2018soft, galashov2018information}, remains an intriguing direction for future work.

% Translating these insights into algorithmic improvements remains for future work.   Intruiging directions include adapting the primal-dual \gls{RL} algorithm of \citet{lee2019stochastic} to the regularized setting, or extending recent work on alternative Bellman error aggregation \citep{dai2018sbeed, nachum2020reinforcement, belousov2019entropic, basserrano2021logistic} to
% policy regularization settings, 
% % \textcolor{red}{actor-critic / soft $Q$}
% % or soft $Q$-learning
% potentially using learned reference distributions \citep{teh2017distral, grau2018soft} and $\alpha$-divergence regularization. %\citep{dai2018sbeed, nachum2020reinforcement, basserrano2021logistic}
%In particular, we have shown how stochastic policies %While the objective function for an unregularized, deterministic policy depends only on the value of the optimal action, stochastic policies crucially depend on $Q$ values across all actions and correspond to impli




% In this work, we have provided an integrated analysis of 
% previous work which interprets regularized policies as providing robustness to adversarial reward perturbations \TG{Don't put the emphasis on unifying previous work. Rather say that we provided an analysis of the robustness and generalization arising from regularized policies. Then mention and discuss the main findings. And then only say that this unifies/integrates previous work along the same interpretations.}.   These interpretations arise from dual representations of a convex regularization function $\Omega_{\pi_0}(\pi)$ in terms of its conjugate function $\Omega^{*}_{\pi_0}(\pi)$, with the reward perturbations $\pr(a,s)$ as dual variables.   
% For a given regularization function and strength, this matches the duality between a stochastic policy and the estimated $Q$-values of an agent, so that adversarial reward perturbations represent a natural justification for including $Q$-values in convex programming formulations of \gls{RL}.  
% We hope that these observations will be useful to further develop and understand \gls{RL} algorithms using convex duality. \TG{Ok, but the main findings/takeaways are missing! What do we conclude about the nature of the robustness that we get from policy regularization? How does it relate to the adversarial interpretation (and the indifference principle)? Comment on maxent vs. KL vs. alpha-div regulariztion. What have we seen from looking at the feasible set?}





==> old/7_pyco.tex <==
\section{Visualizations}\label{sec:visualizations}
\begin{figure*}[t]
\begin{subfigure}{.2\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_world.pdf}\vspace*{.2cm}
\caption{Environment \\
($r(a,s) = -1$ for water, \\
$r(a,s) = 5$ for goal) \label{fig:pyco_env}}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta02_alpha1_gamma99.pdf}
\caption{$\beta = 0.2$ (High Reg.)}\label{fig:pyco_beta02}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta1_alpha1_gamma99.pdf}
\caption{$\beta = 1$}\label{fig:pyco_beta1}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta10_alpha1_gamma99.pdf}
\caption{$\beta = 10$ (Low Reg.)}\label{fig:pyco_beta02}
\end{subfigure} 
% \\
% \begin{subfigure}{.2\textwidth}
% \end{subfigure}
% \begin{subfigure}{.26\textwidth}
% \includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta02_alpha1_gamma99_perturbed.pdf}
% \caption{$\beta = 0.2$ (High Reg.)}\label{fig:pyco_beta02}
% \end{subfigure}
% \begin{subfigure}{.26\textwidth}
% \includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta1_alpha1_gamma99_perturbed.pdf}
% \caption{$\beta = 1$}\label{fig:pyco_beta1}
% \end{subfigure}
% \begin{subfigure}{.26\textwidth}
% \includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta10_alpha1_gamma99_perturbed.pdf}
% \caption{$\beta = 10$ (Low Reg.)}\label{fig:pyco_beta02}
% \end{subfigure}
\caption{\label{fig:pyco} Optimal adversarial reward perturbations $\propt(a,s) = \frac{1}{\beta}\log \frac{\pi(a|s)}{ \pi_0(a|s)}$ for a sequential setting. Policy trained with \textsc{kl} divergence regularization,  $\gamma$ = 0.99.  Red indicates robustness to negative reward perturbations.}
\end{figure*}

\begin{figure*}[t]
\begin{subfigure}{.2\textwidth}
\phantom{\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_world.pdf}\vspace*{.2cm}}
% \caption{\centering Environment \\
% ($r(a,s) = -1$ for water, \\
% $r(a,s) = 5$ for goal)}\label{fig:pyco_env}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta02_alpha1_gamma99_perturbed.pdf}
\caption{$\beta = 0.2$ (High Reg.)}\label{fig:pyco_beta02}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta1_alpha1_gamma99_perturbed.pdf}
\caption{$\beta = 1$}\label{fig:pyco_beta1}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
\includegraphics[width=\textwidth]{figs/pyco_perturb/pyco_beta10_alpha1_gamma99_perturbed.pdf}
\caption{$\beta = 10$ (Low Reg.)}\label{fig:pyco_beta02}
\end{subfigure}
\caption{\label{fig:pyco} Perturbed rewards $\mr(a,s) = r(a,s) - \pr(a,s)$ for policies trained with \textsc{kl} divergence regularization.  The indifference condition holds in all cases, with $\mr(a,s) = c(s)$ for each action, and at each state and $c(s) = V(s)$ for \textsc{kl} regularization.  This confirms that the policy is optimal \citep{ortega2014adversarial, nachum2017bridging}.}
\end{figure*}

==> sections/feasible_fig.tex <==
\begin{figure*}[!t]
\vspace*{-1.5cm}
\centering
% \begin{minipage}{\textwidth}%{0.8\textwidth}
%\centering
\begin{center}
\[\arraycolsep=.003\textwidth
\begin{array}{cccccc} %[width=40mm]
 \begin{subfigure}{0.07\textwidth} \vspace*{-.24cm} \includegraphics[width=\textwidth]
 {figs/feasible/uniform_prior.png} \end{subfigure}& %\qquad  \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_uniform_01.png}
{figs/feasible/kl/beta01alpha1uniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}& % \qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_uniform_1.png}
{figs/feasible/kl/beta1alpha1uniform.pdf}
\caption{ \centering  $D_{KL}, \beta = 1$}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_uniform_10.png} 
{figs/feasible/kl/beta10alpha1uniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 10$}\end{subfigure}& \rulesep
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
% {figs/feasible/alpha-1_no_lambda/alpha_neg1_beta1_uniform.png} 
{figs/feasible/alpha-1/alpha_neg1_beta10uniform.pdf}
\caption{\centering \small $\alpha = -1, \beta = 10$}\end{subfigure}&
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth, trim= 0 0 0 0, clip]
{figs/feasible/alpha3/alpha3_beta10uniform.pdf}
% {figs/feasible/alpha3_no_lambda/alpha3_beta10_uniform_redo.pdf}
\caption{ \centering \small $\alpha = 3, \beta = 10$}\end{subfigure}
\\ %&\hspace*{.2cm}\\
\begin{subfigure}{0.07\textwidth}\vspace*{-.24cm} \includegraphics[width=\textwidth]{figs/feasible/nonuniform_prior.png}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_73_01.png}
{figs/feasible/kl/beta01alpha1nonuniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 0.1$}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_73_1.png}
{figs/feasible/kl/beta1alpha1nonuniform.pdf}
\caption{ \centering \small $D_{KL}, \beta = 1$}\end{subfigure}& %\qquad \hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/kl_73_10.png} 
{figs/feasible/kl/beta10alpha1nonuniform.pdf}
\caption{\centering \small $D_{KL}, \beta = 10$}\end{subfigure}& \rulesep %\hspace*{.2cm}
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip]
% {figs/feasible/alpha-1_no_lambda/alpha_neg1_beta1_nonuniform.png} 
% {figs/feasible/alpha-1_no_lambda/alpha_neg1_beta1_nonuniform_redo.pdf}
{figs/feasible/alpha-1/alpha_neg1_beta10nonuniform.pdf}
\caption{\centering \small $\alpha = -1, \beta = 10$}\end{subfigure}&
\begin{subfigure}{0.175\textwidth}\includegraphics[width=\textwidth,  clip] 
{figs/feasible/alpha3/alpha3_beta10nonuniform.pdf}
% {figs/feasible/alpha3_no_lambda/alpha3_beta10_nonuniform_redo.pdf}
\caption{ \centering \small $\alpha = 3, \beta = 10$}\end{subfigure}
\end{array}
\] 
\end{center}
% \end{minipage}
\vspace*{-.28cm}
\caption{\textbf{Robust Set} (red region) of perturbed reward functions to which a stochastic policy generalizes, in the sense that the policy is guaranteed to achieve an expected modified reward greater than or equal to the value of the regularized objective (\cref{eq:generalization}).  
The robust set characterizes the perturbed rewards achievable by the adversary. Red stars indicate the worst-case perturbed reward $\mr_{\piopt} = r - \pr_{\piopt}$ (\myprop{optimal_perturbations}).
We show feasible sets 
% for \textsc{kl} divergence (at various $\beta$) and $\alpha$-divergence ($\alpha=\{-1, 3\}, \beta =10$) regularization, 
% \TG{Do we need the two statements in brackets? It's obvious from the figure.}
 for the optimal $\pi_*(a|s)$ associated with fixed $Q(a,s)=r(a,s)$ values (blue star), where the policy differs based on the regularization parameters $\alpha, \beta, \pi_0$--- see \cref{eq:optimal_policy}.  The robust set becomes more restricted with decreasing regularization strength (increasing $\beta$), implying decreased generalization.
Importantly, the slope of the boundary of the robust set can be directly linked to the action probabilities under the given policy (see \mysec{visualizations_feasible}). 
% become more axis-aligned with decreasing regularization strength, which c
The shape of the robust set is affected by the choice of $\alpha$-divergence and reference $\pi_0$.
% \TG{This last sentence is also obvious from the figure and we have it in the main text.}.
% stochasticity of the optimal policy (see \mysec{generalization})
% of less regularized policies. choice
% The particular shape of the feasible set is affected by the choice of $\alpha$-divergence and reference $\pi_0$. Importantly, the slopes of the boundaries of the feasible set become more axis-aligned with decreasing regularization strength, which can be directly linked to the stochasticity of the optimal policy (see \mysec{generalization}).
% Top row:  reference distribution $\pi_0=(\frac{1}{2},\frac{1}{2})$, bottom row: $\pi_0 = (\frac{2}{3}, \frac{1}{3})$. 
% \TG{Missing: describe the results (size and shape of the set in relation to regularization strength).} 
% Red dot indicates $Q(a,s)$ associated with policy $\pi(a|s)$
}\label{fig:feasible_set_main}
\end{figure*}
\headerv




==> sections/new/1_tmlr_submit_prelim.tex <==
\headerv
\headerv
\section{Preliminaries}\label{sec:prelim}
\headerv

In this section, we review
% provide background on 
\gls{LP} formulations of %fully observed, 
discounted \gls{MDP} and extensions to convex policy regularization.
We begin by reviewing the convex conjugate function, also known as the Legendre-Fenchel transform, which will play a crucial role throughout our paper.

\headerv
\subsection{Convex Conjugate Function}\label{sec:conj_intro}
\headerv

% Before describing analogous primal and dual optimizations for regularized \gls{MDP}s, we review the convex conjugate function, or Legendre-Fenchel transform, which will play a crucial role throughout our paper.
%First,
For any convex function $\Omega(\primalvar)$ with domain $\primalvar \in \mathcal{D}$, 
%, where $\mathcal{D}$ may indicate the probability simplex $\Delta^{|A|}$ with possible additional constraints, such as $\mu_{\pi}(a,s) \in \mathcal{M}$
%over domain $\pi \in \Delta^{|\mathcal{A}|}$, possibly , 
%the Legendre-Fenchel transform or 
the conjugate function $\Omega^{*}$ is defined via the optimization
% \RB{what choice of primal variable? $\tpi$ is in function space in general, but will end up being a distribution}
% \RB{explain inner product notation here? what choice of primal variable $\primalvar$?} \TG{Yes both, but brief.}
\begin{align}
    \Omega^{*}( \dualvar ) = \sup \limits_{\primalvar \in \mathcal{D}} \, \big \langle \primalvar, \dualvar \big \rangle - \Omega(\primalvar) \label{eq:conjstar}
\end{align} 
where $\dualvar \in \dualdomain$ is 
% a function 
in the 
% continuous 
dual space of $\primalvar$ and $\langle \cdot, \cdot \rangle$ indicates the inner product.
% summation or integration over the dimensionality of the domain.  \RB{awkward?}
% $\mathcal{D}$ or $\dualdomain$. %continuous function in the topological dual space of $\pi$. %arbitrary function whose domain has the same dimension as $\mathcal{D}$.  
 %The conjugate function 
 The conjugate operation is an involution for proper, lower semi-continuous, convex $\Omega$ \citep{boyd2004convex},
 %(\citet{borwein2010convex} Sec. 4.3), 
 so that $(\Omega^{*})^{*} = \Omega$ and $\Omega^{*}$ is also convex.  
 We can thus represent $\Omega(\primalvar)$ via a conjugate optimization
 \begin{align}
     \Omega(\primalvar) = \sup_{\dualvar \in \dualdomain} \big \langle \primalvar, \dualvar \big \rangle - \Omega^{*}(\dualvar). \label{eq:conjomega}
 \end{align}
  %   Solving for the $\arg \sup$ in either \cref{eq:conjstar} or \cref{eq:conjomega} suggests optimality conditions for $\pi_*$ and $\dualvar$
  Differentiating with respect to the optimization variable in \cref{eq:conjstar} or (\ref{eq:conjomega}) suggests the optimality conditions 
%  \begin{align}
%      \primalvar(a,s) = \nabla \Omega^{*}( \dualvar )   \quad \qquad \dualvar(a,s) = \nabla \Omega(\primalvar) \, .     \label{eq:optimal_policy_as_grad}
%  \end{align}
% From the above, conjugacy also implies relationships of the form $\primalvar(a,s) = (\nabla \Omega)^{-1}(\dualvar(a,s))$, for example, when $\primalvar$ and $\dualvar$ are in dual correspondence.
% We provide examples of the convex conjugate for common divergence functions in \mytab{conj_table}.
  \begin{align}
     \primalvar_{\dualvar} = \nabla \Omega^{*}( \dualvar )   \quad \qquad \dualvar_{\primalvar} = \nabla \Omega(\primalvar) \, .     \label{eq:optimal_policy_as_grad}
 \end{align}
 Note that the above conditions also imply relationships of the form $\primalvar_{\dualvar} = (\nabla \Omega)^{-1}(\dualvar)$.   This dual correspondence between 
%  particular 
 values of $\primalvar$ and $\dualvar$ will form the basis of our adversarial interpretation in \mysec{adversarial_perturb}.
 
%  From the above, conjugacy also implies relationships of the form $\primalvar = (\nabla \Omega)^{-1}(\dualvar)$ when $\primalvar$ and $\dualvar$ are in dual correspondence.  
%  This correspondence will form the basis of our adversarial interpretation in \mysec{adversarial_perturb}.
%  We will make use of these conditions to associate 
%  , for example,

\headerv
\subsection{Divergence Functions}\label{sec:divergence_intro}
\headerv
% The family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases, 
% We will consider regularization using 
We are interested in the conjugate duality associated with 
policy regularization, which is often expressed using a
statistical divergence $\Omega(\mu)$ over a joint density $\mu(a,s) = \mu(s) \pi(a|s)$ (see \mysec{mdp_background}).  %commonly-used 
% where 
% The notation $\mu(a,s) = \mu(s) \pi(a|s)$ indicates a joint density
% which we will describe 
% whose meaning is described
% in \mysec{mdp_background}.
% which are used as regularization for \gls{RL} policies in \mysec{mdp_background}.   
In particular, we consider
the family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases.    
In the following, we consider extended divergences that accept unnormalized density functions as input \citep{zhu1995information} 
so that we may
% in order to 
 analyze function space dualities and evaluate Lagrangian relaxations without
%  , for example, 
projection
%the need to project 
 onto the probability simplex.
% so that Lagrangian relaxations in later sections will be well-defined even if normalization constraints are not satisfied.   

% \textcolor{red}{so that Lagrangian relaxations such as \cref{eq:dual_lagrangian} are well defined even when normalization constraints are not satisfied.}
% $\mu(a,s)$ is not normalized.}
% \textcolor{blue}{$\mu(a,s) \not \in \Delta^{|\mathcal{A}| \times |\mathcal{S}|}$.}

%  We primarily focus on policy regularization using a conditional divergence $\Omega^{(\alpha)}_{\pi_0}(\mu)$ to a reference policy $\pi_0(a|s)$.
% % but we also discuss regularization of the joint state-action occupancy to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$, in \textcolor{blue}{in \mysec{?}}.   
% Note that we consider the regularizer to be a function of $\mu(a,s)$, since it is applied 
% % in 
% across
% each 
% % $s \in \mathcal{S}$ 
% state
% % $s \sim \mu_\pi(s)$
% % \textcolor{red}{$s \sim \mu_\pi(s)$} 
% visited by the agent.
% \textcolor{blue}{In \mysec{?}}, we also discuss regularizing the joint state-action occupancy to be close to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$. 
% % \citep{nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.

% \RB{Need 2nd paragraph??  Smoother intro?}

% \RB{Remove all $\mu(s)$ below?}
% % \RB{REMOVE ALL THE $\mu(s)$ in Divergence derivations?}

\paragraph{KL Divergence}
% Taking the limit as $\alpha \rightarrow 1$, we obtain
% an (extended version of) 
The `forward' \textsc{kl} divergence to a reference policy $\pi_0(a|s)$ is commonly used for policy regularization in \gls{RL}.  
Extending the input domain to unnormalized measures, we write the divergence as
% \citep{zhu1995information},
% \citep{cichocki2010families}, 
%  (\citet{tishby2011information, ortega2013thermodynamics, fox2016taming})
\begin{align}
        &\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\Big[D_{KL}[\pi:\pi_0]\Big] = \sum \limits_{s \in \mathcal{S}} \mu(s) \sum \limits_{a \in \mathcal{A}}  \left(\pi(a|s)  \log \frac{\pi(a|s)}{\pi_0(a|s)} -  
        % \sum \limits_{a, s} 
      \pi(a|s) 
        + 
        % \sum \limits_{a,s} 
      \pi_0(a|s)\right). \label{eq:kl_def} 
\end{align}
\normalsize
Using a uniform reference  $\pi_0(a|s) = 1$ $\forall 
\, (a,s)$, we recover the Shannon entropy up to an additive constant.
%Up to an additive constant, we recover the Shannon entropy using a uniform reference, $\pi_0(a|s) = 1$ $\forall \, (a,s).$ 
% \in \mathcal{A} \times \mathcal{S}$.
% \, a \in \mathcal{A}, s \in \mathcal{S}$. 
% the final terms cancel if both $\pi$ and $\pi_0$ are normalized.


\paragraph{$\alpha$-Divergence} The $\alpha$-divergence $\mathbb{E}_{\mu(s)}\big[D_{\alpha}[\pi_0:\pi]\big]$ over possibly unnormalized measures
%$\omegamu &= \mathbb{E}_{\mu(s)}\big[D_{\alpha}[\pi_0:\pi]\big]$, 
is defined as 
% \footnotesize
\begin{align}
\hspace*{-.1cm} 
\Omega^{(\alpha)}_{\pi_0}(\mu)& =
% \mathbb{E}_{\mu(s)}\big[
% D_{\alpha}[\pi_0:\pi]
% \big]
% &= 
\frac{1}{\alpha(1-\alpha)} 
% \sum \limits_{s \in \mathcal{S}}
\sum \limits_{s \in \mathcal{S}}
\mu(s)
    \bigg( (1-\alpha) 
    % \sum \limits_{a \in \mathcal{A}} 
    \sum \limits_{a \in \mathcal{A}}
    \pi_0(a|s) 
    %+\alpha 
    % \\ &\phantom{\sum \limits_{s \in \mathcal{S}}\mu(s)} 
    + \alpha 
    % \sum \limits_{a \in \mathcal{A}} 
    \sum \limits_{a \in \mathcal{A}}
    \pi(a|s) 
    % \nonumber 
    % &- \sum \limits_{a \in \mathcal{A}} 
    % \\ &\phantom{\sum \limits_{s} \mu(s)} 
    - \sum \limits_{a \in \mathcal{A}} 
    \pi_0(a|s)^{1-\alpha} \pi(a|s)^{\alpha} \bigg)  
    % \label{eq:alpha_def}
    \label{eq:alpha_def} 
\end{align}
\normalsize
Taking the limiting behavior, we recover the `forward' \textsc{kl} divergence $D_{KL}[\pi:\pi_0]$ as $\alpha \rightarrow 1$ or the `reverse' \textsc{kl} divergence $D_{KL}[\pi_0:\pi]$ as $\alpha \rightarrow 0$.


To provide intuition for 
% for?  contextualize?  understand?}
the $\alpha$-divergence, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential, with
\begin{align}
    \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , 
    % \label{eq:qlog}  
    \qquad \qquad 
    \exp_{\alpha}(u) = [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, . \label{eq:qexp}
    % \hfill \, \,  \alpha \neq 1 \
\end{align}
\textcolor{black}{where $[\cdot]_+ = \max(\cdot,0)$ ensures fractional powers can be taken and suggests that $\exp_{\alpha}(u)=0$ for $u \leq 1/(1-\alpha)$.}
% Using $\log_{\alpha}$, 
Using the $\alpha$-logarithm, we can rewrite the $\alpha$-divergence 
% in similar fashion to
similarly to
the \kl divergence in 
\cref{eq:kl_def}
% \scriptsize
\resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
\begin{align}
  \Omega^{(\alpha)}_{\pi_0}(\mu) &= \frac{1}{\alpha} \sum \limits_{s \in \mathcal{S}} \mu(s) \bigg( \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)} - \pi(a|s) + \pi_0(a|s) \bigg) \nonumber.
\end{align}
}}
\normalsize
For a uniform reference $\pi_0$, the $\alpha$-divergence 
differs from the Tsallis entropy by only the $1/\alpha$ factor and an additive constant (see \myapp{tsallis}).

\headerv
\subsection{Unregularized MDPs}\label{sec:mdp_background}
% \subsection{MDPs as Linear or Convex Programs}\label{sec:mdp_background}
% \subsection{Linear $\&$ Convex Programming Formulations of MDPs}
\headerv
% \vspace*{\header}

% \paragraph{Unregularized Case}
A discounted \gls{MDP} is a tuple $\{ \mathcal{S}, \mathcal{A}, P, \nu_0, r, \gamma \}$ consisting of a state space $\mathcal{S}$, action space $\mathcal{A}$, transition dynamics $P(s\tick|s,a)$ for $s, s\tick \in \mathcal{S}$, $a \in \mathcal{A}$, initial state distribution $\nu_0(s) \in \Delta^{|\mathcal{S}|}$ in the probability simplex, and reward function $r(a,s):\mathcal{S} \times \mathcal{A} \mapsto \mathbb{R}$.   We also use a discount factor $\gamma\in (0,1)$ 
(\citet{puterman2014markov} Sec 6).
% , although discounting may also be handled by including a transition to an absorbing state in the \gls{MDP} (\citet{puterman2014markov} Sec. 5.3). 
% in the \gls{MDP}

% \paragraph{Unregularized Case}
We consider an agent that seeks to maximize the expected discounted reward by acting according to a decision policy 
% $\{ \pi(a|s) \in \Delta^{|\mathcal{A}|} \}_{s \in \mathcal{S}}$.
$\pi(a_t|s_t) \in \Delta^{|\mathcal{A}|}$. %\, \,\, {\forall s_t \in \mathcal{S}}  
The expected reward is calculated over trajectories ${\tau \sim \pi(\tau):= \nu_0(s_0) \prod \pi(a_t | s_t) P(s_{t+1} | s_t, a_t)}$, which begin from an initial $s_0 \sim \nu_0(s)$ and evolve according to the policy and \gls{MDP} dynamics $P(s\tick|s,a)$  
% We consider an agent that acts according to a decision policy $\pi(a_t|s_t) \in \Delta^{|\mathcal{A}|}$, seeking to maximize the expected discounted reward over trajectories ${\tau \sim \pi(\tau):= \nu_0(s_0) \prod \pi(a_t | s_t) P(s_{t+1} | s_t, a_t)}$ which start from $s_0 \sim \nu_0(s)$ and evolve according to the policy and \gls{MDP} dynamics $P(s\tick|s,a)$.  
% Thus, the objective in \cref{eq:primal_lp} can be rewritten in similar fashion to \cref{eq:reward_perturbation_stmt}
% This leads to the objective function
\small
\begin{align}
  \hspace*{-.2cm}
  \obj(r) := 
   \max \limits_{\pi(a|s)} \, (1-\gamma) \, \mathbb{E}_{\tau \sim \pi(\tau)} \bigg[ \sum \limits_{t=0}^{\infty} \gamma^t \, r(s_t, a_t)  \bigg] \, . \label{eq:policy_only} 
\end{align}
\normalsize
We assume that the policy is stationary and Markovian, and thus independent of both the timestep and trajectory history.  

% \paragraph{MDPs as Linear Programs}
\paragraph{Linear Programming Formulation}
% % \RB{We adopt notation, For the remainder of the paper, heavy use}
% % To highlight connections with the literature on convex duality, we consider 
% For the remainder of the paper, we will consider
% an equivalent \gls{LP} formulation in which optimization is performed over the discounted 
% % joint 
% state-action occupancy measure 
% $\mu(a,s) \coloneqq (1-\gamma) \mathbb{E}_{\tau\sim \pi(\tau)} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$,
% % with
% For the remainder of this work, 
In what follows, we will focus on 
a linear programming (\gls{LP}) form for the objective in \cref{eq:policy_only}, which is common in the literature on convex duality.
% an equivalent \gls{LP} formulation which is common in the literature on convex duality.   
With optimization over the discounted 
state-action occupancy measure, 
% ${\mu(a,s) \coloneqq (1-\gamma)} \mathbb{E} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$, we have
${\mu(a,s) \coloneqq (1-\gamma)} \mathbb{E}_{\tau\sim \pi(\tau)} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$, the objective can be rewritten
% becomes
% With optimization over the discounted 
% state-action occupancy measure 
% ${\mu(a,s) \coloneqq (1-\gamma)} \mathbb{E}_{\tau\sim \pi(\tau)} \left[ \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(a_t = a, s_t = s)\right]$, 
% \small
% \begin{align}
%   \hspace*{-.2cm} &  
%   \obj(r) :=
%   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \, \, \text{subj. to} \, \quad    \left( \forall s \in \mathcal{S} \right) \label{eq:primal_lp}\\[1.25ex]
%   &\sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \nonumber  \, ,
%   %\, \forall s \in \mathcal{S}\nonumber
% \end{align}
\small
\begin{align}
   \hspace*{-.23cm}  
   \obj(r) \coloneqq
   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \qquad \text{subject to } \quad \mu(a,s) &\geq 0 \qquad \forall (a,s) \in \mathcal{A} \times \mathcal{S},   \quad  \label{eq:primal_lp} \\
    \sum_{a} \mu(a,s)& = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \qquad \forall s \in \mathcal{S}, \nonumber 
   %\left( \forall s \in \mathcal{S} \right) 
   %\, \forall s \in \mathcal{S}\nonumber
\end{align}
% \small
% \begin{align}
%   \hspace*{-.23cm}  
%   \obj(r) \coloneqq
%   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \qquad \text{subject to } \quad \forall (a,s) \in \mathcal{A} \times \mathcal{S}:&   \quad  \mu(a,s) \geq 0  \label{eq:primal_lp} \\
%     \quad \forall s \in \mathcal{S}:& \quad \sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick)  \nonumber 
%   %\left( \forall s \in \mathcal{S} \right) 
%   %\, \forall s \in \mathcal{S}\nonumber
% \end{align}
% \footnotesize
% \begin{align}
%   \hspace*{-.2cm} &  
%   \obj(r) :=
%   \max \limits_{\mu(a,s)} \big \langle {\mu(a,s)}, {r(a,s)} \big \rangle \, \, \label{eq:primal_lp} \\
%   &\phantom{ \obj(r) :=} \text{subj. to} \, \,\mu(a,s) \geq 0 \quad \forall (a, s) \in \mathcal{A} \times \mathcal{S}   \nonumber  \\[1.25ex] %
%   &\sum_{a} \mu(a,s) = (1-\gamma) \nu_0(s) + \gamma \sum_{a\tick, s\tick} P(s|a\tick, s\tick) \mu(a\tick,s\tick) \, \,  \forall s \in \mathcal{S}  \nonumber  \, , %\left( \forall s \in \mathcal{S} \right)
%   %\, \forall s \in \mathcal{S}\nonumber
% \end{align}
\normalsize
% \RB{$\mu(a,s) \geq 0 $ leads to $V \geq r + \gamma\transitionv$ \textit{inequality} constraint}
where inner product notation 
% $\langle \cdot, \cdot \rangle$ 
indicates summation or integration over the domain of $\mu$. 
% and nonnegativity constraints apply for each $(a, s) \in \mathcal{A} \times \mathcal{S}$. %\RB{improve} %$\sum \mu \cdot \dualvar$
%The optimization is over state-action visitation distributions $\mu(a,s) \in \Delta^{|\mathcal{S}| \times |\mathcal{A}|} $, and a corresponding policy is obtained via $\pi(a|s) = \mu(a,s) / \sum_a \mu(a,s)$.   
We refer to the constraints in the second line of \cref{eq:primal_lp} as the \textit{Bellman flow constraints}, which force $\mu(a,s)$ to respect the \gls{MDP} dynamics.
%and denote the set of feasible $\mu$ as $\mathcal{M}$. For normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$, we show in \myapp{normalized_mu} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized.
We denote the set of feasible $\mu$ as $\mathcal{M}$.    For normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$,   we show in \myapp{optimal_policy} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s)$
% \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ 
is normalized. 
% we show in \myapp{normalized_mu} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized. 
% We denote the set of feasible $\mu$ as $\mathcal{M}$
% % For normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$, we show in \myapp{normalized_mu} that $\mu(a,s) \in \mathcal{M}$ implies $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized. 
% and in \myapp{normalized_mu}, show that $\mu(a,s) \in \mathcal{M}$ implies that $\mu(a,s) \in \Delta^{|\mathcal{A}|\times|\mathcal{S}|}$ is normalized for normalized $\nu_0(s)$ and $P(s|a\tick, s\tick)$.
% % assuming $\nu_0(s)$ and $P(s|a\tick, s\tick)$ are normalized.

% \RB{Flow constraints force $\mu$ to respect dynamics}
% \RB{Mention that $\nu_0(s), P(s\tick|s,a)$ normalized implies $\mu(a,s) \in \mathcal{M}$ normalized} 
\input{sections/conj_table}

It can be shown that any feasible $\mu(a,s) \in \mathcal{M}$  induces a stationary $\pi(a|s) = \mu(a,s) / 
\mu(s)$, 
% \sum_{a\tick} \mu(a\tick,s)
where  $\mu(s) \coloneqq \sum_{a\tick} \mu(a\tick,s)$ and $\pi(a|s) \in \Delta^{|\mathcal{A}|}$ is normalized by definition.
% \footnote{To see this, since $\sum_a \frac{\mu(a,s)}{\sum_{a'} \mu(s)}= \frac{\sum_a \mu(a,s)}{\mu(s)} = 1$.} 
% \footnote{The policy is always normalized 
% % even if $\mu(a,s)$ is not, 
% since $\sum_a \frac{\mu(a,s)}{\sum_{a'} \mu(s)}= \frac{\sum_a \mu(a,s)}{\mu(s)} = 1$.}$
Conversely, any stationary policy $\pi(a|s)$ induces a unique state-action visitation distribution $\mu(a,s)$ (\citet{syed2008apprenticeship},
\citet{feinberg2012handbook} Sec. 6.3).
%\citet{puterman2014markov} Sec. ??).
 Along with the definition of $\mu(a,s)$ above, 
%  this demonstrates 
this result demonstrates
 the equivalence of the optimizations in \cref{eq:policy_only} and \cref{eq:primal_lp}.  We will proceed with the \gls{LP} notation from \cref{eq:primal_lp} and assume $\mu(s)$ is induced by
%the corresponding 
$\pi(a|s)$ whenever the two appear together in an expression.
% It can be shown that any stationary policy $\pi(a|s)$ induces a unique state-action 
% visitation distribution $\mu(a,s)$, while, conversely, a feasible $\mu(a,s) \in \mathcal{M}$  is induced by some stationary $\pi(a|s) = \mu(a,s) / \mu(s)$ (\citep{syed2008apprenticeship}, \citet{feinberg2012handbook} Sec. 6.3).   

% where the marginal state-visitation distribution $\mu(s) \propto (1-\gamma) \sum_{t=0}^\infty \gamma^t \, \mathbb{I}(s_t = s)$ a
% The flow constraints in \cref{eq:primal_lp} are insightful, as they lead to a dual optimization reflecting the familiar Bellman equations \citep{bellman1957markovian}. 
Importantly, the flow constraints in \cref{eq:primal_lp} lead to a dual optimization which reflects the familiar Bellman equations \citep{bellman1957markovian}. 
To see this, we introduce Lagrange multipliers $V(s)$ for each flow constraint and $\lambdaplus \geq 0$ for the nonnegativity constraints.  Summing over $s \in \mathcal{S}$, and eliminating $\mu(a,s)$ by setting $d/d\mu(a,s) = 0$ yields the \textit{dual} \gls{LP}
% Introducing Lagrange multipliers $V(s)$ for each flow constraint, summing over $s \in \mathcal{S}$, and eliminating $\mu(a,s)$ by setting $d/d\mu(a,s) = 0$ yields the \textit{dual} \gls{LP}
% \begin{align}
%   &\obj^{*}(r):=\min \limits_{V(s)} \,  (1-\gamma) \big \langle \nu_0(s), V(s) \big \rangle \, \text{  subj to: }\, \label{eq:dual_lp} \\ %\quad \forall (a,s) \in \mathcal{S} \times \mathcal{A}
%   & \, V(s) = r(a,s) + \gamma \transitionv + \lambdaplus 
% %   \,\, \forall (a,s) \in \mathcal{A} \times \mathcal{S}  
%  \nonumber \, ,
% \end{align}
% \small
\begin{align}
 \hspace*{-.2cm} \obj^{*}(r)&\coloneqq
  \min \limits_{V(s), \lambdaplus} \,
%   \min \limits_{V(s)} \,  
  (1-\gamma) \big \langle \nu_0(s), V(s) \big \rangle  
%   \\
%   \text{  subj to: }\label{eq:dual_lp} \\ %\quad \forall (a,s) \in \mathcal{S} \times \mathcal{A}
 \quad \text{  subject to } \,\,\, V(s) = r(a,s) + \gamma \transitionv + \lambdaplus 
%  \quad \forall (a,s) \in \mathcal{A} \times \mathcal{S}  
 \label{eq:dual_lp} , 
%  \nonumber \, ,
\end{align}
\normalsize
% where the constraint applies for all $(a,s) \in \mathcal{A} \times \mathcal{S}$ and $\lambdaplus \geq 0$.  By complementary slackness \citep{boyd2004convex}, we know that $\lambdaplus =0$ for $\mu(a,s) > 0$.
% Finally,  we use $\transitionv$ as shorthand for $\mathbb{E}_{P(s\tick|a,s)}[ V(s\tick)]$ and have reindexed the transition tuple from $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared to \cref{eq:primal_lp}. 
where we have used $\transitionv$ as shorthand for $\mathbb{E}_{P(s\tick|a,s)}[ V(s\tick)]$ and reindexed the transition tuple from $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared to \cref{eq:primal_lp}.   Note that the constraint applies for all $(a,s) \in \mathcal{A} \times \mathcal{S}$ and that $\lambdaplus \geq 0$.  By complementary slackness, 
% \citep{boyd2004convex}, 
we know that $\lambdaplus =0$ for $(a,s)$ such that $\mu(a,s) > 0$.

% In similar fashion to the conjugate optimizations in \cref{eq:conjstar}-\ref{eq:conjomega}, these dual objectives have the same solution under strong duality, despite optimizing over different variables.

% where the constraint applies for all $(a,s) \in \mathcal{A} \times \mathcal{S}$ and $\lambdaplus \geq 0$.  By complementary slackness, 
% % \citep{boyd2004convex}, 
% we know that $\lambdaplus =0$ for $(a,s)$ such that $\mu(a,s) > 0$.
% Finally, we have used $\transitionv$ as shorthand for $\mathbb{E}_{P(s\tick|a,s)}[ V(s\tick)]$ and reindexed the transition tuple from $(s\tick, a\tick, s)$ to $(s,a, s\tick)$ compared to \cref{eq:primal_lp}. 

% By complementary slackness \citep{boyd2004convex}, we know that $\lambdaplus =0$ for $(a,s)$ such that $\mu(a,s) > 0$.
% It is easy to show that the optimal policy is deterministic if $a_{\text{max}} \coloneqq \arg \max_a r(a,s) + \gamma \transitionv$ is unique, with $\pi_*(a_{\text{max}}|s) = 1$ and $V(s) = r(a_{\text{max}},s) + \gamma 
% \mathbb{E}_{a_{\text{max}},s}^{s\tick}\left[V(s\tick)\right]$.
% % \transitionv$
% $\lambda(a_{\text{max}}, s) = V(s) - r(a,s) - \gamma \transitionv > 0$.

% \paragraph{Regularized Case}
\headerv
\subsection{Regularized MDPs}\label{sec:mdp_regularized}
\headerv
We now consider regularizing the objective in \cref{eq:primal_lp} using a convex penalty function $\Omega(\mu)$ with coefficient $1/\beta$.   
We primarily focus on regularization using a conditional divergence $\Omega_{\pi_0}(\mu) \coloneqq \mathbb{E}_{\mu(s)\pi(a|s)}[\ptReg(\pi)]$ between the policy and a normalized reference distribution $\pi_0(a|s)$, as in \mysec{divergence_intro} and \citep{ortega2013thermodynamics,fox2016taming,haarnoja17a,haarnoja2018soft}.   
We also use the notation $\Omega_{\mu_0}(\mu) = \mathbb{E}_{\mu(a,s)}[\ptReg(\mu)]$ to indicate regularization of the full state-action occupancy measure to a normalized reference $\mu_0(a,s)$,  which appears, for example, in \gls{REPS} \citep{peters2010relative, belousov2019entropic}.   
% We assume the reference is normalized, either $\sum_a \pi_0(a|s) =1$ or $\sum_{a,s} \mu_0(a,s)=1$.
% We will also consider regularization of the full state-action occupancy measure to a reference $\mu_0(a,s)$, using the notation $\Omega_{\mu_0}(\mu) = \mathbb{E}_{\mu(a,s)}[\ptReg(\mu)]$ \citep{peters2010relative, belousov2019entropic, basserrano2021logistic}.
% The regularizer may be either a conditional divergence $\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)\pi(a|s)}[\ptReg(\pi)]$ between the policy and a reference distribution $\pi_0(a|s)$, or a divergence $\Omega_{\mu_0}(\mu) = \mathbb{E}_{\mu(a,s)}[\ptReg(\mu)]$ over the joint state-action occupancy measure with reference $\mu_0(a,s)$. \RB{?? Later.  reference \mysec{divergence_intro}}
% % We will consider $\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)\pi(a|s)}[\ptReg(\pi)]$ to be a conditional divergence between the policy and a reference distribution $\pi_0(a|s)$ that can be written with an outer expectation over $\mu(a,s)$.~\footnote{We focus on policy regularization \citep{neu2017unified} in this work, but similar reasoning may be applied for regularizing the joint state-action occupancy $\mu(a,s)$ \citep{nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.} 
% Letting $\Omega_{\pi_0}(\pi)$ be a statistical divergence between the policy and a reference distribution $\pi_0(a|s)$, 
% We define the regularized objective as 
The regularized objective $\obj_{\Omega, \beta}(r)$ is then defined as
% $\obj_{\Omega, \beta}(r)$
\begin{equation}
% \resizebox{.87\columnwidth}{!}{ \hspace*{-.2cm}   $
\obj_{\Omega, \beta}(r) :=  \max \limits_{\mu(a,s) \in \mathcal{M} } %\max \limits_{\pi(a|s) \in \Delta^{|A|}} 
   \blangle \mu(a,s), r(a,s) \brangle - \dfrac{1}{\beta}   \Omega_{\pi_0}(\mu) 
%   $ 
%   }
  \label{eq:primal_reg}
\end{equation}
where $\Omega_{\pi_0}(\mu)$ contains an expectation under $\mu(a,s)$ as in \cref{eq:kl_def}-(\ref{eq:alpha_def}).
We can also derive a dual version of the regularized \gls{LP}, 
by first writing the Lagrangian relaxation of \cref{eq:primal_reg}
% starting from a Lagrangian relaxation of \cref{eq:primal_reg}
%\max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}}
% \begin{align}
%     %\mathcal{L}(\mu, V, \Omega) := 
%     & \min \limits_{V(s)} \max \limits_{\ontop{\normalsize \mu(s) \rightarrow \mathcal{M}}{\pi(a|s) \in \Delta^{|A|}}} \, 
%      (1-\gamma) \big\langle \nu_0, V(s) \big  \rangle \\
%      + &\blangle \mu(s)\pi(a|s), r(a,s) +  \gamma \transitionv -V(s) \big \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \nonumber \\
%     &   \label{eq:lagrangian}\, ,
% \end{align}
% \resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
% \scriptsize
\begin{align}
%   \mathcal{L}:= 
  \max \limits_{\mu(a,s)} \min \limits_{V(s), \lambdaplus}  \, 
     (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle 
     + &\langle \mu(a,s), r(a,s) + \gamma \transitionv -V(s) + \lambdaplus \rangle - \frac{1}{\beta} \Omega_{\pi_0}(\mu)  \label{eq:dual_lagrangian} 
\end{align}
\normalsize
% }}
% \resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
% \begin{align}
%   & 
% %   \mathcal{L}:= 
%   \max \limits_{\mu(a,s)} \min \limits_{V(s)}  \, 
%      (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle  \label{eq:dual_lagrangian} \\
%      + &\blangle \mu(a,s), r(a,s) +  \gamma \transitionv -V(s)\brangle - \frac{1}{\beta} \Omega_{\pi_0}(\mu)  \nonumber
% \end{align}
% }}
Swapping the order of optimization 
% using
under 
strong duality, we can recognize the 
maximization over ${\mu(a,s)}$ as a conjugate function $\frac{1}{\beta}\Omega^{*}_{\pi_0, \beta}$, as in \cref{eq:conjstar}, leading to a regularized dual optimization
% \resizebox{\columnwidth}{!}{\parbox{\columnwidth}{
 \begin{align}
 \hspace*{-.2cm} &  \obj_{\Omega, \beta}^{*}(r) = 
%  \min \limits_{V(s)} 
 \min \limits_{V(s), \lambdaplus}
 %\max \limits_{ \mu(s) \rightarrow \mathcal{M}}
 \,  (1-\gamma) \big\langle \nu_0(s), V(s) \big  \rangle  + \frac{1}{\beta}\Omega^{*}_{\pi_0, \beta} \bigg(r(a,s) +  \gamma \transitionv -V(s) + \lambdaplus \bigg)\label{eq:dual_reg} 
%  &+ \mathbb{E}_{\mu(s)} \bigg[\, \frac{1}{\beta}\Omega^{*}_{\pi_0, \beta} \bigg(r(a,s) +  \gamma \transitionv -V(s) \bigg)  \bigg] \nonumber
\end{align}
% }}
% \RB{Omit this, instead consider soft value aggregation? }
which involves optimization over dual variables $V(s)$ only and is unconstrained, in contrast to \cref{eq:dual_lp}. %, and involves sampling under the induced marginal distribution $\mu(s)$. 
% Similar dual objectives
Dual objectives of this form 
% have been considered 
appear 
in \citep{nachum2020reinforcement, belousov2019entropic, basserrano2021logistic, neu2017unified}.
\textcolor{black}{We emphasize the need to include the Lagrange multiplier $\lambdaplus$, with $\lambdaplus > 0$ when the optimal policy has $\piopt(a|s) = 0$, since an important motivation for $\alpha$-divergence regularization is to encourage sparsity in the policy (see \cref{eq:qexp}, \citet{lee2018sparse, lee2019tsallis, chow2018path}).}


\paragraph{Soft Value Aggregation}
In iterative algorithms such as (regularized) modified policy iteration \citep{puterman1978modified, scherrer15a}, it is useful to consider the \textit{regularized Bellman optimality operator} \citep{geist2019theory}.   For given estimates of the state-action value $Q(a,s) \coloneqq r(a,s) + \gamma \transitionv$, the operator $\mathcal{T}^{*}_{\Omega_{\pi_0, \beta}}$ updates $V(s)$ as
% \scriptsize
\begin{align} 
\hspace*{-.2cm} V(s)  \leftarrow \frac{1}{\beta} \Omega^{*}_{\pi_0,\beta}(Q) = \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \blangle \pi(a|s), Q(a,s) \brangle - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \label{eq:soft_value}
\end{align}
\normalsize
Note that this conjugate optimization is performed in each state $s \in \mathcal{S}$ and explicitly constrains each $\pi(a|s)$ to be normalized.
Although we proceed with the notation of \cref{eq:primal_reg} and \cref{eq:dual_reg}, our later developments 
% for conditional policy regularization 
are compatible with the
% the regularized Bellman operator or 
`soft-value aggregation' perspective above.  See \myapp{soft_value} for detailed discussion.
% We provide detailed discussion in \myapp{soft_value}.
% We provide a detailed discussion of this `soft-value aggregation' operator in \myapp{soft_value}.   While we proceed with the notation of \cref{eq:dual_reg}
% While our developments in later sections focus on
% Our developments in later sections are compatible with this approach,

%%%%%%%%%%%%%%%%%%%%%%%%%% Prev Divergence Functions Paragraph %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Divergence Functions}\label{sec:divergence_intro}
% \RB{MOVE and modify this intro to fit?}

% % The family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases, 
% We consider regularization using the family of $\alpha$-divergences \citep{amari2016information, cichocki2010families}, which includes both the forward and reverse \textsc{kl} divergences as special cases.    
% We extend these divergences to accept unnormalized density functions as input \citep{zhu1995information}, \textcolor{red}{so that Lagrangian relaxations such as \cref{eq:dual_lagrangian} are well defined even when 
% normalization constraints are not satisfied.}
% % $\mu(a,s)$ is not normalized.}
% % \textcolor{blue}{$\mu(a,s) \not \in \Delta^{|\mathcal{A}| \times |\mathcal{S}|}$.}

%  We primarily focus on policy regularization using a conditional divergence $\Omega^{(\alpha)}_{\pi_0}(\mu)$ to a reference policy $\pi_0(a|s)$.
% % but we also discuss regularization of the joint state-action occupancy to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$, in \textcolor{blue}{in \mysec{?}}.   
% Note that we consider the regularizer to be a function of $\mu(a,s)$, since it is applied 
% % in 
% across
% each 
% % $s \in \mathcal{S}$ 
% state
% % $s \sim \mu_\pi(s)$
% % \textcolor{red}{$s \sim \mu_\pi(s)$} 
% visited by the agent.
% \textcolor{blue}{In \mysec{?}}, we also discuss regularizing the joint state-action occupancy to be close to a reference $\mu_0(a,s)$, using the notation $\Omega^{(\alpha)}_{\mu_0}(\mu)$. 
% % \citep{nachum2020reinforcement, husain2021regularized, basserrano2021logistic}.

% \RB{Need 2nd paragraph??  Smoother intro?}

% \RB{Remove all $\mu(s)$ below?}
% % \RB{REMOVE ALL THE $\mu(s)$ in Divergence derivations?}

% \paragraph{KL Divergence}
% % Taking the limit as $\alpha \rightarrow 1$, we obtain
% % an (extended version of) 
% The forward \textsc{kl} divergence is commonly used for policy regularization in \gls{RL}.  Extending to unnormalized measures 
% \citep{zhu1995information},
% % \citep{cichocki2010families}, 
% %  (\citet{tishby2011information, ortega2013thermodynamics, fox2016taming})
% \footnotesize
% \begin{align}
%         &\Omega_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\bigg[D_{KL}[\tpi:\tpi_0]\bigg] \label{eq:kl_def} \\
%         &\phantom{\Omega} = \sum \limits_{s \in \mathcal{S}} \mu(s) \sum \limits_{a \in \mathcal{A}}  \left(\tpi(a|s)  \log \frac{\tpi(a|s)}{\tpi_0(a|s)} -  
%         % \sum \limits_{a, s} 
%       \tpi(a|s) 
%         + 
%         % \sum \limits_{a,s} 
%       \tpi_0(a|s)\right). \nonumber
% \end{align}
% % \begin{align}
% %     % \hspace*{-.15cm} D_{KL}[\tpi:\tpi_0] = \sum \limits_{a \in \mathcal{A}} \tpi(a|s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} - \tpi(a|s) + \tpi_0(a|s) \, . \nonumber
% %         % \hspace*{-.2cm}  
% %         \Omega&_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\bigg[D_{KL}[\tpi:\tpi_0]\bigg] \label{eq:kl_def} \\
% %         &= \sum \limits_{a, s} \mu(a,s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} -  
% %         % \sum \limits_{a, s} 
% %         \mu(s) \tpi(a|s) 
% %         + 
% %         % \sum \limits_{a,s} 
% %         \mu(s) \tpi_0(a|s)
% %       . \nonumber
% %         % \sum \limits_{a, s} \mu(a,s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
% %         % \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
% %         % \textcolor{red}{ -\sum \limits_{a \in \mathcal{A}} \tpi(a|s) +\sum \limits_{a \in \mathcal{A}} \tpi_0(a|s) } 
% %     %\sum \limits_{a \in \mathcal{A}} %\lim_{\alpha \rightarrow 1}
% % \end{align}
% \normalsize
% Up to an additive constant, we recover the Shannon entropy using a uniform reference, $\pi_0(a|s) = 1$ $\forall 
% \, (a,s).$ 
% % \in \mathcal{A} \times \mathcal{S}$.
% % \, a \in \mathcal{A}, s \in \mathcal{S}$. 
% % the final terms cancel if both $\tpi$ and $\tpi_0$ are normalized.


% \paragraph{$\alpha$-Divergence} The $\alpha$-divergence $\mathbb{E}_{\mu(s)}\big[D_{\alpha}[\tpi_0:\tpi]\big]$ over possibly unnormalized measures
% %$\omegamu &= \mathbb{E}_{\mu(s)}\big[D_{\alpha}[\tpi_0:\tpi]\big]$, 
% is defined as 
% \footnotesize
% \begin{align}
% \hspace*{-.1cm} 
% \Omega^{(\alpha)}_{\pi_0}(\mu)&=
% % \mathbb{E}_{\mu(s)}\big[
% % D_{\alpha}[\tpi_0:\tpi]
% % \big]
% % &= 
% \frac{1}{\alpha(1-\alpha)} 
% % \sum \limits_{s \in \mathcal{S}}
% \sum \limits_{s \in \mathcal{S}}
% \mu(s)
%     \bigg( (1-\alpha) 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a \in \mathcal{A}}
%     \tpi_0(a|s) 
%     %+\alpha 
%     \\ &\phantom{\sum \limits_{s \in \mathcal{S}}
% \mu(s)} + \alpha 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a \in \mathcal{A}}
%     \tpi(a|s) \nonumber 
%     % &- \sum \limits_{a \in \mathcal{A}} 
%     % \\ &\phantom{\sum \limits_{s} \mu(s)} 
%     - \sum \limits_{a \in \mathcal{A}} 
%     \tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} \bigg)  \label{eq:alpha_def}
% \end{align}
% \normalsize
% To provide intuition for 
% % for?  contextualize?  understand?}
% the $\alpha$-divergence, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential, with
% \begin{align}
%     \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , \\
%     \exp_{\alpha}(u) &= [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, .
%     % \hfill \, \,  \alpha \neq 1 \
% \end{align}
% % Using $\log_{\alpha}$, 
% Using the $\alpha$-logarithm, we can rewrite the $\alpha$-divergence 
% % in a form similar to 
% similarly to
% the \kl divergence in 
% \cref{eq:kl_def}.
% \scriptsize
% \begin{align}
%   \Omega^{(\alpha)}_{\pi_0}(\mu) &= \frac{1}{\alpha} \sum \limits_{s \in \mathcal{S}} \mu(s) \bigg( \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)} - \pi(a|s) + \pi_0(a|s) \bigg) \nonumber
% \end{align}
% \normalsize
% For a uniform reference, the $\alpha$-divergence 
% differs from the Tsallis entropy by only the $1/\alpha$ factor and an additive constant (see \myapp{tsallis}).


% \RB{Bridge}





%%%%%%%%%%%%%%%%%%%%%%%%%% END OF Prev Divergence Functions Paragraph %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





% As discussed in \myapp{tsallis}, the $\alpha$-divergence is closely related to the Tsallis entropy. \RB{Introduce $\log_{\alpha}$ first? (with the goal of reaching this insight)}
% \citep{lee2019tsallis}, as we discuss in detail in \myapp{tsallis}.  
% To see this, 

% For later convenience, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential,
% % \small
% % \begin{align}
% %     \log_{\alpha}(u) &= \begin{cases} \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \hfill \, \, \alpha \neq 1 \\
% %     \log(u) \hfill \, \, \alpha =1 \end{cases} \\
% %     \exp_{\alpha}(u) &= \begin{cases} [1 + (\alpha-1) \cdot u ]_+^{\frac{1}{\alpha-1}} \hfill \, \,  \alpha \neq 1 \\
% %     \exp(u) \hfill \, \, \alpha =1 \end{cases} \, .
% % \end{align}
% \begin{align}
%     \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , \\
%     \exp_{\alpha}(u) &= [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, .
%     % \hfill \, \,  \alpha \neq 1 \
% \end{align}
% \begin{equation}
% \resizebox{.87\columnwidth}{!}{\hspace*{-.36cm}
%     $\log_{\alpha}(u) &= \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \\
%     \quad 
%     \exp_{\alpha}(u) = [1 + (\alpha-1) u ]_+^{\frac{1}{\alpha-1}}$
% }
% \end{equation}
% \normalsize
% and we recover the natural logarithm and exponential in the limit as $\alpha \rightarrow 1$.


% \textcolor{blue}{
% We consider regularization of the policy $\pi(a|s)$ to a reference $\pi_0(a|s)$, with analogous derivations for  regularization of $\mu(a,s)$ to a reference $\mu_0(a,s)$ in \myapp{mu_results}.}
% \RB{Decide how to handle $\mu$ vs. $\pi$ regularization.  Difference is insightful for $\alpha$-divergence}

% \paragraph{KL Divergence}
% % Taking the limit as $\alpha \rightarrow 1$, we obtain
% % an (extended version of) 
% The forward \textsc{kl} divergence commonly used as regularization in \gls{RL} is defined as
% %  (\citet{tishby2011information, ortega2013thermodynamics, fox2016taming})
% \footnotesize
% \begin{align}
%     % \hspace*{-.15cm} D_{KL}[\tpi:\tpi_0] = \sum \limits_{a \in \mathcal{A}} \tpi(a|s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} - \tpi(a|s) + \tpi_0(a|s) \, . \nonumber
%         % \hspace*{-.2cm}  
%         \Omega&_{\pi_0}(\mu) = \mathbb{E}_{\mu(s)}\bigg[D_{KL}[\tpi:\tpi_0]\bigg] \label{eq:kl_def} \\
%         &= \sum \limits_{a, s} \mu(a,s) \log \frac{\tpi(a|s)}{\tpi_0(a|s)} -  
%         % \sum \limits_{a, s} 
%         \mu(s) \tpi(a|s) 
%         + 
%         % \sum \limits_{a,s} 
%         \mu(s) \tpi_0(a|s)
%       . \nonumber
%         % \sum \limits_{a, s} \mu(a,s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
%         % \sum \limits_{a \in \mathcal{A}} \pi(a|s) \log \frac{\pi(a|s)}{\pi_0(a|s)} 
%         % \textcolor{red}{ -\sum \limits_{a \in \mathcal{A}} \tpi(a|s) +\sum \limits_{a \in \mathcal{A}} \tpi_0(a|s) } 
%     %\sum \limits_{a \in \mathcal{A}} %\lim_{\alpha \rightarrow 1}
% \end{align}
% \normalsize
% \RB{$\tpi$ or $\pi$?}
% To derive a closed form for the convex conjugate function, we consider the conditional \kl divergence as a function of $\mu(a,s)$ in the following conjugate optimization
% \footnotesize
% \begin{align}
%   \hspace*{-.25cm}  &\klconjpii(\dualvar) = \max \limits_{\mu(a,s)} \blangle 
%     \mu(a,s), \dualvar(a,s)
%     % \mu(a,s), \dualvar(a,s)
%     \brangle - \klomegamu \label{eq:kl_conj} \\
%   &= \frac{1}{\beta} \sum \limits_s \mu(s) 
%   \left(
%   \sum \limits_{a} \pi_0(a|s) \expof{\beta \cdot \dualvar(a,s)} - \sum \limits_{a} \pi_0(a|s) 
%   \right)
%   \nonumber
% %   &= \frac{1}{\beta} \log \sum \limits_{a,s} \mu(s) \pi_0(a|s) \expof{\beta \cdot \dualvar(a,s)}
%     % - \blangle \lambda , \mu(a,s) - 1\brangle
% \end{align}
% \normalsize
% where the \textcolor{red}{optimizing argument is 
% the occupancy measure
% induced by } $\pir(a|s) = \pi_0(a|s)\exp\{\beta \cdot \dualvar(a,s)\} $.
% See \myapp{kl_conj_all} for detailed derivations.  Note that the log-sum-exp form of the conjugate function arises from enforcing a normalization constraint on the optimization variable \citep{ruderman2012tighter}.   
% % $\mu(a,s) \in \Delta^{\mathcal{A} \times \mathcal{S}}$.

% % Finally, note that the optimizing argument for the conjugate in \cref{eq:kl_conj} is given by 
% % \begin{align}
% %     \piopt(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( \dualvar(a,s) \big) } 
% % \end{align}
% % where $\muopt(a,s) = \muopt(s) \piopt(a|s)$ is induced from $\piopt(a|s)$.

% % With detailed derivations in \myapp{kl_conj_all}, the solution to the conjugate optimization is
% % Considering this conditional \kl divergence as a function of $\mu(a,s)$ and enforcing normalization, we obtain the following conjugate optimization.   With detailed derivations in \myapp{kl_conj_all}, 

% % normalized mu conjugate with log-sum-exp solution
% % \footnotesize
% % \begin{align}
% %   \hspace*{-.25cm}   \klconjpii(\dualvar) &= \max \limits_{\mu(a,s) \in \Delta^{|\mathcal{A}| \times |\mathcal{S}|}} \blangle 
% %     \mu, \dualvar 
% %     % \mu(a,s), \dualvar(a,s)
% %     \brangle - \klomegamu \\
% %   &= \frac{1}{\beta} \log \sum \limits_{a,s} \mu(s) \pi_0(a|s) \expof{\beta \cdot \dualvar(a,s)}
% %     % - \blangle \lambda , \mu(a,s) - 1\brangle
% % \end{align}
% % \normalsize

% % \RB{Emphasize derivation of $\pi_* = \nabla \Omega^{*}(Q)$}
% % The value function, or conjugate $\alphaconjn(Q)$, as a function $Q$ and with restriction to normalized $\pi$, is

% %For the \textsc{kl} divergence, 
% % This matches the normalization constant for the optimal policy, with $V_*(s) = \psi(s;\beta)$ and
% %  \begin{align}
% %  \pi_*(a|s) = \pi_0(a|s) \expof{\beta \cdot \big( Q(a,s) -  \psi(s;\beta)\big)} \, ,\label{eq:kl_opt_policy}
% %  \end{align}
% % This can also be seen by plugging $\alpha = 1$ into \cref{eq:alpha_conj_norm_main}.
% % Apart from the case of $\alpha=1$, we can see from \cref{eq:alpha_conj_norm_main} that $V_*(s) \neq \normalizeralpha$.
% % We discuss the relationship between $V_*(s)$ and $\normalizeralpha$ for general $\alpha$ in more detail in \mysec{optimal_policy}, while the optimal policy expressions in \cref{eq:alpha_opt_policy} and (\ref{eq:kl_opt_policy}) will also play a central role.


% \paragraph{$\alpha$-Divergence} The $\alpha$-divergence over possibly unnormalized measures,  $\omegamu &=
% \mathbb{E}_{\mu(s)}\big[
% D_{\alpha}[\tpi_0:\tpi]
% \big]$, is defined as 
% \footnotesize
% \begin{align}
% \hspace*{-.15cm} 
% \omegamu &=
% % \mathbb{E}_{\mu(s)}\big[
% % D_{\alpha}[\tpi_0:\tpi]
% % \big]
% % &= 
% \frac{1}{\alpha(1-\alpha)} 
% % \sum \limits_{s \in \mathcal{S}}
% \sum \limits_{s}
% \mu(s)
%     \bigg( (1-\alpha) 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a} 
%     \tpi_0(a|s) 
%     %+\alpha 
%     \\ \phantom{\sum \limits_{s}
% \mu(s)} + \alpha 
%     % \sum \limits_{a \in \mathcal{A}} 
%     \sum \limits_{a} 
%     \tpi(a|s) \nonumber 
%     % &- \sum \limits_{a \in \mathcal{A}} 
%     % \\ &\phantom{\sum \limits_{s} \mu(s)} 
%     - \sum \limits_{a} 
%     \tpi_0(a|s)^{1-\alpha} \tpi(a|s)^{\alpha} \bigg)  \label{eq:alpha_def}
% \end{align}
% \normalsize
% with the forward \kl divergence $D_{KL}[\tpi:\tpi_0]$ in \cref{eq:kl_def}
% % in \cref{eq:kl_def}
% % , \textcolor{red}{extended to take unnormalized densities as input, }
% recovered in the limit as $\alpha \rightarrow 1$.  
% As discussed in \myapp{tsallis}, the $\alpha$-divergence is closely related to the Tsallis entropy. \RB{Introduce $\log_{\alpha}$ first? (with the goal of reaching this insight)}
% % \citep{lee2019tsallis}, as we discuss in detail in \myapp{tsallis}.  
% % To see this, 

% For later convenience, we define the deformed $\alpha$-logarithm as in \citet{lee2019tsallis}, which matches Tsallis's $q$-logarithm \citep{tsallis2009introduction} for $\alpha = 2-q$.  Its inverse is the $\alpha$-exponential,
% % \small
% % \begin{align}
% %     \log_{\alpha}(u) &= \begin{cases} \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \hfill \, \, \alpha \neq 1 \\
% %     \log(u) \hfill \, \, \alpha =1 \end{cases} \\
% %     \exp_{\alpha}(u) &= \begin{cases} [1 + (\alpha-1) \cdot u ]_+^{\frac{1}{\alpha-1}} \hfill \, \,  \alpha \neq 1 \\
% %     \exp(u) \hfill \, \, \alpha =1 \end{cases} \, .
% % \end{align}
% \begin{align}
%     \log_{\alpha}(u) &=  \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \, , \\
%     \exp_{\alpha}(u) &= [1 + (\alpha-1) \, u ]_+^{\frac{1}{\alpha-1}} \, .
%     % \hfill \, \,  \alpha \neq 1 \
% \end{align}
% % \begin{equation}
% % \resizebox{.87\columnwidth}{!}{\hspace*{-.36cm}
% %     $\log_{\alpha}(u) &= \frac{1}{\alpha-1} \left( u^{\alpha-1}-1 \right) \\
% %     \quad 
% %     \exp_{\alpha}(u) = [1 + (\alpha-1) u ]_+^{\frac{1}{\alpha-1}}$
% % }
% % \end{equation}
% % \normalsize
% and we recover the natural logarithm and exponential in the limit as $\alpha \rightarrow 1$.

% With detailed derivations in \myapp{alpha_conj_norm}, the conjugate function for conditional divergence regularization takes the form
% \footnotesize
% \begin{align}
%      \hspace*{-.2cm} &\alphaconj(\dualvar) = \max \limits_{\mu(a,s)} \blangle \mu(a|s), \dualvar(a,s) \brangle -  \omegamu \label{eq:alpha_conj_norm_main} \\
%     &\phantom{=}= \frac{\alpha-1}{\alpha} \blangle \mu(s) \pi_{\dualvar}(a|s), \dualvar(a,s) \brangle + \frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi_{\dualvar}] \nonumber
% %   \frac{1}{\alpha}  \normalizeralpha 
%     % \label{eq:alpha_conj_norm_main}
% \end{align}
% \normalsize
% As we discuss in \mysec{adversarial_perturb} or \myapp{alpha_conj_norm}, the final term $\frac{1}{\beta}(1-\alpha) D_{\alpha}[\pi_0:\pi_{\dualvar}]$ 
% % plays the role of the normalization constant for 
% normalizes
% the policy in the optimizing argument $\pi_{\dualvar}(a|s) = \mu_{\dualvar}(a,s)/ \mu(s)$.   In particular, the policy has the form
% \footnotesize
% \begin{align}
%     \pi_{\dualvar}(a|s) = \pi_0(a|s) \exp_{\alpha} \big\{\beta \cdot \big( \dualvar(a,s) - \frac{1}{\beta}(1-\alpha)D_{\alpha}[\pi_0:\pi_{\dualvar}] \big)  \big\}
% \end{align}
% \normalsize
% \textcolor{blue}{wrap up / transition sentence}

% \RB{Introduce notation for normalizer / $D_{\alpha}$?}
% \RB{Inspect.  Reference App. and \textbf{optimal policy expression}}


==> sections/new/2b_generalization.tex <==
% \section{Relationship with Generalization}\label{sec:feasible}\label{sec:generalization}
\headerv
\section{Visualizing the Feasible Set}\label{sec:feasible}\label{sec:generalization}
\headerv
% \subsection{Feasible Set}\label{sec:feasible}
% \TG{I like this section. Maybe worth spending one, two sentences re-iterating that we have established the adversarial interpretation, but we also know that the adversary is limited. The most important missing bit then is: the characterization of the adversary via this limitedness (the feasible set), which we're going to show now.}
% \RB{Although the feasible set is general (any $\pi$), the plot is for the case of an optimal policy and is identical to the setting of \citet{eysenbach2021maximum} referenced previously}
In the previous section, we have established an adversarial interpretation which suggests that regularized policies are robust to worst-case reward perturbations.   However, we have not discussed implications for zero-shot generalization or understood the limitations of this adversary.
% robustness to worst-case reward perturbations 
% The adversarial interpretation in  suggests that regularized policies are robust to worst-case reward perturbations.   
 In particular, it is not clear how the cost function $\alphaconjmu(\pr)$ in \cref{eq:pedro_form} restricts the feasible set $\mathcal{R}$ of perturbations from which the adversary can select.  
 We characterize the feasible set in the following proposition, with visualizations in \cref{fig:feasible_set_main}.
%  In the following proposition, we provide a simple constraint to characterize the feasible set, with visualizations in \cref{fig:feasible_set_main}.
%  The optimal $\propt$ in \myprop{optimal_perturbations} suggest a simple constraint to characterize the feasible set in the following proposition.
\begin{restatable}[]{proposition}{feasible}\label{prop:feasible} For a given policy $\pi(a|s)$ and any $\alpha$-divergence, the feasible set of reward perturbations available to the adversary is defined by the constraint
\begin{align}
\alphaconjmu(\pr) \leq 0 \label{eq:alpha_feasible} 
% \\\frac{\alpha-1}{\alpha} \langle \mu(s) \pi^{(\pr)}_*(a|s), \pr \rangle - \frac{1}{\alpha}(V^{\pr}_*(s)  \leq 0 \label{eq:alpha_feasible}
\end{align}
For \textsc{kl} divergence regularization, we obtain
% this translates to
\begin{align}
   \sum\limits_{a \in \mathcal{A}} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} \leq 1 \, . \label{eq:kl_feasible}
\end{align}
\end{restatable}
\begin{proof} See \myapp{feasible_pf} for proof. 
\textcolor{red}{which proceeds by evaluating the conjugate function at the worst-case $\propt$, with $\alphaconjn(\propt)=0 \, \forall \alpha$.  
% Since $\alphaconjn(\pr)$ is increasing in $\pr$ and the $-\pr(a,s)$ term in \cref{eq:pedro_form} is decreasing, the constraint follows.
The constraint for the minimization problem in \cref{eq:pedro_form} then follows from the fact that $\alphaconjn(\pr)$ is increasing in $\pr$. \RB{\textbf{no longer holds}: alternative proof given in the appendix}}
% \RB{improve}
\end{proof}
The above constraints characterize the robust set of modified reward functions for which we can provide performance guarantees.
% , given a particular stochastic policy and regularized objective.
% for a particular stochastic policy and regularized objective.
More precisely, for given \gls{MDP} transition dynamics, we say that a policy trained with reward $r(a,s)$ and 
% and regularization based on $\Omega, \pi_0, $  
regularized objective $\obj_{\Omega,\beta}(r)$ 
\textit{generalizes} to an environment with a modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$ if 
% , as in \cref{eq:reward_perturbation_stmt},
\small
\begin{align}
  \hspace*{-.2cm} 
%   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) \rangle - \omegamu \, . \label{eq:robust_def} \\
  \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) \rangle - \omegamu \, . \label{eq:robust_def}
%   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(s)\pi(a|s), r(a,s) - \ptReg(\pi) \rangle \\
%   \langle \mu(a,s), \mr(a,s) \rangle &\geq \obj_{\Omega, \beta}(r) = \alphaconjmu \\
%   \alphaconjmu \text{vs.} \alphaconjmuu \\
%   \alphaconjn \text{vs.} \alphaconjnn \\
%   \langle \mu(a,s), \mr(a,s) \rangle &\geq \langle \mu(s), V_*(s; \beta) \rangle = \langle \mu(s),\alphaconjn \rangle \\
%   \obj_{\Omega, \beta}(r)  = \alphaconjmu &= \frac{\alpha-1}{\alpha} \langle \mu(s), \alphaconjn \rangle 
%   \langle \mu(a,s), r(a,s) - \pr(a,s) \rangle &\geq \langle \mu(a,s), r(a,s) - \ptReg(\pi) \rangle  %\blangle \mu(s) \pi(a|s), \mr(a,s) \brangle \geq  \blangle \mu(s) \pi(a|s), r(a,s) - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \brangle \, . \label{eq:robust_def}
\end{align}
\normalsize
% \JG{Ok, I think you need to say a couple of sentences here. I was initially confused by this thinking that it was trivial but it is not at all. I think one expects something of the form: $ \langle \mu(a,s), r(s,a) + \Delta r(s,a) \rangle \geq \langle \mu(a,s), r(a,s) \rangle $ for $\Delta r(s,a) \in Z$ where $r(s,a) + \Delta r(s,a) = r'(s,a)$ and $Z$ is the set of allowed perturbations. In its current form with the regularizer it is not clear what this implies for generalization right?. Sorry if this question is too complicated, It could also be that I need more time to understand this. I think its important to get the explanation right though.} 
In other words, the expected reward using the modified $\mr(a,s)$ is greater than or equal to the value of the regularized objective $\obj_{\Omega,\beta}(r)$ using the original $r(a,s)$. 
%  on the left side on the right side.  
Note that \cref{eq:robust_def} holds with equality for the worst-case modified reward $\mropt(a,s)$ (\mysec{optimal_perturb} or \myapp{preserve}). 
\textcolor{red}{The feasible set in \myfig{feasible_set_main} shows other rewards for which the inequality holds, with equality 
% holding 
at the boundary.} \RB{Is this true?  Otherwise, why would we pick out the particular $\Delta r^{*}$ that we do?  Further, the original $r(a,s)$ is at the boundary, and this does not hold with equality.}
% While it is clear that increasing the reward in both actions preserves the inequality in \cref{eq:robust_def},  
% % is feasible for an adversary that minimizes \cref{eq:pedro_form}, 
% \cref{fig:feasible_set_main} also includes regions where one reward decreases.

% while the feasible set in \myfig{feasible_set_main} shows the other rewards for which the inequality holds. \TG{Shall we mention that the boundary of the feasible set corresponds to the equality?}

It is in this particular sense that we can claim zero-shot generalization for a regularized policy.
We also notice that this form of robustness is sensitive to the value of the regularized objective function in \cref{eq:robust_def}, which we discuss in further detail in \mysec{entropy_vs_div}.
% Note that the expected reward under the worst-case modified reward $\mropt(a,s)$ matches the value of the regularized objective, as we have reasoned in \mysec{optimal_perturb} or \myapp{preserve}, while the feasible set in \myfig{feasible_set_main} shows the other rewards for which \cref{eq:robust_def} holds.
% Note that the right hand side corresponds to the full objective function, including regularization, whereas the left hand side is only the expected reward.  
% .regularization, as we further discuss in \mysec{entropy_vs_div}.
% the other reward functions for a stochastic policy is robust 
% The feasible set characterizes the other reward functions for which a stochastic policy achieves an expected reward greater than or equal to the value of the regularized objective. \TG{This is very important (for the reader) - make sure to emphasize the ``robustness'' and generalization-guarantee (in terms of performance) we get exactly from this fact.}
% to which a stochastic policy is robust.

\headerv
\paragraph{Visualizing the Feasible Set} 
In \myfig{feasible_set_main}, we visualize the feasible set of perturbed rewards in a two-dimensional action space for the \KL or $\alpha$-divergence, various $\beta$, and a uniform or non-uniform prior policy $\pi_0$.
\textcolor{red}{Since the optimal policy can be calculated easily in the single-step case}, we consider fixed $Q(a,s) = r(a,s) = \{1.1, 0.8\}$ and show the robustness of the optimal $\pi_*(a|s)$, which differs based on the regularization scheme (see \cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).
We determine the feasible set of $\pr$ using the constraint in \myprop{feasible} (see \myapp{feasible_plot} for details), and plot the modified reward $r\tick(a,s) = Q(a,s) - \pr(a,s)$ for each action.  
%  For clarify of exposition, we focus on the \KL divergence constraint in \cref{eq:kl_feasible}.

Inspecting the constraint for the adversary in \cref{eq:kl_feasible}, note that both reward increases $\pr(a,s) < 0$ and reward decreases $\pr(a,s) > 0$ contribute non-negative terms at each action, which either up- or down-weight the reference policy $\pi_0(a|s)$.  The constraint on their summation forces the adversary to trade off between perturbations of different actions in a particular state.   
Further, since the constraints in \myprop{feasible} integrate over the action space, the rewards for \textit{all} actions in a particular state must be perturbed together.  
While it is clear that increasing the reward in both actions preserves the inequality in \cref{eq:robust_def},  
% is feasible for an adversary that minimizes \cref{eq:pedro_form}, 
\cref{fig:feasible_set_main} also includes regions where one reward decreases.
% While it is natural that increasing the reward in both actions is feasible for an adversary that minimizes \cref{eq:pedro_form}, \cref{fig:feasible_set_main} also includes regions where one reward decreases.
% In all cases, it is natural that increasing the reward in both actions is feasible for an adversary seeking to minimize the objective in \cref{eq:pedro_form}.

For high regularization strength ($\beta=0.1$), we observe that the boundary of the feasible set is nearly linear, with the slope $-\frac{\pi_0(a_1|s)}{\pi_0(a_2|s)}$ based on the ratio of each action in the prior.  The boundary steepens for lower regularization strength.  \textcolor{red}{We can use the indifference condition to provide further geometric insight.   First, drawing a line from the origin with slope $1$ will intersect the feasible set at the worst-case modified reward (red star) in each panel, with $\mropt(a_1,s) = \mropt(a_2,s)$.  At this point, the slope of the tangent line yields the ratio of action probabilities, as we saw for the $\beta = 0.1$ case.  With decreasing regularization as $\beta \rightarrow \infty$, the slope approaches $0$ or $-\infty$ for a nearly deterministic policy and a rectangular feasible region.} \RB{Where does InDifference go?}
% ince we have plotted the optimal policy $\piopt(a|s)$ corresponding to the reward function $r(a,s)$, we can see that the indifference condition holds, with $\mropt(a_1,s) = \mropt(a_2,s)$ for the red star in each panel.   In this case, we ca  

Finally, we show the feasible set for the $\alpha$-divergence with $\alpha \in \{-1, 3\}$ and $\beta = 10$ in \cref{fig:feasible_set_main} (d)-(e) and (i)-(j), with further visualizations in \myapp{additional_feasible}.   Compared with the \textsc{kl} divergence,
we observe a wider feasible set boundary for $\alpha =-1$, whereas $\alpha = 3$ \textcolor{red}{}
% induces a steeper boundary with smaller worst-case perturbations. 
% \RB{Update the discussion here to reflect modified plots}
% for the $\alpha = 3$ case, corresponding to a steeper boundary of the feasible set.   
% \ref{fig:tabd}-\ref{fig:tabe} and \ref{fig:tabi}-\ref{fig:tabj} .  
% For the optimal policy associated with a given reward function,  we see that the $\alpha = -1$ feasible set may not include this reward function.  
% \input{sections/single_step_fig}
%%%%%%%%%%%%%%%%%%%%% PRE-move to "GENERALIZATION" Section %%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Feasible Set}\label{sec:feasible}
% % \TG{I like this section. Maybe worth spending one, two sentences re-iterating that we have established the adversarial interpretation, but we also know that the adversary is limited. The most important missing bit then is: the characterization of the adversary via this limitedness (the feasible set), which we're going to show now.}
% % \RB{Although the feasible set is general (any $\pi$), the plot is for the case of an optimal policy and is identical to the setting of \citet{eysenbach2021maximum} referenced previously}

% The adversarial interpretation in \cref{eq:pedro_form} suggests that regularized policies are robust to worst-case reward perturbations.   However, it is not clear how the cost function $\alphaconjn(\pr)$ restricts the set of perturbations available to the adversary.
%  In particular, it is not clear how the cost function $\alphaconjn(\pr)$ in \cref{eq:pedro_form} restricts the set of perturbations available to the adversary.
%  The optimal $\propt$ in \myprop{optimal_perturbations} suggest a simple constraint to characterize the feasible set in the following proposition.
% \begin{restatable}[]{proposition}{feasible}\label{prop:feasible} For a given policy $\pi(a|s)$ and any $\alpha$-divergence, the feasible set of reward perturbations is defined by the constraint
% \begin{align}
% \alphaconjn(\pr) \leq 0 \label{eq:alpha_feasible}
% \end{align}
% For \textsc{kl} divergence regularization, this translates to
% \begin{align}
%   \sum\limits_{a \in \mathcal{A}} \pi_0(a|s) \expof{\beta \cdot \pr(a,s)} \leq 1 \, . \label{eq:kl_feasible}
% \end{align}
% \end{restatable}
% \begin{proof} See \myapp{feasible_pf} for proof, which proceeds by evaluating the conjugate function at the optimal $\propt$, with $\alphaconjn(\propt)=0 \, \forall \alpha$.  
% % Since $\alphaconjn(\pr)$ is increasing in $\pr$ and the $-\pr(a,s)$ term in \cref{eq:pedro_form} is decreasing, the constraint follows.
% The constraint for the minimization problem in \cref{eq:pedro_form} then follows from the fact that $\alphaconjn(\pr)$ is increasing in $\pr$.\RB{improve}
% \end{proof}
% \vspace*{-.1cm}

% These constraints precisely characterize the robust set of modified reward functions, for which we can guarantee zero-shot generalization of a particular stochastic policy and regularized objective.\TG{This is very important (for the reader)}
% % the other reward functions for a stochastic policy is robust 
% % The feasible set characterizes the other reward functions for which a stochastic policy achieves an expected reward greater than or equal to the value of the regularized objective. \TG{This is very important (for the reader) - make sure to emphasize the ``robustness'' and generalization-guarantee (in terms of performance) we get exactly from this fact.}
% % to which a stochastic policy is robust.
% In \myfig{feasible_set_main}, we visualize the feasible set of perturbed rewards in a two-dimensional action space for the \KL or $\alpha$-divergence, various $\beta$, and uniform or non-uniform prior policy $\pi_0$.
% Since the optimal policy can be calculated easily in the single-step case, we consider $\pi_*(a|s)$ corresponding to fixed $Q(a,s) = r(a,s) = \{1.1, 0.8\}$, which differ based on the regularization scheme (see \cref{eq:alpha_opt_policy}, (\ref{eq:kl_opt_policy})).
% We determine the feasible set of $\pr$ according to the constraint in \myprop{feasible} (see \myapp{feasible_plot} for details), and plot the modified reward $r\tick(a,s) = Q(a,s) - \pr(a,s)$ for 
%  each action.  
% %  For clarify of exposition, we focus on the \KL divergence constraint in \cref{eq:kl_feasible}.

% Inspecting the constraints for the adversary in \cref{eq:kl_feasible}, note that both reward increases $\pr(a,s) > 0$ and reward decreases $\pr(a,s) < 0$ contribute non-negative terms at each action, which either up- or down-weight the reference policy $\pi_0(a|s)$.  The constraint on their summation forces the adversary to trade off between perturbations of different actions in a particular state.   In all cases, it is natural that increasing the reward in both actions is feasible for an adversary seeking to minimize the objective in \cref{eq:pedro_form}.

% For high regularization strength ($\beta=0.1$), we observe that the boundary of the feasible set is nearly linear, with the slope $-\frac{\pi_0(a_2|s)}{\pi_0(a_1|s)}$ based on the ratio of each action in the prior.  The boundary steepens for lower regularization strength.  However, since we have expanded the optimal policy $\piopt(a|s)$ for the reward $r(a,s)$, we can use the indifference condition provide further geometric insight.   First, drawing a line from the origin with slope $1$ will intersect the feasible set at the worst-case modified reward (red star) in each panel, with $\mropt(a_1,s) = \mropt(a_2,s)$.  At this point, the slope of the tangent line yields the ratio of action probabilities, as we saw for the $\beta = 0.1$ case.  With decreasing regularization as $\beta \rightarrow \infty$, the slope approaches $0$ or $\infty$, with a deterministic policy and rectangular feasible region.
% % ince we have plotted the optimal policy $\piopt(a|s)$ corresponding to the reward function $r(a,s)$, we can see that the indifference condition holds, with $\mropt(a_1,s) = \mropt(a_2,s)$ for the red star in each panel.   In this case, we ca  

% Finally, we show the feasible set for the $\alpha$-divergence with $\alpha \in \{-1, 3\}$ and $\beta = 10$ in \cref{fig:feasible_set_main} (d)-(e) and (i)-(j), with further visualizations in \cref{app:additional_feasible}.   Compared with the \textsc{kl} divergence,
% we observe a wider boundary of the feasible set for $\alpha =-1$, whereas $\alpha = 3$ induces a steeper boundary with smaller worst-case reward perturbations.
% % for the $\alpha = 3$ case, corresponding to a steeper boundary of the feasible set.   
% % \ref{fig:tabd}-\ref{fig:tabe} and \ref{fig:tabi}-\ref{fig:tabj} .  
% % For the optimal policy associated with a given reward function,  we see that the $\alpha = -1$ feasible set may not include this reward function.  

==> sections/new/3_entropy_reg.tex <==
% \section{Discussion}\label{sec:discussion}
% \vspace*{\header}
% % What insights \TG{What are the main insights (sounds less defensive) :))))} 
% What are the main insights that can be obtained from this adversarial interpretation of regularized policies?
% In \mysec{generalization}, we discuss the generalization properties associated with this robustness, which we highlight is particularly sensitive to the form of the objective in \mysec{entropy_vs_div}.  We highlight an additional connection with the notion of path consistency \citep{nachum2017bridging, chow2018path} in \mysec{path}.
% % For the optimal policy, we show that our interpretation is compatible with the modified reward interpretation of \citet{husain2021regularized} in \ref{sec:husain}.  This directly leads to connections with the notion of path consistency \citep{nachum2017bridging, chow2018path} in \ref{sec:path} and the game-theoretic interpretation of \citet{ortega2014adversarial} in \ref{sec:indifference}. 
% % \RB{seems long, is this all necessary?}
% % We
% % connections with the notion of path consistency \citep{nachum2017bridging, chow2018path} in \ref{sec:modified} and , and argue that  adversarial reward perturbations can provides a natural justification for including $Q$-values as dual variables in \gls{LP} formulations of \gls{MDP}s in \ref{sec:qlp}.
% %\RB{Add generalization analysis}
% %\RB{Add reward $\rightarrow$ robustness vs. policy $\rightarrow$ robustness}

% \subsection{Relationship to Generalization}\label{sec:generalization}
% %For our purposes, we consider `zero-shot generalization' of a given policy $\pi(a|s)$ to an environment with a modified reward function $\mr(a,s)$ to mean that
% Our adversarial interpretations imply robustness or generalization of a given policy $\pi(a|s)$ to an environment with a modified reward $\mr(a,s)$ in the sense that, for given \gls{MDP} transition dynamics
% \small
% \begin{align}
%   \hspace*{-.2cm} \langle \mu(a,s), \mr(a,s) \rangle \geq \langle \mu(a,s), r(a,s) \rangle - \omegamu \, \label{eq:robust_def}
%   %\blangle \mu(s) \pi(a|s), \mr(a,s) \brangle \geq  \blangle \mu(s) \pi(a|s), r(a,s) - \frac{1}{\beta} \Omega_{\pi_0}(\pi) \brangle \, . \label{eq:robust_def}
% \end{align}
% \normalsize
% %Our adversarial interpretations imply robustness or generalization of a given policy $\pi(a|s)$ to a modified reward function in this particular sense.   
% %Notice that 
% where the right hand side corresponds to the full objective function, including regularization, whereas the left hand side is only the expected reward.
%  %the regularized objective $\mathcal{R}_{\Omega, \beta}(r\tick) \geq \mathcal{R}_{\Omega, \beta}(r\tick)$
% The constraints in \myprop{feasible} characterize the robust set of modified rewards to which a given policy can generalize, as visualized in \cref{fig:feasible_set_main}.   Since these constraints integrate over the action space, the rewards for all actions in a particular state must be perturbed together.   
% % As we see in \cref{fig:perturb_opt} and \ref{fig:pyco}, this often corresponds to 
% % Due to these constraints on the adversarym we see in \cref{fig:perturb_opt} and \ref{fig:pyco} that 
% % \TG{Maybe we can comment here directly that this typically corresponds to reward-decreases for some actions but (adversarial!) reward increases for other actions of the same state.}

% By running a fixed policy in an environment with higher rewards, we naturally expect the objective function to increase.   However, for useful zero-shot generalization, we might hope that a policy will still perform well when the reward function decreases in at least some states.   We observe in \cref{fig:perturb_opt} and \ref{fig:pyco} that the adversary typically chooses reward decreases in some actions and increases in others, and proceed to further investigate this property in the next subsection.
% % However, we next discuss how
% In the next subsection, we discuss how 
% these qualitative properties can be sensitive to the form of the regularization function $\omegamu$.
% in \cref{eq:robust_def}.

% \section{Divergence vs. Entropy}\label{sec:entropy_vs_div}
\headerv
\section{Comparison with Entropy Regularization}\label{sec:entropy_vs_div}
% \subsection{Comparison with Entropy Regularization }\label{sec:entropy_vs_div}
\vspace*{\header}
% \JG{This whole section is absolutely amazing. Thanks!} 
As argued in \mysec{optimal_perturb}, the worst-case reward perturbations preserve the value of the regularized objective function.  Thus, we should expect our robustness conclusions to depend on the exact form of the regularizer.

When regularizing with the Tsallis or Shannon ($\alpha = 1$) entropy, the worst-case reward perturbations become %perturbed reward is %reward
\small
\begin{align}
    % \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \pi(a|s) \,. \label{eq:ptwise_perturb_ent}
    \hspace*{-.2cm} \propt(a,s) = \frac{1}{\beta} \log_{\alpha} \pi(a|s) + \frac{1}{\beta} \frac{1}{\alpha} \big(1 - \sum 
    % \limits
    _{a \in \mathcal{A}} \pi(a|s)^{\alpha} \big) \,. \label{eq:ptwise_perturb_ent}
\end{align}
\normalsize
% \RB{Change with new $\propt$}
%For entropy regularization,
In \myapp{entropy_nonnegative}, we show that these perturbations yield a pointwise non-negative contribution to the objective $r(a,s) - \propt(a,s)$, with $-\propt(a,s) \geq 0$ when $\pi(a|s) \leq 1$, for $0 < \alpha \leq 1$.   
% \RB{Why does Lee result hold for any $\alpha$?}
%  ONLY} 
% In the following, 
We argue that this property leads to several unsatisfying conclusions in previous work \citep{lee2019tsallis, eysenbach2021maximum}, which are resolved by using the \textsc{kl} and $\alpha$-divergence for analysis instead of the corresponding entropic quantities.\footnote{Entropy regularization corresponds to divergence regularization with the uniform reference distribution $\pi_0(a|s)$.}

% We argue the pointwise non-negative contribution of these perturbations to the objective $r(a,s) - \propt(a,s)$, with $-\propt(a,s) \geq 0$ for $\pi(a|s) \leq 1$, leads to several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}.   As we discuss in the following, this is resolved by using the \textsc{kl} and $\alpha$-divergence instead of the corresponding entropic quantities for the analysis. \footnote{Entropy regularization corresponds to the divergence to the uniform reference distribution $\pi_0(a|s)$ over actions.}
% In particular, entropy regularization should be considered as a divergence to the uniform reference distribution $\pi_0(a|s)$ over actions.
%Our use of the \textsc{kl} and} $\alpha$-divergences, instead of the corresponding entropic quantities, resolves several unsatisfying conclusions from previous work \citep{lee2019tsallis, eysenbach2021maximum}.   

First, this means that an entropy-regularized policy appears to only be `robust' to \textit{increases} in the reward function.   However, for useful generalization, we might hope that a policy will still perform well when the reward function decreases in at least some state-action pairs. 
 Including the reference distribution $\pi_0$ via divergence regularization resolves this issue,
%  changes this property, 
 and we observe in \cref{fig:feasible_set_main}-\ref{fig:pyco} that the adversary typically chooses reward decreases in some actions and increases in others.  For example, for the \textsc{kl} divergence, $\propt(a,s) = \frac{1}{\beta}\log \frac{\pi(a|s)}{\pi_0(a|s)}$ implies robustness to reward decreases when $\pi(a|s) > \pi_0(a|s)$.
 
%  so that the worst-case perturbation $\propt(a,s) = \frac{1}{\beta}\log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}$ %\frac{\pi(a|s)}{ \pi_0(a|s)}$ % yields robustness to reward \textit{decreases} when $\pi(a|s) > \pi_0(a|s)$ and reward increases otherwise.  
% Indeed, using divergence regularization, we observe in \cref{fig:perturb_opt} and \ref{fig:pyco} that the adversary typically chooses reward decreases in some actions and increases in others.  
% , and proceed to further investigate this property in the next subsection.
% For useful zero-shot generalization


% Including the reference distribution as in \myprop{feasible} changes this property, so that the worst-case perturbation $\propt(a,s) = \frac{1}{\beta}\log_{\alpha} \frac{\pi(a|s)}{\pi_0(a|s)}$ %\frac{\pi(a|s)}{ \pi_0(a|s)}$ % yields robustness to reward \textit{decreases} when $\pi(a|s) > \pi_0(a|s)$ and reward increases otherwise.  
% \RB{Include that we would like to be robust to decreases for useful generalization}

Similarly, \citet{lee2019tsallis} note that \textcolor{red}{, for any $\alpha$,}%$\frac{1}{\beta}\Omega^{*}_{\pi_0}(\discussiondual) = \max_{\pi(a|s)} \langle \pi(a|s), \discussiondual(a,s) \rangle + \frac{1}{\beta} H_{\alpha}(\pi) \geq \discussiondual(a_{\max}, s) $
\small
\begin{align*}
    \frac{1}{\beta}\Omega^{*(H_{\alpha})}_{\pi_0,\beta,\pi}(\discussiondual) = %\max_{\pi(a|s)}
    \max \limits_{\pi \in \Delta^{|\mathcal{A}|}} \langle \pi, \discussiondual \rangle + \frac{1}{\beta} H_{\alpha}(\pi) \geq \discussiondual(a_{\max}, s) 
    % \left(-\frac{1}{\beta} H_{\alpha}(\pi)\right)
\end{align*}
\normalsize
\normalsize
where $a_{\max} = \argmax_a \discussiondual(a,s)$ and Tsallis entropy $H_{\alpha}(\pi)$ equals Shannon entropy for $\alpha = 1$. 
% \RB{Soft Value, $\pi$ optimization}
% \textcolor{red}{Due to the pointwise non-negativity of $-\log_{\alpha}\pi(a|s)$ in the (Tsallis) entropy,  this soft value aggregation 
% % with the negative Tsallis entropy as a regularizer,  
% yields a result that is \textit{larger} than any particular $Q$-value. }
\textcolor{red}{This soft value aggregation yields a result that is \textit{larger} than any particular $Q$-value.}
% Due to the pointwise non-negativity of the 
%so that soft value aggregation yields a value which is \textit{larger} than any particular reward. 
% \begin{align}
%     \max_{\pi(a|s)} \langle \pi(a|s), \discussiondual(a,s) \rangle + \beta H_q(\pi) \geq \max_a \discussiondual(a,s)
% \end{align}
% where $H_q$ is the Tsallis entropy.
By contrast, for the $\alpha$-divergence, we show in \myapp{qmax} that
% \footnotesize
% \begin{align*}
%   \hspace*{-.1cm} \discussiondual(a_{\max},s) + \frac{1}{\beta}\frac{1}{\alpha} \log_{\alpha} \pi(a_{\max}| s) \leq \alphaconjn(\discussiondual) \leq  \discussiondual(a_{\max},s)
% \end{align*}
\begin{equation}
\resizebox{\columnwidth}{!}{ $\discussiondual(a_{\max},s) + \frac{1}{\beta}\frac{1}{\alpha} \log_{\alpha} \pi(a_{\max}| s) \leq \alphaconjn(\discussiondual) \leq  \discussiondual(a_{\max},s) $ 
  } \nonumber
\end{equation}
\normalsize
This provides a more natural interpretation of $V_*(s) =  \alphaconjn(Q)$ as a soft maximum function, with $ \mathbb{E}_{\pi_0}[\discussiondual(a_{\max},s)] \leq V_*(s) \leq \discussiondual(a_{\max},s)$, as in \myapp{soft_value}.
% \cref{fig:perturb_opt}.

Finally, entropy regularization also affects interpretations of the feasible set.  %For entropy regularization,
\citet{eysenbach2021maximum} consider the same constraint as in \cref{eq:kl_feasible}, but without the reference distribution
\begin{align}
    \sum \limits_{a} \expof{\beta \cdot \pr(a,s)} \leq 1  \, \, \, \forall s \in \mathcal{S} \, . \label{eq:ent_constraint}
\end{align}
This constraint suggests that the original reward function ($\pr = 0$) is not feasible for the adversary.  
% , unless the policy is deterministic
More surprisingly, \citet{eysenbach2021maximum} App. A5 argues that \textit{increasing} regularization strength (with lower $\beta$) may lead to \textit{less} robust policies based on the constraint in \cref{eq:ent_constraint}.    In \myapp{eysenbach}, we discuss how including $\pi_0(a|s)$ in the constraint via divergence regularization avoids this conclusion.   As expected, 
we observe in 
\cref{fig:feasible_set_main} that increasing regularization strength leads to more robust policies.


% \subsection{Adversarial Modified Rewards}\label{sec:husain}
% \vspace*{\header}
% The adversarial interpretation in the previous sections may also be written directly using the modified reward $\mr(a,s) = r(a,s) - \pr(a,s)$, which has been studied in a more general setting by \citet{husain2021regularized}.

% \citet{husain2021regularized} consider maximizing an arbitrary concave objective $\concaveopt$, and proceed to derive its convex conjugate $(-\concaveopt)^*$.    Translated to our setting and notation,
% this involves the conjugate expansion of the regularized objective $(-\obj_{\Omega, \beta}(r))^*$ instead of the conjugate of the regularizer only, $ (\omegamu)^*$.  
% With detailed derivations in \myapp{husain_conjugate}, this leads to the Lagrangian
% \begin{align}
%     \hspace*{-.2cm} & \quad \max \limits_{\mu(a,s)} \min \limits_{V(s)} \min \limits_{\textcolor{\highlight}{\mr(a,s)}} \, \label{eq:husain_form} \\
%     & \big \langle {\mu(s)\pi(a|s)}, {\textcolor{\highlight}{\mr(a,s)} +\gamma \transitionv - V(s) } \brangle  \nonumber  \\
%     & \quad+ \alphaconjn \big( r(a,s) - \textcolor{\highlight}{\mr(a,s)} \big) + (1-\gamma) \blangle \nu_0(s), V(s) \brangle \, ,  \nonumber
% \end{align}
% which matches \cref{eq:pedro_form} up to simple reparameterization of $\mr(a,s) = r(a,s) - \pr(a,s)$.

% Differentiating \cref{eq:husain_form} with respect to $\pi(a|s)$ and solving for the optimal modified rewards yields the result of \citet{husain2021regularized} that
% \begin{align}
%   \mropt(a,s) = V(s) - \gamma \transitionv  %\quad \forall (a,s) \in (\mathcal{A}, \mathcal{S})
% \end{align}
% Adding the environment reward, we can use the optimal reward perturbations $\propt(a,s) = r(a,s) - \mropt(a,s)$ to rewrite this expression
% \begin{align}
% \propt(a,s) &=  r(a,s) + \gamma \transitionv -  V(s) \label{eq:modified_reward_opt}
% \end{align}
% which matches our advantage function interpretation in 
% % \mysec{advantage} 
% \myprop{advantage}.


\input{sections/pyco_fig}

% \subsection{Connection with Path Consistency}\label{sec:path}
% \vspace*{\header}
% For the \textsc{kl} divergence regularization, \citet{nachum2017bridging} use the \textsc{kkt} conditions to show that the optimal policy satisfies \textit{path consistency} equations, which follow directly from the adversarial rewards in \cref{eq:modified_reward_opt} using \myprop{perturbations}.   In particular,
% \begin{align}
%     r(a,s) - \underbrace{\frac{1}{\beta} \log \frac{\pi(a|s)}{\pi_0(a|s)}}_{\propt(a,s)} = V(s) - \gamma \transitionv 
%     %\, \, \forall s \in \mathcal{S}, a \in \mathcal{A}
% \end{align}
% for all $s \in \mathcal{S}, a \in \mathcal{A}$.
% \citet{chow2018path} derive a path consistency equation for the Tsallis entropy with $\alpha =2$ which, generalized to the arbitrary $\alpha$-divergences and using our notation, becomes
% \begin{align}
% r(a,s) &- \underbrace{\frac{1}{\beta}\log_{\alpha}\frac{\pi(a|s)}{\pi_0(a|s)} - \frac{1}{\beta}(1-\alpha)D_{\alpha}[\pi_0:\pi]}_{\propt(a,s)} \\
% &= V(s) - \gamma \transitionv  + \Lambda(s) \label{eq:path1}
% \end{align}
% where $\Lambda(s) = \normalizerexp - V(s)$.   Using \eqref{eq:psidentity}, we can see that this Lagrange multiplier is equal to $\normalizerexp - V(s)= - \frac{1}{\beta}(1-\alpha)D_{\alpha}[\pi_0:\pi]$, so that we finally obtain
% % is a Lagrange multiplier which can be seen as accounting for the fact that $\normalizerexp \neq V(s)$ for $\alpha \neq 1$.
% % Finally, we are left with
% \begin{align}
%     r(a,s) + \gamma \transitionv - \propt(a,s) = \normalizeralpha   \label{eq:path}
% \end{align}
% \RB{Will change to reflect $\pr(a,s) = Q(a,s) - V(s)$}
% which matches our condition $\pr(a,s) = Q(a,s) - \normalizeralpha$. 
% With detailed derivations in \cref{app:path_consistency}, we show that the optimal $\alpha$-divergence regularized policy satisfies the path consistency condition in \cref{eq:path1}, which generalizes the result of \citet{chow2018path} from $\alpha=2$ to general $\alpha$.


% \subsection{Indifference Condition}\label{sec:indifference}
% For the optimal policy $\opt(a|s)$ in a given \gls{MDP}, \citet{ortega2014adversarial} additionally state an \textit{indifference condition} across actions, which is a well-known property of Nash equilibria in game theory \citep{osborne1994course}.   
% In particular, the adversarial objective has the same value for each action $a \in \mathcal{A}$ in state  $s \in \mathcal{S}$ (see \myapp{indifference}).   
% We can see in \cref{fig:perturb_opt}(a) that the perturbed rewards for each action match the value function $V_*(s)$ in each state.     
% While it is possible to derive an adversarial interpretation for any $\pi(a|s)$ using \cref{eq:pedro_form}, we see in \cref{fig:perturb_opt}(b) that the indifference condition does not hold for suboptimal policies.  

% can be interpreted as the \textit{certainty equivalent} \citep{myerson2019probability, ortega2013thermodynamics}, %myerson2019probability,
% which aggregates over actions $a \in \mathcal{A}$ to measure the payoff of a two-player game where the agent begins in state $s \in \mathcal{S}$ and plays against an adversary defined by the regularizer $\Omega_{\pi}(\pi)$ and strength $\beta$ as in \myprop{perturbations} \citep{ortega2014adversarial}.

==> sections/related_work_table.tex <==

\begin{figure*}[t]
\vspace*{-.2cm}
% \begin{minipage}{\pagewidth}
% \begin{minipage}{.7\textwidth}
\begin{subfigure}{.7\textwidth}
\centering
% \begin{center*}{\textwidth}
% \begin{table*}[t]
% % {\textwidth}
% \centering
% \caption{Comparison of Contributions}\label{table:novelty}
% \vspace*{-.2cm}
\resizebox{\textwidth}{!}
{
\begin{tabular}{lcccc}
    &  \text{\footnotesize \citet{ortega2014adversarial}} & \text{\footnotesize \citet{eysenbach2021maximum}} &  \text{\footnotesize \citet{husain2021regularized}} & Ours \\ \toprule
    \bullets{Multi-Step Analysis} & \tcminus{\xmark} & \tcplus{\cmark} & \tcplus{\cmark} & \tcplus{\cmark} \\ 
%   \bullets{Experiments match Theory} 
% %   \footnote{Our Fig. 3 displays the worst-case reward perturbations, and Fig. 6 confirms the optimality of the policy using the indifference and path consistency conditions. By contrast, \citet{husain2021regularized} evaluate using perturbations which do not match the theory, namely choosing $r\tick(a,s)= r(a,s) + \delta$ with $\delta \sim \mathcal{N}(5,.1)$ for $r(a,s) \leq \epsilon$. Fig. 6 and 9 in \citet{eysenbach2021maximum} lack detail.}
%     % Fig. 6 and 9 in \citet{eysenbach2021maximum} are not discussed in detail.   Our theory would predict that the MaxEnt \textsc{rl} objective with standard rewards matches the 
%     % % It is not appropriate to use the worst-case reward perturbations of MaxEnt \textsc{rl} to train .
%      & \tcminus{single step only} & \tcminus{\xmark} & \tcminus{\xmark} & \tcplus{\cmark} \\
    \bullets{Worst-Case $\propt(a,s)$} & \tcminus{policy form} & \tcminus{policy form} & \tcminus{value form} & \tcplus{policy \& value forms} \\ 
  \bullets{Feasible Set} & \tcminus{\xmark} & \tcminus{
    \cmark \, \,  (see our App G)} & \tcminus{\xmark} & \tcplus{\cmark} \\ 
  \bullets{Divergence Used} & \tcminus{KL ($\alpha = 1$)} & \tcminus{\text{ Shannon entropy (see Sec  5.1)}} & \tcplus{any convex $\Omega$} & \tcplus{$\alpha$-Div.} \\ 
    \bullets{$\mu(a,s)$ or $\pi(a|s)$ Reg.?} & (= in single step) & $\pi(a|s)$ & \tcplus{Both} & \tcplus{Both} \\
    \bullets{Indifference} & \tcplus{\cmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}  \\ 
    \bullets{Path Consistency} & \tcminus{\xmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}  \\ 
    \bottomrule
\end{tabular}
}
% \vspace*{.2cm}
\caption{}\label{table:novelty}
\end{subfigure}
% \captionof{table}{Comparison of Contributions}\label{table:novelty}
% \end{minipage}%
% \begin{minipage}{.3\textwidth}
\begin{subfigure}{.3\textwidth}
\centering
\vspace*{-0.5cm}
\includegraphics[width=.68\textwidth]{figs/feasible/kl/beta1alpha1uniform_adj.pdf}
\vspace*{-1.2cm}
\caption{}\label{fig:derman}
\end{subfigure}
\vspace*{-.3cm}
\caption{(a) Comparison to related work. (b) Comparison to rectangular robust set of \citet{derman2021twice}.  }\label{fig:related}
% \captionof{figure}{\text{\small \citet{derman2021twice}}}\label{fig:derman}
% \end{minipage}
% \end{minipage}
% \end{center}
\end{figure*}


==> sections/related_work_table_no_derman.tex <==
\begin{figure*}[t]
\vspace*{-1cm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc}
    &  \text{ \citet{ortega2014adversarial}} & \text{\citet{eysenbach2021maximum}} &  \text{ \citet{husain2021regularized}} & Ours \\ \toprule
    \bullets{Multi-Step Analysis} & \tcminus{\xmark} & \tcplus{\cmark} & \tcplus{\cmark} & \tcplus{\cmark} \\ 
    \bullets{Worst-Case $\pr(a,s)$} & \tcminus{policy form} & \tcminus{policy form} & \tcminus{value form} & \tcplus{policy $\&$ value forms} \\ 
  \bullets{Robust Set} & \tcminus{\xmark} & 
    \tcplus{\cmark}  \tcminus{(see our \myapp{eysenbach})} & \tcminus{\xmark} & \tcplus{\cmark} \\ 
  \bullets{Divergence Used} & \tcminus{KL ($\alpha = 1$)} & \tcminus{\text{ Shannon entropy (see \mysec{entropy_vs_div})}} & \tcplus{any convex $\Omega$} & \tcplus{$\alpha$-Divergence} \\ 
    \bullets{$\mu(a,s)$ or $\pi(a|s)$ Reg.?} & 
     $\pi(a|s)$ & 
    % (= in single step) & 
    $\pi(a|s)$ & \tcplus{Both} & \tcplus{Both} \\
    \bullets{Indifference} & \tcplus{\cmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}  \\ 
    \bullets{Path Consistency} & \tcminus{\xmark} & \tcminus{\xmark}  & \tcminus{\xmark}  & \tcplus{\cmark}  \\ 
    \bottomrule
\end{tabular}%
}
\vspace*{-.3cm}
\captionof{table}{Comparison to related work. }\label{table:novelty}
\headerv
\end{figure*}
